MAML and ANIL Provably Learn Representations

Recent empirical evidence has driven conventional wisdom to believe that gradient-based meta-learning (GBML) methods perform well at few-shot learning because they learn an expressive data representation that is shared across tasks. However, the mechanics of GBML have remained largely mysterious from a theoretical perspective. In this paper, we prove that two well-known GBML methods, MAML and ANIL, as well as their first-order approximations, are capable of learning common representation among a set of given tasks. Specifically, in the well-known multi-task linear representation learning setting, they are able to recover the ground-truth representation at an exponentially fast rate. Moreover, our analysis illuminates that the driving force causing MAML and ANIL to recover the underlying representation is that they adapt the final layer of their model, which harnesses the underlying task diversity to improve the representation in all directions of interest. To the best of our knowledge, these are the first results to show that MAML and/or ANIL learn expressive representations and to rigorously explain why they do so.

==> Conclusion.tex <==
% \section{Conclusion}








==> Diversity_across_iters.tex <==
\section{Task Diversity Across Iterations}

The current analysis relies principally on having task diversity on each round  (i.e. well-conditioned heads post-inner loop on the same round). In order to satisfy this assumption, the task batch size must be at least as large as the dimension $k$ of the heads, i.e. the dimension of the ground-truth representation.
% , and perhaps much larger since some of the sampled tasks may be linearly dependent. This may be a strong assumption, since a common few-shot learning task is 20-way classification on Omniglot $(k=20)$ and the task batch size may be only $4$ or $8$, yet ANIL and MAML still perform well in this scenario. In the linear case, 
However, empirically ANIL and MAML still learn the representation even when only one task is sampled in each round, as long as the tasks sampled in some number of consecutive round are diverse.
% - in particular, the neighborhood size is exactly the same after correcting the sample sizes/task such that the same total number of samples are used.

Fix a constant number of rounds $C \geq 1$. Assume infinite outer loop samples for now. Let $B$ be the task batch size. We have 
\begin{align}
    \mathbf{B}_{t(C+1)} &= \mathbf{{B}}_{tC}  \prod_{s=1}^C \left(\mathbf{I}_k - \frac{\alpha}{B}\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right) \nonumber \\
    &\quad + \mathbf{{B}}_\ast  \left( \sum_{s=1}^C \frac{\beta}{B}\sum_{i=1}^B\mathbf{w}_{\ast,tC+s,i}\mathbf{w}_{tC+s,i}^\top \prod_{r=s+1}^{C-1} \left(\mathbf{I}_k -\frac{ \alpha}{B}\sum_{i=1}^B\mathbf{w}_{tC+s,i} \mathbf{w}_{tC+r,i}^\top \right) \right)
\end{align}

First we try to show that if the $\mathbf{w}_{tC+s,i}$'s are diverse, then $\left\|\prod_{s=1}^C \left(\mathbf{I}_k - \frac{\alpha}{B}\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right)\right\|_2 < 1- c$.  This implies that $\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{tC}\|_2$ is contracting.

Suppose $C=2$ and the $\mathbf{w}_{tC+s,i}$'s are the standard basis vectors, and $\sum_{s=1}^C\sum_{i=1}^B\mathbf{e}_{s,i} = \frac{2B}{k} \mathbf{I}_k$ (which means $2B$ is a multiple of $k$), and $\alpha=1$.
\begin{align}
    \left\|\prod_{s=1}^2 \left(\mathbf{I}_k - \frac{1}{B}\sum_{i=1}^B \mathbf{e}_{s,i} \mathbf{e}_{s,i}^\top \right) \right\|_2 &= \left\| \left(\mathbf{I}_k - \frac{1}{B}\sum_{i=1}^B \mathbf{e}_{1,i} \mathbf{e}_{1,i}^\top \right) \left(\mathbf{I}_k - \frac{1}{B}\sum_{j=1}^B \mathbf{e}_{2,j} \mathbf{e}_{2,j}^\top \right)\right\|_2 \nonumber \\
    &= \left\| \mathbf{I}_k - \frac{1}{B}\sum_{i=1}^B \mathbf{e}_{1,i} \mathbf{e}_{1,i}^\top  - \frac{1}{B}\sum_{j=1}^B \mathbf{e}_{2,j} \mathbf{e}_{2,j}^\top + \frac{1}{B^2}\sum_{i=1}^B \sum_{j=1}^B \mathbf{e}_{1,i} \mathbf{e}_{1,i}^\top \mathbf{e}_{2,j} \mathbf{e}_{2,j}^\top \right\|_2 \nonumber \\
    &= \left\|\left(1-\frac{2}{k}\right) \mathbf{I}_k  + \frac{1}{B^2}\sum_{i=1}^B \sum_{j=1}^B \mathbf{1}_{\{\mathbf{e}_{1,i} = \mathbf{e}_{2,j}\}}\mathbf{e}_{1,i} \mathbf{e}_{1,i}^\top \right\|_2 \nonumber \\
    &\leq 1-\frac{2}{k} + \left\|\frac{1}{B^2}\sum_{i=1}^B \sum_{j=1}^B \mathbf{1}_{\{\mathbf{e}_{1,i} = \mathbf{e}_{2,j}\}}\mathbf{e}_{1,i} \mathbf{e}_{1,i}^\top \right\|_2
\end{align}
Since there are exactly $\frac{2B}{k}$ tasks per direction, each $\mathbf{e}_{1,i}$ can have at most $\frac{2B}{k} - 1$ matches in the second batch. So 
\begin{align}
    \left\|\prod_{s=1}^2 \left(\mathbf{I}_k - \frac{1}{B}\sum_{i=1}^B \mathbf{e}_{s,i} \mathbf{e}_{s,i}^\top \right) \right\|_2 
    &\leq 1-\frac{2}{k} + \left\|\frac{1}{B^2}\sum_{i=1}^B \left(\frac{2B}{k} - 1\right) \right\|_2 \nonumber \\
    &= 1-\frac{2}{k} + \frac{2}{k} - \frac{1}{B} \nonumber \\
    &= 1 - \frac{1}{B}
\end{align}
We can show an alternative bound: note that the worst case scenario is that the tasks in each direction are split evenly among batches. The total number of matches in this case is: $\sum_{q=1}^k \frac{2B}{2k} \frac{2B}{2k} = \frac{B^2}{k}$ resulting in a bound of
\begin{align}
    \left\|\prod_{s=1}^2 \left(\mathbf{I}_k - \frac{1}{B}\sum_{i=1}^B \mathbf{e}_{s,i} \mathbf{e}_{s,i}^\top \right) \right\|_2 
    &\leq  1-\frac{2}{k} + \frac{1}{k} = 1 - \frac{1}{k}
\end{align}
thus
\begin{align}
    \left\|\prod_{s=1}^2 \left(\mathbf{I}_k - \frac{1}{B}\sum_{i=1}^B \mathbf{e}_{s,i} \mathbf{e}_{s,i}^\top \right) \right\|_2 
    &\leq   1 - \frac{1}{\min(B,k)}
\end{align}
which makes sense, even for $B=1$ (since we have assumed $2B$ is a multiple of $k$).

% Idea: first order terms sum to a well-conditioned matrix, and the higher-order terms must be small because they are the product of matrices with at least some number of orthogonal components (if the heads are evenly spread) so the product strictly loses energy, i.e. $\|\mathbf{AB} \| < \|\mathbf{A}\| \|\mathbf{B}\| - \epsilon$.

% WLOG we can assume tasks have covariance identity.

Now we try to show contraction of $\|\mathbf{I}_k-\alpha \mathbf{B}_{tC}^\top \mathbf{B}_{tC}\|_2$ using first-order approximation of $\prod_{s=1}^C \left(\mathbf{I}_k - \frac{\alpha}{B}\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right)$. Ignoring $O(\beta^2)$ terms yields
\begin{align}
    \mathbf{B}_{t(C+1)} &= \mathbf{{B}}_{tC}  \prod_{s=1}^C \left(\mathbf{I}_k - \frac{\beta}{B}\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right) \nonumber \\
    &\quad + \mathbf{{B}}_\ast  \left( \sum_{s=1}^C \frac{\beta}{B}\sum_{i=1}^B\mathbf{w}_{\ast,tC+s,i}\mathbf{w}_{tC+s,i}^\top \prod_{r=s+1}^{C-1} \left(\mathbf{I}_k -\frac{ \beta}{B}\sum_{i=1}^B\mathbf{w}_{tC+s,i} \mathbf{w}_{tC+r,i}^\top \right) \right) \nonumber \\
    &\approx \mathbf{{B}}_{tC}   \left(\mathbf{I}_k - \frac{\beta}{B}\sum_{s=1}^C\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right) \nonumber \\
    &\quad + \mathbf{{B}}_\ast  \left( \frac{\beta}{B}\sum_{s=1}^C \sum_{i=1}^B\mathbf{w}_{\ast,tC+s,i}\mathbf{w}_{tC+s,i}^\top  \left(\mathbf{I}_k -\frac{ \alpha}{B}\sum_{r=s+1}^C\sum_{i=1}^B\mathbf{w}_{tC+r,i} \mathbf{w}_{tC+r,i}^\top \right) \right) \nonumber \\
    &=  \mathbf{{B}}_{tC} - \frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC}  \mathbf{w}_{tC+s,i} -  \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)\mathbf{w}_{tC+s,i}^\top   \nonumber \\
    &\quad - \frac{ \beta^2}{B^2} \mathbf{{B}}_\ast  \left( \sum_{s=1}^C\sum_{i'=1}^B\sum_{r=s+1}^C\sum_{i=1}^B\mathbf{w}_{tC+s,i'} \mathbf{w}_{tC+s,i'}^\top \mathbf{w}_{tC+r,i} \mathbf{w}_{tC+r,i}^\top  \right) \nonumber \\
    &\approx \mathbf{{B}}_{tC} - \frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC}  \mathbf{w}_{tC+s,i} -  \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)\mathbf{w}_{tC+s,i}^\top \nonumber \\
    &= \mathbf{{B}}_{tC} - \frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC} (\mathbf{I}_k - \alpha \mathbf{B}_{tC+s}^\top  \mathbf{B}_{tC+s}) \mathbf{w}_{tC+s} +\alpha \mathbf{{B}}_{tC}\mathbf{{B}}_{tC+s}^\top \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}-  \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)\mathbf{w}_{tC+s,i}^\top \label{labl} \\
    &= \mathbf{{B}}_{tC} - (\mathbf{I}_k - \alpha \mathbf{B}_{tC}^\top  \mathbf{B}_{tC}) \frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC} \mathbf{w}_{tC+s} -  \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)\mathbf{w}_{tC+s,i}^\top \nonumber \\
    &\quad + \frac{\beta\alpha}{B}\mathbf{B}_{tC}\sum_{i=1}^C\sum_{i=1}^B ((\mathbf{B}_{tC+s}^\top  \mathbf{B}_{tC+s} - \mathbf{B}_{tC}^\top  \mathbf{B}_{tC})\mathbf{w}_{tC+s} -  (\mathbf{B}_{tC+s}^\top- \mathbf{B}_{tC}^\top  )\mathbf{B}_{\ast}\mathbf{w}_{\ast,tC+s,i})\mathbf{w}_{tC+s,i}^\top \nonumber \\
    &= \mathbf{{B}}_{tC} - (\mathbf{I}_d - \alpha \mathbf{B}_{tC} \mathbf{B}_{tC}^\top ) \frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC} \mathbf{w}_{tC+s} -  \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)(\mathbf{w}_{tC+s}^\top(\mathbf{I}_k -\alpha \mathbf{B}_{tC+s}^\top \mathbf{B}_{tC+s}) + 
    \alpha\mathbf{w}_{\ast,tC+s,i}^\top \mathbf{B}_{\ast}^\top \mathbf{B}_{tC+s})\nonumber \\
    &\quad + \frac{\beta\alpha}{B}\mathbf{B}_{tC}\sum_{i=1}^C\sum_{i=1}^B ((\mathbf{B}_{tC+s}^\top  \mathbf{B}_{tC+s} - \mathbf{B}_{tC}^\top  \mathbf{B}_{tC})\mathbf{w}_{tC+s} -  (\mathbf{B}_{tC+s}^\top- \mathbf{B}_{tC}^\top  )\mathbf{B}_{\ast}\mathbf{w}_{\ast,tC+s,i})\mathbf{w}_{tC+s,i}^\top \nonumber
\end{align}
Now multiply the gradient terms by $\mathbf{B}_{tC}$ to obtain (look at \eqref{labl})
\begin{align}
    &\mathbf{B}_{tC}^\top \mathbf{G}_{tC+s}\nonumber \\
    &= \mathbf{B}_{tC}^\top \frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC} (\mathbf{I}_k - \alpha \mathbf{B}_{tC+s}^\top  \mathbf{B}_{tC+s}) \mathbf{w}_{tC+s} +\alpha \mathbf{{B}}_{tC}\mathbf{{B}}_{tC+s}^\top \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}-  \mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)\mathbf{w}_{tC+s,i}^\top \nonumber \\
    &= (\mathbf{I}_k - \alpha \mathbf{B}_{tC}^\top \mathbf{B}_{tC})\frac{\beta}{B}   \sum_{s=1}^C\sum_{i=1}^B\left( \mathbf{{B}}_{tC+s}^\top\mathbf{{B}}_{tC+s} \mathbf{w}_{tC+s} -  \mathbf{{B}}_{tC+s}^\top\mathbf{{B}}_\ast\mathbf{w}_{\ast,tC+s,i}\right)(\mathbf{w}_{tC+s}^\top(\mathbf{I}_k -\alpha \mathbf{B}_{tC+s}^\top \mathbf{B}_{tC+s}) + 
    \alpha\mathbf{w}_{\ast,tC+s,i}^\top \mathbf{B}_{\ast}^\top \mathbf{B}_{tC+s}) \nonumber \\
    &\quad -  \frac{\beta}{B}\sum_{s=1}^C\sum_{i=1}^B ((\mathbf{B}_{tC+s}^\top  \mathbf{B}_{tC+s} - \mathbf{B}_{tC}^\top  \mathbf{B}_{tC})\mathbf{w}_{tC+s} -  (\mathbf{B}_{tC+s}^\top- \mathbf{B}_{tC}^\top  )\mathbf{B}_{\ast}\mathbf{w}_{\ast,tC+s,i})\mathbf{w}_{tC+s,i}^\top \nonumber \\
\end{align}
The last term is the most problematic, but we can say that $\mathbf{B}_{tC+s}^\top- \mathbf{B}_{tC}^\top  $ is again small if the second-order terms in the step sizes are small.

However, the problem with this analysis is that the ignored $O(\beta^2)$ terms will eventually dominate the $\beta^2\alpha^2 \dist^2$ term, and these terms are not going to zero, so according to the analysis, $\|\mathbf{I}_k-\alpha \mathbf{B}_{tC}^\top \mathbf{B}_{tC}\|_2$ is not going to zero. But in reality, it is going to zero.
% Thus we need to use a different technique to bound $\|\mathbf{w}_t\|$.
Also, the first-order approximation loses accuracy with larger $C$, as seen below.


% first need universal lemma showing closeness of first-order approximation

% also figure out why there is no 1/C and if this is a problem

% for maml this will get extremely messy... let's first solidify the writing of the second-order gradient



\begin{lemma}
\begin{align}
    \left\|\prod_{s=1}^C \left(\mathbf{I}_k - \frac{\beta}{B}\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right) \right\|_2 &\leq \left\|  \right\|_2
\end{align}
\end{lemma}
\begin{proof}
First the simplest case:
\begin{align}
    \prod_{s=1}^C \left(1 - {\beta} x_s^2 \right) &= 1 - {\beta}\sum_{s=1}^C x_s^2 + \beta^2 \sum_{s=1}^C \sum_{s'=1}^C x_s^2 x_{s'}^2 - \beta^3 \sum_{s=1}^C \sum_{s'=1}^C\sum_{s''=1}^C x_s^2 x_{s'}^2 x_{s''}^2 +  \nonumber \\
    &\leq 1 - {\beta}\sum_{s=1}^C x_s^2 + \beta^2 \sum_{s=1}^C \sum_{s'=1}^C x_s^2 x_{s'}^2 - \beta^3 C^3 - 3 \beta^3 C^2 - 15 \beta^3 C + ...\nonumber 
\end{align}
so larger $C$ causes more error.
\end{proof}
In practice, $\left\|\prod_{s=1}^C \left(\mathbf{I}_k - \frac{\beta}{B}\sum_{i=1}^B \mathbf{w}_{tC+s,i} \mathbf{w}_{tC+s,i}^\top \right) \right\|_2$ becomes exponentially smaller with larger $C$, suggesting that the first-order approximation is not capturing reality.

Suppose $B=1$. To show $\left\|\prod_{s=1}^C \left(\mathbf{I}_k - \beta\mathbf{w}_{tC+s} \mathbf{w}_{tC+s}^\top \right) \right\|_2 \leq O(e^{-C})$, we take the following approach:
\begin{itemize}
    \item Partition $[C]$ into consecutive subsets. Each subset should be of size $R =\Omega(k\log k)$. Let $\mathbf{S}_{t,l}\coloneqq \prod_{s=1}^R (\mathbf{I}_k -{\beta}\mathbf{w}_{tC+Rl+ s} \mathbf{w}_{tC+Rl+s}^\top)$ Assuming the $ \mathbf{w}_{tC+s}$'s are independent, then we can use anti-concentration property to show that for each subset, for any fixed vector $\mathbf{u}\in \mathbb{R}^k: \|\mathbf{u}\|_2=1$, there exists some $s\in [R]$ such that $|\langle \mathbf{u}, \mathbf{w}_{tC+Rl+s}\rangle|>\delta$ with high probability. This means that $\|(\mathbf{I}_k -{\beta}\mathbf{w}_{tC+Rl+ s} \mathbf{w}_{tC+Rl+s}^\top)\mathbf{u}\|_2^2 \leq 1 -\delta^2(\beta...)$. Note that the $(\mathbf{I}_k -{\beta}\mathbf{w}_{tC+Rl+ s} \mathbf{w}_{tC+Rl+s}^\top)$ matrices are commutative and have spectral norm at most 1. Now construct an epsilon net over $\mathcal{S}^{k-1}$ and union bound to show  $\|(\mathbf{I}_k -{\beta}\mathbf{w}_{tC+Rl+ s} \mathbf{w}_{tC+Rl+s}^\top)\|_2^2 \leq 1 -\delta^2(\beta...)$. 
\end{itemize}

But, this analysis, and the analysis required to complete the full proof, still faces multiple challenges:
\begin{enumerate}
    \item It is not clear how to extend the above argument to $B>1$ (but this should not be hard, the following two issues are more serious).
    \item In reality the $\mathbf{w}_{tC+s}$'s are dependent. In fact, even in the best case scenario when $\mathbf{w}_{tC+s}= \alpha \mathbf{B}_{tC+s}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,tC+s}$, it is not clear that $\sum_{s=1}^C\mathbf{w}_{tC+s}\mathbf{w}_{tC+s}^\top =  \sum_{s=1}^C\mathbf{B}_{tC+s}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,tC+s}\mathbf{w}_{\ast,tC+s}^\top \mathbf{B}_\ast^\top\mathbf{B}_{tC+s}>c >0$ with high probability  since the $\mathbf{B}_{tC+s}$'s are dependent.
    \item In order to show that $\|\del_{tC}\|_2$ is contracting, we need to show contraction for matrix of the form $(\prod_{s=1}^q(\mathbf{I}-\mathbf{w}_{tC+s}\mathbf{w}_{tC+s}^\top +\mathbf{A}_{tC+s}))\del_{tC}(\prod_{s=q+1}^C(\mathbf{I}-\mathbf{w}_{tC+s}\mathbf{w}_{tC+s}^\top +\mathbf{A}_{tC+s}))$ for any $q\in[C]$. Not clear how to do this, both due to presence of $\mathbf{A}_{tC+s}$ and because of split product. 
\end{enumerate}


$\del_{t+1} = \del_{t}(\mathbf{I} - \beta \alpha^2 \mathbf{M}_t + \beta \alpha\mathbf{A}_t ) + \beta^2 \alpha^2 \dist_t^2$

\begin{align}
\implies \del_{t+2} &= \del_{t+1}(\mathbf{I} - \beta \alpha^2 \mathbf{M}_{t+1} + \beta \alpha\mathbf{A}_{t+1} ) + \beta^2 \alpha^2 \dist_{t+1}^2 \nonumber \\
&= \del_{t}(\mathbf{I} - \beta \alpha^2 \mathbf{M}_t + \beta \alpha\mathbf{A}_t )(\mathbf{I} - \beta \alpha^2 \mathbf{M}_{t+1} + \beta \alpha\mathbf{A}_{t+1} ) +\beta^2 \alpha^2 \dist_t^2(\mathbf{I} - \beta \alpha^2 \mathbf{M}_{t+1} + \beta \alpha\mathbf{A}_{t+1} )+ \beta^2 \alpha^2 \dist_{t+1}^2
\end{align}

% \textbf{Question:} Suppose that a set of vectors $\{\mathbf{v}_{i}\}_{i=1}^{CB}$ satisfies $\mu \leq \sigma_{\min}\left(\frac{1}{CB}\sum_{i=1}^{CB}\mathbf{v}_{i}\mathbf{v}_{i}^\top\right) \leq \sigma_{\max}\left(\frac{1}{CB}\sum_{i=1}^{CB}\mathbf{v}_{i}\mathbf{v}_{i}^\top\right) \leq L$. Then for any two disjoint subsets $\mathcal{S}_1$ and $\mathcal{S}_2$ of the vectors with equal cardinality, how can we bound
% \begin{align}
%     \left\| \frac{2}{CB}\sum_{i \in \mathcal{S}_1}\mathbf{v}_{i}\mathbf{v}_{i}^\top \frac{2}{CB}\sum_{j \in \mathcal{S}_2}\mathbf{v}_{j}\mathbf{v}_{j}^\top  \right\|_2 &= \left\| \frac{4}{C^2B^2}\sum_{i \in \mathcal{S}_1}\sum_{j \in \mathcal{S}_2} \langle\mathbf{v}_{i},  \mathbf{v}_{j}\rangle \mathbf{v}_{i}\mathbf{v}_{j}^\top  \right\|_2 ?
% \end{align}
% two approaches used in the simple case: 1) consider bound for each vector in the outer set, and 2) bound over the entire double sum. 1) is easier here, we have:
% \begin{align}
%   \left\| \frac{4}{C^2B^2}\sum_{i \in \mathcal{S}_1} \sum_{j \in \mathcal{S}_2} \langle\mathbf{v}_{i},  \mathbf{v}_{j}\rangle \mathbf{v}_{i}\mathbf{v}_{j}^\top  \right\|_2 &\leq \frac{4}{C^2B^2}\sum_{i \in \mathcal{S}_1}  \left\| \sum_{j \in \mathcal{S}_2} \langle\mathbf{v}_{i},  \mathbf{v}_{j}\rangle \mathbf{v}_{i}\mathbf{v}_{j}^\top  \right\|_2 \nonumber \\
%   &\leq \frac{4}{C^2B^2}\sum_{i \in \mathcal{S}_1} \|\mathbf{v}_i\|_2  \left\| \sum_{j \in \mathcal{S}_2} \langle\mathbf{v}_{i},  \mathbf{v}_{j}\rangle \mathbf{v}_{j} \right\|_2
% \end{align}
% if we can't show anything here, may need to consider isotropic task distrib






% make sure we have distinguished L_ast and L_max
% make sure we know L_ast and mu_ast are close to 1/k, not 1, whereas L_max may be close to 1


==> FO_anil.tex <==
\section{ANIL}
We are ultimately interested in whether iterative procedures to solve \eqref{maml_obj} and \eqref{anil_obj} find the column space of the ground-truth representation. We start by considering the simplest case, the first-order version of ANIL, which aims to solve \eqref{anil_obj}. We also make some simplifying assumptions:
\begin{itemize}
    \item all tasks are sampled on each round,
    \item the same data is used for both inner and outer loop updates, and
    \item the outer update for the head ignores the Hessian term (first-order update).
\end{itemize}
% The first two assumptions are made to simplify the notation and the last assumption is made to simplify the analysis.

Next we define some shorthand notations:
\begin{definition}[Shorthand notation]
For all $i \in [n]$ and each iteration $t >0$:
\begin{align}
   \mathbf{\bar{\Sigma}}_i \coloneqq \frac{1}{m} \sum_{j=1}^m \mathbf{x}_i^j (\mathbf{x}_i^j)^\top = \frac{1}{m} \mathbf{X}_i^\top \mathbf{X}_i,\quad \mathbf{P}_{t,i} \coloneqq \mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{\bar{\Sigma}}_i\mathbf{B}_t, \quad \mathbf{S}_{t,i}\coloneqq \mathbf{B}_t^\top \mathbf{\bar{\Sigma}}_i\mathbf{B}_\ast
\end{align}
\end{definition}

The ANIL update on the $t$-th iteration is:
\begin{enumerate}
    \item (Inner loop) For each $i \in [n]$, compute:
    \begin{align}
        \mathbf{w}_{t,i} &\gets \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} f_i(\mathbf{w}_t, \mathbf{B}_t) =  \mathbf{w}_{t} - \frac{\alpha}{m}  \sum_{j=1}^m \langle  \mathbf{x}_{i}^j,  \mathbf{B}_t \mathbf{w}_{t}-  \mathbf{B}_\ast \mathbf{w}_{i,\ast} \rangle \mathbf{B}_t^\top \mathbf{x}_{i}^j \\
        &= \mathbf{P}_{t,i} \mathbf{w}_t + \alpha \mathbf{S}_{t,i}\mathbf{w}_{\ast,i} \nonumber \\
        \mathbf{g}_{t,i} &\gets \nabla_{\mathbf{w}} f_i(\mathbf{w}_{t,i}, \mathbf{B}_t) = \frac{1}{m} \sum_{j=1}^m \langle  \mathbf{x}_{i}^j,  \mathbf{B}_t \mathbf{w}_{t,i} -  \mathbf{B}_\ast \mathbf{w}_{i,\ast} \rangle \mathbf{B}_t^\top \mathbf{x}_{i}^j
    \end{align}
    \item (Outer loop) Update with step size $\beta$:
    \begin{align}
        \mathbf{w}_{t+1} &\gets \mathbf{w}_{t} - \frac{\beta}{n} \sum_{i=1}^n \nabla_{\mathbf{w}} f_i(\mathbf{w}_{t,i}, \mathbf{B}_t) =  \mathbf{w}_{t} - \frac{\beta}{n} \sum_{i=1}^n \mathbf{g}_{t,i} \\
        \mathbf{B}_{t+1} &\gets \mathbf{B}_{t} - \frac{\beta}{n} \sum_{i=1}^n \nabla_{\mathbf{B}}f_i(\mathbf{w}_{t,i}, \mathbf{B}_t) \nonumber \\
        &= \mathbf{B}_{t} - \frac{\beta}{nm} \sum_{i=1}^n \sum_{j=1}^m \langle  \mathbf{x}_{i}^j,  \mathbf{B}_t \mathbf{w}_{t,i}-  \mathbf{B}_\ast \mathbf{w}_{i,\ast} \rangle \mathbf{x}_{i}^j \mathbf{w}_{t,i}^\top \\
        &= \mathbf{B}_{t} - \frac{\beta}{nm} \sum_{i=1}^n \sum_{j=1}^m  \mathbf{x}_{i}^j ( (\mathbf{x}_{i}^j)^\top \mathbf{B}_t \mathbf{w}_{t,i}) \mathbf{w}_{t,i}^\top - \mathbf{x}_{i}^j ( (\mathbf{x}_{i}^j)^\top \mathbf{B}_\ast \mathbf{w}_{i,\ast}) \mathbf{w}_{t,i}^\top\nonumber \\
        &= \frac{1}{nm} \sum_{i=1}^n \sum_{j=1}^m  \left(\mathbf{B}_{t} - \beta \mathbf{x}_{i}^j  (\mathbf{x}_{i}^j)^\top \mathbf{B}_t \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) + \frac{\beta}{nm} \sum_{i=1}^n \sum_{j=1}^m  \mathbf{x}_{i}^j  (\mathbf{x}_{i}^j)^\top \mathbf{B}_\ast \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top
    \end{align}
\end{enumerate}
Suppose that  the data is isotropic and $m$ is large enough such that $\frac{1}{m} \sum_{j=1}^m \mathbf{x}_{i}^j  (\mathbf{x}_{i}^j)^\top \approx \mathbf{I}_d$. Then we have
\begin{align}
    \mathbf{B}_{t+1} \approx \mathbf{B}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right)
\end{align}
Thus, for appropriately-chosen step-size $\beta$, the more well-spread the vectors $\mathbf{w}_{t,i}$ are (i.e., the closer that $\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$ is to the identity) the more that ANIL moves towards the ground-truth representation. This exposes the benefit of the inner loop update: since the inner loop update brings each $\mathbf{w}_{t,i}$ closer to $\mathbf{w}_{i,\ast}$, and we assume $\mathbf{W}_\ast$ to be well-conditioned, it is safe to assume that the vectors $\mathbf{w}_{t,i}$ are well-spread.

At the very least, $\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$ should be closer to the identity than the corresponding term for standard ERM, which tries to solve the objective \eqref{obj2}. 
The corresponding update procedure for standard ERM is:
\begin{enumerate}
    \item $\mathbf{w}_{t+1} \gets \mathbf{w}_{t} - \frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{w}} f_i(\mathbf{w}_{t}, \mathbf{B}_{t})  $
    \item $\mathbf{B}_{t+1} \gets \mathbf{B}_{t} - \frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} f_i(\mathbf{w}_{t}, \mathbf{B}_{t})  $
\end{enumerate}


In particular, in the limit as $m\rightarrow \infty$, the standard ERM update of the representation is:
\begin{align}
        \mathbf{B}_{t+1} \approx \mathbf{B}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t} \mathbf{w}_{t}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t}^\top\right) =  \mathbf{B}_{t} \left(  \mathbf{I}_d -  {\beta} \mathbf{w}_{t} \mathbf{w}_{t}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{i,\ast} \mathbf{w}_{t}^\top\right)
\end{align}
Since the matrix $\beta \mathbf{w}_{t} \mathbf{w}_{t}^\top$ is rank-1, we expect that $\left(  \mathbf{I}_d -  {\beta} \mathbf{w}_{t} \mathbf{w}_{t}^\top\right)$ preserves more of the energy in $\mathbf{B}_t$ than does the corresponding matrix for ANIL, $\left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)$. So the ERM update preserves relatively more energy from $\mathbf{B}_t$ compared to the ANIL update.

So, this observation suggests that making the inner loop update for the heads effectively increases the estimated task diversity and allows ANIL to find the ground-truth representation faster than ERM (if ERM finds it at all).
% Meanwhile, the effective estimated task diversity is trivial, because there is effectively only a single head when updating the representation. 

% Numerical simulations in this linear setting support this result, although the convergence to the ground truth representation is slow:

% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.45\columnwidth]{sim1.png}}
% \vspace{-0mm}
% % \caption{}
% \label{fig:new_clients2}
% \end{center}
% \vspace{-0mm}
% \end{figure}

% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.58\columnwidth]{spreads.png}}
% \vspace{-0mm}
% \caption{$\mathbf{C}_1$ is coefficient of $\mathbf{B}_t$, and $\mathbf{C}_2$ is coefficient of $\mathbf{B}_\ast$.}
% \label{fig:new_clients2}
% \end{center}
% \vspace{-0mm}
% \end{figure}


% \section{Open meta-learning questions:}
% \begin{enumerate}
%     \item  
% \end{enumerate}
% \newpage
Adding another linear layer, $\mathbf{A}$, to the head would mean that the relevant matrix would become $\frac{\beta}{n} \sum_{i=1}^n \mathbf{A}_{t,i}\mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top \mathbf{A}_{t,i}^\top$, which may help to bring this closer to the identity by reducing the dimension, but would not help for ERM, because the matrix would still be rank-1.

\subsection{Convergence Result}
Now we try to prove the convergence of ANIL to the ground-truth representation. We use the principle angle distance to measure the distance between representations. We use hats to denote orthogonal matrices.

\begin{definition}[Principle angle distance]
Let $ \mathbf{\hat{B}}_{\ast,\perp}$ denote the orthogonal matrix whose columns span the subspace perpendicular to $col(
\mathbf{B}_\ast)$. Let $\mathbf{\hat{B}}$ denote an orthogonalized version of some matrix $\mathbf{B}$. Then the principle angle distance between $\mathbf{B}$ and  $
\mathbf{B}_\ast$ is given by 
\begin{align}
    \dist(\mathbf{B}, \mathbf{B}_\ast) &\coloneqq \|\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{\hat{B}}\|_2.
\end{align}
\end{definition}

Let
$
E_0 \coloneqq 1- \dist^2(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)
$.

\begin{assumption}[Task diversity]
The ground-truth heads satisfy  $\sigma_{\min}(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top )\geq {\mu_\ast^2 }$.
\end{assumption}

\begin{assumption}[Task normalization]
For all $i \in [n]$, $\|\mathbf{w}_{\ast,i} \|_2 = 1$.
\end{assumption}

\begin{assumption}
The initial iterate for the head satisfies $\|\mathbf{w}_{0} \|_2 = 1$.
\end{assumption}

Note that Assumption 2 requires $n\geq k$. Assumptions 2 and 3 are standard in previous work \citep{du2020fewshot,tripuraneni2020provable}. Assumption 4 is made for simplicity and is not fundamental.

We start by considering the \textbf{population case} ($m_{in}=m_{out}= \infty$). In this setting,
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{B}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right)
\end{align}
We use hats to denote orthogonal matrices.
Assume for now that the columns of $\mathbf{B}_t$ are orthogonalized, i.e. $\mathbf{B}_t=\mathbf{\hat{B}}_t$ such that $\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t = \mathbf{I}_k$ (we should be able to later show that this assumption is WLOG). We also have that $\mathbf{B}_\ast$ is orthogonal, so we can also denote it by $ \mathbf{\hat{B}}_\ast$. 
Then
\begin{align}
    \mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{\hat{B}}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)
\end{align}
So
\begin{align}
   \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_{\ast} ) &= \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_{\ast} ) \left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2
\end{align}
where $\mathbf{\hat{B}}_{t+1 } \mathbf{R}_{t+1} = \mathbf{B}_{t+1}$ is the QR-decomposition of $\mathbf{B}_{t+1}$. 


We have, for sufficiently small $\beta$,
\begin{align}
\left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 &\leq 1 - \lambda_{\min}\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) \nonumber \\
&= 1 - \frac{\beta}{n} \lambda_{\min}\left( \sum_{i=1}^n \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{S}_{t,i} \mathbf{w}_{\ast,i}\mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_{\ast,i}^\top \mathbf{S}_{t,i}^\top  + \alpha^2 \mathbf{S}_{t,i} \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{S}_{t,i}^\top \right)
\end{align}
With full measurements and orthogonal $\mathbf{B}_t$, we have $\mathbf{P}_{t,i} = (1- \alpha)\mathbf{I}_k$ and $\mathbf{S}_{t,i} = \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast$ for all $i \in [n]$. Then
\begin{align}
    &\lambda_{\min}\left( \sum_{i=1}^n \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{S}_{t,i} \mathbf{w}_{\ast,i}\mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_{\ast,i}^\top \mathbf{S}_{t,i}^\top  + \alpha^2 \mathbf{S}_{t,i} \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{S}_{t,i}^\top \right) \nonumber \\
    &= \lambda_{\min}\left(n(1-\alpha)^2 \mathbf{w}_t \mathbf{w}_t^\top + \alpha(1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top  + \alpha(1-\alpha)  \mathbf{w}_t\sum_{i=1}^n \left(\mathbf{w}_{\ast,i}^\ast\right) \mathbf{\hat{B}}_\ast \mathbf{\hat{B}}_t^\top + \alpha^2 \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n\left(\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right)  \nonumber \\
    &\geq \lambda_{\min}\left( \alpha(1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top  + \alpha(1-\alpha)  \mathbf{w}_t\sum_{i=1}^n \left(\mathbf{w}_{\ast,i}^\ast\right)^\top \mathbf{\hat{B}}_\ast \mathbf{\hat{B}}_t^\top + \alpha^2 \mathbf{\hat{B}}_t \mathbf{\hat{B}}_\ast^\top \sum_{i=1}^n\left(\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right)  \label{ge1}\\
     &\geq \lambda_{\min}\left( \alpha(1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top  + \alpha(1-\alpha)  \mathbf{w}_t\sum_{i=1}^n \left(\mathbf{w}_{\ast,i}^\ast\right)^\top \mathbf{\hat{B}}_\ast \mathbf{\hat{B}}_t^\top\right) +\lambda_{\min}\left( \alpha^2 \mathbf{\hat{B}}_t \mathbf{\hat{B}}_\ast^\top \sum_{i=1}^n\left(\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) \\
     &\geq  -2\alpha (1- \alpha)  \left\| \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top   \right\|_2 + \alpha^2 \sigma_{\min}\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t \right)  \label{ge2} %\\
    % &\geq \alpha^2 \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\right)  \sigma_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top  \right) + 2 \alpha (1- \alpha) \sigma_{\min} \left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top  \right) \label{ge3} \\
    % &\geq \alpha^2\left( 1 - \text{dist}(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)\right)^2 \lambda_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \nonumber
\end{align}
where \eqref{ge1} follows because $n(1-\alpha)^2 \mathbf{w}_t \mathbf{w}_t^\top$ is PSD, and  \eqref{ge2} follows by Weyl's Inequality.
Note that
\begin{align}
    \left\| \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top   \right\|_2 &\leq  n \; %\text{dist}(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast)
\end{align}
since if $\|\mathbf{w}_0\|_2 = \|\mathbf{w}_{\ast,1}\|_2 = \dots =\|\mathbf{w}_{\ast,n}\|_2 = 1$, then we can easily show that $\|\mathbf{w}_t\|_2 \leq 1$ for all $t$ as long as $\beta \leq 1/(1-\alpha)$. Meanwhile,
\begin{align}
   \sigma_{\min}\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t \right) &\geq \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\right)  \sigma_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top  \right) \nonumber \\
   &\geq \left( 1 - \text{dist}^2(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)\right) \sigma_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \nonumber \\
   &\geq E_0 n\mu_\ast^2 
\end{align}
where the last inequality follows from the assumption of task diversity. Thus we have
\begin{align}
    \left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 &\leq 1  + 2\beta \alpha(1-\alpha)  -  \beta \alpha^2 E_0 \mu_\ast^2  \nonumber \\
     &\leq 1  + 2\beta \alpha(1-\alpha)  -  \beta \alpha^2 E_0 \mu_\ast^2   \label{contract}
\end{align}
We will set $\alpha =1$ to achieve contraction, but first 
we must show that $\|\mathbf{R}_{t+1}^{-1}\|_2$ is small, or equivalently, $\sigma_{\min}(\mathbf{R}_{t+1})$ is large. First, write
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top
\end{align}
Then
\begin{align}
    \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
    &= \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber \\
    &= \mathbf{I}_{k} - \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber
\end{align}
Note that for $\alpha = 1$, 
\begin{align}
    \mathbf{w}_{t,i} = \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}
\end{align}
so the cross terms are zero, i.e.
\begin{align}
    \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top = \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) = \mathbf{0}.
\end{align}
and we have, since the $O(\beta^2)$ term is PSD,
\begin{align}
    \lambda_{\min}\left(\mathbf{R}_{t+1}^\top \mathbf{R}_{t+1}\right) &\geq 1
\end{align}
{\color{blue}
Thus we have, using \eqref{contract} with $\alpha =1,$
\begin{align}
    \text{dist}\left(\mathbf{\hat{B}}_{t+1},\mathbf{\hat{B}}_\ast \right) 
     &\leq({1 -  \beta  E_0 \mu_\ast^2  })\text{dist}\left(\mathbf{\hat{B}}_{t},\mathbf{\hat{B}}_\ast \right) 
\end{align}
}
where $\beta$ can be chosen sufficiently small such that the contraction factor is less than 1.
\textcolor{blue}{Sewoong (old): If I understood correctly, $\mu_\ast^2 \leq 1/d $ and $E_0\leq 1$. So the RHS seems like contracting at a rate at best $\frac{1-\beta/d}{1-c\beta^2}$. Then it looks like we need $\beta\leq 1/d$. }

\textbf{Remark.} With $\alpha = 1$ in the population case, we solve for the optimal head corresponding to the current representation $\mathbf{B}_t$ with only one local update. However, the above result can be generalized to the case in which $\alpha \approx 1$, i.e. the inner loop update is not an exact minimization.

\begin{comment}
In the finite-sample case, we can show that 

\begin{align}
\frac{ \alpha \beta}{n}\sum_{i=1}^n \sigma_{\max}\left( \mathbf{\hat{B}}_t \left( \alpha \mathbf{\bar{\Sigma}}_i - \mathbf{I}_d \right)\mathbf{\hat{B}}_\ast\right)\sigma_{\max}\left( \mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}\right)
\end{align}
which we can upper bound close to zero with high probability given O(k) samples, and setting $\alpha=1$.
Say that this bound is $B$, then
% that the cross terms concentrate to zero, i.e.
% \begin{align}
%     \mathbb{E}(\frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top)  = \mathbf{0}.
% \end{align}
Thus
\begin{align}
    \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \frac{ 1 -  \kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t})
}{\sqrt{1-2B}} \;    \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
with high probability.
\end{comment}
% It remains to compute the high probability bound $B$ and the high probability bound on $\kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t})$.

% can we expand on this analysis to say something unique about MAML/ANIL even when the heads are not solved for exactly?  how about the overparameterized case? need trajectory-based analysis?

% simulations: test whether the outer loop for the heads matters. if it doesn't (i.e. first order or reptile works just as well) then this is consistent with the analysis.

% to do : 
% 1. think about analysis for gd (no min) case - sublinear possible? trajectory?
% 2. simulations - second order matters - how to use this
% 3. read du paper again





%so why is analysis not working
% in general case, with partial measurements, it is not fedrep because we do not solve the minimization exactly, which is why we cannot show convrgence


% Can we show sub-linear convergence?


% Setting $\alpha = 1$ yields contraction*! Note that setting $\alpha$ to be close to 1, but smaller than 1, will also yield contraction, as long as something like $\frac{\alpha}{1-\alpha} \geq \frac{2k }{E_0}$. The intuition is that the closer $\alpha$ is to 1, the closer we come to solving each inner loop minimization problem exactly, and we need to come close to solving it in order for ANIL to learn the representation.
% Can also consider the regime $\alpha \geq 1$, but the expression would be different.


% * as long as $\|\mathbf{R}_{t+1}^{-1}\|_2 \leq 1$, which requires that the B* term in Bt+1 is non-trivial

\begin{comment}
\textbf{Remarks.}
\begin{itemize}
\item At a high level, when we have infinite data for the outer loop, the problem reduces to showing $$\kappa\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) \approx 1$$.
    \item In the case in which we have infinite data for the inner loop update, $\alpha=1$ and $\mathbf{B}_t$ is orthogonal, then we solve the inner problem exactly in one step
    \item but not solving the inner problem exactly makes the analysis significantly more difficult. Importantly, unlike in the analysis of FedRep, the norm of the matrix $\mathbf{Q}_{t,i} \coloneqq \mathbf{B}_t \mathbf{w}_{t,i} - \mathbf{B}_\ast \mathbf{w}_{\ast,i} = (\mathbf{I}_k - \alpha \mathbf{B}_t \mathbf{B}_t^\top \mathbf{\bar{\Sigma}}_i)\mathbf{B}_t \mathbf{w}_{t} - \mathbf{B}_\ast \mathbf{w}_{\ast,i})$ is not proportional to the distance between $\mathbf{\hat{B}}_t$ and  $\mathbf{\hat{B}}_\ast$, so I do not think we can show linear convergence using the current method... and simulations suggest  sublinear convergence. {\em but is their sum proportional to the distance, with full rank heads?}
    \item why do we not have O(d) sample complexity in the finite-sample case??? we have O(k). where is the mistake?
    \item if we solve the inner problem exactly, we are essentially doing FedRep, not ANIL/MAML
    \item indeed, we are not really using much that is unique about ANIL/MAML here - we are not using the outer loop update for $w$ besides to show that the norm of $w_t$ is non-increasing, so $w_{t+1}$ can be computed in any way the does not increase the norm.
    \item how to incorporate second order update? it should make $\mathbf{B}_{t+1} \mathbf{w}_{t+1}$ more centered among the $\mathbf{B}_{\ast} \mathbf{w}_{\ast,i}$'s, since this means that $\mathbf{w}_{t+1,i}$ is closer to isometric. But it is difficult to show that $\mathbf{B}_{t+1} \mathbf{w}_{t+1}$ is more centered with the second-order update
\item idea: less data for the inner loop perhaps makes $\mathbf{w}_{t,i}$ more isometric (again, difficult to show). And assume infinite data for the outer loop.
\item comparison with Saunshi (A Sample Complexity Separation Between Convex and Nonconvex Meta-Learning): is exact parameterization interesting? if not, we need a new form of analysis
\item Du paper achieves result in overparameterized case with regularization - can we use any benign global geometry property to achieve the result? 
% They also take $k$ to infinity, which we would have to avoid for the optimization result 
\end{itemize}
% the smallest singular value of sum(wti wtT) should be large and smallest of C2 should be large...

% \textbf{Questions:}
% \begin{itemize}
%     \item What happens with partial measurements?
%     \begin{itemize}
%         \item problem: unlike in the analysis of FedRep, the norm of the matrix $\mathbf{Q}_{t,i} \coloneqq \mathbf{B}_t \mathbf{w}_{t,i} - \mathbf{B}_\ast \mathbf{w}_{\ast,i} = (\mathbf{I}_k - \alpha \mathbf{B}_t \mathbf{B}_t^\top \mathbf{\bar{\Sigma}}_i)(\mathbf{B}_t \mathbf{w}_{t} - \mathbf{B}_\ast \mathbf{w}_{\ast,i})$ is not proportional to the distance. This is a big problem...
%     \end{itemize}
% \end{itemize}


Assuming standard Gaussian data and orthogonal representation $\mathbf{B}_t \equiv \mathbf{\hat{B}}_t$:
\begin{align}
    \mathbb{E}[\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top] &= (1- \alpha^2) \mathbf{w}_t \mathbf{w}_t^\top - \alpha(1-\alpha) \mathbf{w}_t \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t - \alpha(1-\alpha)   \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_t^\top + \alpha^2 \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}  \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t\nonumber \\
    &\quad \quad + \frac{\alpha^2}{m}(\|\mathbf{\hat{B}}_t \mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \|_2^2 + 1)\mathbf{\hat{B}}_t^\top(\mathbf{\hat{B}}_t \mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})(\mathbf{\hat{B}}_t \mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})^\top \mathbf{\hat{B}}_t
\end{align}
\end{comment}



% to do:
% read implicit bias papers, see if we can extend to multitask
% read recent multitask papers
% the question remains: how to show that we reach a fixed point? 
% more broadly: how to show that a sequence non-monotonically converges
% opportunity to apply recent techniques? 
% to do:
% think abt what problem to solve for unsup
%    multitask or federated? federated presents new challenges, but maybe multi-task is more fundamental and unanswered
% clean this up
% clean up reviews


% areas:
% multi-task semi-supervised
% fed semi-supervised
% multi-task implicit bias
% multi-task rep learn


% We can show that $z_t$ is sub-exponential with parameter $\frac{1}{\sqrt{nm}}$
% \begin{align}
%     \mathbb{P}(z_t > \frac{1}{\mathbf{b}_\ast^\top \mathbf{b}_{t}} ) \leq (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2
% \end{align}

% study saunshi analysis. how to know there is unique fixed point of a linear dynamical system? do the iterates satisfy some invariants? can second-order update meaningfully help?


==> Finite_samples.tex <==

\section{Finite Samples}
% We start by abstracting 

% {\em Note: I removed the old Lemma 1 - Liam}

\begin{assumption}
The ground-truth heads satisfy the following two properties:
\begin{enumerate} \label{assump:gt}
    \item (Task normalization) For all $i\in [n]$, $\|\mathbf{w}_{\ast,i}\|_2 \leq L_{\max}$. 
    % Note that this immediately implies
    \item (Task diversity) $
     0 \leq \mu_\ast^2 \leq  \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \leq
     \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \leq L_\ast^2 
 $. 
% $\sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \leq .$
\end{enumerate}
\end{assumption}
Note that if the ground-truth heads are well-conditioned, then $\mu_{\ast}^2$ and $L_{\ast}^2$ will be close to $1/k$. Also, we always have $L_{\ast}^2\leq L_{\max}^2$.

\begin{assumption} \label{assump:wt}
The current iterate $\mathbf{w}_t$ satisfies $\|\mathbf{w}_t\|_2 \leq L_\max$.
\end{assumption}

\begin{assumption}
\label{assump:data}
For all $i,j$, the sample $\mathbf{x}_{i,j} \in \mathbb{R}^d$ is $\mathbf{I}_d$-sub-Gaussian, in the sense that $\mathbb{E}[\exp(\mathbf{v}^\top \mathbf{x}_{i,j})] \leq \exp \left(\frac{\|\mathbf{v}\|_2^2}{2}\right)$ for all $\mathbf{v}\in \mathbb{R}^d$.
\end{assumption}

\textbf{Notations}

\begin{itemize}
    \item $\mathbf{e}_i \coloneqq \mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$
    \item $\mathbf{E} \coloneqq \begin{bmatrix}\vdots \\
    \mathbf{e}_i^\top \\
    \vdots
    \end{bmatrix}$ 
    % \item $\mathbf{W}_{t,in} \coloneqq \begin{bmatrix}\vdots \\
    % \mathbf{w}_{t,i}^\top \\
    % \vdots
    % \end{bmatrix} = ((\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top )^\top$
    \item $m_{in}$: number of inner loop samples. $m_{out}$: number of outer loop samples.
    \item $\mathbf{\Sigma}_{i,in} \coloneqq \frac{1}{m_{in}}\sum_{j=1}^{m_{in}}\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top$, $\mathbf{\Sigma}_{i,out} \coloneqq \frac{1}{m_{out}}\sum_{j=1}^{m_{out}}\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top$
\end{itemize}

\subsection{Finite inner loop samples}

\begin{lemma} \label{lem:concen}
Let $\alpha=1$. Under assumptions \ref{assump:gt}, \ref{assump:wt}, and \ref{assump:data}, we have 
\begin{align}
   \frac{1}{\sqrt{n}} \| \mathbf{E} \|_F \leq O\left(L_{\max} \frac{\sqrt{k}+ \sqrt{\log(n)}}{\sqrt{m_{in}}}\right)
\end{align}
with probability at least $1 - 4 n^{-99}$.
\end{lemma}
\begin{proof}
For some $i$, we have
\begin{align}
    \mathbf{w}_{t,i} &= \mathbf{w}_t - \alpha \mathbf{\hat{B}}_t^\top \sum_{j=1}^{m_{in}}\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \mathbf{\hat{B}}_t \mathbf{{w}}_t  + \alpha \mathbf{\hat{B}}_t^\top \frac{1}{m_{in}}\sum_{j=1}^{m_{in}}\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \mathbf{\hat{B}}_\ast \mathbf{{w}}_{\ast,i} \nonumber \\
    &= (\mathbf{I}- \alpha\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i}.
\end{align}
Thus, for $\alpha=1$,
\begin{align}
    \| \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2 & = \|(\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t +  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2\nonumber \\
    &\leq \|(\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t\|_2 + \| \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2 \nonumber \\
    &\leq  \|\mathbf{I}_k- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2 \|  \mathbf{{w}}_t\|_2 + \| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2 \|{\mathbf{w}_{\ast,i}}\|_2  \nonumber \\
    &\leq  L_{\max}\|\mathbf{I}_k- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2  + L_{\max}\| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2\label{twoterms}
\end{align}
where we have used $\|{\mathbf{w}_{\ast,i}}\|_2 \leq L_{\max}$ and $\|{\mathbf{w}_{t}}\|_2 \leq L_{\max}$. 
% (assumed for simplicity, but we can likely show that we can normalize $\mathbf{w}_t$ at the end of each round WLOG). 
We first consider the term 
\begin{align}
    \|\mathbf{I}_k- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2  &=  \left\|\mathbf{I}_k-    \frac{1}{m_{in}}\sum_{j=1}^{m_{in}}\mathbf{\hat{B}}_t^\top\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top\mathbf{\hat{B}}_t\right\|_2
\end{align}
where $\mathbf{\hat{B}}_t^\top\mathbf{x}_{i,j}$ is sub-Gaussian with covariance $\mathbf{\hat{B}}_t^\top\mathbf{\hat{B}}_t = \mathbf{I}_k$. Thus, by equation 4.22 in Vershynin, we have
\begin{align}
    \|\mathbf{I}_k- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2 &\leq c  \max\left( \frac{\sqrt{k} + \lambda}{\sqrt{m_{in}}},  \frac{k + \lambda^2}{m_{in}}\right) \label{concen1}
\end{align}
for some absolute constant $c$,
with probability at least $ 1 - 2 e^{-\delta^2}$, for any $\lambda > 0$. The same bound holds for the second term in \eqref{twoterms}, so via a union bound we have 
\begin{align}
    \| \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2 &\leq c' L_{\max} \max\left( \frac{\sqrt{k} + \lambda}{\sqrt{m_{in}}},  \frac{k + \lambda^2}{m_{in}}\right)
\end{align}
with probability at least $ 1 - 4 e^{-\lambda^2}$, for any $\lambda>0$. Now choose $\lambda = 10 \sqrt{\log(n)}$ and union bound over all $i \in [n]$ to obtain
\begin{align}
    \frac{1}{n}\sum_{i=1}^n\| \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2^2 &\leq c'' L_{\max}^2  \left(\max\left( \frac{\sqrt{k} + 10 \sqrt{\log(n)}}{\sqrt{m_{in}}},  \frac{k + 100\log(n)}{m_{in}}\right)\right)^2 \nonumber \\
    \implies \frac{1}{\sqrt{n}}\|\mathbf{E}\|_F \leq \sqrt{\frac{1}{n}\sum_{i=1}^n\| \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2^2} &\leq c' L_{\max} \max\left( \frac{\sqrt{k} + 10 \sqrt{\log(n)}}{\sqrt{m_{in}}},  \frac{k + 100\log(n)}{m_{in}}\right) %=: L_\ast \epsilon
\end{align}
with probability at least $1 - 4n^{-99}$. 
\end{proof}



\begin{lemma} \label{lem:cond}
Let $\beta = O(1/L_{\ast}^2)$.
Define $\mu^2 \coloneqq \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$, $L^2 \coloneqq \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$, and $\delta_{in} \coloneqq c\frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}}$ for some absolute constant $c$. 
Under Assumptions \ref{assump:gt}, \ref{assump:wt} and \ref{assump:data}, we have 
\begin{align}
    L^2 &\leq L_{\max}^2 (2\delta_{in}+1)^2  \nonumber \\
    \text{and} \quad \mu^2 &\geq \mu_\ast^2 E_0 - 4 L_{\max}^2 (\delta_{in} + \delta_{in}^2) 
 \end{align}
 with probability at least $1 - 4 n^{-99}$.
\end{lemma}

\begin{proof}
Note that
\begin{align}
   \left\| \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right\|_2 &= %\left\| \frac{1}{n}  \mathbf{W}_{t,in}^\top \mathbf{W}_{t,in}\right\|_2 \nonumber \\&= %\frac{1}{n}\left\|\mathbf{W}_{t,in}\right\|_2^2 \nonumber \\&= 
   \frac{1}{n}\Big\|\sum_{i=1}^n (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)  + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top  \nonumber \\
   &\quad + (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top + 
   \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}
   \mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) 
   \Big\|_2^2 \nonumber \\
   &\leq \frac{1}{n}\Big\|\sum_{i=1}^n (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) \Big\|_2  +\frac{1}{n}\Big\|\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top \Big\|_2 \nonumber \\
   &\quad +\frac{1}{n}\Big\| \sum_{i=1}^n(\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top + 
   \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}
   \mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) 
   \Big\|_2^2  \label{tri0} \\
   &\leq L_{\max}^2 \max_{i\in [n]}\|\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2^2 + L_{\max}^2 \max_{i\in [n]}\| \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\|_2^2  \nonumber \\
   &\quad  + 2 L_{\max}^2 \max_{i\in [n]}\|\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2 \| \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\|_2  \label{tri1} \\
   &\leq L_{\max}^2 \delta_{in}^2 +  L_{\max}^2(1+\delta_{in})^2 +  2 L_{\max}^2\delta_{in}(1+\delta_{in}) \label{versh1} \\
   &= L_{\max}^2(2\delta_{in} + 1)^2 
%   \frac{2}{n} \left\|(\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top\right\|_2^2 +  \frac{2}{n}\left\|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top \right\|_2^2 \nonumber \\
%   &\leq {2}L_\ast^2 \left\|\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\right\|_2^2 +  {2 L_\ast^2} \left\|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \right\|_2^2 \label{cs1} \\
%   &\leq 2c L_\ast^2 \frac{k+ 100 \log(n)}{m_{in}} + {2 L_\ast^2}\left\|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \right\|_2^2 \label{use_concen1}\\
%   &\leq 2c L_\ast^2 \frac{k+ 100 \log(n)}{m_{in}}+ {2} L_\ast^2 \left( 1 +  c\frac{k+ 100 \log(n)}{m_{in}}\right) \label{use_concen2} \\
%   &\leq {2} L_\ast^2 +  4c L_\ast^2 \frac{k+ 100 \log(n)}{m_{in}}
\end{align}
where \eqref{tri0} and \eqref{tri1} follow from the triangle inequality, and \eqref{versh1} follows from \eqref{concen1} and Theorem 4.6.1. in Vershynin with probability at least $1- 4n^{-99}$ after using a union bound over $i \in [n]$.
% from the Cauchy-Schwarz inequality, and \eqref{use_concen1} follows from \eqref{concen1} with probability at least $1- 2n^{-100}$, and \eqref{use_concen2} follows similarly from Theorem 4.6.1. in Vershynin with probability at least $1- 2n^{-100}$.


Similarly, we can show
\begin{align}
  \sigma_{\min} \left( \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) 
   &=  %\left\| \frac{1}{n}  \mathbf{W}_{t,in}^\top \mathbf{W}_{t,in}\right\|_2 \nonumber \\&= %\frac{1}{n}\left\|\mathbf{W}_{t,in}\right\|_2^2 \nonumber \\&= 
   \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)  + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top  \nonumber \\
   &\quad + (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top + 
   \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}
   \mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) 
   \Big) \nonumber  \\
   &= \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)  + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t^\top  \nonumber \\
   &\quad \quad \quad \quad \quad \quad + \mathbf{A}_i + \mathbf{A}_i^\top
   \Big) \nonumber  \\
   &\geq \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)  + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t^\top\Big) \nonumber \\
   &\quad \quad \quad \quad \quad \quad  - \frac{1}{n}\sigma_{\max}( \sum_{i=1}^n \mathbf{A}_i + \mathbf{A}_i^\top) \label{ab}  \\
   &\geq  \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\Big) \nonumber\\
   &\quad + \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t^\top\Big) - \frac{2}{n}\sigma_{\max}( \sum_{i=1}^n \mathbf{A}_i) \label{ab2} \\
   &\geq \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t^\top\Big) - {2}\max_{i\in [n]}\sigma_{\max}( \mathbf{A}_i) \\
   &\geq \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t^\top\Big) - {2}\max_{i\in [n]}\sigma_{\max}( \mathbf{A}_i)
   \nonumber \\
   &\geq \frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t^\top\Big) -2 L_{\max}^2 \delta_{in}(1+\delta_{in})\label{versh1}
%   & ------------ \nonumber \\
%   & \frac{1}{n} \sigma_{\min}^2\left( (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top  \right) \nonumber \\
%   &\geq \frac{1}{n}  \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top  \right) - \frac{2}{n} \sigma_{\max}\left(  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top \right)  \sigma_{\max}\left( (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top\right)   \label{ab} \\
%   &\geq  \mu_\ast^2 \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \right) - 2L_\ast^2 \sigma_{\max}\left(  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \right) \sigma_{\max}\left( \mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\right)   \nonumber \\
%   &\geq \mu_\ast^2 \left(1 - c \frac{k+ 100 \log(n)}{m_{in}}\right) - 2L_\ast^2 \sqrt{c/2} \left(1 + \sqrt{c/2} \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \right) \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \label{versh1} \\
%   &= \mu_{\ast}^2 - 2c (L_\ast^2+ \mu_{\ast}^2) \frac{k+ 100 \log(n)}{m_{in}} - 2 L_\ast^2 \sqrt{c/2}  \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \\
%   &=: \mu^2
\end{align}
where $\mathbf{A}_i \coloneqq (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t\mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top$, 
\eqref{ab} follows from the fact that $\sigma_{\min}(\mathbf{C}_1 + \mathbf{C}_2) \geq \sigma_{\min}(\mathbf{C}_1) - \sigma_{\max}(\mathbf{C}_2)$, 
% thus $\sigma_{\min}^2(\mathbf{C}_1 + \mathbf{C}_2) \geq \sigma_{\min}^2(\mathbf{A}_1) - 2\sigma_{\min}(\mathbf{C}_1) \sigma_{\max}(\mathbf{C}_2) + \sigma_{\max}^2(\mathbf{C}_2) \geq \sigma_{\min}^2(\mathbf{C}_1) - 2\sigma_{\max}(\mathbf{C}_1) \sigma_{\max}(\mathbf{C}_2) $ 
for any two matrices $\mathbf{C}_1$ and $\mathbf{C}_2$, \eqref{ab2} follows from Weyl's inequality, and \eqref{versh1} follows from Theorem 4.6.1 in Vershynin with probability at least $1- 4 n^{-100}$. Next, note that 
\begin{align}
&\frac{1}{n}\sigma_{\min}\Big(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top  \mathbf{\hat{B}}_t \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast^\top\Big) \nonumber \\
&= 
   \frac{1}{n} \sigma_{\min}\left(  \sum_{i=1}^n\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t + \mathbf{\hat{B}}_t^\top (\mathbf{\Sigma}_{i,in} - \mathbf{I}_k)\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top (\mathbf{\Sigma}_{i,in} - \mathbf{I}_k) \mathbf{\hat{B}}_t \right)  \nonumber \\
   &\geq \frac{1}{n} \sigma_{\min}\left(  \sum_{i=1}^n\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t\right) -\frac{1}{n}\sigma_{\max}\left(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top (\mathbf{\Sigma}_{i,in} - \mathbf{I}_k)\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t\right) \nonumber \\
   &\quad \quad - \frac{1}{n}\sigma_{\max}\left(\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top (\mathbf{\Sigma}_{i,in} - \mathbf{I}_k) \mathbf{\hat{B}}_t \right)  \nonumber \\
   &\geq \sigma_{\min}^2(\mathbf{\hat{B}}_t^\top  \mathbf{\hat{B}}_\ast) \sigma_{\min} \left( \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top\right) - L_{\max}^2 \max_{i\in [n]} \| \mathbf{\hat{B}}_t^\top (\mathbf{\Sigma}_{i,in} - \mathbf{I}_k)\mathbf{\hat{B}}_\ast\|_2 - L_{\max}^2  \max_{i\in [n]} \| \mathbf{\hat{B}}_t^\top (\mathbf{\Sigma}_{i,in} - \mathbf{I}_k)\mathbf{\hat{B}}_\ast\|_2 \| \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_\ast\|_2 \nonumber \\
   &= \mu_\ast^2 E_0 - L_{\max}^2 (2\delta_{in} + \delta_{in}^2) 
\end{align}
Combining this with \eqref{versh1} completes the proof.

\end{proof}

\subsection{Infinite outer loop samples}
The following result shows contraction in the case $m_{in} = \Omega\left(\frac{L_\ast^4(k +\log(n))}{\mu_\ast^4 E_0^2}\right)$ and $m_{out} = \infty$.
\begin{lemma}
Suppose that there are infinite samples for the outer loop update, i.e. $m_{out} = \infty$ and $\mathbf{B}_{t+1}= \mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) + \mathbf{\hat{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right)$. Let $\delta_{in} \coloneqq c \frac{\sqrt{k} + 10\sqrt{\log(n)}}{\sqrt{m_{in}}}$ for some absolute constant $c$ and let $\beta \leq 1/(L_{\max}^2(2\delta_{in}+1)^2)$ and $\alpha=1$.
% Assume that $\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)\geq \mu^2$,  $\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \geq \mu_\ast^2 $, \\
% $ \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)\leq L^2$, and $\max_{i\in[n]} \|\mathbf{w}_{\ast,i}\|_2  \leq L_\ast$, and $\beta \leq 1/L^2$. Further assume that $\|\mathbf{w}_t\|_2 \leq 1$, and that $\|\mathbf{w}_{t,i} - \mathbf{\hat{B}}^\top_{t} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\|_2 \leq L_\ast \epsilon_i$. Define $\epsilon \coloneqq \sqrt{\frac{1}{{n}}\sum_{i=1}^n \epsilon_i^2}$.
Then with probability at least $1-4n^{-99}$,
\begin{align}
   \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast)&\leq \frac{1 - \beta \mu_\ast^2 E_0 + 4\beta L_{\max}^2(\delta_{in} + \delta_{in}^2)}{\sqrt{1 - 2 \beta \delta L_{\max}^2 (2\delta_{in} + 1)}}\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
\end{lemma}
\begin{proof}
Note that 
    \begin{align}
       \mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t}\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)
    \end{align}
    Let $\mathbf{\hat{B}}_{t+1}\mathbf{R}_{t+1} = \mathbf{B}_{t+1}$ be the QR decomposition of $\mathbf{B}_{t+1}$. Then we have 
    \begin{align}
        \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) \left\|\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2 \nonumber \\
        &\leq \dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) (1 - \beta \mu^2) \|\mathbf{R}_{t+1}^{-1}\|_2 \label{contract1} \\
        &\leq \dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) (1 - \beta \mu_\ast^2 E_0 + 4\beta L_{\max}^2(\delta_{in} + \delta_{in}^2) ) \|\mathbf{R}_{t+1}^{-1}\|_2 \label{use_lem_cond}
    \end{align}
    where \eqref{use_lem_cond} follows from Lemma \ref{lem:cond} with probability at least $1- 4n^{-99}$. 
    It remains to upper bound $\|\mathbf{R}_{t+1}^{-1}\|_2$.

% Again we have $\dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast)\leq \dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) (1 - \beta \mu^2) \|\mathbf{R}_{t+1}^{-1}\|_2$. 
Let $\mathbf{e}_i \coloneqq  \mathbf{w}_{t,i} - \mathbf{\hat{B}}^\top_{t} \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$. Observe that 
    \begin{align}
        \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
        &= \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) \nonumber \\
        &\quad + \left(\frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top\right)^\top \left(\frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top \right) \nonumber \\
    &= \mathbf{I}_{k} - \frac{\beta}{n} \sum_{i=1}^n \mathbf{e}_i\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{e}_i^\top +\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{e}_i^\top \right) \left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{e}_i \mathbf{w}_{t,i}^\top \right) 
    \end{align}
Next we use the fact that the $O(\beta^2)$ term is PSD, so we can drop it. 
Define $\mathbf{E} \in \mathbb{R}^{n \times k}$ as the matrix whose $i$-th row is $\mathbf{e}_i^\top$ and $\mathbf{W}_{t,in} \in \mathbb{R}^{n \times k}$ as the matrix whose $i$-th row is $\mathbf{w}_{t,i}^\top$.
We obtain
\begin{align}
\sigma_{\min}^2(\mathbf{R}_{t+1})&\geq 1 - 2 \beta \sigma_{\max}
\left( \frac{1}{n} \sum_{i=1}^n \mathbf{e}_i\mathbf{w}_{t,i}^\top  \right) \nonumber \\
% &\geq 1 - 2 \beta \max_{i \in [n]}
% \|\mathbf{e}_i\|_2 \|\mathbf{w}_{t,i}\|_2 \nonumber \\
&= 1 - 2 \beta \sigma_{\max}
\left( \frac{1}{n}  \mathbf{E}^\top \mathbf{W}_{t,in} \right) \nonumber \\
&\geq 1 - 2 \beta  \left\|\frac{1}{\sqrt{n}}\mathbf{E}\right\|_F \left\|\frac{1}{\sqrt{n}}\mathbf{W}_{t,in}\right\|_2 \nonumber \\
&\geq 1 - 2 \beta L_{\max}^2 \delta_{in} (2\delta_{in} + 1)
% &\geq 1 - 2 \beta  \epsilon L_\ast L
\end{align}
where the last inequality follows with probability at least $1-4n^{-99}$ from Lemmas \ref{lem:concen} and \ref{lem:cond}.
 So we have 
\begin{align}
    \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast)&\leq \frac{1 - \beta \mu_\ast^2 E_0 + 4\beta L_{\max}^2(\delta_{in} + \delta_{in}^2)}{\sqrt{1 - 2 \beta  L_{\max}^2 \delta_{in} (2\delta_{in} + 1)}}\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
\end{proof}
% i don't think the union bounds can be removed

\textbf{The above result shows that $m_{in} = \Omega\left( \frac{L_{\max}^4 (k+\log(n))}{\mu_\ast^4 E_0^2}\right)$ results in linear convergence of the representation with high probability. Since $\mu_\ast^2= \Theta\left(\frac{1}{k}\right)$ and $L_{\max}^2 = \Theta(1)$, we essentially have $m_{in} = \Omega\left( \frac{k^2 (k+\log(n))}{E_0^2}\right)$.}

Why we cannot avoid union bound over tasks: intuitively, we need each task to concentrate individually. Concentration of the average across tasks is not enough. We will see that this is not the case for the outer loop update, which allows us to obtain a $\frac{1}{\sqrt{n}}$ factor in the concentration result.


\subsection{Finite Outer Loop Samples}
Now we consider the case in which we have finitely-many samples for the outer loop. Here the update for $\mathbf{B}$ is:
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_t  - \frac{\beta}{nm_{out}}\sum_{i=1}^n\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top + \frac{\beta}{n m_{out}} \sum_{i=1}^n \sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top  \nonumber \\
    &= \mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) + \mathbf{\hat{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right) \nonumber \\
    &\quad + \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right) \mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top  - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right) \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top  
\end{align}
Therefore
\begin{align}
    \mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) \nonumber \\
    &\quad + \frac{\beta}{n} \sum_{i=1}^n \mathbf{\hat{B}}_{\ast,\perp}^\top\left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top % - \frac{\beta}{n} \sum_{i=1}^n \mathbf{\hat{B}}_{\ast,\perp}^\top\left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right) \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top  
\end{align}
Note that here we do not see a gain in the rate of concentration via multiplying the samples with their adjacent matrices, since $\mathbf{B}_{\ast,\perp}$ has $d-k$ columns, not $k$. So the naive outer loop sample complexity will grow with $d+\log(n)$ (using union bound). But we want $\frac{d}{n}$, otherwise we would be using many more samples than parameters. We would like to show that
\begin{align}
    \left\| \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_{\ast,\perp}^\top\left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})\mathbf{w}_{t,i}^\top  \right\|_2 &= O\left(\dist(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast  )\sqrt{\frac{{d}}{{nm_{out}}}}\right) \label{goal1}
\end{align}
with high probability. Conditioning on $\mathbf{w}_{t,i}$, for any fixed unit vector $\mathbf{u} \in \mathbb{R}^k$,
$\mathbf{x}_{i,j}^\top (\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})\mathbf{w}_{t,i}^\top \mathbf{u}$ is sub-Gaussian with sub-Gaussian norm $O(\|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2)$. Also, for any fixed unit vector $\mathbf{v} \in \mathbb{R}^{d-k}$, $\mathbf{v}^\top \mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{x}_{i,j}$ is sub-Gaussian with norm $O(1)$.

So using the variational definition of the spectral norm, we will obtain a sum of $n m_{out}$ independent sub-exponential random variables with norm $O(\|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2)$ and mean zero, so by Bernstein's inequality and a covering argument over $\mathcal{S}^{d-k-1}$ and $\mathcal{S}^{k-1}$ we can show \eqref{goal1} with $\dist(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast)$ replaced by $\max_{i\in[n]}  \|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2$. 
In particular, conditioning on $\{\mathbf{w}_{t,i}\}_{i=1}^n$, we have 
\begin{align}
    \Bigg\| \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_{\ast,\perp}^\top&\left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})\mathbf{w}_{t,i}^\top  \Bigg\|_2 \nonumber \\
    &\leq c \max_{i\in[n]}  \|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2 \max \left( \frac{\sqrt{d}+ \lambda}{\sqrt{nm_{out}}}, \frac{(\sqrt{d}+ \lambda)^2}{nm_{out}} \right) \label{57}
\end{align}
for some absolute constant $c$, with probability at least $1 - 2 e^{-\lambda^2}$ over the outer loop samples. We will choose $\lambda= 10\sqrt{d}$ and let $\sqrt{nm_{out}} \geq 11\sqrt{d}$ to obtain
\begin{align}
    \Bigg\| \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_{\ast,\perp}^\top&\left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})\mathbf{w}_{t,i}^\top  \Bigg\|_2 \nonumber \\
    &\leq \max_{i\in[n]}  \|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2 \delta_{out}
\end{align}
with probability at least $1-2 e^{-100d}$, where $\delta_{out} \coloneqq \frac{11c\sqrt{d}}{\sqrt{nm_{out}}}$.
Now we must relate $ \max_{i\in [n]}\|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2$ and $\dist(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast)$. Note that for any $i \in [n]$,
\begin{align}
    &\|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2 \nonumber \\
    &=\Big\|\mathbf{\hat{B}}_t \left( (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} \right)  \left(\mathbf{{w}}_t^\top  (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) + \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t  \right) \nonumber \\
    &\quad \quad \quad \quad - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\left(\mathbf{{w}}_t^\top  (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) + \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_t  \right) \Big\|_2 \nonumber \\
    &= \Big\|\mathbf{\hat{B}}_t (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t\mathbf{{w}}_t^\top  (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) + \mathbf{\hat{B}}_t (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t\mathbf{{w}}_{\ast,i}^\top  \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t
    \nonumber \\
    &\quad \quad + \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{{w}}_{\ast,i} \mathbf{{w}}_{t}^\top (\mathbf{I}_d - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) +  
    \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{{w}}_{\ast,i} \mathbf{{w}}_{\ast,i}^\top \mathbf{\hat{B}}_{\ast,i}^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t \nonumber \\
    &\quad \quad  - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{{w}}_t^\top  (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_t   \Big\|_2 \nonumber \\    
    &\leq L_{\max}^2\|\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|^2_2 + 2L_{\max}^2\|\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2\| \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_t \|_2  \nonumber \\
    &\quad + L_{\max}^2\|\mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in}\mathbf{B}_\ast - \mathbf{B}_\ast \|_2   \| \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_t \|_2 + L_{\max}^2\|\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2 
\end{align}
Note that 
\begin{align}
    &\|\mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_\ast \|_2 \nonumber \\
    &= \|\mathbf{\hat{B}}_t (\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_t^\top \mathbf{B}_\ast) + \mathbf{\hat{B}}_t\mathbf{\hat{B}}_t^\top  \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_\ast \|_2 \nonumber \\
    &\leq \|\mathbf{\hat{B}}_t (\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast) \|_2 + \|\mathbf{\hat{B}}_t\mathbf{\hat{B}}_t^\top  \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_\ast \|_2  \nonumber \\
    &\leq \|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\|_2 + \dist(\mathbf{\hat{B}}_t,\mathbf{\hat{B}}_\ast)
\end{align}
From earlier, we have that $\max_{i\in [n]} \|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{B}_\ast - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\|_2 \leq \delta_{in}$ and $\max_{i\in [n]} \|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t - \mathbf{I}_d\|_2 \leq \delta_{in}$ with probability at least $1-4n^{-99}$. Thus we have
\begin{align}
    \max_{i \in [n]}\|\mathbf{\hat{B}}_t  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top- \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\|_2 &\leq L_{\max}^2 (1+ \delta_{in}) \dist(\mathbf{\hat{B}}_t,\mathbf{\hat{B}}_\ast) + L_{\max}^2\delta^2 + 2L_{\max}^2 \delta_{in}(1+\delta_{in}) + L_{\max}^2 \delta_{in}(1+\delta_{in}) \nonumber \\
    &= L_{\max}^2 (1+ \delta_{in}) \dist(\mathbf{\hat{B}}_t,\mathbf{\hat{B}}_\ast) +4 L_{\max}^2 \delta_{in}^2 +  3 L_{\max}^2 \delta_{in}
\end{align}
with probability at least $1-4n^{-99}$, then using the fact that $\mathbb{P}(A) = \mathbb{P}(A|B)\mathbb{P}(B) + \mathbb{P}(A|B^c)\mathbb{P}(B^c)$, we have
\begin{align}
    \Bigg\| \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_{\ast,\perp}^\top&\left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})\mathbf{w}_{t,i}^\top  \Bigg\|_2 \nonumber \\
    &\leq  L_{\max}^2\left(  (1+ \delta_{in}) \dist(\mathbf{\hat{B}}_t,\mathbf{\hat{B}}_\ast) +4 \delta_{in}^2 +  3\delta_{in} \right) \delta_{out} \label{62}
\end{align}
with probability at least $1-4n^{-99}-2e^{-100d}$. So we do not have linear convergence. We instead have
\begin{align}
    \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast ) &\leq \left((1 - \beta \mu^2 + \beta L_{\max}^2 \delta_{out}(1+\delta_{in}))\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) + 4\beta L_{\max}^2 \delta_{out}\delta_{in}^2+ 3\beta L_{\max}^2\delta_{out}\delta_{in})\right) \|\mathbf{R}^{-1}_{t+1}\|_2
\end{align}
where
\begin{align}
    \delta_{in} = O\left(\frac{\sqrt{k}+ \sqrt{\log(n)}}{\sqrt{m_{in}}}\right),\quad \delta_{out} = O\left(\frac{\sqrt{d}}{\sqrt{n m_{out}}}\right)
\end{align}
and 
\begin{align}
    \sigma_{\min}^2\left( \mathbf{R}_{t+1}\right) &= \sigma_{\min}^{2}(\mathbf{B}_{t+1,pop}) - 2\beta \sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t+1,pop}^\top  \left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top  \right) \nonumber \\
    &\quad + \beta^2 \sigma_{\min}^2\left( \frac{1}{n}\sum_{i=1}^n  \left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top  \right) \nonumber \\
    &\geq 1 - 2 \beta L_{\max}^2\delta_{in} (2\delta_{in}+1) - 2\beta \sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t+1,pop}^\top  \left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top  \right)
\end{align}
where $\mathbf{B}_{t+1,pop}= \mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) + \mathbf{\hat{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right)$ from the infinite-outer loop sample case.
Note that we can use the analysis from equations \eqref{57} thru \eqref{62} with $\mathbf{\hat{B}}_{\ast,\perp}$ replaced by $\mathbf{B}_{t+1,pop}$ to obtain
\begin{align}
    &\sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t+1,pop}^\top  \left(\mathbf{I}_d - \frac{1}{m_{out}}\sum_{j=1}^{m_{out}} \mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \right)( \mathbf{\hat{B}}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top  \right) \nonumber \\
    &\leq L_{\max}^2\left((1+\delta_{in})\dist(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast) + 4\delta_{in}^2 +3\delta_{in} \right) \delta_{out}' \|\mathbf{B}_{t+1,pop}\|_2 \nonumber \\
    &\leq  L_{\max}^2 (1+2\delta_{in})^2 \delta_{out}' \|\mathbf{B}_{t+1,pop}\|_2  \nonumber \\
    &=   L_{\max}^2 (1+2\delta_{in})^2 \delta_{out}' \left\|\mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) + \mathbf{\hat{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right)\right\|_2  \nonumber \\
    &\leq L_{\max}^2(1+2\delta_{in})^2 \delta_{out}'\left( \left\|\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right\|_2 + \left\|\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right\|_2 \right) \nonumber \\
    &\leq L_{\max}^2(1+2\delta_{in})^2 \delta_{out}' \left( 1 - \beta \mu^2 + \beta L_\ast L \right) 
\end{align}
with probability at least $1- 4n^{-99} - 2e^{-100k}$, where $\delta_{out}' \coloneqq c\frac{\sqrt{k}}{\sqrt{nm_{out}}}$.
Putting everything together, we obtain the following result.


\begin{theorem}
Let $\delta_{in} = O\left( \frac{\sqrt{k} + 10\sqrt{\log(n)}}{\sqrt{m_{in}}}\right)$, $\delta_{out} = O\left( \frac{\sqrt{d}}{\sqrt{n m_{out}}}\right)$, and $\delta_{out}' = O\left( \frac{\sqrt{k}}{\sqrt{n m_{out}}}\right)$. Choose $\beta \leq 1/(L_{\max}^2(2\delta_{in}+1)^2)$ and $\alpha=1$. Then
\begin{align}
    \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast ) &\leq \frac{1 - \beta E_0\mu_\ast^2 + 4\beta L_{\max}^2 (\delta_{in}+\delta_{in}^2) ) + \beta L_{\max}^2 \delta_{out}(1+\delta_{in})}{\sqrt{1 - 2 \beta L_{\max}^2 \delta_{in} (1+2\delta_{in}) - 2\beta \delta_{out}'(1+2\delta_{in})^2  L_{\max}^2 \left( 1 - \beta \mu^2 + \beta L_{\max} L \right) }}\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) \nonumber \\
    &\quad + \frac{2\beta L_{\max}^2 \delta_{out}\delta_{in} (1+ \delta_{in})}{\sqrt{1 - 2 \beta\delta_{in} L_{\max}^2 (1+2\delta_{in}) - 2\beta L_{\max}^2  \delta_{out}' (1+2\delta_{in})^2  \left( 1 - \beta \mu^2 + \beta L_{\max}L \right) }},
\end{align}
where $L \leq \sqrt{  L_{\max}^2 (2\delta_{in}+1)^2}$ and $\mu^2 \geq \mu_\ast^2 E_0 - 4 L_{\max}^2 (\delta_{in} + \delta_{in}^2)$, all
with probability at least $1- 4n^{-99} - 2e^{-100k} - 2e^{-100d}$. 
\end{theorem}
Assuming the denominator is $\Omega(1)$ (which it is for $m_{in} \gg k + \log(n)$ and $m_{out} \gg d/n$), the representation converges to a neighborhood of size  $O(\delta_{out}\delta) \equiv O\left(\frac{\sqrt{dk}+\sqrt{d\log(n)}}{\sqrt{nm_{in}m_{out}}}\right)$.

Again we require $\delta_{in} = \Omega\left(\frac{L_{\max}^4(k + \log(n))}{\mu_\ast^4 E_0^2 }\right) \approx \Omega\left(\frac{k^2(k + \log(n))}{E_0^2}\right)$ and likewise $\delta_{out} = \Omega\left(\frac{L_{\max}^4d}{\mu_\ast^4 E_0^2 }\right) \approx \Omega\left(\frac{k^2 d}{E_0^2}\right)$ for linear convergence to the neighborhood. 



\textbf{Simulations to verify this:}


\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_pop.png}}
\vspace{-0mm}
\caption{ANIL linearly converges to the ground truth in the population case. Here $k=3$, $d=10$, $n=10$, $\alpha=1$, $\beta=1$, and we orthogonalize $\mathbf{B}_t$ at the end of each round. In the case when we do not orthogonalize $\mathbf{B}_t$, we still have linear convergence for smaller $\alpha, \beta$. Also note that for $n=2<k$, the representation does not converge to the ground truth (since we do not have task diversity).}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

{\color{red}\textbf{NOTE: all plots show $\dist^2$, not $\dist$.}}

\textbf{$\rightarrow$ Neighborhood size should be $O\left(\frac{dk+d\log(n)}{nm_{in}m_{out}}\right)$}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_min_alpha1.png}}
\vspace{-0mm}
% \caption{ }
\caption{Varying $m_{in}$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_mout.png}}
\vspace{-0mm}
% \caption{ }
\caption{Varying $m_{out}$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_n.png}}
\vspace{-0mm}
% \caption{ }
\caption{Varying $n$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}



% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_min_mout_alpha1.png}}
% \vspace{-0mm}
% % \caption{ }
% \caption{Varying $m_{in}m_{out}$, with $\alpha=1$}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}


\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_k.png}}
\vspace{-0mm}
\caption{Varying $k$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_min_largek.png}}
% \vspace{-0mm}
% \caption{Varying $m_{in}$ with larger $k$}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_d.png}}
\vspace{-0mm}
\caption{Varying $d$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_min.png}}
\vspace{-0mm}
% \caption{ }
\caption{Varying $m_{in}$, with $\alpha=0.1 \neq 1$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.68\columnwidth]{anil_fs_50_200.png}}
\vspace{-0mm}
% \caption{ }
\caption{Varying $m_{in}m_{out}$, with $\alpha=0.1 \neq 1$}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

{\color{blue} So we have correct dependence on $m_{out}, m_{in}, d, k$ and $n$.}

% {\color{blue} So we have correct dependence on $d, m_{out}$ and $n$ (up to $\log(n)$), but incorrect for $m_{in}$. The experiments suggests that there is no $\delta$ product in the neighborhood bound. Note that the $d$ term in $\delta_{out}$ is really $d+k$, and we have so this may explain the increasing of the neighborhood size with $k$ if there is indeed no. $\delta$ factor in its bound. }

Note: in order to see dependence on $m_{in}$ experimentally, we must set $\alpha=1$, which makes sense from the theory.






% {\color{red} These plots suggest there is some error in the analysis. Specifically we should have $\frac{1}{nm_{out}}$ in the upper bound on the neighborhood size instead of $\frac{1}{\sqrt{nm_{in}m_{out}}}$. The looseness must be in (58)-(61). But I think the max is unavoidable since we must union bound over the $\epsilon$-net...}

% it is possible that $m_{in}$ does not matter because we only need diverse heads, which we can get by random choice of them. But choosing random heads does not work.

%check role of k



% Also need sims for fixed m-in, then fixed m-out

% also vary d, k, n, fix everything else


% thoughts for meeting:
% 1. this relies on batches with heads spanning Rk, which is not realistic.
% 2. the point of this analysis is to show that you don't need the inner update for the representation - you can learn the ground-truth representation without it as long as you have task diversity in the heads. So what should be our goal in analyzing the MAML case? show that the inner update can hurt you in some cases? no not true. show a lower bound on the sample complexity for maml... or any gradient-based alg? would be difficult. see meta-learning sample complexity paper




% \textbf{The question is, can we capture the benefit of many tasks in the outer loop update? We want $m_{out} = \Omega (\frac{d}{n})$.}

%%%%%%%%%%%%%%% IMPORTANT STUFF

% {\color{red} 3/30}
% \begin{itemize}
%     \item From simulations:
%     \begin{itemize}
%     \item In all linear cases: ERM does not learn representation (principle angle distance of first layer to the ground truth is always between 0.9 and 1).
%     \item In all linear cases: There is no performance difference between ANIL and MAML.
%         \item Exactly parameterized two-layer linear case: ANIL and MAML first layer has principle angle dist roughly 0.1 from the ground truth.
%         \item Overparameterized two-layer linear case: ANIL and MAML first layer reaches principle angle dist 0.01 - 0.3 from the ground truth, but it is not stable, and distance begins to increase after many iterations. But sometimes it decreases again, so it is not quite the classic overfitting U curve. Also, I am using fresh samples on each iteration, so I don't think overfitting should be an issue.
%         \item TODO: All in overparameterized case: What happens with more layers (Arnold paper says more layers help MAML)? What happens with more than 2 tasks? How do MAML/ANIL compare to FedRep ( note that ANIL is roughly Alt-GD with a second-order update for the head)? More grad steps for the head? No task diversity? Eventually, what happens in ReLU case? 
%         \item No task diversity means MAML/ANIL does not learn the representation.
%         \item Random, non-orthogonal tasks increases the principle angle distance for MAML/ANIL ( but the tasks still span R2, so the error is still only 0.2-0.4).
        % \item Things that should happen in experiments on real data: increasing task batch size should help performance, outer loop update for head should not matter much.
    % \end{itemize}
    % \item Jin paper On the Importance of Task Diversity: task diversity is key to learning the representation, as expected. But task diversity for them requires that the tasks span the dimension of the final layer, is this safe to assume? Note that we can still be overparameterized in this case, just not in the last layer. So FedRep performance should increase with higher participation rate... no, this might cause it to learn a better representation but it still might overfit the heads. Can we extend Jin results to case when heads are also over parameterized? i.e. the dimension of the true rep is actually $r' < r$, then you just reed that the r'-th singular value of the task diversity matrix is greater than zero? yes, i think this should doable, and this is roughly what we see in the simulations. It remains to answer the optimization question....
% \end{itemize}


==> Introduction-orig.tex <==
\section{Introduction}

% Training neural networks from scratch is expensive. 
% Using effective representations of data has long been viewed as a means by which both humans and machines learn more complicated relationships. For example, representing patients' extensive medical histories with sets of key features helps to diagnose conditions.
% Recently,  

Deep learning models are effective at solving certain tasks with ample data and computational resources for training. Yet these costly training procedures are inapplicable to many realistic multi-task settings in which
% because the multitude of tasks in such settings require that 
models must rapidly adapt to new tasks on the fly, rather than re-train from scratch on every new task.
% To address this, {\em meta-learning} aims to extract  common information from tasks in multi-task environments that can be exploited to quickly and effectively solve new tasks. 
% In this case the problem of finding rapidly adaptable models reduces to that of finding good representations, a ubiquitous problem in machine learning.
% Meta-learning aims to train rapidly adaptable models by extracting some inductive bias from a set of meta-training tasks. In 
% Training modern neural networks from scratch is highly expensive in terms of both computation and data. 
% , making deep learning problematic in application domains that require fast adaptation. 
% % model-agnostic meta-learning (MAML) \cite{finn2017model}, this 
To train adaptable models,  we can aim to leverage the fact that tasks in multi-task settings often share useful information. In many classification and regression problems, this information is a shared set of features of the data from different tasks which are most relevant to each data point's label. Therefore, a widely popular approach 
to achieve fast adaptation in multi-task settings 
is to learn a representation that extracts the important features  shared across tasks
% , then adapt low-dimensional, task-specific predictors on top of the representation 
\cite{maurer2016benefit}. However, our understanding of {\em how} multi-task representation learning should be done and {\em why} certain methods work well is still nascent. 
% This has led to an extensive literature in multi-task representation learning \citep{}.
% This is motivated by the observation that the shared information in multi-task settings often lies in the feature space (for example, in few-shot image classification, images from different tasks often share similar features relevant to their label), and that learning the proper shared features reduces the number of task-specific model parameters that need to be learned for each task. 
% here is the problem, here is the natural way to solve it, here are the popular methods which do not directly do the natural approach, here we show that they in fact do the natural approach.
% Often this shared information can be captured by a universal feature representation, which %by dimensionality reduction 
% can improve the rate at which the model can adapt to new tasks. 
% which has led  empirical benefits of learning a common data representation in multi-task environments have been widely celebrated.


% However, little is formally known about {\em how} representation learning should be done or {\em why} certain methods work well.% Most notably, 


Recently, a paradigm known as {\em meta-learning} has emerged as a powerful means of learning multi-task representations. This was sparked in large part by the introduction of Model-Agnostic Meta-Learning (MAML) \citep{finn2017model}, 
which achieved impressive results in few-shot image classification and reinforcement learning scenarios, and led to a series of related  gradient-based meta-learning (GBML) methods
\citep{raghu2019rapid,nichol2018reptile,antoniou2018train, hospedales2020meta}.
% A particularly illuminating example of this is in the case of gradient-based meta-learning (GBML) methods. 
% Ostensibly, these methods have nothing to do with representation learning:
Surprisingly, MAML does not explicitly try to learn a useful representation; instead,
it aims to find a good initialization for a small number of task-specific gradient descent steps, agnostic of whether the learning model contains a representation. 
% Yet empirical studies have attributed the fast adaptability of the nerual networks learned by MAML and its related methods to the theory that they consist of a high-quality representation applicable across tasks.
% Yet MAML has achieved impressive empirical successes in learning fast-adapting neural networks
%such as few-shot image classification and meta-reinforcement learning 
% \citep{finn2017model,antoniou2018train}, and further empirical studies have attributed their success to representation learning \cite{raghu2019rapid}. 
Nevertheless, \citet{raghu2019rapid} empirically argued that MAML's impressive performance on neural networks is likely due to its tendency to learn a shared representation across tasks. To make this argument, they noticed that MAML's representation does not change significantly when adapted to each task, and a modified version of MAML that freezes the representation during local adaptation, known as the Almost-No-Inner-Loop algorithm (ANIL), typically performs as well as MAML. 
% These methods aim to ``learn to learn'', i.e. meta-learn, by finding a model that can quickly learn new tasks via only a few steps of stochastic gradient descent (SGD). 
% Notably, there is  no explicit intention by these methods to learn a strong representation, making their representation learning capabilities all the more mysterious.
Yet an explanation for { why} optimizing an objective that rewards good initializations for gradient descent seems to lead to strong representations remains elusive - in particular, it has  not been shown whether MAML, or even ANIL, learn high-quality representations. Thus, in this paper, we aim to address the following questions:
% Nevertheless, a rigorous theoretical understanding of why these algorithms perform well in practice has remained elusive.  To bridge this gap, here we study the following question:

\vspace{-3mm}
\begin{quote}
\em{Do MAML and ANIL provably learn high-quality representations? If so, why?}
\end{quote}
\vspace{-3mm}

% In the most ubiquitous GBML method, model-agnostic meta-learning (MAML), the entire model, including the representation, is adapted via SGD to an incoming task, meaning that there is no direct intention to learn a shared representation across tasks. However, recent empirical results due to \cite{raghu2019rapid} showed that the representation does not change very much during the task-specific adaptation phase of MAML, and that the performance of MAML can be matched by an algorithm that holds the representation fixed across tasks, and only executes task-specific adaptation for the predictor, known as almost-no-inner loop (ANIL). Indeed, this evidence suggests that the key to MAML is that it learns an effective shared representation.
% However, the inner workings of GBML methods remain mysterious from the theoretical perspective. It remains to be proven whether GBML in fact learns good representations, and, more importantly, {\em how} it does so. 

% However, the reasons for such 


% aim to extract the common information among the tasks without formulating the information as a representation. Instead, GBML methods 
% aim to learn an {\em initialization} for a small number of steps of stochastic gradient descent (SGD). In other words, the initial model should contain shared information across the tasks that enables strong performance on a new task after only a few steps of fine-tuning. 
% Meta-learning aims to develop rapidly adaptable models for multi-task settings by extracting this common information from the tasks.
% In gradient-based meta-learning (GBML), this common information is formulated as an initialization for a small number of steps of stochastic gradient descent (SGD). In other words, the initial model should contain some shared information across the tasks that enables strong performance on a new task after only a few steps of fine-tuning. 

%  GBML methods find such an initial model by executing an episodic meta-training procedure, where in each episode, the current initial model is locally adapted to the sampled task in the so-called inner loop, then  updated based on the performance of the adapted models in the outer loop. This episodic procedure mimics the realistic few-shot learning evaluation procedure that considers model performance after a few steps of SGD with few samples for a new task. 
 
 
 
%  A natural explanation for this success is that GBML somehow learns a good representation for downstream tasks. Indeed, this explanation has been substantiated by plentiful empirical evidence. For example, \cite{raghu2019rapid}...
 

%  Once we understand how GBML methods learn good representations, we can leverage these properties to develop more effective and efficient meta-learning and representation learning algorithms more broadly, as we seek to harness the power of neural networks to extract useful features from increasingly high-dimensional data.
% A rigorous understanding of how GBML methods learn effective representations is important not only in the contexts of meta- and few-shot learning, but also for representation learning more broadly, as we seek to harness the power of neural networks to extract useful features from increasingly high-dimensional data. 

To answer these questions we consider the well-known multi-task linear representation learning setting \citep{maurer2016benefit,tripuraneni2020provable,du2020fewshot} in which each task is a noisy linear regression problem in $\mathbb{R}^d$ with optimal solution lying in a shared $k$-dimensional subspace. The learning model is a two-layer linear network consisting of a representation and head, and we would like the learned representation to project data onto the shared subspace so as to reduce the number of samples needed to find the optimal regressor for a new task from $O(d)$ to $O(k)$.
% We show that the answer to the first question is yes in a multi-task linear representation learning setting.
% in which the learning model is a two-layer linear network.
% considered in \citep{maurer2016benefit,tripuraneni2020provable,du2020fewshot}.
Although this setting is simple,  many recent works have shown that the dynamics of deep networks can be explained by studying linear models, and even in this linear case it is not known whether MAML and ANIL can learn accurate representations.
{\em We prove, for the first time, that both MAML and ANIL, as well their first-order approximations, are capable of representation learning and recover the ground-truth subspace in this setting.}

    % Specifically, we consider a well-known setting in which 
    % we prove  that MAML and ANIL,
    % two ubiquitous GBML methods, Model-Agnostic Meta-Learning (MAML) \cite{finn2017model} and the Almost-No-Inner-Loop method (ANIL) \cite{raghu2019rapid}, 
    % as well as their first-order approximations, recover the low-dimensional subspace in which the optimal regressors for linear regression tasks lie. Learning this subspace, i.e. the ground-truth representation, reduces the sample complexity required to solve a new task from the environment, but doing so is non-trivial, as there are infinitely many possible subspaces. Indeed, running standard gradient descent to minimize the average loss across tasks in this environment does not recover the ground-truth subspace. In contrast, our analysis reveals that ANIL and MAML's distinctive inner loop updates for the last layer of the learning model are critical to their ability to recover the ground-truth representation. 
% For example, 
% Here each task 
% % in this 
% % % The $i$-th task in this 
% % setting 
% is a noisy linear regression problem.
% % with data generated by a ground-truth regressor $\boldsymbol{\theta}_{\ast,i} \in \mathbb{R}^d$. 
% To account for the advantage of representation learning, we assume that all ground-truth regressors belong to the same low-dimensional subspace. 
% In other words, there exists a representation that projects data to this low-dimensional space and preserves all the information needed to predict the data's label.
% If we  know this representation, or equivalently, know the subspace, then we can reduce the number of samples needed to solve a new task by projecting the task's data onto the subspace.
% % can learn a representation that projects the data to this subspace, then we will reduce the dimension of the problem and thereby the number of samples needed to solve a new task. 
% %#$k$-dimensional subspace of $\mathbb{R}^d$.
% % which is equal to the column space of an orthogonal matrix $\mathbf{B}_\ast$. 
% can learn a representation that projects the data to this subspace, then we will reduce the dimension of the problem and thereby the number of samples needed to solve a new task. 
%#$k$-dimensional subspace of $\mathbb{R}^d$.
% which is equal to the column space of an orthogonal matrix $\mathbf{B}_\ast$. 
Our analysis reveals that ANIL and MAML's distinctive inner loop updates for the last layer of the learning model are critical to their ability to recover the ground-truth representation. 
Figure \ref{fig:intro} visualizes this observation: both Exact ANIL and MAML and their first-order (FO) versions (which ignore second-order derivatives)  learn representations which approach the ground truth {\em exponentially fast}, while running standard gradient descent to minimize the average loss across tasks, which lacks inner loop updates, fails to recover the ground-truth. We show that the inner loop updates of the head exploit \textit{task diversity} to make the outer loop update for the representation bring it closer to the ground-truth.
% that when running ANIL and MAML and their first-order analogues over a two-layer linear network, where the first layer is a low-dimensional projection,
% the model class consisting of a representation 
% $\mathbf{B} \in \mathbb{R}^{d\times k}$ and a head $\mathbf{w} \in \mathbb{R}^k$, 
%  Moreover, standard risk minimization without ANIL and MAML's distinctive inner loop updates fails to recover the ground-truth subspace. 
\begin{figure}[t]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.9\columnwidth]{anilmamlintro.pdf}
% anil_fs_min_alpha1.png
}
\vspace{-2mm}
% \caption{ }
\caption{Multi-task linear representation learning error for ANIL, MAML and no inner loop algorithm.}
\vspace{-8mm}
\label{fig:intro}
\end{center}
\end{figure}


Showing that ANIL and MAML recover the ground-truth representation involves numerous technical challenges:
{\em (i)~Shared global head}. In contrast to multi-task representation learning approaches that learn unique, stateful heads for
each task, ANIL and MAML learn a global head.
This appears to restrict ANIL and MAML from harnessing
the task diversity which has been shown to aid representation learning in the stateful-heads case \cite{collins2021exploiting, thekumparampil2021statistically}.
% We overcome this by showing that ANIL and MAML's inner loop updates are sufficient to achieve diversity of the heads. 
 {\em (ii) Complicated updates.} ANIL and MAML's inner loop updates cause the outer loop updates to have an overwhelming number of terms even in simple linear settings, requiring prior works to use a symbolic toolbox for analysis \cite{arnold2021maml}.   {\em (iii) Control of parameter norms.} Neither ANIL nor MAML allows for normalization on each iteration nor explicit regularization of the objective function, yet still the energy in the representation  and head  must be controlled. {\em  (iv) Finite samples.} The above challenges exist even with infinite samples per task, and are only accentuated in the finite-sample case. To obtain practical results, we must show that ANIL and MAML can learn the representation with only $o(d)$ samples per task.
 Despite these challenges, we show the following results (see Table~\ref{sample-table} for more details):

% If ANIL and MAML learned a unique, stateful head $\mathbf{w}_i$ for each task, as in alternate multi-task learning \cite{} and pre-training \cite{} approaches, then the linear representation learning problem would reduce to a low-rank matrix sensing problem for which standard algorithms have been shown to find the optimal solution \cite{collins2021exploiting, thekumparampil2021statistically}. Key to these analyses is the idea that the task-unique heads satisfy some notion of diversity, which causes the representation to move towards the ground-truth. However, learning separate heads may not be tractable in settings with many tasks, so 


% ground-truth representation $\mathbf{B}_\ast\in \mathbb{R}^{d\times k}$ and a task-specific head $\mathbf{w}_{\ast,i} \in \mathbb{R}^{k}$, where $k\ll d$. The implicit goal is to recover the low-dimensional column space of $\mathbf{B}_\ast$ by learning a two-layer linear network consisting of a representation $\mathbf{B} \in \mathbb{R}^{d\times k}$ (first layer)  and a head  $\mathbf{w}\in \mathbb{R}^{k}$ (second layer). 
% Although this two-layer linear setting is simplified compared to deep neural networks, many recent works have shown that the dynamics of deep networks can be explained by studying linear models. Moreover, our analysis of this setting explains numerous phenomenon observed in regards to MAML and ANIL's behavior on deep networks.

% , since all of the task-optimal solutions lie in this low-dimensional space.
% The simulations in Figure 1 show that both ANIL and MAML indeed recover $\col(\mathbf{B}_\ast)$ up to statistical accuracy with random initialization and only one step of inner loop task-specific adaptation as long as the tasks are sufficiently diverse. 

% Even in this simple setting, it is impressive that ANIL and MAML learn the desired representation, because the closely related method that lacks an inner loop for the heads does not.
% . These results are shown in Figure \ref{fig:11}.
% ANIL and MAML attempt to learn a two-layer linear network consisting of a representation $\mathbf{B} \in \mathbb{R}^{d\times k}$ and a head (final layer) $\mathbf{w}\in \mathbb{R}^{k}$ in this setting,  where $k$ is the dimension of the data and $d \gg k$ is the ambient dimension of the data. 

% Simulations for this setting show that indeed MAML and ANIL learn the ground-truth representation
% However, even in this simple setting, prior results have not shown whether ANIL and/or MAML recover the ground-truth representation $\mathbf{B}_\ast$ with any number of samples. 
% Until now, no one has proven that either ANIL or MAML recover the ground-truth representation in this (or any other) setting, as doing so in this case requires overcoming numerous technical challenges: 

% The simulations in Figure 1 show that both ANIL and MAML indeed recover $\col(\mathbf{B}_\ast)$ in the multi-task linear representation learning setting up to statistical accuracy with random initialization and only one step of inner loop task-specific adaptation as long as the tasks are sufficiently diverse. 
% Yet even in this simple setting, proving that ANIL and MAML recover the ground-truth representation requires overcoming numerous technical challenges: 



% As a result, we must show that the ANIL and MAML heads updated post-inner loop from the global initialization are diverse.




% (ii) {\em Landscape analysis does not suffice.} A landscape analysis does not suffice because there exist stationary points whose representation does not agree with the ground-truth (for ANIL, note that any $\mathbf{B}\mathbf{w}$ s.t. $\sum_{i=1}^n (\mathbf{B}\mathbf{w} - \mathbf{B}_\ast\mathbf{w}_{\ast,i})(\mathbf{B}\mathbf{w} - \mathbf{B}_\ast\mathbf{w}_{\ast,i})^\top = \mathbf{0}$ and $\sum_{i=1}^n \mathbf{B}\mathbf{w} - \mathbf{B}_\ast\mathbf{w}_{\ast,i} = \mathbf{0}$ is stationary //// but there are no such points////), and the objectives are non-convex, so there is no guarantee to reach a global minimum.
% Also, first-order methods perform nearly as well as the exact versions of the algorithms, even though the objective that these methods minimize is unknown.

% Instead, we must study the dynamics of the algorithms.

% Moreover, these terms may increase on each iteration, with the amount of increase depending on the size of other variables at that time. 



% train a model on many meta-training tasks with an objective that  penalizes the loss of the  model after it has been updated with a small number of task-specific gradient steps with a small number of samples, which is known as the inner loop. 
% This meta-training procedure mimics the typical few-shot learning evaluation procedure, in which the model is allowed to take a small number of gradient steps with few samples in order to learn a new task.
% The task-specific gradient steps are known as the {\em inner loop}, while the refinement of the initial model based on the results of the inner loop is known as the {\em outer loop}.

% From an empirical perspective,
% \citet{raghu2019rapid} showed that model-agnostic meta-learning (MAML), the foundational GBML method, often learns a static set of features during meta-training. They also introduced a modified version of MAML, called the Almost-No-Inner Loop (ANIL) algorithm, that only adapts the final layer of the network in the inner loop, instead of the full model as MAML does. They showed that this method typically matches and sometimes even exceeds the few-shot learning performance of MAML. These observations  suggest that the key to MAML (and ANIL) is that it learns a high-quality global feature representation, one that does not need to be locally adapted to each task. Intuitively, representation learning boosts few-shot learning performance by reducing the number of parameters that need to be updated to learn a new task.

% posed two hypotheses to explain the success of model-agnostic meta-learning (MAML) \citep{finn2017model}, the foundational GBML method: 
% {\em feature reuse} and {\em rapid learning}. According to feature reuse, MAML learns a set of reusable features, i.e. a shared representation, across tasks, and essentially only modifies the last layer of a model to adapt to a new task. In contrast, rapid learning posits that MAML succeeds because it learns a model well-suited for full adaptation to a new task, meaning that even the features change significantly during task-specific adaptation. 
% Their experiments suggest that the latter hypothesis, feature reuse, is the dominant explanation for the success of MAML in neural networks, as they found that the representation layers of networks trained by MAML do not change much when adapting to a new task. Moreover, they showed that a modified version of MAML in which only the last layer is updated in the inner loop, which they call the Almost-No-Inner Loop (ANIL) algorithm, matches and sometimes even exceeds the performance of MAML.

% Nevertheless,
% little is known theoretically about the quality of the representations that GBML methods learn, and if they indeed learn high-quality representations, {\em how} they do so. A rigorous understanding of how MAML and ANIL learn effective representations is important not only in the contexts of meta- and few-shot learning, but also for representation learning more broadly, as we seek to harness the power of neural networks to extract useful features from increasingly high-dimensional data. To study the representation learning abilities of GBML, we work with the multi-task linear representation learning setting considered in \cite{maurer2016benefit,tripuraneni2020provable,du2020fewshot}. Namely, we consider that ANIL and MAML attempt to learn a two-layer linear network consisting of a representation $\mathbf{B} \in \mathbb{R}^{d\times k}$ and a head (final layer) $\mathbf{w}\in \mathbb{R}^{k}$, where $k$ is the dimension of the data and $d \gg k$ is the ambient dimension of the data. The $i$-th task is a noisy linear regression problem with data  generated by a universal ground-truth representation $\mathbf{B}_\ast\in \mathbb{R}^{d\times k}$ and a task-specific head $\mathbf{w}_{\ast,i} \in \mathbb{R}^{k}$. Even in this simple setting, prior results have not shown whether ANIL and and MAML recover the ground-truth representation $\mathbf{B}_\ast$ with any number of samples. Doing so requires overcoming numerous technical challenges: (i) 
% Technical challenges:
% - the main challenge is that people have not shown why maml or anil work
% - discrete gradient steps
% - characterizing sample complexity
% - showing B stays well-conditioned without normalization
% - showing why task diversity matters
% - learning a single head, not personalized heads like in recent papers


% This is especially important as representation learning  becomes increasingly important for 

% \textbf{Contributions.} 


\textbf{ANIL - } Both Exact ANIL and its first-order approximation FO-ANIL converge {\em exponentially fast to the ground-truth subspace with efficient sample complexity} as long as the initialization has constant error and  there is task diversity. Specifically, the ground-truth heads for the tasks sampled on each round {\em must span $\mathbb{R}^k$}. Moreover, the more diverse, or evenly spread, that the sampled ground-truth heads are on average, the {\em faster the exponential rate of convergence}.

\textbf{MAML -} Exact and FO-MAML also converge {\em exponentially fast to the ground-truth subspace} but require more a stringent requirement on the initialization: the initial error must be smaller with less task diversity. {\em The less diverse the tasks are, the more accurate the initialization needs to be}. Moreover, for FO-MAML, is it further required that  average of the ground-truth heads sampled on each iteration is {\em concentrated around zero}. These extra conditions suggest that MAML's distinctive inner loop updates for the representation are unnecessary and even potentially harmful to representation learning. 

% All results are given for both population and finite-sample cases, and verified by numerical simulations.

% we prove that MAML and ANIL learn the ground-truth representation 
% in a well-known linear multi-task representation learning setting with two-layer linear neural networks 
% by exposing the benefit of task diversity. Our contributions are summarized as follows:
% We show the linear convergence of both algorithms to the ground-truth representation with information-theoretically tight sample complexities. In particular, we prove that only $O(k^2)$ samples are required for the inner loop updates for the last layer, where $k$ is the dimension of the representation and is assumed to be small, helping to formally explain the accuracy of ANIL in few-shot learning scenarios. We further show that the inner loop updates for the last layer are critical to representation learning, as without them (standard training) we would not be able to learn the representation. Moreover, the inner loop updates for the representation do not seem to provide any representation learning benefit, and may even inhibit representation learning. 
% % since our upper bound on the convergence rate is smaller and less restrictive for ANIL than for MAML. 
% We verify these results  through extensive numerical simulations.

% {\em another option for intuition: look at ANIL loss: for appropriate step size, $\mathbf{B}$ can only minimize it if if shares column space with $\mathbf{B}_\ast$}


% insert equation for update of B $\mathbf{G}_{\text{reg}}(\mathbf{B}_t)$, where $\mathbf{G}_{\text{reg}}(\mathbf{B}_t)$ is the gradient of a regularization term that encourages $\mathbf{B}_t$ to stay well-conditioned.




% two (mutually exclusive?) benefits: dimensionality reduction and generalization via overparameterization. We focus on dimensionality reduction



% {\color{red}
% Current status 11/7:
% \begin{itemize}
%     \item We have linear convergence result for ANIL and FO-ANIL without regularization in the population case.
%     \item We have linear convergence result for MAML (without regularization) and FO-MAML (without regularization and means of heads close to zero) in the population case.
%     % \item In the finite-sample case, I am stuck on how to show that $\|\mathbf{w}_t\|$ stays bounded, since the finite-sample errors from each iteration are not summable.
%     % \item For FO-MAML, we have linear convergence in the population case  when the mean of the ground-truth heads is small. Empirically, the mean must be very close to zero.
%     % \item For (exact) MAML, empirically, there is linear convergence as long as the norm of the mean of the ground-truth heads is less than a constant. But, I am stuck on how to show that $\|\mathbf{w}_t\|$ stays bounded, because mathematically it may increase by a constant on every round. Unlike for ANIL, we cannot use that $\|\alpha\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k\|_2$ is going to zero, because the upper bound on $\|\alpha\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}_k\|_2$ includes a term with only constants and $\|\mathbf{w}_t\|_2$.
% \end{itemize}
% Please see Appendix for proofs.
% }
% We study whether ANIL and MAML can learn accurate low-dimensional representations in the multi-task linear representation learning setting. Our analysis makes the following contributions:

% \textbf{Provable representation learning abilities of ANIL and MAML.} We prove, for the first time, that ANIL and MAML recover the ground-truth representation up to the statistical accuracy in the realizable linear representation learning setting. Moreover, we show that they do so at a linear rate. 
% These results provide rigorous theoretical justification for the representation learning benefits of ANIL and MAML that have been observed empirically in recent works \cite{finn2017model,raghu2019rapid}.
% % Our analysis overcomes numerous technical challenges, including showing that the learned representation remains well-conditioned and  the learned head is close to zero.

% \textbf{Importance of Task Diversity/ Importance of inner loop head updates.} 
% Recent works have highlighted the role of task diversity in enabling representation learning in generic multi-task settings from a statistical perspective \cite{tripuraneni2020provable, du2020fewshot} as well as empirically \cite{ni2021data}. Our analysis helps to complete the picture by showing that the dynamics of of two ubiquitous meta-learning algorithms critically leverage task diversity to learn the ground-truth representation.

% \textbf{Lack of gain of MAML over ANIL.} While our analysis highlights that task diversity is critical to representation learning, it also demonstrates that MAML's inner loop update for the representation is not. ANIL obtains at least as good theoretical guarantees without an inner loop update for the representation. In fact, MAML's inner loop update of the representation can even hurt in some cases, for instance, FO-MAML can only learn the representation if the ground-truth heads have mean very close to zero. Intuitively, this holds because without an inner loop for the representation, the outer loop gradient is like the gradient with respect to a certain matrix factorization problem whose solutions in $\mathbf{B}$ share column space with $\mathbf{B}_\ast$. With the inner loop update, this gradient is perturbed in a direction that may disagree with $\col({\mathbf{B}_\ast})$.
% These findings are consistent with recent empirical results showing that ANIL performs at least as well as MAML on few-shot learning benchmarks \cite{raghu2019rapid}.


% \textbf{Efficient sample complexity.}


% (v) \textit{Explanation for other empirically-observed phenomena.} Zeroing trick (formal result on this?) strong performance of multi-task representation learning/pretraining


% \textbf{Numerical Simulations.}



% \begin{enumerate}
%     \item We show that both ANIL and FO-ANIL learn a  linear representation that is $\epsilon$-close to the ground-truth representation exponentially fast, where $\epsilon = O(\frac{1}{m_{in}m_{out}})$.
%     \item We show that MAML (and FO-MAML as long as the mean of the ground-truth predictors is sufficiently close to zero) also learns an approximation of the ground-truth linear representation at an exponentially fast rate. In particular, the MAML representation is $\epsilon'$-accurate with $\epsilon' = O()$.
%     \item We verify our theoretical results with extensive numerical simulations.
% \end{enumerate}

% {\color{red}TODO for analysis:

% \begin{itemize}
%     \item extend ANIL to noisy case - done besides high probability upper bound on $\|\mathbf{w}_t\|_2$
%     \item extend MAML to finite-sample, noisy case
% \end{itemize}}

% Motivation for linear setting: Wide neural networks evolve as linear models
% under gradient descent. (Lee et al., NeurIPS 2019) " further showed that a network evolves as a linear model in the infinite width limit
% when trained on certain losses under gradient descent." (kernel regime)
% mathematically tractable





% This pattern of analysis holds for all cases -- population and finite-sample, First 


% \begin{rem}
% This is where {\em task diversity} plays a crucial role: the more diverse that the $\mathbf{w}_{\ast,i}$'s are, the more diverse (better conditioned) that the $\mathbf{w}_{t,i}$'s are due to the inner loop update. If instead there was no inner loop update, i.e. $\mathbf{B}_{t+1} = \mathbf{B}_t(\mathbf{I}_k - \beta \mathbf{w}_t \mathbf{w}_t^\top) + \mathbf{B}_\ast\left(\frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top$, then we would not be able to learn $\mathbf{B}_\ast$ since the column space of $\mathbf{B}_{t+1}$ only becomes closer to the column space of $\mathbf{B}_{\ast}$ in one direction on each iteration, so there is no reason why all $k$ directions would be learned.
% \end{rem}

\begin{table}[t]
\vskip -0.1in
\caption{Summary of results. $n$ is the number of tasks per batch, $d$ is the ambient data dimension, $k$ is the dimension of the representation, and $\kappa_\ast$ is a measure of task diversity. $\natural$ denotes that FO-MAML further requires the norm of the average ground-truth head sampled on each iteration is $O(\kappa_{\ast,\max})^{-3}$. $\dagger$ indicates that the FS methods converge to a neighborhood of the ground-truth.}
\label{sample-table}
\vspace{-3mm}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\toprule
Algorithm(s) & $\!\!$Samples/task$\!\!$ & $\!\!\dist_0$ & Rate \\
\midrule
Exact MAML  & $\infty$ & $O(\kappa_{\ast}^{-1.5})$ & $\log(1/\epsilon)$    \\
FO-MAML & $\infty$  & $O(\kappa_{\ast}^{-1})^\natural$ & $\log(1/\epsilon)$   \\
FO,Exact ANIL    & $\infty$   & $O(1)$ & $\log(1/\epsilon)$  \\
FO-ANIL    &  $\!\tilde{\Omega}(k\!+\!\tfrac{d}{n})$  & $O(1)$ & $\log(1/\epsilon)^*\!$    \\
Exact-ANIL    &  $\tilde{\Omega}(k\!+\!\tfrac{k^2d}{n})$  & $O(1)$  & $\!\log(1/\epsilon)^*\!$   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vspace{-1mm}
\end{table}

\noindent \textbf{Notations.} Matrices are denoted in bold with capital letters and vectors in bold with lowercase letters. The vector of zeros in $\mathbb{R}^d$ is $\mathbf{0}_d$ and the identity matrix in $\mathbb{R}^{d\times d}$ is $\mathbf{I}_d$.  We use $\mathcal{O}^{d\times k}$ to denote the set of matrices in $\mathbb{R}^{d \times k}$ with orthonormal columns. A hat above a matrix implies the matrix belongs to this set, e.g. $\mathbf{\hat{B}}\in \mathcal{O}^{d\times k}$. Also, $\col(\mathbf{B})$ denotes the column space of $\mathbf{B}$.
% For matrices $\mathbf{X}, \mathbf{Y}$, we use $\mathbf{X} \succeq \mathbf{Y}$ to signify that $\mathbf{X} -\mathbf{Y}$ is positive semi-definite (PSD). 
 $\mathcal{N}(0, \sigma^2)$ denotes the Gaussian distribution with mean 0 and variance $\sigma^2$. $O(\cdot)$ and $\Omega(\cdot)$ hide constant factors, and $\tilde{O}(\cdot)$ and $\tilde{\Omega}(\cdot)$ hide log factors.

%do not theoretically consider MAML and 
% observes that GBML methods that only update the last layer of the network in the inner loop essentially solve the multi-task learning problem \cite{maurer2016benefit} of learning a shared representation and personalized heads. 
% Notably, \cite{lin2020learn} empirically shows that with a
% frozen head w across training, ANIL has no performance
% drop, indicating that optimizing over w in the outer loop (3)
% is insignificant.



% We also use a train-validation split, although studying this is not the focus of this paper.
% Instead we focus on whether anil and maml can learn the representation in the tr-val split setting from an optimization perspective.


 
%  gives theoretical explanation for why the zeroing trick works.

% theory of maml:
% \cite{bai2021important} \cite{collins2020does} \cite{chua2021fine}


% \begin{rem}
% [Comparison of MAML/ANIL with multi-task representation learning] 
% Our analysis shows that the diversity of the inner-loop updated heads causes representation learning. This diversity can also be achieved if separate, stateful heads are learned for each task, i.e. perform traditional multi-task representation learning. \citet{collins2021exploiting} and \citet{thekumparampil2021statistically} proved that algorithms that do this indeed learn the ground-truth linear representation
% , and \cite{} pointed out the similarity between multi-task representation learning and gradient-based meta-learning. Also explains strong performance of pre-training.
% \cite{sun2021towards} studies extent of over-parameterization necessary and analyzes method-of-moments algorithm.
% \end{rem}


% toy setting of 1d subspace learning with 2-layer linear models, and shows the
% upper bounds of their sample complexity are of the same
% order.
% Even more recently, \cite{saunshi2021representation} show that the train-validation data split is necessary for representation learning from the statistical perspective for MTL.

%  \citet{fallah2019convergence,wang2020globalb, wang2020global}
% all studied the global convergence of MAML.
% \citet{collins2020does} explored the benefit of MAML's inner loop in settings in which there may not exist a common representation among tasks. 




%https://arxiv.org/pdf/2008.02447.pdf interesting paper but not relevant







==> Introduction.tex <==
\section{Introduction} \label{sec:intro}


%% Deep learning models are effective at solving certain tasks with ample data and computational resources for training. Yet these costly training procedures are inapplicable to many realistic multi-task settings in which models must rapidly adapt to new tasks on the fly, rather than re-train from scratch on every new task. To train adaptable models,  we can aim to leverage the fact that tasks in multi-task settings often share useful information. In many classification and regression problems, this information is a shared set of features of the data from different tasks which are most relevant to each data point's label. Therefore, 
A widely popular approach to achieve fast adaptation in multi-task learning settings 
is to learn a representation that extracts the important features shared across tasks
\cite{maurer2016benefit}. However, our understanding of {\em how} multi-task representation learning should be done and {\em why} certain methods work well is still nascent. 


% However, little is formally known about {\em how} representation learning should be done or {\em why} certain methods work well.% Most notably, 


Recently, a paradigm known as {\em meta-learning} has emerged as a powerful means of learning multi-task representations. This was sparked in large part by the introduction of Model-Agnostic Meta-Learning (MAML) \citep{finn2017model}, 
which achieved impressive results in few-shot image classification and reinforcement learning scenarios, and led to a series of related  gradient-based meta-learning (GBML) methods
\citep{raghu2019rapid,nichol2018reptile,antoniou2018train, hospedales2020meta}.
% A particularly illuminating example of this is in the case of gradient-based meta-learning (GBML) methods. 
% Ostensibly, these methods have nothing to do with representation learning:
Surprisingly, MAML does not explicitly try to learn a useful representation; instead,
it aims to find a good initialization for a small number of task-specific gradient descent steps, agnostic of whether the learning model contains a representation. 
% Yet empirical studies have attributed the fast adaptability of the nerual networks learned by MAML and its related methods to the theory that they consist of a high-quality representation applicable across tasks.
% Yet MAML has achieved impressive empirical successes in learning fast-adapting neural networks
%such as few-shot image classification and meta-reinforcement learning 
% \citep{finn2017model,antoniou2018train}, and further empirical studies have attributed their success to representation learning \cite{raghu2019rapid}. 
Nevertheless, \citet{raghu2019rapid} empirically argued that MAML's impressive performance on neural networks is likely due to its tendency to learn a shared representation across tasks. To make this argument, they noticed that MAML's representation does not change significantly when adapted to each task. Moreover, they showed that a modified version of MAML that freezes the representation during local adaptation, known as the Almost-No-Inner-Loop algorithm (ANIL), typically performs at least as well as MAML on few-shot image classification tasks. Yet it is still not well understood why these algorithms %general purpose algorithms like MAML 
that search for a good initialization for gradient descent should find useful a global representation among tasks.
% These methods aim to ``learn to learn'', i.e. meta-learn, by finding a model that can quickly learn new tasks via only a few steps of stochastic gradient descent (SGD). 
% Notably, there is  no explicit intention by these methods to learn a strong representation, making their representation learning capabilities all the more mysterious.
% an explanation for {why} optimizing an objective that rewards good initializations for gradient descent seems to lead to strong representations remains elusive.  - in particular, it has  not been shown whether MAML, or even ANIL, learn high-quality representations. 
Thus, in this paper, we aim to address the following questions:
% Nevertheless, a rigorous theoretical understanding of why these algorithms perform well in practice has remained elusive.  To bridge this gap, here we study the following question:

\vspace{-1mm}
\begin{quote}
\em{Do MAML and ANIL provably learn high-quality representations? If so, why?}
\end{quote}
\vspace{-1mm}

% In the most ubiquitous GBML method, model-agnostic meta-learning (MAML), the entire model, including the representation, is adapted via SGD to an incoming task, meaning that there is no direct intention to learn a shared representation across tasks. However, recent empirical results due to \cite{raghu2019rapid} showed that the representation does not change very much during the task-specific adaptation phase of MAML, and that the performance of MAML can be matched by an algorithm that holds the representation fixed across tasks, and only executes task-specific adaptation for the predictor, known as almost-no-inner loop (ANIL). Indeed, this evidence suggests that the key to MAML is that it learns an effective shared representation.
% However, the inner workings of GBML methods remain mysterious from the theoretical perspective. It remains to be proven whether GBML in fact learns good representations, and, more importantly, {\em how} it does so. 

% However, the reasons for such 


% aim to extract the common information among the tasks without formulating the information as a representation. Instead, GBML methods 
% aim to learn an {\em initialization} for a small number of steps of stochastic gradient descent (SGD). In other words, the initial model should contain shared information across the tasks that enables strong performance on a new task after only a few steps of fine-tuning. 
% Meta-learning aims to develop rapidly adaptable models for multi-task settings by extracting this common information from the tasks.
% In gradient-based meta-learning (GBML), this common information is formulated as an initialization for a small number of steps of stochastic gradient descent (SGD). In other words, the initial model should contain some shared information across the tasks that enables strong performance on a new task after only a few steps of fine-tuning. 

%  GBML methods find such an initial model by executing an episodic meta-training procedure, where in each episode, the current initial model is locally adapted to the sampled task in the so-called inner loop, then  updated based on the performance of the adapted models in the outer loop. This episodic procedure mimics the realistic few-shot learning evaluation procedure that considers model performance after a few steps of SGD with few samples for a new task. 
 
 
 
%  A natural explanation for this success is that GBML somehow learns a good representation for downstream tasks. Indeed, this explanation has been substantiated by plentiful empirical evidence. For example, \cite{raghu2019rapid}...
 

%  Once we understand how GBML methods learn good representations, we can leverage these properties to develop more effective and efficient meta-learning and representation learning algorithms more broadly, as we seek to harness the power of neural networks to extract useful features from increasingly high-dimensional data.
% A rigorous understanding of how GBML methods learn effective representations is important not only in the contexts of meta- and few-shot learning, but also for representation learning more broadly, as we seek to harness the power of neural networks to extract useful features from increasingly high-dimensional data. 

To answer these questions we consider the multi-task linear representation learning setting \citep{maurer2016benefit,tripuraneni2020provable,du2020fewshot} in which each task is a noisy linear regression problem in $\mathbb{R}^d$ with optimal solution lying in a shared $k$-dimensional subspace, where $k \ll d$. The learning model is a two-layer linear network consisting of a representation (the first layer of the model) and head {(the last layer)}. {The goal is to learn a representation that projects} data onto the shared subspace so as to reduce the number of samples needed to find the optimal regressor for a new task from $\Omega(d)$ to $\Omega(k)$.
% We show that the answer to the first question is yes in a multi-task linear representation learning setting.
% in which the learning model is a two-layer linear network.
% considered in \citep{maurer2016benefit,tripuraneni2020provable,du2020fewshot}.
% {\color{blue} Although this setting is simple,  many recent works have shown that the dynamics of deep networks can be explained by studying linear models, and even in this linear case it is not known whether MAML and ANIL can learn accurate representations.}

\textbf{Main contributions}.
{\em We prove, for the first time, that both MAML and ANIL, as well their first-order approximations, are capable of representation learning and recover the ground-truth subspace in this setting.}
    % Specifically, we consider a well-known setting in which 
    % we prove  that MAML and ANIL,
    % two ubiquitous GBML methods, Model-Agnostic Meta-Learning (MAML) \cite{finn2017model} and the Almost-No-Inner-Loop method (ANIL) \cite{raghu2019rapid}, 
    % as well as their first-order approximations, recover the low-dimensional subspace in which the optimal regressors for linear regression tasks lie. Learning this subspace, i.e. the ground-truth representation, reduces the sample complexity required to solve a new task from the environment, but doing so is non-trivial, as there are infinitely many possible subspaces. Indeed, running standard gradient descent to minimize the average loss across tasks in this environment does not recover the ground-truth subspace. In contrast, our analysis reveals that ANIL and MAML's distinctive inner loop updates for the last layer of the learning model are critical to their ability to recover the ground-truth representation. 
% For example, 
% Here each task 
% % in this 
% % % The $i$-th task in this 
% % setting 
% is a noisy linear regression problem.
% % with data generated by a ground-truth regressor $\boldsymbol{\theta}_{\ast,i} \in \mathbb{R}^d$. 
% To account for the advantage of representation learning, we assume that all ground-truth regressors belong to the same low-dimensional subspace. 
% In other words, there exists a representation that projects data to this low-dimensional space and preserves all the information needed to predict the data's label.
% If we  know this representation, or equivalently, know the subspace, then we can reduce the number of samples needed to solve a new task by projecting the task's data onto the subspace.
% % can learn a representation that projects the data to this subspace, then we will reduce the dimension of the problem and thereby the number of samples needed to solve a new task. 
% %#$k$-dimensional subspace of $\mathbb{R}^d$.
% % which is equal to the column space of an orthogonal matrix $\mathbf{B}_\ast$. 
% can learn a representation that projects the data to this subspace, then we will reduce the dimension of the problem and thereby the number of samples needed to solve a new task. 
%#$k$-dimensional subspace of $\mathbb{R}^d$.
% which is equal to the column space of an orthogonal matrix $\mathbf{B}_\ast$. 
Our analysis reveals that MAML and ANIL's distinctive adaptation updates for the last layer of the learning model are critical to their recovery of the ground-truth representation. 
Figure 1 visualizes this observation: all meta-learning approaches (Exact ANIL, MAML, and their first-order (FO) versions that ignore second-order derivatives) approach the ground truth exponentially fast, while a non-meta learning baseline of average loss minimization {empirically} fails to recover the ground-truth. We show that the inner loop updates of the head exploit \textit{task diversity} to make the outer loop updates bring the representation  closer to the ground-truth.
% - the more diverse the tasks, the faster the exponential rate of convergence. 
 However, MAML's inner loop updates for the representation can inhibit this behavior, thus, our results for MAML require an initialization with error {\em related to task diversity}, whereas ANIL requires only {\em constant} error. We also show that ANIL learns the ground-truth representation with only $\tilde{O}(\tfrac{k^3d}{n}+k^3)\ll d$ samples per task, demonstrating that ANIL's representation learning is {\em sample-efficient}.

% Additionally, our results require a more 

% analysis exposes why MAML's inner loop updates for the representation {\em do not contribute to representation learning} - and in fact, they necessitate  a more accurate initialization compared to ANIL. 

% that when running ANIL and MAML and their first-order analogues over a two-layer linear network, where the first layer is a low-dimensional projection,
% the model class consisting of a representation 
% $\mathbf{B} \in \mathbb{R}^{d\times k}$ and a head $\mathbf{w} \in \mathbb{R}^k$, 
%  Moreover, standard risk minimization without ANIL and MAML's distinctive inner loop updates fails to recover the ground-truth subspace. 
\begin{figure}[t]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.91\columnwidth]{anilmamlintro12.pdf}
% anil_fs_min_alpha1.png
}
\vspace{-2mm}
% \caption{ }
\caption{Distance of learned representation from the ground-truth for ANIL, MAML and average risk minimization run on task population losses in multi-task linear representation learning setting.}
\vspace{-8mm}
\label{fig:intro}
\end{center}
\end{figure}


\textbf{Related work.} Several works have studied why 
% MAML and other 
meta-learning algorithms are effective; please see 
% we mention a subset here and provide a comprehensive discussion in 
Appendix \ref{app:related_work} for a comprehensive discussion. 
Building off \citet{raghu2019rapid}, most of these works have studied meta-learning from a representation learning perspective \cite{goldblum2020unraveling,saunshi2021representation, arnold2021maml, wang2021bridging,kao2022maml}. Among these, 
 \citet{ni2021data,bouniot2020towards,setlur2020support} and \citet{kumar2021effect} showed mixed  empirical impacts of training task diversity on model performance. Most related to our work is \citep{saunshi2020sample}, which proved that the continuous version of a first-order GBML method, Reptile \cite{nichol2018reptile}, learns a one-dimensional linear representation in a two-task setting with a specific initialization, explicit regularization, and infinite samples per task.
%  {\color{blue} Our MAML and ANIL analysis relaxes these conditions via a novel induction.}
 %wang, saunshi
Other works studied multi-task  representation learning  in the linear setting we consider from a statistical perspective \cite{maurer2016benefit,du2020fewshot,tripuraneni2020provable}. Furthermore, \citet{collins2021exploiting} and \citet{thekumparampil2021statistically} gave optimization results for gradient-based methods in this setting. 
% However, unlike MAML and ANIL's shared global head, these methods learn unique, stateful heads for
% each task, which makes it relatively easy to show how the heads capture task diversity to improve the representation.
However, the algorithms they studied are customized for the assumed low-dimensional linear representation model, which makes it relatively easy to learn the correct representation efficiently. A more challenging task is to understand how general purpose and model-agnostic meta-learning algorithms perform, such as the algorithms we study.

% , unlike  ANIL and MAML learn a shared global head.
% This appears to restrict ANIL and MAML from harnessing
% the task diversity which aids representation learning in the stateful-heads case 




% Showing that ANIL and MAML recover the ground-truth representation involves numerous technical challenges:
% {\em (i)~Shared global head}. In contrast to multi-task representation learning approaches that learn unique, stateful heads for
% each task, ANIL and MAML learn a global head.
% This appears to restrict ANIL and MAML from harnessing
% the task diversity which has been shown to aid representation learning in the stateful-heads case \cite{collins2021exploiting, thekumparampil2021statistically}.
% % We overcome this by showing that ANIL and MAML's inner loop updates are sufficient to achieve diversity of the heads. 
%  {\em (ii) Complicated updates.} ANIL and MAML's inner loop updates cause the outer loop updates to have an overwhelming number of terms even in simple linear settings, requiring prior works to use a symbolic toolbox for analysis \cite{arnold2021maml}.   {\em (iii) Control of parameter norms.} Neither ANIL nor MAML allows for normalization on each iteration nor explicit regularization of the objective function, yet still the energy in the representation  and head  must be controlled. {\em  (iv) Finite samples.} The above challenges exist even with infinite samples per task, and are only accentuated in the finite-sample case. To obtain practical results, we must show that ANIL and MAML can learn the representation with only $o(d)$ samples per task.
%  Despite these challenges, we show the following results (see Table~\ref{sample-table} for more details):

% % If ANIL and MAML learned a unique, stateful head $\mathbf{w}_i$ for each task, as in alternate multi-task learning \cite{} and pre-training \cite{} approaches, then the linear representation learning problem would reduce to a low-rank matrix sensing problem for which standard algorithms have been shown to find the optimal solution \cite{collins2021exploiting, thekumparampil2021statistically}. Key to these analyses is the idea that the task-unique heads satisfy some notion of diversity, which causes the representation to move towards the ground-truth. However, learning separate heads may not be tractable in settings with many tasks, so 


% ground-truth representation $\mathbf{B}_\ast\in \mathbb{R}^{d\times k}$ and a task-specific head $\mathbf{w}_{\ast,i} \in \mathbb{R}^{k}$, where $k\ll d$. The implicit goal is to recover the low-dimensional column space of $\mathbf{B}_\ast$ by learning a two-layer linear network consisting of a representation $\mathbf{B} \in \mathbb{R}^{d\times k}$ (first layer)  and a head  $\mathbf{w}\in \mathbb{R}^{k}$ (second layer). 
% Although this two-layer linear setting is simplified compared to deep neural networks, many recent works have shown that the dynamics of deep networks can be explained by studying linear models. Moreover, our analysis of this setting explains numerous phenomenon observed in regards to MAML and ANIL's behavior on deep networks.

% , since all of the task-optimal solutions lie in this low-dimensional space.
% The simulations in Figure 1 show that both ANIL and MAML indeed recover $\col(\mathbf{B}_\ast)$ up to statistical accuracy with random initialization and only one step of inner loop task-specific adaptation as long as the tasks are sufficiently diverse. 

% Even in this simple setting, it is impressive that ANIL and MAML learn the desired representation, because the closely related method that lacks an inner loop for the heads does not.
% . These results are shown in Figure \ref{fig:11}.
% ANIL and MAML attempt to learn a two-layer linear network consisting of a representation $\mathbf{B} \in \mathbb{R}^{d\times k}$ and a head (final layer) $\mathbf{w}\in \mathbb{R}^{k}$ in this setting,  where $k$ is the dimension of the data and $d \gg k$ is the ambient dimension of the data. 

% Simulations for this setting show that indeed MAML and ANIL learn the ground-truth representation
% However, even in this simple setting, prior results have not shown whether ANIL and/or MAML recover the ground-truth representation $\mathbf{B}_\ast$ with any number of samples. 
% Until now, no one has proven that either ANIL or MAML recover the ground-truth representation in this (or any other) setting, as doing so in this case requires overcoming numerous technical challenges: 

% The simulations in Figure 1 show that both ANIL and MAML indeed recover $\col(\mathbf{B}_\ast)$ in the multi-task linear representation learning setting up to statistical accuracy with random initialization and only one step of inner loop task-specific adaptation as long as the tasks are sufficiently diverse. 
% Yet even in this simple setting, proving that ANIL and MAML recover the ground-truth representation requires overcoming numerous technical challenges: 



% As a result, we must show that the ANIL and MAML heads updated post-inner loop from the global initialization are diverse.




% (ii) {\em Landscape analysis does not suffice.} A landscape analysis does not suffice because there exist stationary points whose representation does not agree with the ground-truth (for ANIL, note that any $\mathbf{B}\mathbf{w}$ s.t. $\sum_{i=1}^n (\mathbf{B}\mathbf{w} - \mathbf{B}_\ast\mathbf{w}_{\ast,i})(\mathbf{B}\mathbf{w} - \mathbf{B}_\ast\mathbf{w}_{\ast,i})^\top = \mathbf{0}$ and $\sum_{i=1}^n \mathbf{B}\mathbf{w} - \mathbf{B}_\ast\mathbf{w}_{\ast,i} = \mathbf{0}$ is stationary //// but there are no such points////), and the objectives are non-convex, so there is no guarantee to reach a global minimum.
% Also, first-order methods perform nearly as well as the exact versions of the algorithms, even though the objective that these methods minimize is unknown.

% Instead, we must study the dynamics of the algorithms.

% Moreover, these terms may increase on each iteration, with the amount of increase depending on the size of other variables at that time. 



% train a model on many meta-training tasks with an objective that  penalizes the loss of the  model after it has been updated with a small number of task-specific gradient steps with a small number of samples, which is known as the inner loop. 
% This meta-training procedure mimics the typical few-shot learning evaluation procedure, in which the model is allowed to take a small number of gradient steps with few samples in order to learn a new task.
% The task-specific gradient steps are known as the {\em inner loop}, while the refinement of the initial model based on the results of the inner loop is known as the {\em outer loop}.

% From an empirical perspective,
% \citet{raghu2019rapid} showed that model-agnostic meta-learning (MAML), the foundational GBML method, often learns a static set of features during meta-training. They also introduced a modified version of MAML, called the Almost-No-Inner Loop (ANIL) algorithm, that only adapts the final layer of the network in the inner loop, instead of the full model as MAML does. They showed that this method typically matches and sometimes even exceeds the few-shot learning performance of MAML. These observations  suggest that the key to MAML (and ANIL) is that it learns a high-quality global feature representation, one that does not need to be locally adapted to each task. Intuitively, representation learning boosts few-shot learning performance by reducing the number of parameters that need to be updated to learn a new task.

% posed two hypotheses to explain the success of model-agnostic meta-learning (MAML) \citep{finn2017model}, the foundational GBML method: 
% {\em feature reuse} and {\em rapid learning}. According to feature reuse, MAML learns a set of reusable features, i.e. a shared representation, across tasks, and essentially only modifies the last layer of a model to adapt to a new task. In contrast, rapid learning posits that MAML succeeds because it learns a model well-suited for full adaptation to a new task, meaning that even the features change significantly during task-specific adaptation. 
% Their experiments suggest that the latter hypothesis, feature reuse, is the dominant explanation for the success of MAML in neural networks, as they found that the representation layers of networks trained by MAML do not change much when adapting to a new task. Moreover, they showed that a modified version of MAML in which only the last layer is updated in the inner loop, which they call the Almost-No-Inner Loop (ANIL) algorithm, matches and sometimes even exceeds the performance of MAML.

% Nevertheless,
% little is known theoretically about the quality of the representations that GBML methods learn, and if they indeed learn high-quality representations, {\em how} they do so. A rigorous understanding of how MAML and ANIL learn effective representations is important not only in the contexts of meta- and few-shot learning, but also for representation learning more broadly, as we seek to harness the power of neural networks to extract useful features from increasingly high-dimensional data. To study the representation learning abilities of GBML, we work with the multi-task linear representation learning setting considered in \cite{maurer2016benefit,tripuraneni2020provable,du2020fewshot}. Namely, we consider that ANIL and MAML attempt to learn a two-layer linear network consisting of a representation $\mathbf{B} \in \mathbb{R}^{d\times k}$ and a head (final layer) $\mathbf{w}\in \mathbb{R}^{k}$, where $k$ is the dimension of the data and $d \gg k$ is the ambient dimension of the data. The $i$-th task is a noisy linear regression problem with data  generated by a universal ground-truth representation $\mathbf{B}_\ast\in \mathbb{R}^{d\times k}$ and a task-specific head $\mathbf{w}_{\ast,i} \in \mathbb{R}^{k}$. Even in this simple setting, prior results have not shown whether ANIL and and MAML recover the ground-truth representation $\mathbf{B}_\ast$ with any number of samples. Doing so requires overcoming numerous technical challenges: (i) 
% Technical challenges:
% - the main challenge is that people have not shown why maml or anil work
% - discrete gradient steps
% - characterizing sample complexity
% - showing B stays well-conditioned without normalization
% - showing why task diversity matters
% - learning a single head, not personalized heads like in recent papers


% This is especially important as representation learning  becomes increasingly important for 

% \textbf{Contributions.} 


% \textbf{ANIL - } Both Exact ANIL and its first-order approximation FO-ANIL converge {\em exponentially fast to the ground-truth subspace with efficient sample complexity} as long as the initialization has constant error and  there is task diversity. 
% Specifically, the ground-truth heads for the tasks sampled on each round {\em must span $\mathbb{R}^k$}. 
% Moreover, the more diverse, or evenly spread, that the sampled ground-truth heads are on average, the {\em faster the exponential rate of convergence}.

% \textbf{MAML -} Exact and FO-MAML also converge {\em exponentially fast to the ground-truth subspace} but require more a stringent requirement on the initialization: the initial error must be smaller with less task diversity. {\em The less diverse the tasks are, the more accurate the initialization needs to be}. Moreover, for FO-MAML, is it further required that  average of the ground-truth heads sampled on each iteration is {\em concentrated around zero}. These extra conditions suggest that MAML's distinctive inner loop updates for the representation are unnecessary and even potentially harmful to representation learning. 

% All results are given for both population and finite-sample cases, and verified by numerical simulations.

% we prove that MAML and ANIL learn the ground-truth representation 
% in a well-known linear multi-task representation learning setting with two-layer linear neural networks 
% by exposing the benefit of task diversity. Our contributions are summarized as follows:
% We show the linear convergence of both algorithms to the ground-truth representation with information-theoretically tight sample complexities. In particular, we prove that only $O(k^2)$ samples are required for the inner loop updates for the last layer, where $k$ is the dimension of the representation and is assumed to be small, helping to formally explain the accuracy of ANIL in few-shot learning scenarios. We further show that the inner loop updates for the last layer are critical to representation learning, as without them (standard training) we would not be able to learn the representation. Moreover, the inner loop updates for the representation do not seem to provide any representation learning benefit, and may even inhibit representation learning. 
% % since our upper bound on the convergence rate is smaller and less restrictive for ANIL than for MAML. 
% We verify these results  through extensive numerical simulations.

% {\em another option for intuition: look at ANIL loss: for appropriate step size, $\mathbf{B}$ can only minimize it if if shares column space with $\mathbf{B}_\ast$}


% insert equation for update of B $\mathbf{G}_{\text{reg}}(\mathbf{B}_t)$, where $\mathbf{G}_{\text{reg}}(\mathbf{B}_t)$ is the gradient of a regularization term that encourages $\mathbf{B}_t$ to stay well-conditioned.




% two (mutually exclusive?) benefits: dimensionality reduction and generalization via overparameterization. We focus on dimensionality reduction



% {\color{red}
% Current status 11/7:
% \begin{itemize}
%     \item We have linear convergence result for ANIL and FO-ANIL without regularization in the population case.
%     \item We have linear convergence result for MAML (without regularization) and FO-MAML (without regularization and means of heads close to zero) in the population case.
%     % \item In the finite-sample case, I am stuck on how to show that $\|\mathbf{w}_t\|$ stays bounded, since the finite-sample errors from each iteration are not summable.
%     % \item For FO-MAML, we have linear convergence in the population case  when the mean of the ground-truth heads is small. Empirically, the mean must be very close to zero.
%     % \item For (exact) MAML, empirically, there is linear convergence as long as the norm of the mean of the ground-truth heads is less than a constant. But, I am stuck on how to show that $\|\mathbf{w}_t\|$ stays bounded, because mathematically it may increase by a constant on every round. Unlike for ANIL, we cannot use that $\|\alpha\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k\|_2$ is going to zero, because the upper bound on $\|\alpha\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}_k\|_2$ includes a term with only constants and $\|\mathbf{w}_t\|_2$.
% \end{itemize}
% Please see Appendix for proofs.
% }
% We study whether ANIL and MAML can learn accurate low-dimensional representations in the multi-task linear representation learning setting. Our analysis makes the following contributions:

% \textbf{Provable representation learning abilities of ANIL and MAML.} We prove, for the first time, that ANIL and MAML recover the ground-truth representation up to the statistical accuracy in the realizable linear representation learning setting. Moreover, we show that they do so at a linear rate. 
% These results provide rigorous theoretical justification for the representation learning benefits of ANIL and MAML that have been observed empirically in recent works \cite{finn2017model,raghu2019rapid}.
% % Our analysis overcomes numerous technical challenges, including showing that the learned representation remains well-conditioned and  the learned head is close to zero.

% \textbf{Importance of Task Diversity/ Importance of inner loop head updates.} 
% Recent works have highlighted the role of task diversity in enabling representation learning in generic multi-task settings from a statistical perspective \cite{tripuraneni2020provable, du2020fewshot} as well as empirically \cite{ni2021data}. Our analysis helps to complete the picture by showing that the dynamics of of two ubiquitous meta-learning algorithms critically leverage task diversity to learn the ground-truth representation.

% \textbf{Lack of gain of MAML over ANIL.} While our analysis highlights that task diversity is critical to representation learning, it also demonstrates that MAML's inner loop update for the representation is not. ANIL obtains at least as good theoretical guarantees without an inner loop update for the representation. In fact, MAML's inner loop update of the representation can even hurt in some cases, for instance, FO-MAML can only learn the representation if the ground-truth heads have mean very close to zero. Intuitively, this holds because without an inner loop for the representation, the outer loop gradient is like the gradient with respect to a certain matrix factorization problem whose solutions in $\mathbf{B}$ share column space with $\mathbf{B}_\ast$. With the inner loop update, this gradient is perturbed in a direction that may disagree with $\col({\mathbf{B}_\ast})$.
% These findings are consistent with recent empirical results showing that ANIL performs at least as well as MAML on few-shot learning benchmarks \cite{raghu2019rapid}.


% \textbf{Efficient sample complexity.}


% (v) \textit{Explanation for other empirically-observed phenomena.} Zeroing trick (formal result on this?) strong performance of multi-task representation learning/pretraining


% \textbf{Numerical Simulations.}



% \begin{enumerate}
%     \item We show that both ANIL and FO-ANIL learn a  linear representation that is $\epsilon$-close to the ground-truth representation exponentially fast, where $\epsilon = O(\frac{1}{m_{in}m_{out}})$.
%     \item We show that MAML (and FO-MAML as long as the mean of the ground-truth predictors is sufficiently close to zero) also learns an approximation of the ground-truth linear representation at an exponentially fast rate. In particular, the MAML representation is $\epsilon'$-accurate with $\epsilon' = O()$.
%     \item We verify our theoretical results with extensive numerical simulations.
% \end{enumerate}

% {\color{red}TODO for analysis:

% \begin{itemize}
%     \item extend ANIL to noisy case - done besides high probability upper bound on $\|\mathbf{w}_t\|_2$
%     \item extend MAML to finite-sample, noisy case
% \end{itemize}}

% Motivation for linear setting: Wide neural networks evolve as linear models
% under gradient descent. (Lee et al., NeurIPS 2019) " further showed that a network evolves as a linear model in the infinite width limit
% when trained on certain losses under gradient descent." (kernel regime)
% mathematically tractable





% This pattern of analysis holds for all cases -- population and finite-sample, First 


% \begin{rem}
% This is where {\em task diversity} plays a crucial role: the more diverse that the $\mathbf{w}_{\ast,i}$'s are, the more diverse (better conditioned) that the $\mathbf{w}_{t,i}$'s are due to the inner loop update. If instead there was no inner loop update, i.e. $\mathbf{B}_{t+1} = \mathbf{B}_t(\mathbf{I}_k - \beta \mathbf{w}_t \mathbf{w}_t^\top) + \mathbf{B}_\ast\left(\frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top$, then we would not be able to learn $\mathbf{B}_\ast$ since the column space of $\mathbf{B}_{t+1}$ only becomes closer to the column space of $\mathbf{B}_{\ast}$ in one direction on each iteration, so there is no reason why all $k$ directions would be learned.
% \end{rem}

% \begin{table}[t]
% \vskip -0.1in
% \caption{Summary of results. $\dist_0$ is the initial representation error, $n$ is the number of tasks per batch, $d$ is the ambient data dimension, $k$ is the dimension of the representation, and $\kappa_\ast$ is a measure of task diversity. $\natural$ denotes that FO-MAML further requires the norm of the average ground-truth head sampled on each iteration is $O(\kappa_{\ast,\max}^{-3})$. $\dagger$ indicates that the FS methods converge to a neighborhood of the ground-truth.}
% \label{sample-table}
% \vspace{-3mm}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccc}
% \toprule
% Algorithm(s) & $\!\!$Samples/task$\!\!$ & $\!\!\dist_0$ &\! Iters\! \\
% \midrule
% Exact MAML  & $\infty$ & $\!O(\kappa_{\ast}^{-1.5})\!$ & $\!\log(1/\epsilon)\!$    \\
% FO-MAML & $\infty$  & $\!O(\kappa_{\ast}^{-1})^\natural\!$ & $\log(1/\epsilon)$   \\
% FO,Exact ANIL    & $\infty$   & $O(1)$ & $\log(1/\epsilon)$  \\
% FO-ANIL    &  $\!\tilde{\Omega}(k\!+\!\tfrac{d}{n})$  & $O(1)$ & $\log(1/\epsilon)^\dagger\!$    \\
% Exact-ANIL    &  $\!\!\tilde{\Omega}(k\!+\!\tfrac{k^2d}{n})\!\!$  & $O(1)$  & $\!\log(1/\epsilon)^\dagger\!$   \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vspace{-1mm}
% \end{table}

\noindent \textbf{Notations.} We use bold capital letters for matrices and bold lowercase letters for vectors.  %The vector of zeros in $\mathbb{R}^d$ is $\mathbf{0}_d$ and the identity matrix in $\mathbb{R}^{d\times d}$ is $\mathbf{I}_d$.  
We use $\mathcal{O}^{d\times k}$ to denote the set of matrices in $\mathbb{R}^{d \times k}$ with orthonormal columns. 
A hat above a matrix, e.g. $\mathbf{\hat{B}}$, implies the matrix is a member of $\mathcal{O}^{d\times k}$. We let $\col(\mathbf{B})$ denote the column space of $\mathbf{B}$, and $\col^\perp(\mathbf{B} )$ denote its orthogonal complement.
% For matrices $\mathbf{X}, \mathbf{Y}$, we use $\mathbf{X} \succeq \mathbf{Y}$ to signify that $\mathbf{X} -\mathbf{Y}$ is positive semi-definite (PSD). 
 $\mathcal{N}(0, \sigma^2)$ denotes the Gaussian distribution with mean 0 and variance $\sigma^2$. $O(\cdot)$ and $\Omega(\cdot)$ hide constant factors, and $\tilde{O}(\cdot)$ and $\tilde{\Omega}(\cdot)$ hide constant and logarithmic factors.

%do not theoretically consider MAML and 
% observes that GBML methods that only update the last layer of the network in the inner loop essentially solve the multi-task learning problem \cite{maurer2016benefit} of learning a shared representation and personalized heads. 
% Notably, \cite{lin2020learn} empirically shows that with a
% frozen head w across training, ANIL has no performance
% drop, indicating that optimizing over w in the outer loop (3)
% is insignificant.



% We also use a train-validation split, although studying this is not the focus of this paper.
% Instead we focus on whether anil and maml can learn the representation in the tr-val split setting from an optimization perspective.


 
%  gives theoretical explanation for why the zeroing trick works.

% theory of maml:
% \cite{bai2021important} \cite{collins2020does} \cite{chua2021fine}


% \begin{rem}
% [Comparison of MAML/ANIL with multi-task representation learning] 
% Our analysis shows that the diversity of the inner-loop updated heads causes representation learning. This diversity can also be achieved if separate, stateful heads are learned for each task, i.e. perform traditional multi-task representation learning. \citet{collins2021exploiting} and \citet{thekumparampil2021statistically} proved that algorithms that do this indeed learn the ground-truth linear representation
% , and \cite{} pointed out the similarity between multi-task representation learning and gradient-based meta-learning. Also explains strong performance of pre-training.
% \cite{sun2021towards} studies extent of over-parameterization necessary and analyzes method-of-moments algorithm.
% \end{rem}


% toy setting of 1d subspace learning with 2-layer linear models, and shows the
% upper bounds of their sample complexity are of the same
% order.
% Even more recently, \cite{saunshi2021representation} show that the train-validation data split is necessary for representation learning from the statistical perspective for MTL.

%  \citet{fallah2019convergence,wang2020globalb, wang2020global}
% all studied the global convergence of MAML.
% \citet{collins2020does} explored the benefit of MAML's inner loop in settings in which there may not exist a common representation among tasks. 




%https://arxiv.org/pdf/2008.02447.pdf interesting paper but not relevant







==> MAML.tex <==
\section{MAML}

We only consider first-order updates.
The update for the representation is:
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i} \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top +   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
    &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{t}\left(\mathbf{I}_d  - \alpha\mathbf{w}_{t}\mathbf{w}_{t}^\top\right) \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top - \frac{\alpha\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast}\mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top+   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
    &= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top \right)
    +   \frac{\beta}{n}\sum_{i=1}^n ( 1- \alpha \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle) \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber 
\end{align}
where $\mathbf{w}_{t,i} = (\mathbf{I}_d - \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t)\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}= (1 - \alpha )\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$.

\subsection{Main Result}


\begin{theorem}
For $\alpha=1$, $\beta \in (0,1]$ and any $0 < c < \beta E_0 \mu_\ast^2$, if for all $t = 1,\dots,T$,
\begin{align}
   \|\mathbf{w}_t\|_2^2 &\leq \frac{1}{F}\left( -(A + (1-c)^2 D)+ (1-c)\sqrt{1 + 2 AD + (1-c)^2D}\right),
    % \frac{2 \beta L_{\ast}^2(2 - 2 \beta E_0 \mu_\ast^2+\beta L_{\ast}^2 ) + \beta L_\ast^2 \sqrt{ (Z + 2)^2 - 4 \beta^2 E_0 L_\ast^2 Z}}{4\beta E_0 \mu_\ast^2 - 2 \beta^2 E_0^2 \mu_{\ast}^4 }
\end{align}
where $A\coloneqq 1 - \beta E_0 \mu_\ast^2$, $D\coloneqq 1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  $, $F \coloneqq \beta L_\ast^2$, and the representation $\mathbf{B}_t$ is orthogonalized at the end of each outer loop, then MAML learns the representation at a linear rate with contraction factor at most $1-c$, i.e.
\begin{align}
    \dist(\mathbf{\hat{B}}_T, \mathbf{\hat{B}}_\ast) &\leq (1 - c)^{T}\dist(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast).
\end{align}
\end{theorem}


\subsection{Proof Sketch: Population Case}




\subsection{Simulations}




==> MAML_notes.tex <==
\section{MAML}

For MAML the initial head $\mathbf{w}_t$ matters for representation learning.
We only consider first-order updates.
The update for the representation is:
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i} \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top +   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
    &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{t}\left(\mathbf{I}_d  - \alpha\mathbf{w}_{t}\mathbf{w}_{t}^\top\right) \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top - \frac{\alpha\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast}\mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top+   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
    &= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top \right)
    +   \frac{\beta}{n}\sum_{i=1}^n ( 1- \alpha \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle) \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber 
\end{align}
where $\mathbf{w}_{t,i} = (\mathbf{I}_d - \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t)\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}= (1 - \alpha )\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$.

{\color{blue}
If $\alpha=1$, the perturbation term is:
\begin{align}
    \frac{\beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\rangle \mathbf{w}_{t} \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t &=  \mathbf{w}_{t}\mathbf{w}_{t}^\top \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \frac{\beta}{n}\sum_{i=1}^n(\mathbf{w}_{\ast,i}  \mathbf{w}_{\ast,i}^\top) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t
\end{align}
we need to lower bound\begin{align}
    \sigma_{\min}\left((\mathbf{I}_k - \alpha \mathbf{w}_{t}\mathbf{w}_{t}^\top)  \frac{\beta}{n}\sum_{i=1}^n(\mathbf{w}_{\ast,i}  \mathbf{w}_{\ast,i}^\top) \right) &\geq \sigma_{\min}\left(\mathbf{I}_k - \alpha \mathbf{w}_{t}\mathbf{w}_{t}^\top\right) \sigma_{\min}\left( \frac{\beta}{n}\sum_{i=1}^n(\mathbf{w}_{t,i}  \mathbf{w}_{t,i}^\top)  \right)\nonumber \\
    &\geq \sigma_{\min}\left(\mathbf{I}_k - \alpha \mathbf{w}_{t}\mathbf{w}_{t}^\top\right)\beta (\alpha^2 E_0 \mu_{\ast}^2 - 2 \alpha(1-\alpha)\|\mathbf{w}_t\|_2 L_\ast)
\nonumber \\
    &\geq (1 - \alpha \|\mathbf{w}_t\|_2^2)\beta (\alpha^2 E_0 \mu_{\ast}^2 - 2 \alpha(1-\alpha)\|\mathbf{w}_t\|_2 L_\ast)
\end{align}
% Suppose for now that $\|\mathbf{w}_t\|_2 = 1$. We can choose $\alpha$ s.t. $\phi \leq \alpha \leq 1$
% such that 
% \begin{align}
%     \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2
%     &\leq 1-(1 - \alpha)\beta (\alpha^2 E_0 \mu_\ast^2 + 2 \alpha^2 L_\ast - 2 \alpha L_\ast)
% \end{align}
% % where $\phi \coloneqq \frac{2\|\mathbf{w}_t\|_2 L_\ast + \sqrt{2\|\mathbf{w}_t\|_2 L_\ast c} + \sqrt{E_0 \mu_\ast^2 c}}{2\|\mathbf{w}_t\|_2 L_\ast +E_0 \mu_\ast^2}$
% % and $c \leq \left(\frac{E_0 \mu_\ast^2}{\sqrt{2\|\mathbf{w}_t\|_2 L_\ast } + \sqrt{E_0 \mu_\ast^2}} \right)^2$. Now, 
% Suppose $\mu_\ast^2= L_\ast^2 = \frac{1}{k}$ and $E_0 = 0.5$. Pick any constant $c \in (0,0.5)$.  Then for any $\alpha$ such that $\frac{4 \sqrt{k}+2 c}{4\sqrt{k} + 1} \leq \alpha \leq 1$, then we have 
% \begin{align}
%     \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2
%     &\leq 1-(1 - \alpha)\beta \alpha \frac{c}{k}
% \end{align}
% Experiments verify that the convergence rate decreases with $k$.

Now the question is how to control the minimum singular value of $\mathbf{R}_{t+1}$. 
We have 
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_t - \left(\frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right)  \nonumber
\end{align}
Define $\mathbf{\nabla} \coloneqq \frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top$. We have
\begin{align}
    \sigma_{\min}^2(\mathbf{R}_{t+1}) &= \sigma_{\min}(\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}) \nonumber \\
    &= \sigma_{\min}(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} - \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t} + \mathbf{\nabla}^\top \mathbf{\nabla}) \nonumber \\
    &\geq \sigma_{\min}(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t}- \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} - \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t} )% - 2 \left\|\mathbf{\hat{B}}_{t}^\top\mathbf{\nabla}  \right\|_2 \nonumber \\
    % &= 1- 2 \left\|\mathbf{\hat{B}}_{t}^\top\mathbf{\nabla}  \right\|_2 \nonumber 
\end{align}
Next, define $\mathbf{v}_{t,i} \coloneqq \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}$, and note that $\mathbf{w}_{t,i} \coloneqq (1-\alpha)\mathbf{w}_t  + \alpha \mathbf{v}_{t,i}$. Note that 
\begin{align}
    \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} 
    &= \mathbf{\hat{B}}_{t}^\top\frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top \nonumber \\
    &= \frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{w}_t - \mathbf{v}_{t,i})\mathbf{w}_{t,i}^\top \nonumber \\
    &= \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(\mathbf{w}_t - \mathbf{v}_{t,i})((1-\alpha)\mathbf{w}_t + \alpha \mathbf{v}_{t,i})^\top \nonumber \\
    &= \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)\mathbf{w}_t\mathbf{w}_t^\top  \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})\alpha\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \nonumber \\
    &\quad + \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})\alpha( \mathbf{w}_t \mathbf{v}_{t,i}^\top +  \mathbf{v}_{t,i}\mathbf{w}_t^\top ) \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i}) \mathbf{v}_{t,i}\mathbf{w}_t^\top  \nonumber
\end{align}
Making the same computation for the transposed term $\mathbf{\nabla}^\top \mathbf{\hat{B}}_{t}$ and rearranging terms yields
\begin{align}
    \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} + \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t}
    &=  \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)\mathbf{w}_t\mathbf{w}_t^\top  \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})\alpha\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)( \mathbf{w}_t \mathbf{v}_{t,i}^\top +  \mathbf{v}_{t,i}\mathbf{w}_t^\top ) \nonumber
\end{align}


We have
\begin{align}
    \left\|\mathbf{\hat{B}}_{t}^\top\mathbf{\nabla}  \right\|_2 \nonumber \\
    &=     \beta\left\|\mathbf{\hat{B}}_{t}^\top\frac{1}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top \right\|_2 \nonumber \\
    &=  \beta\left\|\frac{1}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{w}_t - \mathbf{v}_{t,i})\mathbf{w}_{t,i}^\top \right\|_2 \nonumber \\ 
    &= \beta\left\|\frac{1}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(\mathbf{w}_t - \mathbf{v}_{t,i})((1-\alpha)\mathbf{w}_t + \alpha \mathbf{v}_{t,i})^\top \right\|_2 \nonumber \\ 
    &= \beta\bigg\|\frac{1}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)\mathbf{w}_t - \mathbf{v}_{t,i})((1-\alpha)\mathbf{w}_t + \alpha \mathbf{v}_{t,i})^\top \bigg\|_2 \nonumber \\ 
\end{align}


Writing $\mathbf{B}_{t+1} = \mathbf{B}_t - \beta \nabla \dots$ as in the analysis for ANIL, the problem reduces to controlling the cross term $-\beta \mathbf{B}_t^\top \nabla \dots$. We can  show that the sum of both cross terms reduces to:
\begin{align}
    &\frac{\beta}{n}\sum_{i=1}^n 2\left(1 - 2\alpha + \alpha^2 -\alpha^2 \mathbf{w}_t^\top \mathbf{v}_i \right)\alpha(\mathbf{v}_i - \mathbf{w}_t)(\mathbf{v}_i - \mathbf{w}_t)^\top \nonumber \\
    &\quad + \left(1 - 2\alpha + \alpha^2 -\alpha^2 \mathbf{w}_t^\top \mathbf{v}_i \right)\left((\mathbf{v}_i - \mathbf{w}_t) \mathbf{w}_t^\top + \mathbf{w}_t(\mathbf{v}_i - \mathbf{w}_t)^\top \right) \\
    &= \frac{\beta}{n}\sum_{i=1}^n 2\left(1 - \alpha \right)^2\alpha(\mathbf{v}_i - \mathbf{w}_t)(\mathbf{v}_i - \mathbf{w}_t)^\top - 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i - \mathbf{w}_t)(\mathbf{v}_i - \mathbf{w}_t)^\top  \nonumber \\
    &\quad + \left(1 - \alpha  \right)^2 \left((\mathbf{v}_i - \mathbf{w}_t) \mathbf{w}_t^\top + \mathbf{w}_t(\mathbf{v}_i - \mathbf{w}_t)^\top \right)  \nonumber \\
    &\quad - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_i \left((\mathbf{v}_i - \mathbf{w}_t) \mathbf{w}_t^\top + \mathbf{w}_t(\mathbf{v}_i - \mathbf{w}_t)^\top \right) \\
    &= \frac{\beta}{n}\sum_{i=1}^n 2\left(1 - \alpha \right)^2\alpha(\mathbf{v}_i - \mathbf{w}_t)(\mathbf{v}_i - \mathbf{w}_t)^\top - 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i - \mathbf{w}_t)(\mathbf{v}_i - \mathbf{w}_t)^\top  \nonumber \\
    &\quad -2 \left(1 - \alpha  \right)^2 \mathbf{w}_t \mathbf{w}_t^\top  + \left(1 - \alpha  \right)^2 (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top)\nonumber \\
    &\quad - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) +  2\alpha^2 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{w}_t \mathbf{w}_t^\top
\end{align}
where $\mathbf{v}_i = \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}$. 

We have 

The PSD terms can be dropped (note that they are mostly rank-1, and do not have significant minimum singular value. Thus we effectively deal with:
\begin{align}
&\frac{\beta}{n}\sum_{i=1}^n  - 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i - \mathbf{w}_t)(\mathbf{v}_i - \mathbf{w}_t)^\top  \nonumber \\
    &\quad -2 \left(1 - \alpha  \right)^2 \mathbf{w}_t \mathbf{w}_t^\top  + \left(1 - \alpha  \right)^2 (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) \nonumber\\
    &\quad - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) +  \alpha^2 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{w}_t \mathbf{w}_t^\top \\
    &=\frac{\beta}{n}\sum_{i=1}^n  - 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{v}_i \mathbf{v}_i^\top  - 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{w}_t \mathbf{w}_t^\top 
    + 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{v}_i \mathbf{w}_t^\top + 2 \alpha^3 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{w}_t \mathbf{v}_i^\top \nonumber \\
    &\quad -2 \left(1 - \alpha  \right)^2 \mathbf{w}_t \mathbf{w}_t^\top  + \left(1 - \alpha  \right)^2 (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) \nonumber\\
    &\quad - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) +  \alpha^2 \mathbf{w}_t^\top \mathbf{v}_i \mathbf{w}_t \mathbf{w}_t^\top \\ 
    &=\frac{\beta}{n}\sum_{i=1}^n  - 2 \alpha^3 (\mathbf{w}_t^\top \mathbf{v}_i \mathbf{v}_i) \mathbf{v}_i^\top  
    \nonumber \\
    &\quad -2 \left(1 - \alpha  \right)^2 \mathbf{w}_t \mathbf{w}_t^\top  + \left(1 - \alpha  \right)^2 (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) \nonumber\\
    &\quad - \alpha^2 (1 - 2 \alpha) \mathbf{w}_t^\top \mathbf{v}_i (\mathbf{v}_i \mathbf{w}_t^\top +  \mathbf{w}_t \mathbf{v}_i^\top) +  \alpha^2(1-2\alpha) (\mathbf{w}_t^\top \mathbf{v}_i) \mathbf{w}_t \mathbf{w}_t^\top 
\end{align}
The bad term is the one term that does not have any $\sqrt{k}$ dependence ( $-2 (1-\alpha)^2 \mathbf{w}_t\mathbf{w}_t^\top$). But we cannot get rid of this term... this is the issue.
}

{\color{red}
Empirically, we can have 
\begin{align}
    \left\|\mathbf{I}_k -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2
    &> \sigma_{\min}(\mathbf{R}_{t+1})
\end{align}
yet still have linear convergence. So the looseness in our analysis is due to using Cauchy-Schwarz to write
\begin{align}
    \dist_{t+1} \leq \dist_t \frac{
    \left\|\mathbf{I}_k -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2}{\sigma_{\min}(\mathbf{R}_{t+1})}
\end{align}
We need to upper bound 
\begin{align}
    \left\|(\mathbf{I}_k -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top ) \mathbf{R}_{t+1}^{-1}\right\|_2
\end{align}
but we cannot use C-S. 

empirically: we cannot use triangle inequality either.
}

So the inner update step for the representation seems to hurt representation learning, since it moves energy in the update for $\mathbf{B}_{t+1}$ from $\mathbf{B}_\ast$ to $\mathbf{B}_t$ compared to ANIL. But if $\mathbf{w}_t$ is close to zero, then this perturbation is small, so we should still learn the representation.

We have 
\begin{align}
    \dist_{t+1}&\leq \dist_t \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2
\end{align}
where 
\begin{align}
    &\left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \nonumber\\
    &\leq \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|  + \left\| \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \\
    &\leq 1 - \beta (\alpha E_0 \mu_\ast^2 - (1- \alpha)) + \left\| \frac{\alpha \beta}{n}\sum_{i=1}^n \mathbf{w}_{t} ( (1-\alpha)\|\mathbf{w}_{t}\|_2^2 + \alpha \mathbf{w}_t^\top \mathbf{\hat{B}}^\top_t \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})   ((1- \alpha) \mathbf{w}_{t}^\top + \alpha \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t)  \right\|_2  \nonumber \\
    &\leq 1 - \beta (\alpha E_0 \mu_\ast^2 - (1- \alpha)) + \left\|\mathbf{w}_{t}\mathbf{w}_{t}^\top  \frac{\alpha(1- \alpha) \beta}{n}\sum_{i=1}^n ( (1-\alpha)\|\mathbf{w}_{t}\|_2^2 + \alpha \mathbf{w}_t^\top \mathbf{\hat{B}}^\top_t \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})      \right\|_2  \nonumber  \\
    &\quad + \left\| \frac{\alpha^2 \beta}{n}\sum_{i=1}^n \mathbf{w}_{t} ( (1-\alpha)\|\mathbf{w}_{t}\|_2^2 + \alpha \mathbf{w}_t^\top \mathbf{\hat{B}}^\top_t \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})   \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t  \right\|_2  \\
    &\leq 1 - \beta (\alpha E_0 \mu_\ast^2 - (1- \alpha)) + \alpha(1 - \alpha)^2 \beta \|\mathbf{w}_t\|_2^4 + \alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3 L_\ast + \alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3 L_\ast + \alpha^3 \beta \|\mathbf{w}_t\|_2^2 L_\ast^2  \\
    &= 1 -  \alpha\beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha(1 - \alpha)^2 \beta \|\mathbf{w}_t\|_2^4 + 2\alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3 L_\ast + \alpha^3 \beta \|\mathbf{w}_t\|_2^2 L_\ast^2 %\\
    % &------- \\
    % &\leq 1 - \beta (\alpha E_0 \mu_\ast - (1- \alpha)) + \alpha \beta (1-\alpha)((1-\alpha)+\alpha ) + \alpha \beta \alpha((1-\alpha) +\alpha L_\ast) \\
    % &= 1 - \beta \alpha E_0 \mu_\ast + \beta - \beta \alpha + \alpha \beta  - \alpha^2 \beta + \alpha^2 \beta - \alpha^3 \beta + \alpha^3 \beta L_\ast \\
    % &= 1 - \beta (\alpha E_0 \mu_\ast-1)  - \alpha^3 \beta (1- L_\ast) 
\end{align}
% In the best case scenario, $\mu_\ast^2 = L_\ast^2 = 1/k$.  Then
% \begin{align}
%     &\left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \\
%     &\leq 1 -  \alpha\beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha(1 - \alpha)^2 \beta \|\mathbf{w}_t\|_2^4 + 2\alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3/\sqrt{k} + \alpha^3 \beta \|\mathbf{w}_t\|_2^2/k %\\
%     % &----- \\
%     % &\leq 1 + \beta \alpha \frac{k - E_0}{k}  - \alpha^3 \beta \frac{k-1}{k} \\
%     % &= 1 + \beta \alpha \frac{k - E_0 - \alpha^2(k-1)}{k}
% \end{align}
If we  assume that $\mathbf{w}_t = \mathbf{0}$, we have
\begin{align}
    \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 
    &\leq 1 -  \alpha\beta E_0 \mu_\ast^2 + (1 - \alpha)\beta,
\end{align}
where the RHS is less than 1 for $\alpha$ close to 1. 
If we alternatively assume that $\alpha = 1$, we have
\begin{align}
     \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 
    &\leq 1 -  \beta E_0 \mu_\ast^2 + \beta\|\mathbf{w}_t\|_2^2 L_\ast^2,
\end{align}
where the RHS is less than 1 for $\|\mathbf{w}_t\|_2^2  \leq E_0 \frac{\mu_\ast^2}{L_\ast^2}$.
If $\alpha =1$ and $\mathbf{w}_t = \mathbf{0}$, we have
\begin{align}
     \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 
    &\leq 1 -  \beta E_0/\sqrt{k}
\end{align}
This makes sense because it matches the bound from ANIL with $\alpha=1$.

Next, note that we can write the MAML outer loop representation update as:
\begin{align}
    \mathbf{B}_{t+1}&= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top  \nonumber \\
    &\quad + \mathbf{\hat{B}}_{t} \left(\frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top \right)
    -   \mathbf{\hat{B}}_{\ast}\frac{\alpha \beta}{n}\sum_{i=1}^n  \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle  \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top   \\
    &= \mathbf{B}_{ANIL} + \mathbf{B}'
\end{align}
where $\mathbf{B}_{ANIL} \coloneqq \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top$ and $\mathbf{B}' \coloneqq  \frac{\alpha \beta}{n}\sum_{i=1}^n  \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle (\mathbf{\hat{B}}_{t}\mathbf{w}_{t} -  \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top$.
    From earlier analysis, we know that
        $\sigma_{\min}(\mathbf{B}_{ANIL}) \geq 1$,
    so we have 
\begin{align}
    \sigma_{\min}^2(\mathbf{R}_{t+1}) &= \sigma_{\min}(\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}) \nonumber \\
    &=\sigma_{\min}(\mathbf{B}_{ANIL}^\top \mathbf{B}_{ANIL} + \mathbf{B}_{ANIL}^\top \mathbf{B}' + (\mathbf{B}')^\top \mathbf{B}_{ANIL} + (\mathbf{B}')^\top \mathbf{B}') \nonumber \\
    &\geq  \sigma_{\min}^2(\mathbf{B}_{ANIL}) - 2 \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}') +  \sigma_{\min}^2( \mathbf{B}') \nonumber \\
    &\geq 1 - 2 \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}') 
\end{align}
Note that $\sigma_{\min}^2( \mathbf{B}')$ may be zero, so we drop it. If $\mathbf{w}_t = \mathbf{0}$, we have $\sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}') = 0$, so we recover the convergence rate from ANIL (of $1 - \beta E_0 \mu_\ast^2$). Otherwise, we have  
\begin{align}
    \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}')  &\leq  \sigma_{\max}(\mathbf{B}_{ANIL}^\top) \sigma_{\max}(\mathbf{B}')  \nonumber \\
    &\leq (1 - \alpha \beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha \beta L_\ast^2 + (1-\alpha)\beta L_\ast \|\mathbf{w}_t\|_2 ) \sigma_{\max}(\mathbf{B}') \nonumber \\
    &\leq \Big(1 - \alpha \beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha \beta L_\ast^2 + (1-\alpha)\beta L_\ast \|\mathbf{w}_t\|_2 \Big) \nonumber \\
    &\quad \times \alpha \beta\Big((1-\alpha)^2 \|\mathbf{w}_t\|_2^4  + 2 \alpha(1-\alpha)\|\mathbf{w}_t\|_2^3 L_\ast + \alpha^2 \|\mathbf{w}_t\|_2^2 L_\ast^2 \Big) .
\end{align}
Now, if $\alpha=1$, we have
\begin{align}
    \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}')  
    &\leq \Big(1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  \Big)  \beta  \|\mathbf{w}_t\|_2^2 L_\ast^2 
\end{align}
{
so we obtain
\begin{align}
    \dist_{t+1}&\leq \dist_t \frac{1 -  \beta E_0 \mu_\ast^2 + \beta\|\mathbf{w}_t\|_2^2 L_\ast^2}{\sqrt{1 - 2\Big(1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  \Big)  \beta   \|\mathbf{w}_t\|_2^2 L_\ast^2 }} 
\end{align}
where the contraction factor is less than $1-c$ if and only if
\begin{align}
    \|\mathbf{w}_t\|_2^2 &\leq \frac{1}{F}\left( -(A + (1-c)^2 D)+ (1-c)\sqrt{1 + 2 AD + (1-c)^2D}\right) \label{88}
    % \frac{2 \beta L_{\ast}^2(2 - 2 \beta E_0 \mu_\ast^2+\beta L_{\ast}^2 ) + \beta L_\ast^2 \sqrt{ (Z + 2)^2 - 4 \beta^2 E_0 L_\ast^2 Z}}{4\beta E_0 \mu_\ast^2 - 2 \beta^2 E_0^2 \mu_{\ast}^4 }
\end{align}
where $A\coloneqq 1 - \beta E_0 \mu_\ast^2$, $D\coloneqq 1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  $, $F \coloneqq \beta L_\ast^2$. 
Note that 
$1 + 2 A D + (1-c)^2 D^2 \geq 0$ for all $\beta \in (0,1]$, so we do not have to worry about a complex square root.  
The RHS of \eqref{88} is positive for all $c>0$ such that $
    (1-c)^2 > {A^2}$, i.e., $0< c < \beta E_0 \mu_\ast^2$. This leads to the following theorem.
% $< \beta E_0 \mu_\ast^2$. So this result says that for any $c < \beta E_0 \mu_\ast^2$, there exists some $\delta > 0$ such that as long as $\|\mathbf{w}_t\|_2^2 \leq \delta$ for all $t$, we have linear convergence of the representation with rate $1 - c$ for all $t$.
}

\begin{thm}
For $\alpha=1$, $\beta \in (0,1]$ and any $0 < c < \beta E_0 \mu_\ast^2$, if for all $t = 1,\dots,T$,
\begin{align}
   \|\mathbf{w}_t\|_2^2 &\leq \frac{1}{F}\left( -(A + (1-c)^2 D)+ (1-c)\sqrt{1 + 2 AD + (1-c)^2D}\right),
    % \frac{2 \beta L_{\ast}^2(2 - 2 \beta E_0 \mu_\ast^2+\beta L_{\ast}^2 ) + \beta L_\ast^2 \sqrt{ (Z + 2)^2 - 4 \beta^2 E_0 L_\ast^2 Z}}{4\beta E_0 \mu_\ast^2 - 2 \beta^2 E_0^2 \mu_{\ast}^4 }
\end{align}
where $A\coloneqq 1 - \beta E_0 \mu_\ast^2$, $D\coloneqq 1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  $, $F \coloneqq \beta L_\ast^2$, and the representation $\mathbf{B}_t$ is orthogonalized at the end of each outer loop, then MAML learns the representation at a linear rate with contraction factor at most $1-c$, i.e.
\begin{align}
    \dist(\mathbf{\hat{B}}_T, \mathbf{\hat{B}}_\ast) &\leq (1 - c)^{T}\dist(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast).
\end{align}
\end{thm}

Intuitively: in the outer loop update, the heads serve to remove energy from the representation resulting from the inner loop and add energy to $\mathbf{B}_\ast$. But if the representation is updated during the inner loop, then it no longer contains enough energy from $\mathbf{B}_t$ such that the energy in $\mathbf{B}_t$ can be reduced by the heads in the outer update. However, if we send $\mathbf{w}_t$ to zero, then the inner loop gradient of the representation goes to zero, so effectively we remove the inner loop update step for the representation.


Experiments:
\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.6\columnwidth]{anil_vs_maml20050.png}}
\vspace{-0mm}
\caption{Average PA distance over 20 trials. $m_{out} = 200, m_{in} = 50, d=10, n=20, k = 3$. ANIL and MAML-0 learn the representation faster than MAML, as expected.}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.6\columnwidth]{anil_vs_maml400100.png}}
\vspace{-0mm}
\caption{Average PA distance over 20 trials. $m_{out} = 400, m_{in} = 100, d=10, n=20, k = 3$.}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.6\columnwidth]{anil_vs_maml2000500.png}}
\vspace{-0mm}
\caption{Average PA distance over 20 trials. $m_{out} = 2000, m_{in} = 500, d=10, n=20, k = 3$.}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}


Can we show that $\|\mathbf{w}_t\|_2$ is naturally small?

Empirically:
\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.6\columnwidth]{mamlnorm.png}}
\vspace{-0mm}
\caption{Average $\|\mathbf{w}_t\|_2$ for MAML over 20 trials. $m_{out} = 400, m_{in} = 400, d=10, n=20, k = 3$.}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{align}
    \mathbf{w}_{t+1} &= \mathbf{w}_t - \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{w}_{t,i} +\frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{B}_{\ast} \mathbf{w}_{\ast,i} \\
    &= \mathbf{w}_t - \frac{\beta}{n}\sum_{i=1}^n (1 - \alpha)\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{w}_{t} - \alpha \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} +\frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \\
    &= \mathbf{w}_t - \frac{\beta}{n}\sum_{i=1}^n (1 - \alpha)\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{w}_{t}  +\frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top( \mathbf{I}_k - \alpha \mathbf{B}_{t,i} \mathbf{\hat{B}}_{t}^\top) \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} 
\end{align}
where $\mathbf{B}_{t,i} = \mathbf{\hat{B}}_{t}(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top) + \alpha \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i}\mathbf{w}_t^\top$. Thus \begin{align}
    \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} &= \mathbf{I}_k - 2\alpha \mathbf{w}_t \mathbf{w}_t^\top + \alpha^2 \|\mathbf{w}_t\|_2^2 \mathbf{w}_t \mathbf{w}_t^\top + \alpha(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top)\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i}\mathbf{w}_t^\top \nonumber \\
    &\quad +\alpha  \mathbf{w}_t\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_{\ast}^\top \mathbf{\hat{B}}_t(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top) + \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2 \mathbf{w}_t  \mathbf{w}_t^\top \\
    &= \mathbf{I}_k + (\|\mathbf{w}_{\ast,i}\|_2^2 - 2\alpha + \alpha^2 \|\mathbf{w}_t\|_2^2) \mathbf{w}_t \mathbf{w}_t^\top + \alpha(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top)\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i}\mathbf{w}_t^\top \nonumber \\
    &\quad +\alpha  \mathbf{w}_t\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_{\ast}^\top \mathbf{\hat{B}}_t(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top)
\end{align}
No, there is no reason to think that $\mathbf{w}_t$ is close to zero unless we assume a stronger condition on the $\mathbf{w}_{\ast,i}$'s than task diversity (that the heads are well-conditioned). Consider for example that each $\mathbf{w}_{\ast,i} = \mathbf{e}_i$. We must at least assume the heads sum to approximately zero, i.e. $\|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\|_2 \leq \epsilon$. But even with this stronger assumption it is not clear that $\mathbf{w}_t$ is becoming small:
\begin{align}
    \|\mathbf{w}_{t+1} \|_2
    &\leq \left\|\mathbf{I}_k - \frac{\beta}{n}\sum_{i=1}^n (1 - \alpha)\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}  \right\|_2\|\mathbf{w}_t\|_2  +\left\|\frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top( \mathbf{I}_k - \alpha \mathbf{B}_{t,i} \mathbf{\hat{B}}_{t}^\top) \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \right\|_2\\
    &\leq (1 - \beta(1- \alpha) + \beta(1- \alpha) (L_{\max}^2 - 2 \alpha + \alpha^2 \|\mathbf{w}_t\|_2^2)\|\mathbf{w}_t\|_2^2 + 2\beta(1- \alpha)\alpha L_\ast \|\mathbf{w}_t\|_2)\|\mathbf{w}_t\|_2 \nonumber\\
    &\quad + \left\|\frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \right\|_2 + \alpha \left\|\frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \right\|_2 \\
    &\leq (1 - \beta(1- \alpha) + \beta(1- \alpha) (L_{\max}^2 + 2 \alpha + \alpha^2 \|\mathbf{w}_t\|_2^2)\|\mathbf{w}_t\|_2^2 + 2\beta(1- \alpha)\alpha L_\ast \|\mathbf{w}_t\|_2)\|\mathbf{w}_t\|_2 \nonumber\\
    &\quad + \beta \epsilon + \beta L_{\max}^2 + \alpha \beta \epsilon + (L_{\max}^2 + 2 \alpha + \alpha^2\|\mathbf{w}_t\|_2^2)\epsilon\|\mathbf{w}_t\|_2^2  + 2 \alpha^2 \beta L_{\max}^2 \|\mathbf{w}_t\|_2  
\end{align}




%finite samples


% We need $k - E_0 - \alpha^2(k-1) \leq 0$. We have $k - E_0 - \alpha^2(k-1) = (1 - \alpha^2)k - E_0 + \alpha^2 > 0$ for all $\alpha \leq 1$ since $k \geq 1$ and $E_0 < 1$. So we cannot show that MAML learns the representation using this analysis.

% Intuitively: in the outer loop update, the heads serve to remove energy from the representation resulting from the inner loop and adds energy to $\mathbf{B}_\ast$. But if the representation is updated during the inner loop, then it no longer contains enough energy from $\mathbf{B}_t$ such that the energy in $\mathbf{B}_t$ can be reduced by the heads in the outer update.


% Empirically (need to add plots that use same learning rate)

% Clearly larger $\alpha$ helps. Choose $\alpha^2 = 1$, then $k - E_0 - \alpha^2(k-1) = 1 - E_0$ which 

% How does the inner update step for $\mathbf{B}$ help? Does it help in simulations?



% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.6\columnwidth]{anil_vs_maml.png}}
% \vspace{-0mm}
% \caption{Average PA dist over 5 trials. $m_{out} = 2000, m_{in} = 500$, and standard model (all tasks share exactly the same ground-truth representation).  There is no meaningful gain for MAML over ANIL.}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}



% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.6\columnwidth]{anil_vs_maml_mout200.png}}
% \vspace{-0mm}
% \caption{Average PA dist over 10 trials. $m_{out} = 200, m_{in} = 50$, and standard model (all tasks share exactly the same ground-truth representation). Again, there is no meaningful gain for MAML over ANIL.}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}


----------

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.6\columnwidth]{anil_vs_maml_perturb.png}}
\vspace{-0mm}
\caption{The ground truth representation for the $i$-th client is $\mathbf{\hat{B}}_\ast + \boldsymbol{\Delta}_{\ast,i}$. Still there is no meaningful gain for MAML over ANIL, in fact ANIL does slightly better. Tried with varying norms for the $\boldsymbol{\Delta}_{\ast,i}$ but results were the same.
Average PA dist over 10 trials. $m_{out} = 200, m_{in} = 50$. }
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

% \begin{figure}[H]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.6\columnwidth]{Screen Shot 2021-08-09 at 5.46.31 PM.png}}
% \vspace{-0mm}
% \caption{The ANIL paper gives experiments showing that ANIL and MAML perform essentially the same for few-shot image classification and RL problems (Table 2, Figure 5).}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}



\textbf{Similar recent work:}

\url{https://arxiv.org/pdf/2106.15367.pdf} \cite{kao2021maml}

MAML is a Noisy Contrastive Learner

This paper shows that the ANIL outer loop update for the representation in the classification setting is  a gradient step  with respect to a contrastive loss, if the head is initially zero (before inner loop).  They  propose ``zeroing trick'': set head to zero at the start of each round. This is similar to our paper because we have also noticed the benefit of initializing the head to be zero. Their empirical results are promising (at least Figures 3,4, and 7), as they show that zeroing the head on every round can improve the performance of both ANIL and MAML. But they do not have a notion of dimensionality of the representation or of task diversity. Their theorem (and corollary) simply state that ANIL with the zeroing trick satisfies their definition of a supervised contrastive learning algorithm.

In more detail, note that for classification, the network has multiple heads, one for each class.
Effectively, this paper shows that ANIL with zeroing trick does weight imprinting of the heads with the features of the support data.  In other words, the values of the heads are the features of the support data. When a new image comes, the prediction is the maximum inner product of features for the new image with the heads, i.e. the features of the support images for each class. Thus, the resulting loss  encourages the features for images of the same classes to be similar, and encourages the features for images of different classes to be dissimilar, i.e. it is a contrastive loss. This is the contribution of this paper, and it is explained nicely in Figure 1.

The idea of weight imprinting has been used elsewhere for initializing a new head for few-shot learning a new task \cite{dhillon2019baseline,qi2018low,gidaris2018dynamic}. However, these works do not discuss the representation-learning benefits from weight imprinting. From \cite{qi2018low}, the main intuition is that imprinting directly leads to a better-performing classifier without any further optimization: ``The underlying assumption is that test
examples from new classes are closer to the corresponding
training examples, even if only one or a few are observed''. They do mention that `` fine-tuning (using backpropagation
to further optimize the network weights) should move the
embedding space towards having unimodal distribution for
the new class'' which is essentially the same insight as \cite{kao2021maml}, but they  do not discuss this further. Note that \cite{kao2021maml} does not mention the prior works that use weight imprinting. 


Contrastive Learning is Just Meta-Learning

They experimentally show that meta-learning methods (Prototypical Networks and R2-D2) can achieve state-of-the-art self-supervised representation learning performance. This is because the current state-of-the-art self-supervised representation learning methods, namely contrastive learning methods, are a special case of meta-learning. The idea of self-supervised contrastive learning is that you take an image and rotate it or apply some other augmentation, to create a "positive pair". Meanwhile, you take two images that you know are not from the same class (this may be tricky because you don't have labels, but if there are many classes, you can assume two random images are from different classes) and you call this a "negative pair". Then you compute your representations for all images (in the meta-learning framework, this is the inner loop). Finally, you update your representation by taking a gradient step with respect to a loss that encourages representations of positive pairs to be similar and negative pairs to be different (outer loop). The paper argues that this is a meta-learning method, and experimentally shows strong performance of established meta-learning techniques (Proto Nets and R2-D2) when applied to the self-supervised learning setting.

Both papers are suggesting that meta-learning methods learn good representations because they have close connections with contrastive learning. But they are arguing mostly from an empirical perspective and have not rigorously established the strong representation learning abilities of meta-learning methods.


Another paper \url{https://arxiv.org/pdf/2105.02221.pdf} \cite{chua2021fine}

I think this one is less of an issue because it does not deal with the optimization dynamics. Also the algorithm is not MAML or ANIL. But it is similar, and the given statistical rates for learning the representation depend on task diversity. They also show that the inner loop update for the representation is critical when the tasks do not share exactly the same representation.
I.e. your model structure must match the ground-truth structure, not surprising, but not easy to show. They consider both linear and nonlinear cases. No optimization results for learning rep.



% What else can we show? Consider classification case?



Consider the case in which the ground-truth model for the $i$-th task is $(\mathbf{B}_\ast + \boldsymbol{\Delta}_{\ast,i})\mathbf{w}_{\ast,i}$, where $\|\boldsymbol{\Delta}_{\ast,i}\|_2 \leq \delta_0$ and $\|\mathbf{w}_{\ast,i}\|_2=1$. Then
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i} \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top +   \frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_{\ast}+\boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
    &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{t}\left(\mathbf{I}_d  - \alpha\mathbf{w}_{t}\mathbf{w}_{t}^\top\right) \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top - \frac{\alpha\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_{\ast}+ \boldsymbol{\Delta}_{\ast,i})\mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top+   \frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_{\ast}+ \boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
    &= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top \right)
    +   \frac{\beta}{n}\sum_{i=1}^n ( 1- \alpha \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle) (\mathbf{\hat{B}}_{\ast}+ \boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \label{75}
\end{align}
where $\mathbf{w}_{t,i} = (\mathbf{I}_d - \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t)\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_\ast+ \boldsymbol{\Delta}_{\ast,i})\mathbf{w}_{\ast,i}= (1 - \alpha )\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_\ast+ \boldsymbol{\Delta}_{\ast,i})\mathbf{w}_{\ast,i}$.




If we did not have inner loop update for $\mathbf{B}$, we would have
\begin{align}
    \mathbf{B}_{t+1} 
    &= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top   \right)
    +   \frac{\beta}{n}\sum_{i=1}^n  (\mathbf{\hat{B}}_{\ast}+ \boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top 
\end{align}


Consider $\alpha=1$ and consider the second term in \eqref{75}. The inner loop update for the rep causes matrices  $\boldsymbol{\Delta}_{\ast,i}\mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top$ to be weighted more when $\mathbf{w}_t$ is less aligned with $\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$, and vice versa. 

For each i: more aligned $\rightarrow$ more $\mathbf{\hat{B}}_t$, less $\boldsymbol{\Delta}_{\ast,i}$; less aligned $\rightarrow$ less $\mathbf{\hat{B}}_t$, more $\boldsymbol{\Delta}_{\ast,i}$.

So the inner loop update tells the representation to only pay attention to perturbations in new directions. This makes sense because if $\mathbf{w}_{t,i} \approx \mathbf{w}_{t}$, then $\mathbf{\hat{B}}_{t}\mathbf{w}_{t} \approx (\mathbf{\hat{B}}_{\ast}+\boldsymbol{\Delta}_{\ast,i})\mathbf{w}_{\ast,i}$, so there is no need to update the representation towards $\mathbf{\hat{B}}_{\ast}+\boldsymbol{\Delta}_{\ast,i}$ in this case. Whereas if $\langle \mathbf{w}_{t,i}, \mathbf{w}_{t}\rangle$ is small, then it might be the case that the column space of $\mathbf{\hat{B}}_t$ is far from the column space of $\mathbf{\hat{B}}_{\ast}+\boldsymbol{\Delta}_{\ast,i}$ (although this is not necessarily the case), so it would make sense for the update to more heavily weight $\mathbf{\hat{B}}_{\ast}+\boldsymbol{\Delta}_{\ast,i}$. Anyway, it is believable that this iteration would converge to something like $\mathbf{\hat{B}}_{\ast}+ \mathbf{P}$, where the column space of $ \mathbf{P}$ is  the column spaces of the average of the $\boldsymbol{\Delta}_{\ast,i}$'s. If the average is zero, then we recover $\mathbf{\hat{B}}_{\ast}$. 
But ANIL would also converge to this...





In the  Chua paper, they make no such isotropic assumption on the $\boldsymbol{\Delta}_{\ast,i}$'s, rather, they only assume that they have bounded norm... How is this possible? They should have a bias term. Say that $\boldsymbol{\Delta}_{\ast,i} = \delta_0 \mathbf{\hat{Q}}$ for all $i$. Then there should be an irreducible bias in their representation learning error.

It makes sense that the final test error can go to zero with more samples because they are adapting the rep at test time. So with enough test samples, they can learn any correction to the rep learned during training. This would also be the case for FrozenRep if we allowed it to adapt the rep at test time (which would be the fair comparison in my opinion, but they do not do this).

But still, it does not make sense that they can achieve representation learning error going to zero with the number of training samples. Is this really the representation learning error? No, it is not. It is just the training error. So they never have a representation learning result. {\em They do not show any evidence that the inner loop update helps for learning the rep. It seems that the claimed benefits of AdaptRep (roughly MAML) over FrozenRep (roughly ANIL) are only due to the fact that AdaptRep can adapt the rep at test time to account for the assumed perturbation of the ground-truth representation for the new task, while FrozenRep cannot - there is no training benefit.}

Note that they require $\Omega(d)$ samples per training task and $\Omega(d)$ samples per target task.


{\color{blue} 
Let $\mathbf{v}_{t,i} \coloneqq \mathbf{\hat{B}}_{t}(\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i}$, thus $\mathbf{w}_{t,i} = (1 - \alpha) \mathbf{w}_t +\alpha \mathbf{v}_{t,i}$.

Let $\alpha = 1$.

We have
\begin{align}
\mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  (\mathbf{I}_d - \mathbf{w}_{t}\mathbf{w}_{t}^\top)\frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t  \right)\\
&\quad +\frac{\beta}{n}\sum_{i=1}^n ( 1- \alpha \mathbf{w}_{t}^\top \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i}) (\mathbf{\hat{B}}_{\ast}+ \boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t  \\
&=  \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{t}\mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t  \\
&\quad + \mathbf{\hat{B}}_{t}\mathbf{w}_{t}\mathbf{w}_{t}^\top \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t \\
&\quad +\frac{\beta}{n}\sum_{i=1}^n ( 1- \alpha \mathbf{w}_{t}^\top \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i}) (\mathbf{\hat{B}}_{\ast}+ \boldsymbol{\Delta}_{\ast,i}) \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t  \\
\end{align}
Need to show that the following spectral norm is strictly less than 1. 
\begin{align}
    &\left\|\mathbf{I}_d -  (\mathbf{I}_d - \mathbf{w}_{t}\mathbf{w}_{t}^\top)\frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t   \right\|_2 \nonumber \\
    &\leq 1 - \sigma_{\min}\left((\mathbf{I}_d - \mathbf{w}_{t}\mathbf{w}_{t}^\top)\frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top (\mathbf{\hat{B}}_{\ast} + \boldsymbol{\Delta}_{\ast,i} )\mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top(\mathbf{\hat{B}}_{\ast}^\top + \boldsymbol{\Delta}_{\ast,i}^\top)\mathbf{\hat{B}}_t  \right)
\end{align}
But the $\sigma_{\min}$ of the above matrix is zero since $\|\mathbf{w}_t\|_2 = 1$. So we need to consider $\alpha \neq 1$.

In the general case the relevant spectral norm is:
\begin{align}
     &\left\|\mathbf{I}_d -  (\mathbf{I}_d - \alpha \mathbf{w}_{t}\mathbf{w}_{t}^\top)\frac{\beta}{n}\sum_{i=1}^n (1-\alpha)^2\mathbf{w}_{t}\mathbf{w}_{t}^\top + \alpha(1- \alpha) \mathbf{w}_{t}\mathbf{v}_{t,i}^\top+ \alpha(1- \alpha) \mathbf{w}_{t}\mathbf{v}_{t,i}^\top+ \alpha^2 \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top\right\|_2 \nonumber \\
     &\leq 1 + \beta (1 - \alpha)^2 \sigma_{\max} (\mathbf{w}_{t}\mathbf{w}_{t}^\top) + 2 \beta \alpha (1 - \alpha)(1+\delta_0) L_{\max} + \beta \alpha^3 (1+\delta_0)^2 L_{\ast}^2 \nonumber \\
     &\quad + \beta \alpha^2  (2\delta_0+\delta_0^2) L_\ast^2 - \beta \alpha^2 E_0 \mu_\ast^2
\end{align}
This bound is even worse than in the case with $\boldsymbol{\Delta}_{\ast,i}=\mathbf{0}$, for which we were not able to show the bound is less than 1.

What if we make $\tau$ inner loop updates?
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{B}_t - \frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} f_i(\mathbf{B}_{t,i,\tau}, \mathbf{w}_{t,i,\tau}) \\
    &= \mathbf{B}_t - \frac{\beta}{n}\sum_{i=1}^n 
    (\mathbf{B}_{t,i,\tau} \mathbf{w}_{t,i,\tau} \mathbf{w}_{t,i,\tau}^\top - \mathbf{B}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i,\tau}^\top )
     \\
     &= \mathbf{B}_t - \frac{\beta}{n}\sum_{i=1}^n 
    \Bigg( \left(\mathbf{B}_{t} \prod_{s =1}^{\tau-1}(\mathbf{I}_k - \alpha\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top) + \alpha \mathbf{B}_{\ast} \mathbf{w}_{\ast,i}  \left( \sum_{s=0}^{\tau-1}\mathbf{w}_{t,i,s}^\top \prod_{r=s+1}^{\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,r}\mathbf{w}_{t,i,r}^\top) \right) \right) \mathbf{w}_{t,i,\tau} \mathbf{w}_{t,i,\tau}^\top \nonumber \\
    &\quad \quad \quad \quad \quad \quad \quad \quad- \mathbf{B}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i,\tau}^\top \Bigg) \\
    &= \mathbf{B}_t \left(\mathbf{I}_k - \frac{\beta}{n}\sum_{i=1}^n 
    \left( \prod_{s =1}^{\tau-1}(\mathbf{I}_k - \alpha\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top)\right) \mathbf{w}_{t,i,\tau} \mathbf{w}_{t,i,\tau}^\top \right) \nonumber \\
     &\quad + \frac{\beta}{n} \mathbf{B}_\ast \sum_{i=1}^n\left(\mathbf{w}_{\ast,i} \mathbf{w}_{t,i,\tau}^\top - \alpha \mathbf{w}_{\ast,i}  \left( \sum_{s=0}^{\tau-1}\mathbf{w}_{t,i,s}^\top \prod_{r=s+1}^{\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,r}\mathbf{w}_{t,i,r}^\top) \right) \mathbf{w}_{t,i,\tau} \mathbf{w}_{t,i,\tau}^\top \right)
\end{align}
where
\begin{align}
    \mathbf{w}_{t,i,s} &=  \prod_{r=0}^{s-1} (\mathbf{I}_k - \alpha \mathbf{B}_{t,i,r}^\top \mathbf{B}_{t,i,r}) \mathbf{w}_{t} + \alpha \sum_{r=0}^{s-1} \left(\prod_{z=r+1}^{s-1}(\mathbf{I}_k - \alpha \mathbf{B}_{t,i,z}^\top \mathbf{B}_{t,i,z})\right) \mathbf{B}_{t,i,r}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i} 
\end{align}
The $\left( \prod_{s =1}^{\tau-1}(\mathbf{I}_k - \alpha\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top)\right)$ factor in the coefficient of $\mathbf{B}_t$ in the outer loop update for $\mathbf{B}_{t+1}$ may mitigate the benefit of task diversity. So we should not expect to do any better in this case.

}






% algorithms:
% larger batch size

% compare with arnold aistats paper - multi-layer case

% address catastrophic forgetting

% overparameterization

% deal with orthogonalization


% issues with classification:
% W_*i^T B_*^T x is always a standard basis vector. So really the model needs to be max(W_*i^T B_*^T x)? 

% Loss:
% || phi_b(q)T sum_i phi_b(si) e_{j_i}^T - e_{q_i}^T ||_2^2
% 
% clearly this is a contrastive loss
%
% when you backprop wrt b, do you take bckprop through phi_b(si)? only if making second-order update (equiv to taking I - hessian)

% in linear case it would be || x^T B \sum_i B^T x_i e_{j_i}^T - e_x^T ||

% note that previous works have shown that pretraining does well when you can learn new fine-tuned heads

% Recent empirical works have shown  that a simple baseline for few-shot image classification is competitive with and sometimes even outperforms MAML and ANIL, as well as other meta-learning methods. Recall that in the few-shot image classification setting, tasks are $N$-way, $K$-shot classification problems. A subset of the classes in the dataset are used for meta-training and the rest are used for meta-validation and meta-testing. The simple baseline ignores the episodic training procedure of meta-learning, and instead trains a representation and some sort of head (linear, distance-based) on all of the meta-training classes simultaneously. Let $C$ be the number of meta-training classes. Importantly, the head is large. 


% the implications of this would be that... we need either task diversity or class diversity depending on the algorithm

% % optimization with softmax layer:
% % but for the classification setting this would just be standard GD... do we need large C to recover rep here

% case 1: $k > C$: then we cannot have sufficient class diversity to learn rep (analogous to $k > n$)

% case 2: $k < C$: then we cannot have well-separated features (some of the feature vectors for different classes will overlap)

% case 3: $k=C$: ideal scenario since we can have sufficient diversity to learn the representation, but , but not realistic. 

% case 4: $k > C$, but eff$(k) = C$: is this effectively the same setting as case 3? Note that we should be able to learn an effective initialization as long as the ``heads'' for each class are almost orthogonal.

% $\rightarrow$ orthogonalizing the heads should help empirically

% \textbf{Question:} do the heads need to be imprinted, or do they only need to be orthogonal and fixed? Theory says orthogonal and fixed.
% If they are orthogonal and fixed, then we have effectively just reduced the number of layers in the network by one. So how could this help? Is it really the case that self-contrastive is better than outer-contrastive? i guess so, because in the latter you are forcing the rep to fit to a particular orthogonalization that may be suboptimal. But then why does standard training with many classes still learn good reps (note it is not doing weight imprinting).  --Because the heads are not random in this case.

% Empirically: random heads do not learn rep for ANIL, ERM regression does not learn rep with random heads




% Tewari paper also notices that single task, multi-class classification problem can be sufficiently diverse

% notes on tewari paper:
% it is required for transferability that any optimal rep for the source tasks is also optimal for the target task
% in order for this to be true, the class of source heads cannot be more complex than the class of target heads, since the source task heads could otherwise correct too many errors
% Appendix H - single-task, multi-class problem with softmax cross entropy loss can be diverse under strong boundedness assumption on function outputs (e^B is effective bound). 
% Labels sampled from softmax distrib over true rep and head. --> try to optimize this. but i think there is a mistake in theorem 1 with K, no? 
% this theorem is supposed to show that more classes (larger K) increases diversity, but I think there is a mistake in accounting
% problem: to achieve diversity when the heads are ReLU nets, need at least 2^d tasks
% for linear heads and ReLU rep, how many tasks needed?
%--answer, from Tripureneni Importance of Task Diversity Lemma 6: same as linear rep case, need linear heads to be well-conditioned in R^k (R^r in Trip). In fact, this holds even when the rep is a many-layer deep nonlinear network
%--note: Trip does not discuss classification, unless you include logistic regression
%--problem with Theorem 4 in Trip (log regress): requires d samples per task
%--but corollary 3 corrects this, sharper
% note: for optimizing ReLU case, just need to so it reaches close to empirical risk minimizer, not necessarily the ground truth
% ***** inconsistency between Trip and Tewari: Tewari exponential lower bound on number of tasks required to achieve diversity when head is 1-layer non-linear NN. But according to Trip, k heads are sufficient in the case of logistic regression, where head is effectively 1-layer NN
% so i'm not sure about this...




Takeaways:

\begin{itemize}
\item Empirically there is no benefit of the inner loop update step for the representation in our setting. And if we assume that the task optimal solutions exactly belong to a ground-truth subspace, then I think there is no benefit to making inner loop update for rep. Can we prove this? Upper bound error for solution to no inner loop objective, lower bound error for solution to inner loop objective. But how would we show no optimization benefit?

In the case that the task optimal solutions may have some perturbation away from the ground-truth subspace, it is less clear. In \cite{chua2021fine}, they show that the inner update step is necessary in a special case: the task optimal solutions are close to the ground-truth subspace, but not within it. Further, the data $\mathbf{x}$ has most of its variance aligned with the directions of the perturbations away from the ground-truth subspace, and very little variance in the ground-truth subspace itself. So, without the inner loop update step for the representation, any representation that minimizes the empirical risk is aligned with the perturbation away from the ground-truth, since the perturbation actually has more energy in the loss function. Meanwhile, solutions to the objective with inner loop update align with the ground-truth subspace, as long as the total number of training samples is $\Omega(d^2)$.

Is this is just a degenerate case? In a typical case, it seems that there is no difference made by the inner loop update for the rep...

    \item Weight imprinting of the head is a technique that has been used to initialize the head for few-shot learning. A recent paper \cite{kao2021maml} has shown that  MAML effectively does weight imprinting of the head in every iteration, and this means that the meta-validation loss is contrastive and thereby should help with representation learning after backpropagating through this loss in the the outer loop. However they do not make the connection that prior works that did weight imprinting induced a contrastive loss.
    
    Our paper can provide theoretical justification for these observations. In regression, weight imprinting increases the diversity of the heads post-inner loop (either setting $\mathbf{w}_t=0$ or $\alpha=1$ executes weight imprinting, we have seen this). We will have to consider the classification setting to provide a more complete and applicable analysis however.
    \item (Tangent) Instead of leveraging many tasks that are diverse, in classification  we can alternatively leverage many diverse {\em classes} to learn a good representation with only a {\em single} task. This has also been noticed in \cite{xu2021representation} from a statistical learning standpoint, and it aligns with empirical works that achieve high performance and positive transfer by standard training on e.g. ImageNet with many classes (no meta-learning). It works essentially the same way as task diversity. Consider the simple linear case. The representation is $\mathbf{B} \in \mathbb{R}^{d \times k}$ with ground-truth $\mathbf{\hat{B}}_\ast$. The head is $\mathbf{W} \in \mathbb{R}^{C \times k}$ with ground-truth $\mathbf{W}_\ast$, where $C$ is the number of classes. The $i$-th row of $\mathbf{W}$ maps a vector of features to a weight roughly  corresponding to the likelihood that the features belong to the $i$-th class. The loss for the task is typically the cross entropy loss with a final softmax activation, i.e.
    \begin{align}
        f(\mathbf{B},\mathbf{W}) \coloneqq \mathbb{E}_{\mathbf{x}, y} \left[ -\sum_{i=1}^C \mathbf{1}_{y = i} \log\left(\frac{\exp({-\mathbf{w}_i^\top \mathbf{B}^\top \mathbf{x}})}{\sum_{i'=1}^C \exp({-\mathbf{w}_{i'}^\top \mathbf{B}^\top \mathbf{x}}) }\right) \right]
    \end{align}
    where $\mathbb{P}(y=i | \mathbf{x}) = \frac{\exp({-\mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top \mathbf{x}})}{\sum_{i'=1}^C \exp({-\mathbf{w}_{\ast,i'}^\top \mathbf{B}_\ast^\top \mathbf{x}} )}$. Ignoring the softmax, cross entropy loss, and random labels, we are again trying to sense a matrix $\mathbf{B}_\ast \mathbf{W}_\ast^\top$, and in particular, recover the column space of $\mathbf{B}_\ast$. Each row of $\mathbf{W}_\ast$ (column of $\mathbf{W}_\ast^\top$) gives us a different view of the ground-truth representation, and corresponds to the decision vector for a particular class. If the classes are diverse enough (i.e. their ground-truth decision vectors span $\mathbb{R}^k$), then we should have a full view of $col(\mathbf{B}_\ast)$ and be able to recover it.
    As seen in the logistic regression special case below, it is not straightforward to show this with the softmax, CE loss, and random labels, but it should be possible...
\end{itemize}





\section{Multitask Logistic Regression}

$\mathcal{X} = \mathbb{R}^d, \mathcal{Y} = \{0,1\}$.

Let $\sigma(z) \coloneqq \frac{1}{1+e^{-z}}$. 

Let $\mathcal{D}_{i} \coloneqq \{(\mathbf{x}_{i,j}, y_{i,j}) \}_{j=1}^m$. Loss function for task $i$:
\begin{align}
    \hat{f}_i (\mathbf{B},\mathbf{w}; \mathcal{D}_{i}) \coloneqq \frac{1}{m}\sum_{j=1}^m - y_{i,j}\log(\sigma(\mathbf{w}^\top \mathbf{B}^\top \mathbf{x}_{i,j})) - (1 - y_{i,j})\log(1-\sigma(\mathbf{w}^\top \mathbf{B}^\top \mathbf{x}_{i,j}))
\end{align}

Ground-truth:
\begin{align}
   \mathbb{P}(y_{i,j}=1| \mathbf{x}_{i,j},i) = \sigma(\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top\mathbf{x}_{i,j})\quad \forall \; i \in [n],j\in[m]
\end{align}

\textbf{Question:} can ANIL and MAML recover $\mathbf{\hat{B}}_\ast$?

ANIL:
\begin{align}
    \mathbf{w}_{t,i} &= \mathbf{w}_t - \alpha \nabla_{\mathbf{w}} \hat{f}_i (\mathbf{B},\mathbf{w}; \mathcal{D}_{i,in}) \nonumber \\
    &= \mathbf{w}_t + \frac{\alpha}{m_{in}}\sum_{j=1}^{m_{in}}\left( y_{i,j,in} - \frac{1}{1+e^{-\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{x}_{i,j,in}}}  \right)\mathbf{B}_t^\top \mathbf{x}_{i,j,in}
    % &= \mathbf{w}_t - \frac{\alpha}{m_{in}}\sum_{j=1}^{m_{in}}\left( \frac{(1 -y_{i,j,in})+(1 -2y_{i,j,in}) e^{-\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{x}_{i,j,in}}}{1+e^{-\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{x}_{i,j,in}}} \right)\mathbf{B}_t^\top \mathbf{x}_{i,j,in} \nonumber \\
    % &= 
\end{align}
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{B}_t - \frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \hat{f}_i (\mathbf{B}_t,\mathbf{w}_{t,i}; \mathcal{D}_{i,out}) \nonumber \\
    &= \mathbf{B}_t + \frac{\alpha}{m_{out}}\sum_{j=1}^{m_{out}}\left( y_{i,j,out} - \frac{1}{1+e^{-\mathbf{w}_{t,i}^\top \mathbf{B}_t^\top \mathbf{x}_{i,j,out}}}  \right) \mathbf{x}_{i,j,out}\mathbf{w}_{t,i}^\top
\end{align}

Experiments:
% note that these experiments differ from ones considered previously because we are using the cross entropy loss and y_{i,j,in} is a Bernoulli random variable

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{logreg_anil_maml_d5.png}}
\vspace{-0mm}
\caption{$d=5,k=2,n=10, m_{in}=m_{out}=500$. Average over 3 trials: ANIL and MAML recover the ground-truth representation (with no benefit for MAML) in the case of logistic regression... }
\label{fig:logreg}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{logreg_erm_d5.png}}
\vspace{-0mm}
\caption{... while standard training (ERM) does not. $d=5,k=2,n=10$}
\label{fig:logreg_erm}
\end{center}
\vspace{-0mm}
\end{figure}


% see email draft about where left off



\section{General Function Classes}

How to measure closeness of representations? We want a representation that admits similar classifiers as the ground-truth representation. Can we show anything here from an optimization perspective?

% Can we show that without task diversity, we cannot learn anything? this has already been answered from learning theory perspective

ANIL Objective:
\begin{align}
    \min_{\mathbf{B},\mathbf{w}}\frac{1}{2nm}\sum_{i=1}^n\sum_{j=1}^m (\langle h_{\mathbf{B}}(\mathbf{x}_{i,j}), U_i(\mathbf{w})\rangle - \langle h_{\mathbf{B}_\ast}(\mathbf{x}_{i,j}), \mathbf{w}_{\ast,i} \rangle )^2
\end{align}

Loss is a nonconvex function of $\mathbf{B}$ with potentially spurious local minima. 





Three regimes: (i) over-parameterized (more parameters than samples) (a) make $k > m$, or (b) try two-layer linear network, (ii) over-specified (below), (iii) high-dimensional (e.g. you are doing multi-class classification with $T \gg 0$ classes, and since the classes/tasks are mutually exclusive, you need a $T$-dimensional representation. But it is still intrinsically low-dimensional, so this is similar to the over-specified case. Over-specified is easier to analyze from an optimization perspective I think)

issues with over-parameterization and representation learning: a popular over-parameterization perspective on training neural networks is that with many parameters, the network is essentially a random feature model. so it doesn't matter how high-quality the features are, it only matters that you have many of them. so there is really no representation learning according to this theory

on the other hand, result from Du paper suggests that representation learning can improve dependence of excess risk on the input dimension in potentially over-parameterized settings. but this result does not show any improvement due to having more parameters, in fact it does not even capture the relationship between the number of params and the excess risk and number of samples. also note that they learn with regularization. and they do not say anything about whether they learn the teacher representation, only talk about generalization

dimensionality-reduction and overparameterization seem to be at odds...

if you have many features, why does it matter what those features are? somehow Du result is showing that pre-training these features captures some of the complexity of the problem. If the learned representation is intrinsically low-dimensional, then it makes sense.

\url{https://arxiv.org/pdf/2011.14522.pdf} recent work showing that NTK and other regimes in which NNs are analyzed are such that the network in these regimes cannot learn features. They propose an alternative parameterization that provably allows for feature learning (vanishing model weights but constant step size). Experimentally they show that MAML does not learn omniglot features in NTK regime but it does in the new regime. This makes sense because NTK regimen is essentially saying that the representation does not change much from its initialization, it is like a random feature model.

qualities of a good representation:
\begin{itemize}
    \item intrinsically low-dimensional
    \item for classification: data from different classes is well separated, data from same class is clustered
\end{itemize}

over-parameterized case i think is a new paper, I don't think we have the machinery to understand what a good over-parameterized representation is yet. but over-specified case may be doable. Two-layer linear net may also be doable. column space of product should match true column space. but people don't seem to be interested in this case.

\subsection{Over-specified case}

Say $\mathbf{B} \in \mathbb{R}^{d \times d}$, $\mathbf{B}_\ast \in \mathbb{R}^{d \times d}$, $\mathbf{w}_{\ast,i} \in \mathbb{R}^{d}$, $\mathbf{B}_{\ast,i} = [\mathbf{U}, \;
\mathbf{V}] \begin{bmatrix}
\mathbf{D}_\mathbf{S}^\ast & \mathbf{0} \\
\mathbf{0} & \mathbf{D}_\mathbf{T}^\ast  \\
\end{bmatrix}[\mathbf{U}, \;
\mathbf{V}]^\top$, $\mathbf{D}_{\mathbf{S}}^\ast \in \mathbb{R}^{k \times k}$, $\mathbf{D}_{\mathbf{T}}^\ast \in \mathbb{R}^{d-k \times d-k}$ (SVD), $\mathbf{U} \in \mathbb{R}^{d \times k}$, $\mathbf{V} \in \mathbb{R}^{d \times d-k}$. $\mathbf{U}, \mathbf{V}$ are two orthonormal matrices which are orthogonal to each other and whose columns together span $\mathbb{R}^d$ \citep{zhuo2021computational}.

For any $\mathbf{B}_t \in \mathbb{R}^{d \times d}$, there are two matrices $\mathbf{S}_t \in \mathbb{R}^{k \times d}$ and $\mathbf{T}_t \in \mathbb{R}^{d-k \times d}$ we can write:
\begin{align}
    \mathbf{B}_t &= \mathbf{U}\mathbf{S}_t + \mathbf{V}\mathbf{T}_t
\end{align}






% What is distance to ground-truth representation? literature says - signal part and noise part. want to show signal goes to GT, noise goes to zero.


% \begin{align}
%     \mathbf{B} &= \begin{bmatrix} \mathbf{S} & \mathbf{T} \\
%     \end{bmatrix}
% \end{align}
% where $\mathbf{S} \in \mathbb{R}^{d \times k}$, $\mathbf{T} \in \mathbb{R}^{d \times R-k}$. 
Need some sort of regularization of the heads in order to make representation learning useful. This would help at meta-test time, but it may not help for learning the representation.

So during meta-training the population problem we aim to solve is:
\begin{align}
    \min_{\mathbf{B}\in \mathbb{R}^{d \times d}}\min_{\mathbf{w} \in \mathbb{R}^{d}} &\frac{1}{n} \sum_{i=1}^n f_i(\mathbf{B}, \mathbf{w} - \nabla_{\mathbf{w}} f_i(\mathbf{B}, \mathbf{w}))\\
   f_i(\mathbf{B}, \mathbf{w}) &=\frac{1}{2} \|\mathbf{B}\mathbf{w} - \mathbf{B}_\ast \mathbf{w}_{\ast,i}\|_2^2 %+ {\lambda} \|\mathbf{w}\|_{1}
\end{align}

Representation learning error:
\begin{align}
   \max \big\{ \| \mathbf{S}_t \mathbf{S}_t^\top - \mathbf{D}_{\mathbf{S}}^\ast \|_2^2, \; \| \mathbf{T}_t \mathbf{T}_t^\top - \mathbf{D}_{\mathbf{T}}^\ast \|_2^2, \; \| \mathbf{T}_t \mathbf{S}_t^\top\|_2^2 \big\}
\end{align}

ANIL Updates:
\begin{align}
\mathbf{w}_{t,i} &= \mathbf{w}_{t} - \alpha (\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_{t} - \mathbf{B}_t^\top \mathbf{B}_{\ast} \mathbf{w}_{\ast,i} ) \\ %- \alpha \lambda \partial \|\mathbf{w}\|_{1} \\
&= (\mathbf{I} - \alpha \mathbf{S}_t^\top \mathbf{S}_t - \alpha \mathbf{T}_t^\top \mathbf{T}_t ) \mathbf{w}_{t} + \alpha \mathbf{B}_t^\top \mathbf{B}_{\ast} \mathbf{w}_{\ast,i} \\
    \mathbf{B}_{t+1} &=  \mathbf{B}_t\left(\mathbf{I}_d  - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) +  \frac{\beta}{n} \mathbf{B}_{\ast} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \\
    &= (\mathbf{U}\mathbf{S}_{t}+\mathbf{V}\mathbf{T}_t)\bigg(\mathbf{I}_d  - (\mathbf{I} - \alpha \mathbf{S}_t^\top \mathbf{S}_t - \alpha \mathbf{T}_t^\top \mathbf{T}_t )\mathbf{w}_t\mathbf{w}_{t}^\top (\mathbf{I} - \alpha \mathbf{S}_t^\top \mathbf{S}_t - \alpha \mathbf{T}_t^\top \mathbf{T}_t ) - \mathbf{B}_t^\top \mathbf{B}_\ast \frac{\beta \alpha^2}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  \nonumber \\
    &\quad - (\mathbf{I} - \alpha \mathbf{S}_t^\top \mathbf{S}_t - \alpha \mathbf{T}_t^\top \mathbf{T}_t )\mathbf{w}_t \frac{\beta \alpha}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t - \mathbf{B}_t^\top\mathbf{B}_\ast \frac{\beta \alpha}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}^\top \mathbf{w}_t^\top (\mathbf{I} - \alpha \mathbf{S}_t^\top \mathbf{S}_t - \alpha \mathbf{T}_t^\top \mathbf{T}_t )  \bigg) \nonumber \\
    &\quad +  \frac{\beta}{n} \mathbf{B}_{\ast} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t}^\top (\mathbf{I} - \alpha \mathbf{S}_t^\top \mathbf{S}_t - \alpha \mathbf{T}_t^\top \mathbf{T}_t) + \frac{\beta \alpha}{n} \mathbf{B}_{\ast} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t 
\end{align}
The dynamics are highly coupled...


% The representation learning error is 
% \begin{align}
%     \min_{\mathbf{R}\in \mathcal{O}^{R \times R}} \|(\mathbf{I} - \mathbf{B}_\ast \mathbf{B}_\ast^\top) [\mathbf{B}\mathbf{R}]_{1:k}\|_2^2 + \| [\mathbf{B}\mathbf{R}]_{k:R}\|_2^2
% \end{align}
% i.e., rotate the columns of $\mathbf{B}$ in the best possible way such that the principle angle distance of the matrix formed by  first $k$ columns to $\mathbf{B}_\ast$ plus the operator norm of the matrix formed by the remaining columns is minimized. Maybe rotations should be restricted to permutations.





\section{Experiments}

Tewari paper: Multi-output regression with deep networks. The number of outputs is a proxy for task diversity (since the more outputs you have, effectively the more tasks you have). Data is synthetic and generated from a ground-truth deep neural network. They show that with more outputs, the pre-trained representation generalizes better to new tasks.
% note on Tewari paper: implication is that simpler heads generalize better because they force more of the complexity to be stored in the representation.

Can we show that... more classes are better for 

Need to consider: 

ERM with many classes vs 

Train MAML very the number of samples per





\section{old proof thoughts}

Let $C_1 \coloneqq (1-\alpha)(1 - \alpha \|\mathbf{w}_t\|_2^2)\Big(1-\alpha+ 2\alpha\frac{p_1}{\|\mathbf{w}_t\|_2} \Big)\|\mathbf{w}_t\|_2^2$, $C_2\coloneqq p_2 \|\mathbf{w}_t\|_2 \alpha(1-\alpha)(1-\alpha\|\mathbf{w}_t\|_2^2)$, $C_3 = p_2 \|\mathbf{w}_t\|_2 \alpha (1-\alpha)$, and  $\boldsymbol{\Gamma} \coloneqq \alpha^2 \frac{1}{n}\sum_{i=1}^n \mathbf{{v}}_{t,i} \mathbf{{v}}_{t,i}^\top$. 
Notice that for $\alpha \leq \frac{1}{\max(1+2|p_1|/\|\mathbf{w}_t\|_2}, \|\mathbf{w}_t\|_2^2$, $C_1$ is nonnegative. Also, we know that $\boldsymbol{\Gamma}$ has minimum singular value at least $\alpha^2 E_0 \mu_\ast^2$. It remains to deal with the middle terms. 
We have
\begin{align}
    (\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top)\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top &= C_1\mathbf{\hat{w}}_t \mathbf{\hat{w}}_t^\top + C_2 \mathbf{\hat{w}}_t \mathbf{\hat{w}}_{t,\perp}^\top + C_3 \mathbf{\hat{w}}_{t,\perp} \mathbf{\hat{w}}_t^\top + \boldsymbol{\Gamma}
\end{align}
Next we use the variational definition of the minimum singular value:
\begin{align}
    &\sigma_{\min}\left((\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top)\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)\nonumber \\
    &= \min_{\mathbf{\hat{y}}: \|\mathbf{\hat{y}}\|_2 =1}\mathbf{\hat{y}}^\top  (\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top)\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)^\top \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)(\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top) \mathbf{\hat{y}}.
\end{align}
For any such $\mathbf{\hat{y}}$, we have:
\begin{align}
    &\mathbf{\hat{y}}^\top  (\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top)\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)^\top \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)(\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top) \mathbf{\hat{y}}\nonumber \\
    &=  \mathbf{\hat{y}}^\top(C_1\mathbf{\hat{w}}_t \mathbf{\hat{w}}_t^\top + C_2 \mathbf{\hat{w}}_t \mathbf{\hat{w}}_{t,\perp}^\top + C_3 \mathbf{\hat{w}}_{t,\perp} \mathbf{\hat{w}}_t^\top + \boldsymbol{\Gamma})^\top (C_1\mathbf{\hat{w}}_t \mathbf{\hat{w}}_t^\top + C_2 \mathbf{\hat{w}}_t \mathbf{\hat{w}}_{t,\perp}^\top + C_3 \mathbf{\hat{w}}_{t,\perp} \mathbf{\hat{w}}_t^\top + \boldsymbol{\Gamma})\mathbf{\hat{y}} \nonumber \\
    &= (C_1^2 + C_3^2) \langle\mathbf{\hat{y}},\mathbf{\hat{w}}_t\rangle^2 + 2 C_1 C_2 \langle\mathbf{\hat{y}},\mathbf{\hat{w}}_t\rangle\langle\mathbf{\hat{y}},\mathbf{\hat{w}}_{t,\perp}\rangle + (C_2^2) \langle\mathbf{\hat{y}},\mathbf{\hat{w}}_{t,\perp}\rangle^2   \nonumber \\
    &\quad + \mathbf{\hat{y}}^\top\boldsymbol{\Gamma}(C_1\mathbf{\hat{w}}_t \mathbf{\hat{w}}_t^\top + C_2 \mathbf{\hat{w}}_t \mathbf{\hat{w}}_{t,\perp}^\top + C_3 \mathbf{\hat{w}}_{t,\perp} \mathbf{\hat{w}}_t^\top) \mathbf{\hat{y}} + \mathbf{\hat{y}}^\top(C_1\mathbf{\hat{w}}_t \mathbf{\hat{w}}_t^\top + C_2 \mathbf{\hat{w}}_t \mathbf{\hat{w}}_{t,\perp}^\top + C_3 \mathbf{\hat{w}}_{t,\perp} \mathbf{\hat{w}}_t^\top)^\top \boldsymbol{\Gamma}\mathbf{\hat{y}} \nonumber \\
    &\quad + 2 \mathbf{\hat{y}}^\top \boldsymbol{\Gamma}\mathbf{\hat{y}} \nonumber 
\end{align}
%    (1-\alpha)(1 - \alpha \|\mathbf{w}_t\|_2^2)\Big(1-\alpha+ 2\alpha\frac{p_1}{\|\mathbf{w}_t\|_2} \Big)\|\mathbf{w}_t\|_2^2 \langle \mathbf{\hat{y}}, \mathbf{\hat{w}}_t\rangle^2 
% \nonumber\\
% &\quad + p_2 \|\mathbf{w}_t\|_2 \alpha(1-\alpha)(1-\alpha\|\mathbf{w}_t\|_2^2) \langle\mathbf{\hat{y}}, \mathbf{\hat{w}}_t\rangle \langle \mathbf{\hat{w}}_{t,\perp}, \mathbf{\hat{z}}\rangle  + p_2 \|\mathbf{w}_t\|_2 \alpha (1-\alpha)  \langle\mathbf{\hat{y}}, \mathbf{\hat{w}}_{t,\perp}\rangle \langle \mathbf{\hat{w}}_t, \mathbf{\hat{z}}\rangle \nonumber \\
%     &\quad + \alpha^2 \frac{1}{n}\sum_{i=1}^n \mathbf{\hat{y}}^\top \mathbf{{v}}_{t,i} \mathbf{{v}}_{t,i}^\top \mathbf{\hat{z}}
Let $q_1 = \langle\mathbf{\hat{y}},\mathbf{\hat{w}}_t\rangle$ and $q_2 =\langle\mathbf{\hat{y}},\mathbf{\hat{w}}_{t,\perp}\rangle$. WLOG we can assume $\mathbf{\hat{y}} = q_1 \mathbf{\hat{w}}_t + q_2 \mathbf{\hat{w}}_{t,\perp} + q_3 \mathbf{\hat{u}}_3$ for some vector $\mathbf{\hat{u}}$ that is orthogonal to the others.

Let $\mathbf{z} \coloneqq \boldsymbol{\Gamma}\mathbf{\hat{y}}$, and let $r_1 = \langle\mathbf{z},\mathbf{\hat{w}}_{t}\rangle$ and $r_2 = \langle\mathbf{z},\mathbf{\hat{w}}_{t,\perp}\rangle$. Note that 
$r_1 = \langle (q_1 \mathbf{\hat{w}}_t + q_2 \mathbf{\hat{w}}_\perp + q_3 \mathbf{\hat{u}}_3)\mathbf{\Gamma},\mathbf{\hat{w}}_{t}\rangle = q_1 \mathbf{\hat{w}}_t^\top  \gamma \mathbf{\hat{w}}_t + q_2 \mathbf{\hat{w}}_{t,\perp}^\top  \gamma \mathbf{\hat{w}}_t + q_3 \mathbf{\hat{u}}_{3}^\top  \gamma \mathbf{\hat{w}}_t$ Then we have
\begin{align}
    &\mathbf{\hat{y}}^\top  (\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top)\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)^\top \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)(\mathbf{I}- \alpha \mathbf{w}\mathbf{w}^\top) \mathbf{\hat{y}} \nonumber \\
    &= (C_1^2 + C_3^2) q_1^2 + 2 C_1 C_2 q_1 q_2 + C_2^2 q_2^2   \nonumber \\
    &\quad + 2C_1 r_1 q_1 + 2C_2 r_1 q_2 + 2C_3 r_2 q_1 + 2  \mathbf{\hat{y}}^\top \mathbf{\Gamma}\mathbf{\hat{y}} \nonumber \\
    &\geq C_3^2 q_1^2 + (C_1 q_1 + C_2 q_2)^2  \nonumber \\
    &\quad + 2C_1 (q_1 \mathbf{\hat{w}}_t^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_t + q_2 \mathbf{\hat{w}}_{t,\perp}^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_t + q_3 \mathbf{\hat{u}}_{3}^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_t) q_1 + 2C_2 (q_1 \mathbf{\hat{w}}_t^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_t + q_2 \mathbf{\hat{w}}_{t,\perp}^\top \boldsymbol{\Gamma} \mathbf{\hat{w}}_t + q_3 \mathbf{\hat{u}}_{3}^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_t) q_2 \nonumber \\
    &\quad + 2C_3 (q_1 \mathbf{\hat{w}}_t^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_{t,\perp} + q_2 \mathbf{\hat{w}}_{t,\perp}^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_{t,\perp} + q_3 \mathbf{\hat{u}}_{3}^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_{t,\perp}) q_1 + 2  \alpha^4 E_0^2 \mu_{\ast}^4
\end{align}

% bad case: $q_3 >> q_2 >> q1$, $q_3 \mathbf{\hat{u}}_{3}^\top  \boldsymbol{\Gamma} \mathbf{\hat{w}}_t q_2<0$. set $q_2 = -C_1 q_1/C_2$. then all the good terms are $O(q_1^2)$ and the 2 bad terms are $O(q_1)$.

% we can choose $q_1=O(\alpha^2)$, q2 = alpha, q3 = 1 this is bad

% it must come down to the constants

% how to prove this?



-----------


Now we need to control the minimum singular value of $\mathbf{R}_{t+1}$. 
We have 
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_t - \left(\frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right)  \nonumber
\end{align}
Define $\mathbf{\nabla} \coloneqq \frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top$. We have
\begin{align}
    \sigma_{\min}^2(\mathbf{R}_{t+1}) &= \sigma_{\min}(\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}) \nonumber \\
    &= \sigma_{\min}(\mathbf{I}_{k} - \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} - \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t} + \mathbf{\nabla}^\top \mathbf{\nabla}) \nonumber \\
    &\geq \sigma_{\min}(\mathbf{I}_{k} - \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} - \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t} )% - 2 \left\|\mathbf{\hat{B}}_{t}^\top\mathbf{\nabla}  \right\|_2 \nonumber \\
    % &= 1- 2 \left\|\mathbf{\hat{B}}_{t}^\top\mathbf{\nabla}  \right\|_2 \nonumber 
\end{align}
Next, define $\mathbf{v}_{t,i} \coloneqq \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}$, and note that $\mathbf{w}_{t,i} \coloneqq (1-\alpha)\mathbf{w}_t  + \alpha \mathbf{v}_{t,i}$. Note that 
\begin{align}
    \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} 
    &= \mathbf{\hat{B}}_{t}^\top\frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{\hat{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top \nonumber \\
    &= \frac{\beta}{n} \sum_{i=1}^n (1- \alpha\langle \mathbf{w}_t, \mathbf{w}_{t,i} \rangle)(\mathbf{w}_t - \mathbf{v}_{t,i})\mathbf{w}_{t,i}^\top \nonumber \\
    &= \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(\mathbf{w}_t - \mathbf{v}_{t,i})((1-\alpha)\mathbf{w}_t + \alpha \mathbf{v}_{t,i})^\top \nonumber \\
    &= \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)\mathbf{w}_t\mathbf{w}_t^\top  \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})\alpha\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \nonumber \\
    &\quad + \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})\alpha( \mathbf{w}_t \mathbf{v}_{t,i}^\top +  \mathbf{v}_{t,i}\mathbf{w}_t^\top ) \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i}) \mathbf{v}_{t,i}\mathbf{w}_t^\top  \nonumber
\end{align}
Making the same computation for the transposed term $\mathbf{\nabla}^\top \mathbf{\hat{B}}_{t}$ and rearranging terms yields
\begin{align}
    \mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} + \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t}
    &=  \frac{2\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)\mathbf{w}_t\mathbf{w}_t^\top  \nonumber \\
    &\quad - \frac{2\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})\alpha\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \nonumber \\
    &\quad - \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-2\alpha)( \mathbf{w}_t \mathbf{v}_{t,i}^\top +  \mathbf{v}_{t,i}\mathbf{w}_t^\top ) \nonumber
\end{align}
Recall that we need a lower bound on the minimum singular value of $\mathbf{I}_k - (\mathbf{\hat{B}}_{t}^\top \mathbf{\nabla} + \mathbf{\nabla}^\top \mathbf{\hat{B}}_{t})$. The positive definite terms in this matrix are given as follows:
\begin{align}
    \mathbf{I}_k + \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2)\alpha\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top, 
\end{align}
which has minimum singular value lower bounded by $1+ \beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2)\alpha E_0 \mu_\ast^2$. The non-positive definite terms are given as follows:
\begin{align}
   &- \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)\mathbf{w}_t\mathbf{w}_t^\top \nonumber \\
   &\quad + \frac{\beta}{n} \sum_{i=1}^n \alpha^3 (\mathbf{w}_t^\top \mathbf{v}_{t,i})\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \nonumber \\
   &\quad + \frac{\beta}{n} \sum_{i=1}^n (1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 - \alpha^2 \mathbf{w}_t^\top \mathbf{v}_{t,i})(1-\alpha)( \mathbf{w}_t \mathbf{v}_{t,i}^\top +  \mathbf{v}_{t,i}\mathbf{w}_t^\top )
\end{align}
The first line has maximum singular value at most $\beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 + \alpha^2\|\mathbf{w}_t\|_2 L_\ast)(1-\alpha )\|\mathbf{w}_t\|_2^2$. The second line has spectral norm at most $\beta \alpha^3 \|\mathbf{w}_t\|_2 L_\ast^3$ (???? verify this). The third line has spectral norm at most $ 2\beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2)(1-\alpha )\|\mathbf{w}_t\|_2 L_\ast + 2 \alpha^2(1-\alpha) L_\ast^2 \|\mathbf{w}_t\|_2^2$. Combining these, the sum of all the non-PD terms has spectral norm at most:\begin{align}
   & \beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 + \alpha^2\|\mathbf{w}_t\|_2 L_\ast)(1-\alpha )(\|\mathbf{w}_t\|_2^2+ 2\|\mathbf{w}_t\|_2 L_\ast) + \beta \alpha^3 \|\mathbf{w}_t\|_2 L_\ast^3
\end{align}
meaning that the contraction factor is given by
\begin{align}
    \frac{1 - (1 - \alpha \|\mathbf{w}_t\|_2^2)\beta (\alpha^2 E_0 \mu_{\ast}^2 - 2 \alpha(1-\alpha)\|\mathbf{w}_t\|_2 L_\ast)}{\left(1+p- \beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 + \alpha^2\|\mathbf{w}_t\|_2 L_\ast)(1-\alpha )(\|\mathbf{w}_t\|_2^2+ 2\|\mathbf{w}_t\|_2 L_\ast) - \beta \alpha^3 \|\mathbf{w}_t\|_2 L_\ast^3\right)^{0.5}}
\end{align}
where $p=\beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2)\alpha E_0 \mu_\ast^2$. Assume $\mu_{\ast} = 1-\delta$, $L_{\ast}= 1+\delta$, $E_0 = 0.5$. For what values of $\delta, \alpha, \beta, \|\mathbf{w}_t\|_2$ is the above less than 1? 

Assume perfect task diversity, i.e. $\mu_\ast = L_\ast = 1$. Also let $E_0=0.5$. Then
\begin{align}
    \frac{1 - \beta(1 - \alpha \|\mathbf{w}_t\|_2^2) (0.5 \alpha^2  - 2 \alpha(1-\alpha)\|\mathbf{w}_t\|_2 )}{\left(1+p- \beta(1-\alpha)(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2 + \alpha^2\|\mathbf{w}_t\|_2 )(\|\mathbf{w}_t\|_2^2+ 2\|\mathbf{w}_t\|_2 ) - \beta \alpha^3 \|\mathbf{w}_t\|_2 \right)^{0.5}}
\end{align}
where $p = \beta(1- \alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^2)\alpha/2$. Assume $\|\mathbf{w}_t\|_2 = 0.5 = E_0$. Then we can choose $\alpha=1$ to obtain contraction.


Roughly speaking, assuming high task diversity, we need $\|\mathbf{w}_t\|_2 \leq E_0$ for contraction, or , $\leq E_t$. Intuitively this makes sense based on the coefficient of $\mathbf{\hat{B}}_t$. But there is no reason why $\|\mathbf{w}_t\|_2$ should be this small.

If we choose $\alpha =1$, we have \begin{align}
    \frac{1 - \beta(1 -  \|\mathbf{w}_t\|_2^2)E_0  )}{\left(1+\beta. E_0 - \beta \|\mathbf{w}_t\|_2 \right)^{0.5}}
\end{align}


For the rest of the analysis we will assume that $\|\mathbf{w}_t\|_2 = 0$. This can be enforced by setting $\mathbf{w}_t = \mathbf{0}_d$ at the start of each iteration. Note that it is possible to show convergence with nonzero $\mathbf{w}_t$ (see Appendix \ref{app:maml}) but doing so requires a complicated upper bound on $\|\mathbf{w}_t\|_2$ without setting $\|\mathbf{w}_t\|_2 = 0$.

Thus, with $\mathbf{w}_t = \mathbf{0}_d$, we have
\begin{align}
    \mathbf{B}_{t+1} 
    &= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  \right)
    +   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top \nonumber 
\end{align}
where $\mathbf{w}_{t,i} =  \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$.
Therefore,
\begin{align}
    \dist_{t+1}&\leq \dist_t \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  \right\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2 \leq \dist_t (1- \alpha\beta E_0 \mu_\ast^2 )\|\mathbf{R}_{t+1}^{-1}\|_2
\end{align}
% where 
% \begin{align}
%     &\left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \nonumber\\
%     &\leq \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|  + \left\| \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \\
%     &\leq 1 - \beta (\alpha E_0 \mu_\ast^2 - (1- \alpha)) + \left\| \frac{\alpha \beta}{n}\sum_{i=1}^n \mathbf{w}_{t} ( (1-\alpha)\|\mathbf{w}_{t}\|_2^2 + \alpha \mathbf{w}_t^\top \mathbf{\hat{B}}^\top_t \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})   ((1- \alpha) \mathbf{w}_{t}^\top + \alpha \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t)  \right\|_2  \nonumber \\
%     &\leq 1 - \beta (\alpha E_0 \mu_\ast^2 - (1- \alpha)) + \left\|\mathbf{w}_{t}\mathbf{w}_{t}^\top  \frac{\alpha(1- \alpha) \beta}{n}\sum_{i=1}^n ( (1-\alpha)\|\mathbf{w}_{t}\|_2^2 + \alpha \mathbf{w}_t^\top \mathbf{\hat{B}}^\top_t \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})      \right\|_2  \nonumber  \\
%     &\quad + \left\| \frac{\alpha^2 \beta}{n}\sum_{i=1}^n \mathbf{w}_{t} ( (1-\alpha)\|\mathbf{w}_{t}\|_2^2 + \alpha \mathbf{w}_t^\top \mathbf{\hat{B}}^\top_t \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})   \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t  \right\|_2  \\
%     &\leq 1 - \beta (\alpha E_0 \mu_\ast^2 - (1- \alpha)) + \alpha(1 - \alpha)^2 \beta \|\mathbf{w}_t\|_2^4 + \alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3 L_\ast + \alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3 L_\ast + \alpha^3 \beta \|\mathbf{w}_t\|_2^2 L_\ast^2  \\
%     &= 1 -  \alpha\beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha(1 - \alpha)^2 \beta \|\mathbf{w}_t\|_2^4 + 2\alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3 L_\ast + \alpha^3 \beta \|\mathbf{w}_t\|_2^2 L_\ast^2 %\\
%     % &------- \\
%     % &\leq 1 - \beta (\alpha E_0 \mu_\ast - (1- \alpha)) + \alpha \beta (1-\alpha)((1-\alpha)+\alpha ) + \alpha \beta \alpha((1-\alpha) +\alpha L_\ast) \\
%     % &= 1 - \beta \alpha E_0 \mu_\ast + \beta - \beta \alpha + \alpha \beta  - \alpha^2 \beta + \alpha^2 \beta - \alpha^3 \beta + \alpha^3 \beta L_\ast \\
%     % &= 1 - \beta (\alpha E_0 \mu_\ast-1)  - \alpha^3 \beta (1- L_\ast) 
% \end{align}
% In the best case scenario, $\mu_\ast^2 = L_\ast^2 = 1/k$.  Then
% \begin{align}
%     &\left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 \\
%     &\leq 1 -  \alpha\beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha(1 - \alpha)^2 \beta \|\mathbf{w}_t\|_2^4 + 2\alpha^2 (1 - \alpha)\beta \|\mathbf{w}_t\|_2^3/\sqrt{k} + \alpha^3 \beta \|\mathbf{w}_t\|_2^2/k %\\
%     % &----- \\
%     % &\leq 1 + \beta \alpha \frac{k - E_0}{k}  - \alpha^3 \beta \frac{k-1}{k} \\
%     % &= 1 + \beta \alpha \frac{k - E_0 - \alpha^2(k-1)}{k}
% \end{align}
% If we  assume that $\mathbf{w}_t = \mathbf{0}$, we have
% \begin{align}
%     \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 
%     &\leq 1 -  \alpha\beta E_0 \mu_\ast^2 + (1 - \alpha)\beta,
% \end{align}
% where the RHS is less than 1 for $\alpha$ close to 1. 
% If we alternatively assume that $\alpha = 1$, we have
% \begin{align}
%      \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 
%     &\leq 1 -  \beta E_0 \mu_\ast^2 + \beta\|\mathbf{w}_t\|_2^2 L_\ast^2,
% \end{align}
% where the RHS is less than 1 for $\|\mathbf{w}_t\|_2^2  \leq E_0 \frac{\mu_\ast^2}{L_\ast^2}$.
% If $\alpha =1$ and $\mathbf{w}_t = \mathbf{0}$, we have
% \begin{align}
%      \left\|\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top  \right\|_2 
%     &\leq 1 -  \beta E_0\mu_\ast^2
% \end{align}
% This makes sense because it matches the bound from ANIL with $\alpha=1$.


% ---------

Next, using $\mathbf{B}_{t+1} = \mathbf{\hat{B}}_t - \frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_t\mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top$ and $ \mathbf{B}_{t+1}^\top\mathbf{{B}}_{t+1} =\mathbf{R}_{t+1}^\top\mathbf{{R}}_{t+1}  $, we have
\begin{align}
    &\sigma_{\min}^2(\mathbf{R}_{t+1}) \nonumber\\
    &= \sigma_{\min}(\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}) \nonumber \\
    &= \sigma_{\min}\Bigg(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t\mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top \nonumber \\
    &\quad - \left(\frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t\mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right)^\top \nonumber \\
    &\quad + \left(\frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t\mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right)^\top\left(\frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t\mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right) \Bigg) \nonumber \\
    &\geq \sigma_{\min}\left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} \right) -2 \left\|\frac{\beta}{n}\sum_{i=1}^n (\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t\mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right\|_2 \nonumber \\
    &= 1 -2 \left\|\frac{\beta}{n}\sum_{i=1}^n (\mathbf{w}_{t,i} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top\right\|_2 \nonumber \\
\end{align}


-------



Next, note that we can write the MAML outer loop representation update as:
\begin{align}
    \mathbf{B}_{t+1}&= \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top  \nonumber \\
    &\quad + \mathbf{\hat{B}}_{t} \left(\frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top \right)
    -   \mathbf{\hat{B}}_{\ast}\frac{\alpha \beta}{n}\sum_{i=1}^n  \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle  \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top   \\
    &= \mathbf{B}_{ANIL} + \mathbf{B}'
\end{align}
where $\mathbf{B}_{ANIL} \coloneqq \mathbf{\hat{B}}_{t} \left(\mathbf{I}_d -  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top$ and $\mathbf{B}' \coloneqq  \frac{\alpha \beta}{n}\sum_{i=1}^n  \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle (\mathbf{\hat{B}}_{t}\mathbf{w}_{t} -  \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i}) \mathbf{w}_{t,i}^\top$.
    From earlier analysis, we know that
        $\sigma_{\min}(\mathbf{B}_{ANIL}) \geq 1$,
    so we have 
\begin{align}
    \sigma_{\min}^2(\mathbf{R}_{t+1}) &= \sigma_{\min}(\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}) \nonumber \\
    &=\sigma_{\min}(\mathbf{B}_{ANIL}^\top \mathbf{B}_{ANIL} + \mathbf{B}_{ANIL}^\top \mathbf{B}' + (\mathbf{B}')^\top \mathbf{B}_{ANIL} + (\mathbf{B}')^\top \mathbf{B}') \nonumber \\
    &\geq  \sigma_{\min}^2(\mathbf{B}_{ANIL}) - 2 \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}') +  \sigma_{\min}^2( \mathbf{B}') \nonumber \\
    &\geq 1 - 2 \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}') 
\end{align}
Note that $\sigma_{\min}^2( \mathbf{B}')$ may be zero, so we drop it. If $\mathbf{w}_t = \mathbf{0}$, we have $\sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}') = 0$, so we recover the convergence rate from ANIL (of $1 - \beta E_0 \mu_\ast^2$). Otherwise, we have  
\begin{align}
    \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}')  &\leq  \sigma_{\max}(\mathbf{B}_{ANIL}^\top) \sigma_{\max}(\mathbf{B}')  \nonumber \\
    &\leq (1 - \alpha \beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha \beta L_\ast^2 + (1-\alpha)\beta L_\ast \|\mathbf{w}_t\|_2 ) \sigma_{\max}(\mathbf{B}') \nonumber \\
    &\leq \Big(1 - \alpha \beta E_0 \mu_\ast^2 + (1 - \alpha)\beta + \alpha \beta L_\ast^2 + (1-\alpha)\beta L_\ast \|\mathbf{w}_t\|_2 \Big) \nonumber \\
    &\quad \times \alpha \beta\Big((1-\alpha)^2 \|\mathbf{w}_t\|_2^4  + 2 \alpha(1-\alpha)\|\mathbf{w}_t\|_2^3 L_\ast + \alpha^2 \|\mathbf{w}_t\|_2^2 L_\ast^2 \Big) .
\end{align}
Now, if $\alpha=1$, we have
\begin{align}
    \sigma_{\max}(\mathbf{B}_{ANIL}^\top \mathbf{B}')  
    &\leq \Big(1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  \Big)  \beta  \|\mathbf{w}_t\|_2^2 L_\ast^2 
\end{align}
{
so we obtain
\begin{align}
    \dist_{t+1}&\leq \dist_t \frac{1 -  \beta E_0 \mu_\ast^2 + \beta\|\mathbf{w}_t\|_2^2 L_\ast^2}{\sqrt{1 - 2\Big(1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  \Big)  \beta   \|\mathbf{w}_t\|_2^2 L_\ast^2 }} 
\end{align}
where the contraction factor is less than $1-c$ if and only if
\begin{align}
    \|\mathbf{w}_t\|_2^2 &\leq \frac{1}{F}\left( -(A + (1-c)^2 D)+ (1-c)\sqrt{1 + 2 AD + (1-c)^2D}\right) \label{88}
    % \frac{2 \beta L_{\ast}^2(2 - 2 \beta E_0 \mu_\ast^2+\beta L_{\ast}^2 ) + \beta L_\ast^2 \sqrt{ (Z + 2)^2 - 4 \beta^2 E_0 L_\ast^2 Z}}{4\beta E_0 \mu_\ast^2 - 2 \beta^2 E_0^2 \mu_{\ast}^4 }
\end{align}
where $A\coloneqq 1 - \beta E_0 \mu_\ast^2$, $D\coloneqq 1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  $, $F \coloneqq \beta L_\ast^2$. 
Note that 
$1 + 2 A D + (1-c)^2 D^2 \geq 0$ for all $\beta \in (0,1]$, so we do not have to worry about a complex square root.  
The RHS of \eqref{88} is positive for all $c>0$ such that $
    (1-c)^2 > {A^2}$, i.e., $0< c < \beta E_0 \mu_\ast^2$. This leads to the following theorem.
% $< \beta E_0 \mu_\ast^2$. So this result says that for any $c < \beta E_0 \mu_\ast^2$, there exists some $\delta > 0$ such that as long as $\|\mathbf{w}_t\|_2^2 \leq \delta$ for all $t$, we have linear convergence of the representation with rate $1 - c$ for all $t$.
}

\begin{thm}
For $\alpha=1$, $\beta \in (0,1]$ and any $0 < c < \beta E_0 \mu_\ast^2$, if for all $t = 1,\dots,T$,
\begin{align}
   \|\mathbf{w}_t\|_2^2 &\leq \frac{1}{F}\left( -(A + (1-c)^2 D)+ (1-c)\sqrt{1 + 2 AD + (1-c)^2D}\right),
    % \frac{2 \beta L_{\ast}^2(2 - 2 \beta E_0 \mu_\ast^2+\beta L_{\ast}^2 ) + \beta L_\ast^2 \sqrt{ (Z + 2)^2 - 4 \beta^2 E_0 L_\ast^2 Z}}{4\beta E_0 \mu_\ast^2 - 2 \beta^2 E_0^2 \mu_{\ast}^4 }
\end{align}
where $A\coloneqq 1 - \beta E_0 \mu_\ast^2$, $D\coloneqq 1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  $, $F \coloneqq \beta L_\ast^2$, and the representation $\mathbf{B}_t$ is orthogonalized at the end of each outer loop, then MAML learns the representation at a linear rate with contraction factor at most $1-c$, i.e.
\begin{align}
    \dist(\mathbf{\hat{B}}_T, \mathbf{\hat{B}}_\ast) &\leq (1 - c)^{T}\dist(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast).
\end{align}
\end{thm}

Intuitively: in the outer loop update, the heads serve to remove energy from the representation resulting from the inner loop and add energy to $\mathbf{B}_\ast$. But if the representation is updated during the inner loop, then it no longer contains enough energy from $\mathbf{B}_t$ such that the energy in $\mathbf{B}_t$ can be reduced by the heads in the outer update. However, if we send $\mathbf{w}_t$ to zero, then the inner loop gradient of the representation goes to zero, so effectively we remove the inner loop update step for the representation.







% So the inner update step for the representation seems to hurt representation learning, since it moves energy in the update for $\mathbf{B}_{t+1}$ from $\mathbf{B}_\ast$ to $\mathbf{B}_t$ compared to ANIL. But if $\mathbf{w}_t$ is close to zero, then this perturbation is small, so we should still learn the representation.

% The only negative term is $ - \beta(1+\alpha\lambda)\frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top$, which is not enough for contraction...

% now just need to ensure $\mathbf{B}_{t,i}$ and $\mathbf{B}_{t+1}$ are well-conditioned

% To show that energy is lower bounded, we need to 

% $\mathbf{w}_{t,i} \mathbf{w}_{t,i}$

If $\left\|\mathbf{w}_t - \frac{1}{n}\sum_{i=1}^n \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}\right\|_2\leq \gamma_t$, then 

WLOG let $\mathbf{w}_{\ast,i} = \mathbf{\bar{w}}+ \mathbf{\tilde{w}}_{\ast,i}$, where the $\mathbf{\tilde{w}}_{\ast,i}$'s are well-conditioned.


We have 
\begin{align}
    &\|\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 \nonumber \\
    &\leq \|\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{B}_t\|_2(
    1 -\beta(1+\alpha\lambda)((1-\tau)E_0\mu_\ast^2 ....)
    )
\end{align}
We need to upper bound the following matrix norm:
\begin{align}
    &\left\|\mathbf{I}_k - \beta(1+\alpha\lambda)\frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top + \beta \alpha \mathbf{w}_t\mathbf{w}_t^\top \frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top + \beta \alpha \lambda \mathbf{B}_t^\top\mathbf{B}_t^\top \frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right\|_2 \nonumber \\
    &\leq 1 - \beta\sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) + \beta \alpha ( L_{\mathbf{w}}^2  + \lambda \tau) \sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) \nonumber \\
    &\leq 1 - \beta\sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) + \beta \alpha ( L_{\mathbf{w}}^2  + \lambda \tau)((1-\alpha(1-\tau)) \|\mathbf{w}_t\|_2+ \sqrt{(1+\tau)}L_{\max} )^2 \nonumber \\
    &\leq  1  + \beta \alpha ( L_{\mathbf{w}}^2  + \lambda \tau)((1-\alpha(1-\tau)) \|\mathbf{w}_t\|_2+ \sqrt{(1+\tau)}L_{\max} )^2
    % &\leq 1  + \lambda \tau)((1-\alpha(1-\tau)) \|\mathbf{w}_t\|_2+ \sqrt{(1+\tau)}L_{\max} )^2
\end{align}
Meanwhile,
\begin{align}
   & \beta \lambda \left\|- (1+\alpha \lambda)\frac{1}{n}\sum_{i=1}^n (\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) + \alpha \mathbf{w}_t \mathbf{w}_t^\top(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) + \alpha \lambda \mathbf{B}_t \mathbf{B}_t^\top(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k)\right\|_2  \nonumber \\
   &\leq \tau'(\beta\lambda + \beta \alpha \lambda^2 + \beta \alpha \lambda L_{\mathbf{w}}^2 +  )
\end{align}

So after $T_1$ iterations, we have 
\begin{align}
    
\end{align}


Now, how may iterations do we need for $\mathbf{w}_t$ to converge?
\begin{align}
    \mathbf{w}_{t+1} &=\mathbf{w}_t - \beta \frac{1}{n} \sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\mathbf{w}_{t,i} +\beta \frac{1}{n} \sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{\hat{B}}_{\ast}\mathbf{w}_{\ast,i} \nonumber 
\end{align}

---------------

we have 

coefficient of $\mathbf{B}_t:$

$\mathbf{I}_k - \beta( \mathbf{I}_k - \alpha \mathbf{ww}^\top)\mathbf{A}^\top \mathbf{A}$




\begin{align}
    &\lambda_{\max}((\mathbf{I}_k - \beta( \mathbf{I}_k - \alpha \mathbf{ww}^\top)\mathbf{A}^\top \mathbf{A})^\top (\mathbf{I}_k - \beta( \mathbf{I}_k - \alpha \mathbf{ww}^\top)\mathbf{A}^\top \mathbf{A})) 
    \nonumber \\
    &\leq 1 - \beta \lambda_{\min}(( \mathbf{I}_k - \alpha \mathbf{ww}^\top)\mathbf{A}^\top \mathbf{A} + \mathbf{A}^\top \mathbf{A}( \mathbf{I}_k - \alpha \mathbf{ww}^\top)) +O(\beta^2) \nonumber \\
    &= 1 - \beta \lambda_{\min}(2\mathbf{A}^\top \mathbf{A} - \alpha \mathbf{ww}^\top\mathbf{A}^\top \mathbf{A} - \alpha \mathbf{A}^\top \mathbf{A} \mathbf{ww}^\top ) +O(\beta^2) 
\end{align}




also need to upper bound lambda min... but it should be the same

empirically: coeff of $\mathbf{B}_t$ is less than 1 for random $\mathbf{w}_t$ at the start of each round (but cannot get convergence in this case). but, if you replace wt in the coeff of Bt with a random vector, the norm may be greater than 1.


Current status: have proof that shows that:
\begin{align}
    (\mathbf{I} - \alpha \mathbf{w}_t \mathbf{w}_t^\top) \left(\frac{1}{n}\sum_{i=1}^n ((1-\alpha)\mathbf{w}_t + \alpha \mathbf{B}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})((1-\alpha)\mathbf{w}_t + \alpha \mathbf{B}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i})^\top \right) \succeq f(\alpha) \mathbf{I}
\end{align}
where $ f(\alpha)$ is a strictly positive function of $\alpha$, as long as $\alpha \leq \sqrt{3}/2$. We also need: $\|\mathbf{w}_t\|_2 = \|\mathbf{B}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\|_2=1$ for all $i$.

Concerns: 

- requires $\alpha$ bounded away from 1. But we may need require $\alpha \approx 1$ to show that $\mathbf{B}_t$ stays almost orthogonal.

In coeff of $\mathbf{B}_t$, we will have:

$1+ \beta \alpha \lambda \tau + \beta c \tau + \beta c' \tau^2 - \beta f(\alpha)$

$\implies$ need $\tau$ to be very large, can we accomplish this with small $\alpha$, smaller $\lambda$?

- If we do not have exact normalization $\|\mathbf{w}_t\|_2=1$, argument gets messy. but non-normalization of $\mathbf{B}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$ is easy to deal with as long as the average have norm at most 1.


To show that $\mathbf{B}$ stays almost orthogonal, we need to show that the gradient can be written as the product of I - BTB terms


Issues:

- instead of $\mathbf{B}_{t}$ we have $\mathbf{B}_{t,i}$ in two places, and the difference between these terms grows with $\alpha$

- which implies we should choose $\alpha$ to be small. but we also have $\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t$, so we need a $(1-\alpha)$ error term, so need to choose $\alpha$ large to get rid of this...

We have 
\begin{align}
    \nabla &= \frac{}{}
\end{align}




The outer loop updates can be written as:
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{{B}}_t  - \frac{\beta}{n}\sum_{i=1}^n\nabla_{\mathbf{B}} \mathcal{L}_i(\mathbf{{B}}_t, \mathbf{w}_{t,i}) =  \underbrace{\mathbf{{B}}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)}_{\text{prior term}} +  \underbrace{\mathbf{{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right)}_{\text{signal term}} \label{upd_rep_anil_out_pop}
\end{align}
From \eqref{upd_head_anil_out_pop}, we can see that if the inner loop updates $\{\mathbf{w}_{t,i}\}_i$ are well-conditioned, then the outer loop update of the representation subtracts energy from $\mathbf{B}_t$ (small prior term) and replaces it with energy from $\mathbf{B}_\ast$ (large signal term). 

\begin{rem}
This is exactly where {\em task diversity} plays a crucial role: the more diverse that the $\mathbf{w}_{\ast,i}$'s are, the more diverse (better conditioned) that the $\mathbf{w}_{t,i}$'s are due to the inner loop update. If instead there was no inner loop update, i.e. $\mathbf{B}_{t+1} = \mathbf{B}_t(\mathbf{I}_k - \beta \mathbf{w}_t \mathbf{w}_t^\top) + \mathbf{B}_\ast\left(\frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\right)\mathbf{w}_t^\top$, then we would not be able to learn $\mathbf{B}_\ast$ since the column space of $\mathbf{B}_{t+1}$ only becomes closer to the column space of $\mathbf{B}_{\ast}$ in one direction on each iteration, so there is no reason why all $k$ directions would be learned.
\end{rem}

Now multiply both sides of \eqref{upd_rep_anil_out_pop} by $\mathbf{\hat{B}}_{\ast,\perp}^\top$ to obtain $\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{B}_{t+1} = \mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{\hat{B}}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)$, then take the spectral norm of both sides and use the Cauchy-Schwarz inequality to yield
\begin{align}
\text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_{\ast} ) 
&\leq \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_{\ast} ) \bigg\|  \mathbf{I}_k - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\bigg\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2 %\label{ineq1}
\end{align}
where $\mathbf{\hat{B}}_{t+1} \mathbf{R}_{t+1} = \mathbf{B}_{t+1}$ is the QR-decomposition of $\mathbf{B}_{t+1}$. For $\beta \leq \|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\|_2^{-1}$, we have that $\left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 \leq 1 - \beta\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)$, where
\begin{align}
\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)
&= \sigma_{\min}\Bigg(\frac{1}{n} \sum_{i=1}^n (1-\alpha)^2\mathbf{w}_{t} \mathbf{w}_{t}^\top + \alpha (1-\alpha)\mathbf{w}_{t} \mathbf{w}_{\ast,t,i}\mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \nonumber \\
&\quad \quad  + \alpha (1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t}^\top + \alpha^2 \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}\mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t  \Bigg) \nonumber \\
% &\geq -(1-\alpha)^2 L^2 - 2 \alpha (1 - \alpha)L L_\ast  + \alpha^2 \sigma_{\min}\left(\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right)  \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t\right) \nonumber \\
&\geq  \alpha^2 E_0 \mu_\ast^2 - 2 \alpha (1 - \alpha)L_\ast^2  \label{weyl1}
\end{align}
% where \eqref{weyl1} follows from
by Weyl's inequality, $\mathbf{w}_t\mathbf{w}_t^\top \succeq \mathbf{0}$, and the fact that \begin{align} \sigma_{\min}\left(\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right)  \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t\right)&\geq \sigma_{\min}^2\big(\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\big) \sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right) \nonumber \\
&\geq E_0 \mu_\ast^2
\end{align}
by  the relation $\sigma_{\min}^2\big(\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\big) = 1 - \dist^2(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast )$ and inductive hypothesis 1.
Thus we have
\begin{align}
    \left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 &\leq 1    -  \beta \alpha^2 E_0 \mu_\ast^2 + 2\beta \alpha(1-\alpha)L_\ast^2     \label{contract}
\end{align}
Note that the RHS is strictly less than 1 for sufficiently large values of $\alpha$ and sufficiently diverse heads (i.e. $\mu_\ast \approx L_\ast$). We now must  show that $\|\mathbf{R}_{t+1}^{-1}\|_2$ is small, or equivalently, $\sigma_{\min}(\mathbf{R}_{t+1})$ is large, to complete the proof. First, we write $\mathbf{B}_{t+1} = \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top$, then
\begin{align}
    \sigma_{\min}^2\left( \mathbf{R}_{t+1}\right) \!&=\! \sigma_{\min}\left(\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\right)\!\geq \! \sigma_{\min}(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t})\! - \!2\left\| \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i}\! -\! \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top\right\|_2  \nonumber% \label{weyl2}
    % &= \mathbf{I}_{k} - \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber
\end{align}
% where \eqref{weyl2} follows from Weyl's inequality.
% where $O(\beta^2)$ denotes a PSD matrix whose spectral norm is $O(\beta^2)$, and 
Next, since $\alpha = 1$,  
    $\mathbf{w}_{t,i} = \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$
and the matrix in the spectral norm above is zero:
% in \eqref{weyl2}
\begin{align}
    \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top = \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top  = \mathbf{0}.
\end{align}
Therefore, by using \eqref{contract} with $\alpha =1$ and $\beta \leq \|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\|_2^{-1} \leq \frac{1}{L_\ast^2}$, we obtain
\begin{align}
    \dist\left(\mathbf{\hat{B}}_{t+1},\mathbf{\hat{B}}_\ast \right) 
     &\leq({1 -  \beta  E_0 \mu_\ast^2  })\dist\left(\mathbf{\hat{B}}_{t},\mathbf{\hat{B}}_\ast \right) \leq ({1 -  \beta  E_0 \mu_\ast^2  })^t\dist\left(\mathbf{\hat{B}}_{0},\mathbf{\hat{B}}_\ast \right),
\end{align}
completing the proof.

==> MainResults.tex <==
\section{Main Results}

In this section we formalize our intuition discussed previously and prove that both MAML and ANIL and their first-order approximations are capable learning the column space of the ground-truth representation.
% Now we formalize these insights and present our main results.
% First we establish a notion of task diversity.
% \begin{definition}[Task Diversity] 
% We say that a set of vectors $\mathcal{S}\coloneqq \{\mathbf{w}_i\}_{i} \subset \mathbb{R}^{k}$ is {\em $({\mu},{L})$-diverse}  if $\mu^2 \leq \sigma_{\min}\left(\frac{1}{|\mathcal{S}|}\sum_{i} \mathbf{w}_{i}\mathbf{w}_{i}^\top \right)\leq\sigma_{\max}\left(\frac{1}{|\mathcal{S}|}\sum_{i} \mathbf{w}_{i}\mathbf{w}_{i}^\top \right) \leq L^2$.
% \end{definition}
% Thus, if $\{\mathbf{w}_i\}_{i=1}^n$ do not span $\mathbf{R}^k$, they have diversity $(0,\sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{i}\mathbf{w}_{i}^\top \right))$. Otherwise, they have nonzero diversity, with diversity approaching 1 the better conditioned they are. 
To do so, we first make the following assumption concerning the diversity of the sampled ground-truth heads.
% benign conditions on the distribution $\nu$ of the ground-truth heads which enable us to establish the diversity of the ground-truth heads sampled on each iteration.
% Under this assumption on $\nu$, we can easily compute high-probability bounds on the diversity parameters $(\mu,L)$ for the sets of $n$ ground-truth heads sampled on each iteration.
% In particular, 

\begin{assumption}[Task diversity]\label{assump:tasks_diverse_main}
The eigenvalues of the symmetric matrix  $\boldsymbol{{\Psi}}_{\ast,t} \coloneqq (\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top)$ are uniformly bounded below and above by $\mu_\ast^2$ and $L_\ast^2$, respectively\footnote{We could instead assume the ground-truth heads are sub-gaussian and use standard concentration results show that with $n\!=\!\Omega(k+\log(T))$, the set of ground-truth heads $\{\mathbf{w}_{\ast,t,i}\}_{i=1}^n$ sampled on iteration $t$ are $(1+O(1),1-O(1))$-diverse for all $T$ iterations with high probability, but instead we assume generic bounds for simplicity.}, i.e., $\mu_\ast^2 \mathbf{I} \preceq \boldsymbol{{\Psi}}_{\ast,t} \preceq L_\ast^2 \mathbf{I}$, for all $ t \in [T]$.
\end{assumption} 


The lower bound on the eigenvalues of the matrix $\boldsymbol{{\Psi}}_{\ast,t}$ ensures that the $k\times k$ matrix $\boldsymbol{{\Psi}}_{\ast,t}$ is full rank and hence the vectors $\{\mathbf{w}_{\ast,t,i}\}_{i=1}^n$ span $\mathbb{R}^k$, therefore they are diverse. However, the diversity level of the tasks is defined by ratio of the eigenvalues of the  matrix $\boldsymbol{{\Psi}}_{\ast,t}$, i.e., $\kappa_\ast\coloneqq \frac{L_{\ast}}{\mu_\ast}$. If this ratio is close to 1, then the ground-truth heads are very diverse and have equal energy in all directions. On the other hand, if $\kappa_\ast$ is large, then the ground-truth heads are not very diverse as their energy is mostly focused in  a specific direction. Hence, as the following results reveal, smaller  $\kappa_\ast$ leads to faster convergence for ANIL and MAML.


%We say that the ground-truth heads are very diverse if they are evenly spread in all directions in $\mathbb{R}^k$. Formally, this means that  $\kappa_\ast\!\coloneqq\! \frac{L_{\ast}}{\mu_\ast}\! \approx \! 1$. On the other hand, if the ground-truth heads do not span $\mathbb{R}^k$, i.e. $\mu_\ast\!=\!0$, then they are not diverse. 




%  and $\kappa_{\ast,\max}\coloneqq \frac{L_{\max}}{\mu_\ast}$. 
% Next, we characterize the diversity of the inner loop-updated heads in terms of $L_\ast$ and $\mu_\ast$.
% Next, we investigate whether ANIL and  MAML recover $\text{col}(\mathbf{B}_\ast)$, starting with ANIL.
% If  $\frac{L}{\mu}$ is close to 1, then  $\{\mathbf{w}_i\}_{i}$ is very diverse. On the other hand, if $\{\mathbf{w}_i\}_{i}$ does not span $\mathbb{R}^k$, i.e. $\mu=0$, then  $\{\mathbf{w}_i\}_{i}$ is not diverse. 
% We show that neither MAML nor ANIL learn $\col(\mathbf{B}_\ast)$ when the set of ground-truth heads $\{\mathbf{w}_{\ast,i}\}_i$ used for training is not diverse in Section \ref{sec:negative}.
% It is standard in the linear representation learning setting to assume that the set of ground-truth heads $\{\mathbf{w}_{\ast,i}\}_i$ used for training are diverse \citep{du2020fewshot, tripuraneni2020provable}, 
%Task diversity across the training set was shown to be necessary to representation learning from a statistical perspective by \citet{tripuraneni2020theory}. Here, we show how the dynamics of MAML and ANIL depend on task diversity to learn a quality representation.


{
% After formalizing the required assumptions,
Now we are ready to state our main results for the ANIL and FO-ANIL algorithms in the infinite sample case. % $m_{in}\! = \!m_{out}\! =\! \infty$.
% in which ANIL and MAML are run on the population losses for each task.
\begin{thm}\label{thm:anil_pop_main}
% \begin{thm}[ANIL, Infinite Samples]
Consider the infinite sample case for ANIL and FO-ANIL, where  $m_{in}\!=\!m_{out}\!= \!\infty$. Further, suppose the conditions in Assumption \ref{assump:tasks_diverse_main} hold, the initial weights are selected as $\mathbf{w}_0 = \mathbf{0}_k$ and ${\alpha}\mathbf{B}_0^\top\mathbf{B}_0  = \mathbf{I}_k$. Let the step sizes are chosen as $\alpha = O(\nicefrac{1}{L_{\ast}})$ and 
 $\beta = O({\alpha}{\kappa_{\ast}^{-4}})$ for ANIL and $\beta = O({\alpha}{\kappa_{\ast}^{-4}\min(1,{\nicefrac{\mu_\ast^2}{\eta_\ast^{2}}}}))$ for FO-ANIL, where ${\eta}_\ast$ satisfies $\|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\|_2 \leq \eta_\ast$ for all times $t\in [T]$ almost surely. If the initial error satisfies the condition $\dist_0 \leq \sqrt{0.9}$, then almost surely for both  ANIL and FO-ANIL we have,
\begin{align}
    \dist(\mathbf{{B}}_T, \mathbf{{B}}_\ast) \leq \left(1 - 0.5\beta \alpha E_0 \mu_\ast^2   \right)^{T-1},
\end{align}
where 
 $E_0 \coloneqq  0.9 - \dist_0^2$.
%  Suppose Assumption \ref{assump:init} holds. 
\end{thm}
Theorem \ref{thm:anil_pop_main} shows that both FO-ANIL and Exact ANIL learn a representation that approaches the ground-truth exponentially fast as long as the initial representation $\mathbf{B}_0$ is normalized and is a constant distance away from the ground-truth, the initial head $\mathbf{w}_0=\mathbf{0}$, and the sampled tasks are diverse. {Note that $\beta$ is larger for ANIL and hence its convergence is faster, demonstrating the benefit of second-order updates.}

Next, we state our results for FO-MAML and Exact MAML for the same infinite sample setting. 
Due to the adaptation of both the representation and head, the MAML and FO-MAML updates involve  third- and fourth-order products of the ground-truth heads, unlike the ANIL and FO-ANIL updates which involve at most second-order products. 
% as opposed to only first- and second-order products as for ANIL.
To analyze the higher-order terms, we assume that the 
 energy in each ground-truth head is balanced. %\cite{thekumparampil2021statistically,collins2021exploiting,du2020fewshot,tripuraneni2020provable}.

\begin{assumption}[Task incoherence]\label{assump:tasks_main}
    For all times $t\in [T]$ and tasks $i \in [n]$, we almost surely have
$
    % \sigma_{\min}\big(\tfrac{1}{n}\!\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\big)\!&\geq\!\mu_\ast^2,\;   
    % \big\|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\big\|_2\!\leq\!\eta_\ast,\quad 
    % \sigma_{\max}\big(\tfrac{1}{n}\!\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\big)\!&\leq\!L_\ast^2,\; 
\|\mathbf{w}_{\ast,t,i}\|_2\!\leq\! c{\sqrt{k}}L_\ast 
$, where $c$ is a constant.
\end{assumption} 

Next, as discussed in Section \ref{sec:intuition}, MAML's adaptation of the representation complicates its ability to learn the ground-truth subspace. As a result, we require an additional condition to show that MAML learns the representation: the distance of the initialization to the ground-truth must small in the sense that it must scale with the task diversity and inversely with $k$. We formalize this in the following theorem. 

\begin{thm}\label{thm:maml_pop_main} Consider the infinite sample case for MAML, where $m_{in}=m_{out}= \infty$. Further, suppose the conditions in Assumptions \ref{assump:tasks_diverse_main} and \ref{assump:tasks_main} hold, the initial weights are selected as $\mathbf{w}_0 = \mathbf{0}_k$ and ${\alpha}\mathbf{B}_0^\top\mathbf{B}_0  = \mathbf{I}_k$, and the step sizes satisfy $\alpha = O({k^{-2/3} L_\ast^{-1} T^{-1/4}})$ and $ \beta = 
O({\alpha }{ \kappa_\ast^{-4} })$. If $\dist_0 =O({k}^{-0.75}\kappa_{\ast}^{-1.5})$, then almost surely 
\begin{align*}
    \dist(\mathbf{{B}}_T, \mathbf{{B}}_\ast) \leq \left(1 - 0.5\beta \alpha E_0 \mu_\ast^2   \right)^{T-1} ,
\end{align*}
where $E_0 \coloneqq  0.9 - \dist_0^2$.
\end{thm}
Theorem \ref{thm:maml_pop_main} shows that the initial representation learning error for MAML must scale as $O({k}^{-0.75}\kappa_{\ast}^{-1.5})$, which can be much smaller than the constant scaling that is sufficient for ANIL to learn the representation (see Theorem \ref{thm:anil_pop_main}). Next we give the main result for FO-MAML, which requires an additional condition that the norm of the average of the ground-truth heads sampled on each iteration is small. This condition arises due to the fact that the FO-MAML updates are approximations of the exact MAML updates, and thus have a bias that depends on the average of the ground-truth heads. Without control of this bias,  the iterates $\mathbf{B}_t$ and $\mathbf{w}_t$ may diverge. 
%\begin{itemize}
 %   \item If the initial error satisfies $\dist_0 =O({k}^{-0.5}\kappa_{\ast}^{-1})$, the outer loop stepsize is selected as $\beta = O({\alpha}{\kappa_{\ast}^{-4}})$, and the average of true heads is close to zero and almost surely satisfies $  \|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\|_2= O(k^{-1.5}\kappa_{\ast}^{-3} \mu_\ast) $, then the iterates of FO-MAML satisfy 
   % $$
    % \dist(\mathbf{{B}}_T, \mathbf{{B}}_\ast) \leq \left(1 - 0.5\beta \alpha E_0 \mu_\ast^2   \right)^{T-1}
    %$$
%\end{itemize}
%A. FO-MAML:
%\vspace{-2mm}
%\begin{enumerate}
%\vspace{-2mm}
%    \item Good initialization: $\dist_0 =O({k}^{-0.5}\kappa_{\ast}^{-1})$,
 %   \vspace{-2mm}
  %  \item Average true heads near zero: $  \|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\|_2= O(k^{-1.5}\kappa_{\ast}^{-3} \mu_\ast) $ almost surely for all $t\in [T]$.  
   % \vspace{-2mm}
%    \item Step size: $\beta = O({
%\alpha}{\kappa_{\ast}^{-4}})$.
%\vspace{-1mm}
%\end{enumerate}
%\vspace{-2mm}
%B. Exact MAML:
%\vspace{-2mm}
%\begin{enumerate}
%\vspace{-2mm}
 %   \item Good initialization: $\dist_0 =O({k}^{-0.75}\kappa_{\ast}^{-1.5})$, 
  %  \vspace{-2mm}
  %  \item Step size:  $\beta = 
%O({\alpha k^{-1}}{ \kappa_\ast^{-2} })$,
%\vspace{-2mm}
%\item Total iterations: $T = O( \tfrac{1}{\beta %\alpha^3 k^{2.5} L_{\ast}^4 \kappa_\ast})$.
%\end{enumerate}
%\vspace{-1mm}
%Then each algorithm learns a representation that %satisfies:
% \begin{assumption}[Fourth-order diversity]\label{assump:fourth_main} Define $\boldsymbol{\tilde{\Psi}}_t \coloneqq (\tfrac{1}{n}\sum_{i=1}^n \|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top) \; \forall t \in [T]$. 
% Then $\mu_\ast^4  \leq \sigma_{\min}(\boldsymbol{\tilde{\Psi}}_t)\leq \sigma_{\max}(\boldsymbol{\tilde{\Psi}}_t) \leq L_\ast^4 \; \forall t \in [T]$ almost surely.
% % \begin{align}
% %     % \mu_\ast^2 \leq  \tilde{\mu}_{\ast}^2  \leq \sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n \|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right) \leq  \sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n \|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right) \leq \tilde{L}_{\ast}^2 \leq L_\ast^2
% % \end{align}
% \end{assumption}
% Like Assumption \ref{assump:tasks_diverse_main}, Assumption \ref{assump:fourth_main} ensures that the ground-truth heads are well-spread, this time with an extra weighting by norm. It is needed for fourth-order products that arise in Exact MAML.
\begin{thm}\label{thm:fomaml_pop_main} Consider the infinite sample case for FO-MAML, where $m_{in}=m_{out}= \infty$. Further, suppose the conditions in Assumptions \ref{assump:tasks_diverse_main} and \ref{assump:tasks_main} hold, the initial weights are selected as $\mathbf{w}_0 = \mathbf{0}_k$ and ${\alpha}\mathbf{B}_0^\top\mathbf{B}_0  = \mathbf{I}_k$, and the step sizes satisfy $\alpha = O(\tfrac{1}{\sqrt{k}L_\ast})$ and $\beta = O({\alpha}{\kappa_{\ast}^{-4}})$. If the initial error satisfies $\dist_0 =O({k}^{-0.5}\kappa_{\ast}^{-1})$, and the average of the true heads  almost surely satisfies $  \|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\|_2= O(k^{-1.5}\kappa_{\ast}^{-3} \mu_\ast) $ for all times $t$, then almost surely
    $$
     \dist(\mathbf{{B}}_T, \mathbf{{B}}_\ast) \leq \left(1 - 0.5\beta \alpha E_0 \mu_\ast^2   \right)^{T-1},
    $$
    where $E_0 \coloneqq  0.9 - \dist_0^2$.
\end{thm}
Theorem \ref{thm:fomaml_pop_main} shows that FO-MAML learns $\col(\mathbf{B}_\ast)$ as long as the initial principal angle is small and $ \|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\|_2= O(k^{-1.5}\kappa_{\ast}^{-3} \mu_\ast) $ on all iterations, due to the biased updates.
Note that the FO-ANIL updates are also biased, but this bias scales with $\|\mathbf{I}_k-\alpha\mathbf{B}_t^\top \mathbf{B}_t\|_2$, which is eventually decreasing quickly enough to make the cumulative error induced by the bias negligible without any additional conditions.  In contrast, $\|\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t\|_2$ is not guaranteed to decrease for FO-MAML due to the inner loop adaptation of the representation, so we need the additional condition.



% (i) $\dist_0 =O({k}^{-0.75}\kappa_{\ast}^{-1.5})$, (ii) $\beta = 
% % O(\min(\tfrac{\alpha L_{\max}^2}{ \kappa_\ast^2 L_\ast^2}, \tfrac{\mu_\ast}{\alpha^3 L_{\max}^5  T }))$,
% O(\min({\alpha k}{ \kappa_\ast^{-2} }, \tfrac{1}{\alpha^3 k^{2.5} L_{\ast}^4 \kappa_\ast  T }))$.
%\beta \leq \min\left(\frac{\alpha E_0 L_{\max}^2 \mu_\ast^2}{6 L_\ast^4}, \frac{{E_0} \mu_\ast}{ 640 \alpha^3 L_{\max}^5 T}\right)
% \begin{enumerate}
%     % \item $\dist_0 =O(\kappa_{\ast,\max}^{-1})$, \item $\eta_\ast = O(\kappa_{\ast,\max}^{-3} \mu_\ast)$, \item $\beta = O({\alpha^2 L_{\max}}{\kappa_{\ast}^{-4}})$;
%     \item Exact MAML: $\dist_0 =O(\kappa_{\ast,\max}^{-1.5})$,
% $\beta = O(\min(\alpha \kappa_\ast^2 L_\ast^2/L_{\max}^2, \tfrac{1}{\alpha^3 T \kappa_{\ast,\max}L_{\max}^4}))$,  and Assumption \ref{assump:fourth} holds.
% \end{enumerate}

% Define 
%  $E_0\!\coloneqq\! 0.9 -\! \dist_0^2$ and assume $\dist_0 \leq \sqrt{0.9}$. 
% %  Suppose Assumption \ref{assump:init} holds. 
%  and set $\alpha = O(\tfrac{1}{L_{\max}})$ and 
%  $\beta = O({\alpha^2 L_{\max}}{\kappa_{\ast}^{-4}})$. Further, for $\kappa_{\ast,\max}\coloneqq \frac{L_{\max}}{\mu_\ast}$, assume:
%  $$\dist_0 =O(\kappa_{\ast,\max}^{-1})\quad \eta_\ast = O(\kappa_{\ast,\max}^{-3} \mu_\ast) $$
% For Exact MAML, we need $\dist_0 =O(\kappa_{\ast,\max}^{-1.5})$. 
% $\beta = O(\alpha \kappa_\ast^2 L_\ast^2/L_{\max}^2)$
% bounded fourth-order products




% simulate this.
% for exact maml, we must choose w = O(rt(alpha)). this causes dist_0 = O(kappa-1.5) regardless of choice of other params. for fo-maml, we can choose  w = O(alpha1.5), and w gradient admits less stringent initialization dependence. but strict eta-ast dependence. 


To the best of our knowledge, the above theorems  are the first results to show that ANIL, MAML, and their first-order approximations learn representations in any setting. Moreover, they are the first to show
how {\em task diversity} plays a key role in representation learning from an {optimization} perspective, to the best of our knowledge. 
% highlight the {\em importance of task diversity } to representation learning. 
Due the the restrictions on $\beta$ and $\alpha$, Theorems \ref{thm:anil_pop_main} and \ref{thm:maml_pop_main} show that the rate of contraction of principal angle distance diminishes with less task diversity. Thus, the more diverse the tasks, i.e. the smaller $\kappa_\ast$, the faster that ANIL and MAML learn the representation. Additionally, the less diverse the tasks, the more accurate initialization that MAML requires, and the tighter that the true heads must be centered around zero to control the FO-MAML bias.
%{\color{blue} Under ideal conditions, all algorithms converge }
% To the best of our knowledge, these are the first results to show
% how task diversity plays a key role in representation learning from an {\em optimization} perspective. 



}


% \textbf{Role of task diversity.} Due the the restrictions on $\beta$ and $\alpha$, Theorems \ref{thm:anil_pop_main} and \ref{thm:maml_pop_main} show that the rate of contraction of principal angle distance diminishes with less task diversity. Thus, the more diverse the tasks, i.e. the smaller $\kappa_\ast$, the faster that ANIL and MAML learn the representation. Moreover, the more diverse the tasks, the less accurate initialization that MAML requires. %To the best of our knowledge, 
% % check beta to make sure that rate decrease with less task diversity
% % the linear convergence rates of ANIL and MAML are $\poly(\frac{\mu_\ast}{L_{\max}})$.
% % So, the more diverse the sampled ground-truth heads are on average, the faster that ANIL and MAML converge.  
% To the best of our knowledge, these are the first results to show
% how task diversity plays a key role in representation learning from an {\em optimization} perspective. 


% \textbf{Normalized initialization.} The results require $\mathbf{w}_0\! =\! \mathbf{0}$ and $\mathbf{I}_k\!-\!{\alpha}\mathbf{B}_0^\top\mathbf{B}_0  \!=\!\mathbf{0}$. These quantities being small is critical to the $\mathbf{w}_{t,i}$'s being diverse, and thereby critical to ANIL and MAML's representation learning abilities.
% Importantly, if these quantities are initially small, they remain small for all $t$.
% % Aside from algorithmic stability, the intuition for this is that $\mathbf{w}_{t,i}\!=\!(\mathbf{I}_k \!-\! {\alpha}\mathbf{B}_t^\top\mathbf{B}_t) \mathbf{w}_t \!+\!\alpha \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$, so the smaller that $(\mathbf{I}_k \!-\! {\alpha}\mathbf{B}_t^\top\mathbf{B}_t) \mathbf{w}_t$ is, the more diverse the $\mathbf{w}_{t,i}$'s are, and the faster the representation is learned. 
% % Surprisingly, if $\mathbf{w}_0$ and $\mathbf{I}_k - \alpha \mathbf{B}_0^\top \mathbf{B}_0$ are small, then these quantities remain small for all $t$. Showing this is a key focus of the proof.
% Our analysis therefore gives a theoretical explanation for the empirical benefits of the ``zeroing trick'' of setting the MAML head to zero at the start of each round  \cite{kao2021maml} and further shows that the head only needs to be set to zero initially, then it will naturally remain near zero.


% \textbf{ANIL vs MAML.} Compared to ANIL, MAML requires more strict conditions on the initialization $\mathbf{B}_0$, and, in the case of FO-MAML, on $\eta_\ast$. We discuss why these conditions arise in Section \ref{sec:sketch} and numerically verify their necessity in Section \ref{sec:sims}.

% \textbf{FO-MAML vs Exact MAML.}
% Reason why FO-MAML has better $\kappa$ dependence for initialization than Exact MAML: Exact gradient has an extra  term that must be controlled with better initialization, otherwise head may blow up. We know that FO-MAML inner loop  representation update is not helpful for representation learning, so second-order-update accentuates the non-helpfulness

% \begin{lemma} \label{lem:task_diversity}
% Define $L_\ast \coloneqq 1 + \|\mathbf{\bar{w}}_\ast\|_2^2\left(1+  c \frac{\sqrt{k}+ \sqrt{\log(T)}}{\sqrt{n}}\right)$ and $\mu_\ast \coloneqq 1 - c \frac{\sqrt{k}+ \sqrt{\log(T)}}{\sqrt{n}}(1+ \|\mathbf{\bar{w}}_{\ast}\|_2^2)$ for some absolute constant $c$. Define the event $A \coloneqq \bigcap_{t=1}^T \left\{\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top\right) \geq \mu_\ast^2 \cap \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top\right) \leq L_\ast^2\right\}$. Then
%     $P(A) \geq 1 - 2T^{-99}$.
% \end{lemma}
% The proof follows standard sub-Gaussian concentration results and is given in Appendix \ref{app:anil}. The parameters $(L_\ast,\mu_{\ast})$ dictate the underlying diversity of the ground-truth task heads sampled on each iteration. 

% % \begin{proof}[Proof outline]
% Pick any iteration $t \in \{0,\dots,T\}$. Let $\mu_{\ast,t}^2 = \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top\right)$ and $L_{\ast,t}^2 = \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{\ast,i}^\top\right)$.
%  By standard sub-Gaussian concentration results, 
% %  (equation 4.22 in \cite{vershynin2018high}), 
%  we have that for sufficiently large $n$,  $\mu_{\ast,t}^2 \!\geq\! \mu_{\ast}^2\! \coloneqq \!1 - C\frac{k+ \gamma}{n}$ and $L_{\ast,t}^2 \!\leq \!L_{\ast}^2\! \coloneqq\! 1 + C\frac{k+ \gamma}{n}$ with probability at least $1 -2 e^{-\gamma^2}$ for some absolute constant $C$ and any $\gamma\!> \!0$. By union bounding over all $t \in \{1, \dots, T\}$, we obtain that the event  occurs with probability at least $1\!- \!2 T e^{-\gamma^2}$. Please refer to Lemma \ref{lem:task_diversity} for details. We condition on this event for the remainder of the proof.
% % \end{proof}

% \textbf{ANIL.} We first state our main theorem for ANIL.
%formal version of Theorem \ref{thm:anil_informal}.

% [THEOREM WITH LOG FACTORS]
% \begin{thm}[ANIL]\label{thm:anil_informal}
% For any $T>0$, $\alpha\leq $, $\beta \leq T\alpha^3$, initial representation satisfying $\dist(\mathbf{B}_0, \mathbf{B}_\ast)\leq c$ for some absolute constant $c$, 

% Exact ANIL:
% $m_{out}\geq  T^2(k+\log(n))/n + \sqrt{T}d/n$

% $m_{in} \geq T(k+\log(n)) + T^2 ( k^2 {d} \log(nm_{in}) + d\log^3(nm_{in}))/n$

% FO-ANIL:

% $m_{out}= \Omega((d+T(k+\log(n)))T/n),$  and $m_{in}= \Omega((k+\log(n))T(1+T/n)$,
% % $m_{in} =\tilde{\Omega}(T^2\frac{(L_{\max}^4+\sigma^2)k}{\mu_{\ast}^4})$, and
% % $n m_{out} =\tilde{\Omega}(T^2\frac{(L_{\max}^4+\sigma^2)d}{\mu_{\ast}^4})$,
% then both FO-ANIL and Exact ANIL satisfy that the $T$-th iterate of the representation obtains:
% \begin{align}
%   \dist(\mathbf{{B}}_{T}, \mathbf{{B}}_\ast ) &\leq \left(1 - \Omega(\beta \alpha \mu_{\ast}^2)\right)^{T-1} + \varepsilon
% \end{align}
% where for FO-ANIL,
% \begin{align}
%   \varepsilon&= O\bigg(\tfrac{ L_{\max}(L_{\max}+\sigma)\sqrt{d}}{\mu_\ast^2\sqrt{nm_{out}}}+ \tfrac{\sigma^2 \sqrt{dk}+\sqrt{d\log(n)}}{\mu_\ast^2 \sqrt{n m_{in} m_{out}}} \bigg)\nonumber
% %   O(L_{\max}^3\sigma +L_{\max}^2\sigma^2 +1) \delta_{in}^2\delta_{out}   \nonumber \\
%     % &\quad +  O(L_{\max}^4+L_{\max}^3\sigma +1) \tfrac{(\delta_{in}+ \delta_{out,k})\delta_{out}}{\sqrt{n}} \nonumber
% \end{align}
% and for Exact ANIL,
% \begin{align}
%   \varepsilon&\coloneqq (L_{\max}+\sigma)^2(\delta(m_{in},k)+ \delta(m_{out},k)+  \bar{\delta}(m_{out},d) + \tfrac{1+M^2}{m_{in}}) \nonumber\\
%   &\quad +  (L_{\max}+\sigma)^2(k+\log(nm_{in}))\sqrt{\log(nm_{in})}\bar{\delta}(m_{in},d)\nonumber
% %   \tfrac{L_{\max}(L_{\max}+\sigma)}{\mu_\ast^2}O\left( \tfrac{k \sqrt{d} + \log^2(nm_{in})}{\sqrt{nm_{in}}}\! +\! \tfrac{1}{m_{in}}\! +\! \tfrac{\sqrt{d}}{\sqrt{nm_{out}}} \right) \nonumber
% \end{align}
% (ignore log factors) 
% % \delta = O\left( \frac{k \sqrt{d} + \log^2(nm_{in})}{\sqrt{nm_{in}}} + \frac{1}{m_{in}} + \frac{\sqrt{d}}{\sqrt{nm_{out}}} \right)
% % where $\delta_{in}\coloneqq O(\tfrac{\sqrt{k}+\sqrt{\log(n)}}{\sqrt{m_{in}}}),  \delta_{out,k}\coloneqq O( \tfrac{\sqrt{k}}{\sqrt{nm_{out}}})$, and
% % $\delta_{out}\coloneqq O( \tfrac{\sqrt{d}}{\sqrt{nm_{out}}})$,
% with probability at least $1- \tfrac{1}{\poly(n)}- \tfrac{1}{\poly(m_{in})}$ over the random selection of 
% % tasks and 
% samples per task.
% \end{thm}



% total: fo: Tk + T2 k/n + dT/n = k + d/n
% exact: Tk + T2 k2 d/n  = k + k^2d/n

% Theorem \ref{thm:anil_informal} shows that the ANIL representation {\em linearly} converges to a neighborhood of the ground-truth column space of size $\varepsilon$ in principal angle distance with contraction factor $1 \!- \!\Omega(\beta \alpha \mu_{\ast}^2)$. 
% We have a similar result for MAML:


% \begin{thm}[MAML]\label{thm:maml_informal}
% For any $T>0$, $\alpha\leq $, $\beta \leq T\alpha^3$, initial representation satisfying $\dist(\mathbf{B}_0, \mathbf{B}_\ast)\leq c$ for some absolute constant $c$, $m_{in} =\tilde{\Omega}(T^2\frac{(L_{\max}^4+\sigma^2)k}{\mu_{\ast}^4})$,
% $n m_{out} =\tilde{\Omega}(T^2\frac{(L_{\max}^4+\sigma^2)d}{\mu_{\ast}^4})$,
% and $n \gg k + \log(T)$,
% then both FO-ANIL and Exact MAML satisfy that the $T$-th iterate of the representation obtains:
% \begin{align}
% %   \dist(\mathbf{{B}}_{T}, \mathbf{{B}}_\ast ) &\leq \left(1 - \Omega(\beta \alpha \mu_{\ast}^2)\right)^{T-1} + O(\varepsilon) 
% \end{align}
% where for FO-MAML,
% \begin{align}
% %   \varepsilon&\coloneqq \sigma L_{\max}\delta_{out} + O(L_{\max}^3\sigma +L_{\max}^2\sigma^2 +1) \delta_{in}^2\delta_{out}   \nonumber \\
% %     &\quad +  O(L_{\max}^4+L_{\max}^3\sigma +1) \tfrac{(\delta_{in}+ \delta_{out,k})\delta_{out}}{\sqrt{n}} \nonumber\\
% \end{align}
% and for Exact MAML,
% \begin{align}
%   \varepsilon&\coloneqq    \nonumber \\
%     &\quad  \nonumber
% \end{align}
% where
% $\delta_{in}\coloneqq c_{in} \tfrac{\sqrt{k}+\sqrt{\log(n)}}{\sqrt{m_{in}}},  \delta_{out,k}\coloneqq c_{out,k} \tfrac{\sqrt{k}}{\sqrt{nm_{out}}}$, and
% $\delta_{out}\coloneqq c_{out} \tfrac{\sqrt{d}}{\sqrt{nm_{out}}}$.
% for absolute constants $c_{in}, c_{out,k}, c_{out}$,
% with high probability over the random selection of tasks and samples per task.
% \end{thm}


% A few comments are in order for interpreting these results:


% \begin{enumerate}[(i)]


% that $\rho \geq 1 - c\sqrt{R}$ for some constant $c>0$. The only positive term in $\rho$ is  
% $E_0 \mu_\ast^2$, where $E_0$ is the initial signal energy (a constant) and $\mu_{\ast}$.
% % is a lower bound on the minimum singular value of the matrix of ground-truth heads of the tasks sampled on each iteration. 
% So, we cannot show convergence if $\mu_{\ast} = 0$, meaning that the tasks are not diverse. 
% If $\mu_{\ast} = \Omega(1)$ and $L_\ast$  is finite, then we can show linear convergence with sample complexities that scale with $L_{\ast}^4/\mu_{\ast}^4$. Also, note that we must choose $\beta \leq 1/L_{\ast}^2$, which results in a convergence rate that grows with $\mu_{\ast}^2/L_{\ast}^2$.
% (since the negative terms in $\rho$ scale with $L_\ast$). 
% {So as long as there is {\em some} task diversity ($\mu_{\ast} > 0$ and $L_\ast <  \infty$), ANIL learns the representation with a total number of samples that diminishes, and a convergence rate that increases, with increasing task diversity.} 
% Note that the requirement $n\gg k$ ensures that the tasks sampled on each round are highly diverse with high probability, so $L_{\ast}^4/\mu_{\ast}^4$ is a constant close to $1$.
% Meanwhile, the negative terms scale with $L_\ast$. Therefore, the more diverse that the tasks are, i.e. the larger that $\mu_{\ast}$ is and the smaller that $L_\ast$ is,  the larger the $\rho$ will be .
% $\mu$, the minimum singular value of the matrix of inner loop-updated heads, which is in turn 


    % Note that $d$ dependence is unavoidable because we must search $\mathbb{R}^d$ for the correct subspace.
% note that the neighborhood size is irreducible. for fedrep, the neighborhood size scale with distance, so we do not have this issue

% \textbf{(iv) Requirement on $n$.} The condition $n\gg k+ \log(T)$ ensures that the tasks sampled on every iteration are $(1\!-\!\Delta, 1\!+\!\Delta)$-diverse with small $\Delta$ (i.e., highly diverse). Nevertheless, experiments have shown that ANIL can succeed even with a very small task-batch size $n$ \citep{raghu2019rapid}. We conjecture that this is because high task diversity only needs to be satisfied by sets of tasks sampled across iterations, not  by each batch of tasks sampled on every iteration (although in the former case, the convergence rate would be slower).




\subsection{Finite-sample results}

Thus far we have only considered the infinite sample case, i.e.,  $m_{in}\!=\!m_{out}\!=\!\infty$, to highlight the reasons that the adaptation updates in MAML and ANIL are essential for representation learning. Next, we study the finite sample setting.
% Next, we move on to a more realistic setting that we have a finite number of samples. 
Indeed, establishing our results for the finite sample case is more challenging, but the mechanisms by which ANIL and MAML learn representations for finite $m_{in}$ and $m_{out}$ are very similar to the infinite-sample case, and the finite-sample problem reduces to showing concentration of the  updates to the infinite-sample updates.
% , rather than revealing any new insights about how ANIL and MAML learn representations. 

For MAML, this concentration requires assumptions on  sixth and eighth-order products of the data which arise due to the inner-loop updates. In light of this, for the sake of  readability we  only give the finite-sample result for ANIL and FO-ANIL, whose analyses require only standard assumptions on the data, as we state below.
 \begin{assumption}[Sub-gaussian feature distribution]
\label{assump:data}
For $\mathbf{x}\sim p$,  $\mathbb{E}[\mathbf{x}]\!=\!\mathbf{0}$ and  $\Cov(\mathbf{x})\!=\!\mathbf{I}_d$. Moreover, $\mathbf{x}$ is $\mathbf{I}_d$-sub-gaussian in the sense that $\mathbb{E}[\exp(\mathbf{v}^\top \mathbf{x})]\!\leq\! \exp(\tfrac{\|\mathbf{v}\|_2^2}{2})$ $\forall\; \mathbf{v}$.
\end{assumption}
% The hypercontractivity assumption is needed to show the concentration of higher-order products of the data in the Exact ANIL updates, and is also assumed in other works \cite{tripuraneni2020provable}.
Under this assumption, we can show the following.
\begin{thm}[ANIL Finite Samples]\label{thm:anil_fs} Consider the finite-sample case for  ANIL and FO-ANIL.
Suppose Assumptions \ref{assump:tasks_diverse_main}, \ref{assump:tasks_main} and \ref{assump:data} hold,  $\alpha = O((\sqrt{k}L_\ast+\sigma)^{-1})$ 
and $\beta$ is chosen as in Theorem \ref{thm:anil_pop_main}.
%  $\beta = O({\alpha}{\kappa_{\ast}^{-4}})$ for ANIL and $\beta = O({\alpha}{\kappa_{\ast}^{-4}\min(1,{\nicefrac{\mu_\ast^2}{\eta_\ast^{2}}}}))$ for FO-ANIL, where ${\eta}_\ast$ satisfies $\|\tfrac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\|_2 \leq \eta_\ast$ for all times $t\in [T]$ almost surely.
For some $\delta \!>\!0$ to be defined later, let $E_0\! =\! 0.9\!-\!\dist^2_0-\delta$ and 
assume $E_0$ is lower bounded by a positive constant. Suppose the sample sizes  satisfy  $m_{in} = \tilde{\Omega}(M_{in})$ and $m_{out} = \tilde{\Omega}(M_{out})$ for some expressions $M_{in},M_{out}$ to be defined later. 
% Then after $T= O(\beta \alpha\mu_\ast^2\log(\nicefrac{1}{\epsilon}))$, both FO-ANIL and Exact ANIL satisfy that the $T$-th iterate of the representation obtains:
Then %after $T\!>\!0$ iterations, 
both ANIL and FO-ANIL satisfy:
\vspace{-1mm}
\begin{align}
  \dist(\mathbf{{B}}_{T}, \mathbf{{B}}_\ast ) &\leq \left(1 - 0.5\beta \alpha \mu_{\ast}^2\right)^{T-1} + \tilde{O}(\delta) \nonumber
\end{align}
\vspace{-2mm}
where for ANIL,
\vspace{-0.2mm}
\begin{align}
   M_{in}&=  k^3+\tfrac{k^3d}{n}
    , \; M_{out}= k^2 + \tfrac{dk+k^3}{n} \nonumber,  \\
  \delta&=  (\sqrt{k}\kappa_{\ast}^2+\tfrac{\kappa_\ast\sigma}{\mu_\ast}+\tfrac{\sigma^2}{\mu_\ast^2})({k}\!+\!\tfrac{\sqrt{dk}}{\sqrt{n}})(\tfrac{1}{\sqrt{m_{in}}} \!+\!\tfrac{1}{\sqrt{m_{out}}}) \nonumber
%   \tfrac{(\sqrt{k}L_{\ast}+\sigma)^2(\sqrt{k} +\sqrt{d/n})}{\mu_\ast^2}\big(\tfrac{\sqrt{k} }{\sqrt{m_{in}}} + \tfrac{1}{\sqrt{m_{out}}}\big)\nonumber
\end{align}
\vspace{-2mm}
and for FO-ANIL,
\vspace{-0.2mm}
\begin{align}
  M_{in}&=  k^2%+k\log(n) %+\tfrac{k^3}{n} %+ \log(n)
    , \; M_{out}= \tfrac{dk+  k^3}{n} \nonumber  \\
     \delta&= (\sqrt{k}\kappa_{\ast}^2+\tfrac{\kappa_\ast\sigma}{\mu_\ast}+ \tfrac{\sigma^2}{\mu_\ast^2\sqrt{m_{in}}})\tfrac{\sqrt{dk}}{\sqrt{nm_{out}}} \nonumber
\end{align}
\vspace{-0mm}
with probability at least $1\!-\!\tfrac{T}{\poly(n)}\!-\!\tfrac{T}{\poly(m_{in})}\!-O(Te^{-90k})$.% over the random selection of tasks and
% samples per task.
\end{thm}
For ease of presentation, the $\tilde{\Omega}()$ notation excludes log factors and all parameters besides $k,d$ and $n$; please refer to Theorem \ref{thm:anil_fs_app} in Appendix \ref{app:anil_fs} for the full statement. 
% In terms of dimension parameters and number of task dependence,
We focus on dimension parameters and $n$ here to highlight the sample complexity benefits conferred by ANIL and FO-ANIL compared to solving each task separately ($n\!=\!1$).
Theorem \ref{thm:anil_fs} shows that ANIL requires only  $m_{in}+m_{out} = \tilde{\Omega}(k^3+\frac{k^3d}{n})$  samples per task to reach a neighborhood of the ground-truth solution. 
% which is roughly the cost to learn a task-specific head ($k$) plus learn the task's share of the global representation ($kd/n$). 
Since $k\ll d$ and $n$ can be large, this sample complexity is far less than the 
% this result 
% % helps to explain why ANIL achieves high performance in few-shot learning settings, in which only a small number of samples per task are allowed for inner loop  adaptation, and  
% demonstrates the benefit of global representation learning
% The outer loop sample complexity also grows with $\polylog(k,\frac{d}{n})$, which fully 
% as the sample complexity benefit of collaboration conferred by ANIL,
% as the sample complexity to learn each task individually is 
$\tilde{\Omega}(d)$ required to solve each task individually \citep{hsu2012random}. Note that more samples are required for Exact ANIL because the second-order updates involve higher-order products of the data, which have heavier tails than the analogous terms for FO-ANIL.

% In MAML case we need assumptions on higher-order moments of the data, 

% discuss initialization w = 0 etc?

% \textbf{MAML.} Now we state our main theorem for MAML.


% \begin{thm}[MAML Informal]\label{thm:maml_informal}
% For appropriate choice of step sizes and initialization with constant error, $m_{in} = \tilde{\Omega}()$, $n m_{out} = \tilde{\Omega}()$, and $n \gg k$,
% then the $T$-th iterate of the representation $\mathbf{B}_T$ for the MAML algorithm as described in Algorithm \ref{alg:algs} satisfies:
% % \begin{align}
% %   \dist(\mathbf{{B}}_{T}, \mathbf{{B}}_\ast ) &\leq \left(1 - \Omega(1)\right)^{T}\dist(\mathbf{{B}}_{0}, \mathbf{{B}}_\ast) + \tilde{O}\left(\frac{(k+\sigma\sqrt{k})\sqrt{kd}}{\sqrt{n m_{in} m_{out}}} + \frac{\sigma\sqrt{kd}}{\sqrt{n m_{out}}}\right) \nonumber
% % \end{align}
% with high probability over the random selection of tasks and samples per task.
% \end{thm}

% \begin{thm} \label{thrm:maml}
% For $\alpha=1$, $\beta \in (0,1]$ and any $0 < c < \beta E_0 \mu_\ast^2$, if for all $t = 1,\dots,T$,
% \begin{align}
%   \|\mathbf{w}_t\|_2^2 &\leq \frac{1}{F}\left( -(A + (1-c)^2 D)+ (1-c)\sqrt{1 + 2 AD + (1-c)^2D}\right),
%     % \frac{2 \beta L_{\ast}^2(2 - 2 \beta E_0 \mu_\ast^2+\beta L_{\ast}^2 ) + \beta L_\ast^2 \sqrt{ (Z + 2)^2 - 4 \beta^2 E_0 L_\ast^2 Z}}{4\beta E_0 \mu_\ast^2 - 2 \beta^2 E_0^2 \mu_{\ast}^4 }
% \end{align}
% where $A\coloneqq 1 - \beta E_0 \mu_\ast^2$, $D\coloneqq 1 -  \beta E_0 \mu_\ast^2  +  \beta L_\ast^2  $, $F \coloneqq \beta L_\ast^2$, and the representation $\mathbf{B}_t$ is orthogonalized at the end of each outer loop, then MAML learns the representation at a linear rate 

% with contraction factor at most $1-c$, i.e.
% \begin{align}
%     \dist(\mathbf{\hat{B}}_T, \mathbf{\hat{B}}_\ast) &\leq (1 - c)^{T}\dist(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast).
% \end{align}
% \end{thm}
% The proof of Theorem \ref{thrm:maml} can be found in Appendix \ref{app:maml}.






==> Problem_Formulation.tex <==
\section{Problem Formulation}

% \textbf{Shared information across tasks.} The principal goal of meta-learning is to recover shared information among a set of tasks in order to more efficiently learn new tasks. Often, this shared information is a common, and often small, set of useful features of the data. For instance, the label of a street sign is closely related to the shape and color of the sign, so models that identify these features may perform very well across all tasks involving classifying street signs.

% At each time $t,$ we sample a collection of $n$ tasks. For each of these tasks, we collect $m_{in} + m_{out}$ data samples; specifically, for task $i$ at time $t,$ we collect the samples $\mathcal{D}_{t,i}^{in} = \{(x_{t,i,l}), y_{t, i, l})\}_{l=1,\ldots, m_{in}}$ and $\mathcal{D}_{t,i}^{out} = \{(x_{t,i,l}), y_{t, i, l})\}_{l\in [m_{out}]}.$ These samples are drawn i.i.d. from 

We employ the multi-task linear representation learning framework \citep{maurer2016benefit,  du2020fewshot, tripuraneni2020provable} studied in prior works. 
Each task in this setting is a linear regression problem in $\mathbb{R}^d$. We index tasks by $(t,i)$, corresponding to the $i$-th task sampled on iteration $t$. {
The inputs $\mathbf{x}_{t,i}\in \mathbb{R}^d$ and labels $y_{t,i}\in \mathbb{R}$ for the $(t,i)$-th task are sampled i.i.d. from a distribution $P_{t,i}$ over $\mathbb{R}^d\times\mathbb{R}$ such that:
\begin{equation}
    \mathbf{x}_{t,i} \sim p, \quad z_{t,i} \sim \mathcal{N}(0,\sigma^2), \quad y_{t,i} = \langle \boldsymbol{\theta}_{\ast,t,i}, \mathbf{x}_{t,i}\rangle + z_{t,i} \nonumber
\end{equation}
where  $\boldsymbol{\theta}_{\ast,t,i} \in \mathbb{R}^d$ is the ground-truth regressor for task $(t,i)$, $p$  is a distribution over $\mathbb{R}^d$ and $z_{t,i}$ is white Gaussian noise with variance $\sigma^2$. Each task has a set of $m$ samples $\mathcal{D}_{t,i}\coloneqq \{(\mathbf{x}_{t,i,j},y_{t,i,j})\}_{j\in [m]}$ drawn i.i.d. from $P_{t,i}$ available for training.

% where $z_i$ is additive noise with mean zero and variance $\sigma^2$. 
% there exists a universal linear mapping from $\mathbb{R}^d \rightarrow \mathbb{R}^k$, where $k\ll d$, which extracts features from data that are sufficient to predict its label. 
% That is, 
To account for shared information across tasks, we suppose there exists a matrix $\mathbf{B}_\ast \in \mathcal{O}^{d \times k}$ 
% which, for each task $i$,  maps any data point $\mathbf{x}_i$ to a shared $k \ll d$-dimensional subspace $\col{(\mathbf{B}_\ast)}$ which preserves all of the information in the data relevant to its label.
% there exists a $\mathbf{w}_{\ast,i}\in \mathbb{R}^k$ which optimally predicts their label, 
% i.e. $\mathbb{E}[y_i|\mathbf{x}_i]= \mathbf{w}_{\ast,i}^\top \mathbf{B}_{\ast}^\top \mathbf{x}_i$.
% More specifically, 
such that the ground-truth regressors $\{\boldsymbol{\theta}_{\ast,t,i}\}_i$ for all tasks lie in $\col(\mathbf{B}_\ast)$, so they can be written as $\boldsymbol{\theta}_{\ast,t,i} = \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$ for all $t,i$, where $\mathbf{w}_{\ast,t,i} \in \mathbb{R}^k$. We refer to $\mathbf{B}_\ast$ as the ground-truth representation and $\mathbf{w}_{\ast,t,i}$ as the ground-truth head for task $(t,i)$. 
The task environment consists of $\mathbf{B}_\ast$ and a distribution $\nu$ over ground-truth heads.
% Let $\mathbf{B}_\ast \in \mathcal{O}^{d \times k}$ be an orthogonal matrix whose columns span this $k$-dimensional subspace. Then   
% For any input $\mathbf{x}_i$, its projection onto $\text{col}(\mathbf{B}_\ast)$, specifically $\mathbf{B}_\ast^\top \mathbf{x}_i$, yields the values of its $k$ shared features, and thereby reduces the prediction problem from $d$ dimensions to $k \ll d$ dimensions.  Then, for every $i$, there exists a unique vector $\mathbf{w}_{\ast,i} \in \mathbb{R}^k$ such that $ \mathbf{B}_\ast \mathbf{w}_{\ast,i} = \boldsymbol{\theta}_{\ast,i}$ recovers the ground-truth regressor for the $i$-th task.
% We call $\mathbf{B}_\ast$ and  $\mathbf{w}_{\ast,i}$ the ground-truth representation and  head for task $i$, respectively.  
% Without loss of generality we assume that $\mathbf{B}_\ast$ has orthonormal columns. 
% \textbf{Learning model.} 
% As a result, 
% the goal of meta-learning this setting is to recover $\col{(\mathbf{B}_\ast)}$ from labeled samples across many tasks. 
% In this section we formalize the question of whether ANIL and MAML learn a representation in the  linear multi-task representation learning setting. 
% We make the following standard assumption on the distribution of the ground-truth heads, which determines the distribution of tasks.
% This generative model with a shared representation and task-specific heads is a simplified version motivated by real-world problems such as few-shot image classification in which there may exist a shared set of relevant features across images from different tasks, but a each task has a unique head based on the unique labeling of the data for that task.
% We ask the simple question of whether ANIL and MAML recover $\text{col}(\mathbf{B}_\ast)$ in this setting.
% problem now becomes to recover $\text{col}(\mathbf{B}_\ast)$. 
% In this setting, both ANIL and MAML aim to learn a single
With knowledge of $\col{(\mathbf{B}_\ast)}$, we can reduce the number of samples needed to solve a task from $\Omega(d)$ to $\Omega(k)$ by projecting the task data onto $\col{(\mathbf{B}_\ast)}$, then learning a head in $\mathbb{R}^k$. The question becomes how to learn the ground-truth subspace $\col{(\mathbf{B}_\ast)}$.}

% At each time $t$, the algorithms are allowed to draw a set of $n$ tasks with ground-truth heads $\{ \mathbf{w}_{\ast,t,i}\}_{i=1}^n$ from a possibly infinite collection $\mathcal{W}_\ast$.
The learning model consists of a  representation $\mathbf{B} \!\in\! \mathbb{R}^{d\times k}$ and a head $\mathbf{w}\!\in\! \mathbb{R}^{k}$.
% The unde goal of meta-learning in this setting is to learn  from labeled samples across many tasks a representation $\mathbf{B}$ whose column space recovers $\col{(\mathbf{B}_\ast)}$.
% Ultimately, we aim to determine whether  ANIL and/or MAML learn the column space of the  ground-truth representation $\mathbf{B}_\ast$. 
We would like the column space of $\mathbf{B}$ to be close to that of $\mathbf{B}_\ast$, measured as follows. 
% , we measure the closeness of a representation $\mathbf{B}$ to the ground-truth $\mathbf{B}_\ast$  
\begin{definition}[Principle angle distance]
 Let $\mathbf{\hat{B}}\in \mathcal{O}^{d\times k}$ and $ \mathbf{\hat{B}}_{\ast,\perp}\in \mathcal{O}^{d\times (d-k)}$ denote orthonormal matrices whose columns span $\col(\mathbf{B})$ and $ \col^\perp(\mathbf{B}_\ast)$, respectively. Then the principle angle distance between $\mathbf{B}$ and  $
\mathbf{B}_\ast$ is
\begin{align}
    \dist(\mathbf{B}, \mathbf{B}_\ast) &\coloneqq \|\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{\hat{B}}\|_2.
\end{align}
For shorthand, we denote $\dist_t \coloneqq \dist(\mathbf{B}_t, \mathbf{B}_\ast)$.
\end{definition}
Notice that $\dim(\col(\mathbf{B}_\ast)) = k$. Thus, the learned representation $\mathbf{B}$ must extract $k$ orthogonal directions belonging to $\col(\mathbf{B}_\ast)$. As we will show, MAML and ANIL's task-specific adaptation of the head critically leverages task diversity to learn $k$ such directions.

% To do so, they aim to minimize the average linear regression task losses after one step of task-specific adaptation. We consider the following population loss function for the $i$-th task (without any adaptation):

% for some regularization parameter $\lambda > 0$, where the regularization $\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2$...

% while the average population loss across all tasks for the model $(\mathbf{B}, \mathbf{w})$ is
% \begin{align}
%     \mathcal{L}(\mathbf{B}, \mathbf{w})\!
%     &\coloneqq \mathbb{E}_{\mathbf{w}_{\ast,i}}\left[\mathcal{L}_i ( \mathbf{B}, \mathbf{w} )\right] \label{minthis} %\!=\! \tfrac{1}{2}\mathbb{E}_{\mathbf{w}_{\ast,i}}\left[\mathbb{E}_{\mathbf{x}_i,y_i} \left[(\langle \mathbf{B} \mathbf{w}, \mathbf{x}_i\rangle\!-\! y_i)^2 \right]\right]%\!+\!\frac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top\!-\! \mathbf{I}_k\|_F^2 . \label{glob_obj}
% \end{align}

% \begin{rem}[Naive approach]\label{rem:1} Assuming access to infinitely many samples, a naive approach to recovering $\col(\mathbf{B}_\ast)$ would be to minimize the  average population loss across tasks, i.e., to solve
% \begin{align}
%     \min_{\mathbf{B},\mathbf{w}}\big\{\mathcal{L}(\mathbf{B}, \mathbf{w})\!
%     &\coloneqq \mathbb{E}_{\mathbf{w}_{\ast,i}}\left[\mathcal{L}_i ( \mathbf{B}, \mathbf{w} )\right]\big\} \label{minthis}
% \end{align}
% However,  minimizing $\mathcal{L}(\mathbf{B}, \mathbf{w})$ \textbf{does not} recover $\col(\mathbf{B}_\ast)$. This is because  $(\mathbf{\tilde{B}}, \mathbf{\tilde{w}})$ is a global minimum of $\mathcal{L}(\mathbf{B}, \mathbf{w})$ if and only if $\mathbf{\tilde{B}} \mathbf{\tilde{w}}\!= \!\mathbf{{B}}_\ast \mathbb{E}[\mathbf{w}_{\ast,i}]$. Thus, $\col(\mathbf{\tilde{B}})$ need only agree with $\col(\mathbf{{B}}_\ast)$ in one direction (the direction given by $\mathbf{{B}}_\ast \mathbb{E}[\mathbf{w}_{\ast,i}]$), and the other potentially $k\!-\!1$ orthogonal directions in $\col(\mathbf{\tilde{B}})$ can be arbitrarily chosen. 
% % The same argument holds for trying to minimizing the finite task, finite sample surrogate of $f(\mathbf{B}, \mathbf{w})$. 
% % {\em Thus, recovering the optimal representation in this setting is a non-trivial problem.}
% \end{rem}


\section{Algorithms}
{{
{Here we formally state the implementation of ANIL and MAML for the problem described above. 
First, letting $\boldsymbol{\theta} \coloneqq [\mathbf{w}; \vec(\mathbf{B})]\in \mathbb{R}^{(d+1)k}$ denote the vector of model parameters, 
we define the population loss for task $(t,i)$:
\begin{align*}
    \mathcal{L}_{t,i}(\boldsymbol{\theta}) \coloneqq \tfrac{1}{2}\mathbb{E}_{(\mathbf{x}_{t,i},y_{t,i})\sim P_{t,i}} \left[(\langle \mathbf{B} \mathbf{w}, \mathbf{x}_{t,i}\rangle - y_{t,i})^2 \right]. %+ 
\end{align*}
Often we approximate this loss with the finite-sample loss  for a dataset $\mathcal{D}_{t,i}'\coloneqq \{ (\mathbf{x}_{t,i,j},y_{t,i,j})\}_{j\in [m']}$:
\begin{align}
 \hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta};\mathcal{D}_{t,i}')  &\coloneqq   \tfrac{1}{2m'}\sum_{j=1}^{m'}  (\langle \mathbf{Bw}, \mathbf{x}_{t,i,j}\rangle\! -\! y_{t,i,j})^2. \nonumber
%  + \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
 \label{fs_loss}
 \end{align}
%  At iteration $t$, 
% For task $(t,i)$, both ANIL and MAML partition the $m$
 
% %  it samples $n$ tasks and two i.i.d. datasets $\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out}$ for each task consisting of $m_{in}$ labeled inner loop samples and $m_{out}$ labeled outer loop samples, respectively.
 
%  1. at each t maml and anil sample n tasks w*ti (should assump on heads be moved up?)
 
%  2. they partition the Dti into inner and outer
 
%  3. we write the losses as follows
 
% no, keep it as previous. say maml and anil partiion samples later
 
% To learn the ground-truth representation, one may naively try to minimize the average loss across tasks:
% But first, we describe a naive algorithm which highlights the benefit of ANIL and MAML's adaptation steps.

% to highlight the role inner loop updates we also describe a simple algorithm that one might use to learn the representation, which contains no inner loop updates.


% \noindent\textbf{No Adaptation.}
% A naive approach one may take to learning $\col(\mathbf{B}_\ast)$ is to minimize the average loss over tasks, without considering adaptation.
% % Considering the above model on the ground-truth regressors $\boldsymbol{\theta}_{\ast,t,i} = \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$, 
% In particular, if we define the population loss corresponding to task $(t,i)$ as
% \begin{align}
%     \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w}) \coloneqq \tfrac{1}{2}\mathbb{E}_{\mathbf{x}_{t,i},y_{t,i}} \left[(\langle \mathbf{B} \mathbf{w}, \mathbf{x}_{t,i}\rangle - y_{t,i})^2 \right], %+ \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
% \end{align}
% then we may try to solve $\min_{\mathbf{B},\mathbf{w}} \mathbb{E}_{\mathbf{w}_{\ast,t,i}} [\mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w})]$ with minibatch SGD.
% % , by sampling a batch of tasks, taking an SGD step fro each task, and average this results.
% % A natural method for learning the ground truth representation is running a 
% % stochastic gradient update with respect to problem parameters $(\mathbf{B},\mathbf{w})$ for each task and then averaging them to obtain new models. 
%  Letting $(\mathbf{B}_t,\mathbf{w}_t)$ denote the model parameters at step $t$, we sample a batch of $n$ tasks and run the following SGD update for each task
% $$
% (\mathbf{B}_{t,i},\mathbf{w}_{t,i})=
% (\mathbf{B}_{t},\mathbf{w}_{t}) -\alpha 
% \nabla_{\mathbf{B},\mathbf{w}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}),
% $$
% where for a task $(t,i)$ and dataset $\mathcal{D}_{t,i} \coloneqq \{ \mathbf{x}_{t,i,j}, y_{t,i,j}\}_{j}$, the finite-sample loss is defined as
% \begin{align}
%  \hat{\mathcal{L}}_{t,i}(\mathbf{B},\mathbf{w};\mathcal{D}_{t,i})  &\coloneqq   \tfrac{1}{2|\mathcal{D}_{t,i}|}\sum_{j}  (\langle \mathbf{Bw}, \mathbf{x}_{t,i,j}\rangle\! -\! y_{t,i,j})^2. \nonumber
% %  + \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
%  \label{fs_loss}
%  \end{align}
% The new model parameters are the average of the task-specific updates, consistent with SGD on the non-adaptive objective. One can easily show that for $|\mathcal{D}_{t,i}| = \infty$, the new representation in this case is
% \begin{align}
%     \mathbf{B}_{t+1}\! &=\! 
%     \underbrace{\mathbf{{B}}_{t} \Big(  \mathbf{I}_k\! - \!{\beta}\mathbf{w}_{t} \mathbf{w}_{t}^\top\Big)}_{\text{prior term}}\! +\!  \underbrace{\mathbf{{B}}_\ast\Big(\tfrac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{\ast,t,i} \mathbf{w}_{t}^\top\Big)}_{\text{signal term}} \label{noadapt}
% \end{align}
% Observe that the coefficient of $\b$ in the update is rank $k-1$, while the coefficient of $\mathbf{B}_\ast$ is rank 1. Thus, $\col(\mathbf{B}_{t+1})$ can move closer to $\col(\mathbf{B}_{\ast})$ in at most one direction on any iteration. 

% concern: it can still learn the rep if wt changes enough


% can be defined as the average of them, i.e.,
% $$
% \mathbf{B}_{t+1}=\frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i}, \qquad \mathbf{w}_{t+1}=\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}.
% $$
% The above procedure can also be  interpreted as running stochastic gradient with respect to the global loss over all tasks at time~$t$. 



\noindent\textbf{MAML.} 
% Instead of minimizing the average loss over tasks, 
MAML  minimizes the average loss across tasks {\em after} a small number of task-specific gradient updates. Here, we consider that the task-specific updates are one step of minibatch SGD with batch $\mathcal{D}_{t,i}^{in}$ consisting of $m_{in}$ i.i.d. samples from $P_{t,i}$.  
Specifically, the loss function that MAML minimizes is
\begin{equation}
  \min_{\boldsymbol{\theta}} \mathcal{L}_{\text{\tiny{\textit{MAML}}}}(\boldsymbol{\theta}) \coloneqq
   \mathbb{E}_{\mathbf{w}_{\ast,t,i}, \mathcal{D}_{t,i}^{in}}[
  \mathcal{L}_{t,i}( \boldsymbol{\theta}\!-\! \alpha\nabla_{\boldsymbol{\theta}} \hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta};   \mathcal{D}_{t,i}^{in}))
  )
   ] \label{maml_obj_main}
\end{equation}
where for ease of notation we have written $\mathbb{E}_{\mathbf{w}_{\ast,t,i}, \mathcal{D}_{t,i}^{in}}$ as shorthand for $\mathbb{E}_{\mathbf{w}_{\ast,t,i} \sim \nu, \; \mathcal{D}_{t,i}^{in}\sim P_{t,i}^{m_{in}}}$.
MAML essentially solves \eqref{maml_obj_main} with minibatch SGD. At iteration $t$, it draws $n$ tasks with ground-truth heads $\{\mathbf{w}_{\ast,t,i}\}_{i\in [n]}$ drawn from $\nu$, and for each drawn task, draws $m$ samples contained in $\mathcal{D}_{t,i}$ i.i.d. from $P_{t,i}$. MAML then 
partitions $\mathcal{D}_{t,i}$ into  $\mathcal{D}_{t,i}^{in}$ and $\mathcal{D}_{t,i}^{out}$ such that $|\mathcal{D}_{t,i}^{in}| =m_{in}$, $|\mathcal{D}_{t,i}^{out}|=m_{out}$, and $m_{in}+m_{out}=m$ (we assume $m_{in}< m$).} For task $(t,i)$, in what is known as the inner loop, MAML takes a task-specific stochastic gradient step from the initial model $(\mathbf{B}_t, \mathbf{w}_t)$ using the samples $\mathcal{D}_{t,i}^{in}$ and step size $\alpha$ to obtain the adapted parameters $\boldsymbol{\theta}_{t,i}$:
\begin{align*}
% \boldsymbol{\theta}_{t+1}& \gets \begin{bmatrix} \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})  \\
% \mathbf{B}_{t,i} \gets \mathbf{B}_{t} - \alpha \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}) \\
% \end{bmatrix}
\boldsymbol{\theta}_{t,i}\!&=\! \begin{bmatrix} \mathbf{w}_{t,i} \\
\vec(\mathbf{B}_{t,i}) \\
\end{bmatrix} \!\gets\!\! 
\begin{bmatrix}
\mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})  \\ \!
\vec(\mathbf{B}_{t})\! -\! \alpha \nabla_{\vec(\mathbf{B})} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t},
\!\mathbf{w}_{t};\! \mathcal{D}_{t,i}^{in}) \! \\
\end{bmatrix}
\end{align*}
Then, in the so-called outer loop, MAML takes a minibatch SGD step with respect to the loss after task-specific adaptation using  the samples $\{\mathcal{D}_{t,i}^{out}\}_{i\in[n]}$ and step size $\beta$:
\begin{align}
    \boldsymbol{\theta}_{t+1}&\!\gets\! \boldsymbol{\theta}_t\!-\!\tfrac{\beta}{n}\!\sum_{i=1}^n (\mathbf{I}\!-\!\alpha \nabla^2_{\boldsymbol{\theta}}\hat{\mathcal{L}}_{t,i} (\boldsymbol{\theta}_t; \!\mathcal{D}_{t,i}^{out})) \nabla\!\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_{t,i}; \!\mathcal{D}_{t,i}^{out}) \nonumber
% &\quad \quad \quad \quad \nabla\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_t-\alpha  \nabla\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_t; \mathcal{D}_{t,i}^{in}); \mathcal{D}_{t,i}^{out})\big)
\end{align}
Note that the above Exact MAML update requires expensive second-order derivative computations. In practice, FO-MAML, which drops the Hessian,  is often used, {since it typically achieves similar performance \cite{finn2017model}}.
% , which is known as
%  FO-MAML. We refer to the version of MAML that includes the Hessian as Exact MAML.
% That is, MAML samples a batch of $n$ tasks on each round. For every sampled task, the model parameters take the task-specific gradient step in what is known as the ``inner loop'', namely:
% \begin{align}
%     \boldsymbol{\theta}_{t+1} &= \begin{bmatrix} \mathbf{B}_{t} - \alpha 
%     \end{bmatrix}
% \end{align}


\textbf{ANIL.} 
Surprisingly, \citet{raghu2019rapid} noticed that training neural nets with a modified version of MAML that lacks inner loop updates for the representation resulted in models that matched and sometimes even exceeded the performance of models trained by MAML on few-shot image classification tasks. 
This modified version is ANIL, and its  inner loop updates in our linear case are given as follows:
\begin{align*}
\boldsymbol{\theta}_{t,i}&%=\hat{Q}_{t,i}(\boldsymbol{\theta}_{t}) 
=
\begin{bmatrix} \mathbf{w}_{t,i} \\
\vec(\mathbf{B}_{t,i}) \\
\end{bmatrix}  =
\begin{bmatrix}
\mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}) \\
\vec(\mathbf{B}_{t})  \\
\end{bmatrix}.
\end{align*}
In the outer loop, ANIL again takes a minibatch SGD step with respect to the loss after the inner loop update. 
 Then, the outer loop updates for  Exact ANIL are given by:
\begin{align*}
\boldsymbol{\theta}_{t+1}\gets \boldsymbol{\theta}_{t} - \frac{\beta}{n}\sum_{i=1}^n 
\hat{\mathbf{H}}_{t,i}(\boldsymbol{\theta}_{t}; \mathcal{D}_{t,i}^{out})
\nabla_{\boldsymbol{\theta}}\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_{t,i},  \mathcal{D}_{t,i}^{out})
\end{align*}
where, for Exact ANIL,
\begin{align*}
\hat{\mathbf{{H}}}_{t,i}&(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out})
\coloneqq \begin{bmatrix}
\mathbf{I}_k - \alpha \nabla_{\mathbf{w}}^2 \hat{\mathcal{L}}_{t,i}( \boldsymbol{\theta}_{t}; \mathcal{D}_{t,i}^{out}) &  \mathbf{0} \\
  -\alpha \tfrac{\partial^2}{\partial \vec({\mathbf{B}}) \partial{\mathbf{w}}} \hat{\mathcal{L}}_{t,i}( \boldsymbol{\theta}_{t}; \mathcal{D}_{t,i}^{out})   &  \mathbf{I}  
\end{bmatrix}
\end{align*} 
% {\color{red} this update is incorrect - dimensions off - need tensor notation}
To avoid computing second order derivatives, we can instead treat $\hat{\mathbf{{H}}}_{t,i}$ as the identity operator, in which case we call the algorithm FO-ANIL. 

% In some settings we may not be able to afford second-order updates, in which case we treat $\hat{\mathbf{{H}}}_{t,i}$ as the identity operation.

% \textbf{Advantage of MAML and ANIL.}

\subsection{Role of Adaptation} \label{sec:intuition}
% The key to MAML and ANIL is that their  outer loop gradients for the representation are evaluated at the tas
% As of yet, it is not clear why the MAML and ANIL updates should yield a representation close to the ground truth. 
Now we present new intuition for MAML and ANIL's representation learning ability which motivates our proof structure.
% The key observation is that the fact that the outer loop gradients for the representation are {\em evaluated at the inner loop-adapted parameters} harnesses the power of task diversity  to improve the representation in all $k$ directions. 
The key observation is that the outer loop gradients for the representation are {\em evaluated at the inner loop-adapted parameters}; this harnesses the power of task diversity  to improve the representation in {\em all} $k$ directions. 
This is easiest to observe in the FO-ANIL case with $m_{in}=m_{out}=\infty$. In this case, the update for the representation is given as:
\begin{align}
    \mathbf{B}_{t+1}\! &=\! 
   \mathbf{{B}}_{t}  \Big(\underbrace{  \mathbf{I}_k\! - \!\tfrac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top}_{\text{FO-ANIL prior weight}}\Big)\! +\! \mathbf{{B}}_\ast\underbrace{\tfrac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top}_{\text{FO-ANIL signal weight}} \label{intuition}
\end{align}
If the `prior weight' is small and the `signal weight' is large, then the update replaces energy from $\col(\mathbf{B}_t)$ with energy from $\col({\mathbf{B}_\ast})$.
% (i.e.,the norm of the projection of $\mathbf{B}_{t+1}$ onto $\col(\mathbf{B}_t)$ is less than $\|\mathbf{B}_{t+1}\|$ and the spectral norm of the projection of $\mathbf{B}_{t+1}$ onto $\col(\mathbf{B}_\ast)$ is greater than that of the projection of $\mathbf{B}_{t}$ onto $\col(\mathbf{B}_\ast)$). 
Roughly, this is true as long as  $\boldsymbol{\Psi}_t\coloneqq \tfrac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$ is well-conditioned, i.e. 
% which is determined by task diversity: assuming 
the $\mathbf{w}_{t,i}$'s are diverse. Assuming
$\mathbf{w}_{t,i}\!\approx\! \mathbf{w}_{\ast,t,i}$ for each task,  
then $\boldsymbol{\Psi}_t$ 
is well-conditioned if and only if the tasks are diverse.
% Note that if the ground-truth heads $\{\mathbf{w}_{\ast,t,i}\}_i$ are diverse, meaning they span $\mathbb{R}^k$, then the $\{\mathbf{w}_{t,i}\}_i$ are also diverse as long as  Assume for now that this is the case.
% Assume for now that the set of inner-loop updated heads $\{\mathbf{w}_{t,i}\}_i$ span $\mathbb{R}^k$. 
% We can now see that the update removes energy from $k$ orthogonal directions in $\col(\mathbf{B}_t)$, and replaces it with energy from $k$ orthogonal directions in $\col(\mathbf{B}_\ast)$. 
This shows how task diversity 
% $\mathbf{w}_{t,i}\!\approx\! \mathbf{w}_{\ast,t,i}$ 
% implies that 
% $\boldsymbol{\Psi}_t$ is well-conditioned 
causes the column space of the representation learned by FO-ANIL to approach the ground-truth. For FO-MAML, we observe similar behavior, with a caveat. The representation update is:
\begin{align}
    \mathbf{B}_{t+1}\! &\stackrel{(a)}{=}\! 
    {\mathbf{{B}}_{t}\! - \!\tfrac{\beta}{n} \sum_{i=1}^n \mathbf{{B}}_{t,i}\mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top} +  {\mathbf{{B}}_\ast\tfrac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top} \nonumber \\
    %  \mathbf{B}_{t+1}\! 
    \vspace{-1mm}
     &\stackrel{(b)}{=}\! 
    {\mathbf{{B}}_{t}\Big(\underbrace{\mathbf{I}_k\! -\!(\mathbf{I}_k\! -\!\alpha \mathbf{w}_t\mathbf{w}_t^\top) \tfrac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top}_{\text{FO-MAML prior weight}}\Big)}\!\nonumber \\
        \vspace{-2mm}
    &\quad +\!  {\mathbf{{B}}_\ast\Big(\underbrace{\tfrac{\beta}{n} \sum_{i=1}^n  (1 - \alpha\langle \mathbf{w}_{t,i},\mathbf{w}_t\rangle) \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top}_{\text{FO-MAML signal weight}}\Big)} \nonumber
\end{align}
Equation $(a)$ is similar to \eqref{intuition} except that one $\mathbf{B}_t$ is replaced by the $\mathbf{B}_{t,i}$'s resulting from inner loop adaptation. Expanding $\mathbf{B}_{t,i}$ in $(b)$, we notice that the prior weight is at least as large as in \eqref{intuition}, since $\lambda_{\max}(\mathbf{I}_k\! -\!\alpha \mathbf{w}_t\mathbf{w}_t^\top)\leq 1$, but it can still be small as long as the $\mathbf{w}_{t,i}$'s are diverse and $\|\mathbf{w}_t\|_2$ is small. Thus we conclude that FO-MAML also can learn the representation, yet its inner loop adaptation complicates its ability to do so.
% Since $\mathbf{B}_{t,i}\!\neq\! \mathbf{B}_t$, FO-MAML does not quite  replace  bad energy in all directions of $\col(\mathbf{B}_t)$ with good energy from $\col(\mathbf{B}_{\ast})$ (and neither does Exact MAML), which suggests why MAML requires a stronger initialization than ANIL. However, since the perturbation $\mathbf{B}_{t,i}\! - \!\mathbf{B}_t$ is small and the $\mathbf{w}_{t,i}$'s are diverse, we will see that MAML can still learn the ground-truth representation.

{\textbf{Comparison with no inner-loop adaptation.}} Compare these updates to the case when there is {no inner loop adaptation}, i.e. we run SGD on the non-adaptive objective $\min_{\boldsymbol{\theta}} \mathbb{E}_{\mathbf{w}_{\ast,t,i}} [\mathcal{L}_{t,i}(\boldsymbol{\theta})]$ instead of \eqref{maml_obj_main}. In this case, $\mathbf{B}_{t+1}$ is:
\begin{align}
    \mathbf{B}_{t+1}\! &=\! 
    {\mathbf{{B}}_{t} \big(  \mathbf{I}_k\! - \!{\beta}\mathbf{w}_{t} \mathbf{w}_{t}^\top\big)}\! +\!  \beta{\mathbf{{B}}_\ast{} \mathbf{\bar{w}}_{\ast,t} \mathbf{w}_{t}^\top} \label{noadapt}
\end{align}
where $\mathbf{\bar{w}}_{\ast,t} \coloneqq \frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}$.
Observe that the coefficient of $\b$ in the update is rank $k\!-\!1$, while the coefficient of $\mathbf{B}_\ast$ is rank 1. Thus, $\col(\mathbf{B}_{t+1})$ can approach $\col(\mathbf{B}_{\ast})$ in at most one direction on any iteration. Empirically, $\mathbf{w}_t$ points in roughly the same direction throughout training, preventing this approach from learning  $\col(\mathbf{B}_\ast)$ (e.g. see Figure \ref{fig:intro}).
%all directions of
% Despite these intuitions, 
%%% To formalize our intuition, we will overcome a number of technical  challenges in later Sections in order to prove that ANIL and MAML learn $\col(\mathbf{B}_\ast)$ even with infinite samples per task. First, we need to quantify the diversity of the $\mathbf{w}_{t,i}$'s and how much this improves the representation in each iteration. We need to show that $\col(\mathbf{B}_t)$ retains equal energy in $k$ directions (i.e. $\mathbf{B}_t$ stays well-conditioned) and that the head does not blow up, otherwise the algorithms will not converge. We also need to deal with additional terms from the Exact updates, and control the impact of MAML's inner loop perturbation of the representation.


% Lastly, the Exact updates 
% For example, we need to show that the $\mathbf{w}_{t,i}$'s are sufficiently diverse, that the representation stays well-conditioned throughout algorithm execution, that the 
% Moreover, for MAML, we need to show that the perturbation terms 
% Still, we will utilize the above intuition task diver.
%
%
%
%

\textbf{Technical challenges.} 
The intuition on the role of adaptation, while appealing, makes strong assumptions; most notably that the $\mathbf{w}_{t,i}$'s are diverse enough to improve the representation and that the algorithm dynamics are stable. 
% {\color{blue} 
To show these points, we observe that $\mathbf{w}_{t,i}$ can be written as the linear combination of a vector distinct for each task and a vector that is shared across all tasks at time $t$. Showing that the shared vector is small implies the $\mathbf{w}_{t,i}$'s are diverse, and we can control the magnitude of the shared vector by controlling $\|\mathbf{w}_t\|_2$ and $\|\mathbf{I}_k\! -\! \alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2$. 
Showing that these  quantities are small at all times also ensures the stability of the algorithms.
% since these quantities detract from the diversity of the $\mathbf{w}_{t,i}$'s (see equation \eqref{updw}), and ensure stability when small. 
Meanwhile, we must prove that $\|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_t\|_2$ and $\dist_t=\|\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{\hat{B}}_t\|_2 $ are contracting. 
% }
% {\color{red}In order to prove that ANIL and MAML indeed learn $\col(\mathbf{B}_\ast)$, we must show that the following conditions hold for all $t$: (i) $\|\mathbf{w}_t\|_2$ is small, (ii) $\|\mathbf{I}_k\! -\! \alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2$ is small, (iii) $\|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_t\|_2$ is contracting, and finally, (iv) $\dist_t $ is contracting. Each of these conditions are related to the diversity of the $\mathbf{w}_{t,i}$'s, the stability of the algorithm, and/or showing that $\col(\mathbf{B}_t)$ approaches $\col(\mathbf{B}_\ast)$.} 
It is not obvious that any of these conditions hold individually; in fact, they require a novel 
multi-way inductive argument to show that they  hold simultaneously for each $t$ (see Section \ref{sec:sketch}).





%% To formalize our intuition, we will overcome a number of technical  challenges in later Sections in order to prove that ANIL and MAML learn $\col(\mathbf{B}_\ast)$ even with infinite samples per task. First, we quantify the diversity of the $\mathbf{w}_{t,i}$'s and how much this improves the representation in each iteration. We show that $\col(\mathbf{B}_t)$ retains equal energy in $k$ directions (i.e. $\mathbf{B}_t$ stays well-conditioned) and that the head does not blow up, otherwise the algorithms will not converge. We also deal with additional terms from the Exact updates, and control the impact of MAML's inner loop perturbation of the representation.





% {\color{green}
% ----

% Next, we formally state the implementation of ANIL and MAML for the above described problem. But to highlight the role inner loop updates we also describe a simple algorithm that one might use to learn the representation, which contains no inner loop updates. 

% \noindent\textbf{No Adaptation.}
% Considering the above model on the ground-truth regressors $\boldsymbol{\theta}_{\ast,t,i} = \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$, the population loss corresponding to task $(t,i)$ can be written as
% \begin{align}
%     \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w}) \coloneqq \tfrac{1}{2}\mathbb{E}_{\mathbf{x}_{t,i},y_{t,i}} \left[(\langle \mathbf{B} \mathbf{w}, \mathbf{x}_{t,i}\rangle - y_{t,i})^2 \right]. %+ \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
% \end{align}
% A natural method for learning the ground truth representation is running a stochastic gradient update with respect to problem parameters $(\mathbf{B},\mathbf{w})$ for each task and then averaging them to obtain new models. More precisely, if $(\mathbf{B}_t,\mathbf{w}_t)$ are the model parameters at step $t$, we run the following SGD update for each task
% $$
% (\mathbf{B}_{t,i},\mathbf{w}_{t,i})=
% (\mathbf{B}_{t},\mathbf{w}_{t}) -\alpha 
% \nabla_{\mathbf{B},\mathbf{w}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}),
% $$
% where for a dataset $\mathcal{D}_{t,i} \coloneqq \{ \mathbf{x}_{t,i,j}, y_{t,i,j}\}_{j}$, the finite-sample loss for task $(t,i)$ is defined as
% \begin{align}
%  \hat{\mathcal{L}}_{t,i}(\mathbf{B},\mathbf{w};\mathcal{D}_{t,i})  &\coloneqq   \tfrac{1}{2|\mathcal{D}_{t,i}|}\sum_{j}  (\langle \mathbf{Bw}, \mathbf{x}_{t,i,j}\rangle\! -\! y_{t,i,j})^2. \nonumber
% %  + \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
%  \label{fs_loss}
%  \end{align}
% After performing these task-specific updates, the new model parameters can be defined as the average of them, i.e.,
% $$
% \mathbf{B}_{t+1}=\frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i}, \qquad \mathbf{w}_{t+1}=\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}.
% $$
% The above procedure can also be  interpreted as running stochastic gradient with respect to the global loss over all tasks at time~$t$. 


% \noindent\textbf{MAML.} Unlike the previous procedure that  minimizes the average loss across tasks, MAML  minimizes the average loss across tasks {\em after} a small number of task-specific gradient updates. Here, we consider that the task-specific updates are one step of SGD for simplicity.  
% Specifically, letting $\boldsymbol{\theta} \coloneqq [\mathbf{w}^\top; \mathbf{B}]$ the loss function that MAML minimizes is
% \begin{equation*}
%   \min_{\boldsymbol{\theta}} \mathcal{L}_{\text{\tiny{\textit{MAML}}}}(\boldsymbol{\theta}) \coloneqq
%   \mathbb{E}_{\mathbf{w}_{\ast,t,i}}[
%   \mathcal{L}_{t,i}( \boldsymbol{\theta}\!-\! \alpha\nabla_{\boldsymbol{\theta}} \hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta} ))
%   )
%   ].
% \end{equation*}
% MAML essentially runs minibatch SGD on this objective in order to solve it. More precisely, at iteration $t$, it samples $n$ tasks and two i.i.d. datasets $\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out}$ for each task consisting of $m_{in}$ labeled inner loop samples and $m_{out}$ labeled outer loop samples, respectively. For the $i$-th sampled task, in what is known as the inner loop, MAML takes the task-specific gradient step from the initial model $(\mathbf{B}_t, \mathbf{w}_t)$ with step size $\alpha$ using the $m_{in}$ samples for  both the head and representation:
% \begin{align*}
% % \boldsymbol{\theta}_{t+1}& \gets \begin{bmatrix} \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})  \\
% % \mathbf{B}_{t,i} \gets \mathbf{B}_{t} - \alpha \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}) \\
% % \end{bmatrix}
% \boldsymbol{\theta}_{t,i}&= \begin{bmatrix} \mathbf{w}_{t,i}^\top \\
% \mathbf{B}_{t,i} \\
% \end{bmatrix} \gets 
% \begin{bmatrix}
% (\mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}))^\top  \\
% \mathbf{B}_{t} - \alpha \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})  \\
% \end{bmatrix}
% \end{align*}
% Then, in the outer loop, the new parameters are computed by taking a minibatch SGD step with respect to the loss after task-specific adaptation, using step size $\beta$ and the samples $\mathcal{D}_{t,i}^{out}$ for each task. Specifically, 
% \begin{align}
%     \boldsymbol{\theta}_{t+1}&\!\gets\! \boldsymbol{\theta}_t\!-\!\tfrac{\beta}{n}\!\sum_{i=1}^n (\mathbf{I}\!-\!\alpha \nabla^2\!\hat{\mathcal{L}}_{t,i} (\boldsymbol{\theta}_t; \!\mathcal{D}_{t,i}^{out})) \nabla\!\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_{t,i}; \!\mathcal{D}_{t,i}^{out}) 
% % &\quad \quad \quad \quad \nabla\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_t-\alpha  \nabla\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_t; \mathcal{D}_{t,i}^{in}); \mathcal{D}_{t,i}^{out})\big)
% \end{align}
% Note that the above update requires computing second-order derivatives, which is expensive. In practice, the Hessian matrix is often treated as zero, in which case we refer to the algorithm as FO-MAML. We refer to the version of MAML that does not drop the Hessian as Exact MAML.
% % That is, MAML samples a batch of $n$ tasks on each round. For every sampled task, the model parameters take the task-specific gradient step in what is known as the ``inner loop'', namely:
% % \begin{align}
% %     \boldsymbol{\theta}_{t+1} &= \begin{bmatrix} \mathbf{B}_{t} - \alpha 
% %     \end{bmatrix}
% % \end{align}


% \textbf{ANIL.} Surprisingly, \citet{raghu2019rapid} noticed that training neural nets with a modified version of MAML that lacks inner loop updates for the representation resulted in models that matched and sometimes even exceeded the performance of models trained by MAML on few-shot image classification tasks. This modified version is ANIL, and its  inner loop updates in our linear case are given as follows: $\hat{Q}_{t,i}: \mathbb{R}^{D}\rightarrow \mathbb{R}^{D}$
% \begin{align*}
% % \boldsymbol{\theta}_{t+1}& \gets \begin{bmatrix} \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})  \\
% % \mathbf{B}_{t,i} \gets \mathbf{B}_{t} - \alpha \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}) \\
% % \end{bmatrix}
% \boldsymbol{\theta}_{t,i}&%=\hat{Q}_{t,i}(\boldsymbol{\theta}_{t}) 
% =
% \begin{bmatrix} \mathbf{w}_{t,i}^\top \\
% \mathbf{B}_{t,i} \\
% \end{bmatrix}  =
% \begin{bmatrix}
% (\mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}))^\top  \\
% \mathbf{B}_{t}  \\
% \end{bmatrix}
% \end{align*}
% In the outer loop, ANIL again takes a minibatch SGD step with respect to the loss after the inner loop update. 
% % In order to capture the second order-terms resulting from the inner gradient step, we introduce the functions
% %  $\hat{L}_{t,i}(\mathbf{B}_t, \mathbf{w}_t; \mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out})\coloneqq \hat{\mathcal{L}}_{t,i} ( \mathbf{B}_{t,i}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})$. 
%  Then, the outer loop updates for  Exact ANIL are given by:
% %\begin{align*}
% %\boldsymbol{\theta}_{t+1}& \gets \boldsymbol{\theta}_{t+1} - \frac{\beta}{n}\sum_{i=1}^n \begin{bmatrix}
% %\mathbf{I}_k - \alpha \nabla_{\mathbf{w}}^2 \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out}) &  \mathbf{0} \\
% %  -\alpha \tfrac{\partial^2}{\p {\mathbf{B}} \partial{\mathbf{w}}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out})   &  \mathbf{I}  \\  
% %\end{bmatrix}
% %\begin{bmatrix}
% % \mathbf{w}_{t} - \frac{\beta}{n}\sum_{i=1}^n (\mathbf{I}_k - \alpha \nabla_{\mathbf{w}}^2 \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out})) 
% %\nabla_{\mathbf{w}} %\hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, %\mathbf{w}_{t,i}; %\mathcal{D}_{t,i}^{out})^\top  \\
% % \mathbf{B}_{t} - \frac{\beta}{n}\sum_{i=1}^n  
% %\nabla_{\mathbf{B}} %\hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, %\mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out}) %\\
% %\end{bmatrix} \nonumber 
% %\end{align*}
% %or
% \begin{align*}
% \boldsymbol{\theta}_{t+1}\gets \boldsymbol{\theta}_{t} - \frac{\beta}{n}\sum_{i=1}^n 
% \hat{\mathbf{H}}_{t,i}(\mathbf{\theta}_{t}; \mathcal{D}_{t,i}^{out})
% \nabla_{\boldsymbol{\theta}}\hat{\mathcal{L}}_{t,i}(\boldsymbol{\theta}_{t,i},  \mathcal{D}_{t,i}^{out})
% \end{align*}
% where
% \begin{align*}
% \hat{\mathbf{{H}}}_{t,i}&(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out})
% \coloneqq \begin{bmatrix}
% \mathbf{I}_k - \alpha \nabla_{\mathbf{w}}^2 \hat{\mathcal{L}}_{t,i}( \mathbf{\thea}_{t}; \mathcal{D}_{t,i}^{out}) &  \mathbf{0} \\
%   -\alpha \tfrac{\partial^2}{\partial {\mathbf{B}} \partial{\mathbf{w}}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out})   &  \mathbf{I}  
% \end{bmatrix}
% \end{align*}
% In some settings we may not be able to afford second-order updates, in which case we treat $\hat{\mathbf{{H}}}_{t,i}$ as the identity operation.

% }

% execute the FO-ANIL updates:
% \begin{align*}
% \boldsymbol{\theta}_{t+1}& \gets 
% \begin{bmatrix}
% \mathbf{w}_{t} - \frac{\beta}{n}\sum_{i=1}^n  \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})  \\
% \mathbf{B}_{t} - \frac{\beta}{n}\sum_{i=1}^n  \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out}) \\
% \end{bmatrix}
% \end{align*}
% Note the difference between FO and Exact: Exact differentiates through the inner loop update, while FO does not.

% Then, the outer loop gradient is computed by 

% Unlike the previous procedure that has a simple one-loop update, in MAML we have inner and outer loop updates. In the inner loop, we adapt the representation and head based on each task and then in the outer loop we compute the new model by running gradient updates evaluated at the outputs of the inner loop updates. As shown in ???, these inner and outer updates are basically equivalent to minimizing the loss after one step of SGD adaptation. Specifically, letting $\boldsymbol{\theta} \coloneqq [\mathbf{B},\mathbf{w}]$ the loss function that MAML aims to minimize is
% \begin{align*}
%   \min_{\boldsymbol{\theta}} \mathcal{L}_{\text{\tiny{\textit{MAML}}}}(\boldsymbol{\theta})\! \coloneqq
%   &\!\mathbb{E}_{\mathbf{w}_{\ast,t,i}}[
%   \mathcal{L}_{t,i}( \boldsymbol{\theta}\!-\! \alpha\nabla_{\boldsymbol{\theta}} \mathcal{L}_{t,i}(\boldsymbol{\theta} ))
%   )
%   ].
% \end{align*}
% Hence, to solve this objective function by running SGD one has to follow the update:
}}


%\begin{figure}[t]
%\begin{center}
%\vspace{-2mm}
%\centerline{\includegraphics[width=\columnwidth]{inner_loops_.pdf}
% anil_fs_min_alpha1.png}
%\vspace{-2mm}
% \caption{ }
%\caption{GBML algorithm structure.}
%\vspace{-8mm}
%\label{fig:intro2}
%\end{center}
%\end{figure}


% {\color{red}{
% \textbf{ANIL and MAML.}
% % Remark \ref{rem:1} shows that it does not make sense 
% % to minimize the average loss $\mathcal{L}(\mathbf{B}, \mathbf{w})$ if we aim to learn a good representation.
% % To recover $\col{(\mathbf{B}_\ast)}$, 
% Neither ANIL nor MAML directly tries to recover $\col{(\mathbf{B}_\ast)}$. Instead, they execute episodic training procedures that aim to find initial models that minimize the average loss across tasks {\em after a small number of steps of task-specific adaptation}.
% % Formally, 
% To be more precise, we  first introduce the population loss of $(\mathbf{B}, \mathbf{w})$ on task $(t,i)$ by
% \begin{align}
%     \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w}) \coloneqq \tfrac{1}{2}\mathbb{E}_{\mathbf{x}_{t,i},y_{t,i}} \left[(\langle \mathbf{B} \mathbf{w}, \mathbf{x}_{t,i}\rangle - y_{t,i})^2 \right]. %+ \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
% \end{align}
% In MAML, the entire model $(\mathbf{B}, \mathbf{w})$ is adapted to each task with one step of gradient descent on $\mathcal{L}_{t,i}$ which is equivalent to solving the problem
% \begin{align*}
%   &  \min_{\mathbf{B}, \mathbf{w}} \mathcal{L}_{\text{\tiny{\textit{MAML}}}}(\mathbf{B},\! \mathbf{w})\! \coloneqq\\
%   &\!\mathbb{E}_{\mathbf{w}_{\ast,t,i}}[
%   \mathcal{L}_{t,i}( \mathbf{B}\!-\! \alpha\nabla_{\mathbf{B}} \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w} ),  \mathbf{w} \!-\! \alpha \nabla_{\mathbf{w}} \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w} )
%   )
%   ],
% \end{align*}
% while ANIL only locally adapts the head $\mathbf{w}$, and hence its objective is
% \begin{align*}
%     & \min_{\mathbf{B}, \mathbf{w}} \mathcal{L}_{\text{\tiny{\textit{ANIL}}}}(\mathbf{B},\! \mathbf{w})\!  \coloneqq \!\mathbb{E}_{\mathbf{w}_{\ast,t,i}}[\mathcal{L}_{t,i} ( \mathbf{B},\! \mathbf{w} \!-\! \alpha \nabla_{\mathbf{w}} \mathcal{L}_{t,i}(\mathbf{B},\! \mathbf{w} ))] \nonumber %\label{anil_glob_obj} 
%  %\label{maml_glob_obj} 
% \end{align*}
% % papers that use full gradient step in population case:
% % On the Global Optimality of Model-Agnostic Meta-Learning wang et al
% % When MAML Can Adapt Fast and How to Assist When It Cannot arnold et al.
% In practice, evaluating the expectations above
% % in \eqref{anil_glob_obj} and \eqref{maml_glob_obj} 
% is intractable since we can only access finitely-many tasks and samples per task. As a result, ANIL and MAML find approximate solutions during meta-training by executing updates with finite samples.
% % aiming to minimize finite-sample surrogates of \eqref{anil_glob_obj} and \eqref{maml_glob_obj}. 
% For a dataset $\mathcal{D}_{t,i} \coloneqq \{ \mathbf{x}_{t,i,j}, y_{t,i,j}\}_{j}$, the finite-sample loss for task $(t,i)$ is defined as
% \begin{align}
%  \hat{\mathcal{L}}_{t,i}(\mathbf{B},\mathbf{w};\mathcal{D}_{t,i})  &\coloneqq   \frac{1}{2|\mathcal{D}_{t,i}|}\sum_{j}  (\langle \mathbf{Bw}, \mathbf{x}_{t,i,j}\rangle\! -\! y_{t,i,j})^2 \nonumber
% %  + \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 
%  \label{fs_loss}
%  \end{align}
 

% % Using this finite-sample task loss, 
% % we can write the ANIL and MAML meta-training objectives as 
% % \begin{align}&\min_{\mathbf{B}, \mathbf{w}} \hat{\mathcal{L}}_{ANIL}(\mathbf{B}, \mathbf{w}) \coloneqq \nonumber \\
% % &\quad \quad \frac{1}{N }\sum_{i=1}^N \hat{\mathcal{L}}_i(\mathbf{B}, \mathbf{w}\!-\!\alpha \nabla_{\mathbf{w}}\hat{\mathcal{L}}_i(\mathbf{B},\mathbf{w}; \mathcal{D}_{i}^{in});\mathcal{D}_{i}^{out}),  \label{anil_mtloss} \\
% % &\min_{\mathbf{B}, \mathbf{w}} \hat{\mathcal{L}}_{MAML}(\mathbf{B}, \mathbf{w})\! \coloneqq \! \frac{1}{N }\sum_{i=1}^N \hat{\mathcal{L}}_i(\mathbf{B}\!-\!\alpha \nabla_{\mathbf{B}}\hat{\mathcal{L}}_i(\mathbf{B},\mathbf{w}; \mathcal{D}_{i}^{in}),
% % \nonumber \\
% % &\quad \quad \mathbf{w}\!-\!\alpha \nabla_{\mathbf{w}}\hat{\mathcal{L}}_i(\mathbf{B},\mathbf{w}; \mathcal{D}_{i}^{in});\mathcal{D}_{i}^{out})
% % \end{align} 
%     % \text{where } \mathbf{w}_{i} &= \mathbf{w} - \alpha \sum_{j=1}^{m_{in}}  \left(\mathbf{B}^\top \mathbf{x}_{i,j}^{in} (\mathbf{x}_{i,j}^{in})^\top \mathbf{B}\mathbf{w} - y_{i,j}^{in} \mathbf{B}^\top \mathbf{x}_{i,j}^{in}  \right) \label{anil_fs_obj} \\
%     %  \min_{\mathbf{B}, \mathbf{w}} \hat{\mathcal{L}}_{MAML}(\mathbf{B}, \mathbf{w}) &\coloneqq \frac{1}{N}\sum_{i=1}^N \sum_{j=1}^{m_{out}} \tfrac{1}{2} (\langle \mathbf{B}_i \mathbf{w}_{i}, \mathbf{x}_{i,j}^{out}\rangle - y_{i,j}^{out})^2 + \tfrac{\lambda}{2}\|\alpha \mathbf{B}_i^\top \mathbf{B}_i^\top - \mathbf{I}_k\|_F^2 \nonumber\\
%     % \text{where } \mathbf{B}_{i} &= \mathbf{w} - \alpha \sum_{j=1}^{m_{in}}  \left( \mathbf{x}_{i,j}^{in} (\mathbf{x}_{i,j}^{in})^\top \mathbf{B}\mathbf{w}\mathbf{w}^\top - y_{i,j}^{in} \mathbf{x}_{i,j}^{in}\mathbf{w}^\top  \right) - \lambda \alpha \mathbf{B} (\alpha \mathbf{B}^\top\mathbf{B} - \mathbf{I}_k) \label{maml_fs_obj}
% % \begin{align}
% %     \min_{\mathbf{B}, \mathbf{w}} \hat{\mathcal{L}}_{ANIL}(\mathbf{B}, \mathbf{w}) &\coloneqq \frac{1}{N m_{out}}\sum_{i=1}^N \sum_{j=1}^{m_{out}} \tfrac{1}{2} (\langle \mathbf{Bw}_{i}, \mathbf{x}_{i,j}^{out}\rangle - y_{i,j}^{out})^2 + \tfrac{\lambda}{2}\|\alpha \mathbf{B}^\top \mathbf{B}^\top - \mathbf{I}_k\|_F^2 \nonumber\\
% %     \text{where } \mathbf{w}_{i} &= \mathbf{w} - \alpha \sum_{j=1}^{m_{in}}  \left(\mathbf{B}^\top \mathbf{x}_{i,j}^{in} (\mathbf{x}_{i,j}^{in})^\top \mathbf{B}\mathbf{w} - y_{i,j}^{in} \mathbf{B}^\top \mathbf{x}_{i,j}^{in}  \right) \label{anil_fs_obj} \\
% %      \min_{\mathbf{B}, \mathbf{w}} \hat{\mathcal{L}}_{MAML}(\mathbf{B}, \mathbf{w}) &\coloneqq \frac{1}{N}\sum_{i=1}^N \sum_{j=1}^{m_{out}} \tfrac{1}{2} (\langle \mathbf{B}_i \mathbf{w}_{i}, \mathbf{x}_{i,j}^{out}\rangle - y_{i,j}^{out})^2 + \tfrac{\lambda}{2}\|\alpha \mathbf{B}_i^\top \mathbf{B}_i^\top - \mathbf{I}_k\|_F^2 \nonumber\\
% %     \text{where } \mathbf{B}_{i} &= \mathbf{w} - \alpha \sum_{j=1}^{m_{in}}  \left( \mathbf{x}_{i,j}^{in} (\mathbf{x}_{i,j}^{in})^\top \mathbf{B}\mathbf{w}\mathbf{w}^\top - y_{i,j}^{in} \mathbf{x}_{i,j}^{in}\mathbf{w}^\top  \right) - \lambda \alpha \mathbf{B} (\alpha \mathbf{B}^\top\mathbf{B} - \mathbf{I}_k) \label{maml_fs_obj}
% % \end{align}
% % (\mathbf{x}_{i,j}^{out}, y_{i,j}^{out}) \in \mathcal{D}_{i}^{out}
% % (\mathbf{x}_{i,j}^{in}, y_{i,j}^{in}) \in \mathcal{D}_{i}^{in}
% % note that we use separate samples for task-specific adaptation and outer evaluation, as prior work has shown that this is statistically nec for a similar meta-learnign framework \cite{saunshi2021representation}
% % where $N$ is the total number of meta-training tasks, and $\mathcal{D}_i^{in}$ and $\mathcal{D}_{i}^{out}$ are the datasets of the outer and inner loop samples, respectively, for the $i$-th task. We denote $m_{out} = |\mathcal{D}_{i}^{out}|$ and $m_{in} = |\mathcal{D}_{i}^{in}|$  as the numbers of outer and inner loop samples, respectively,  for each task.
% % ANIL and MAML solve the above meta-training objectives by running stochastic gradient descent (SGD). 
% On each iteration $t$, ANIL and MAML sample $n$ tasks and two i.i.d. datasets $\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out}$ for each task consisting of $m_{in}$ labeled inner loop samples and $m_{out}$ labeled outer loop samples, respectively. For the $i$-th sampled task, ANIL and MAML take one step of task-specific SGD from the initial model $(\mathbf{B}_t, \mathbf{w}_t)$ with step size $\alpha$ using the $m_{in}$ samples for the head only (ANIL) or for both the head and representation (MAML), as follows:
% \begin{align}
% &\text{ANIL:}\; \; \mathbf{w}_{t,i} \gets \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}),\; \mathbf{B}_{t,i}\gets  \mathbf{B}_{t} \nonumber \\
% % &\quad \quad \quad \quad  \nonumber \\
% &\text{MAML:}\; \mathbf{w}_{t,i} \gets \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}) \nonumber \\
% &\quad \quad \quad \;\;\; \mathbf{B}_{t,i} \gets \mathbf{B}_{t} - \alpha \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in}) \nonumber 
% \end{align}
% Then, in the outer loop, the initial model is 
% modified with one step of SGD with step size $\beta$ based on the losses of all $n$ inner-loop adapted models.
% The exact outer loop gradient involves second order derivatives of the parameters that are updated on the inner loop. Since evaluating these second-derivatives is expensive, often first-order versions of these algorithms are used, in which the Hessians are treated as zero \citep{finn2017model}. We analyze both first-order ANIL and first-order MAML (FO-ANIL and FO-MAML, respectively) as well as Exact ANIL and Exact MAML (which include the second-order terms) in this paper. 
% % Also, to avoid dealing with higher order products of the data when considering the exact methods, we split each $\mathcal{D}_{t,i}^{out}$ into two equal-sized sets $\mathcal{D}_{t,i}^{out,g}$ and $\mathcal{D}_{t,i}^{out,h}$, which are used to separately  estimate the outer loop gradient and Hessian, respectively.  \ref{firstalg})-(\ref{lastalg}
% The FO-ANIL and FO-MAML outer loop updates are written as follows:
% \begin{align}
%     &\mathbf{w}_{t+1} \gets \mathbf{w}_{t} - \tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t,i}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out}) \label{firstalg} \\
%     & \mathbf{B}_{t+1}\!\gets\!\mathbf{B}_{t}\! - \!\tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{t,i}(\mathbf{{B}}_{t,i}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})
%     % (\mathbf{I}_k\!-\!\alpha \nabla^2_{\mathbf{w}}\hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t},\!\mathbf{w}_{t};\! \mathcal{D}_{t,i}^{out}))\nonumber \\
%     % &\quad\quad\quad\quad \quad\quad\quad\quad \quad\quad \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i};\! \mathcal{D}_{t,i}^{out})
% \end{align}
% Let $\hat{L}_{t,i}(\mathbf{B}_t, \mathbf{w}_t; \mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out})\coloneqq \hat{\mathcal{L}}_{t,i} ( \mathbf{B}_{t,i}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})$. The outer loop updates for Exact ANIL and Exact MAML are:
% \begin{align}
%     &\mathbf{w}_{t+1} \gets \mathbf{w}_{t} - \tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{w}} \hat{{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t};\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out})  \\
%     & \mathbf{B}_{t+1}\!\gets\!\mathbf{B}_{t}\! - \!\tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \hat{{L}}_{t,i}(\mathbf{{B}}_{t}, \mathbf{w}_{t};\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out}) \label{lastalg}
%     % (\mathbf{I}_k\!-\!\alpha \nabla^2_{\mathbf{w}}\hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t},\!\mathbf{w}_{t};\! \mathcal{D}_{t,i}^{out}))\nonumber \\
%     % &\quad\quad\quad\quad \quad\quad\quad\quad \quad\quad \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i};\! \mathcal{D}_{t,i}^{out})
% \end{align}
% Note that $\nabla \hat{L}_{t,i}(\b,\w;\cdot)$ differentiates through the inner loop updates, unlike $\nabla \hat{\mathcal{L}_{t,i}}(\mathbf{B}_{t,i}, \mathbf{w}_{t,i};\cdot)$, which is the gradient of $\hat{\mathcal{L}}_{t,i}$ evaluated at $(\mathbf{B}_{t,i}, \mathbf{w}_{t,i})$.  

% }}
% \begin{align}
%     {F}_{t,i}(\mathbf{B}_t, \mathbf{w}_t; \mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out})&\coloneqq \hat{\mathcal{L}}_{t,i} ( \mathbf{B}_{t,i}, \mathbf{w}_{t,i}
%     % \mathbf{w} - \alpha \nabla_{\mathbf{w}} \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w};\mathcal{D}_{t,i}^{in} )
%     ; \mathcal{D}_{t,i}^{out}) \nonumber \\
%     F_{t,i,\mathbf{B},\mathbf{w};\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out}}(\mathbf{B}, \mathbf{w})&\coloneqq \mathcal{L}_{t,i} ( \mathbf{B}- \alpha\nabla_{\mathbf{B}} \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w};\mathcal{D}_{t,i}^{in} ), \mathbf{w} - \alpha \nabla_{\mathbf{w}} \mathcal{L}_{t,i}(\mathbf{B}, \mathbf{w};\mathcal{D}_{t,i}^{in} ); \mathcal{D}_{t,i}^{out})
% \end{align}

% For \textbf{ANIL and MAML}, the FO and Exact updates for the head are identical up to the different definitions of $\mathbf{B}_{t,i}$: 

% \begin{align}
%     &\text{\small{FO:}}\; \mathbf{w}_{t+1} \gets \mathbf{w}_{t} - \tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out}) \label{firstalg} \\
%     &\text{\small{Exact:}}\; \mathbf{w}_{t+1}\!\gets\!\mathbf{w}_{t}\! - \!\tfrac{\beta}{n}\sum_{i=1}^n (\mathbf{I}_k\!-\!\alpha \nabla^2_{\mathbf{w}}\hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t},\!\mathbf{w}_{t};\! \mathcal{D}_{t,i}^{out}))\nonumber \\
%     &\quad\quad\quad\quad \quad\quad\quad\quad \quad\quad \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i};\! \mathcal{D}_{t,i}^{out})
%     % &\text{FO-ANIL and Exact ANIL:}\; \mathbf{B}_{t+1} \gets \mathbf{B}_{t} - \tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out}) \nonumber
% \end{align}
% % in practice these terms are often ignored with only minor drops in performance .
% % We consider both the first-order versions of these methods 
% Meanwhile, the \textbf{ANIL} outer loop representation updates are equivalent in both FO and Exact cases:
% \begin{align}
%     % &\text{FO-ANIL and Exact ANIL:}\;\nonumber\\ 
%     &\!\text{\small{FO, Exact:}}\; \mathbf{B}_{t+1}\!\gets\! \mathbf{B}_{t}\!-\!\tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i};\! \mathcal{D}_{t,i}^{out})
% \end{align}
% Lastly, the \textbf{MAML} outer loop representation updates are:
% \begin{align}
%     &\text{\small{FO: }}\; \mathbf{B}_{t+1}\! \gets\! \mathbf{B}_{t}\!-\!\tfrac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})\;\\ 
%     &\text{\small{Exact:}}\;\mathbf{B}_{t+1}\!\gets\! \mathbf{B}_{t}\!-\!\tfrac{\beta}{n}\sum_{i=1}^n (\mathbb{I}_{d\times k}\!-\!\alpha \nabla_{\mathbf{B}}^2 \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t},\! \mathbf{w}_{t}; \mathcal{D}_{t,i}^{out,h}))\nonumber \\
%     &\quad \quad  \quad \quad\quad \quad\quad \quad\quad \quad \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out,g}), \label{lastalg}
% \end{align}
% % \citep{finn2017model}. Also, since the only property that our analysis requires of the head iterates  $\{\mathbf{w}_t\}_t$ is that they have norm that is bounded by a constant, and proving this holds is tedious. Also, prior work has observed experimentally that the outer loop updates for the head are irrelevant for representation learning. Thus, for simplicity we enforce the bounded norm by clipping  $\mathbf{w}_t$ if necessary at the end of each iteration. We verify that this clipping is unnecessary in our simulations.
% % Also, we orthogonalize the representation at the end of each round $t$ for both algorithms to simplify the analysis. 
% % {\color{red} address normalization of heads.} 
% where $\mathbb{I}_{d\times k} $ is the identity tensor in $\mathbb{R}^{d\times k\times d \times k}$.
%  The entire procedures are detailed in Algorithm \ref{alg:algs}. A priori, it is not clear that any of these update procedures should lead $\col(\mathbf{B}_t)$
%  to $\col(\mathbf{B}_\ast)$. For instance, if $\alpha=0$, meaning there are no inner loop updates, then  
 
 % Surprisingly, we will show that inner loop updates of the heads can force the column space of the found representation to agree with the ground-truth in all $k$ directions.
% The goal of gradient-based meta-learning is that if we try to find a model $(\mathbf{B}, \mathbf{w})$ that performs well on average across tasks after a few steps of task-specific gradient-based 
% It has been found that such methods perform surprisingly well on 
% Crucially, this model should be able to be quickly modified via a few steps of gradient descent on a new task in order to accurately predict the labels of samples corresponding to that task.
% Neither ANIL nor MAML directly aim to minimize the principle angle distance from their solution $\mathbf{B}$ to $\mathbf{B}_\ast$. Instead, we will show that these algorithms indirectly learn $\mathbf{B}_\ast$ as a byproduct of their optimization dynamics when trying to minimize the linear regression task losses after one step of task-specific adaptation.

% \begin{algorithm}
% \caption{{ FO, Exact ANIL and MAML for Linear Representation Learning}}\label{alg:algs}
% \begin{algorithmic}[1]
% \Require Initialization $\mathbf{{B}}_0: \dist(\mathbf{{B}}_0,\mathbf{{B}}_\ast) \leq c_{init}$, $\alpha \mathbf{B}_0^\top \mathbf{B}_0=\mathbf{I}_k$; $\mathbf{w}_0=\mathbf{0}_k$.
% % \Ensure $y = x^n$
% % \State [Outer Loop]
% \For{$t=0,\dots,T$} \Comment{Outer Loop}
% % \If{MAML}:
% %     \State $\mathbf{w}_t \gets \mathbf{0}_d$ %\gamma \frac{\mathbf{w}_t}{\|\mathbf{w}_t\|_2}$ for some small constant $\gamma$.
% % \EndIf
% \State Sample $\{\mathbf{w}_{\ast,t,i}\}_{i=1}^n \stackrel{iid}{\sim} \nu^n$ (unobserved) and corresponding datasets $\{(\mathcal{D}_{t,i}^{in}, \mathcal{D}_{t,i}^{out})\}_{i=1}^n$
% % \stackrel{iid}{\sim} \nu_{t,i}^{m_{in}+m_{out}}$  $\forall i \in [n]$. %$|\mathcal{D}_{t,i}^{in}|\!=\!m_{in}$, $|\mathcal{D}_{t,i}^{out}|\!=\!m_{out}$ $\forall i \in [n]$
% % \State [Inner Loop]
% \For{$i = 1,\dots,n$} \Comment{Inner Loop}
%     \State $\mathbf{w}_{t,i} \gets \mathbf{w}_{t} - \alpha \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})$
%     \If{MAML}
%     % \State $\mathbf{B}_{t,i} \gets \mathbf{B}_{t} $
%     % \ElsIf{MAML}
%     \State $\mathbf{B}_{t,i} \gets \mathbf{B}_{t} - \alpha \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t}, \mathbf{w}_{t}; \mathcal{D}_{t,i}^{in})$
%     \EndIf
% \EndFor
% % \If{ANIL}
% % \State $\mathbf{w}_{t+1} = \mathbf{w}_{t} - \frac{\beta}{n}\sum_{i=1}^n  \nabla_{\mathbf{B}} f_{i}(\mathbf{\hat{B}}_{t}, \mathbf{w}_{t,i}, \mathcal{D}_{t,i}^{out})$
% % \State  $\mathbf{B}_{t+1} = \mathbf{B}_{t} - \frac{\beta}{n}\sum_{i=1}^n  \nabla_{\mathbf{B}} f_{i}(\mathbf{\hat{B}}_{t}, \mathbf{w}_{t,i}, \mathcal{D}_{t,i}^{out})$
% % \ElsIf{MAML}
% % \If{FO}
% % \State $\mathbf{w}_{t+1}\! \gets \!\mathbf{w}_{t}\! -\! \frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{w}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})$ 
% % \State  $\mathbf{B}_{t+1} \!\gets\! \mathbf{B}_{t}\! -\! \frac{\beta}{n}\sum_{i=1}^n  \nabla_{\mathbf{B}} \hat{\mathcal{L}}_{i}(\mathbf{{B}}_{t,i},\! \mathbf{w}_{t,i}; \mathcal{D}_{t,i}^{out})$ 
% % \Else
% % \State ...
% % \EndIf
% \State Compute outer loop updates $\mathbf{w}_{t+1},\mathbf{B}_{t+1}$ in (\ref{firstalg})-(\ref{lastalg})
% % \State $\mathbf{\hat{B}}_{t+1}, \mathbf{R}_{t+1} = \text{QR}(\mathbf{{B}}_{t+1})$
% % \EndIf
% % \If{$N$ is even}
% %     \State $X \gets X \times X$
% %     \State $N \gets \frac{N}{2}$  
% % \ElsIf{$N$ is odd}
% %     \State $y \gets y \times X$
% %     \State $N \gets N - 1$
% % \EndIf
% % \If{$\|\mathbf{w}_{t+1}\|_2 \geq L_{\max}$}
% % \State $\mathbf{w}_{t+1} \gets L_{\max}\mathbf{w}_{t+1}/\|\mathbf{w}_{t+1}\|_2$ \Comment{Parameter clipping}
% % \EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}


% \begin{rem}[Usefulness of representation learning] Prior work has shown that  if we learn an $\epsilon$-accurate representation $\mathbf{\tilde{B}}$, i.e. $\dist(\mathbf{\tilde{B}}, \mathbf{\hat{B}}_\ast)\leq \delta$, then at meta-test time we use $m_{new}$ samples to learn a head $\mathbf{w}_{new}$ for a new task at meta-test time, we will achieve excess risk $O\left(\delta + \frac{\sqrt{k}}{\sqrt{m_{new}}}\right)$ \citep{tripuraneni2020provable,du2020fewshot}. If $\delta$ is small, {\em then this excess risk is  much smaller than the excess risk of $O\left( \frac{\sqrt{d}}{\sqrt{m_{new}}}\right)$ we would expect by solving for the full $d$-dimensional regressor $\boldsymbol{\theta}_i$ without using the representation.}
% \end{rem}



% \begin{align}
%     \hat{f}_i(\mathbf{B}, \mathbf{w}; (\mathbf{X}_i,\mathbf{y}_i)) &\coloneqq \frac{1}{2}\left\| \mathbf{X}_i \mathbf{B} \mathbf{w} - \mathbf{y}_{i} \right\|_2^2, \quad \mathbf{X}_i \in \mathbb{R}^{m \times d}, \mathbf{y}_i\in \mathbb{R}^{m}
% \end{align}

% MAML
% \begin{align}
%     &\hat{f}_i(U_{r}(\mathbf{B}; (\mathbf{X}_{i}^{m_{in}}, \mathbf{y}_i^{m_{in}})), U_{h}(\mathbf{w}; (\mathbf{X}_{i}^{m_{in}}, \mathbf{y}_i^{m_{in}})); ((\mathbf{X}_{i}^{m_{out}}, \mathbf{y}_i^{m_{out}}))) \nonumber \\
%     U_{r}(\mathbf{B}; (\mathbf{X}_{i}^{m_{in}}, \mathbf{y}_i^{m_{in}}) ) &\coloneqq \mathbf{B} - \alpha \nabla \hat{f}_i(\mathbf{B},\mathbf{w}; (\mathbf{X}_{i}^{m_{in}}, \mathbf{y}_i^{m_{in}})) \nonumber \\
%     U_{h}(\mathbf{w}; (\mathbf{X}_{i}^{m_{in}}, \mathbf{y}_i^{m_{in}}) ) &\coloneqq \mathbf{w} - \alpha \nabla \hat{f}_i(\mathbf{B},\mathbf{w}; (\mathbf{X}_{i}^{m_{in}}, \mathbf{y}_i^{m_{in}})) \nonumber \\
%     %\frac{1}{2}\sum_{j=1}^m \left(\langle \mathbf{B} \mathbf{w}, \mathbf{x}_{i,j} \rangle - y_{i,j} \right)^2,
% \end{align}


% Even for this simple setting, it has not been shown whether ANIL or MAML learn the ground-truth representation.



% Each task is associated with $m$ samples.
% of which $m_{out}$ are used for the outer loop update and $m_{in}$ are used for the inner loop update.  


% \begin{definition}[Principle angle distance]
% Let $ \mathbf{\hat{B}}_{\ast,\perp}$ denote the orthogonal matrix whose columns span the subspace perpendicular to $col(
% \mathbf{B}_\ast)$. Let $\mathbf{\hat{B}}$ denote an orthogonalized version of some matrix $\mathbf{B}$. Then the principle angle distance between $\mathbf{B}$ and  $
% \mathbf{B}_\ast$ is given by 
% \begin{align}
%     \dist(\mathbf{B}, \mathbf{B}_\ast) &\coloneqq \|\mathbf{\hat{B}}_{\ast,\perp}^\top \mathbf{\hat{B}}\|_2.
% \end{align}
% \end{definition}

% Let
% $
% E_0 \coloneqq 1- \dist^2(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)
% $.

% \begin{assumption}[Task diversity]
% The ground-truth heads satisfy  $\sigma_{\min}(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top )\geq {\mu_\ast^2 }$.
% \end{assumption}

% \begin{assumption}[Task normalization]
% For all $i \in [n]$, $\|\mathbf{w}_{\ast,i} \|_2 \leq  L_{\max}$.
% \end{assumption}

% \begin{assumption}
% The initial iterate for the head satisfies $\|\mathbf{w}_{0} \|_2 = 1$.
% \end{assumption}

% The algorithms sample a batch of $n$ tasks on each iteration $t$ as follows: first,  $\mathbf{w}_{\ast,i,t} \sim \mathcal{N}(\mathbf{0}_k, \mathbf{I}_k)$ for all $i \in [n]$. Then, $m$ samples are taken for each task.  



% \textbf{Connections to classification.} Although we focus on multi-task, single-output regression in this paper, our results can be easily extended to the setting in which we try to learn a representation for single-task, multi-output regression problem. The connection between multi-task, single-output regression and single-task, multi-output regression was pointed out in \citet{xu2021representation}. similar to single-task, multi-class classification, our analysis sort of explains the success of pre-training methods for multi-class classification, but these methods are really doing fedrep

% note that by doing label shuffling, we are effectively learning a single head (vector) in the multi-class classification problem. so we are not doing fedrep, so we need local updates.



% \textbf{Importance of inner loop updates.}
% One may first try to learn the representation without performing inner loop updates, i.e. trying to solve the standard problem $\min_{\mathbf{B}, \mathbf{w}} \mathbb{E}_{i} [f_i(\mathbf{B}, \mathbf{w})]$. However, solving this problem does not guarantee that we find the ground-truth representation $\mathbf{B}_\ast$.  A model $(\mathbf{\tilde{B}}, \mathbf{\tilde{w}})$ solves the above problem if and only if $\mathbf{\tilde{B}} \mathbf{\tilde{w}} = \mathbf{\hat{B}}_\ast \mathbb{E}_{i}[\mathbf{w}_{\ast,i}]$. Since this is only one matrix equation, $\mathbf{\tilde{B}}$ must only agree with $\mathbf{\hat{B}}_\ast$ in only one direction, and the other $k-1$ directions of their column spaces may be arbitrarily different. Surprisingly, we will show that inner loop updates of the heads can force the column space of the found representation to agree with the ground-truth in all $k$ directions.






==> ProofSketch.tex <==
\section{Proof sketch} \label{sec:sketch}




We now  discuss how we prove the results in greater detail. We focus on the FO-ANIL case because the presentation is simplest yet still illuminates the key ideas used in all proofs.

\subsection{Theorem 1 (FO-ANIL)}

\noindent {\textbf{Intuition.}} 
Our goal is to show that the distance between the column spaces of $\mathbf{B}_{t}$ and $\mathbf{B}_\ast$, i.e. $\dist_{t} \coloneqq \|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t}\|_2$ is converging to zero at a linear rate for all $t$. 
We will use an inductive argument in which we assume favorable conditions to hold up to time $t$, and will prove they continue to hold at time $t+1$.
% Indeed, when this distance is zero the column space of $\mathbf{{B}}_{t+1}$ equals the column space of $\mathbf{\hat{B}}_*$.
% Our proof will follow an induction structure in which we assume 
% Observe that this distance can be interpreted as the  normalized energy of the learned representation in the subspace orthogonal to  the ground-truth. 
% Our goal is to show that the normalized energy of the learned representation in the subspace orthogonal to  the ground-truth subspace, i.e., $\dist_{t+1} \coloneqq \|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t+1}\|_2$ is converging to zero at a linear rate. Indeed, when this distance is zero the column space of $\mathbf{{B}}_{t+1}$ is identical to the column space of $\mathbf{\hat{B}}_*$.
To show $\dist_{t+1}$ is linearly decaying, it is helpful to first consider the non-normalized energy in the subspace orthogonal to the ground-truth, namely $\|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{{B}}_{t+1}\|_2$.  
 We have observed in equation \eqref{intuition} that if the inner-loop adapted heads $\mathbf{w}_{t,i}$ at time $t$ are diverse, then the FO-ANIL update of the representation subtracts energy from the previous representation and adds energy from the ground-truth representation.
Examining \eqref{intuition} closer, we notice that the only energy in the column space of the new representation that can be orthogonal to the ground-truth subspace is contributed by the previous representation, and this energy 
% in the previous representation 
is contracting at a rate proportional to  the condition number of the matrix formed by the adapted heads. In particular, if we define the matrix $\boldsymbol{\Psi}_t\coloneqq \tfrac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$, then we have
\begin{align}
    \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 &=\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}(\mathbf{I}-\beta \mathbf{\Psi}_t)\|_2 \nonumber \\
    &\leq ( 1 - \beta \lambda_{\min}(\mathbf{\Psi}_t))\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}\|_2, \label{psisi}
\end{align}
% where the inequality holds
as long as $\beta \leq \nicefrac{1}{\lambda_{\max}(\mathbf{\Psi}_t)}$. 
Therefore, to show that the normalized energy $\|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t+1}\|_2$ approaches zero, we aim to show: (I) The condition number of $\mathbf{\Psi}_t$ continues to stay controlled and finite, which implies linear convergence of the non-normalized energy in $\col(\mathbf{B}_\ast)^\perp$ according to \eqref{psisi}; and (II) The minimum singular value of the representation $\mathbf{B}_{t+1}$ is staying the same. Otherwise, the energy orthogonal to the ground-truth subspace could be decreasing, but the representation could be becoming singular, which would mean the distance to the ground-truth subspace is not decreasing. 


% OLD
% -------------
% \noindent {\textbf{Intuition.}} Our goal is to show that the normalized energy of the learned representation in the subspace orthogonal to  the ground-truth subspace, i.e., $\dist_{t+1} \coloneqq \|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t+1}\|_2$ is converging to zero at a linear rate. Indeed, when this distance is zero the column space of $\mathbf{{B}}_{t+1}$ is identical to the column space of $\mathbf{\hat{B}}_*$.
%  It is helpful to first consider the non-normalized energy in the orthogonal subspace, namely $\|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{{B}}_{t+1}\|_2$.  We have seen in equation \eqref{intuition} that if the inner-loop adapted heads $\mathbf{w}_{t,i}$ are diverse, then the FO-ANIL update of the representation subtracts energy from the previous representation and adds energy from the ground-truth representation.
% Examining \eqref{intuition} closer, we see that the only energy in the column space of the new representation that can be orthogonal to the ground-truth subspace is contributed by the previous representation, and the energy in the previous representation is contracting at a rate proportional to  the condition number of the matrix formed by the adapted heads. In particular, if we define the matrix $\boldsymbol{\Psi}_t\coloneqq \tfrac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$, then we have
% \begin{align}
%     \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 &=\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}(\mathbf{I}-\beta \mathbf{\Psi}_t)\|_2 \nonumber \\
%     &\leq ( 1 - \beta \lambda_{\min}(\mathbf{\Psi}_t))\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}\|_2, \label{psisi}
% \end{align}
% % where the inequality holds
% as long as $\beta \leq \nicefrac{1}{\lambda_{\max}(\mathbf{\Psi}_t)}$. 
% Therefore, to show that the normalized energy $\|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t+1}\|_2$ approaches zero, we aim to show: (I) The condition number of $\mathbf{\Psi}_t$ is controlled and finite, which implies linear convergence of the non-normalized energy in $\col^\perp(\mathbf{B}_\ast)$ according to \eqref{psisi}; and (II) The minimum singular value of the representation $\mathbf{B}_{t+1}$ is staying the same. Otherwise, the energy orthogonal to the ground-truth subspace could be decreasing, but the representation could be becoming singular, which would mean the distance to the ground-truth subspace is not decreasing. 
%----------------------

To show (I), note that the adapted heads are given by:
\begin{align}
    \mathbf{w}_{t,i}=
    \underbrace{\del_t\mathbf{w}_t}_{\text{non-unique}} +\; \alpha \underbrace{\mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}}_{\text{unique}}, \label{updw}
    \vspace{-2mm}
\end{align}
where $\del_t \coloneqq \mathbf{I}_k \!- \alpha \b^\top \b$. 
The vector $\del_t \mathbf{w}_t$ is present in every $\mathbf{w}_{t,i}$,
% so it does not contribute to the diversity of the $\mathbf{w}_{t,i}$'s, 
so we refer to it as the non-unique part of $\mathbf{w}_{t,i}$. On the other hand, $\alpha \mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}$ is the unique part of $\mathbf{w}_{t,i}$. 
Equation \eqref{updw} shows that if the non-unique part of each $\mathbf{w}_{t,i}$ is relatively small compared to the unique part, then $\mathbf{\Psi}_t \approx \alpha^2 \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\Psi}_{\ast,t} \mathbf{B}_\ast^\top \mathbf{B}_t$, 
% then the diverse part of $\mathbf{w}_{t,i}$ dominates, and 
meaning the $\mathbf{w}_{t,i}$'s are almost as diverse as the ground-truth heads. So we aim to show $\|\del_t\|_2$ and $\|\mathbf{w}_t\|_2$ remain small for all $t$. We specifically need to show they are small compared to $\sigma_{\min}^2(\mathbf{B}_{t}^\top \mathbf{B}_\ast)$, since this quantity roughly lower bounds the energy in the diverse part of $\mathbf{w}_{t,i}$. {One can show that $\sigma_{\min}^2(\mathbf{\hat{B}}_{t}^\top \mathbf{B}_\ast) = 1 - \dist_t^2$, so we need to use that $\dist_t$ is decreasing in order to lower bound the energy in the unique part of $\mathbf{w}_{t,i}$.}


% To show (I), note that the adapted heads are given by:
% \begin{align}
%     \mathbf{w}_{t,i}\!=
%     \!\underbrace{\del_t\mathbf{w}_t}_{\text{non-diverse}}\!+\alpha \underbrace{\mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}}_{\text{diverse}}, \label{updw}
% \end{align}
% where $\del_t \coloneqq \mathbf{I}_k \!- \alpha \b^\top \b$. 
% The vector $\del_t \mathbf{w}_t$ is present in every $\mathbf{w}_{t,i}$
% % so it does not contribute to the diversity of the $\mathbf{w}_{t,i}$'s, 
% so we refer to it as the non-diverse part of $\mathbf{w}_{t,i}$. On the other hand, $\alpha \mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}$ is unique for each $i$, so this is the diverse part of $\mathbf{w}_{t,i}$. 
% Equation \eqref{updw} shows that if $\del_t \mathbf{w}_t$  is relatively small compared to $\alpha\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{t,i}$, 
% % then the diverse part of $\mathbf{w}_{t,i}$ dominates, and 
% then the $\mathbf{w}_{t,i}$'s are almost as diverse as the ground-truth heads. So we aim to show $\|\del_t\|_2$ and $\|\mathbf{w}_t\|_2$ remain small throughout the algorithm's execution, most importantly in relation to $\sigma_{\min}^2(\mathbf{B}_{t}^\top \mathbf{B}_\ast)$, since this quantity lower bounds the energy in the diverse part of $\mathbf{w}_{t,i}$, roughly speaking. One can show that $\sigma_{\min}^2(\mathbf{\hat{B}}_{t}^\top \mathbf{B}_\ast) = 1 - \dist_t^2$, so we need to use that $\dist_t$ is decreasing in order to lower bound the energy in the diverse part of $\mathbf{w}_{t,i}$.


It is also convenient to track $\|\del_t\|_2$ in order to show (II), since $\|\del_{t+1}\|_2\leq \varepsilon$ implies  $\sigma_{\min}(\mathbf{B}_{t+1})\geq  \tfrac{\sqrt{1-\varepsilon}}{\sqrt{\alpha}}$. Note that for (II), we need control of $\|\del_{t+1}\|_2$, whereas to show (I) we needed control of $\|\del_t\|_2$. This difference in time indices is accounted for by the induction we will soon discuss.
 

% The choice of initialization entails $\|\del_0\|_2=0$ and $\|\mathbf{w}_t\|_2=0$, so these quanties are initially small (in fact, these quantites to not have to be initialized at exactly


It is now evident why it makes sense to initialize with $\|\del_0\|_2=0$ and $\|\mathbf{w}_t\|_2=0$ (in fact, they do not have to be exactly zero; any initialization with $\|\mathbf{w}_0\|_2=O(\sqrt{\alpha})$ and  $\|\del_t\|_2=O({\alpha}^2)$ would suffice). 
However, proving that $\|\del_t\|_2$ and $\|\mathbf{w}_t\|_2$ remain small  is difficult
because the algorithm lacks explicit regularization or a normalization step after each round. 
Empirically, $\sigma_{\min}(\mathbf{B}_t)$ may decrease and $\|\mathbf{w}_t\|_2$ may increase on any particular round, so it is not clear why $\sigma_{\min}(\mathbf{B}_t)$ does not go to zero (i.e. $\|\del_t\|_2$ does not go to 1) and $\|\mathbf{w}_t\|_2$ does not blow up. To address these issues, one could add an explicit regularization term to the loss functions or an orthonormalization step to the algorithm, but doing so is empirically unnecessary and  would not be consistent with the ANIL formulation or algorithm.


\begin{figure*}[t]
\vspace{3mm}
\begin{center}
\centerline{\includegraphics[width=0.98\textwidth]{flow.pdf}
% anil_fs_min_alpha1.png
}
\vspace{0mm}
% \caption{ }
\caption{Logical flow of the proof. Note that there are no cycles among the implications from $t+1$ to $t+1$, so the logic is consistent.}
\vspace{-2mm}
\label{fig:flow}
\end{center}
\end{figure*}





% Indeed, we prove that $\|\mathbf{w}_t\|_2$ naturally remains small and the spectrum of $\mathbf{B}_t$ naturally stays roughly the same throughout algorithm execution.
\textbf{Inductive structure.}
We overcome the aforementioned challenges by executing a multi-way induction that involves the following six inductive hypotheses:
\begin{enumerate}
\vspace{-2mm}
\item $A_1(t) \coloneqq \{\|\mathbf{w}_t\|_2 = O(\sqrt{\alpha} \min(1,\tfrac{\mu_\ast^2}{\eta_\ast^2})\eta_\ast  )\}$,
   \item $A_2(t) \!\coloneqq\! \!\big\{\|\del_t\|_2 \!\leq\! \rho\|\del_{t-1}\|_2
 \!+\! O(\beta^2\alpha^2 L_{\ast}^4 \dist^2_{t-1})\big\}$, %redefine like A5
       \item $A_3(t) \coloneqq \big\{\|\del_t  \|_2 \leq \tfrac{1}{10}\big\}$, 
       \item $A_4(t) \coloneqq \big\{0.9\alpha E_0 \mu_\ast\mathbf{I}_k \preceq \mathbf{\Psi}_t \preceq 1.2\alpha L_\ast^2 \mathbf{I}_k \big\}$, 
        \item $A_5(t) \coloneqq \big\{\|\mathbf{{B}}_{\ast,\perp}^\top \mathbf{{B}}_{t} \|_2  \leq \rho \|\mathbf{{B}}_{\ast,\perp}^\top \mathbf{{B}}_{t-1} \|_2  \big\}$,  
     \item  $A_6(t) \coloneqq \{\dist_{t}=\|\mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_t\|_2 \leq \rho^{t-1} \}$,  
\end{enumerate}
\vspace{-2mm}
where $\rho\!=\!1 - 0.5\beta \alpha E_0 \mu_\ast^2$.  Our previous intuition motivates our choice of inductive hypotheses $A_1(t),\dots,A_5(t)$ as intermediaries to ultimately show that $\dist_t$ linearly converges to zero.  More specifically,  $A_1(t),A_2(t),$ and $A_3(t)$ bound  $\|\mathbf{w}_t\|_2$ and  $\|\del_t\|_2$, $A_4(t)$ controls the diversity of the inner loop-adapted heads, and  $A_5(t)$ and $A_6(t)$ confirm that the learned representation approaches the ground-truth.
We employ two upper bounds on $\|\del_t\|_2$ because we need to use that $\{\|\del_t\|_2\}_t$ is both summable $(A_2(t))$ and uniformly small $(A_3(t))$ to complete different parts of the induction. In particular, if true for all $t$, $A_2(t)$ shows that $\|\del_t\|_2$ may initially increase, but eventually linearly converges to zero due to the linear convergence of $\dist_t$. The initialization implies each inductive hypothesis holds at time $t=1$. We must show they hold at time $t+1$ if they hold up to time $t$. 



To do this, we employ the logic visualized in 
Figure \ref{fig:flow}. 
The top level events ($A_1(t+1), A_2(t+1), A_5(t+1)$) are most ``immediate'' in the sense that they follow directly from other events at all times up to and including $t$ (via the dashed green arrows). The proofs of all other events at time $t\!+\!1$ require the occurrence of other events at time $t+1$, with more logical steps needed as one moves down the graph, and solid red arrows denoting implications from and to time $t+1$. In particular, $A_3(t+1)$ requires the events up to and including time $t$ {\em and} a top-level event at $t+1$, namely $A_2(t+1)$, so it is in the second level. Similarly, $A_6(t+1)$ requires events up to and including  time $t$ and the second-level event at $t\!+\!1$, so it is in the third level, and so on. 

% The inductive logic in Figure \ref{fig:flow} is consistent with our intuition.
Recall that our intuition is that diverse adapted heads lead to contraction of the non-normalized representation distance. This logic drives the implication $A_4(t)\!\implies\! A_5(t+1)$. 
 We then reasoned that contraction of the non-normalized distance leads to linear convergence of the distance as long as the minimum singular value of the representation is controlled from below. This intuition is captured in the implication  $A_5(t+1)\cap A_3(t+1)\! \implies \!A_6(t+1)$.  


We also discussed that the diversity of the adapted heads depends on the global head being small, the representation being close to a scaled orthonormal matrix, and the representation distance being bounded away from 1 at the start of that iteration. This is ensured by the implication that the adapted heads are again diverse on iteration $t+1$, in particular
%  Then, to show that the adapted heads are again diverse at $t+1$, we need to use that $\|\mathbf{w}_{t+1}\|_2$, $\|\del_{t+1}\|_2$, and $\dist_{t+1}$ are all small (
 $A_1(t+1)\cap A_3(t+1)\cap A_6(t+1)\! \implies\! A_4(t+1)$.
% Now, in order to have diversity of the adapted heads on the next round, our intuition was that the concurrent global head $\|\mathbf{w}_{t+1}\|_2$ and $\|\del_{t+1}\|_2$ must be small. We see this logic
% Note that the structure of the logic graph appears different than our intuition, because here we assume that the  $\mathbf{w}_{t,i}$'s are diverse at time $t$ in order make the inductive argument. But if we look one step in the future, we can see that small $\|\mathbf{w}_{t+1}\|_2$ and small $\|\del_{t+1}\|_2$ imply diverse $\mathbf{w}_{t+1,i}$'s, which in turn implies $\dist_{t+2}\leq \rho^{t+1}$, consistent with our intuition.
The other implications in the graph are technical and needed to control $\|\mathbf{w}_{t+1}\|_2$ and $\|\del_{t+1}\|_2$.


\textbf{Proving the implications.}
We now formally discuss each implication, starting with the top level. Full proofs are provided in Appendix \ref{app:anil}.
\begin{itemize}[leftmargin=10pt]
\vspace{-2mm}
        \item $A_4(t)\!\implies \! A_5(t\!+\!1)$. This is true by equation \eqref{psisi}.
\vspace{-1mm}
    \item $A_1(t)\cap A_3(t)\cap A_6(t) \!\implies\! A_2(t\!+\!1)$. It can be shown that $\del_{t+1}$ is of the form:
    \begin{align}
        \del_{t+1}\!&=\! \del_t(\mathbf{I}_k\!-\! \beta \alpha^2  \b^\top \mathbf{B}_\ast \mathbf{\Psi}_{\ast, t} \mathbf{B}_\ast^\top \b) \!+\! \mathbf{N}_{t}
    \end{align}
    for some matrix $\mathbf{N}_{t}$ whose norm is upper bounded by a linear combination of $\|\del_t\|_2$ and $\dist_t$. We next use
    \begin{align}
        \lambda_{\min}(\b^\top \mathbf{B}_\ast \mathbf{\Psi}_{\ast, t} \mathbf{B}_\ast^\top \b )\! &\geq \! \mu_\ast^2 \sigma_{\min}^2(\b^\top \mathbf{B}_\ast)\nonumber \\
        &\geq \! \tfrac{0.9}{\alpha} \mu_\ast^2 (1 \!-\! \dist_t^2 )\label{eoo}
    \end{align}
    where \eqref{eoo} follows by $\sigma_{\min}^2(\mathbf{\hat{B}}_t^\top \mathbf{B}_\ast)\!=\!1\!-\!\dist_t^2$ and $A_3(t)$.  The proof follows by applying $A_6(t)$ to control $1\!-\!\dist_t^2$.
    \vspace{-3mm}
    \item $\left( \cap_{s=1}^{t}A_2(s) \cap A_6(s)\right)\!\implies\! A_1(t\!+\!1)$. This is the most difficult induction to show. The FO-ANIL dynamics are such that $\|\mathbf{w}_t\|_2$ may increase on every iteration throughout the entire execution of the algorithm. However, we can exploit the fact that the amount that it increases is proportional to $\|\del_t\|_2$, which we can show is summable due 
    to the linear convergence of $\dist_t$. First, we have
    \begin{equation*}
    \vspace{-1mm}
        \mathbf{w}_{t+1}\! =\! (\mathbf{I}_k\! - \!\beta \mathbf{B}_t^\top \mathbf{B}_t\del_t)\mathbf{w}_t +\frac{\beta}{n}\sum_{i=1}^n \del_t \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}
        \vspace{-1mm}
    \end{equation*}
    which implies $\|\mathbf{w}_t\|_2$ increases on each iteration by $O(\frac{\beta}{\sqrt{\alpha}}\|\del_{t}\|_2 \eta_\ast)$. In particular,
     \begin{align}
        \|\mathbf{w}_{t+1}\|_2 &\stackrel{(a)}{\leq} (1 +\tfrac{2\beta}{\alpha}\|\del_t\|_2)\|\mathbf{w}_{t}\|_2 + \tfrac{2\beta L_\ast}{\sqrt{\alpha}}\|\del_t\|_2 \nonumber \\
        &\stackrel{(b)}{\leq} \sum_{s=0}^{t-1}\tfrac{2\beta \eta_\ast}{\sqrt{\alpha}}\|\del_s\|_2 \prod_{r=s}^{t-1}(1 +\tfrac{2\beta}{\alpha}\|\del_r\|_2)  \nonumber \\
        &\stackrel{(c)}{\leq} \sum_{s=0}^{t-1}\!\tfrac{2\beta \eta_\ast}{\sqrt{\alpha}}\|\del_s\|_2 \Big(1 \!+\!\tfrac{1}{t-s}\sum_{r=s}^{t-1}\!\tfrac{2\beta}{\alpha}\|\del_r\|_2\Big)^{t-s} \nonumber %\label{eqn1} %
        % &\leq  \sum_{s=0}^{t-1}\frac{2\beta\eta_\ast}{\sqrt{\alpha}} z_s \prod_{r=s}^{t-1}(1 +\frac{2\beta}{\alpha}z_r) \nonumber
    \end{align}
    where $(b)$ follows by recursively applying $(a)$ for $t,t\!-\!1,...$. and $(c)$ follows by the AM-GM inequality.
    Next, for any $s\in[t]$, recursively apply $A_2(s)$,$A_2(s\!-\!1),...$ and use $A_6(r)\; \forall r \in [s]$ to obtain, for an absolute constant $c$,
    \begin{align}
        \|\del_{s}\|_2 %&\leq \gamma \|\del_{s-1}\|_2 + c\beta^2 \alpha^2 L_\ast^4 \dist_{s-1}^2 \nonumber \\
        \!&\stackrel{(d)}{\leq}\! c\sum_{r=0}^{s-1} \rho^{s-r}\beta^2 \alpha^2 L_\ast^4 \dist_{r}^2\! \leq \!c \rho^{s} \sum_{r=0}^{s-1}\rho^r \beta^2 \alpha^2 L_\ast^4 \nonumber%\label{eqn_trott}
    \end{align}
    Plugging $(d)$ into $(c)$, computing the sum of geometric series, and applying the choice of $\beta$ completes the proof.
    % \begin{align}
    %     \|\mathbf{w}_{t+1}\|_2 \leq c\tfrac{\beta}{\sqrt{\alpha}}\kappa_\ast^4L_\ast =:\sqrt{\tau_1}
    % \end{align}
    
    
    
    
    
    % First, we recursively apply $A_1(s)$, $A_1(s\!-\!1), ...$ to obtain
    % \begin{align}
    %     \|\del_{s}\|_2 %&\leq \gamma \|\del_{s-1}\|_2 + c\beta^2 \alpha^2 L_\ast^4 \dist_{s-1}^2 \nonumber \\
    %     &\leq c\sum_{r=0}^{s-1} \rho^{s-r}\beta^2 \alpha^2 L_\ast^4 \dist_{r}^2\label{eqn_trot}
    % \end{align}
    % where we have also used the fact that $\|\del_0\|_2=0$. 
    % % , and $\gamma$ is the contractive factor in $A_1(\cdot)$. Note that we can write $ \gamma\!=\!1\!-\! c_\gamma \beta \alpha\mu_{\ast}^2 $ for some constant $c_\gamma$ and sufficiently small $\beta, \alpha$. 
    % % From $A_5(r)$, we have $\dist_r \leq \rho^{r-1}$ for $\rho \!=\! 1\!-\!c_\rho \beta\alpha\mu_{\ast}^2$. Let $q\coloneqq \max(\gamma,\rho) $. 
    % Equation \eqref{eqn_trot} implies 
    % \begin{align}\|\del_{s}\|_2 &\leq c q^{s-1}\sum_{r=0}^{s-1} \beta^2 \alpha^2 L_\ast^4 \min(q^{r-1},1)\nonumber\\
    % &\leq c q^{s-1}\frac{\beta^2 \alpha^2 L_\ast^4}{1-q} \leq c' q^{s-1} \beta \alpha \kappa_{\ast}^4 \label{eqneqn}
    % \end{align}
    % Now we use the equation , which implies $\|\mathbf{w}_t\|_2$ increases on each iteration by $O(\frac{\beta}{\sqrt{\alpha}}\|\del_{t}\|_2(\eta_\ast\!+\!\frac{\|\mathbf{w}_t\|_2}{\sqrt{\alpha}}))$, that is:
    % \begin{align}
    %     \|\mathbf{w}_{t+1}\|_2 &\stackrel{(a)}{\leq} (1 +\tfrac{2\beta}{\alpha}\|\del_t\|_2)\|\mathbf{w}_{t}\|_2 + \tfrac{2\beta\eta_\ast}{\sqrt{\alpha}}\|\del_t\|_2 \nonumber \\
    %     &\stackrel{(b)}{\leq} \sum_{s=0}^{t-1}\tfrac{2\beta\eta_\ast}{\sqrt{\alpha}}\|\del_s\|_2 \prod_{r=s}^{t-1}(1 +\tfrac{2\beta}{\alpha}\|\del_r\|_2)  \nonumber \\
    %     &\stackrel{(c)}{\leq} \sum_{s=0}^{t-1}\tfrac{2\beta\eta_\ast}{\sqrt{\alpha}}\|\del_s\|_2 \Big(1 +\tfrac{1}{t-s}\sum_{r=s}^{t-1}\tfrac{2\beta}{\alpha}\|\del_r\|_2\Big)^{t-s}  %\label{eqn1} %
    %     % &\leq  \sum_{s=0}^{t-1}\frac{2\beta\eta_\ast}{\sqrt{\alpha}} z_s \prod_{r=s}^{t-1}(1 +\frac{2\beta}{\alpha}z_r) \nonumber
    % \end{align}
    % where $(b)$ follows by recursively applying $(a)$ for $t,t\!-\!1,$ etc. and $(c)$ follows by the AM-GM inequality. Plugging \eqref{eqneqn} into $(c)$ shows that \begin{align}
    %     \|\mathbf{w}_{t+1}\|_2 \leq c\tfrac{\beta}{\sqrt{\alpha}}\kappa_\ast^4\eta_\ast =:\sqrt{\tau_1}
    % \end{align}
    
    \vspace{-1mm}
    \item $A_2(t\!+\!1) \cap A_3(t)\! \implies\! A_3(t\!+\!1)$. This follows straightforwardly since $\beta$ is chosen sufficiently small.
    \vspace{-1mm}
    \item $A_3(t\!+\!1) \cap \left(\cap_{s=1}^{t+1} A_5(s)\right) \cap A_6(t)\! \implies \! A_6(t\!+\!1)$.  Using the definition of the principal angle distance, the Cauchy-Schwarz inequality, and $\cap_{s=1}^{t+1} A_5(s)$, we can show
    \begin{align*}
        \dist_{t\!+\!1}\! &\leq \! \tfrac{1}{\sigma_{\min}(\mathbf{B}_{t+1})}\|\mathbf{\hat{B}}_{\ast,\perp}^\top\! \mathbf{{B}}_{t\!+\!1}\|_2
        \!\leq\! \tfrac{\sigma_{\max}(\mathbf{B}_{0})}{\sigma_{\min}(\mathbf{B}_{t+1})}\rho^t\dist_0 
    \end{align*}
    from which the proof follows after applying $A_3(t\!+\!1)$ and the initial conditions. Note that here we have normalized the representation only once at time $t\!+\!1$ and used the contraction of the non-normalized energy to recurse from $t\!+\!1$ to $0$, resulting in a $\tfrac{\sigma_{\max}(\mathbf{B}_0)}{\sigma_{\min}(\mathbf{B}_{t+1})}$ scaling error. If we instead tried to directly show the contraction of distance and thereby normalized analytically on every round, we would obtain $\dist_{t\!+\!1}\leq \big(\prod_{s=0}^t \tfrac{\sigma_{\max}(\mathbf{B}_{s})}{\sigma_{\min}(\mathbf{B}_{s+1})}\big) \rho^t \dist_0$, meaning a $\prod_{s=0}^t \tfrac{\sigma_{\max}(\mathbf{B}_{s})}{\sigma_{\min}(\mathbf{B}_{s+1})}$ scaling error, which is too large because $\mathbf{B}_s$ is in fact not normalized on every round.
    \vspace{-4mm}
    \item $A_1(t+1) \cap  A_3(t+1) \cap A_6(t+1)\!\implies \! A_4(t+1)$. This follows by expanding each $\mathbf{w}_{t,i}$ as in \eqref{updw}, and using similar logic as in \eqref{eoo}. 
    % Observe that in order to lower bound the magnitude of the diverse part of each $\mathbf{w}_{t,i}$, we need to lower bound $\sigma_{\min}(\mathbf{\hat{B}}_{\ast,\perp}^\top\! \mathbf{{B}}_{t})$, which can be obtained via $A_6(t)$ as in \eqref{eoo}.
\vspace{-1mm}
\end{itemize}


\subsection{Other results -- ANIL, FO-MAML, and MAML} \label{sec:52}

% Now we discuss how to extend the proof to the other algorithms. 
For ANIL, the inductive structure is nearly identical. The only meaningful change in the proof is that the second-order updates imply $\|\mathbf{w}_{t+1}\|_2\!-\!\|\mathbf{w}_{t}\|_2= O(\|\del_t\|_2^2)$, which is smaller than the $O(\|\del_t\|_2)$ for FO-ANIL, and thereby allows to control $\|\mathbf{w}_{t+1}\|_2$ with  a potentially larger $\beta$. %{\color{red}This demonstrates the benefit of second-order updates for ANIL.}


For FO-MAML and MAML, recall that the inner loop update of the representation weakens the benefit of adapted head diversity (see Section~\ref{sec:intuition}). Thus, {larger} adapted head diversity is needed to learn $\col(\mathbf{B}_\ast)$.
Specifically, we require a tighter bound of $\|\del_t\|_2=O(\alpha^2)$, compared to the  $\|\del_t\|_2=O(1)$ bound in ANIL, and for FO-MAML, we also require a tighter bound on $\|\w\|_2$ (recall from Section \ref{sec:sketch} that smaller $\|\del_t\|_2$ and $\|\w\|_2$ improves adapted head diversity). Moreover, to obtain tight bounds on $\|\mathbf{w}_{t+1}\|_2$ we can no longer use that $\|\mathbf{w}_{t+1}\|_2\!-\!\|\mathbf{w}_{t}\|_2$ is controlled by $\|\del_t\|_2$ due to to additional terms in the outer loop update. To overcome these issues, we must make 
stricter assumptions on the initial distance, and in the case of FO-MAML, on the average ground-truth head. Please see Appendix \ref{app:maml} for details.

% fig 1: initialization

% 95-100, 90-95, 80-90, 70-80 random init quality
% hold diversity constant. spherical gaussian samples from not mean zero

% fig 2: avg
% standard basis vectors
% vs normal at mean zero





% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\columnwidth}
%          \centering
%          \includegraphics[width=0.3\columnwidth]{anilmamlsims1.pdf}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\columnwidth}
%          \centering
%          \includegraphics[width=0.3\columnwidth]{anilmamlsims2.pdf}
%          \caption{$y=3sinx$}
%          \label{fig:three sin x}
%      \end{subfigure}
% \end{figure}

% \begin{figure}[h]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=\columnwidth]{anilmamlsims.pdf}
% % anil_fs_min_alpha1.png
% }
% \vspace{-2mm}
% % \caption{ }
% \caption{Random initialization of $\mathbf{B}_0$. Methodical initialization of $\mathbf{B}_0$. In both cases, the mean of the average ground-truth heads is far from zero. }
% \vspace{-8mm}
% \label{fig:sims2}
% \end{center}
% \end{figure}



Finally, the proof of Theorem \ref{thm:anil_fs} relies on showing concentration of the finite-sample gradients to the population gradients. 
The principal challenge is showing this concentration  for fourth-order products of the data that arise in the ANIL updates, since we cannot apply standard methods to these higher-order products while maintaining $o(d)$ samples per task. Instead, we leverage the low-rankness of the products by applying a truncated version of the concentration result for low-rank random matrices from \citep{magen2011low}. We also use the L4-L2-hypercontractiveness of the data to control the bias in these higher-order products. Details are found in Appendix \ref{app:anil_fs}.

% First observe that $A_{4}(t+1)\implies A_5(t+1)$ by equation \eqref{psisi}.



% $A_3(t),A_4(t),A_5(t) \!\implies\! A_5(t+1)$ since the contraction of the representation's non-normalized energy in the orthogonal subspace $(A_4(t))$ and the stability of its singular values $(A_3(t))$ imply that its distance to the ground-truth subspace is decreasing, as previously discussed. Likewise, we have seen in \eqref{psisi} that $A_4(t+1)$ holds as long as the inner-loop adapted heads are sufficiently diverse, which, recalling \eqref{updw}, is implied by $A_1(t)$ and $A_3(t)$. Next,
%  $A_3(t+1)$ follows straightforwardly by $A_2(t)$, $A_3(t)$, and choice of outer loop step size $\beta$.
%  This uniform upper bound on $\|\del_t\|_2$ is sufficient to show $A_4(t+1)$, but we need a tighter bound, given by $A_2(t)$, in order to prove $A_1(t+1)$. 
%  Indeed, $A_1(t\!+\!1)$ and $A_2(t\!+\!1)$ are the most difficult parts of the induction.
 
% It remains to show the most difficult parts of the induction: $A_1(t\!+\!1)$ and $A_2(t\!+\!1)$. For $A_2(t\!+\!1)$ 


 
 
%  We will soon see that both bounds on $\del_t\|_2$ are useful for other parts of the induction.
% Note that showing $A_5(t)$ holds for all $t$ implies that $\dist_t$ is linearly converging to zero.

% and $\tau_1 = O(\frac{\beta^2 \kappa_{\ast}^8 \eta_\ast^2}{\alpha})$ and $\tau_2 = O(\frac{1}{\kappa_\ast^4})$ are parameters used in the analysis only.




% As a result, it becomes imperative to control two quantities: $\|\del_t\|_2$ and $\|\mathbf{w}_t\|_2$. To see this, we can observe that the 


% By definition of the inner loop update, if we assume the ground-truth heads are diverse, then the updated heads are diverse as long as $\|\mathbf{w}_t\|_2$ and $\|\del_t\|_2$ are small, where $\del_t := \mathbf{I}- \alpha \b^\top \b$. So, to show (1), we aim to prove that $\|\mathbf{w}_t\|_2$ and $\|\del_t\|_2$ remain small. Conveniently, showing that $\|\del_t\|_2$ remains small also implies (2). Showing these quantities remain small requires an interconnected inductive argument that also accounts for the distance to ground-truth subspace going to zero. In particular, we can show that if the distance is non-increasing and $\|\mathbf{w}_t\|_2$ is small, then $\|\del_{t+1}\|_2$ is the sum of a contraction of $\|\del_{t}\|_2$ plus $\dist_t$, so it is eventually going to zero. Also, $\|\mathbf{w}_{t+1}\|_2$ is the sum of $\|\del_{s}\|_2$ terms for $s=1,\dots,t$, so $\|\mathbf{w}_{t+1}\|_2$ is small because $\|\del_{s}\|_2$ is going to zero.  Lastly, if $\|\w\|_2$ and $\|\del_t\|_2$ are small, then $\dist_{t+1}$ contracts. This completes the proof. 

% 14 arrows

% 1, 7: w eq

% 3, 6: easy, don't include

% 2, 5, 9: easy, probably don't include

% 11: diversity implies unnormalized bad energy contracting, already shown

% 4, 12, 13: delta, messy

% 8, 10, 14: wtis are diverse, already shown












% {\color{red} but empirically the condition number bound is loose, since we only need task diversity over multiple iterations, which can be satisfied with $n=1$. See Appendix A.}

% {\color{red} also Lmax may be loose}





% \textbf{Finite sample cases.} The population case analyses are extended to the finite-sample cases by showing concentration of the following key terms: . Critically, we are able to show dimensionality reduction to reduce $m_{in}$ for the inner loop updates for the heads. However, for MAML the inner loop representation update still requires $\Omega(d)$ samples per task, which makes sense. Another challenge is to show efficient $m_{out}$, which we do by carefully summing the outer loop updates. Require at least $T$ samples per  user, but since we have linear convergence, this is fine. 



% - dimensionality reduction, but for maml we don't have dimensionality reduction


% to do:
% clean up population proofs
% finalize finite sample proofs
% think about negative results
% think about multiiter diversity
% run sims
% try with neural networks: don't use an inner loop, just make heads random each round

% anse either: why is this hard/necessary or why is it useful/important
% takeaway: learned heads need to be diverse. . can we use this in nnns
% should writing focus more on why this result is. important/useful and less on why it is hard?




%one may argue that the true rep is smaller in this case though.







==> Sims_main.tex <==

\section{Numerical simulations} \label{sec:sims}

\begin{figure}[t]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.93\columnwidth]{anilmamldiversity1.pdf}}
\vspace{-3mm}
\caption{\textbf{Task diversity improves convergence rate.} Principal angle distance vs number of iterations for MAML with varying ground-truth head distributions. The larger value of $\mu^2$, the more diverse ground-truth heads.
}
 \label{fig:fig44}
\end{center} 
% \vspace{-3mm}
\end{figure}


\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{anilmamlsims11.pdf}
% anil_fs_min_alpha1.png
}
% \caption{ }
\caption{\textbf{MAML and FO-MAML initialization and ground-truth mean conditions are empirically necessary.}
(Left) Random $\mathbf{B}_0$. (Right) Methodical $\mathbf{B}_0$. In both cases, the mean ground-truth head is far from zero. 
% (Step Size $\alpha = \beta = 0.5$ and averaged over 5 runs)
}
\vspace{-4mm}
\label{fig:sims1}
\end{center}
\end{figure}
% Simulations to verify:
% \begin{itemize}
%     \item MAML (FO and Exact) requires good initialization relative to condition number, and FO-MAML further requires small $\|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast.t,i}\|_2$. ANIL does not have these restrictions, and can learn the representation in situations when MAML cannot.
%     \item Task diversity is necessary to learn the full representation, and better task diversity speeds up the rate of convergence.
%     \item ANIL can choose larger step size than FO-ANIL when there is less task diversity.
%     % \item Inner loop updates are necessary.
%     \item In the finite-sample case, ANIL and MAML can learn the representation with $O(dk)$ total samples, as expected.
% \end{itemize}


% In this section we empirically verify the necessity of the additional assumptions in the MAML and FO-MAML results.
In this section we run numerical simulations to verify our theoretical findings. First, we explore the effect of task diversity on MAML's rate of convergence to the ground-truth representation. In Figure \ref{fig:fig44}, we execute MAML on the task population losses ($m_{in}=m_{out}=\infty$) in the multi-task linear representation learning setting. We set $d\!=\!100$ and $k\!=\!n\!=\!5$. On each round, the ground-truth heads are sampled i.i.d. from $\mathcal{N}(\mathbf{0}, \text{diag}([1,\dots,1, \mu^2]))$, where $\mu^2 <1$. We randomly draw $\mathbf{B}_\ast$ and $\mathbf{B}_0$ at the start of algorithm execution. The parameter $\mu^2$ controls task diversity, with larger $\mu^2$ meaning the ground-truth heads are closer to isotropic and therefore more diverse. The results show that MAML's linear convergence rate improves with greater task diversity, consistent with Theorem \ref{thm:maml_pop_main}.
% % where $\mathbf{\Sigma}_\mu \coloneqq \text{diag}(\mathbf{1}_{k-1}, \mu^2)$

Next, we show that the additional conditions relative to ANIL and FO-ANIL required for MAML and FO-MAML to learn the ground-truth representation are empirically necessary.  That is, (i) MAML and FO-MAML require a good initialization relative to the underlying task diversity, and (ii) FO-MAML further requires  the ground-truth heads to be concentrated around zero.
To test these conditions,  we set $d\!=\!20$, $n\!=\!k=\!3$, randomly draw $\mathbf{B}_\ast$, and use the task population losses. {The ground-truth heads are drawn as $\mathbf{w}_{\ast,t,i}%\stackrel{{iid}}
{\sim} \mathcal{N}(10 \mathbf{1}_k, \mathbf{I}_k)$.}
% and plot $\dist_t$ versus the number of rounds $t$ for each algorithm. 
% {\color{red}This is the same setting as Figure \ref{fig:intro}, except that here, we shift the distribution of the ground-truth heads to have non-zero mean, specifically $\mathbf{w}_{\ast,t,i}%\stackrel{{iid}}
% {\sim} \mathcal{N}(10 \mathbf{1}_k, \mathbf{I}_k)$.} 
Ground-truth task diversity is thus low, since most of the energy points in the direction $\mathbf{1}_k$. In Figure \ref{fig:sims1} (left), we use a random Gaussian initialization of $\mathbf{B}_0$, which has $\dist_0\approx 0.99$. In Figure \ref{fig:sims1} (right), we initialize with a noisy version of $\mathbf{B}_\ast$ satisfying $\dist_0 \in [0.65,0.7]$. The plots show that in this low-diversity setting, MAML requires good initialization to achieve linear convergence, whereas FO-MAML cannot obtain it even with good initialization, as $\|\mathbb{E}[\mathbf{w}_{\ast,t,i}]\|\!\gg\! 0$. {Lastly, note that Figure \ref{fig:intro} employs the same setting as Figure \ref{fig:sims1} (left), except that the mean of the ground-truth heads is zero in the former case, which leads to all four GBML approaches  learning $\col(\mathbf{B}_\ast)$.}
% Yet ANIL and FO-ANIL learn $\col({\mathbf{B}_\ast})$ in both cases. 

%% Please see Appendix \ref{sec:app_sims} for further experimental results and details.
% , including experiments focusing on task diversity and the finite-sample case.

% Compare these results to Figure \ref{fig:intro}, in which the setting is the same except that the distribution of the ground-truth heads is shifted to have mean zero. 

% In Figure \ref{fig:sims2}, 

% Figure \ref{fig:sims1} shows that these conditions are 
% We show that these conditions are empirically necessary in Figure \ref{fig:}. Here, we let $d=10$, $k=3$, and $n=3$. For Figure \ref{fig:}, we 


% Step sizes are tuned appropriately and we average over 5 random trials.


\section{Conclusion}

Our analysis reveals that ANIL, MAML, and their first-order approximations exploit task diversity via inner adaptation steps of the head to recover the ground-truth representation in the multi-task linear representation learning setting. 
Further, task diversity helps these algorithms exhibit an implicit regularization that keeps the learned representation well-conditioned. 
However, the inner adaptation of the representation plays a restrictive role, inhibiting MAML and FO-MAML from achieving global convergence. To the best of our knowledge, these are the first results showing that GBML algorithms can learn a low-dimensional subspace. 

%% These results  provide a basis for future analysis of the role of task diversity in the dynamics of meta-learning algorithms in non-linear settings.

% {\color{red}{Future work remains to determine whether similar behavior occurs in over-parameterized and non-linear models. Likewise, future work should examine whether task diversity is as critical in nonlinear cases as it is in the linear case.}}


==> Simulations.tex <==
\section{Numerical Simulations} \label{sec:app_sims}

% In this section we numerically verify the following observations from our analysis:
% \begin{enumerate}
%     \item ANIL learns the representation with ${O}()$ samples and converges to a neighborhood of size...
%     \item MAML learns the representation at a slower rate with how many samples?
%     \item Standard training (ERM) cannot learn the representation.
% \end{enumerate}

% for maml, need to choose $\alpha$ small enough (cannot choose $\alpha=1$). but, we do not need to downscale the heads.

% {\color{red} Further, we give evidence suggesting that our ideas generalize to more complex models.

% Logistic regression is easy.

% But it would be nice to show for non-linear neural networks. However, we need to determine what a good representation is in that setting. E.g. for ReLU, know the correct column space does not necessarily help.}

% For non-linear neural networks, we need to determine what a good representation is. E.g. for ReLU, knowing the correct column space does not necessarily help.
% simulations on neural nets showing benefit of larger inner learning rate? but this is just hyperparameter tuning. Indeed in other papers the inner lr is larger than the outer lr.




% \begin{figure}[h]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.45\columnwidth]{anil_fs_min_alpha1.png}}
% \vspace{-0mm}
% % \caption{ }
% \caption{Varying $m_{in}$}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}

% \begin{figure}[h]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.45\columnwidth]{anil_fs_mout.png}}
% \vspace{-0mm}
% % \caption{ }
% \caption{Varying $m_{out}$}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}

% \begin{figure}[h]
% \begin{center}
% \vspace{-2mm}
% \centerline{\includegraphics[width=0.45\columnwidth]{anil_fs_n.png}}
% \vspace{-0mm}
% % \caption{ }
% \caption{Varying $n$}
% \label{fig:n}
% \end{center}
% \vspace{-0mm}
% \end{figure}

==> SummaryTechniques.tex <==
\begin{comment}

\subsection{Summary of Techniques} \label{sec:sot}

The key to our analysis is in noticing that the  outer loop updates for the representation can be written as:
\begin{align}
    \mathbf{B}_{t+1}\! &=\! 
    % \mathbf{{B}}_t  - \frac{\beta}{n}\sum_{i=1}^n\nabla_{\mathbf{B}} \mathcal{L}_i(\mathbf{{B}}_t, \mathbf{w}_{t,i}) =  
    \underbrace{\mathbf{{B}}_{t} \Big(  \mathbf{I}_k\! - \!\tfrac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\Big)}_{\text{prior term}}\! +\!  \underbrace{\mathbf{{B}}_\ast\Big(\tfrac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top\Big)}_{\text{signal term}} 
    % - \underbrace{\frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \mathbf{R}(\mathbf{B}_{t,i})}_{\text{regularization}} \
    \label{upd_rep_anil_out_pop}
\end{align}
% where $\mathbf{\Lambda}_{t}\!\coloneqq\!\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$
From \eqref{upd_rep_anil_out_pop}, we can see that if the inner loop updates $\{\mathbf{w}_{t,i}\}_i$ have energy in all directions of $\mathbb{R}^k$, i.e. they are {\em diverse}, then the outer loop update of the representation subtracts energy from $\mathbf{B}_t$ (small prior term) and replaces it with energy from $\mathbf{B}_\ast$ (large signal term). Moreover, the inner loop updates for the head should satisfy that in some sense, $\mathbf{w}_{t,i}$ moves away from $\mathbf{w}_t$ and towards the ground-truth solution for the $i$-th task on round $t$, $\mathbf{w}_{\ast,t,i}$. So, if the $\mathbf{w}_{\ast,t,i}$'s are spread in all directions, then the $\mathbf{w}_{t,i}$'s should also be spread in all directions -- they should be diverse. 
% We show that this is the case after only one gradient step by writing $\mathbf{w}_{t,i}\!=\!(\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t +\alpha \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$, and showing that $\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t$ and $\mathbf{w}_t$ naturally remain close to zero, without any normalization step or regularization.

However, showing sufficient diversity after only one gradient step requires careful upper bounds on the norms of $\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t$ and $\mathbf{w}_t$, since these terms compose the ``non-diverse'' parts of $\mathbf{w}_{t,i}$. Establishing such upper bounds is particularly challenging because these quantities may increase on any given round, and we cannot use regularization or normalization to control them. We overcome this via an intricate multi-way induction that bounds $\|\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t\|_2$ and $\|\mathbf{w}_t\|_2$ while simultaneously showing contraction of the principal angle distance between $\mathbf{B}_t$ and $\mathbf{B}_\ast$. We show this first in the infinite-sample per task case, then show that the dynamics of the finite-sample case are close to the infinite-sample case by sub-Gaussian and sub-exponential concentration results and the dimensionality-reduction provided by $\mathbf{B}_t$ and $\mathbf{B}_\ast$.
\end{comment}


==> hyercontractive.tex <==

\begin{lemma}\label{l4l2}
Suppose $\mathbf{x}$ is drawn from a $C$-L4-L2 hypercontractive distribution on $\mathbb{R}^d$ with covariance $\mathbf{\Sigma}$. Let $\mathbf{v} \in \mathbb{R}^d$, $\mathbf{A}\in \mathbf{R}^{d \times k}$ and $\mathbf{C}\in \mathbf{R}^{d \times d_1}$ be a fixed vector and  fixed matrices, respectively. Then the following relations hold:
\begin{align}
    \|\mathbb{E}[(\mathbf{x}^\top \mathbf{AA}^\top \mathbf{x}) (\mathbf{x}^\top \mathbf{v}) \mathbf{C}^\top\mathbf{x}]\|_2 &\stackrel{\text{(i)}}{\leq} k C^2 \|\mathbf{A}\|_2^2 \|\mathbf{v}\|_2 \|\mathbf{C}\|_2\|\mathbf{\Sigma}\|_2^2   ;\; \|\mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2 \mathbf{C}^\top \mathbf{x}  \mathbf{x}^\top \mathbf{A}] \|_2 \stackrel{\text{(ii)}}{\leq}  C^2  \|\mathbf{\Sigma}\|_2^2\|\mathbf{A}\|_2 \|\mathbf{C}\|_2\|\mathbf{v}\|_2^2 \;\nonumber 
\end{align}
\end{lemma}
\begin{proof}
(i) Fix some $\mathbf{u}\in \mathbb{R}^{d_1}:\|\mathbf{u}\|_2\leq 1$. Using the Cauchy-Schwarz Inequality, we obtain
\begin{align}
    \mathbb{E}[(\mathbf{x}^\top \mathbf{AA}^\top \mathbf{x}) (\mathbf{x}^\top \mathbf{v}) \mathbf{C}^\top\mathbf{x}] &\leq (\mathbb{E}[(\mathbf{x}^\top \mathbf{AA}^\top \mathbf{x})^2] \mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2 (\mathbf{u}^\top\mathbf{C}^\top\mathbf{x})^2] )^{1/2} \label{97}
    % \leq (C^2 k^2\| \mathbf{A}\|_2^4 \|\mathbf{\Sigma}\|_2^2 \mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2 (\mathbf{u}^\top\mathbf{C}^\top\mathbf{x})^2] )^{1/2}
\end{align}
Again applying the Cauchy-Schwarz Inequality, we obtain
\begin{align}
   \mathbb{E}[(\mathbf{x}^\top \mathbf{A} \mathbf{A}^\top \mathbf{x})^2] &= \mathbb{E}[\| \mathbf{A}^\top \mathbf{x}\|_2^4]  =\mathbb{E}\left[\left(\sum_{\ell=1}^k (\mathbf{e}_\ell^\top \mathbf{A}^\top \mathbf{x})^2 \right)^2\right]  = \mathbb{E}\left[\sum_{\ell,\ell'} (\mathbf{e}_{\ell}^\top \mathbf{A}^\top \mathbf{x})^2 (\mathbf{e}_{\ell'}^\top \mathbf{A}^\top \mathbf{x})^2 \right]  \nonumber\\
   &\leq \sum_{\ell,\ell'}\left(\mathbb{E}\left[(\mathbf{e}_\ell^\top \mathbf{A}^\top \mathbf{x})^4 \right]\mathbb{E}\left[ (\mathbf{e}_{\ell'}^\top \mathbf{A}^\top \mathbf{x})^4 \right] \right)^{1/2} \stackrel{\text{(a)}}{\leq} C^2 \sum_{\ell,\ell'}\mathbb{E}\left[(\mathbf{e}_\ell^\top \mathbf{A}^\top \mathbf{x})^2 \right]\mathbb{E}\left[ (\mathbf{e}_{\ell'}^\top \mathbf{A}^\top \mathbf{x})^2 \right] \nonumber \\
   &{\leq} C^2 (\Tr(\mathbf{A}\mathbf{A}^\top\mathbf{\Sigma}))^2 \stackrel{\text{(b)}}{\leq} C^2k^2 \|\mathbf{A}\|_2^4 \|\mathbf{\Sigma}\|_2^2 \label{98}
\end{align}
where (a) follows from $C$-L4-L2 hypercontractivity and (b) follows from the von Neumann trace inequality and the fact that rank$(\mathbf{AA}^\top)\leq k$. 
Similarly,
\begin{align}
    \mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2 (\mathbf{u}^\top\mathbf{C}^\top\mathbf{x})^2]&\leq  (\mathbb{E}[(\mathbf{x}^\top \mathbf{v})^4]\mathbb{E}[ (\mathbf{u}^\top\mathbf{C}^\top\mathbf{x})^4]^{1/2} \leq C^2 \|\mathbf{v}\|_2^2 \|\mathbf{C}\|_2^2\|\mathbf{\Sigma}\|_2^2. \label{99}
\end{align}
% (i) Note that for any $\mathbf{u}_1\in \mathbb{R}^d:\|\mathbf{u}_1\|_2\leq 1$ and $\mathbf{u}_2\in \mathbb{R}^k:\|\mathbf{u}_2\|_2\leq 1$, by the Cauchy-Schwarz Inequality we have
% \begin{align}
%   \mathbb{E}[ (\mathbf{x}^\top \mathbf{A} \mathbf{A}^\top \mathbf{x}) \mathbf{u}_1^\top \mathbf{x} \mathbf{x}^\top \mathbf{A}\mathbf{u}_2] &\leq (\mathbb{E}[ (\mathbf{x}^\top \mathbf{A} \mathbf{A}^\top \mathbf{x})^2] \mathbb{E}[ (\mathbf{u}_1^\top \mathbf{x})^2 (\mathbf{x}^\top \mathbf{A}\mathbf{u}_2)^2]  )^{1/2} \label{97}
% \end{align}
% Again applying Cauchy-Schwarz and $C$-L4-L2 hypercontractivity shows that 
% \begin{align}
%      \mathbb{E}[ (\mathbf{u}_1^\top \mathbf{x})^2 (\mathbf{x}^\top \mathbf{A}\mathbf{u}_2)^2] &\leq  C^2 \mathbb{E}[ (\mathbf{u}_1^\top \mathbf{x})^2] \mathbb{E}[ (\mathbf{x}^\top \mathbf{A}\mathbf{u}_2)^2] \leq C^2  \|\mathbf{\Sigma}\|_2^2 \|\mathbf{A}\|_2^2 
% \end{align}
Combining \eqref{97}, \eqref{98}, and \eqref{99} and maximizing over $\mathbf{u}$ completes the proof.

(ii) Fix some  $\mathbf{u}_1\in \mathbb{R}^{d_1}:\|\mathbf{u}_1\|_2\leq 1$ and $\mathbf{u}_2\in \mathbb{R}^d:\|\mathbf{u}_2\|_2\leq 1$. Using similar calculations as above, we have:
\begin{align}
   \mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2 \mathbf{u}_1^\top\mathbf{C}^\top \mathbf{x}  \mathbf{x}^\top \mathbf{A}\mathbf{u}_2] &\leq (\mathbb{E}[(\mathbf{x}^\top \mathbf{v})^4] (\mathbb{E}[(\mathbf{u}_1^\top\mathbf{C}^\top \mathbf{x})^4]\mathbb{E}[(\mathbf{u}_2^\top\mathbf{A}^\top \mathbf{x})^4])^{1/2})^{1/2}\nonumber \\
   &\leq C^2 \mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2](\mathbb{E}[(\mathbf{u}_1^\top\mathbf{C}^\top \mathbf{x})^2]\mathbb{E}[(\mathbf{u}_2^\top\mathbf{A}^\top \mathbf{x})^2] )^{1/2} 
\end{align}
which implies the result.
% (iii) Fix some $\mathbf{u}_1\in \mathbb{R}^d:\|\mathbf{u}_1\|_2\leq 1$ and $\mathbf{u}_2\in \mathbb{R}^k:\|\mathbf{u}_2\|_2\leq 1$. By similar calculations as above, we obtain
% \begin{align}
%     \mathbb{E}[(\mathbf{x}^\top \mathbf{v})^2  \mathbf{u}_1^\top \mathbf{x}  \mathbf{x}^\top \mathbf{A}\mathbf{u}_2] \leq (\mathbb{E}[(\mathbf{x}^\top \mathbf{v})^4]\mathbb{E}[ (\mathbf{u}_1^\top \mathbf{x})^2  (\mathbf{x}^\top \mathbf{A}\mathbf{u}_2)^2] )^{1/2} \leq (C^2 \|\mathbf{\Sigma}\|_2^2 \|\mathbf{v}\|_2^4 C^2 \|\mathbf{\Sigma}\|_2^2   \|\mathbf{A}\|_2^2] )^{1/2}
% \end{align}
% as desired.
\end{proof}

==> maml_derive.tex <==
\subsection{Derivation of Exact MAML Updates}

The updates for the head are straightforward, noting that $\nabla_{\mathbf{w}} f_{t,i}(\mathbf{B}_t,\mathbf{w}_t) = \mathbf{B}_{t}^\top \mathbf{B}_t$. The inner loop updates for the representation are straightforward. However, computing the Hessian for the outer loop update for the representation involve taking the second derivative of a scalar-valued matrix function, which results in a fourth-order tensor. Specifically,
% First we compute the Hessian of $f_{t,i}(\mathbf{B},\mathbf{w})$ with respect to $\mathbf{B}$.
\begin{align}
\mathbf{B}_{t+1} &= \mathbf{B}_t - \beta \frac{1}{n}\sum_{i=1}^n (\mathbb{I} - \alpha\nabla_\mathbf{B}^2  f_{t,i}(\mathbf{B}_t,\mathbf{w}_t)) \nabla_\mathbf{B} f_{t,i}(\mathbf{B}_{t,i},\mathbf{w}_{t,i})  \nonumber \\
\nabla_\mathbf{B}f_{t,i}(\mathbf{B}_{t,i},\mathbf{w}_{t,i}) &= (\mathbf{B}_{t,i}\mathbf{w}_{t,i}-\mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top =: \mathbf{G}_{t,i}\nonumber \\
\nabla_\mathbf{B}^2f_{t,i}(\mathbf{B}_t,\mathbf{w}_t) &= \nabla_\mathbf{B}(\mathbf{B}_t\mathbf{w}_t\mathbf{w}_t^\top )\nonumber 
% = \mathbb{I}_{d\times k}\otimes \mathbf{w}_t\mathbf{w}_t^\top  
\end{align}
Let $\mathbf{b}_{\ell,t}\in \mathbb{R}^{k}$ be the $\ell$-th row of $\mathbf{B}_t$. Let $\mathbf{\Tilde{b}}_t = \begin{bmatrix}\mathbf{b}_{1,t}\\
\vdots\\
\mathbf{b}_{d,t} \\
\end{bmatrix}\in\mathbb{R}^{dk}$ be the vectorization of $\mathbf{B}_t$ that stacks the rows of $\mathbf{B}_t$ vertically.  Similarly, let $\mathbf{q}_{\ell,t}\in \mathbb{R}^{k}$ be the $\ell$-th row of the matrix $\mathbf{Q}_{t}\coloneqq \mathbf{B}_t \mathbf{w}_t\mathbf{w}_t^\top$, and let $\mathbf{\Tilde{q}}_t = \begin{bmatrix}\mathbf{q}_{1,t}\\
\vdots\\
\mathbf{q}_{d,t} \\
\end{bmatrix}\in\mathbb{R}^{dk}$ be the vectorization of $\mathbf{Q}_t$ that stacks the rows of $\mathbf{Q}_t$ vertically. 
Note that  $\mathbf{\Tilde{q}}_t = \begin{bmatrix}\mathbf{w}_t\mathbf{w}_t^\top \mathbf{b}_{1,t} \\
\vdots\\
\mathbf{w}_t\mathbf{w}_t^\top \mathbf{b}_{d,t} \\
\end{bmatrix}= (\mathbf{I}_d\otimes \mathbf{w}_t\mathbf{w}_t^\top)\mathbf{\Tilde{b}}_{t}$, where $(\mathbf{I}_d\otimes \mathbf{w}_t\mathbf{w}_t^\top)\in\mathbb{R}^{dk\times dk}$ is the tensor product of $\mathbf{I}_d$ and $\mathbf{w}_t\mathbf{w}_t^\top$. Now it is easy to see that $\nabla^2_{\mathbf{\Tilde{b}}_t}(\mathbf{\Tilde{q}}_t) = \mathbf{I}_d\otimes \mathbf{w}_t\mathbf{w}_t^\top$. To utilize this, we can write the outer loop update in vectorized form:

\begin{align}
    \mathbf{\Tilde{b}}_{t+1}&=  \mathbf{\Tilde{b}}_{t} - \beta \frac{1}{n}\sum_{i=1}^n(\mathbf{I}_{dk} - \alpha \mathbf{I}_d\otimes \mathbf{w}_t\mathbf{w}_t^\top)\mathbf{\Tilde{g}}_{t,i} \nonumber \\
    &= \mathbf{\Tilde{b}}_{t} - \beta \frac{1}{n}\sum_{i=1}^n \begin{bmatrix}
   ( \mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top)\mathbf{{g}}_{1,t,i} \\
   \vdots \\
   ( \mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top)\mathbf{{g}}_{d,t,i} \\
    \end{bmatrix}
\end{align}
Transferring this back into matrix form yields
\begin{align}
    \mathbf{B}_{t+1}&= \mathbf{B}_t - \beta\frac{1}{n} \sum_{i=1} \mathbf{G}_{t,i}( \mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top) \nonumber \\
    &=  \mathbf{B}_t - \beta\frac{1}{n} \sum_{i=1} (\mathbf{B}_{t,i}\mathbf{w}_{t,i}-\mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top ( \mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top)
\end{align}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\simiid}{\overset{\text{i.i.d.}}{\sim}}
\def\dist{\operatorname{dist}}

==> negative.tex <==

% observations from experiments:
% w_t converges too fast to kill all of zt. note that for optimal wt and fixed average, grad w is proportional to dist +. tau_2
\subsection{Negative results} Here we show that task diversity and inner loop updates are necessary to learn the true representation.

% {\color{red} empirically, diversity over multiple iterations is sufficient to learn the representation at a linear rate; we do not need task diversity on each round. It should be possible to extend proofs to this case...}
% \begin{rem}[Task diversity is necessary.] If the ground-truth heads across all iterations are not diverse, neither ANIL nor MAML learn the rep. Easy to show via simple counterarg with $\mathbf{B}_\ast, \mathbf{B}_\ast'$.  But, mention gap in analysis in the sense that diversity across iters is sufficient (as long as there is inner loop for the head) but we require diversity in each round.
% \end{rem}


% But this is a special case of general learning theory result in Tripuraneni paper. Also mention gap in analysis in the sense that diversity across iters is sufficient (as long as there is inner loop for the head) but we require diversity in each round.

\begin{rem}[ANIL/MAML without an inner loop cannot learn the representation.]
% Intuitively, this is because $\mathbf{w}_t$ does not kill enough of the bad directions in $\mathbf{B}_t$. 
Empirically, this happens because $\mathbf{w}_t$ converges before it kills all the bad directions. 
{\color{red} hard to prove.}
\end{rem}



% Note that removing the inner loop updates altogether corresponds to minimizing the standard average loss over tasks: $\min_{\mathbf{B,w}}\{\tfrac{1}{2}\mathbb{E}_{\mathbf{w}_{\ast,i}}\mathbb{E}_{\mathbf{x}_i,y_i}[(\mathbf{x}_i^\top \mathbf{B}\mathbf{w} - y_i)^2] \equiv \tfrac{1}{2}\mathbb{E}_{\mathbf{w}_{\ast,i}}[\|\mathbf{B}\mathbf{w} - \mathbf{B}_\ast \mathbf{w}_{\ast,i}\|_2^2]  \}$. but there may be an implicit regularization in the alg that causes it to find the right soln... 
% As pointed out by \cite{collins}, solving this problem does not guarantee that the 
% We now show that task diversity is not only sufficient but also necessary to learn $\text{col}(\mathbf{B}_\ast)$.
% Suppose that 

Idea: $\mathbf{B}_0$ has large energy in a bad direction which is not killed by $\mathbf{w}_0$. Show that $\mathbf{w}_t$ never kills this bad energy.  -- but $\mathbf{w}_t$ eventually will not be orthogonal to this direction.

Idea: show that in simple case, different initialization $\mathbf{B}_0$ leads to different column space of $\mathbf{B}_T$.


Idea: The algorithm is SGD on the objective: $\min_{\mathbf{B},\mathbf{w}}\mathbb{E}_{\mathbf{w}_\ast}[\|\mathbf{Bw}-\mathbf{B}_\ast \mathbf{w}_\ast\|^2] = \mathbf{w}^\top \mathbf{B}^\top \mathbf{Bw} - 2\mathbf{w}^\top \mathbf{B}^\top\mathbf{B}_\ast \mathbf{\bar{w}}_\ast + c$. But this objective is nonconvex so we don't know how to characterize the fixed point SGD reaches.

The following lemma shows the necessity of the inner loop updates for the head.
\begin{lemma}

\end{lemma}

\begin{proof}
Suppose that for some $\mathbf{B}_\ast \in \mathcal{O}^{d \times k}$ and ground-truth head distribution $\nu$, when FO-ANIL is run on the environment $(\mathbf{B}_\ast, \nu)$, there is an iteration $T$ such that for all $t\geq T$, $\dist(\mathbf{B}_t,\mathbf{B}_\ast) \leq \epsilon$. 

Let $\mathbf{\bar{w}}_{\ast,t}\coloneqq \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}$ for all $t$.
Note that the outer-loop updates in this case can be written as:
\begin{align}
    \mathbf{w}_{t+1} &\gets \mathbf{w}_t \!- \! \beta (\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t - \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}) \nonumber \\
    \mathbf{B}_{t+1} &\gets \mathbf{B}_t \!- \! \beta (\mathbf{B}_t \mathbf{w}_t \mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t} \mathbf{w}_t^\top) \nonumber 
\end{align}
empirically: ANIL fails in this case because there is no inner loop. if there is an inner loop and $n=1$ but there is diversity across iterations, then ANIL still works. 

case 1: $\mathbf{\bar{w}}_{\ast,t}$ do not span $\mathbb{R}^k$: easy because the updates would be identical to another instance with $\mathbf{B}_{\ast}'$, $\col(\mathbf{B}_\ast')\neq \col(\mathbf{B}_\ast)$. Note that this case holds if $n=\infty$.

case 2: they do span $\mathbb{R}^k$: then can we show instability? no... this is the hard part
\end{proof}

If no proof: make remark that says that representation learning is provably not possible with no inner loop when ${\mathbf{\bar{w}}_{\ast,t}}_t$, which happens for instance when $n=\infty$, and cite simulations to show that it doesn't happen even when ${\mathbf{\bar{w}}_{\ast,t}}_t$ is diverse.

==> notes.tex <==
notes from Saunshi paper:

they only use the population loss (full measurements) for meta-learning analysis

differences in analysis:
they assume B is d by d, and show that it learns a rank 1 matrix (here, k=1)
they us gradient plow for RepLearn and reptile
they used trajectory-based analysis. initialization is critical.

potential hope:
maml doesn't require special initialization, and doesn't require gradient flow.
- we have this result as long as we can orthogonalize the rep.
- but it still requires large batch size... (as do the algs in saunshi)
- i think the initialization only matters in overparameterized case. If A is d by k, their counterexample fails.
- is the exactly parameterized case interesting?

todo: read Gidel and Saxe papers.

gidel discrete dynamics should show the difficulties in this type of analysis

does loss is reptile minimizing? does such a bad minimizer exist for it? cannot show -- too hard

it is not clear that if you are only trying to find a single head, then you might find a bad representation, even in the overparameterized case.

We






Can we actually orthogonalize Bt? 
in the full measurements case yes, i think so - since the column space of [hat(B)t Rt, B*] Z is equal to the column space of [hat(B)t, B*] Z'... as long as Z1, Z2, Z'1, Z'2 are all full rank...
but with partial measurements, no....



is this critical to the analysis? without orthogonalization, we have another Rt, and P and S are messier, but i think it is not critical

with partial measurements, even getting the starting dist is hard...

What about including second order? 

- does not help

to do: -solidify full measurements case without ortho

- then add second order

- then add maml?

- then add partial measurements, with first order anil

maybe make assumption that inner loop head is within some epsilon ball of optimal soln. then can we make ortho assumption? i don't think so, but other analysis will be easier.

% Consider
% \begin{align}
%     \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
%     &= \left( \mathbf{B}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right)\right)^\top \left( \mathbf{B}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right)\right) \nonumber \\
%     &= 
%     \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)\left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)  
%     +
%     \left(\frac{\beta}{n} \sum_{i=1}^n    \mathbf{w}_{t,i} \mathbf{w}_{i,\ast}^\top\right) \left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right) \nonumber \\
%     &\quad \quad +
%     \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)\mathbf{B}_t^\top \mathbf{B}_\ast \left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right) 
%     +
%     \left(\frac{\beta}{n} \sum_{i=1}^n  \mathbf{w}_{t,i} \mathbf{w}_{i,\ast}^\top\right) \mathbf{B}_\ast^\top \mathbf{B}_t\left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right)  
%     \nonumber 
% \end{align}
% Let $\mathbf{A}_1 = \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$, $\mathbf{A}_2 = \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top$. Then
% \begin{align}
%     \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} 
%     &= 
%     \left(\mathbf{I}_d - \mathbf{A}_1\right)\left(\mathbf{I}_d - \mathbf{A}_1\right)  
%     +
%     \mathbf{A}_2^\top \mathbf{A}_2 +
%     \left(  \mathbf{I}_d - \mathbf{A}_1\right)\mathbf{B}_t^\top \mathbf{B}_\ast \left(\mathbf{A}_2\right) 
%     +
%     \mathbf{A}_2^\top \mathbf{B}_\ast^\top \mathbf{B}_t\left(  \mathbf{I}_d -  \mathbf{A}_1\right)  
%     \nonumber \\
%     &= \mathbf{I}_d - 2\mathbf{A}_1  + \mathbf{A}_1^\top \mathbf{A}_1
%     +
%     \mathbf{A}_2^\top \mathbf{A}_2 + \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2 -
%      \mathbf{A}_1\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2 
%     +
%     \mathbf{A}_2^\top \mathbf{B}_\ast^\top \mathbf{B}_t -  \mathbf{A}_2^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{A}_1
% \end{align}
% Note that  can be written as
% \begin{align}
%     h
% \end{align}


% -------------

% By Weyl's Inequality, we have, for small enough $\beta$,
% \begin{align}
%     \lambda_{\min}(\mathbf{R}_{t+1}^\top \mathbf{R}_{t+1}) &= \lambda_{\min}(\mathbf{I}_d - 2\mathbf{A}_1  + \mathbf{A}_1^\top \mathbf{A}_1
%     +
%     \mathbf{A}_2^\top \mathbf{A}_2 + \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2 -
%      \mathbf{A}_1\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2 
%     +
%     \mathbf{A}_2^\top \mathbf{B}_\ast^\top \mathbf{B}_t -  \mathbf{A}_2^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{A}_1)\nonumber \\
%     &\geq 1 - 2\lambda_{\max}(\mathbf{A}_1) + \lambda_{\min}(\mathbf{A}_1^\top \mathbf{A}_1) + 2\lambda_{\min} (\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2) - 2 \lambda_{\max} (\mathbf{A}_1\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2) \nonumber \\
%     &\geq  1 - 2\beta + \lambda_{\min}(\mathbf{A}_1^\top \mathbf{A}_1) + 2\lambda_{\min} (\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2) - 2 \beta^2 \label{up_max} \\
%     &\geq  1 - 2\beta + \lambda_{\min}(\mathbf{A}_1^\top \mathbf{A}_1) - 2\beta - 2 \beta^2
% \end{align}
% where \eqref{up_max} follows since $\lambda_{\max} (\mathbf{A}_1\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{A}_2) \leq \|\mathbf{A}_1\|_2 \| \mathbf{B}_t^\top \mathbf{B}_\ast \|_2 \| \mathbf{A}_2 \|_2$.
% Also, we have $\|\mathbf{A}_1\|_2 \leq \beta \max_{i\in n} \|\mathbf{w}_{t,i}\|_2^2$. 
% Further, $$
% \|\mathbf{w}_{t,i}\|_2 = \|\mathbf{P}_{t,i} \mathbf{w}_t + \alpha \mathbf{S}_{t,\ast,i}\mathbf{w}_{\ast,i}\|_2 = \|(1-\alpha)\mathbf{w}_t + \alpha \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,i}\|_2 \leq (1-\alpha)\|\mathbf{w}_t\|_2 + \alpha \|\mathbf{w}_{\ast,i}\|_2 \leq 1-\alpha + \alpha = 1,
% $$
% thus $\|\mathbf{A}_1\|_2 \leq \beta$.
% % (1-ax)2 < 1 - bx
% % 1 - 2ax + a2 x2 < 1 - bx
% % a2 x < 2a-b
% % x < (2a-b)/a2 
% % --> beta < (2a-b)/a2
% % but we might have a << b...
% We have already shown that $\lambda_{\min}(\mathbf{A}_1) \geq \beta \alpha^2 E_0 \mu/k - 2 \beta \alpha (1-\alpha)$. Let $\alpha =1$, then we have $\lambda_{\min}(\mathbf{A}_1^\top \mathbf{A}_1) \geq \beta^2  E_0^2 \mu^2/k^2 := \nu^2 \beta^2$. Therefore, we have
% \begin{align}
%     \sigma_{\min}^2(R_{t+1}) \geq 1- 4 \beta - (2 - \nu^2) \beta^2
% \end{align}
% Putting everything together, we have
% \begin{align}
%     \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) \frac{1 - \nu \beta}{\sqrt{1 - 4\beta - (2-\nu^2)\beta^2}}
% \end{align}
% We thus require $1 - 2 \nu \beta + \nu^2 \beta^2 <  1 - 4\beta - (2-\nu^2)\beta^2 \longleftrightarrow (2+\nu^2) \beta <  2\nu - 4$ so we need $\nu > 2$ --> need $\sigma$

% {\color{red} the above is wrong for R, we do get contraction, see below, since this case is exactly equal to fed rep with full measurements... }





{\color{blue} 
\subsection{MAML vs ERM}

What we expect:
\begin{itemize}
    \item The gain for MAML over ERM will be largest in settings with heterogenous easy tasks and homogenous hard tasks. Example: cifar10 with 5 classes/user (hard), cifar 100 with 2 classes/user (easy)
    \item the standard settings: cifar10 2 classes/user is easy and heterogeneous, so MAML and ERM should do about the same. cifar10 5 classes/user is hard and homoogeneous, so MAML and ERM should do about the same.
\end{itemize}

\begin{table}[H]
\caption{CIFAR10 and CIFAR100 (separately). $T=100$ unless otherwise noted. Learning rate and batch size parameters are tuned.}
\vspace{-2mm}
\label{table:data}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Setting & FedAvg+FT ($\sim$ERM) &  PerFedAvg ($\sim$MAML) \\
\midrule
C10, $S=2, n=100, r=0.1$,  WD & 91.26 &  91.44 \\
C10, $S=5, n=100, r=0.1$,  WD & 81.98 & 82.19 \\
\midrule
% C100, $S=5, n=100, r=0.1$, conv, WD & 80.60 & 71.43  \\
C100, $S=20, n=100, r=0.1$, conv, WD & 56.12 &  51.37  \\
C100, $S=50, n=100, r=0.1$, conv, WD & 42.18 &  37.09  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\begin{table}[H]
\caption{CIFAR10 and CIFAR100 combined: 100 users with 5 classes from CIFAR10, and 100 users with 5 classes from CIFAR100. The 100 users from CIFAR10 are homogeneous and hard. The 100 users from CIFAR100 are heterogeneous and ... also hard.}
\vspace{-2mm}
\label{table:data}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Algorithm & CIFAR10 Acc. &  CIFAR100 Acc. \\
\midrule
FedAvg+FT ($\sim$ERM) & 50.32  &  6.00\\
PerFedAvg ($\sim$MAML) & 51.75  & 2.59  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
}

With 10 classes/user for CIFAR10 and 2 classes/user for CIFAR100, both algorithms do extremely poorly on CIFAR100.

Need to make CIFAR100 homogeneous and hard (i.e. 50+ classes/user) and CIFAR10 heterogeneous and easy (2 classes/user)

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.48\columnwidth]{relu_erm.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.48\columnwidth]{relu_maml.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.42\columnwidth]{relu_erm_eh.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.42\columnwidth]{relu_maml_eh_1step.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.42\columnwidth]{relu_maml_eh_2steps.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.48\columnwidth]{sigmoid_erm_eh.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.48\columnwidth]{sigmoid_maml_eh_1step.png}}
\vspace{-0mm}
\caption{}
\label{fig:n}
\end{center}
\vspace{-0mm}
\end{figure}






\textbf{Two-task, one-layer, one neuron NN case}
Let $d=1, b_{1,\ast} = 1, b_{2,\ast} = 1$.

Let $f_1(b) = \mathbb{E}_{x_1 \sim p_1}[(\sigma(bx_1) - \sigma(x_1))^2]$ and $f_2(b) = \mathbb{E}_{x_2 \sim p_2}[(\sigma(bx_2) - \sigma(-x_2))^2]$. Let $f(b) = f_1(b) + f_2(b)$. 

% When $p_1$ and $p_2$ are mean zero and symmetric and $\sigma$ is the ReLU activation, the landscape of $f$ is given in the figure. However the global min of $\sum_i f_i(b - \eta \nabla f_i(b))$ should be at zero.

It can be shown that the hardness of each task $i$ depends on the variance of $p_i$.

% to do on omni:
% reduce dataset size
% make network have many nodes in the last layer
% do not shuffle labels
% put all of data in outer loop, take inner step size to zero
% how are we evaluating?
% alternately: keep shuffling and last layer small. but make sure evaluation is the same
% first though take care of cifar

%maml 5shards/user is last saved, ends w 450.
% need to make fed tune for 1 iter, same batch size
% need.a fmwrk..

% Conjecture: In deep learning settings, MAML learns a representation that is ``close'' to local minima of the tasks for 

\begin{table}[H]
\caption{CIFAR10.}
\vspace{-2mm}
\label{table:data}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Alg  & CIFAR10 $S=2$ pre & CIFAR10 $S=2$ post &  CIFAR100 $S=5$ pre & CIFAR100 $S=5$ post   \\
\midrule
ERM & 51.40  & 54.56 &  59.96 & 61.73 \\
MAML & 50.41 & 72.10  & 58.56 & 68.82 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{CIFAR10 $S=8$ (hard and homogeneous),  CIFAR100 $S=2$ (easy and heterogeneous).}
\vspace{-2mm}
\label{table:data}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Algorithm  & CIFAR10 Pre & CIFAR10 Post  & CIFAR100 Pre & CIFAR100 Post\\
\midrule
ERM & 15.60  & 21.78 & 20.54 & 50.81 \\
MAML & 12.39& 22.04 & 17.67 & 50.51  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{Note: a critical reason why MAML $>>$ ERM for few-shot learning is that in few-shot learning experiments, the class labels are typically shuffled. So, there is no model $w$ that can perform well on $f(w) = \sum_{i=1}^n f_i(w)$ (since performing well on $f_1(w)$ may imply poor performance on $f_2(w)$, if both tasks involve the same classes but with permuted labels, i.e. the tasks are { mutually exclusive}). Here we test  on non-mutually exclusive tasks sampled from one language from Omniglot. The output layer of the network now contains the number of neurons equal to the total number of classes (42) as opposed to the number of classes in each task (5) so each neuron corresponds to a particular task. Both MAML and ERM perform well in this case. \\
$\rightarrow$ From the good performance of MAML on mutually exclusive tasks, we conjecture that  MAML can learn a representation that makes mutually exclusive tasks close together, whereas ERM does not. How to connect this with main arguments? MAML learns an advantageous landscape for itself? (now that we know what an advantageous landscape is)}
\vspace{-2mm}
\label{table:data}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Algorithm & Acc Post, 500 iters  \\
\midrule
ERM &  97.7    \\
MAML &  98.5      \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


Prescription: Re-sample the hard tasks and/or weight the hard task losses heavier while running ERM and MAML. 

Motivation: We have seen that the key advantage of MAML over ERM is that it can perform better on the hard tasks by initializing closer to them and ignoring the easy tasks. So, we need to make sure it accesses hard tasks during training. For ERM, we can improve its performance by encouraging it to initialize close to the hard tasks. This may be a simple way to improve the performance of FedAvg.

However, this has already been tried for MAML: \url{https://arxiv.org/pdf/2007.06240.pdf}, \url{https://arxiv.org/pdf/1910.03648.pdf}. 

One of the above papers proposes to re-sample the hard classes, which is not really what we want. The other paper proposes to sample easy tasks first, then hard tasks later. We could show that the first stage (easy tasks) is unnecessary.

% plan: run mutually exclusive hard-easy: show erm chooses easy while maml chooses hard. (need to measure pre-update acc. too)
% 



----

\begin{enumerate}
    \item Run MAML.
    \begin{enumerate}
        \item On each iteration,  measure the change incurred in both the representation and the last layer on the inner loop for each task.
        \item If the change is small for the representation for all tasks, then the representation has reached a point that performs well on all tasks, so you should switch to ERM.
        \item ... reduces to early stopping
    \end{enumerate}
\end{enumerate}

% Figures:
% - MAML and ERM do similarly for NME easy tasks, and for NME hard tasks that are similar
% - otherwise MAML does better: NME tasks that are easy and hard, with hards close together
% - the performance of MAML can be further improved by resampling hard tasks




{\color{red} simple upper bound on $z_t$:  $z_t \leq \bar{z}_t \coloneqq  \gamma^{t+1} \frac{\alpha^{1.5}\beta^2}{\gamma - \rho^2}$ fix: really $\gamma^{t}\rho^2 \frac{\alpha^{1.5}\beta^2}{\gamma - \rho^2}$ . So we can see that $\bar{z}_t$ is a geometric series (**but the distance is not exactly linearly decreasing, ignore this for now). 

Now,
\begin{align}
    a_{t+1} &\leq (1 + \tfrac{\beta}{\alpha} \bar{z}_t)a_t + \tfrac{\beta}{\sqrt{\alpha}} \bar{z}_t c \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{\beta}{\alpha}\bar{z}_s) +\tfrac{\beta}{\sqrt{\alpha}} c\sum_{s=1}^t \bar{z}_s\prod_{r=s+1}^t(1+ \tfrac{\beta}{\alpha}\bar{z}_r) \nonumber \\
    &=  \tfrac{\beta}{\sqrt{\alpha}} c\sum_{s=1}^t \bar{z}_s\prod_{r=s+1}^t(1+ \tfrac{\beta}{\alpha}\bar{z}_r) \nonumber \\
    &= \tfrac{\beta}{\sqrt{\alpha}} c\sum_{s=1}^t \gamma^{s+1} \tfrac{\alpha^{1.5}\beta^2}{\gamma - \rho^2}\prod_{r=s+1}^t(1+ \gamma^{r+1} \tfrac{\alpha\beta^3}{\gamma - \rho^2}) \nonumber \\
    &= \tfrac{\alpha\beta^3}{\gamma - \rho^2} c\sum_{s=1}^t \gamma^{s+1} \prod_{r=s+1}^t(1+ \gamma^{r+1} \tfrac{\alpha\beta^3}{\gamma - \rho^2}) \nonumber
\end{align}    
where the first equality follows under the assumption that $a_0 = 0$. By the AM-GM inequality, we have
\begin{align}
    \prod_{r=s+1}^t(1+ \gamma^{r+1} \tfrac{\alpha\beta^3}{\gamma - \rho^2}) &\leq \left(1 + \tfrac{1}{t-s+1} \sum_{r=s+1}^t \gamma^{r+1} \tfrac{\alpha\beta^3}{\gamma - \rho^2}\right)^{t-s+1} \nonumber \\
    &\leq \left(1 + \tfrac{1}{t-s+1} \tfrac{\alpha\beta^3}{\gamma - \rho^2}\tfrac{\gamma^{s+1}}{1- \gamma} \right)^{t-s+1} 
\end{align}
The RHS is monotonically increasing in $t$ (since each additional $t$ means multiplication by a number greater than 1) so we can upper bound it by its limit as $t \rightarrow \infty$. If $s=1$, this limit is $\exp\left( \tfrac{\alpha\beta^3}{\gamma - \rho^2}\tfrac{\gamma^{2}}{1- \gamma}\right) $, where the exponent is less than 1 for sufficiently small $\alpha, \beta$. For general $s$, the RHS limit is $\exp\left( \tfrac{\alpha\beta^3}{\gamma - \rho^2}\tfrac{\gamma^{s+1}}{1- \gamma}\right) $. So we have
\begin{align}
    a_{t+1} &\leq \tfrac{\alpha\beta^3}{\gamma - \rho^2} c\sum_{s=1}^t \gamma^{s+1} \exp\left( \tfrac{\alpha\beta^3}{\gamma - \rho^2}\tfrac{\gamma^{s+1}}{1- \gamma}\right) \nonumber \\
    &\leq \tfrac{\alpha\beta^3}{\gamma - \rho^2} c \exp\left( \tfrac{\alpha\beta^3}{\gamma - \rho^2}\tfrac{\gamma^{2}}{1- \gamma}\right)\sum_{s=1}^t \gamma^{s+1}  \nonumber \\
    &\leq \tfrac{\alpha\beta^3}{\gamma - \rho^2} c \exp\left( \tfrac{\alpha\beta^3}{\gamma - \rho^2}\tfrac{\gamma^{2}}{1- \gamma}\right)\tfrac{\gamma^2}{1-\gamma} 
\end{align}   
so we must choose $\alpha \beta^3 \leq {(\gamma-\rho^2)(1-\gamma)}$. It remains to account for the fact that dist is not exactly linearly decreasing.







test whether norm grows with k
}




Even if we assume $\sum_{i=1}^n  \mathbf{w}_{\ast,t,i} = 0$, $\|\mathbf{w}_t\|$ may still grow, because $\mathbf{I}- \alpha\mathbf{B}_t^\top \mathbf{B}_t$ is not positive definite. numerically, $\mathbf{I}- \alpha\mathbf{B}_t^\top \mathbf{B}_t$ may indeed have negative eigenvalues

so  $\|\mathbf{w}_t\|$ may grow by $ \tau$ on each iteration. this is too much
% if we choose $\tau = 1/T$, this forces $B = O(1/T)$, no good

indeed, experimentally, the max spectral norm that the coef of $w_t$ reaches is $1+\tau$. Most of the time it is much less than this, but this would be difficult to prove.

% need to show that if norm(w) > tau
we know that if $t1$ is like $1+\tau$ and $t2$ is small, but not necessarily negative

problem is first term is $1+\tau$. second term doesn't matter.

we can't even say that the gradient is non-increasing:
\begin{align}
    \mathbf{B}_t \mathbf{w}_{t+1} - \frac{1}{n}\sum_{i=1}^n \mathbf{B}_\ast \mathbf{w}_{\ast,i} &= (\mathbf{I}_k - \beta \mathbf{B}_t (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{B}_t^\top )\left(\mathbf{B}_t \mathbf{w}_{t} - \frac{1}{n}\sum_{i=1}^n \mathbf{B}_\ast \mathbf{w}_{\ast,i}  \right)
\end{align}
thus it may increase...

Tried using $\|\mathbf{I}_k - \mathbf{B}^{\top}\mathbf{B}\|_F^2$ as the regularization, since then we would have PSD, but this does not work in simulation, even with mean zero $\mathbf{w}_{\ast,i}$ (e.g. for MAML finite samples)

Looked at product, but it is no help

% In pop. case for ANIL, we can show that $\|\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2$ converges to a neighborhood of size $\alpha^{2}\beta^2$. But empirically, it gets much smaller. Is $\alpha^2 \beta^2$ small enough

We can show that $\|\mathbf{I}_k - \alpha\mathbf{B}_t^{\top}\mathbf{B}_t\|_2$ is almost linearly decreasing, in the sense that $\|\mathbf{I}_k - \alpha\mathbf{B}_{t+1}^{\top}\mathbf{B}_{t+1}\|_2 \leq (1- \rho)\|\mathbf{I}_k - \alpha\mathbf{B}_{t}^{\top}\mathbf{B}_{t}\|_2 + \alpha^{1.5}\beta^2 r_t^2 \dist^2(\mathbf{B}_t, \mathbf{B}_\ast)$. This brings us close to the experimental results but it still doesn't help to bound norm(w).




Let $\mathbf{C}_t \coloneqq \mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha\mathbf{B}_t^\top \mathbf{B}_t) \mathbf{B}_t^\top \mathbf{B}_t$, and note that all $\|\mathbf{C}_t\|_2 \leq 1+\beta \tau \frac{1+\tau}{\alpha}$ for all $t \in [T]$ by inductive hypothesis 2. Assume $\left\|\mathbf{B}_t \mathbf{\hat{B}}_\ast \frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i,n}\right\|_2 \leq c$.
Since we initialize $\mathbf{w}_0 = \mathbf{0}_k$, we have
\begin{align}
   \| \mathbf{w}_{t+1}\|_2 &\leq c\left\|\sum_{t=1}^T \left(\prod_{t'=1}^t\mathbf{C}_{t'}\right)\right\|_2
\end{align}

% Now, with probability at least , $\left\| \mathbf{\bar{w}}_{\ast} - \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\right\|_2 \leq \delta$








Now,% letting $\alpha = \Theta(\beta)$, 
\begin{align}
    a_{t+1} &\leq (1 + \tfrac{\beta}{\alpha} z_t)a_t + \tfrac{\beta}{\sqrt{\alpha}} z_t c \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{\beta}{\alpha}z_s) +\tfrac{\beta}{\sqrt{\alpha}} c\sum_{s=1}^t z_s\prod_{r=s+1}^t(1+ \tfrac{\beta}{\alpha}z_r) \nonumber \\
    &=  \tfrac{\beta}{\sqrt{\alpha}} c\sum_{s=1}^t z_s\prod_{r=s+1}^t(1+ \tfrac{\beta}{\alpha}z_r)
\end{align}    
where the last equality follows under the assumption that $a_0 = 0$. 

% But for reasonable $\rho, \gamma$ (optimistic estimate: $\rho, \gamma = 0.9$), this upper bound blows up with $t$, reaches $10^{18}$.


Other ideas: we could use randomness of the ground-truth heads and anti-concentration results to show that the negative gradient sometimes points towards the origin. but this is difficult to show because $\mathbf{I}_k - \alpha\mathbf{B}_t^{\top}\mathbf{B}_t$ may always rotate the vector in the same direction. also, empirically we do not need randomness, and this argument would require an upper bound on $n$, which is inconsistent with the message of the paper.

If we are in convex hull do we stay in convex hull? not necessarily because norm may increase, and the matrix $ \mathbf{I}- \alpha \mathbf{B}_t^\top \mathbf{B}_t$ may do something strange with direction.

Suppose $\|\mathbf{w}_t\|_2 \geq C \|\mathbb{E}[\mathbf{w}_\ast]\|_2$ for some large $C$. Is this a contradiction?



\begin{lemma}
contraction of $\tau_1$ and $\tau_2$
\end{lemma}

\begin{proof}
Let $a_t \coloneqq \|\mathbf{w}_t\|_2$ and $b_t \coloneqq \|\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2$ for all $t$. Let $\dist_t \leq (1-\delta_3)^t$. 

We have

\begin{align}
    a_{t+1} &\leq (1-\delta_1)a_t + \beta \sqrt{\alpha}\eta b_t \nonumber \\
    &\leq \sum_{s=1}^t (1-\delta_1)^{t-s}\beta \sqrt{\alpha}\eta b_s \nonumber \\
    b_{t+1} &\leq (1-\delta_2)b_t + \epsilon_1 a_t + \epsilon_3 \dist_t^2 \nonumber \\
    &\leq \sum_{s=1}^t (1-\delta_2)^{t-s}(\epsilon_1 a_s + \epsilon_3 \dist_s^2) \nonumber \\
    &\leq \sum_{s=1}^t (1-\delta_2)^{t-s}(\epsilon_1 a_s + \epsilon_3 (1-\delta_3)^{2s}) \nonumber \\
\end{align}

inductive hypothesis: 
\begin{align}
    b_{t+1} &\leq \sum_{s=1}^t (1-\delta_2)^{t-s} b_s + \epsilon_3 (1-\delta_3)^{2t} \nonumber \\
    &\leq \sum_{s=1}^t (1-\delta_2)^{t-s} \sum_{r=1}^{s-1}\left( (1-\delta_2)^{s-1-r} b_r + \epsilon_3 (1-\delta_3)^{2s}\right) + \epsilon_3 (1-\delta_3)^{2t} 
    % &\leq (1-\delta_2) \sum_{s=1}^{t-1} (1-\delta_2)^{t-1-s} b_s + (1-\delta_2)\epsilon_3 \dist_{t-1}^2  + b_t
\end{align}
you're getting a little bit less of bt plus a small distance plus a decayed version of the previous bs.

if delta2 bt is larger than the rest we have decreasing, but we already knew this,

how can we improve the rates?

simulate this

note that if we upper bound bs by 1, we have easy bounds

try this: assume bt leq f(alpha), does it stay leq f(alpha)?

but this is not tighter than previous case


b4 leq 1 b3 + 2 b2 + 3 b1 leq 2 b2 + 3 b1 + 3 b1 + 3 b1

\begin{align}
    &b_{t+1} \nonumber \\
    &\leq \sum_{s=1}^t (1-\delta_2)^{t-s} b_s + \epsilon_3 (1-\delta_3)^{2t} \nonumber \\
    &\leq \epsilon_3 (1-\delta_3)^{2t} + \sum_{s=1}^t (1-\delta_2)^{t-s} \sum_{r=1}^{s-1}\left( (1-\delta_2)^{s-1-r} b_r + \epsilon_3 (1-\delta_3)^{2s}\right) \nonumber \\
    &\leq \epsilon_3 (1-\delta_3)^{2t} + \sum_{s=1}^t (1-\delta_2)^{t-s} \epsilon_3 (1-\delta_3)^{2s}  \nonumber \\
    &\leq \epsilon_3 (1-\delta_3)^{2t} \nonumber \\
    &+ \sum_{s=1}^t \left((1-\delta_2)^{t-s} \epsilon_3 (1-\delta_3)^{2s} + (1-\delta_2)^{t-s} \sum_{r=1}^{s-1} (1-\delta_2)^{s-1-r} \epsilon_3(1-\delta_3)^{2r} +  (1-\delta_2)^{t-r}\sum_{q=1}^{r-1}(1-\delta_2)^{r-1-q} \epsilon_3(1-\delta_3)^{2q} + \dots\right) 
    % &\leq (1-\delta_2) \sum_{s=1}^{t-1} (1-\delta_2)^{t-1-s} b_s + (1-\delta_2)\epsilon_3 \dist_{t-1}^2  + b_t
\end{align}

$1,t,t(t-1)/2, ...$
binomial coefficients

\end{proof}














-------------------

{\color{blue}
why do the heads need to have mean zero for MAML to work?

for simplicity assume mean zero implies $\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i} = \mathbf{0}$. Then 
\begin{align}
    \mathbf{w}_{t+1}  &= \frac{1}{n}\sum_{i=1}^n(\mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}) \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i})\mathbf{w}_t \nonumber \\
    &= \left(\mathbf{I}_{k}\! - \! \beta \frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}+  \beta\alpha\frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \right )\mathbf{w}_t
\end{align}
where 
\begin{align}
    \mathbf{B}_{t,i} &= \mathbf{B}_{t}(\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) + \alpha \mathbf{B}_{\ast}\mathbf{w}_{\ast,i}\mathbf{w}_t^\top
\end{align}
so 
\begin{align}
    \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} &= (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))\mathbf{B}_{t}^\top \mathbf{B}_{t} (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))  \nonumber \\
    &\quad + \alpha (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))\mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,i}\mathbf{w}_t^\top \nonumber \\
    &\quad + \alpha \mathbf{w}_{t} \mathbf{w}_{\ast,i}^\top\mathbf{B}_\ast^\top  \mathbf{B}_{t} (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) + \alpha^2 L_{\max}^2 \mathbf{w}_{t} \mathbf{w}_t^\top  \nonumber \\
   \frac{1}{n} \sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} &= (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))\mathbf{B}_{t}^\top \mathbf{B}_{t} (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top - \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) + \alpha^2  \mathbf{w}_{t} \mathbf{w}_t^\top  \nonumber \\
   &= \mathbf{B}_t^\top\mathbf{B}_t - \alpha \mathbf{w}_t \mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{B}_t - \alpha \mathbf{B}_t^\top \mathbf{B}_t\mathbf{w}_t \mathbf{w}_t^\top + \alpha^2 \mathbf{w}_t \mathbf{w}_t^\top\mathbf{B}_t^\top \mathbf{B}_t\mathbf{w}_t \mathbf{w}_t^\top + \alpha^2 \mathbf{w}_t \mathbf{w}_t^\top \nonumber \\
   &\quad + \dots  \nonumber \\
\frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}  &= \mathbf{U}_t^\top \mathbf{U}_t \mathbf{U}_t^\top \mathbf{U}_t + \alpha^2 \mathbf{U}_t^\top \mathbf{U}_t \mathbf{w}_t \mathbf{w}_t^\top + \alpha^2  \mathbf{w}_t \mathbf{w}_t^\top \mathbf{U}_t^\top \mathbf{U}_t \nonumber \\
&\quad + \alpha^4 \|\mathbf{w}_t\|_2^2 \mathbf{w}_t \mathbf{w}_t^\top + \alpha^2 \mathbf{V}_{t,i}^\top \mathbf{U}_t\mathbf{V}_{t,i}^\top \mathbf{U}_t + \alpha^2 \mathbf{V}_{t,i}^\top \mathbf{U}_t\mathbf{U}_{t}^\top \mathbf{V}_{t,i} \nonumber \\
&\quad + \alpha^2 \mathbf{U}_{t,}^\top \mathbf{V}_{t,i}\mathbf{V}_{t,i}^\top \mathbf{U}_t + \alpha^2 \mathbf{U}_{t}^\top \mathbf{V}_{t,i}\mathbf{U}_{t}^\top \mathbf{V}_{t,i}
\end{align}
where  $\mathbf{U}_t \coloneqq \mathbf{B}_{t} (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))$ and $\mathbf{V}_{t,i} \coloneqq \mathbf{B}_{\ast}\mathbf{w}_{\ast,i}\mathbf{w}_t^\top$.


ignoring dominated terms, we have
\begin{align}
    \mathbf{w}_{t+1} &=  \bigg(\mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))\mathbf{B}_{t}^\top \mathbf{B}_{t}(\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) \nonumber \\
    &\quad + \beta\alpha(\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k))\mathbf{B}_{t}^\top \mathbf{B}_{t}(\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) \nonumber \\
    &\quad \quad \times (\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) \mathbf{B}_{t}^\top \mathbf{B}_{t}(\mathbf{I}- \alpha \mathbf{w}_t\mathbf{w}_t^\top- \alpha\lambda (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)) \bigg )\mathbf{w}_t 
\end{align}
% the negative coefficient has minimum singular value $\frac{(1- \alpha L_{\max})^2}{\alpha}$ and max singular value $\frac{1}{\alpha}$. The positive coefficient has max singular value $1/\alpha^2$. However, applying it to $\mathbf{w}_t$ results in a vector with norm at most $\frac{L_{\max}(1-\alpha L_{\max}^2)}{\alpha^2}$.
However, we cannot show that this contracts. But empirically, $\|\mathbf{w}_t\|_2$ is almost linearly converging to zero. How can it do this without contraction?

Left off: need to show that $\|\mathbf{w}_t\|_2$ is almost linearly converging to zero when mean is zero. First show that $\|\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2$ is going to zero, then show that the same is true for all $\mathbf{B}_{t,i}$. Empirically these are true.

But empirically, $\|\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2$ does not go to zero, so $\|\mathbf{w}_t\|_2$ grows and eventually explodes.

empirically, coefff of wt has spect norm at least 1, and it increases wt sometimes, even with large n. but gradually it decreases...

\begin{align}
    \mathbf{w}_{t+1} = (\mathbf{I} - \beta \frac{1}{n})
\end{align}

need to write $\mathbf{w}_{t+1}$ as something that is contracting $\mathbf{w}_t$ plus something that we already know is linearly decreasing

from experiments: indeed we must use contraction. the reason that wt decreases is not because of the mean of the wstars is close to zero. contraction factor matters.

but how to prove contraction...
}






% We use the loss function:
% \begin{align}
%     f_{i}(\mathbf{B}_t,\mathbf{w}_t) &\coloneqq \frac{1}{2}\left\|\mathbf{Bw}-\mathbf{B}_\ast\mathbf{w}_{\ast,i} \right\|_2 + \frac{\lambda}{2}\|\mathbf{B}^\top\mathbf{B}-\mathbf{I}_k\|_F^2
% \end{align}
Denote
\begin{align}
    % \mathbf{w}_{t,i} &= (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) \mathbf{w}_t+ \alpha \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i} \\
    \mathbf{B}_{t,i} &= \mathbf{B}_t - \alpha \mathbf{G}_{t,i} \\
    \mathbf{G}_{t,i} &= \mathbf{B}_t \mathbf{w}_t \mathbf{w}_t^\top -\mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_t^\top +\alpha \lambda \mathbf{B}_t(\mathbf{B}_t^\top \mathbf{B}_t\alpha - \mathbf{I}) \\
    \mathbf{B}_{t+1} &= \mathbf{B}_t - \beta \mathbf{G}_t \\
    \mathbf{G}_t &= \frac{1}{n}\sum_{i=1}^n \bigg( \big(\mathbf{B}_{t,i} \mathbf{w}_{t,i} - \mathbf{B}_{\ast} \mathbf{w}_{\ast,i}\big)\mathbf{w}_{t,i} + \alpha \lambda \mathbf{B}_{t,i}(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) \bigg) \\
    &= \frac{1}{n}\sum_{i=1}^n \big(\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top\big) \big(\mathbf{B}_{t} \mathbf{w}_{t} - \mathbf{B}_{\ast} \mathbf{w}_{\ast,i}\big)\mathbf{w}_{t,i} + \alpha \lambda \mathbf{B}_t(\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k) \bigg) \nonumber \\
    &\quad \quad \quad  + \alpha \mathbf{G}_{t,i}(\mathbf{I} - \alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t \mathbf{w}_{t,i}^\top - \alpha^2 \mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top \nonumber \\
    &\quad \quad \quad  +\alpha \lambda \mathbf{B}_t \mathbf{P}_{t,i} - \alpha^2 \lambda \mathbf{G}_{t,i} \mathbf{P}_{t,i} - \alpha^2 \lambda \mathbf{G}_{t,i}(\mathbf{B}_t^\top \mathbf{B}_t \alpha - \mathbf{I}_d)  \\
   \mathbf{B}_{t+1}\mathbf{B}_{t+1}\alpha - \mathbf{I}_k &= \mathbf{B}_{t}\mathbf{B}_{t}\alpha - \mathbf{I}_k - \beta \mathbf{B}_t^\top \mathbf{G}_t  - \beta \mathbf{G}_t^\top \mathbf{B}_t \nonumber 
\end{align}



Note that the inner loop updates for the head are identical to the updates for ANIL, so Lemma \ref{lem:cond_app} still applies. In this case we have the following linear convergence result.



% where $\mathbf{B}_{t,i} = \mathbf{B}_t(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top) + \alpha \mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top -\alpha^2\lambda \mathbf{B}_t (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)$ 
% and $\mathbf{w}_{t,i}$ is the same as for ANIL. 

% In this case, the update for the representation is:
% \begin{align}
%     \mathbf{B}_{t+1} &= \mathbf{{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i} \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top +   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top - \beta \lambda \frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i}(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) \nonumber \\
%     &= \mathbf{{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{{B}}_{t}\left((1+\alpha \lambda)\mathbf{I}_k  - \alpha\mathbf{w}_{t}\mathbf{w}_{t}^\top - \alpha \lambda \mathbf{B}_t^\top\mathbf{B}_t )\right) \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top - \frac{\alpha\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast}\mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top+   \frac{\beta}{n}\sum_{i=1}^n \mathbf{\hat{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \nonumber \\
%     &\quad - \beta \lambda \frac{1}{n}\sum_{i=1}^n (\mathbf{B}_{t}(\mathbf{I}_k(1+\alpha \lambda )- \alpha \mathbf{w}_t \mathbf{w}_t^\top - \alpha \mathbf{B}_t^\top \mathbf{B}_t) + \alpha \mathbf{\hat{B}}_\ast \frac{1}{n}\sum_{i'=1}^n \mathbf{w}_{\ast,i'}\mathbf{w}_t^\top )(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) \nonumber \\
%     &= \mathbf{B}_t \left(\mathbf{I}_k - \beta(1+\alpha\lambda)\frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top + \beta \alpha \mathbf{w}_t\mathbf{w}_t^\top \frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top + \beta \alpha \lambda \mathbf{B}_t^\top\mathbf{B}_t^\top \frac{1}{n}\sum_{i=1}\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) \nonumber \\
%     &\quad + \mathbf{B}_t \beta \lambda  \left(-(1+\alpha \lambda)\frac{1}{n}\sum_{i=1}^n (\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) + \alpha \mathbf{w}_t \mathbf{w}_t^\top(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) + \alpha \lambda \mathbf{B}_t \mathbf{B}_t^\top(\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k)\right) \nonumber \\
%     &\quad + \mathbf{\hat{B}}_\ast \left( \right)
% \end{align}
% where $\mathbf{w}_{t,i} = (\mathbf{I}_d - \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t)\mathbf{w}_t + \alpha \mathbf{{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}$.


    

    % Choosing $\alpha < $ and $\beta< $ and $\lambda > $ means that we have ...
    
    % we need 
    % $\tau \leq \sqrt{\alpha}$
    
    % $\alpha \lambda > \tau + \sqrt{\alpha}$

    % $\alpha^2 \lambda < \tau\alpha \lambda $ meaning $ \alpha < \tau $
    
    % $ \alpha \tau^2 < \tau\alpha \lambda$ meaning $ \tau <  \lambda$
    
    % from $A_3$, we need
    
    % $\sqrt{\alpha} > \tau$
    
    % $\alpha > \alpha \lambda (\alpha + \tau)$ meaning $1 > \alpha \lambda > \tau + \sqrt{\alpha}$ (from earlier) and $ 1 > \tau \lambda$
    
    %these are feasible
    
    % we can show $\|\mathbf{P}_{t,i}\|_2 \leq 2\alpha^{1.5} \sqrt{1+\tau} \|\mathbf{G}_{t,i}\|_2 + \alpha^3 \|\mathbf{G}_{t,i}\|_2^2$ and $\|\mathbf{G}_{t,i}\|_2 \leq \sqrt{\frac{1+\tau}{\alpha}}\|\mathbf{w}_t\|_2^2 + \|\mathbf{w}_t\|_2 + \lambda \tau \sqrt{\alpha(1+\tau)}$ so $\|\mathbf{P}_{t,i}\|_2 = o(\alpha \|\mathbf{w}_t\|_2^2 + \alpha^2 \|\mathbf{w}_t\|_2^4 + \lambda \tau \alpha ^2)$. Thus $\alpha \lambda \mathbf{B}_t \mathbf{P}_{t,i} = o(\lambda \alpha^{1.5} \|\mathbf{w}_t\|_2 +\lambda \alpha^{2.5} \|\mathbf{w}_t\|_2^2 + \lambda^2 \tau \alpha^{2.5})$
    
    
    % implies that we need to show $\|\mathbf{w}_t\|_2 = O(\alpha)$
    
    % good terms are $\tau \lambda(1-\tau)$, $\tau E_0\mu_\ast^2(1-\tau)$. 
    
    % bad terms:
    % $ \tau^2 \sqrt{\frac{1+\tau}{\alpha}}L_{\max}^2 + \tau^2 L_{\max} + \tau (1+\tau)L_{\max}L_\ast + \dots + (\lambda \alpha^{1.5} \|\mathbf{w}_t\|_2 +\lambda \alpha^{2.5} \|\mathbf{w}_t\|_2^2 + \lambda^2 \tau \alpha^{2.5} )$
    
    % implies that we need $\alpha^{1.5} \leq 1/\lambda$, $\tau \geq \alpha^{1.5}$ if $\|\mathbf{w}_t\|_2$ is a constant 
    
    % -----
    
    % First, we write
    % \begin{align}
    %     \boldsymbol{\Delta}_{t+1} &= \boldsymbol{\Delta}_{t} - \beta \mathbf{G}_{t}^\top \mathbf{B}_t - \beta \mathbf{B}_t^\top \mathbf{G}_t + \beta^2 \mathbf{G}_{t}^\top \mathbf{G}_{t} \nonumber \\
    %     &= 
    % \end{align}
    
    

\begin{lemma}[Representation stays well-conditioned]\label{lem:reg_fs}


\end{lemma}

\begin{proof}
Recall the infinite-sample proof.

By definition of $\tau$, \eqref{res:control_spectrum} holds for iteration $t=0$. Suppose it holds at arbitrary iteration $t$. We will show that this implies it holds at iteration $t+1$. 
Note that we can write:
\begin{align}
    \mathbf{B}_{t+1} &=\mathbf{{B}}_t  - \beta(\mathbf{I}_d -  \alpha \mathbf{{B}}_t \mathbf{{B}}_t^\top)\frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top + \alpha \beta \lambda (\mathbf{I}_d - \alpha\mathbf{{B}}_t \mathbf{{B}}_t^\top) \mathbf{{B}}_t \nonumber \\
    &\quad + \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{I}_d - \mathbf{\Sigma}_{t,i}^{out}\right) \left(\mathbf{B}_t  \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\right)\mathbf{w}_{t,i}^\top  + \frac{\beta}{n m_{out}}\sum_{i=1}^n(\mathbf{X}^{out}_{t,i})^\top \mathbf{z}^{out}_{t,i}\mathbf{w}_{t,i}^\top \nonumber \\
    &=\mathbf{{B}}_t  - \beta(\mathbf{I}_d -  \alpha \mathbf{{B}}_t \mathbf{{B}}_t^\top)\frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top + \alpha \beta \lambda (\mathbf{I}_d - \alpha\mathbf{{B}}_t \mathbf{{B}}_t^\top) \mathbf{{B}}_t \nonumber \\
    &\quad + \beta\mathbf{E}_1 + \beta \mathbf{E}_2
\end{align}
% \begin{align}
%     \mathbf{B}_{t+1} 
%     &=  \mathbf{{B}}_t  - \beta(\mathbf{I}_d -  \alpha \mathbf{{B}}_t \mathbf{{B}}_t^\top)\frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top + \alpha \beta \lambda (\mathbf{I}_d - \alpha\mathbf{{B}}_t \mathbf{{B}}_t^\top) \mathbf{{B}}_t  %\\
% \end{align}
From equations \eqref{boundE1anil} and \eqref{boundE2anil}, we have high-probability upper bounds on $\|\mathbf{E}_1\|$ and $\|\mathbf{E}_2\|$, respectively.
Let $\mathbf{B}_{t+1}^{pop} \coloneqq \mathbf{{B}}_t  - \beta(\mathbf{I}_d -  \alpha \mathbf{{B}}_t \mathbf{{B}}_t^\top)\frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top + \alpha \beta \lambda (\mathbf{I}_d - \alpha\mathbf{{B}}_t \mathbf{{B}}_t^\top) \mathbf{{B}}_t$ as the update of the representation in the infinite sample case. We have
\begin{align}
   &\| \mathbf{I}_k\!-\!\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \|_2 \nonumber \\
   \!&=\! \|\mathbf{I}_k\!-\!\alpha (\mathbf{B}_{t}^{pop})^\top \mathbf{B}_{t}^{pop} \|_2  + 2\alpha \beta \| (\mathbf{E}_1\!+ \!\mathbf{E}_2)^\top \mathbf{B}_{t}^{pop}\|_2\!+\!\alpha \beta^2\|\mathbf{E}_1\!+ \!\mathbf{E}_2\|_2^2 \nonumber \\
    &\leq  \tau \bigg(
    1 - 2 \beta ( E_0 \mu_\ast^2+ \lambda) (1-\tau)+ 2 \beta\tau (1+\tau)L_{\max}^2  + 2 \beta(1+2\tau)\sqrt{\alpha(1+\tau)} L_{\ast} L_{\max} \bigg) \nonumber \\
   &\quad  +\alpha \beta^2 \Phi + 2\alpha \beta \| (\mathbf{E}_1\!+ \!\mathbf{E}_2)^\top \mathbf{B}_{t}^{pop}\|_2\!+\!\alpha \beta^2\|\mathbf{E}_1\!+ \!\mathbf{E}_2\|_2^2 \nonumber \\
   &\leq \tau \bigg(
    1 - 2 \beta ( E_0 \mu_\ast^2+ \lambda) (1-\tau)+ 2 \beta\tau (1+\tau)L_{\max}^2  + 2 \beta(1+2\tau)\sqrt{\alpha(1+\tau)} L_{\ast} L_{\max} \bigg) \nonumber \\
   &\quad  +\alpha \beta^2 \Phi + 2\alpha \beta (\sigma+e_1)e_2\delta_{out} \|  \mathbf{B}_{t}^{pop}\|_2 \!+\!\alpha \beta^2(\sigma+e_1)^2e_2^2\delta_{out}^2 \label{111}
\end{align}
where the last inequality follows with high probability from . We have 
\begin{align}
    \|\mathbf{B}_{t}^{pop}\|_2 &= \left\|\mathbf{B}_t\left(\mathbf{I}_k - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top  - \beta \alpha \lambda (\mathbf{B}_t^\top \mathbf{B}_t -\mathbf{I}_k)\right) + \mathbf{\hat{B}}_\ast \left(\frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top \right) \right\|_2  \nonumber \\
    &\leq \sqrt{\tfrac{1+\tau}{\alpha}}(1 - \beta \mu_{\ast}^2 + \beta \alpha\lambda \tau + \beta L_{\ast}L ) \label{use_prev}
\end{align}
where \eqref{use_prev} follows with probability at least . 
Combining \eqref{111} and \eqref{use_prev} yields
\begin{align}
    \|\mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2  &\leq \tau \bigg(
    1 - 2 \beta ( E_0 \mu_\ast^2+ \lambda) (1-\tau)+ 2 \beta\tau (1+\tau)L_{\max}^2  + 2 \beta(1+2\tau)\sqrt{\alpha(1+\tau)} L_{\ast} L_{\max} \bigg) \nonumber \\
   &\quad  +\alpha \beta^2 \Phi + 2\alpha \beta (\sigma+e_1)e_2\delta_{out}  \sqrt{\tfrac{1+\tau}{\alpha}}(1 - \beta \mu_{\ast}^2 + \beta \alpha\lambda \tau + \beta L_{\ast}L ) \!+\!\alpha \beta^2(\sigma+e_1)^2e_2^2\delta_{out}^2
\end{align}
Choosing $\beta$ such that
\begin{align}
    \beta &\leq \frac{2}{  }\Big( 
    \Big) 
    \nonumber  %\\
\end{align}
completes the proof.
\end{proof}




% \begin{align}
%     a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
%     &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} {z}_{t-1})(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_{t-1} L_\ast(1 + \tfrac{2\beta}{\alpha} {z}_t)  + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
%     &\;\; \vdots \nonumber \\
%     &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t {z}_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
%     & {\color{red} ----------} \\
%     &=  \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t (z_s + \tfrac{c}{t})\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r + \tfrac{\beta}{\alpha}\tfrac{c}{t}) \nonumber \\
%     &= \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t (\rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1- \rho} + \tfrac{\beta}{\alpha}\tfrac{c}{t})\prod_{r=s+1}^t(1+ \rho^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1- \rho}+\tfrac{\beta}{\alpha}\tfrac{c}{t}) \nonumber \\
%     &= \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast \sum_{s=0}^t \rho^{s} \prod_{r=s+1}^t\left(1+ \rho^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - \rho}\right) + \tfrac{\beta}{\alpha}\tfrac{c}{t}\sum_{s=1}^t \prod_{r=s+1}^t(1+ \rho^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1- \rho}+\tfrac{\beta}{\alpha}\tfrac{c}{t})  \nonumber
% \end{align}    
{\color{red}
\begin{align}
    \tfrac{\beta}{\alpha}\tfrac{c}{t}\sum_{s=1}^t \prod_{r=s+1}^t(1+ \rho^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1- \rho}+\tfrac{\beta}{\alpha}\tfrac{c}{t}) &\leq  \tfrac{\beta}{\alpha}\tfrac{c}{t}\sum_{s=1}^t \left( 1+ \tfrac{1}{t-s}\sum_{r=s+1}^t(\rho^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1- \rho}+\tfrac{\beta}{\alpha}\tfrac{c}{t})\right)^{t-s} \nonumber \\
    &\leq  \tfrac{\beta}{\alpha}\tfrac{c}{t}\sum_{s=1}^t \left( 1+ \tfrac{1}{t-s} (\tfrac{{20\alpha}\beta^3 L_\ast^4 }{\alpha^2\beta^2}+\tfrac{\beta}{\alpha}c)\right)^{t-s}
\end{align}
$\implies $ finite samples add only a small additive constant, do not change the upper bound on $\mathbf{w}_t$.

but $z_t$ also has an additive term, but this is fine because it also becomes $1/T$, i think constants don't matter
}

where the first equality follows under the assumption that $a_0 = 0$. By the AM-GM inequality and sum of geometric series, we have, for $s\leq t-1$,
\begin{align}
    \prod_{r=s+1}^t\left(1+ \rho^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1 - \rho}\right) &\leq \left(1 + \tfrac{1}{t-s} \sum_{r=s+1}^t \rho^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - \rho}\right)^{t-s} \nonumber \\
    &\leq \left(1 + \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3\rho^{s+1}L_\ast^4 }{(1- \rho)^2} \right)^{t-s} 
\end{align}



The RHS is monotonically increasing in $t$ (since each additional $t$ means multiplication by a number greater than 1) so we can upper bound it by its limit as $t \rightarrow \infty$. This limit is 
% $\exp\left(\left(1 + \tfrac{1}{t-s+1} \tfrac{\sqrt{\alpha}\beta^3\rho^{2}}{(1- \rho)^2} \right)^{t-s-1} \right) $, where the exponent is less than 1 for sufficiently small $\alpha, \beta$. For general $s$, the RHS limit is 
$\exp\left( \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3\rho^{s+1}}{(1- \rho)^2} \right)$ (note that it is of the form $\lim_{t\rightarrow \infty} (1+\tfrac{a}{x})^x$). To ensure this exponent is less than 1, we can choose
\begin{align}
  {20\alpha}\beta^3 L_\ast^4  &\leq   (1- \rho)^2 \nonumber \\
  \iff {20\alpha}\beta^3 L_\ast^4 &\leq   \alpha^2 \beta^2 \nonumber \\
  \iff \beta &\leq \alpha/(20 L_\ast^4).
\end{align}
Under this condition on $\beta$, we have
\begin{align}
    a_{t+1} &\leq \tfrac{20 \alpha^{1.5}\beta^3L_\ast^4 }{1 - \rho} L_\ast\sum_{s=1}^{t-1} \rho^{s} \exp\left( \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3\rho^{s+1}L_\ast^4 }{(1- \rho)^2} \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - \rho} L_\ast \rho^{t} \nonumber \\
    &\leq \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast\sum_{s=1}^{t-1} \rho^{s}\left(1+ \tfrac{2\rho^{s+1}}{t-s} \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - \rho} L_\ast \rho^{t} \nonumber \\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast\sum_{s=1}^{t} \rho^{s} \nonumber \\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{(1 - \rho)^2} L_\ast \nonumber \\
    &\leq  L_\ast
\end{align} 
where the second inequality follows from the numerical inequality $e^x \leq 1+2x$ for $x\in [0,1]$, and the last inequality follows for $\beta \leq\alpha/(60 L_\ast^4).$




Next, we characterize the diversity of the inner loop-updated heads.
\begin{lemma} \label{lem:cond_app}
Let $\alpha=1$ and $\beta \leq 1/L_{\ast}^2$.
Define $\mu^2 \coloneqq \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$ and $L^2 \coloneqq \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$. 
Under Assumption \ref{assump:data}, $\|\mathbf{w}_t\|_2 \leq L_{\max}$ and $\max_{i \in [n]} \|\mathbf{w}_{\ast,t,i}\|_2 \leq L_{\max}$, we have 
\begin{align}
    L &\leq L_{\max} \tau + L_\ast \sqrt{\alpha(1+\tau)}+ 2 L_{\max}(1+\tau)\delta_{in}  + \sigma \sqrt{\alpha (1+\tau)}\delta_{in} \\
    \text{and} \quad \mu &\geq \sqrt{\alpha(1-\tau) E_0^2 \mu_\ast^2 - 2 \tau \sqrt{\alpha(1+\tau)} L_{\ast} - 2  (L_{\max} \tau+ L_\ast \sqrt{\alpha(1+\tau)} )  (2L_{\max}(1+\tau) + \sigma \sqrt{\alpha (1+\tau)} )\delta_{in} }
%\mu_\ast^2 E_0 - 4 L_{\max}^2 (\delta_{in} + \delta_{in}^2) 
 \end{align}
 with probability at least $1 - 4 n^{-99}$.
\end{lemma}

\begin{proof}
Note that $\mathbf{w}_{t,i}$ can be written as:
\begin{align}
    \mathbf{w}_{t,i} &= \mathbf{r} + \mathbf{s}_i   + \mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i}
\end{align}
where $\mathbf{r} = (\mathbf{I}- \alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t$, $\mathbf{s}_i = \alpha \mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}$,  $\mathbf{p}_{1,i} = \alpha(\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{B}_t^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )  \mathbf{{w}}_{t}$,  $\mathbf{p}_{2,i} = -\alpha(\mathbf{B}_t^\top \mathbf{\hat{B}}_\ast - \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,t,i}$, and  $\mathbf{p}_{3,i} =\frac{\alpha}{m_{in}} \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in}$ for all $i \in [n]$ (for ease of notation we drop the iteration index $t$). For any $i \in [n]$, we have 
\begin{align}
    \| \mathbf{p}_{1,i}\|_2 &\leq L_{\max}{{(1+\tau)}}  \delta_{in}, \quad
    \| \mathbf{p}_{2,i}\|_2 \leq L_\ast \sqrt{{\alpha(1+\tau)}} \delta_{in}, \quad 
    \| \mathbf{p}_{3,i}\|_2 \leq   \sigma\sqrt{{{\alpha}(1+\tau)}}\delta_{in}  \label{basicbounds}
\end{align}
each with probability at least $1 - 2 n^{-100}$ (so all of these events  happen simultaneously with probability at least $1- 6 n^{-100}$). Further, a union bound over all $i \in [n]$ shows that $P\left(\cap_{i\in [n]}\left\{\| \mathbf{p}_{1,i}\|_2 \leq L_{\max}{{(1+\tau)}}  \delta_{in} \cap \| \mathbf{p}_{2,i}\|_2 \leq L_{\ast}\sqrt{{{\alpha}(1+\tau)}}  \delta_{in}\cap \| \mathbf{p}_{3,i}\|_2 \leq \sigma \sqrt{{{\alpha}(1+\tau)}} \delta_{in}  \right\} \right) \geq 1 - 6 n^{-99}$. Furthermore, note that for any $i \in [n]$
    \begin{align}
       \| \mathbf{p}_{1,i} +  \mathbf{p}_{2,i} + \mathbf{p}_{3,i}\|_2  &\leq (L_{\max}{{(1+\tau)}} +L_{\ast}\sqrt{{{\alpha}(1+\tau)}} + \sigma\sqrt{{{\alpha}(1+\tau)}})  \delta_{in} \nonumber \\
       &\leq (2L_{\max}{{(1+\tau)}}  + \sigma\sqrt{{{\alpha}(1+\tau)}})  \delta_{in}
    \end{align}
    with high probability (where we have used the fact that $L_{\ast} \sqrt{\alpha(1+\tau)}\leq L_{\max} (1+\tau)$ in the second inequality), and
\begin{align}
    &\left\|\frac{1}{n}\sum_{i=1}^n (\mathbf{r}+\mathbf{s}_i)(\mathbf{r}+ \mathbf{s}_i)^\top \right\|_2 \nonumber \\
    &\leq \|(\mathbf{I}_k-\alpha \mathbf{B}_t^\top\mathbf{B}_t)\mathbf{w}_t\|_2^2 + 2 \alpha \|(\mathbf{I}_k-\alpha \mathbf{B}_t^\top\mathbf{B}_t)\mathbf{w}_t\|_2 \|\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\|_2 \left\|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i} \right\|_2 \nonumber \\
    &\quad + \alpha^2\|\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\|_2^2 \left\|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \right\|_2 \nonumber \\
    &\leq L_{\max}^2 \tau^2 + 2 L_{\max}L_\ast \tau \sqrt{\alpha(1+\tau)} +  \alpha L_\ast^2({{1+\tau}})
    \end{align}
    
    So,
% \begin{align}
%     &\|\mathbf{q}_{t,i}\|_2 \nonumber \\ 
%     &= \| \mathbf{w}_{t,i} - (\mathbf{I}_k -\alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t - \alpha \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
%     &= \left\|  (\mathbf{{B}}_t^\top\mathbf{{B}}_t\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_t)\mathbf{{w}}_{t} - (\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast ) \mathbf{{w}}_{\ast,t,i}\! +\!  \frac{1}{m_{in}} \mathbf{B}_t^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 \nonumber \\
%     &\leq \left\| (\mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )  \mathbf{{w}}_{t}\right\|_2 + \left\|(\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,t,i}\right\|_2\! \nonumber \\
%     &\quad \quad +\frac{1}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 
%     % \|(\mathbf{I}- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )\mathbf{{w}}_t +  \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2\nonumber \\
%     % &\leq \|(\mathbf{I}- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )\mathbf{{w}}_t\|_2 + \| \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
%     % &\leq  \|\mathbf{I}_k- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2 \|  \mathbf{{w}}_t\|_2 + \| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2 \|{\mathbf{w}_{\ast,t,i}}\|_2  \nonumber \\
%     % &\leq  L_{\max}\|\mathbf{I}_k- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2  + L_{\max}\| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2
%     \label{twoterms}\\
%     &\leq L_{\max}\left\| \mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t  \right\|_2 + L_\ast \left\|\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\right\|_2\! \nonumber \\
%     &\quad \quad +\frac{1}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2  \label{cs31}
% \end{align}
\begin{align}
   \left\| \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right\|_2 &= \Bigg\|\frac{1}{n} \sum_{i = 1}^n (\mathbf{r}+\mathbf{s}_i)(\mathbf{r}+\mathbf{s}_i)^\top + (\mathbf{r}+\mathbf{s}_i)(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top \nonumber \\
   &\quad + (\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})(\mathbf{r}+\mathbf{s}_i)^\top  + (\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})^\top \Bigg\|_2 \nonumber \\
   &\leq \left\|\frac{1}{n} \sum_{i = 1}^n (\mathbf{r}+\mathbf{s}_i)(\mathbf{r}+\mathbf{s}_i)^\top\right\|_2 + 2 \left\|\frac{1}{n} \sum_{i = 1}^n (\mathbf{r}+\mathbf{s}_i)(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top \right\|_2 \nonumber \\
   &\quad \quad \quad + \left\|\frac{1}{n} \sum_{i = 1}^n (\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})^\top \right\|_2 \nonumber \\
   &\leq L_{\max}^2 \tau^2 + 2 L_{\max}L_\ast \tau \sqrt{\alpha(1+\tau)} +  \alpha L_\ast^2({{1+\tau}}) + 2 \left\|\frac{1}{n} \sum_{i = 1}^n \mathbf{r}(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top \right\|_2 \nonumber\\
   &\quad + 2\alpha\|\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\|_2 \left\| \frac{1}{n}\mathbf{W}_{\ast,t}^\top \begin{bmatrix}\vdots \\
(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top    \\
   \vdots \\
   \end{bmatrix}\right\|_2  + \max_{i\in [n]} \|\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} \|_2^2 \label{tri32}\\
%   &\leq                                                         \nonumber\\
   &\leq L_{\max}^2 \tau^2 + 2 L_{\max}L_\ast \tau \sqrt{\alpha(1+\tau)} +  \alpha L_\ast^2({{1+\tau}})\nonumber \\
   &\quad + 2 L_{\max} \tau(2 L_{\max}(1+\tau)  + \sigma \sqrt{\alpha (1+\tau)} ) \delta_{in}
%   \left\|\frac{1}{n} \sum_{i = 1}^n \mathbf{r}(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top \right\|_2    
   \nonumber \\
   &\quad + 2 \sqrt{\alpha(1+\tau)} L_\ast (2L_{\max}(1+\tau) + \sigma \sqrt{\alpha (1+\tau)} )\delta_{in} 
\nonumber \\
&\quad + \left(2 L_{\max}(1+\tau)  + \sigma \sqrt{\alpha (1+\tau)} \right)^2\delta_{in}^2  \nonumber\\
%   &= (L_{\max} \tau + L_\ast \sqrt{\alpha(1+\tau)})^2 \nonumber \\
%   &\quad 2(L_{\max} \tau + L_\ast \sqrt{\alpha(1+\tau)})(2 L_{\max}(1+\tau)  + \sigma \sqrt{\alpha (1+\tau)} ) \delta_{in} \nonumber \\
%   + \left(2 L_{\max}(1+\tau)  + \sigma \sqrt{\alpha (1+\tau)} \right)^2\delta_{in}^2 \nonumber \\
   &= \left(L_{\max} \tau + L_\ast \sqrt{\alpha(1+\tau)}+ 2 L_{\max}(1+\tau)\delta_{in}  + \sigma \sqrt{\alpha (1+\tau)}\delta_{in} \right)^2
%   L_{\max}^2 \tau^2 + 2 L_{\max}L_\ast \tau \sqrt{\alpha(1+\tau)} +  \alpha L_\ast^2({{1+\tau}}) \nonumber \\
%   &\quad + 2 L_{\max}^2 \tau(1+\tau)\delta_{in} + 4 L_{\max}^2 L_{\ast} \tau^2\sqrt{\alpha (1+\tau)}\delta_{in} + 2 L_{\max} \tau  (   + \alpha L_\ast^2 (1+\tau) ) \delta_{in}
% %   \left\|\frac{1}{n} \sum_{i = 1}^n \mathbf{r}(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top \right\|_2    
%   \nonumber \\
%   &\quad + 2 \sqrt{\alpha} L_\ast  (1+\tau)\left(L_{\max}\sqrt{{(1+\tau)}}+\sigma \sqrt{\alpha} \right)\delta_{in}  + (1+\tau)\left(L_{\max}\sqrt{{(1+\tau)}}+\sigma \sqrt{\alpha} \right)^2\delta_{in}^2 
%   &\leq  L_\ast^2{\tfrac{1+\tau}{\alpha}} + 2  L_\ast \sqrt{\tfrac{1+\tau}{\alpha}} \max_{i \in [n]}
% \|\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} \|_2 + (1+\tau)\left(L_{\max}\sqrt{{(1+\tau)}}+\sigma \sqrt{\alpha} \right)^2\delta_{in}^2  \nonumber\\
% &\leq L_\ast^2{\tfrac{1+\tau}{\alpha}} + 2  L_\ast {\tfrac{1+\tau}{\alpha}}\left(2 L_{\max}\sqrt{\tfrac{(1+\tau)}{\alpha}} + \sigma\right)\delta_{in} + (1+\tau)\left(L_{\max}\sqrt{{(1+\tau)}}+\sigma \sqrt{\alpha} \right)^2\delta_{in}^2 \nonumber \\
% &= {\frac{1+\tau}{\alpha}}\left( L_\ast +  \left(2L_{\max}\sqrt{\tfrac{(1+\tau)}{\alpha}}+\sigma\right)\delta_{in} \right)^2 
\label{hp1}
% &= \left(L_{\ast} +  \right)
\end{align}
where $\mathbf{W}_{\ast,t} = [\mathbf{w}_{\ast,t,1},\dots,\mathbf{w}_{\ast,t,n}]^\top$, \eqref{tri32} follows from the triangle inequality, and \eqref{hp1} follows with probability at least $1 - 6 n^{-99}$ from the discussion above.

We make an analogous argument to lower bound $\sigma_{\min}\left(\frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)$. We have
\begin{align}
  \sigma_{\min} \left( \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) 
   &=  \sigma_{\min}  \Bigg(\frac{1}{n} \sum_{i = 1}^n (\mathbf{r}+\mathbf{s}_i)(\mathbf{r}+\mathbf{s}_i)^\top + (\mathbf{r}+\mathbf{s}_i)(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top + (\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})(\mathbf{r}+\mathbf{s}_i)^\top \nonumber \\
   &\quad \quad \quad + (\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i})^\top \Bigg) \nonumber \\
   &\geq  \sigma_{\min}  \left(\frac{1}{n} \sum_{i = 1}^n (\mathbf{r}+\mathbf{s}_i)(\mathbf{r}+\mathbf{s}_i)^\top\right) - 2    \left\|\frac{1}{n}\sum_{i=1}^n(\mathbf{r}+\mathbf{s}_i)(\mathbf{p}_{1,i} + \mathbf{p}_{2,i} + \mathbf{p}_{3,i} )^\top\right\|_2  \nonumber \\
   &\geq \sigma_{\min}  \left(\frac{1}{n} \sum_{i = 1}^n \mathbf{s}_i\mathbf{s}_i^\top\right) - 2 \left\|\frac{1}{n} \sum_{i = 1}^n \mathbf{r}\mathbf{s}_i^\top \right\|_2  \nonumber \\
   &\quad - 2  (L_{\max} \tau+ L_\ast \sqrt{\alpha(1+\tau)} )  (2L_{\max}(1+\tau) + \sigma \sqrt{\alpha (1+\tau)} )\delta_{in}  \nonumber \\
   &\geq \alpha(1-\tau) E_0^2 \mu_\ast^2 - 2 \tau \sqrt{\alpha(1+\tau)} L_{\ast}  \nonumber \\
   &\quad - 2  (L_{\max} \tau+ L_\ast \sqrt{\alpha(1+\tau)} )  (2L_{\max}(1+\tau) + \sigma \sqrt{\alpha (1+\tau)} )\delta_{in}  \nonumber \\
\end{align}
 with probability at least $1 - 6 n^{-99}$.
\end{proof}

Intuitively, we cannot use a union bound bound over tasks because we need each task to concentrate individually. Concentration of the average across tasks is not enough. We will see that this is not the case for the outer loop update, which allows us to obtain a $\frac{1}{\sqrt{n}}$ factor in the concentration result.




\begin{lemma} \label{lem:concen}
Pick any iteration $t\in [T]$. Define $\mathbf{q}_{t,i} \coloneqq \mathbf{w}_{t,i} - (\mathbf{I}_k -\alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t -\alpha \mathbf{{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}$ for all $i \in [n]$ and $\mathbf{Q}_t \coloneqq \begin{bmatrix}\vdots \\
    \mathbf{q}_{t,i}^\top \\
    \vdots
    \end{bmatrix}$. Assume $\|\mathbf{w}_t\|_2 \leq L_{\max}$ and $\max_{i\in[n]}\|\mathbf{w}_{\ast,t,i}\|_{2}\leq L_{\max}$ and event $A$ occurs. Assume $m_{in}\geq 2c (k + 10 \log(n))$.  Then
\begin{align}
   \frac{1}{\sqrt{n}} \| \mathbf{Q}_t \|_F \leq (L_{\max}+\sigma)  \delta_{in}
\end{align}
with probability at least $1 - 6 n^{-99}$.
\end{lemma}
\begin{proof}
% For $\alpha=1$ and any $i$, we have
% \begin{align}
%     \mathbf{w}_{t,i} &= (1-\alpha)\mathbf{{w}}_t + \alpha \mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,t,i}  \nonumber \\
% &\quad - \alpha (\mathbf{I}_k - \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )  \mathbf{{w}}_{t} - \alpha (\mathbf{I}_k - \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,t,i}  +  \frac{\alpha}{m_{in}} \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in}
% \end{align}
\begin{align}
    &\|\mathbf{q}_{t,i}\|_2 \nonumber \\ 
    &= \| \mathbf{w}_{t,i} - (\mathbf{I}_k -\alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t - \alpha \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
    &= \left\|  (\mathbf{{B}}_t^\top\mathbf{{B}}_t\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_t)\mathbf{{w}}_{t} - (\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast ) \mathbf{{w}}_{\ast,t,i}\! +\!  \frac{1}{m_{in}} \mathbf{B}_t^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 \nonumber \\
    &\leq \left\| (\mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )  \mathbf{{w}}_{t}\right\|_2 + \left\|(\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,t,i}\right\|_2\! \nonumber \\
    &\quad \quad +\frac{1}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 
    % \|(\mathbf{I}- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )\mathbf{{w}}_t +  \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2\nonumber \\
    % &\leq \|(\mathbf{I}- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )\mathbf{{w}}_t\|_2 + \| \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
    % &\leq  \|\mathbf{I}_k- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2 \|  \mathbf{{w}}_t\|_2 + \| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2 \|{\mathbf{w}_{\ast,t,i}}\|_2  \nonumber \\
    % &\leq  L_{\max}\|\mathbf{I}_k- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2  + L_{\max}\| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2
    \label{twoterms}\\
    &\leq L_{\max}\left\| \mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t  \right\|_2 + L_\ast \left\|\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\right\|_2\! \nonumber \\
    &\quad \quad +\frac{1}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2  \label{cs31}
\end{align}

For any $i \in [n]$, we have 
\begin{align}
    &\|\mathbf{q}_{t,i}\|_2 \nonumber \\ 
    &= \| \mathbf{w}_{t,i} - (\mathbf{I}_k -\alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t - \alpha \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
    &= \alpha\left\|  (\mathbf{{B}}_t^\top\mathbf{{B}}_t\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_t)\mathbf{{w}}_{t} - (\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast ) \mathbf{{w}}_{\ast,t,i}\! +\!  \frac{1}{m_{in}} \mathbf{B}_t^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 \nonumber \\
    &\leq \alpha\left\| (\mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )  \mathbf{{w}}_{t}\right\|_2 + \left\|(\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,t,i}\right\|_2\! \nonumber \\
    &\quad \quad +\frac{\alpha}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 
    % \|(\mathbf{I}- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )\mathbf{{w}}_t +  \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2\nonumber \\
    % &\leq \|(\mathbf{I}- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )\mathbf{{w}}_t\|_2 + \| \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
    % &\leq  \|\mathbf{I}_k- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2 \|  \mathbf{{w}}_t\|_2 + \| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2 \|{\mathbf{w}_{\ast,t,i}}\|_2  \nonumber \\
    % &\leq  L_{\max}\|\mathbf{I}_k- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2  + L_{\max}\| \mathbf{\hat{B}}_{t}^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast\|_2
    \label{twoterms}\\
    &\leq \alpha L_{\max}\left\| \mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t  \right\|_2 + \alpha L_\ast \left\|\mathbf{B}_t ^\top \mathbf{\hat{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{\hat{B}}_\ast\right\|_2\! \nonumber \\
    &\quad \quad +\frac{\alpha}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2  \label{cs31}
\end{align}
where \eqref{twoterms} follows from the triangle inequality, \eqref{cs31} follows from the Cauchy-Schwarz inequality and the assumptions that $\|{\mathbf{w}_{\ast,t,i}}\|_2 \leq L_{\max}$ and $\|{\mathbf{w}_{t}}\|_2 \leq L_{\max}$. 
% (assumed for simplicity, but we can likely show that we can normalize $\mathbf{w}_t$ at the end of each round WLOG). 
We first consider the term 
\begin{align}
    \| \mathbf{{B}}_t^\top\mathbf{{B}}_t- \mathbf{B}_t^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2  &=  \left\| \mathbf{{B}}_t^\top\mathbf{{B}}_t-    \frac{1}{m_{in}}\sum_{j=1}^{m_{in}}\mathbf{B}_t ^\top\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top\mathbf{B}_t \right\|_2
\end{align}
where $\mathbf{B}_t ^\top\mathbf{x}_{i,j}$ is sub-Gaussian with covariance $\mathbf{B}_t^\top\mathbf{B}_t$. Thus, by equation 4.22 in \cite{vershynin2018high} and the fact that $\| \mathbf{{B}}_t^\top\mathbf{{B}}_t\|_2 \leq \frac{1+\tau}{\alpha}$, we have
\begin{align}
    \| \mathbf{{B}}_t^\top\mathbf{{B}}_t- \mathbf{B}_t ^\top \mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t \|_2 &\leq c \frac{1+\tau}{\alpha} \max\left( \frac{\sqrt{k} + \lambda}{\sqrt{m_{in}}},  \frac{k + \lambda^2}{m_{in}}\right) \label{concen1}
\end{align}
for some absolute constant $c$,
with probability at least $ 1 - 2 e^{-\lambda^2}$, for any $\lambda > 0$. Analogous arguments show that similar upper bound holds for the second and third terms in \eqref{cs31}, e.g. for the third term, the same bound holds with $L_{\max}$ replaced by $\sigma$.
Therefore, via a union bound over $i \in [n]$ we have 
\begin{align}
    \| \mathbf{q}_{t,i} \|_2 &\leq c'\left(L_{\max}{{(1+\tau)}} + L_\ast\sqrt{{\alpha(1+\tau)}{}} +\sigma\sqrt{{\alpha(1+\tau)}} \right) \max\left( \frac{\sqrt{k} + \lambda}{\sqrt{m_{in}}},  \frac{k + \lambda^2}{m_{in}}\right) 
\end{align}
with probability at least $ 1 - 6 e^{-\lambda^2}$, for any $\lambda>0$. Now choose $\lambda = 10 \sqrt{\log(n)}$ and union bound over all $i \in [n]$ to obtain
\begin{align}
    % \frac{1}{n}\sum_{i=1}^n\| \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top\mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2^2 &\leq c'' L_{\max}^2  \left(\max\left( \frac{\sqrt{k} + 10 \sqrt{\log(n)}}{\sqrt{m_{in}}},  \frac{k + 100\log(n)}{m_{in}}\right)\right)^2 \nonumber \\
    % \implies 
    \frac{1}{\sqrt{n}}\|\mathbf{Q}_t\|_F &= \sqrt{\frac{1}{n}\sum_{i=1}^n\| \mathbf{q}_{t,i} \|_2^2} \nonumber \\
    &\leq c'\left(L_{\max}{{(1+\tau)}} + L_\ast\sqrt{{\alpha(1+\tau)}} +\sigma\sqrt{{\alpha(1+\tau)}{}} \right) \max\left( \frac{\sqrt{k} + 10 \sqrt{\log(n)}}{\sqrt{m_{in}}},  \frac{k + 100\log(n)}{m_{in}}\right) \nonumber \\
    &\leq \left(L_{\max}{{(1+\tau)}}  +\sigma\sqrt{{\alpha(1+\tau)}{}} \right)  \delta_{in} %=: L_\ast \epsilon
\end{align}
with probability at least $1 - 6n e^{-100 \log(n)}= 1 - 6n^{-99}$, where we have dropped the $ L_\ast\sqrt{{\alpha(1+\tau)}{}}$ because it is dominated by $L_{\max}{(1+\tau)}$. 
\end{proof}






Next, let $\gamma \coloneqq 1 - 0.5 \beta ( E_0 \mu_\ast^2+ \lambda)  + 5 \beta \sqrt{\alpha} L_{\ast}^2$. By $\bigcup_{s=0}^t A_2(s)$, we have
\begin{align}
    \|\mathbf{I}-\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2 &\leq \gamma\|\mathbf{I}-\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2 + 10 \alpha^{2}\beta^2 L_\ast^4 \dist_t^2 \nonumber \\
    &\leq \gamma^2\|\mathbf{I}-\alpha \mathbf{B}_{t-1}^\top \mathbf{B}_{t-1}\|_2 + 10\alpha^{2}\beta^2\gamma \dist_{t-1}^2 +  10\alpha^{2}\beta^2 \dist_t^2 \nonumber \\
    &\;\;\vdots \nonumber \\
    &\leq  \gamma^{t+1}\|\mathbf{I}-\alpha \mathbf{B}_{0}^\top \mathbf{B}_{0}\|_2 + 10 \alpha^{2}\beta^2 L_\ast^4  \sum_{s=0}^t \gamma^{t-s} \dist_s^2  \nonumber \\
    &= 10\alpha^{2}\beta^2 L_\ast^4  \sum_{s=0}^t \gamma^{t-s} \dist_s^2
    % \nonumber \\
    % &\leq \sum_{s=1}^t \gamma^{t-s} \rho^s \nonumber \\
    % &= \gamma^t \sum_{s=1}^t \left(\frac{\rho}{\gamma}\right)^s \nonumber \\
    % &=: z_t
\end{align}
since $\|\mathbf{I}-\alpha \mathbf{B}_{0}^\top \mathbf{B}_{0}\|_2 = 0$ by choice of initialization.
Now, let $\rho\coloneqq 1 + \alpha \beta \lambda \tau - \beta \left(0.5 \alpha E_0 \mu_\ast^2 - 3  \tau \sqrt{\alpha} L_\ast^2 \right)$. We have that $\dist_s \leq \rho^s$ for all $s\in \{0,...,t\}$ by $\bigcup_{s=0}^t A_5(s)$. We also have $\gamma \leq \rho$ by choice of $\alpha,\lambda$.
Thus, for any $s\in \{0,...,t\}$, we have
\begin{align}
    \|\mathbf{I}-\alpha \mathbf{B}_{s+1}^\top \mathbf{B}_{s+1}\|_2 &\leq 10 \alpha^{2}\beta^2 L_\ast^4 \sum_{r=0}^s \gamma^{s-r} \rho^{2r} \nonumber \\
    &\leq 10 \alpha^{2}\beta^2L_\ast^4  \sum_{r=0}^s \rho^{s-r} \rho^{2r} \nonumber \\
    &= 10 \alpha^{2}\beta^2 L_\ast^4  \rho^s \sum_{r=0}^s \rho^r \nonumber \\
    &\leq  \rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1-\rho} \nonumber \\
    &=: {z}_s
\end{align}
% Now, suppose that $\|\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\|_2 \leq L_\ast$ for all $t$ with high probability. Let $a_t \coloneqq \|\mathbf{w}_t\|_2$ for all $t$.
Now, applying \eqref{forall} recursively for $s=t,t-1,\dots,0$ and plugging in the definition of $z_s$ yields
\begin{align}
    a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
    &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} {z}_{t-1})(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_{t-1} L_\ast(1 + \tfrac{2\beta}{\alpha} {z}_t)  + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
    &\;\; \vdots \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t {z}_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
    &=  \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t z_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
    &= \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t \rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1- \rho}\prod_{r=s+1}^t(1+ \rho^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1- \rho}) \nonumber \\
    &= \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast \sum_{s=0}^t \rho^{s} \prod_{r=s+1}^t\left(1+ \rho^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - \rho}\right) \nonumber
\end{align}    
where the first equality follows under the assumption that $a_0 = 0$. By the AM-GM inequality and sum of geometric series, we have, for $s\leq t-1$,
\begin{align}
    \prod_{r=s+1}^t\left(1+ \rho^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1 - \rho}\right) &\leq \left(1 + \tfrac{1}{t-s} \sum_{r=s+1}^t \rho^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - \rho}\right)^{t-s} \nonumber \\
    &\leq \left(1 + \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3\rho^{s+1}L_\ast^4 }{(1- \rho)^2} \right)^{t-s} 
\end{align}
The RHS is monotonically increasing in $t$ (since each additional $t$ means multiplication by a number greater than 1) so we can upper bound it by its limit as $t \rightarrow \infty$. This limit is 
% $\exp\left(\left(1 + \tfrac{1}{t-s+1} \tfrac{\sqrt{\alpha}\beta^3\rho^{2}}{(1- \rho)^2} \right)^{t-s-1} \right) $, where the exponent is less than 1 for sufficiently small $\alpha, \beta$. For general $s$, the RHS limit is 
$\exp\left( {20} \tfrac{{\alpha}\beta^3\rho^{s+1}}{(1- \rho)^2} \right)$ (note that it is of the form $\lim_{t\rightarrow \infty} (1+\tfrac{a}{x})^x$). To ensure this exponent is less than 1, we can choose
\begin{align}
  {20\alpha}\beta^3 L_\ast^4  &\leq   (1- \rho)^2 \nonumber \\
  \iff {20\alpha}\beta^3 L_\ast^4 &\leq   \alpha^2 \beta^2 \nonumber \\
  \iff \beta &\leq \alpha/(20 L_\ast^4).
\end{align}
Under this condition on $\beta$, we have
\begin{align}
    a_{t+1} &\leq \tfrac{20 \alpha^{1.5}\beta^3L_\ast^4 }{1 - \rho} L_\ast\sum_{s=1}^{t-1} \rho^{s} \exp\left( \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3\rho^{s+1}L_\ast^4 }{(1- \rho)^2} \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - \rho} L_\ast \rho^{t} \nonumber \\
    &\leq \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast\sum_{s=1}^{t-1} \rho^{s}\left(1+ \tfrac{2\rho^{s+1}}{t-s} \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - \rho} L_\ast \rho^{t} \nonumber \\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast\sum_{s=1}^{t} \rho^{s} \nonumber \\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{(1 - \rho)^2} L_\ast \nonumber \\
    &\leq  L_\ast
\end{align} 
where the second inequality follows from the numerical inequality $e^x \leq 1+2x$ for $x\in [0,1]$, and the last inequality follows for $\beta \leq\alpha/(60 L_\ast^4).$



% -----------------
% \begin{align}
%   \left\| (\mathbf{I}-\alpha\mathbf{B}_s^\top \mathbf{B}_s)\frac{\beta \alpha}{n}\sum_{i=1}^n \mathbf{B}_s^\top \mathbf{B}_s \mathbf{B}_s^\top(\mathbf{I}_d - \mathbf{\Sigma}_{s,i}^{in})(\mathbf{B}_s \mathbf{w}_s - \mathbf{B}_\ast \mathbf{w}_{\ast,s,i}) \right\|_2 &\leq \tfrac{\beta}{\alpha}b_s \delta_{in} a_s + \tfrac{\beta}{\sqrt{\alpha}}b_s \delta_{in} L_\ast \nonumber 
%   \end{align}
%   \begin{align}
%   \Bigg\|(\mathbf{I}-&\alpha\mathbf{B}_s^\top \mathbf{B}_s)\frac{ \beta}{n}\sum_{i=1}^n\mathbf{B}_s^\top (\mathbf{I}_d - \mathbf{\Sigma}_{s,i}^{out})(\mathbf{B}_s \mathbf{w}_{s,i} -\mathbf{B}_\ast \mathbf{w}_{\ast,s,i} ) \Bigg\|_2 \nonumber \\
%   &\leq \frac{\beta}{\alpha}\tau_2\delta_{out}\max_{i\in[n]}\|\mathbf{w}_{s,i}\|_2 +\frac{\beta}{\sqrt{\alpha}}\tau_2\delta_{out}L_{\max} \nonumber \\
%   &\leq \frac{\beta}{\alpha}\tau_2\delta_{out}(\|\mathbf{I}_k\!-\!\alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2 a_s\!+\!\sqrt{\alpha} L_{\max} + \delta_{in}a_s\!+\!\sqrt{\alpha} \delta_{in} L_{\max})\!+\!\frac{\beta}{\sqrt{\alpha}}\delta_{out}L_{\max} \nonumber \\
%   &\leq  \frac{\beta}{\alpha}\tau_2 \delta_{out}(\tau_2 a_s +  \delta_{in}a_s+ \sqrt{\alpha}L_{\max}) +\frac{\beta}{\sqrt{\alpha}}\delta_{out}L_{\max} \nonumber  \\
%   \Bigg\|\frac{\beta \alpha}{n}&\sum_{i=1}^n (\mathbf{B}_s^\top \mathbf{B}_s - \mathbf{B}_s^\top \mathbf{\Sigma}_{t,i}^{out} \mathbf{B}_s) \mathbf{B}_s^\top \mathbf{B}_s(\mathbf{I}- \alpha\mathbf{B}_s^\top \mathbf{B}_s)\mathbf{w}_s \Bigg\|_2 \nonumber \\
%   &\leq \frac{\beta}{\alpha}\tau_2 \sqrt{\tau_1} \delta_{out} 
% \end{align}
% with probability at least $1-6n^{-99}$.
% {\color{blue} For Exact ANIL, we have 
% \begin{align}
%     a_{s+1} &\leq a_s + \frac{\beta}{\sqrt{\alpha}}\tau_s^2 \eta_\ast + \frac{\beta}{{\alpha}}\tau_s(\delta_{in}+\delta_{out}(\tau_s +  \delta_{in})a_s + \frac{\beta}{\sqrt{\alpha}}\tau_s\delta_{out}(\dist_s + \tau_s  +\sqrt{\alpha}\delta_{in})  L_\ast  \nonumber \\
%     &\quad + \frac{\beta}{\alpha}\tau_s \delta_{H}(a_s + \sqrt{\alpha} L_\ast)+ \frac{\beta }{\alpha}\delta_{H} \delta_{in} (a_s+\sqrt{\alpha} L_\ast) + \frac{\beta}{\alpha} \delta_{H}(\tau_s a_s +\delta_{in} a_s +\dist_s L_\ast + \tau_s L_\ast + \sqrt{\alpha}\delta_{in}L_\ast) \nonumber 
% \end{align}
% why do stochastic processes with mean zero noise not diverge? besides azuma hoeffding
% we have terms with no $a_s$ and no $\tau_s$, and these terms are not summable
% }


% Using this fact with \eqref{uuu}, we obtain
% \begin{align}
%     a_{s+1} &\leq \left(1 + (2+\delta_{out})\tfrac{\beta}{\alpha} \|\mathbf{I}_k - \alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2 + \frac{\beta}{\alpha}\delta_{in}\right)a_s + \tfrac{2\beta}{\sqrt{\alpha}} \|\mathbf{I}_k - \alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2 L_\ast \nonumber \\
%     &\quad + \frac{\beta}{\sqrt{\alpha}} (\delta_{in}+\delta_{out}) L_\ast
%     \label{foralll}
% \end{align}  

    %\nonumber \\
    % &\leq a_0\prod_{s=1}^t(1+\tfrac{\beta}{\alpha}{z}_s) +\tfrac{\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t {z}_s\prod_{r=s+1}^t(1+ \tfrac{\beta}{\alpha}z_r) \nonumber \\
    % &=  \tfrac{\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t z_s\prod_{r=s+1}^t(1+ \tfrac{\beta}{\alpha}z_r) \nonumber \\
    % &= \tfrac{\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t \rho^{s} \tfrac{\alpha^{2}\beta^2 L_\ast^4 }{1- \rho}\prod_{r=s+1}^t(1+ \rho^{r} \tfrac{{\alpha}\beta^3L_\ast^4 }{1- \rho}) \nonumber \\
    % &= \tfrac{\alpha^{1.5}\beta^3 L_\ast^4 }{1 - \rho} L_\ast \sum_{s=0}^t \rho^{s} \prod_{r=s+1}^t\left(1+ \rho^{r} \tfrac{{\alpha}\beta^3L_\ast^4 }{1 - \rho}\right) \nonumber

% {\color{blue} In the exact ANIL case, we have 
% \begin{align}
%     a_{s+1} &\leq (1+)
% \end{align}
% }
% {\color{red} We have problems because the $\delta$'s are not summable....}

% for all $s\in\{0,\dots,t\!+\!1\}$.

% Letting $s \equiv t$ and substituting  $\mathbf{w}_{s,i} = (\mathbf{I}_k  - \alpha \mathbf{B}_s^\top \mathbf{B}_s )\mathbf{w}_s + \alpha \mathbf{B}_s^\top \mathbf{B}_{\ast} \mathbf{w}_{\ast,s,i} +\alpha \mathbf{B}_s^\top(\mathbf{I}_d - \mathbf{\Sigma}_{s,i}^{in})(\mathbf{B}_s \mathbf{w}_s - \mathbf{B}_\ast \mathbf{w}_{\ast,s,i})$, we have 
% \begin{align}
% \mathbf{w}_{s+1}
% &= (\mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha\mathbf{B}_s^\top \mathbf{B}_s) \mathbf{B}_s^\top \mathbf{B}_s)\mathbf{w}_s +
% \beta (\mathbf{I}- \alpha\mathbf{B}_s^\top \mathbf{B}_s)\mathbf{{B}}_s^\top \mathbf{{B}}_\ast \frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,s,i}  \nonumber \\
% &\quad - \frac{\beta \alpha}{n}\sum_{i=1}^n \mathbf{B}_s^\top \mathbf{B}_s \mathbf{B}_s^\top(\mathbf{I}_d - \mathbf{\Sigma}_{t,i}^{in})(\mathbf{B}_s \mathbf{w}_s - \mathbf{B}_\ast \mathbf{w}_{\ast,s,i}) \nonumber \\
% &\quad + \frac{ \beta}{n}\sum_{i=1}^n\mathbf{B}_s^\top (\mathbf{I}_d - \mathbf{\Sigma}_{t,i}^{out})(\mathbf{B}_s \mathbf{w}_{s,i} -\mathbf{B}_\ast \mathbf{w}_{\ast,s,i} ) 
% \end{align}



% In this section we discuss our main results. We start by analyzing ANIL.



% Starting from initialization $\mathbf{w}_t$, the inner loop update for the $i$-th task on iteration $t$ is given as follows. For ease of notation we drop the iteration subscript $t$ on the data and ground-truth heads.
% \begin{align}
%     \mathbf{w}_{t,i} %&= \mathbf{w}_t - \alpha \mathbf{\hat{B}}_t^\top \sum_{j=1}^{m_{in}}\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \mathbf{\hat{B}}_t \mathbf{{w}}_t  + \alpha \mathbf{\hat{B}}_t^\top \frac{1}{m_{in}}\sum_{j=1}^{m_{in}}\mathbf{x}_{i,j}\mathbf{x}_{i,j}^\top \mathbf{\hat{B}}_\ast \mathbf{{w}}_{\ast,i} \nonumber \\
%     &= \mathbf{w}_t - \alpha \nabla_{\mathbf{w}} \hat{f}_i(\mathbf{B}_t, \mathbf{w}_t, \mathcal{D}_{i}^{in}), \label{upd_head_anil_in_gen}% =  (\mathbf{I}_k- \alpha\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i}^{in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i}^{in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} + \frac{\alpha}{m_{in}} \mathbf{\hat{B}}_t^\top \mathbf{X}_{i}^{in}\mathbf{z}_{i}^{in}. \label{upd_head_anil}
% \end{align}
% while the outer loop updates are:
% \begin{align}
% \mathbf{w}_{t+1} &= \mathbf{w}_t - \frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{w}} \hat{f}_i(\mathbf{\hat{B}}_t, \mathbf{w}_{t,i}) \label{upd_head_anil_out_gen}\\
% % &= \label{upd_head_out_anil} \\
%     \mathbf{{B}}_{t+1} &= \mathbf{\hat{B}}_t  - \frac{\beta}{n}\sum_{i=1}^n\nabla_{\mathbf{B}}\hat{f}_i(\mathbf{\hat{B}}_t, \mathbf{w}_{t,i}, \mathcal{D}_{i}^{out}) \label{upd_rep_anil_gen} \\
%     \mathbf{\hat{B}}_{t+1}, \mathbf{R}_{t+1} &= \text{QR}(\mathbf{\bar{B}}_{t+1})
% \end{align}

% {\color{red} need to show heads stay within convex hull
% }

% \subsection{Main Result}

% \begin{thm} \label{thrm:anil}
% Let $\delta_{in} = O\left( \frac{\sqrt{k} + 10\sqrt{\log(n)}}{\sqrt{m_{in}}}\right)$, $\delta_{out} = O\left( \frac{\sqrt{d}}{\sqrt{n m_{out}}}\right)$, and $\delta_{out}' = O\left( \frac{\sqrt{k}}{\sqrt{n m_{out}}}\right)$. Choose $\beta \leq 1/(L_{\max}^2(2\delta_{in}+1)^2)$ and $\alpha=1$. Then
% \begin{align}
%     \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast ) &\leq \frac{1 - \beta E_0\mu_\ast^2 + 4\beta L_{\max}^2 (\delta_{in}+\delta_{in}^2) ) + \beta L_{\max}^2 \delta_{out}(1+\delta_{in})}{\sqrt{1 - 2 \beta L_{\max}^2 \delta_{in} (1+2\delta_{in}) - 2\beta \delta_{out}'(1+2\delta_{in})^2  L_{\max}^2 \left( 1 - \beta \mu^2 + \beta L_{\max} L \right) }}\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) \nonumber \\
%     &\quad + \frac{2\beta L_{\max}^2 \delta_{out}\delta_{in} (1+ \delta_{in})}{\sqrt{1 - 2 \beta\delta_{in} L_{\max}^2 (1+2\delta_{in}) - 2\beta L_{\max}^2  \delta_{out}' (1+2\delta_{in})^2  \left( 1 - \beta \mu^2 + \beta L_{\max}L \right) }},
% \end{align}
% where $L \leq \sqrt{  L_{\max}^2 (2\delta_{in}+1)^2}$ and $\mu^2 \geq \mu_\ast^2 E_0 - 4 L_{\max}^2 (\delta_{in} + \delta_{in}^2)$, all
% with probability at least $1- 4n^{-99} - 2e^{-100k} - 2e^{-100d}$. 
% \end{thm}


by using $\tau_1 = \tau_2$ and 
 $\tau_1 \alpha^{7/2} \tilde{L}_\ast^2 \leq \tau_2 \sqrt{\alpha}L_\ast^2$.


-- we need $\beta \leq \alpha^{1.5}$. unless we can choose $\tau_1=\tau_2=\alpha^2$, but there is one condition for w that is not satisfied

the bad dist term in w can be fixed with the same trick we used for del

% but still we must choose tau1 = alpha2.5

major issue with w bc alpha 7/2 --> alpha3/2

current issues:

empirically, in the worst case (large eta) we have $\tau_1 = \alpha$ and $\tau_2 = \alpha^2$. But, analytically these values do not work, because the error terms are larger than the contracting terms by factors of condition number. So we may grow by factors of condition number on each iteration. 

But we cannot choose tau1 < alpha because we cannot guarantee w will stay smaller than rt(alpha). Meanwhile, we cannot choose tau1 >= alpha because this will cause tau2 to blow up (in the case that tau1 = alpha, the best we can do is choose tau2 = alpha2, but this will cause blow up do to condition number). So nothing works...

Tried recombining terms to kill more of them. Empirically, when eta is small, w and del are very small, and almost the same. Otherwise, when eta is large, w is larger than del and approaches rt(alpha). 

strangest thing is that ||w|| can become greater than 1 when d and k are large, regardless of n and alpha, but it never blows up.
whereas for FO-ANIL, this is not true. as long as n is sufficiently large, ||w|| is controlled by alpha.
this suggests that we cannot get an upper bound on w that relies on alpha or n. but how else can we bound it? are we sure that it converges? yes, it does for large n.

need to lower bound sigma min BT e0

and need tighter bound on w

if we can show that tau1 is a little bit less than alpha, we're done... we need this

tau1 stays less than alpha times cond number - that's fine

tau2 stays less than alpha2 times more cond number - that's fine but we need sigma min(sum Bw - Bstar wistar) to be lower bounded 

the contraction rate of tau2 does matter because the un-aided tau1 term. Otherwise tau2 would grow as beta alpha2 tau1 T.

somehow norm of Bw is way larger than mu even though sigma min of dif is still lower bounded 

empirically, when mean is zero, large n, tau1 scales with alpha2, tau2 scales with alpha2 as long as alpha is small, then it becomes alpha. tau1 and tau2 both scale with beta

how can tau1 scale with alpha2???

but constant for tau2 is much smaller, not sure why. 

Neither tau1 nor tau2 scales with condition number unless cond number is very large,


but when mean is nonzero, relationship between tau1, tau2 and alpha is non-monotonic:
large alpha: rt(tau1)=tau
medium alpha: rt(tau1) = 10x rt(tau1) for large alpha
              tau2 = 0.1x tau2 for large alpha
small alpha: rt(tau1) = rt(tau1) for large alpha
              tau2 = 0.001x tau2 for large alpha
smaller alpha: rt(tau1) = 0.1x rt(tau1) for large alpha
              tau2 = 0.00001x tau2 for large alpha              

when kappa is large but mean is zero (small n):
tau1, tau2 both scale as alpha2





\begin{lemma}
control max
\end{lemma}

\begin{proof}
 We have 
 \begin{align}
     m_{t+1} &\leq (1 - \beta \alpha^3 E_0 \tilde{\mu}_\ast^2)m_t + \dist_t^2 \nonumber \\
     &\leq \sum_{s=1}^t  (1 - \beta \alpha^3 E_0 \tilde{\mu}_\ast^2)^{t-s}\dist_s^2 \nonumber \\
     &\leq  \sum_{s=1}^t  (1 - \beta \alpha^3 E_0 \tilde{\mu}_\ast^2)^{t-s} q^{2s} \nonumber \\
     &\leq (1 - \beta \alpha^3 E_0 \tilde{\mu}_\ast^2)^t \sum_{s=1}^t  (1 - \beta \alpha E_0 {\mu}_\ast^2)^{s}
     \nonumber\\
     &\leq \frac{(1 - \beta \alpha^3 E_0 \tilde{\mu}_\ast^2)^t}{\beta \alpha E_0 \tilde{\mu}_\ast^2}
 \end{align}
 
how to fix this... need dist2
unless (1-beta alpha)/(1 - beta alpha3) works
it almost works... but not quite because wt+1 is not less than tau1


\end{proof}


\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\begin{lemma}
For exact MAML, suppose that $\|\mathbb{E}[\mathbf{w}_{\ast,t,i}]\|_2 \leq C$ for some absolute constant $C$, $\mathbf{w}_0 = \mathbf{0}$, $\alpha$ and $\beta$ are sufficiently small, and $1 - \dist_0^2 \geq 0.5$. Then for all $t\leq \tfrac{c}{\beta \alpha^{2.75}}$,
\begin{align}
    \|\mathbf{w}_t \|_2^2 \leq \tau_1
\end{align}
with high probability.
\end{lemma}
\begin{proof}
\begin{align}
    \mathbf{w}_{t+1} &= \left(\mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\left(\frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\right)(\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t}) \right)\mathbf{w}_t \nonumber \\
    &\quad  + \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\frac{1}{n}\sum_{i=1}^n \mathbf{{B}}_{t,i}^\top  (\mathbf{I}- \alpha\mathbf{B}_{t,i} \mathbf{B}_{t}^\top) \mathbf{{B}}_\ast \mathbf{w}_{\ast,t,i} \nonumber  \\
    &= \left(\mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\left(\frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\right)(\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t}) \right)\mathbf{w}_t \nonumber \\
    &\quad + \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\frac{1}{n}\sum_{i=1}^n \mathbf{{B}}_{t,i}^\top  (\mathbf{I}- \alpha\mathbf{B}_{t} \mathbf{B}_{t}^\top) \mathbf{{B}}_\ast \mathbf{w}_{\ast,t,i} \nonumber  \\
    &\quad + \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\frac{1}{n}\sum_{i=1}^n \mathbf{{B}}_{t,i}^\top  \alpha^2(\mathbf{B}_{t}\mathbf{w}_t\mathbf{w}_t^\top -\mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top)\mathbf{B}_{t}^\top \mathbf{{B}}_\ast \mathbf{w}_{\ast,t,i} \nonumber 
\end{align}
Note that due to the second-order update, the coefficient of $\mathbf{w}_t$ has spectral norm at most one as long as $\beta$ is sufficiently small, since $(\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\left(\frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\right)(\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})$ is PSD. Using this along with $\|\del_t\|_2 \leq \tau_2$.
Thus
\begin{align}
    \|\mathbf{w}_{t+1}\| &\leq
\|\mathbf{w}_t\|_2  + \frac{\beta}{\sqrt{\alpha}}  \tau_2^2 \eta_\ast + \beta \alpha \|\mathbf{w}_t\|_2\tau_2(\dist_t +\tau_2)L_{\max}^2 + \beta \tau_2 c\frac{1}{\sqrt{\alpha}} \alpha^2\left(\frac{\|\mathbf{w}_t\|_2^2}{{\alpha}}\eta_\ast  +  \frac{\|\mathbf{w}_t\|_2}{\sqrt{\alpha}} L_\ast^2 \right)  \nonumber \\
&\quad + \beta \alpha^3 \tau_2 \tau_1^{3/2} \frac{L_\ast^2}{\alpha} + \beta \alpha^3 \tau_2 \tau_1 L_{\max}^3 \frac{1}{\sqrt{\alpha}} \nonumber \\
&\leq \|\mathbf{w}_t\|_2  + \frac{\beta}{\sqrt{\alpha}}  \tau_2^2 \eta_\ast + \beta \alpha \|\mathbf{w}_t\|_2\tau_2(\dist_t +\tau_2)L_{\max}^2 + \beta \tau_2 \alpha^{0.5} \|\mathbf{w}_t\|_2^2 \eta_\ast +\beta \tau_2 \alpha \|\mathbf{w}_t\|_2 L_\ast^2
% \beta \tau_2 \frac{1}{\sqrt{\alpha}} \alpha^2\left(\frac{\|\mathbf{w}_t\|_2^2}{{\alpha}}\eta_\ast  +  \frac{\|\mathbf{w}_t\|_2}{\sqrt{\alpha}} L_\ast^2 \right)  
\nonumber \\
&\quad + \beta \alpha^2 \tau_2 \tau_1^{3/2} {L_\ast^2} + \beta \alpha^{2.5} \tau_2 \tau_1 L_{\max}^3 \nonumber \\
&\leq \|\mathbf{w}_t\|_2  + \frac{\beta}{\sqrt{\alpha}}  \tau_2^2 \eta_\ast + \beta \alpha \sqrt{\tau_1} \tau_2 L_{\max}^2 + \beta {\sqrt{\alpha}} \tau_2 \tau_1 \eta_\ast +\beta \alpha \tau_2\sqrt{\tau_1}L_\ast^2   \nonumber \\
&\quad  + \beta \alpha^2 \tau_2 \tau_1^{3/2} {L_\ast^2} + \beta \alpha^{2.5} \tau_2 \tau_1 L_{\max}^3  \nonumber 
% &----\nonumber \\
% &\leq \|\mathbf{w}_t\|_2 + \frac{\beta}{\sqrt{\alpha}}  \tau_2^2 \eta_\ast  + \beta \tau_2 c\alpha  \left(\frac{\|\mathbf{w}_t\|_2^2}{\sqrt{\alpha}} + L_\ast \|\mathbf{w}_t\|_2\right) \eta_\ast \nonumber \\
% &\leq \|\mathbf{w}_t\|_2+ \frac{\beta}{\sqrt{\alpha}} \tau_2^2 \eta_\ast  + \beta \tau_2 c \alpha^{2} \eta_\ast + \beta \tau_2 c \alpha^{1.75} L_\ast \eta_\ast \nonumber \\
% &\leq \|\mathbf{w}_t\|_2+ {\beta}\alpha^{3.5}\eta_\ast  + c\beta  \alpha^{4} \eta_\ast + c \beta  \alpha^{3.75} L_\ast \eta_\ast \nonumber \\
% % &\leq \|\mathbf{w}_t\|_2+ c \frac{\beta}{\sqrt{\alpha}} \tau_2^2 \eta_\ast  \nonumber \\
% &\leq \|\mathbf{w}_t\|_2 + c{\beta}\alpha^{3.5}\eta_\ast \max(L_\ast,1)\nonumber \\
% &\leq c \beta \alpha^{3.5}\eta_\ast \max(L_\ast,1) t 
\end{align}
{\color{red} note: we can tighten $L_{\max}^3$ using assumption on third moment, since this term is proportional to $\frac{1}{n}\sum_{i=1}^n\|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{\ast,t,i}$, but leave as is for now.

the dominant terms in the above eqn are $\frac{\beta}{\sqrt{\alpha}}  \tau_2^2 \eta_\ast$ and $\beta \alpha \sqrt{\tau_1} \tau_2 L_{\max}^2$, use this to get final bound}
\end{proof}











--------------

% 10/28: still not clear how to bound $\|\mathbf{w}_t\|$. We can't use argument from FO-MAML case because we don't have any contraction term. We can't use argument from ANIL case because $\Delta_t$ is not going to zero (because here, upper bound on $\Delta_t$ relies on a term with only $\|\mathbf{w}_t\|$...)
% The update is:
% \begin{align}
%     \mathbf{w}_{t+1} &= \left(\mathbf{I}_{k}\! - \! \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\left(\frac{1}{n}\sum_{i=1}^n\mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\right)(\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t}) \right)\mathbf{w}_t \nonumber \\
%     &\quad \quad + \beta (\mathbf{I}- \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t})\frac{1}{n}\sum_{i=1}^n \mathbf{{B}}_{t,i}^\top  (\mathbf{I}- \alpha\mathbf{B}_{t,i} \mathbf{B}_{t}^\top) \mathbf{{B}}_\ast \mathbf{w}_{\ast,t,i} \nonumber  \\
%     &\approx \mathbf{w}_t - \beta (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t)^2 (\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t - \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}) \nonumber
% \end{align}
% where the approximation is due to $\mathbf{B}_{t,i}\approx\mathbf{B}_t$.
% Thus
% \begin{align}
%     \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_{t+1} -\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}  &\approx (\mathbf{I}_k - \beta PSD)(\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_{t} -  \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast} ) \nonumber \\
%     \implies \|\mathbf{w}_{t+1}\|_2 &\leq \alpha (\tfrac{1}{\alpha}a_t + \tfrac{1}{\sqrt{\alpha}}c) + \sqrt{\alpha}c = a_t + 2\sqrt{\alpha} c
% \end{align}
% We also have 
% \begin{align}
%     \|\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}\|_2 &\leq \tau \nonumber \\
%     \implies \|\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \mathbf{w}_{t+1} - \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}  \|_2 &\leq \|\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \mathbf{w}_{t+1} -  \mathbf{B}_{t}^\top \mathbf{B}_{t} \mathbf{w}_{t+1}\|_2 +  \| \mathbf{B}_{t}^\top \mathbf{B}_{t} \mathbf{w}_{t+1} - \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}  \|_2 \nonumber \\
%     &\leq 2 \tfrac{\tau}{\alpha}a_{t+1} +  \| \mathbf{B}_{t}^\top \mathbf{B}_{t} \mathbf{w}_{t} - \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}  \|_2
% \end{align}

% \begin{align}
%     \|\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \mathbf{w}_{t+1} - \mathbf{B}_{t+1}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}\|_2 &\leq 1/\sqrt{\alpha} \|\alpha\mathbf{B}_{t+1}\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \mathbf{w}_{t+1} - \alpha\mathbf{B}_{t+1}\mathbf{B}_{t+1}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}\|_2 \nonumber \\
%     &= 1/\sqrt{\alpha} \|\alpha \mathbf{B}_{t+1}\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \mathbf{w}_{t+1} - \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}\| +  \|(\mathbf{I}_k - \alpha\mathbf{B}_{t+1}\mathbf{B}_{t+1}^\top) \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}\|_2 \nonumber \\
%     &\leq \|\|_2  +   \dist_t + \tau
% \end{align}
% suppose $\|\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t - \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{\bar{w}}_\ast\|_2 \leq \tau_3$, which is approx equivalent to $\| \mathbf{B}_t \mathbf{w}_t -  \mathbf{B}_\ast\mathbf{\bar{w}}_\ast\|_2 \leq \sqrt{\alpha}\tau_3$. Then $\|\mathbf{w}_{t+1}-\mathbf{w}_t\|_2\leq \beta \tau_2^2 \tau_3$. 
% So, 
% \begin{align}
%     \|\mathbf{B}_{t+1} \mathbf{w}_{t+1} - \mathbf{B}_\ast \mathbf{\bar{w}}_\ast\|_2 &\leq \|\mathbf{B}_{t+1} \mathbf{w}_{t+1} - \mathbf{B}_{t+1} \mathbf{w}_{t} \|_2+ \|\mathbf{B}_{t+1} \mathbf{w}_{t}   - \mathbf{B}_\ast \mathbf{\bar{w}}_\ast\|_2 \nonumber \\
%     &\leq 
% \end{align}
% first term is less than $\tau_3$ is the second as well?
% but we don't know that this is true even for the best case update for $\mathbf{B}$... 
% also, this is not the right pop update if we don't have different samples for the hessian
% experimentally: wt is decreasing when it is large and increasing when it is small
% we have increase on every iteration, and the increase is not summable. but it is still negligible
% Let $a_t= c+ \epsilon t$ for $ t\leq T$
% hard part is showing that first $a_t$ may grow significantly  but not more than a constant $c$, then afterwards it only grows by very small amount $\epsilon$. need to study dynamics of $\tau$. summation argument from earlier should work...



\begin{lemma} \label{lem:maml_ind22}
Suppose that $A', A_1(t)$,$A_2(t)$ and $A_4(t)$ hold for $\tau_1 = c\alpha$ and $\tau_2 = c \alpha^2$. Then $A_2(t+1)$ holds almost surely, i.e.
\begin{align}
    \|\mathbf{I}_k-\alpha\mathbf{B}_t^\top \mathbf{B}_t\|_2\leq {\tau_2}.
\end{align}
\end{lemma}

\begin{proof}
    Recall the notation $\boldsymbol{\Delta}_t \coloneqq \mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t $.
    Denote the outer loop gradient for the representation as:
    \begin{align}
        {\mathbf{G}}_t &\coloneqq \frac{1}{n}\sum_{i=1}^n\left(\mathbf{B}_{t,i} \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top - \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\right)(\mathbf{I}- \alpha\mathbf{w}_t\mathbf{w}_t^\top)  \nonumber
    \end{align}
    Next, denote the inner loop gradient for the representation for the $i$-th task as:
    \begin{align}
        \mathbf{G}_{t,i} &\coloneqq \mathbf{B}_t\mathbf{w}_t \mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top 
    \end{align}
    We have
    \begin{align}
        % \mathbf{T}_{1,t,i} &= (\mathbf{I}_d -\alpha \mathbf{B}_t\mathbf{B}_t^\top) (\mathbf{B}_t \mathbf{w}_t - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}) + \alpha \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t - \alpha^2 \mathbf{G}_{t,i}\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \nonumber \\
         \mathbf{G}_{t} &= \frac{1}{n}\sum_{i=1}^n (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top)(\mathbf{B}_t \mathbf{w}_t - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top(\mathbf{I}-\alpha\mathbf{w}_t\mathbf{w}_t^\top) \nonumber \\
         &\quad + \frac{1}{n}\sum_{i=1}^n\Big( -\alpha \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top - \alpha^2 \mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top \Big)(\mathbf{I}-\alpha\mathbf{w}_t\mathbf{w}_t^\top) \label{eqbigG2}
    \end{align}
    The proof relies on showing that the terms in the second and third lines of equation \eqref{eqbigG} are small. First, we know that $\|\boldsymbol{\Delta}_t\|_2\leq \tau_2$. Next, we have
    \begin{align}
        \|\mathbf{G}_{t,i}\|_2 &\leq c\left(\frac{\tau_1}{\sqrt{\alpha}} + L_{\max}\sqrt{\tau_1} \right)
    \end{align}
    and
    \begin{align}
        \left\|\alpha\frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top\right\|_2 &\leq c\left( \tau_1^{2} \tau_2^2 \sqrt{\alpha} + \alpha \tau_1^{3/2}\tau_2 \eta_\ast + \alpha \tau_1^{3/2} \tau_2^2 \eta_\ast 
        + \alpha^{3/2} \tau_1 \tau_2 L_*^2 \right) \nonumber \\
        &\leq c' \left(\tau_1^{2} \tau_2^2 \sqrt{\alpha} + \alpha \tau_1^{3/2}\tau_2 \eta_\ast 
        + \alpha^{3/2} \tau_1 \tau_2 L_*^2 \right) \nonumber
    \end{align}
    Further,
    \begin{align}
         &\left\|\alpha^2 \frac{1}{n} \sum_{i=1}^n\mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\right\|_2 \leq c\left(\alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2 + \alpha^{3/2} \tau_1 \tau_2 L_*^2 + \alpha^2 \sqrt{\tau_1} L_{\max} L_*^2\right)
    \end{align}
    Thus,
    \begin{align}
         \mathbf{E}_t &\coloneqq \left\|\left(\alpha\frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top + \alpha^2 \frac{1}{n} \sum_{i=1}^n\mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\right)(\mathbf{I}_k - \alpha\mathbf{w}_t\mathbf{w}_t^\top)\right\|_2 \nonumber \\
         &\leq c\left(\sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2 + \alpha^{3/2} \tau_1 \tau_2 L_*^2 + \alpha^2 \sqrt{\tau_1} L_{\max} L_*^2 \right) \nonumber \\
         &\leq c'\left( \sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  \right) \nonumber 
    \end{align}
    % assuming $\tau_1^{1/2}\tau_2 \eta_\ast < \alpha^{1/2}L_\ast^2$.
    % , $\tau_2^2 \lambda < L_\ast^2$, and $ \tau_2^2 \lambda \eta_\ast < L_{\max}^3$.
Now, expanding $\mathbf{w}_{t,i}$, we have 
    \begin{align}
        \mathbf{B}_t^\top \mathbf{G}_t &= -\boldsymbol{\Delta}_t \frac{1}{n}\sum_{i=1}^n \Big(-\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_t^\top \boldsymbol{\Delta}_t(\mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top) + \alpha \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t (\mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top) \nonumber \\
        &\quad \quad \quad \quad  \quad \quad + \mathbf{B}_t^\top  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top \boldsymbol{\Delta}_t(\mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top) - \alpha \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t (\mathbf{I}_k - \alpha \mathbf{w}_t\mathbf{w}_t^\top)\Big)\nonumber \\
        &\quad + \mathbf{B}_t^\top \mathbf{E}_t \\
        &=  \alpha \boldsymbol{\Delta}_t \frac{1}{n}\sum_{i=1}^n\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  - \boldsymbol{\Delta}_t\mathbf{D}_t + \mathbf{B}_t^\top \mathbf{E}_t
    \end{align}
    where  $\mathbf{D}_t \coloneqq  \frac{1}{n}\sum_{i=1}^n \Big(\alpha^2 \mathbf{B}_t^\top \mathbf{B}_\ast  \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \mathbf{w}_t\mathbf{w}_t^\top-\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_t^\top \boldsymbol{\Delta}_t + \alpha \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \mathbf{B}_t^\top  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top \boldsymbol{\Delta}_t \Big)$, which by triangle inequality satisfies:
    \begin{align}
        \|\mathbf{D}_t\|_2 &\leq  c\left(\alpha L_\ast^2 \tau_1+ \frac{\tau_1 \tau_2}{\alpha} + \frac{\sqrt{\tau_1}\eta_\ast}{\sqrt{\alpha}}  \right) \leq c'  \left( \frac{\tau_1 \tau_2}{\alpha} + \frac{\sqrt{\tau_1}\eta_\ast}{\sqrt{\alpha}}  \right)
    \end{align}
    % for some absolute constant $c$ 
    (note that the last term is dominated). 
    We have 
    \begin{align}
        \|\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}_k\|_2
        &= \|\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t} - \mathbf{I}_k - \beta \alpha  \mathbf{B}_{t}^\top\mathbf{G}_t - \beta \alpha  \mathbf{G}_{t}^\top\mathbf{B}_t + \beta^2 \alpha \mathbf{G}_{t}^\top\mathbf{G}_t\|_2 \nonumber \\
        &\leq \|\boldsymbol{\Delta}_t\|_2 \Bigg( 1 - 2\beta \alpha^2 \sigma_{\min}\left( \frac{1}{n}\sum_{i=1}^n\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \right) + 2 \beta \alpha \|\mathbf{D}_t\|_2  \Bigg) \nonumber \\
        &\quad \quad+2 \beta \alpha \|\mathbf{B}_t^\top \mathbf{E}_t\|_2  + \beta^2 \alpha \|\mathbf{G}_t\|_2^2 \nonumber \\
        &\leq \tau_2 \Bigg( 1 - c\beta \alpha E_0 \mu_{\ast}^2 + c'\beta{\tau_1 \tau_2} + c'\beta \sqrt{\alpha \tau_1}\eta_\ast\Bigg) \nonumber \\
        &\quad +c'\bigg(\beta \alpha \tau_1^{2} \tau_2^2  + \beta \alpha^{3/2} \tau_1^{3/2} \tau_2 \eta_\ast + \beta \alpha^{2}\tau_1 L_*^2  + \beta \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3 + \beta^2 \alpha \|\mathbf{G}_t\|_2^2 \bigg) \nonumber
    \end{align}
    Finally, we have 
    \begin{align}
        \|\mathbf{G}_t\|_2 &\leq \left\|\frac{1}{n}\sum_{i=1}^n\Big( (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top)(\mathbf{B}_t \mathbf{w}_t - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top  \Big)(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top) \right\|_2 + \|\mathbf{E}_t\|_2 \nonumber \\
        &\leq \frac{\tau_1 \tau_2^2}{\sqrt{\alpha}}  + \sqrt{\tau_1}\tau_2 \eta_\ast + L_\ast^2 \sqrt{\alpha}\dist_t + \sqrt{\tau_1}\tau_2 \eta_\ast \dist_t + L_\ast^2 \sqrt{\alpha} \tau_2 + \sqrt{\tau_1} \tau_2^2 \eta_\ast \nonumber \\
        &\quad + \sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2}\tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  \nonumber \\
         &\leq \frac{\tau_1 \tau_2^2}{\sqrt{\alpha}} +  \sqrt{\tau_1}\tau_2 \eta_\ast+ \alpha \tau_1^{3/2}\tau_2 \eta_\ast + L_\ast^2 \sqrt{\alpha}\dist_t  +  \sqrt{\alpha} \tau_2 L_\ast^2   +  \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  \nonumber
    \end{align}
    assuming $\sqrt{\tau_1}\tau_2 \eta_\ast \leq L_\ast^2\sqrt{\alpha}$ ({\color{red} which is true by our choice of parameters but only slightly so we should not drop this}),
    using similar analysis as in the proof for ANIL, noting that the matrix in the RHS of the first equation is equivalent to $\mathbf{G}_t$ from the ANIL case.
    Thus
    \begin{align}
     \|\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}_k\|_2 
        &\leq \tau_2 \Bigg( 1 - c\beta \alpha E_0 \mu_{\ast}^2 + c'\beta{\tau_1 \tau_2} + c'\beta \sqrt{\alpha \tau_1}\eta_\ast\Bigg) \nonumber \\
        &\quad +c'\bigg(\beta \alpha \tau_1^{2} \tau_2^2  + \beta \alpha^{3/2} \tau_1^{3/2} \tau_2 \eta_\ast + \beta \alpha^{2}\tau_1 L_*^2  + \beta \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3  \bigg) \nonumber \\
      &\quad + \beta^2 \tau_1^2 \tau_2^4 + \beta^2 \alpha \tau_1 \tau_2^2 \eta_\ast^2 + \beta^2 \alpha^2 \tau_2^2 L_\ast^4 + \beta^2 \alpha^{4}\tau_1^2  L_\ast^4 \nonumber \\
      &\quad + \beta^2 \alpha^5 \tau_1 L_{\max}^6 + \beta^2 \alpha^2\tau_1^3\tau_2^2 \eta_\ast^2   +\beta^2 \alpha^2 L_\ast^4 \dist_t^2 \bigg) \nonumber \\
      &\leq \tau_2 \Bigg( 1 - c'\beta \alpha E_0 \mu_{\ast}^2 + c\beta{\tau_1 \tau_2} + c\beta \sqrt{\alpha \tau_1}\eta_\ast  \Bigg)  + c\beta \alpha^{2}\tau_1 L_*^2  + c\beta \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3 \nonumber \\
      &\quad + c\beta^2 \tau_1^2 \tau_2^4 + c\beta^2 \alpha \tau_1 \tau_2^2 \eta_\ast^2 + c \beta^2 \alpha^3 \tau_1^3 \tau_2^2 \eta_\ast^2 + c\beta^2 \alpha^2 \tau_2^2 L_\ast^4 + c\beta^2 \alpha^2 L_\ast^4 \dist_t^2 + c\beta^2 \alpha^4 \tau_1^2 L_\ast^4 + c\beta^2\alpha^5\tau_1 L_{\max}^6
      \end{align}
    For this to stay less than $\tau_2$, we need to choose 
    \begin{align}
       0< \beta \leq \frac{c'
       \alpha \tau_2  E_0 \mu_{\ast}^2 - c {\tau_1 \tau_2^2}- c \tau_2 \sqrt{\alpha \tau_1}\eta_\ast -c \alpha^{2}\tau_1 L_*^2  - c \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3 }{c\tau_1^2 \tau_2^4 + c\alpha \tau_1 \tau_2^2 \eta_\ast^2 + c  \alpha^3 \tau_1^3 \tau_2^2 \eta_\ast^2 + c \alpha^2 \tau_2^2 L_\ast^4 + c\alpha^2 L_\ast^4 \dist_0^2 + c \alpha^4 \tau_1^2 L_\ast^4 + c\alpha^5\tau_1 L_{\max}^6} \label{beta_req}
    \end{align}
    Note that this implies we need:
    \begin{align}
        \tau_1 \tau_2 &\leq \alpha E_0 \mu_\ast^2 \label{req1} \\
        \tau_1 \eta_\ast^2 &\leq \alpha E_0^2 \mu_\ast^4  \label{req2}  \\
        \alpha \tau_1 L_*^2 &\leq \tau_2 E_0 \mu_\ast^2   \label{req3} \\
        \alpha^{3/2} \sqrt{\tau_1} L_{\max}^3 &\leq \tau_2 E_0 \mu_\ast^2 \label{req4} 
    \end{align}
    % Let  $\tau_1 = \mu_\ast^{5/2} \alpha^{3/2}$ and $\tau_2 = \alpha^2$, $\alpha = 1/L_{\max}$, $\beta = 1/L_\ast$ and note that this assignment satisfies requirements \eqref{req1} thru \eqref{req4}.
    % % we could take $\tau_2$ to be arbitrarily small, then T could be arbitrarily large, but $\beta$ would have to be arbitrarily small.
    % Also, from earlier we have $ \tfrac{\beta}{\sqrt{\alpha}}\tau_2^2 \eta_\ast T \leq \sqrt{\tau_1}$. Plugging in our definitions of $\tau_1$ and $\tau_2$, we obtain that for all $T \leq c \frac{1}{\beta \alpha^{11/4}\eta_\ast}$, we have 
    % \begin{align}
    %     \dist_{T} \leq (1- c \beta \alpha E_0\mu_\ast^2)^{T}
    % \end{align}
    % for $\beta, \alpha$ sufficiently small.
    
    \end{proof}
    
    
    
      Further, for any $i \in [n]$, we have
    \begin{align}
      \mathbf{I}_k - \alpha \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}
        &= \mathbf{I}_k - \alpha  \mathbf{B}_{t}^\top \mathbf{B}_{t} + \alpha^2 \mathbf{B}_{t}^\top \mathbf{G}_{t,i} + \alpha^2 \mathbf{G}_{t,i}^\top \mathbf{B}_{t} - \alpha^3 \mathbf{G}_{t,i}^\top \mathbf{G}_{t,i}  \nonumber \\
        &= \boldsymbol{\Delta}_{t} + \alpha^2 \mathbf{B}_{t}^\top (\mathbf{B}_t \mathbf{w}_t\mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top ) + \alpha^2 (\mathbf{B}_t \mathbf{w}_t\mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top)^\top \mathbf{B}_{t} - \alpha^3 \mathbf{G}_{t,i}^\top \mathbf{G}_{t,i}  \nonumber 
    \end{align}
    Thus
    \begin{align}
        \left\|\frac{1}{n}\mathbf{I}_k - \alpha \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\right\|_2 &\leq 
        %(1 
        % - 2 \alpha^2 \lambda (1 - \tau_2))
        \tau_2
        + 2\alpha(1+\tau_2)\tau_1 + 2\alpha \sqrt{\alpha(1+\tau_2)\tau_1}\eta_\ast 
        % \nonumber \\
        % &\quad 
        +  3\alpha^3\left({\frac{1+\tau_2}{\alpha}}\tau_1^2 + L_\ast^2 \tau_1 
        %  + \alpha \lambda^2 \tau_2^2 (1+\tau_2)
        % ) 
        \right) \nonumber \\
        &\leq \tau_2 + c\alpha\tau_1     \nonumber \\
    \end{align}
    assuming $L_\ast^2 \alpha^2 \leq 1$.
    % and $\alpha^4\tau_2 \lambda^2 \leq 1$.

      We can also bound $\|\mathbf{w}_{t,i}\|_2$:
    \begin{align}
       \|\mathbf{w}_{t,i}\|_2 &\leq c(\tau_2 \sqrt{\tau_1} + \sqrt{\alpha} L_{\max}).
    \end{align}
    
    
    % Again, we leave $\tau_1$ and $\tau_2$ unspecified for now. 
In order to simplify expressions, we make the benign assumption that $\alpha < 1$. We will verify this later. %assume that $\tau_1$ and $\tau_2$ are $\leq 1/2$, which enforces a benign upper bound on $\alpha$.

We have that $A_{1}(t), A_{2}(t), A_{4}(t)$ imply that
% \begin{align}
%     \|\mathbf{B}_{t,i}\|_2 &\leq \|\mathbf{B}_{t}\|_2 + \alpha 
% \end{align}
% as long as $\alpha \leq \tfrac{1}{\tau_1^2}$, 
for any $i \in [n]$, we have
    \begin{align}
        \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}  
        &= \mathbf{B}_{t}^\top \mathbf{B}_{t} - \alpha \mathbf{B}_{t}^\top \mathbf{G}_{t,i} - \alpha \mathbf{G}_{t,i}^\top \mathbf{B}_{t} + \alpha^2 \mathbf{G}_{t,i}^\top \mathbf{G}_{t,i}  \nonumber \\
        &= \mathbf{B}_{t}^\top \mathbf{B}_{t} - \alpha \mathbf{B}_{t}^\top (\mathbf{B}_t \mathbf{w}_t\mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top )\nonumber \\
        &\quad - \alpha (\mathbf{B}_t \mathbf{w}_t\mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top )^\top \mathbf{B}_{t} + \alpha^2 \mathbf{G}_{t,i}^\top \mathbf{G}_{t,i}  \nonumber %+ \alpha \lambda \mathbf{B}_t\boldsymbol{\Delta}_t
    \end{align}
    Thus
    \begin{align}
        \left\|\frac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i}\right\|_2 &\leq \frac{1+\tau_2}{\alpha} + 2(1+\tau_2)\tau_1+ 2\sqrt{\alpha(1+\tau_2)\tau_1}\eta_\ast 
        % \nonumber \\ % +  2 \alpha\lambda (1+\tau_2)\tau_2 
        % &\quad 
        + \alpha^2\left(\tfrac{\sqrt{1+\tau_2}}{\sqrt{\alpha}}\tau_1 + L_\ast \sqrt{\alpha \tau_1}\right)^2\nonumber \\ %+ \alpha \lambda {(1+\tau_2)}\tau_2 
        % &\quad +  3\alpha^3\left({\frac{1+\tau}{\alpha}}L_{\max}^4 + L_\ast^2 L_{\max}^2 + \alpha \lambda^2 \tau^2 (1+\tau) \right) \nonumber \\
        &\leq \tfrac{c}{\alpha}
    \end{align}
for some absolute constant $c$ and sufficiently small $\alpha$.

\begin{align} %+ \lambda \sqrt{\alpha} \tau_2
    \|\mathbf{G}_{t,i}\|_2 &\leq c\left(\frac{\tau_1}{\sqrt{\alpha}} + L_{\max}\sqrt{\tau_1} \right), \quad \left\|\sum_{i=1}^n\mathbf{G}_{t,i}\right\|_2 \leq c\left(\frac{\tau_1}{\sqrt{\alpha}} + \eta_\ast\sqrt{\tau_1} \right)% \leq \frac{c \tau_1}{\sqrt{\alpha}}
\end{align}



%     where \begin{align}\delta_1 &\coloneqq \alpha E_0 \mu_\ast^2 - \tfrac{\tau_2}{\alpha} - \sqrt{\alpha \tau_1}\eta_\ast - \alpha^{5/2} \left(\frac{\tau_1}{\sqrt{\alpha}} + L_{\max}\sqrt{\tau_1}% + \lambda \sqrt{\alpha} \tau_2
%     \right) \left(\tfrac{c}{\sqrt{\alpha}}\sqrt{\tau_1} +L_{\max} \right)L_{\max}  - \alpha (\dist_t +\tau_2) L_\ast^2 \nonumber %\\
% %   &\quad- \alpha^{5/2}\lambda \sqrt{\tau_1}\tau_2 \eta_\ast - \alpha^{3}\lambda L_\ast^2  \nonumber
%     \end{align}
    % \begin{align}
    %     \left\|\mathbf{{B}}_{t}^\top  (\mathbf{I}_d- \alpha\mathbf{B}_{t} \mathbf{B}_{t}^\top) \mathbf{{B}}_\ast \frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i} \right\|_2 &\leq \frac{\sqrt{1+\tau_2}}{\sqrt{\alpha}}  (\dist_t+\tau_2) \eta_\ast
    % \end{align}
which implies that in order for $\|\mathbf{w}_{t+1}\|_2 \leq \sqrt{\tau_1}$, the following conditions must hold:
\begin{align}
    &\tau_2 \leq c\alpha^2 E_0 \mu_{\ast}^2 \\
    &\sqrt{\tau_1} \eta_\ast \leq c\sqrt{\alpha} E_0 \mu_{\ast}^2  \\
    &\alpha^{3/2} \left(\frac{\tau_1}{\sqrt{\alpha}} + L_{\max}\sqrt{\tau_1}
    % + \lambda \sqrt{\alpha} \tau_2
    \right) \left(\tfrac{\sqrt{\tau_1}}{\sqrt{\alpha}} +L_{\max} \right)L_{\max}\leq  c E_0\mu_\ast^2 \\
    &\dist_t L_\ast^2 \leq  E_0 \mu_\ast^2\label{122}\\
    & \tau_2L_\ast^2 \leq c E_0 \mu_\ast^2\\
    % &\alpha^{3/2} \lambda \sqrt{\tau_1}\tau_2 \eta_{\ast}\leq c E_0 \mu_{\ast}^2 \\
    % &\alpha^2 \lambda L_{\ast}^2 \leq c E_0 \mu_{\ast}^2 \\
    &\tau_2 \eta_\ast 
    % (1+\lambda \alpha \tau_2 + \lambda \alpha^2)  
    \leq c \sqrt{\tau_1} \alpha^{3/2} E_0 \mu_{\ast}^2 %\\
    % &\sqrt{\tau_1}  \leq \sqrt{\alpha} 
\end{align}
% Besides \eqref{122}, each of the above inequalities are satisfied by choosing $\tau_1 = c \alpha^2$ and $\tau_2 = c \alpha^3$, and choosing $\alpha$ to be sufficiently small. In particular, we require $\alpha \leq c \max \left\{E_0 \mu_\ast^2,\left(\tfrac{E_0\mu_\ast^2}{\eta_\ast}\right)^2, \left(\tfrac{E_0\mu_\ast^2}{L_\ast^2}\right)^{1/3}\right\}$. We also require $\beta \leq \frac{1}{c\delta_1}$.

To deal with \eqref{122}, note from the definition of $E_0$ and the fact that $\dist_t\leq \dist_0$ by $A_4(t)$, that \eqref{122} is implied by
\begin{align}
    \kappa_\ast^{-2}\dist_0^2 +\dist_0 -  \kappa_\ast^{-2} \leq 0,
\end{align}
where $\kappa_\ast = \frac{L_\ast}{\mu_\ast}$. Applying the quadratic formula results in
\begin{align}
    \dist_0 \leq \frac{-1+ \sqrt{1+4\kappa_\ast^{-4}}}{2\kappa_\ast^{-2}},\label{127}
\end{align}
For example, if $\kappa_\ast = 2$, then we require $\dist_{0} < 2(\sqrt{2}-1)\approx 0.24$. Roughly we need $\dist_0 \leq \kappa_\ast^{-2}$ because $\sqrt{1+x}\approx 1+\tfrac{x}{2}$ for $x \in [0,1]$. 


% instead: wt increases for at most 



% We have
% \begin{align}
%     \|\mathbf{w}_{t+1}\|_2 &\leq (1 - \beta \alpha \mu_{\ast}^2 +\beta \alpha \dist_t L_{\ast}^2)\|\mathbf{w}_{t}\|_2 + \beta \alpha^{-1/2}\tau_2 \eta_\ast \nonumber \\
%     &\leq \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast \prod_{r=s}^t(1 - \beta \alpha \mu_{\ast}^2 +\beta \alpha \rho^r L_{\ast}^2) \nonumber \\
%     &\leq \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast \left(1 - \frac{1}{t-s}\sum_{r=s}^t\beta \alpha \mu_{\ast}^2 + \frac{1}{t-s}\sum_{r=s}^t\beta \alpha \rho^r L_{\ast}^2\right)^{t-s} \nonumber \\
%     &\leq \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast \left(1 - \beta \alpha \mu_{\ast}^2 + \frac{1}{t-s}\frac{\rho^s\beta \alpha L_{\ast}^2}{1-\rho}\right)^{t-s} \nonumber \\
%     &\leq   \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast \left(1 + \frac{1}{t-s}\frac{\rho^s\beta \alpha L_{\ast}^2}{1-\rho}\right)^{t-s} \nonumber \\
%     &\leq  \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast \left(1 + \frac{1}{t-s}\rho^s \kappa_{\ast}^2\right)^{t-s} \nonumber \\
%     &\leq \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast \exp({\rho^s \kappa_{\ast}^2}) \nonumber\\
%     &\leq \sum_{s=1}^t \beta \alpha^{-1/2}\tau_2 \eta_\ast (1+{\rho^s \kappa_{\ast}^2})
% \end{align}
% derivative of ln is zero at $t-s = b/(e-a)--> e^{b/(e-a)}= e^{\rho^s \kappa^{2}_\ast/(e-1+\beta\alpha\mu_{\ast}^2)}$... no benefit from this

% {\color{red} For second-order updates, we do not have any contraction. we must make similar argument as ANIL. but this relies on $\tau_2$ going to zero, which we do not have because $\tau_2$ is upper bounded by a term with only wt.  so not clear how to show wt stays bounded in this case.

% But empirically second order works without $\mathbf{w}_t$ or $\boldsymbol{\Delta}_t$ going to zero.
% Note that $\mathbf{w}_t$ does not converge to the avg, it stays near 0.


% For first-order updates, we still have $\lambda > L_{\max}$ and $\eta_{\ast} \ll 1$ (but not necessarily zero) requirements. can't get rid of $L_{\max}$ requirement. So this suggests that regularization is necessary. But exact MAML case should be different.
% }

 
%  $\tau_1=\mu_\ast^4 \kappa_{\ast,\max}^{-4} \alpha^3$,
 
%  $\tau_2=\mu_\ast^3 \kappa_{\ast,\max} \alpha^3$,
 
%  $\alpha \leq 1/L_{\max}$, 
 
%  $\beta \leq \frac{E_0^2 \mu_\ast \kappa_{\ast,\max}}{\kappa_{\ast}^4}\alpha^2$, $\kappa_{\ast,\max}\coloneqq \frac{L_{\max}}{\mu_\ast}$.  


    
    Next, denote the inner loop gradient for the representation for the $i$-th task as:
    \begin{align}
        \mathbf{G}_{t,i} &\coloneqq \mathbf{B}_t\mathbf{w}_t \mathbf{w}_t^\top - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top %+ \alpha \lambda \mathbf{B}_t\boldsymbol{\Delta}_{t}
    \end{align}
%   Now,  using $\mathbf{B}_{t,i} = \mathbf{B}_t -  \beta \mathbf{G}_{t,i}$, we have
%     \begin{align}
%         \alpha \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k &= \alpha \mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k - \alpha^2 \mathbf{B}_t^\top \mathbf{G}_{t,i} - \alpha^2 \mathbf{G}_{t,i}^\top \mathbf{B}_{t} + \alpha^3 \mathbf{G}_{t,i}^\top \mathbf{G}_{t,i} \nonumber \\
%         &= \boldsymbol{\Delta}_t + \mathbf{P}_{t,i}
%     \end{align}
%     where $\mathbf{P}_{t,i} \coloneqq - \alpha^2 \mathbf{B}_t^\top \mathbf{G}_{t,i} - \alpha^2 \mathbf{G}_{t,i}^\top \mathbf{B}_{t} + \alpha^3 \mathbf{G}_{t,i}^\top \mathbf{G}_{t,i}$.
%     So 
    then we have
    \begin{align}
        \mathbf{T}_{t,i} &= (\mathbf{I}_d -\alpha \mathbf{B}_t\mathbf{B}_t^\top) (\mathbf{B}_t \mathbf{w}_t - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}) - \alpha \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t - \alpha^2 \mathbf{G}_{t,i}\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \nonumber \\
        %  \mathbf{T}_{2,t,i} &= \mathbf{B}_t\boldsymbol{\Delta}_t + \mathbf{B}_t \mathbf{P}_{t,i} - \alpha \mathbf{G}_{t,i}\mathbf{P}_{t,i} - \alpha \mathbf{G}_{t,i} \boldsymbol{\Delta}_t \nonumber \\
         \mathbf{G}_{t} &= \frac{1}{n}\sum_{i=1}^n  (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top)(\mathbf{B}_t \mathbf{w}_t - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top -\mathbf{E}_t \label{eqbigG}  \\
         \mathbf{E}_t &\coloneqq \frac{1}{n}\sum_{i=1}^n\Big( \alpha \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top + \alpha^2 \mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\Big) % +  \alpha \lambda \mathbf{B}_t\boldsymbol{\Delta}_t \Big)
        %  &\quad - \frac{1}{n}\sum_{i=1}^n\Big( \alpha \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top + \alpha^2 \mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\Big) \label{eqbigG} %\nonumber \\
         %&\quad \quad \quad \quad \quad \; + \alpha \lambda \mathbf{B}_t \mathbf{P}_{t,i} - \alpha^2 \lambda \mathbf{G}_{t,i} \mathbf{P}_{t,i} - \alpha^2 \lambda \mathbf{G}_{t,i} {\boldsymbol{\Delta}}_t 
    \end{align}
    % {\color{red} Need to decompose gradient $\mathbf{G}_t$ as the sum of distance and non-distance terms, as for ANIL. Then we can see that Vt may increase.
    % We have:
    % \begin{align}
    %     V_{t,i} &\leq (1-\delta_1)V_t + 
    % \end{align}
    % the norm of Bt-Bti
    % For MAML, showing that $\boldsymbol{\Delta}_t$ is diminishing almost linearly requires showing that $\|\mathbf{w}_t\|_2$ is diminishing almost linearly (and empirically this is true, unlike for ANIL). This is necessary because there is an extra $\|\mathbf{w}_t\|_2$-term in the bound for $\boldsymbol{\Delta}_t$. 
    % Empirically: regularization 
    % 
    The first step of the proof is to show that the energy in the error terms due to the inner loop representation update, represented by $\|\mathbf{E}_t\|_2$, is small.
    % , via Lemmas \ref{lem}.
    We know that $\|\boldsymbol{\Delta}_t\|_2\leq \tau_2$. 
    Next, we have
    % \begin{align}
    %     \|\mathbf{G}_{t,i}\|_2 &\leq c\left(\frac{\tau_1}{\sqrt{\alpha}} + L_{\max}\sqrt{\tau_1} 
    %     %+ %\lambda \sqrt{\alpha} \tau_2
    %     \right)
    %     % L_{\max}^2 \left(\sqrt{\frac{1+\tau}{\alpha}}+ 1\right) + {\color{gray}L_{\max}^2}  \lambda \tau \sqrt{\alpha (1+\tau)}
    % \end{align}
    % % and
    % % \begin{align}
    % %     \|\mathbf{P}_{t,i}\|_2 &\leq 2\alpha^{1.5} \sqrt{1+\tau_2} \|\mathbf{G}_{t,i}\|_2 + \alpha^3\|\mathbf{G}_{t,i}\|_2^2 \nonumber \\
    % %     &\leq c \alpha^{1.5} \|\mathbf{G}_{t,i}\|_2 \nonumber \\
    % %     &\leq c \alpha^{1.5} \left(\frac{\tau_1}{\sqrt{\alpha}} + L_{\max}\sqrt{\tau_1}\right) \nonumber
    %     % + \lambda \sqrt{\alpha} \tau_2... &\leq 2\alpha \sqrt{1+\tau}L_{\max}^2 (\sqrt{1+\tau} + \sqrt{\alpha} + \lambda \tau \alpha \sqrt{1+\tau}) \nonumber \\
    %     % &\quad + 3\alpha^3L_{\max}^4\left(\frac{1+\tau}{\alpha} + 1 + \lambda^2 \tau^2 \alpha (1+\tau)  \right) \nonumber \\
    %     % &\leq c_0 L_{\max}^2\alpha (1 +\lambda \tau \alpha)+ c_0'  L_{\max}^4 \alpha^2 (1 + \lambda^2 \tau^2 \alpha^2)\nonumber \\
    %     % &\leq c_0'' L_{\max}^2\alpha (1 +\lambda \tau \alpha) ( 1 +  L_{\max}^2 \alpha (1 + \lambda \tau \alpha)) \nonumber\\
    %     % &\leq c L_{\max}^2\alpha (1 +\lambda \tau \alpha)
    %     % &\leq 2\alpha ({1+\tau}) (L_{\max}^2  + \alpha \lambda \tau + \alpha L_{\max}^4 + \alpha^{3}\lambda \tau L_{\max}^4) 
    % % \end{align}
    % % for some absolute constants $c_0, c_0', c_0''$, and where the last inequality follows under the reasonable assumption $L_{\max}^2\alpha (1 +\lambda \tau \alpha) \leq c_0'''$ for some absolute constant $c_0'''$.
    % % For now, we do not try to optimize $L_{\max}$ vs $L_\ast$, which would give the strictest possible bound in terms of $k$. 
    % % Instead we use triangle inequality to bound each term inside the sum separately. 
    % therefore
%   alpha tau2 rt(tau1) ( tau1/rt(alpha) + w*i rt(tau1) +rt(alpha) lambda tau2 )(tau2 rt(tau1) + rt(alpha)w*i )
%   =  alpha tau2 rt(tau1) (tau1(3/2) tau2/rt(alpha) + tau1 eta + tau1 tau2 eta + rt(alpha) rt(tau1) L*2 + rt(alpha) rt(tau1) tau2(2) lambda + alpha tau2 lambda eta )
    \begin{align}
        % \|\mathbf{w}_{t,i} \|_2 &\leq \tau L_{\max} + \sqrt{\alpha(1+\tau)} L_{\max}  \nonumber \\
        \left\|\alpha\frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top\right\|_2 &\leq \left\|\alpha\frac{1}{n}\sum_{i=1}^n (\mathbf{B}_{t}\mathbf{w}_{t} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i})\mathbf{w}_{t}^\top\boldsymbol{\Delta}_t \mathbf{w}_t(\mathbf{w}_t^\top\del_t +\alpha  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_{\ast}^\top\mathbf{B}_{t} )\right\|_2  \nonumber \\
        &\leq \alpha \|\mathbf{B}_{t}\mathbf{w}_{t}\mathbf{w}_{t}^\top\boldsymbol{\Delta}_t \mathbf{w}_t \mathbf{w}_t^\top\del_t \|_2 + \alpha\|\mathbf{B}_{\ast}\|_2 \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\right\|_2\|\mathbf{w}_{t}^\top\boldsymbol{\Delta}_t \mathbf{w}_t \mathbf{w}_t^\top\del_t \|_2   \nonumber \\
        &\quad + \alpha^2 \|\mathbf{B}_{t}\mathbf{w}_{t}\mathbf{w}_{t}^\top\boldsymbol{\Delta}_t \mathbf{w}_t \|_2 \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i} \right\|_2 \|\mathbf{B}_\ast^\top \mathbf{B}_t\|_2 +\alpha^2 |\mathbf{w}_{t}^\top\boldsymbol{\Delta}_t \mathbf{w}_t| \left\|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \right\|_2\|\mathbf{B}_\ast^\top \mathbf{B}_t\|_2 \nonumber \\
        &\leq c\left( \tau_1^{2} \tau_2^2 \sqrt{\alpha} + \alpha \tau_1^{3/2}\tau_2^2 \eta_\ast + \alpha \tau_1^{3/2} \tau_2 \eta_\ast 
        + \alpha^{3/2} \tau_1 \tau_2 L_*^2  
        % +\alpha^{3/2} \tau_1 \tau_2^3 \lambda + \alpha^2 \sqrt{\tau_1} \tau_2^2  \eta_\ast \lambda
        \right) \nonumber \\
        &\leq c' \left(\tau_1^{2} \tau_2^2 \sqrt{\alpha} + \alpha \tau_1^{3/2}\tau_2 \eta_\ast 
        + \alpha^{3/2} \tau_1 \tau_2 L_*^2  
        % + \alpha^{3/2} \tau_1 \tau_2^3 \lambda + \alpha^2 \sqrt{\tau_1} \tau_2^2  \eta_\ast \lambda
        \right) %\nonumber
        % \sqrt{\alpha}\tau_1^{2} \tau_2^2 + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha \tau_1^{3/2} \tau_2^2 \eta_\ast + \alpha^{3/2} L_\ast^2 \tau_1 \tau_2 + \alpha^{3/2}\lambda \sqrt{\tau_1} \tau_2^2 (\tau_2 \sqrt{\tau_1} + \sqrt{\alpha} \eta_\ast) \nonumber \\
        % &\leq \sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2^2 \eta_\ast + \alpha^{3/2} L_\ast^2 \tau_1 \tau_2 + \alpha^{3/2}\lambda \sqrt{\tau_1} \tau_2^2 (\tau_2 \sqrt{\tau_1} + \sqrt{\alpha} \eta_\ast) \nonumber \\
        % \tau L_{\max}^4 \nonumber \\
        % &\leq \left( \sqrt{\frac{1+\tau}{\alpha}} + 1 +   \lambda \tau \sqrt{\alpha (1+\tau)} \right)\left(\tau  + \sqrt{\alpha(1+\tau)} \right)  \nonumber \\
        % &= \alpha \tau  L_{\max}^4\nonumber \\
        % &\quad \left(\frac{\tau\sqrt{1+\tau}}{\sqrt{\alpha}} + {1+\tau} + \tau^2 \lambda \sqrt{\alpha(1+\tau)} + \tau \lambda \sqrt{\alpha}(1+\tau) + \tau + \sqrt{\alpha(1+\tau)}\right) \nonumber \\
        % &=  \alpha \tau  L_{\max}^4\nonumber \\
        % &\quad \left(\frac{\tau\sqrt{1+\tau}}{\sqrt{\alpha}} +1 + \tau^2 \lambda \sqrt{\alpha(1+\tau)} + \tau \lambda \sqrt{\alpha}(1+\tau)  + \sqrt{\alpha(1+\tau)}\right) \nonumber \\
        % \|\alpha^2 \mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\|_2 &\leq \alpha^{1.5}\sqrt{1+\tau} L_{\max}^5 \left( \sqrt{\frac{1+\tau}{\alpha}} + 1 +   \lambda \tau \sqrt{\alpha (1+\tau)} \right)\left(\tau  + \sqrt{\alpha(1+\tau)}\right) 
    \end{align}
    Further,
    % 1/rt(alpha) w*i 
    % (tau1(3/2) tau2/rt(alpha) + tau1 eta + tau1 tau2 eta + rt(alpha) rt(tau1) L*2 + rt(alpha) rt(tau1) tau2(2) lambda + alpha tau2 lambda eta )
    % tau1(3/2) tau2 eta/alpha + tau1 L*2/rt(alpha) + tau1 tau2 L*2 /rt(alpha) + rt(tau1) Lmax L*2 + rt(tau1) tau2(2) lambda eta + rt(alpha) tau2 L*2 lambda
    \begin{align}
         \left\|\alpha^2 \frac{1}{n} \sum_{i=1}^n\mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\right\|_2 
         &\leq c\left(\alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2 + \alpha^{3/2} \tau_1 \tau_2 L_*^2 + \alpha^2 \sqrt{\tau_1} L_{\max} L_*^2 
        %  + \alpha^2 \sqrt{\tau_1} \tau_2^2 \lambda \eta_\ast + \alpha^{5/2} \tau_2 L_*^2 \lambda
         \right)
        %  &\leq (\alpha \tau  L_{\max}^4+\alpha^{1.5}\sqrt{1+\tau} L_{\max}^5 )\left( \sqrt{\frac{1+\tau}{\alpha}} + 1 +   \lambda \tau \sqrt{\alpha (1+\tau)} \right)\left(\tau  + \sqrt{\alpha(1+\tau)}\right)  \nonumber \\
        % %  &\leq c_1 L_{\max}^5\alpha(\tau + \sqrt{\alpha})\left(\frac{1}{\sqrt{\alpha} }+ \lambda \tau \sqrt{\alpha} \right)\left(\tau + \sqrt{\alpha} \right) \nonumber \\
        %  &\leq c_1 L_{\max}^5\alpha(\tau + \sqrt{\alpha})^2\left(\frac{1}{\sqrt{\alpha} }+ \lambda \tau \sqrt{\alpha} \right) \nonumber \\
        %  &= c_1 L_{\max}^5\sqrt{\alpha}(\tau + \sqrt{\alpha})^2\left(1+ \lambda \tau {\alpha} \right)
    \end{align}
    % $\tau_1^{2} \tau_2^2 \sqrt{\alpha} $
    % $\alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2 + \alpha^{3/2} \tau_1 \tau_2 L_*^2 + \alpha^2 \sqrt{\tau_1} L_{\max} L_*^2 + \alpha^2 \sqrt{\tau_1} \tau_2^2 \lambda \eta_\ast + \alpha^{5/2} \tau_2 L_*^2 \lambda$
    Combining these two bounds yields
    \begin{align}
        \|\mathbf{E}_t\|_2 &\leq \left\|\alpha\frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top\right\|_2 + \left\|\alpha^2 \frac{1}{n} \sum_{i=1}^n\mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top\right\|_2 \nonumber \\
         &\leq c\left(\sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2 + \alpha^{3/2} \tau_1 \tau_2 L_*^2 + \alpha^2 \sqrt{\tau_1} L_{\max} L_*^2
        %  + \alpha^2 \sqrt{\tau_1} \tau_2^2 \lambda \eta_\ast + \alpha^{5/2} \tau_2 L_*^2 \lambda
         \right) \nonumber \\
         &\leq c'\left( \sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  
        %  +  \alpha^{5/2} \tau_2 L_*^2 \lambda 
         \right) \nonumber 
    \end{align}
    % assuming $\tau_1^{1/2}\tau_2 \eta_\ast < \alpha^{1/2}L_\ast^2$.
Now, expanding $\mathbf{w}_{t,i}$ in \eqref{eqbigG} yields
    \begin{align}
        \mathbf{B}_t^\top \mathbf{G}_t &= -\boldsymbol{\Delta}_t \frac{1}{n}\sum_{i=1}^n \Big(\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_t^\top \boldsymbol{\Delta}_t + \alpha \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \nonumber \\
        &\quad \quad \quad \quad  \quad \quad - \mathbf{B}_t^\top  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top \boldsymbol{\Delta}_t - \alpha \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \Big) 
        % \nonumber \\
        % &\quad \quad 
        % + \alpha \lambda \mathbf{B}_t^\top \mathbf{B}_t \boldsymbol{\Delta}_t 
        - \mathbf{B}_t^\top \mathbf{E}_t \\
        &=  \alpha \boldsymbol{\Delta}_t \frac{1}{n}\sum_{i=1}^n\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t
        % + \alpha \lambda \mathbf{B}_t^\top \mathbf{B}_t \boldsymbol{\Delta}_t 
        + \boldsymbol{\Delta}_t\mathbf{D}_t - \mathbf{B}_t^\top \mathbf{E}_t
    \end{align}
    where  $\mathbf{D}_t \coloneqq  \frac{1}{n}\sum_{i=1}^n \Big(-\mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_t^\top \boldsymbol{\Delta}_t + \alpha \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \mathbf{B}_t^\top  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top \boldsymbol{\Delta}_t \Big)$. Note that $\mathbf{D}_t$ satisfies
    \begin{align}
        \|\mathbf{D}_t\|_2 &\leq c\left(\frac{\tau_1 \tau_2}{\alpha} + \frac{\sqrt{\tau_1}\eta_\ast}{\sqrt{\alpha}} + \frac{\sqrt{\tau_1}\tau_2\eta_\ast}{\sqrt{\alpha}} \right)   \leq   c'\left(\frac{\tau_1 \tau_2}{\alpha} + \frac{\sqrt{\tau_1}\eta_\ast}{\sqrt{\alpha}}  \right)  
    \end{align}
    % for some absolute constant $c$ 
    % (note that the last term is dominated). 
    We have 
    \begin{align}
        \|\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}_k\|_2
        &= \|\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t} - \mathbf{I}_k - \beta \alpha  \mathbf{B}_{t}^\top\mathbf{G}_t - \beta \alpha  \mathbf{G}_{t}^\top\mathbf{B}_t + \beta^2 \alpha \mathbf{G}_{t}^\top\mathbf{G}_t\|_2 \nonumber \\
        &\leq \|\boldsymbol{\Delta}_t\|_2 \Bigg( 1 - 2\beta \alpha^2 \sigma_{\min}\left( \frac{1}{n}\sum_{i=1}^n\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \right) 
        % - 2 \beta \alpha^2 \lambda \sigma_{\min}(\mathbf{B}_t^\top \mathbf{B}_t) 
        % \nonumber \\
        % &\quad \quad 
        + 2 \beta \alpha \|\mathbf{D}_t\|_2  \Bigg)\nonumber \\
         &\quad \quad +2 \beta \alpha \|\mathbf{B}_t^\top \mathbf{E}_t\|_2  + \beta^2 \alpha \|\mathbf{G}_t\|_2^2 \nonumber \\
        &\leq \tau_2 \Bigg( 1 - c\beta \alpha E_0 \mu_{\ast}^2 
        % -  c \beta \alpha \lambda 
        + c'\beta{\tau_1 \tau_2} + c'\beta \sqrt{\alpha \tau_1}\eta_\ast\Bigg) \nonumber \\
        &\quad \quad +c'\bigg(\beta \alpha \tau_1^{2} \tau_2^2  + \beta \alpha^{3/2} \tau_1^{3/2} \eta_\ast + \beta \alpha^{2}\tau_1 L_*^2  + \beta \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3  + \beta^2 \alpha \|\mathbf{G}_t\|_2^2 \bigg)  \nonumber% \\
    %   &\quad \quad %+  \beta \alpha^{3} \tau_2 \lambda (\lambda +L_*^2) 
    %   + \beta \alpha^{5/2} \sqrt{\tau_1}\lambda \eta_\ast  + \beta \alpha^{5} \lambda^3 \tau_2^2
        % +2 c \beta \alpha L_{\max}^2( L_{\max}^3\tau^2 + L_{\max}^3{\alpha} +  \lambda \alpha) (1 +\lambda \tau \alpha)
    \end{align}
    % \sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 (\lambda +L_*^2)  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  +  \alpha^{5/2} \tau_2 \lambda (\lambda +L_*^2) \nonumber \\
    %      &\quad + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast  + \alpha^{9/2} \lambda^3 \tau_2^2
    Finally, we have 
    \begin{align}
        \|\mathbf{G}_t\|_2 &\leq \left\|\frac{1}{n}\sum_{i=1}^n\Big( (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top)(\mathbf{B}_t \mathbf{w}_t - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top 
        % +  \alpha \lambda \mathbf{B}_t\boldsymbol{\Delta}_t 
        \Big) \right\|_2 + \|\mathbf{E}_t\|_2 \nonumber \\
        &\leq \frac{\tau_1 \tau_2^2}{\sqrt{\alpha}} + \sqrt{\tau_1}\tau_2 \eta_\ast + L_\ast^2 \sqrt{\alpha}\dist_t + \sqrt{\tau_1}\tau_2 \eta_\ast \dist_t + L_\ast^2 \sqrt{\alpha} \tau_2 + \sqrt{\tau_1} \tau_2^2 \eta_\ast \nonumber \\
        &\quad + \sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2}\tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3 
        % +  \alpha^{5/2} \tau_2 \lambda (\lambda +L_*^2) 
        \nonumber \\
        %  &\quad + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast  + \alpha^{9/2} \lambda^3 \tau_2^2 \nonumber \\
         &\leq \frac{\tau_1 \tau_2^2}{\sqrt{\alpha}} +  \sqrt{\tau_1}\tau_2 \eta_\ast+ \alpha \tau_1^{3/2} \tau_2\eta_\ast + L_\ast^2 \sqrt{\alpha}\dist_t  +  \sqrt{\alpha} \tau_2 L_\ast^2 +  \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3 % +  \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast  + \alpha^{9/2} \lambda^3 \tau_2^2 
        \nonumber
        % (1+\tau)L_\ast^2 + \lambda\tau \sqrt{\alpha(1+\tau)} + \|\mathbf{D}_t\|_2 +  \|\mathbf{E}_t\|_2 \nonumber\\
        % &\leq c_8 L_\ast^2 + \lambda \tau\sqrt{\alpha} + c_7 L_{\max}^2\sqrt{\alpha}( L_{\max}^3(\tau + \sqrt{\alpha})^2 +  \lambda \alpha) (1 +\lambda \tau \alpha) \nonumber \\
        % &\quad + c \left(\frac{\tau}{\alpha} L_{\max}^2 + \frac{1}{\sqrt{\alpha}} L_{\max} L_\ast  \right) \nonumber\\
        % &\leq  \lambda \tau\sqrt{\alpha} + c_7' L_{\max}^5\sqrt{\alpha}( \tau^2 + {\alpha}) + c'\frac{\tau}{\alpha} L_{\max}^2 + c''\frac{1}{\sqrt{\alpha}} L_{\max}^2  \nonumber\\  % c_9 \left(\lambda \tau\sqrt{\alpha}    \right)
    \end{align}
    assuming $\sqrt{\tau_1}\tau_2 \eta_\ast \leq L_\ast^2\sqrt{\alpha}$ {\color{red} true but don't drop this}
    %$\alpha^2\lambda \leq 1$,
    using similar analysis as in the proof for ANIL, noting that the matrix in the RHS of the first equation is equivalent to $\mathbf{G}_t$ from the ANIL case.
    Thus
    \begin{align}
     &\|\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} - \mathbf{I}_k\|_2 \nonumber \\
        &\leq \tau_2 \Bigg( 1 - 2\beta \alpha E_0 \mu_{\ast}^2 
        % - 2 \beta \alpha \lambda 
        + \beta{\tau_1 \tau_2} + \beta \sqrt{\alpha \tau_1}\eta_\ast\Bigg) %\nonumber \\
     %   &\quad \quad
        +c\bigg(\beta \alpha \tau_1^{2} \tau_2^2  + \beta \alpha^{3/2} \tau_1^{3/2} \eta_\ast + \beta \alpha^{2}\tau_1 L_*^2  + \beta \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3   \nonumber \\
    %   &\quad \quad + \beta \alpha^{5/2} \sqrt{\tau_1}\lambda \eta_\ast  + \beta \alpha^{5} \lambda^3 \tau_2^2 \nonumber \\
    %     +\beta \alpha^{3/2} \tau_1^{2} \tau_2^2  + \beta \alpha^2 \tau_1^{3/2} \tau_2 \eta_\ast + \beta \alpha^{5/2}\tau_1 (\lambda +L_*^2)  + \beta \alpha^3 \sqrt{\tau_1} L_{\max}^3   \nonumber \\
    %   &\quad \quad +  \beta \alpha^{7/2} \tau_2 \lambda (\lambda +L_*^2) + \beta \alpha^3 \sqrt{\tau_1}\lambda \eta_\ast  + \beta \alpha^{11/2} \lambda^3 \tau_2^2 \nonumber \\
       &\quad 
      + \beta^2 \tau_1^2 \tau_2^4 + \beta^2 \alpha \tau_1 \tau_2^2 \eta_\ast^2 + \beta^2 \alpha^2 \tau_2^2 L_\ast^4 + \beta^2 \alpha^{4}\tau_1^2  L_\ast^4 %\nonumber \\
    %   &\quad 
      + \beta^2 \alpha^5 \tau_1 L_{\max}^6 
    %   + \beta^2 \alpha^3 \tau_1 \lambda^2 \eta_\ast^2 
      + \beta^2 \alpha^2\tau_1^3 \eta_\ast^2 
    %   + \beta^2 \alpha^{10}\lambda^6 \tau_2^4   
      +\beta^2 \alpha^2 L_\ast^4 \dist_t^2 \bigg) \nonumber \\
      &\leq \tau_2 \Bigg( 1 - 2\beta \alpha E_0 \mu_{\ast}^2 
    %   - 2 \beta \alpha \lambda 
      + \beta{\tau_1 \tau_2} + \beta \sqrt{\alpha \tau_1}\eta_\ast 
    %   + \beta\alpha^{3} \lambda(\lambda + L_\ast^2) + \beta \alpha^{5}\lambda^3 \tau_2
      \Bigg) +  \beta \alpha^{2}\tau_1 L_*^2  + \beta \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3  
    %   + \beta \alpha^{5/2} \sqrt{\tau_1}\lambda \eta_\ast 
      + \beta \alpha^{3/2}\tau_1^{3/2}\eta_\ast \nonumber \\
      &\quad   + \beta^2 \alpha^2 (\alpha^2\tau_1^2 +\tau_2^2)L_\ast^4 
    %   + \beta^2 \alpha^3 \tau_1 \lambda^2 \eta_\ast^2 
    %   + \beta^2 \alpha^{10}\lambda^6 \tau_2^4   
      +\beta^2 \alpha^2 L_\ast^4 \dist_t^2 + \beta^2 \tau_1^2 \tau_2^4 + \beta^2 \alpha \tau_1 \tau_2^2 \eta_\ast^2 +\beta^2 \alpha^3 \tau_1^3\tau_2^2 \eta_\ast^2 +\alpha^5 \tau_1 L_{\max}^6
      \end{align}
      
      {\color{red} need to upd below, and eq before 199, correct but old}
      
    %   \begin{align}
    %   &\leq \tau_2 \Bigg( 1 - 2\beta \alpha E_0 \mu_{\ast}^2 - 2 \beta \alpha \lambda + \beta{\tau_1 \tau_2} + \beta \sqrt{\alpha \tau_1}\eta_\ast + \beta\alpha^{7/2} \lambda(\lambda + L_\ast^2) + \beta \alpha^{11/2}\lambda^3 \tau_2 \Bigg) \nonumber \\
    %     &\quad + \beta \alpha^{5/2}\tau_1 (\lambda +L_*^2)  + \beta \alpha^3 \sqrt{\tau_1} L_{\max}^3  + \beta \alpha^3 \sqrt{\tau_1}\lambda \eta_\ast  \nonumber \\
    %   &\quad   + \beta^2 \alpha^2 (\alpha^2\tau_1^2 +\tau_2^2)(\lambda+L_\ast^2)^2  + \beta^2 \alpha^3 \tau_1 \lambda^2 \eta_\ast^2 + \beta^2 \alpha^{10}\lambda^6 \tau_2^4   +\beta^2 \alpha^2 L_\ast^4 \dist_t^2  \nonumber \\
    %   &\leq \tau_2 \Bigg( 1 - 2\beta \alpha E_0 \mu_{\ast}^2 - 2 \beta \alpha \lambda + \beta{\tau_1 \tau_2} + \beta \sqrt{\alpha \tau_1}\eta_\ast + \beta\alpha^{7/2} \lambda(\lambda + L_\ast^2) + \beta \alpha^{11/2}\lambda^3 \tau_2  \Bigg) \nonumber \\
    %   &\quad +\tau_2 \left(\beta^2\alpha^2 (\lambda+L_\ast^2)^2 \tau_2  + \beta^2 \alpha^{10}\lambda^6 \tau_2^3 \right) \nonumber \\
    %     &\quad + \sqrt{\tau_1}\left(\beta \alpha^3 \left(\tfrac{\sqrt{\tau_1} (\lambda\!+\!L_\ast^2)}{\sqrt{\alpha}}+\! L_{\max}^3 \! + \!\lambda \eta_\ast \right) + \beta^2 \alpha^4 (\lambda+L_\ast^2)^2 \tau_1^{3/2} +  \beta^2 \alpha^3  \lambda^2 \eta_\ast^2 \sqrt{\tau_1}\right) \nonumber \\
    %   &\quad +\beta^2 \alpha^2 L_\ast^4 \dist_t^2  \nonumber
    % \end{align}
    % % for $\beta$ sufficiently small.
    % assuming $\beta \alpha^2 \sqrt{\tau_1} \leq L_{\max}^3$.
    For this to stay less than $\tau_2$, we need to choose  %\alpha^{3} \tau_2 \lambda (\lambda +L_*^2) \! \!  +  \!  \alpha^{5/2} \sqrt{\tau_1}\lambda \eta_\ast  + \alpha^{5} \lambda^3 \tau_2^2 
    \begin{align}
       0< \beta \leq \frac{c\alpha \tau_2 E_0 \mu_\ast^2  \!-\!c'\left(\tau_1\tau_2^2 \!+\! \sqrt{\alpha \tau_1}\tau_2 \eta_\ast \!+\!\alpha^{2}\tau_1 L_*^2\!  + \! \alpha^{5/2} \sqrt{\tau_1} L_{\max}^3  \right) }{ \alpha^2 (\alpha^2\tau_1^2 +\tau_2^2)L_\ast^4  + \alpha^2 L_\ast^4 \dist_0^2 + \tau_1^2 \tau_2^4 +  \alpha \tau_1 \tau_2^2 \eta_\ast^2 + \alpha^3 \tau_1^3\tau_2^2 \eta_\ast^2+ \alpha^5 \tau_1 L_{\max}^6}
    \end{align}



% Now, suppose that $\|\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\|_2 \leq L_\ast$ for all $t$ with high probability. Let $a_t \coloneqq \|\mathbf{w}_t\|_2$ for all $t$.
Now, applying \eqref{forall} recursively for $s=t,t-1,\dots,0$ and plugging in the definition of $z_s$ yields
\begin{align}
    a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
    &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} {z}_{t-1})(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_{t-1} L_\ast(1 + \tfrac{2\beta}{\alpha} {z}_t)  + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
    &\;\; \vdots \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t {z}_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
    &=  \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t z_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
    &= \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t q^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1- q}\prod_{r=s+1}^t(1+ q^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1- q}) \nonumber \\
    &= \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast \sum_{s=0}^t q^{s} \prod_{r=s+1}^t\left(1+ q^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - q}\right) \nonumber
\end{align}    
where the first equality follows under the assumption that $a_0 = 0$. By the AM-GM inequality and sum of geometric series, we have, for $s\leq t-1$,
\begin{align}
    \prod_{r=s+1}^t\left(1+ q^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1 - q}\right) &\leq \left(1 + \tfrac{1}{t-s} \sum_{r=s+1}^t q^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - q}\right)^{t-s} \nonumber \\
    &\leq \left(1 + \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3q^{s+1}L_\ast^4 }{(1- q)^2} \right)^{t-s} 
\end{align}
The RHS is monotonically increasing in $t$ (since each additional $t$ means multiplication by a number greater than 1) so we can upper bound it by its limit as $t \rightarrow \infty$. This limit is
% $\exp\left(\left(1 + \tfrac{1}{t-s+1} \tfrac{\sqrt{\alpha}\beta^3q^{2}}{(1- q)^2} \right)^{t-s-1} \right) $, where the exponent is less than 1 for sufficiently small $\alpha, \beta$. For general $s$, the RHS limit is 
$\exp\left( {20} \tfrac{{\alpha}\beta^3q^{s+1}}{(1- q)^2} \right)$ (note that it is of the form $\lim_{x \rightarrow \infty} (1+\tfrac{a}{x})^x = a$). Note that $q = 1 - \Omega(\beta \alpha \mu_{\ast}^2)$ for sufficiently small $\beta,\alpha$, 
% {\color{red} (since $\tau_2 = $}), 
thus $1-q \leq c\beta \alpha \mu_{\ast}^2$.
As a result, to ensure $\exp\left( {20} \tfrac{{\alpha}\beta^3q^{s+1}}{(1- q)^2} \right)\leq 1$, we can choose
\begin{align}
  {20\alpha}\beta^3 L_\ast^4  &\leq   (1- q)^2 \nonumber \\
  \iff {20\alpha}\beta^3 L_\ast^4 &\leq  c \alpha^2 \beta^2\mu_{\ast}^4 \nonumber \\
  \iff \beta &\leq c' \frac{\alpha \mu_{\ast}^4}{L_\ast^4}. \label{betac1}
\end{align}
Under this condition on $\beta$, we have
\begin{align}
    a_{t+1} &\leq \tfrac{20 \alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast\sum_{s=1}^{t-1} q^{s} \exp\left( {20} \tfrac{{\alpha}\beta^3q^{s+1}L_\ast^4 }{(1- q)^2} \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast q^{t} \nonumber \\
    &\leq \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast\sum_{s=1}^{t-1} q^{s}\left( 1+ {40} \tfrac{{\alpha}\beta^3q^{s+1}L_\ast^4 }{(1- q)^2}  \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast q^{t} \label{usenum}\\
    &\leq \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast \sum_{s=1}^{t-1} q^{s}\left( 1+ 2q^{s+1}  \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast q^{t} \label{usebeta}\\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast\sum_{s=1}^{t} q^{s} \nonumber \\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{(1 - q)^2} L_\ast \nonumber \\
    &\leq c \frac{\beta}{\sqrt{\alpha}}\kappa_\ast^4 \eta_\ast \nonumber
    % &\leq \sqrt{\alpha}
    % &\leq \tfrac{\alpha\beta^3}{\gamma - q^2} c \exp\left( \tfrac{1}{t-s} \tfrac{\sqrt{\alpha}\beta^3}{(1- q)^2} \right)\sum_{s=1}^t \gamma^{s+1}  \nonumber \\
    % &\leq \tfrac{\alpha\beta^3}{\gamma - q^2} c \exp\left( \tfrac{\alpha\beta^3}{\gamma - q^2}\tfrac{\gamma^{2}}{1- \gamma}\right)\tfrac{\gamma^2}{1-\gamma} 
\end{align} 
where \eqref{usenum} follows from the numerical inequality $e^x \leq 1+2x$ for $x\in [0,1]$ and \eqref{usebeta} follows from the condition on $\beta$ in \eqref{betac1}. %, and the last inequality follows for $\beta \leq\alpha/(60 L_\ast^5).$
% and $\|\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\|_2 \leq c$ for all $t$ with high probability. 
% The only condition is $\beta \leq \alpha$.






-----

For ease of notation we define the following matrices and vectors:
\begin{align}
     \mathbf{G}_t &\coloneqq (\mathbf{I}_d -  \alpha \mathbf{{B}}_t \mathbf{{B}}_t^\top)\frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top \nonumber \\% -  \alpha \lambda (\mathbf{I}_d - \alpha \mathbf{{B}}_t \mathbf{{B}}_t^\top) \mathbf{{B}}_t \nonumber \\
    % &\quad - (1-\alpha)\mathbf{{B}}_t \mathbf{{B}}_t^\top \frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top \nonumber \\
    \mathbf{A}_t &\coloneqq \frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{{B}}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top  \nonumber \\
    \mathbf{u}_t &\coloneqq \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_{t} \nonumber \\
    \mathbf{v}_{t,i} &\coloneqq   \mathbf{B}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i}. \nonumber
\end{align}
Observe that $\mathbf{B}_{t+1} = \mathbf{B}_t - \beta \mathbf{G}_t$ and 
\begin{align}
    \mathbf{B}_t^\top \mathbf{G}_t &= (\mathbf{I}_k - \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t)\frac{1}{n}\sum_{i=1}^n( \mathbf{{B}}_t^\top  \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top %-  \alpha \lambda (\mathbf{I}_k - \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t )\mathbf{{B}}_t^\top \mathbf{{B}}_t  
    =
    % &\quad - (1-\alpha)\mathbf{{B}}_t^\top \mathbf{{B}}_t \frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{{B}}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top \nonumber \\
    % &= (\mathbf{I}_k -  \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t)\left( \mathbf{A}' -\alpha\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top  - \alpha\lambda \mathbf{{B}}_t^\top \mathbf{{B}}_t\right). 
    % &= 
    (\mathbf{I}_k -  \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t)\mathbf{A}_t. 
    %- (1-\alpha)\mathbf{{B}}_t^\top \mathbf{{B}}_t\mathbf{A}.
\end{align}
% We will show that the $-\alpha \lambda \mathbf{B}_t^\top \mathbf{B}_t$ term helps to diminish the energy in $\mathbf{I}_k -  \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t$, as long as we have control of $\mathbf{A}_t$.
Let us examine $\mathbf{A}_t$ more closely.
\begin{align}
   \mathbf{A}_t &=\frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{{B}}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top \nonumber \\
    &= \frac{1}{n}\sum_{i=1}^n(  \mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t} -  \mathbf{{B}}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )(\mathbf{w}_{t}^\top (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) + \alpha \mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top\mathbf{B}_t) \nonumber \\
    &= \mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t}\mathbf{w}_{t}^\top (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) + %(1-\alpha)\mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t}\mathbf{w}_{t}^\top \mathbf{{B}}_t^\top \mathbf{{B}}_t + 
    \alpha \frac{1}{n}\sum_{i=1}^n \mathbf{{B}}_t^\top \mathbf{{B}}_t  \mathbf{w}_{t}\mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{{B}}_t \nonumber \\
    &\quad - \left(  \frac{1}{n}\sum_{i=1}^n \mathbf{{B}}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{t}^\top (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) %+ (1-\alpha ) \mathbf{B}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{t}^\top\mathbf{B}_t^\top \mathbf{B}_t 
    + \alpha \mathbf{B}_t^\top\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top\mathbf{\hat{B}}_{\ast}^\top \mathbf{B}_t \right) \nonumber \\
    &= \left(\mathbf{u}_t - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{w}_t^\top (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t)  %(1-\alpha) \left(\mathbf{u} - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{u}^\top 
    +\alpha \mathbf{u}_t\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}^\top-\alpha \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \nonumber \\
    &= \mathbf{A}_t' - \alpha\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \label{help}
\end{align}
where 
    $\mathbf{A}_t' \coloneqq \left(\mathbf{u}_t - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{w}_t^\top (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) %(1-\alpha) \left(\mathbf{u} - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{u}^\top 
    +\alpha \mathbf{u}_t\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}^\top$.
    % \left(\mathbf{u} - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{B}_t^\top \mathbf{B}_t) + (1-\alpha) \left(\mathbf{u} - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{u}^\top +\alpha \mathbf{u}\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}^\top$. 
   Note that the $\alpha\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top$ term in \eqref{help} is a positive definite matrix due to the diversity of the ground-truth heads, so it will help to diminish the energy in $\mathbf{I}_k -  \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t$. 
    With this notation in place, we have
\begin{align}
    \mathbf{I}_k -  \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} 
    &= \mathbf{I}_k - \alpha \Bigg( \mathbf{B}_{t}^\top \mathbf{B}_{t} - \beta  \mathbf{B}_{t}^\top \mathbf{G}_t - \beta \mathbf{G}_t^\top \mathbf{B}_{t} + \beta^2 \mathbf{G}_t^\top \mathbf{G}_t  \Bigg) \nonumber \\
    &= \left(\mathbf{I}_k -  \alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \left(\tfrac{1}{2}\mathbf{I}_k +\alpha \beta \mathbf{A}_t' -\beta \alpha^2\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \right) \nonumber \\
    &\quad +  \left(\tfrac{1}{2}\mathbf{I}_k + \alpha \beta (\mathbf{A}_t')^\top  -\beta \alpha^2\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top  \right) \left(\mathbf{I}_k - \alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) +\alpha \beta^2 \mathbf{G}_t^\top \mathbf{G}_t \label{imbt1}
    % &\quad - (1-\alpha) \beta \mathbf{B}_{t}^\top \mathbf{B}_{t}\mathbf{A}_t-  (1-\alpha)\beta\mathbf{A} \mathbf{B}_{t}^\top \mathbf{B}_{t} + \beta^2 \nabla^\top \nabla 
\end{align}
Note that we have written $\mathbf{I}_k -  \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}$ as a factor of $\mathbf{I}_k -  \alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}$ plus a term that scales with $\alpha \beta^2$. 
% Therefore, if we can show that the coefficients of $\mathbf{I}_k -\alpha  \mathbf{B}_{t}^\top \mathbf{B}_{t}$ have spectral norm at most 1, then we will show that $\|\mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2$ is less than some threshold $\tau_2$ by choosing  $\beta$ sufficiently small. First,
Next, we show that the coefficients of $\mathbf{I}_k -\alpha  \mathbf{B}_{t}^\top \mathbf{B}_{t}$ have spectral norm strictly less than 1.
% \begin{align}
%     &\mathbf{I}_k -  \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}  \nonumber \\
%     &= \left(\mathbf{I}_k -  \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \left(\tfrac{1}{2}\mathbf{I}_k +\beta \mathbf{A} -  \beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t}  \right) +  \left(\tfrac{1}{2}\mathbf{I}_k + \beta \mathbf{A}^\top - \beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t}  \right) \left(\mathbf{I}_k - \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \nonumber \\
%     &\quad - (1-\alpha) \beta \mathbf{B}_{t}^\top \mathbf{B}_{t}\mathbf{A} -  (1-\alpha)\beta\mathbf{A} \mathbf{B}_{t}^\top \mathbf{B}_{t} + \beta^2 \nabla^\top \nabla \nonumber \\
%     % &= \left(\mathbf{I}_k -  \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \left(\tfrac{1}{2}\mathbf{I}_k + \beta \mathbf{A} - \beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t}  \right) +  \left(\tfrac{1}{2}\mathbf{I}_k + \beta \mathbf{A}^\top - \beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t}  \right) \left(\mathbf{I}_k - \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \nonumber \\
%     % &\quad - (1-\alpha)\beta\mathbf{B}_{t}^\top \mathbf{B}_{t}\left((\mathbf{u} - \mathbf{v})\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{B}_t^\top \mathbf{B}_t) + (1-\alpha) (\mathbf{u} - \mathbf{v})\mathbf{u}^\top +\alpha \mathbf{u}\mathbf{v}^\top-\alpha \mathbf{v}\mathbf{v}^\top\right) \nonumber \\
%     % &\quad -  (1-\alpha)\beta \left( (\mathbf{I}_k - \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t(\mathbf{u} - \mathbf{v})^\top + (1-\alpha) \mathbf{u}(\mathbf{u} - \mathbf{v})^\top +\alpha \mathbf{v}\mathbf{u}^\top-\alpha \mathbf{v}\mathbf{v}^\top \right) \mathbf{B}_{t}^\top \mathbf{B}_{t} + \beta^2 \nabla^\top \nabla \nonumber \\
%     &= \left(\mathbf{I}_k -  \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \left(\tfrac{1}{2}\mathbf{I}_k + \beta \mathbf{A}' - \beta \alpha \mathbf{vv}^\top  -  \beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t}  \right) +  \left(\tfrac{1}{2}\mathbf{I}_k + \beta (\mathbf{A}')^\top - \beta \alpha \mathbf{vv}^\top -  \beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t}  \right) \left(\mathbf{I}_k - \mathbf{B}_{t}^\top \mathbf{B}_{t}\right) \nonumber \\
%     &\quad - (1-\alpha)\beta\mathbf{B}_{t}^\top \mathbf{B}_{t}\left((\mathbf{u} - \mathbf{v})\mathbf{w}_t^\top (\mathbf{I}_k - \mathbf{B}_t^\top \mathbf{B}_t) + (1-\alpha) (\mathbf{u} - \mathbf{v})\mathbf{u}^\top +\alpha \mathbf{u}\mathbf{v}^\top-\alpha \mathbf{v}\mathbf{v}^\top\right) \nonumber \\
%     &\quad -  (1-\alpha) \beta \left( (\mathbf{I}_k - \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t(\mathbf{u} - \mathbf{v})^\top + (1-\alpha) \mathbf{u}(\mathbf{u} - \mathbf{v})^\top +\alpha \mathbf{v}\mathbf{u}^\top-\alpha \mathbf{v}\mathbf{v}^\top \right) \mathbf{B}_{t}^\top \mathbf{B}_{t} + \beta^2 \nabla^\top \nabla 
% \end{align}
From \eqref{imbt1}, we use the Cauchy-Schwarz and triangle inequalities to obtain
\begin{align}
    \left\| \mathbf{I}_k -  \alpha\mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \right\|_2 &\leq \left\| \mathbf{I}_k -  \alpha\mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2\left\| \mathbf{I}_k + 2\alpha \beta \mathbf{A}_t' - 2\beta \alpha^2 \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  \right\|_2  + \alpha \beta^2 \|\mathbf{G}_t\|_2^2 \label{32}
    % &\quad + %2(1-\alpha)\beta \|\mathbf{B}_{t}\|_2^2 \|\mathbf{A}\|_2 +
    % &\leq \left\| \mathbf{I}_k -  \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2\left\| \mathbf{I}_k + 2\beta \mathbf{A}' - 2\beta \alpha \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  -  2\beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 \nonumber \\
    % &\quad + 2\beta (1-\alpha)\| \mathbf{B}_t\|_2^2\left\| \mathbf{I}_k -  \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 L_{\max}(L_{\max} \| \mathbf{B}_t\|_2^2+ L_\ast \| \mathbf{B}_t\|_2) \nonumber \\
    % &\quad + 2\beta (1-\alpha)\| \mathbf{B}_t\|_2^2\big((1-\alpha)L_{\max}^2\|\mathbf{B}_t\|_2^4 + \|\mathbf{B}_t\|_2^3 L_{\max}L_\ast + \alpha \|\mathbf{B}_t\|_2^2 L_\ast^2   \big) \nonumber \\
    % &\quad +\beta^2 \|\nabla\|_2^2 \nonumber \\
    % &\leq \tau_2 \left\| \mathbf{I}_k + 2\beta \mathbf{A}' - 2\beta \alpha \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  -  2\beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 \nonumber \\
    % &\quad + 2\beta (1-\alpha)(1+\tau_2)\tau_2 L_{\max}(L_{\max} (1+\tau_2)+ L_\ast \sqrt{1+\tau_2}) \nonumber \\
    % &\quad + 2\beta (1-\alpha)(1+\tau_2)\big((1-\alpha)L_{\max}^2(1+\tau_2)^2 + (1+\tau_2)^{3/2} L_{\max}L_\ast + \alpha (1+\tau_2) L_\ast^2   \big) \nonumber \\
    % &\quad +\beta^2 \|\nabla\|_2^2 \nonumber \\
    % &= \tau_2 \left\| \mathbf{I}_k + 2\beta \mathbf{A}' - 2\beta \alpha \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  -  2\beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 \nonumber \\
    % &\quad + 2\beta (1-\alpha)(1+\tau_2)\big(L_{\max}^2(1+\tau_2)((1-\alpha)(1+\tau_2) + \tau_2) + (1+2\tau_2)\sqrt{1+\tau_2} L_{\max}L_\ast + \alpha (1+\tau_2) L_\ast^2   \big) \nonumber \\
    % &\quad +\beta^2 \|\nabla\|_2^2 \nonumber 
\end{align}
where 
\begin{align}
    &\left\| \mathbf{I}_k + 2\alpha \beta \mathbf{A}_t' - 2\beta \alpha^2 \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  \right\|_2 \nonumber \\
    &\leq 1 - 2 \beta \alpha^2 \sigma_{\min}^2\left(\frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top\right) + 2 \alpha \beta \|\mathbf{A}_t'\|_2 \nonumber \\
    &=1 - 2 \beta \alpha^2 \sigma_{\min}^2\left(\frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top\right)  + 2 \alpha \beta\tau_2 \left\| \frac{1}{n}\sum_{i=1}^n (\mathbf{u}_t-\mathbf{v}_{t,i})\mathbf{w}_t^\top\right\|_2  
    % 2\beta (1-\alpha)\left\| \frac{1}{n}\sum_{i=1}^n (\mathbf{u}_t-\mathbf{v}_{t,i})\mathbf{u}^\top\right\|_2 
    + 2 \beta \alpha^2 \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{u}_t\mathbf{v}_{t,i}^\top\right\|_2 \nonumber \\
    &\leq 1 - 2 \beta \alpha E_0 \mu_\ast^2(1-\tau_2)  + 2 \beta\tau_2 (1+\tau_2)\tau_1 + 2 \beta\tau_2 \sqrt{\alpha(1+\tau_2)} \sqrt{\tau_1}\eta_{\ast} % + 2\beta (1-\alpha)(1+\tau_2)^2 L_{\max}^2 
    + 2 \beta \sqrt{\alpha} (1+\tau_2)^{3/2} \sqrt{\tau_1}\eta_{\ast} \nonumber \\
    &\leq   1 - \beta \alpha E_0 \mu_\ast^2  + c\beta(\tau_1 \tau_2 + \sqrt{\tau_1\alpha}\eta_\ast) % + 2\beta (1-\alpha)(1+\tau_2)^2 L_{\max}^2
    .\label{first}
\end{align}
where the last inequality follows as long as $\tau_2 \leq  0.5$.




% {\color{red} need $\lambda > \kappa_\ast^2/\sqrt{\alpha}$, or, tighter: $\lambda > mean(wi*s)wt/(\sqrt{\alpha}\mu_\ast^2)$

% but now this interferes with convergence of distance

% empirically, regularization not necessary

% questions: can we complete the proof without regularization? can we anaylze second-order case?

% $\tau_2_2^2 \sqrt{\tau_2_1} > \tau_2_2^2 \eta$
% $\sqrt{\alpha} > \sqrt{\tau_2_1} $.. no

% conclusion: reg feels unnec for maml, just need to get rid of lambda > Lmax condition, the values of tau1 and tau2 will change with 2nd order update

% but for anil, it seems that we still need it, andwe still have issue with lambda being needed to be be tuned exactly

% need $\tau_2_1 \leq \sqrt{\alpha}$
% }



% Next, we have
% \begin{align}
%     \|\mathbf{A}_t\|_2 &\leq  \left\| \mathbf{I}_k - \alpha  \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 L_{\max}(L_{\max} \| \mathbf{B}_t\|_2^2+ L_\ast \| \mathbf{B}_t\|_2)  + \alpha \|\mathbf{B}_t\|_2^3 L_{\max}L_\ast + \alpha \|\mathbf{B}_t\|_2^2 L_\ast^2    \nonumber \\
%     % &\quad +\beta^2 \|\nabla\|_2^2 \nonumber \\
%     % &\leq \tau_2 \left\| \mathbf{I}_k + 2\beta \mathbf{A}' - 2\beta \alpha \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  -  2\beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 \nonumber \\
%     % &\leq  \tau_2 L_{\max}(L_{\max} (1+\tau_2)+ L_\ast \sqrt{1+\tau_2}) \nonumber \\
%     % &\quad + \big((1-\alpha)L_{\max}^2(1+\tau_2)^2 + (1+\tau_2)^{3/2} L_{\max}L_\ast + \alpha (1+\tau_2) L_\ast^2   \big) \nonumber \\
%     % &\quad +\beta^2 \|\nabla\|_2^2 \nonumber \\
%     % &= \tau_2 \left\| \mathbf{I}_k + 2\beta \mathbf{A}' - 2\beta \alpha \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i} \mathbf{v}_{t,i}^\top  -  2\beta \lambda \mathbf{B}_{t}^\top \mathbf{B}_{t} \right\|_2 \nonumber \\
%     &= \tau_2 \frac{1+\tau_2}{\alpha} L_{\max}^2 + \tau_2 \sqrt{\frac{1+\tau_2}{\alpha}}L_{\max}L_\ast + \frac{(1+\tau_2)^{3/2}}{\sqrt{\alpha}}L_{\max}L_\ast + (1+\tau_2)L_\ast^2 \label{A}
%     % \big(L_{\max}^2(1+\tau_2)((1-\alpha)(1+\tau_2) + \tau_2) + (1+2\tau_2)\sqrt{1+\tau_2} L_{\max}L_\ast + \alpha (1+\tau_2) L_\ast^2   \big) 
%     % &\quad +\beta^2 \|\nabla\|_2^2 \nonumber 
% \end{align}
Lastly, note that
\begin{align}
   \| \mathbf{G}_t \|_2 
  &= \left\|(\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top) \frac{1}{n} \sum_{i=1}^n (\mathbf{{B}}_t\mathbf{w}_t - \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} )\mathbf{w}_{t,i}^\top  \right\|_2 \nonumber \\
%   &= \left\|\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top\right\|_2 \|\mathbf{A}_t\|_2 + \alpha \lambda \left\|\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top\right\|_2 \|\mathbf{B}_t\|_2 \nonumber \\
%   &\leq \tau_2 (\tau_2 \frac{1+\tau_2}{\alpha} L_{\max}^2 + \tau_2 \sqrt{\frac{1+\tau_2}{\alpha}}L_{\max}L_\ast + \frac{(1+\tau_2)^{3/2}}{\sqrt{\alpha}}L_{\max}L_\ast + (1+\tau_2)L_\ast^2) + \lambda \tau_2 \sqrt{\alpha(1+\tau_2)} \\
    &=  \left\| \mathbf{{B}}_t(\mathbf{I}_k - \alpha  \mathbf{B}_t^\top \mathbf{B}_t )\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_t \mathbf{w}_{t,i}^\top\right) - (\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top ) \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2 \nonumber \\
    &\leq \left\| \mathbf{{B}}_t(\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t )\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_t \mathbf{w}_{t,i}^\top \right)\right\|_2 + \left\| (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top ) \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2 
    \label{firstsecond}
    \end{align}
    by the Cauchy-Schwarz inequality. The first term can be bounded as follows:
\begin{align}
  \left\| \mathbf{{B}}_t(\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t )\frac{1}{n} \sum_{i=1}^n \mathbf{w}_t \mathbf{w}_{t,i}^\top \right\|_2
&\leq \tau_2\sqrt{\frac{1+\tau_2}{\alpha}} \left\|\frac{1}{n} \sum_{i=1}^n \mathbf{w}_t \mathbf{w}_{t,i}^\top \right\|_2 \label{t12}  \\
&=
% \left\|\mathbf{w}_t \mathbf{w}_{t}^\top (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) +  \alpha \mathbf{w}_t\frac{1}{n} \sum_{i=1}^n  \mathbf{w}_{\ast,t,i} \mathbf{\hat{B}}_\ast \mathbf{B}_t - \lambda \mathbf{I}_k \right\|_2
\tau_2\sqrt{\frac{1+\tau_2}{\alpha}}\left( \left\|\mathbf{w}_t \mathbf{w}_{t}^\top (\mathbf{I}_k -  \alpha \mathbf{B}_t^\top \mathbf{B}_t)\right\| +  \alpha\left\|  \mathbf{w}_t\frac{1}{n} \sum_{i=1}^n  \mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t  \right\|_2\right)
\nonumber\\
&\leq \tau_2 \sqrt{\frac{1+\tau_2}{\alpha}}\left( \tau_1 \tau_2 +    \eta_\ast \sqrt{\tau_1 \alpha({1+\tau_2})} \right) \nonumber \\
&\leq c\left(\frac{\tau_1\tau_2^2}{\alpha} + \eta_\ast \tau_2 \sqrt{\tau_1}\right)\label{t11}
% &\leq 2 \tau_2 (L_\ast^2 +\sqrt{\alpha}\lambda) 
\end{align}
% where \eqref{t11} follows.
% from the facts $\mathbf{B}$   
For the second term in \eqref{firstsecond}, we first use 
$$ \left\| (\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top ) \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2 \nonumber \\
    \leq \left\| (\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top )\mathbf{\hat{B}}_\ast\right\|_2 \left\| \frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2
$$
then exploit the fact that $\| (\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top ) \mathbf{\hat{B}}_\ast\|_2$ can be upper bounded by the distance of $\mathbf{B}_t$ to $\mathbf{B}_\ast$ plus the extent to which $\sqrt{\alpha}\mathbf{B}_t$ is not orthonormal, as follows:
\begin{align}
    % &\left\| (\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top ) \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2 \nonumber \\
    \left\| (\mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top )\mathbf{\hat{B}}_\ast\right\|_2 &= \left\| (\mathbf{I}_d -  \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top )\mathbf{\hat{B}}_\ast + ( \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top - \alpha \mathbf{B}_t \mathbf{B}_t^\top )\mathbf{\hat{B}}_\ast\right\|_2  \nonumber \\
    &\leq 
    \left\| (\mathbf{I}_d -  \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top )\mathbf{\hat{B}}_\ast\right\|_2  + \left\| ( \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top - \alpha \mathbf{B}_t \mathbf{B}_t^\top )\mathbf{\hat{B}}_\ast\right\|_2  \nonumber \\
    &\leq \dist_t + \left\|  \mathbf{I}_k  - \alpha \mathbf{R}_t \mathbf{R}_t^\top \right\|_2  \nonumber \\
    &\leq  \dist_t  + \tau_2 \label{222}
\end{align}
where $\mathbf{R}_t \in \mathbb{R}^{k\times k}$ is the upper triangular matrix resulting from the QR factorization of $\mathbf{B}_t$, i.e. $\mathbf{B}_t = \mathbf{\hat{B}}_t \mathbf{R}_t$, and the last inequality follows because 
$ \left\|  \mathbf{I}_k  - \alpha \mathbf{R}_t \mathbf{R}_t^\top \right\|_2 \leq \max\left(1 - \alpha \tfrac{1-\tau_2}{\alpha}, \alpha \tfrac{1+\tau_2}{\alpha} - 1 \right) = \tau_2$.
Now, recall
\begin{align}
 \left\|\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2 &= \left\| \frac{1}{n} \sum_{i=1}^n  \alpha \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{{B}}_t +  \mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top(\mathbf{I}_k - \alpha \mathbf{{B}}_t^\top \mathbf{{B}}_t) \right\|_2  \nonumber \\ %+ (1-\alpha)\mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_t^\top\mathbf{{B}}_t^\top \mathbf{{B}}_t 
    &\leq  L_{\ast}^2 \sqrt{\alpha({1+\tau_2})} +  \eta_{\ast} \tau_2 \sqrt{\tau_1}   \nonumber \\
    &\leq c ( L_{\ast}^2 \sqrt{\alpha} +  \eta_{\ast} \tau_2 \sqrt{\tau_1}  )
    % \nonumber \\
    % &\leq 3 L_\ast^2 \sqrt{\alpha} 
    \label{33},
\end{align}
yielding an upper bound on the second term in \eqref{firstsecond} of 
\begin{align}
     \left\| (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top ) \frac{1}{n} \sum_{i=1}^n \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top  \right\|_2 \leq 3 (\dist_t  + \tau_2)(L_\ast^2 \sqrt{\alpha}+\eta_\ast \tau_2 \sqrt{\tau_1}),
\end{align}
% for some absolute constant $c$, under the construction $\tau_2 \leq \sqrt{\alpha}$.
% where \eqref{where} follows since $\| \mathbf{I}_d -  \alpha \mathbf{B}_t \mathbf{B}_t^\top \|_2 \leq \max(1, \tau_2)\leq 1$.
% NEED TO CHOOSE $\beta = 1/L_\ast, \alpha=1/L_\ast$, $\tau_2=c$ 
which when combined with \eqref{firstsecond} and \eqref{t11} results in %\eqref{t11} and \eqref{222} and \eqref{33} yields
\begin{align}
    \| \mathbf{G}_t \|_2^2 &\leq  
   ( \tau_2^2\tau_1/\alpha + \eta_\ast \tau_2 \sqrt{\tau_1} + (\dist_t + \tau_2)L_\ast^2\sqrt{\alpha})^2 %\nonumber\\
   %&\leq    \label{Phi}. 
%     \Bigg( 2  \tau_2 (L_\ast^2 +\sqrt{\alpha}\lambda)
%     % \tau_2\sqrt{{1+\tau_2}} \left( L_{\max}^2 (\tau_2 +(1-\alpha)(1+\tau_2)) + \lambda +  (1-\alpha) L_{\max} L_\ast \sqrt{{1+\tau_2}} \right) \nonumber \\
%  + 3 (\dist_t + \tau_2) L_{\ast}^2 \sqrt{\alpha} \Bigg)^2%\alpha L_{\ast}^2 \sqrt{{1+\tau_2}} +  L_{\ast} L_{\max}(\tau_2 + (1-\alpha)(1+\tau_2))
    % \nonumber \\
    % &\leq 10 \tau_2^2 (L_\ast^2 +\sqrt{\alpha}\lambda)^2 + 10{\alpha} \dist_t^2 L_{\ast}^4  \label{Phi}. 
\end{align}
%note this scales as $(\sqrt{\alpha})^2$.
Combining \eqref{32}, \eqref{first} and \eqref{Phi} yields
\begin{align}
   \|\mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2 
   &\leq \left(
   1 - \beta \alpha E_0 \mu_\ast^2 + c \beta \tau_1\tau_2 + c\beta \sqrt{\alpha\tau_1} \eta_{\ast} + c \beta^2 \alpha^2 \tau_2 L_\ast^4\right)\|\mathbf{I}_k\!-\!\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2   
     \!+\!10  \beta^2 \alpha^2 \dist_t^2 L_\ast^4. \label{tight_reg}
\end{align}
Finally, recalling that $\tau_1$ is any upper bound on $\|\mathbf{w}_t\|_2^2$, we replace $\tau_1$ with $\frac{\beta^2}{\alpha}\kappa^8 \eta_{\ast}^2$ due to inductive hypothesis $A_1(t)$ to obtain
\begin{align}
    \|\mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2  
   &\leq \left(
   1 - \beta \alpha E_0 \mu_\ast^2 + c \tfrac{\beta^3}{\alpha}\kappa_\ast^8 \eta_{\ast}^2\tau_2 + c\beta^2 \kappa_\ast^4 \eta_{\ast}^2 + c \beta^2 \alpha^2 \tau_2 L_\ast^4\right)\|\mathbf{I}_k\!-\!\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2   
     \!+\!10 \beta^2 \alpha^2 \dist_t^2 L_\ast^4 \label{tight_reg}
    %  &\leq \left(1 - \beta \alpha E_0 \mu_\ast^2 + c \tfrac{\beta^2}{\alpha}\kappa_\ast^8 \eta_{\ast}\tau_2 + c\beta^2 \kappa_\ast^4 \eta_{\ast}^2 + c \beta^2 \alpha^2 \tau_2 L_\ast^4\right)\|\mathbf{I}_k\!-\!\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2   
    %  \!+\! 10 \beta^2 \alpha^2 \dist_t^2 L_\ast^4 \label{tight_reg}
\end{align}
% where the second line follows as long as $\beta \leq \frac{1}{\eta_\ast}$. We next enforce an even tighter bound on $\beta$ in order to ensure $\|\mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2 \leq \tau_2$:
% % choosing % a b2 + d b - c < -
% % b < (d + sqrt(d2 - 4 a c))/(2a)
% \begin{align}
%     \beta &\leq  c\frac{\alpha E_0 \mu_\ast^2 \tau_2 
%   }{ \kappa_{\ast}^8\eta_\ast \tau_2^2/\alpha +\kappa_{\ast}^4\eta_\ast^2\tau_2 + \alpha^2 \tau_2^2 L_\ast^4  +\alpha^2 L_{\ast}^4}
% %     c\frac{\alpha E_0 \mu_\ast^2  - c \tau_1\tau_2 -c \sqrt{\alpha\tau_1} L_{\ast} 
% %   }{ \alpha \tau_2 (L_\ast^2 +\sqrt{\alpha}\lambda)^2}
% %     \nonumber  %\\
% \end{align}
% % {\color{red} need to replace $\tau_1$ with $\tau_1 \leq \frac{\beta^2}{\alpha}L_\ast^8\eta_\ast^2$}
% is necessary 
to complete the proof. 

% ------

% However, later we will need a different  bound on $\beta$ to ensure that 
% $\|\mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2$ remains less than $\tau_2$ (Corollary \ref{cor:reg}). So, we choose $\beta$ such that it is less than the  minimum of these bounds
% \begin{align}
%     \beta &\leq \frac{\tau_2 \alpha E_0 \mu_\ast^2 - c \tau_1\tau_2^2 -c \tau_2 \sqrt{\alpha\tau_1} L_{\ast}
%   }{20 \alpha \tau_2 (L_\ast^2 +\sqrt{\alpha}\lambda)^2 + 10 \alpha^2 \dist_t^2 L_\ast^4} \nonumber \\
%   &\leq 
%   \min\left(c\frac{\alpha E_0 \mu_\ast^2 - c \tau_1\tau_2 -c \sqrt{\alpha\tau_1} L_{\ast} 
%   }{ \alpha L_\ast^4},  \frac{\tau_2 E_0 \mu_\ast^2  - 10 \tau_2 \sqrt{\alpha} L_{\ast}^2 
%   }{20 \alpha \tau_2^2 L_\ast^4 + 10 \alpha^2 \dist_t^2 L_\ast^4}  \right).
%     \nonumber 
% \end{align}
% Note that we implicitly assume $E_0 \mu_\ast^2 > c\tau_1\tau_2 -c \sqrt{\alpha\tau_1} L_{\ast} $  (note that $\alpha$ can be chosen sufficiently large to achieve this, since we will choose $\mu_\ast$ and $\tau_1,\tau_2$ as functions of $\al0pha$).
% % ensures contraction of the $\|\mathbf{I}_k\!-\!\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2$ term.

% -----


% We need the following two inequalities to hold simultaneously:
% \begin{align}
%      \alpha^2 E_{0}\mu_\ast^2 (1-\tau_2)  &>  2\alpha (\tau_2 + (1-\alpha)(1+\tau_2) ) \sqrt{(1+\tau_2)}L_{\max} L_{\ast} + \lambda \tau_2  \\
%      \tau_2(\alpha E_0 \mu_\ast^2+ \lambda) (1-\tau_2)  
%   &>  L_{\max}^2 (1+\tau_2)\bigg((1-\alpha)(1+\tau_2)\left(1 -\alpha -\alpha\tau_2 + 3\tau_2 \right)+\tau_2^2\bigg)  \nonumber \\
%     &\quad + L_{\ast}^2(1-\alpha)\alpha(1+\tau_2)^2 \nonumber \\
%     &\quad + L_{\max}L_{\ast}  (1+2\tau_2)\sqrt{1+\tau_2} \bigg((1-\alpha)(1+\tau_2) +\tau_2 \bigg)
% \end{align}
% large $\lambda$ is necessary to kill the last term (consider $\alpha=1$).
% First inequality is for contraction. Second inequality is to ensure that we can choose a positive outer loop step size such that the spectrum will not increase beyond $\tau_2$.
% -------------------------
% \subsection{Warm Up: Infinite Sample Case}
% We start by considering the infinite sample case, wherein $m_{in}\!=\!m_{out}\!=\!\infty$. 
% \begin{thm}
% Suppose we run ANIL in the multi-task linear representation learning setting with $n$ tasks sampled per round and $m_{in}\!=\!m_{out}\!= \!\infty$. Let $E_0\!\coloneqq\! 1\! -\! \dist(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)$. Further, let $\mu_\ast^2 \coloneqq  1 - C\frac{k + 10\log(T)}{n}$ and $L_\ast^2 \coloneqq  1 + C\frac{k + 10\log(T)}{n}$ for some absolute constant $C$. Then for any $\alpha\leq $ and any $\beta \in (0,\nicefrac{1}{L_{\ast}^2}]$, we have that after $T$ iterations,
% \begin{align}
%     \dist(\mathbf{{B}}_T, \mathbf{{B}}_\ast) \leq (1 - \beta E_0 \mu_\ast^2)^{T-1} \dist(\mathbf{{B}}_0, \mathbf{{B}}_\ast).
% \end{align}
% with probability at least $1 - 2 T^{-99}$.
% \end{thm}
% Thus, for appropriate choice of $\beta$, we obtain a contraction factor that depends on $\frac{\mu_{\ast}^2}{L_\ast^2}$. This suggests that the more diverse the tasks, the faster that ANIL converges to the ground-truth representation. The proof sketch follows below.
% \begin{proof}[Proof]
% We provide a proof overview and defer minor details to Appendix \ref{app:anil}.
%  {\color{red} need to change proof structure to align with finite-sample proof}




We have 
\begin{align}
    \mathbf{B}_t^\top \mathbf{G}_t &= \del_t\mathbf{B}_t^\top \mathbf{e}_t \mathbf{w}_t^\top\del_t - \alpha \mathbf{B}_t^\top \mathbf{B}_t(\mathbf{w}_t\mathbf{v}_{t,i}^\top \mathbf{B}_t+ \mathbf{B}_t^\top\mathbf{v}_{t,i}\mathbf{w}_t^\top ) \nonumber \\
    &\quad + \alpha \del_t \mathbf{B}_t \mathbf{w}_t\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top \mathbf{B}_t -  \alpha \del_t \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top \mathbf{B}_t + \alpha \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t}^\top \mathbf{B}_t^\top \mathbf{B}_t \del_t  - \alpha \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \del_t
\end{align}

For $\dist$, the good term is again the same, use $-\alpha\mathbf{B}_t^\top \mathbf{B}_t$ part. Analysis is easy.

same values of tau1 tau2 as for exact maml.







----

only thing that changes is the outer loop update of $\mathbf{w}_{t+1}$. Now we have 
\begin{align}
    \mathbf{w}_{t+1}&= \left(\mathbf{I}_k - \beta (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t) \mathbf{B}_t^\top \mathbf{B}_t(\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t)\right) \mathbf{w}_t + \beta (\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t)^2\mathbf{B}_t^\top \mathbf{B}_\ast \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}
\end{align}
In the analysis this only affects the bound on $\|\mathbf{w}_t\|_2$ (Lemma 10). But this is easy to modify, and in fact we can show a tighter bound in terms of constants, since the new update helps keep $\mathbf{w}_{t}$ closer to zero. Again, the regularization is unnecessary.




\begin{comment}
We have, for sufficiently small $\beta$,
\begin{align}
\left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 &\leq 1 - \sigma_{\min}\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) \nonumber \\
&= 1 - \frac{\beta}{n} \sigma_{\min}\left( \sum_{i=1}^n \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{S}_{t,i} \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{S}_{t,i}^\top  + \alpha^2 \mathbf{S}_{t,i} \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{S}_{t,i}^\top \right)
\end{align}
With full measurements and orthogonal $\mathbf{B}_t$, we have $\mathbf{P}_{t,i} = (1- \alpha)\mathbf{I}_k$ and $\mathbf{S}_{t,i} = \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast$ for all $i \in [n]$. Then
\begin{align}
    &\lambda_{\min}\left( \sum_{i=1}^n \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{S}_{t,i} \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{S}_{t,i}^\top  + \alpha^2 \mathbf{S}_{t,i} \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{S}_{t,i}^\top \right) \nonumber \\
    &= \lambda_{\min}\left(n(1-\alpha)^2 \mathbf{w}_t \mathbf{w}_t^\top + \alpha(1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}\right)\mathbf{w}_t^\top  + \alpha(1-\alpha)  \mathbf{w}_t\sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}^\ast\right) \mathbf{\hat{B}}_\ast \mathbf{\hat{B}}_t^\top + \alpha^2 \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n\left(\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \right) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right)  \nonumber \\
    &\geq \lambda_{\min}\left( \alpha(1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}\right)\mathbf{w}_t^\top  + \alpha(1-\alpha)  \mathbf{w}_t\sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}^\ast\right)^\top \mathbf{\hat{B}}_\ast \mathbf{\hat{B}}_t^\top + \alpha^2 \mathbf{\hat{B}}_t \mathbf{\hat{B}}_\ast^\top \sum_{i=1}^n\left(\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \right) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right)  \label{ge1}\\
     &\geq \lambda_{\min}\left( \alpha(1-\alpha) \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}\right)\mathbf{w}_t^\top  + \alpha(1-\alpha)  \mathbf{w}_t\sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}^\ast\right)^\top \mathbf{\hat{B}}_\ast \mathbf{\hat{B}}_t^\top\right) +\lambda_{\min}\left( \alpha^2 \mathbf{\hat{B}}_t \mathbf{\hat{B}}_\ast^\top \sum_{i=1}^n\left(\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \right) \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) \\
     &\geq  -2\alpha (1- \alpha)  \left\| \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}\right)\mathbf{w}_t^\top   \right\|_2 + \alpha^2 \sigma_{\min}\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t \right)  \label{ge2} %\\
    % &\geq \alpha^2 \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\right)  \sigma_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top  \right) + 2 \alpha (1- \alpha) \sigma_{\min} \left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}\right)\mathbf{w}_t^\top  \right) \label{ge3} \\
    % &\geq \alpha^2\left( 1 - \text{dist}(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)\right)^2 \lambda_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \right) \nonumber
\end{align}
where \eqref{ge1} follows because $n(1-\alpha)^2 \mathbf{w}_t \mathbf{w}_t^\top$ is PSD, and  \eqref{ge2} follows by Weyl's Inequality.
Note that
\begin{align}
    \left\| \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n \left(\mathbf{w}_{\ast,t,i}\right)\mathbf{w}_t^\top   \right\|_2 &\leq  n \; %\text{dist}(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast)
\end{align}
since if $\|\mathbf{w}_0\|_2 = \|\mathbf{w}_{\ast,1}\|_2 = \dots =\|\mathbf{w}_{\ast,n}\|_2 = 1$, then we can easily show that $\|\mathbf{w}_t\|_2 \leq 1$ for all $t$ as long as $\beta \leq 1/(1-\alpha)$. Meanwhile,
\begin{align}
   \sigma_{\min}\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t \right) &\geq \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\right)  \sigma_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top  \right) \nonumber \\
   &\geq \left( 1 - \text{dist}^2(\mathbf{\hat{B}}_0, \mathbf{\hat{B}}_\ast)\right) \sigma_{\min}\left(\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \right) \nonumber \\
   &\geq E_0 n\mu_\ast^2 
\end{align}
where the last inequality follows from the assumption of task diversity. Thus we have
\begin{align}
    \left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 &\leq 1  + 2\beta \alpha(1-\alpha)  -  \beta \alpha^2 E_0 \mu_\ast^2    \label{contract}
\end{align}
We will set $\alpha =1$ to achieve contraction, but first 
we must show that $\|\mathbf{R}_{t+1}^{-1}\|_2$ is small, or equivalently, $\sigma_{\min}(\mathbf{R}_{t+1})$ is large. First, write
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\right)\mathbf{w}_{t,i}^\top
\end{align}
Then
\begin{align}
    \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
    &= \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t - \mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber \\
    &= \mathbf{I}_{k} - \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber
\end{align}
Note that for $\alpha = 1$, 
\begin{align}
    \mathbf{w}_{t,i} = \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}
\end{align}
so the cross terms are zero, i.e.
\begin{align}
    \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\right)\mathbf{w}_{t,i}^\top = \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,t,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) = \mathbf{0}.
\end{align}
and we have, since the $O(\beta^2)$ term is PSD,
\begin{align}
    \sigma_{\min}\left(\mathbf{R}_{t+1}^\top \mathbf{R}_{t+1}\right) &\geq 1
\end{align}

\begin{align}
\left\|  \mathbf{I}_k -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right\|_2 &\leq 1 - \sigma_{\min}\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) \nonumber \\
&= 1 - \frac{\beta}{n} \sigma_{\min}\left( \sum_{i=1}^n \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{S}_{t,i} \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top \mathbf{P}_{t,i}^\top  + \alpha \mathbf{P}_{t,i} \mathbf{w}_t \mathbf{w}_{\ast,t,i}^\top \mathbf{S}_{t,i}^\top  + \alpha^2 \mathbf{S}_{t,i} \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{S}_{t,i}^\top \right)
\end{align}
\end{comment}




% \textbf{Inductive hypothesis 1:} Note that 
% \begin{align}
%     \|\mathbf{w}_{t+1}\|_2 &= \left\|\mathbf{w}_t - \alpha(1- \alpha)\mathbf{w}_t +  \frac{\alpha - \alpha^2 }{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,t,i}\right\|_2 \nonumber \\
%     &\leq (1 - \alpha+\alpha^2)\|\mathbf{w}_t\|_2 + (\alpha - \alpha^2) \left\|\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \right\|_2\left\|\frac{1}{n}\sum_{i=1}^n  \mathbf{w}_{\ast,t,i}\right\|_2 \label{cstri1}\\
%     &\leq (1 - \alpha+\alpha^2) L_\ast + (\alpha - \alpha^2) L_\ast \label{ind1} \\
%     &= L_\ast
% \end{align}
% where \eqref{cstri1} follows from the Cauchy-Shwarz and triangle ineqaulities, and \eqref{ind1} follows from the fact that we are conditioning on the event $A$, and $\|\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\|_2 = \|\frac{1}{n}[\mathbf{w}_{\ast,t,1}, \dots, \mathbf{w}_{\ast,t,n}] \mathbf{1}_n\|_2 \leq \|\frac{1}{\sqrt{n}}[\mathbf{w}_{\ast,t,1}, \dots, \mathbf{w}_{\ast,t,n}]\|_2 \|\frac{1}{\sqrt{n}} \mathbf{1}_{n}\|_2 \leq L_\ast$. 
% \end{comment}





% Xo BBT Xi B, BT Xi Xo 

% the question is, how do we utilize n?

% delta

% axb y cxd - axb cxd < small

% want:
% axb y cxd - abcd < small

% axb y cxd - axb cxd + axb cxd - abcd

% 1/n sum axibcxid - axibcd
% we have a sum of n random matrices with 
% nonzero mean
% but mean approaches zero with min

% sum of n min2 random variables
% we can deal with n min (min - 1) of them
% we have


% 1/(n min2) sum  - (n min (min-1))/(n min2) avg --> 0
% {\em use truncation argument}

% [+ 1/(n min2) sum  - n min/(n min2) avg]

% <= | 1/(n min2) sum | + [1/min |avg|] -- fine


% the mean of each term is upper bounded by k by L4-L2 hypercontractivity.
% so we can reduce to the sum of n min random variables with mean zero.

% each variable is the fourth product of dependent subgaussian random random variables.

% we should be able to control this.

% just use boundedness. nope we have d.

% want a bound on uvT. 

% xxT B xxT BwwT
% u = (xT B x) x, v = wwTBTx

% z = [u; v]
% we have bound on zzT = [ uuT uvT; vuT vvT ] = [ 0 uvT; vuT 0 ] + PSD
% thus ||[ 0 uvT; vuT 0 ]|| \leq ||[ uuT uvT; vuT vvT ]|| \leq bound
% x1T uvT x2 \leq bound vor all x1, x2.... done

% S < t
% implied by 
% 1/n sum xi < t
% 1/n sum xi < t



% BXBBXB = BXBBXB - BBBB + BBBB 
% = BXBBXB - BXBBB + BXBBB - BBBB + BBBB 
% avg yi xi yi - 1 is small
% = avg yi xi yi - avg yi2 + avg yi2 - 1
% = 

% P(|| A X B X C - ABC || leq small)
% P( || ||)

% P(avg yi xi yi - 1 is small) = P(avg yi xi yi - 1 is small | avg yi < m )P(  )


Proof outline for Exact ANIL and FO-MAML:

First show concentration of outer loop samples at a rate of dk/(min rt(n mout))

Then show concentration of inner loop samples: 

- result will be c/min + 2 rt(dk/(n min)) + E[]/rt(n min)
\cite{magen2011low, rudelson2007sampling}

- to control expectation, use L4-L2 hypercontractivity. mean will be c k/min

General lemmas:

bound matrices of the form:



\begin{lemma}[Exact ANIL] \label{lem:w_anil_fs_exact}
For any $t$, suppose that the events
\begin{align}
A_2(s) &\coloneqq \{\| \mathbf{I}_k-\alpha \mathbf{B}_s^\top \mathbf{B}_s  \|_2 \leq (1 - 0.5 \beta  E_0 \mu_\ast^2  + 5 \beta \sqrt{\alpha} L_{\ast}^2)\|\mathbf{I}_k - \alpha \mathbf{B}_{s-1}^\top \mathbf{B}_{s-1} \|_2 \nonumber \\
 &\quad\quad \quad \quad \quad \quad \quad \quad \quad \quad  + 10 \alpha^2 \beta^2 L_\ast^4 \dist_{s-1}^2\},
\nonumber \\
A_3(s) &\coloneqq \{\| \mathbf{I}_k-\alpha \mathbf{B}_s^\top \mathbf{B}_s  \|_2 \leq \tau\}, \nonumber \\
 A_5(s) &\coloneqq \{\dist(\mathbf{B}_s, \mathbf{\hat{B}}_\ast) \leq \left(1 - \beta \left(0.5 \alpha E_0 \mu_\ast^2 - 3  \tau \sqrt{\alpha} L_\ast^2  \right) \right)^{s-1}\}
 \end{align}
hold for all $s\in[t]$.
Then
\begin{align}
    \|\mathbf{w}_{t+1}\|_2 \leq \sqrt{\tau_1}
\end{align}
with probability at least  .
\end{lemma}

\begin{proof}
The exact ANIL proof is similar to the FO-ANIL proof. Recall the outer loop updates for ANIL from \eqref{anil_e_b_exact} and \eqref{anil_e_w_exact}. (here we replace $t$ with $s$): 
\begin{align}
\mathbf{w}_{s+1} &= (\mathbf{I}_{k} - \beta (\mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s ) \mathbf{B}_s^\top\mathbf{B}_s (\mathbf{I}_k-\alpha\mathbf{B}_s^\top\mathbf{B}_s)) \mathbf{{w}}_{s} + \beta (\mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s )^2  \mathbf{B}_s^\top \mathbf{\hat{B}}_\ast\frac{1}{n}\sum_{i=1}^n\mathbf{{w}}_{\ast,s,i}  \nonumber \\
    &\quad + \alpha\beta\left( \mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s \right)\mathbf{B}_s^\top\mathbf{B}_s
    \frac{1}{n}\sum_{i=1}^n\left( \mathbf{B}_s^\top\mathbf{B}_s -  \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{in}\mathbf{B}_s\right)\mathbf{w}_s \nonumber \\
    &\quad - \alpha \beta \left( \mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s \right)\mathbf{B}_s^\top\mathbf{B}_s \frac{1}{n}\sum_{i=1}^n (\mathbf{B}_s^\top \mathbf{B}_\ast - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{in}\mathbf{B}_\ast) \mathbf{w}_{\ast,s,i}\nonumber \\
    &\quad +  \alpha \beta \left( \mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s \right)\mathbf{B}_s^\top\mathbf{B}_s\frac{1}{n}\sum_{i=1}^n \mathbf{B}_s^\top (\mathbf{X}_{s,i}^{in})^\top \mathbf{z}_{s,i}^{in} \nonumber \\
&\quad + (\mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s )\frac{\beta}{n}\sum_{i=1}^n (\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s ^\top\mathbf{\Sigma}_{s,i}^{out,g} \mathbf{B}_s )  \mathbf{{w}}_{s,i} \nonumber \\
&\quad - (\mathbf{I}_k - \alpha\mathbf{B}_s^\top\mathbf{B}_s )\frac{\beta}{n}\sum_{i=1}^n  (\mathbf{B}_s ^\top \mathbf{\hat{B}}_\ast - \mathbf{B}_s ^\top  \mathbf{\Sigma}_{s,i}^{out,g} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,s,i} \nonumber \\
&\quad +   (\mathbf{I}_k - \alpha \mathbf{B}_s^\top\mathbf{B}_s)\frac{2\beta}{nm_{out}} \sum_{i=1}^n \mathbf{B}_s^\top (\mathbf{X}_{s,i}^{out,g})^\top \mathbf{z}_{s,i}^{out,g} \nonumber  \\
&\quad - \alpha \frac{\beta}{n}\sum_{i=1}^n(\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s ) (\mathbf{B}_s^\top\mathbf{B}_s  \mathbf{{w}}_{s,i} -  \mathbf{B}_s^\top \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,s,i})  \nonumber \\
&\quad + \alpha \frac{\beta}{n}\sum_{i=1}^n (\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s )(\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s ^\top\mathbf{\Sigma}_{s,i}^{out,g} \mathbf{B}_s )  \mathbf{{w}}_{s,i} \nonumber \\
&\quad + \alpha \frac{\beta}{n}\sum_{i=1}^n  (\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s )(\mathbf{B}_s ^\top \mathbf{\hat{B}}_\ast - \mathbf{B}_s ^\top  \mathbf{\Sigma}_{s,i}^{out,g} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,s,i}\nonumber \\
&\quad + \alpha \frac{2\beta}{nm_{out}} \sum_{i=1}^n  (\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s)\mathbf{B}_s ^\top (\mathbf{X}_{s,i}^{out,g})^\top \mathbf{z}_{s,i}^{out,g} 
\end{align}

Let $a_s \coloneqq \|\mathbf{w}_s\|_2$ and $b_s\coloneqq \|\mathbf{I}_k - \alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2$ for all $s\in\{0,\dots,t\!+\!1\}$. Note that $\bigcup_{s=0}^t A_3(s)$ implies $\sigma_{\max}(\mathbf{B}_s^\top \mathbf{B}_s) \leq \frac{1+\tau}{\alpha}< \frac{2}{\alpha}$ for all $s\in\{0,\dots,t\!+\!1\}$. Also, can straightforwardly use Lemma \ref{lem:basic_concen} with the Cauchy-Schwartz inequality to obtain
\begin{align}
       \Bigg\| \alpha\beta( \mathbf{I}_k - &\alpha\mathbf{B}_t^\top\mathbf{B}_t )\mathbf{B}_t^\top\mathbf{B}_t
    \frac{1}{n}\sum_{i=1}^n\left( \mathbf{B}_t^\top\mathbf{B}_t -  \mathbf{B}_t^\top\mathbf{\Sigma}_{t,i}^{in}\mathbf{B}_t\right)\mathbf{w}_t \Bigg\|_2
    \leq \frac{\beta}{\alpha} b_s a_s \frac{\delta_{in}}{\sqrt{n}} \nonumber \\
    \Bigg\|\alpha \beta ( \mathbf{I}_k - &\alpha\mathbf{B}_t^\top\mathbf{B}_t )\mathbf{B}_t^\top\mathbf{B}_t \frac{1}{n}\sum_{i=1}^n (\mathbf{B}_t^\top \mathbf{B}_\ast - \mathbf{B}_t^\top\mathbf{\Sigma}_{t,i}^{in}\mathbf{B}_t) \mathbf{w}_{\ast,t,i}\Bigg\|_2 \leq \frac{\beta}{\sqrt{\alpha}}  b_s L_\ast {\delta_{in}}
\end{align}
\begin{align}
\Bigg\|(\mathbf{I}_k - &\alpha\mathbf{B}_s^\top\mathbf{B}_s )\frac{\beta}{n}\sum_{i=1}^n  (\mathbf{B}_s ^\top \mathbf{\hat{B}}_s - \mathbf{B}_s ^\top  \mathbf{\Sigma}_{s,i}^{out,g} \mathbf{\hat{B}}_s) \mathbf{{w}}_{s,i}\Bigg\|_2 \nonumber \\
&\leq \frac{\beta}{\alpha} b_s \delta_{out,k}\max_{i\in[n]}\|\mathbf{w}_{s,i}\|_2 \nonumber \\
&\leq \frac{\beta}{\alpha} b_s \delta_{out,k}(\|\mathbf{I}_k\!-\!\alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2 a_s\!+\!\sqrt{\alpha} L_{\max} + \delta_{in}a_s\!+\!\sqrt{\alpha} \delta_{in} L_{\max} +\sqrt{\alpha} \sigma \delta_{in}) \nonumber \\
&\leq \frac{\beta}{\alpha} b_s \delta_{out,k}(b_s a_s\!+\!2\sqrt{\alpha} L_{\max} + \delta_{in}a_s+\sqrt{\alpha} \sigma \delta_{in}) \\
\Bigg\|(\mathbf{I}_k -& \alpha\mathbf{B}_s^\top\mathbf{B}_s )\frac{\beta}{n}\sum_{i=1}^n  (\mathbf{B}_s ^\top \mathbf{\hat{B}}_\ast - \mathbf{B}_s ^\top  \mathbf{\Sigma}_{s,i}^{out,g} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,s,i}\Bigg\|_2 \leq \frac{\beta}{\sqrt{\alpha}} b_s L_{\max} \delta_{out,k} \nonumber \\
\Bigg\|  (\mathbf{I}_k - &\alpha \mathbf{B}_s^\top\mathbf{B}_s)\frac{2\beta}{nm_{out}} \sum_{i=1}^n \mathbf{B}_s^\top (\mathbf{X}_{s,i}^{out,g})^\top \mathbf{z}_{s,i}^{out,g}\Bigg\|_2 \leq  \frac{\beta}{\sqrt{\alpha}} b_s \sigma \frac{\delta_{out,k}}{\sqrt{n}} \nonumber \\
\Bigg\|\alpha \frac{\beta}{n}\sum_{i=1}^n &(\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s ) (\mathbf{B}_s^\top\mathbf{B}_s  \mathbf{{w}}_{s,i} -  \mathbf{B}_s^\top \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,s,i}) \Bigg\|_2  \nonumber \\
&\leq {\beta} \delta_{out,k}\left(\frac{1}{\alpha}(b_s a_s + 2\sqrt{\alpha}L_{\max}+\delta_{in}a_s +\sqrt{\alpha} \sigma \delta_{in})+\frac{1}{\sqrt{\alpha}}L_{\max} \right) \nonumber \\
\Bigg\| \alpha \frac{\beta}{n}\sum_{i=1}^n &(\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s )(\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s ^\top\mathbf{\Sigma}_{s,i}^{out,g} \mathbf{B}_s )  \mathbf{{w}}_{s,i} \Bigg\|_2 \nonumber \\
&\leq  \frac{\beta}{\alpha}\delta_{out,k}^2(b_s a_s + 2\sqrt{\alpha}L_{\max}+\delta_{in}a_s+\sqrt{\alpha} \sigma \delta_{in})\nonumber \\
\Bigg\|\alpha \frac{\beta}{n}\sum_{i=1}^n &  (\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s )(\mathbf{B}_s ^\top \mathbf{\hat{B}}_\ast - \mathbf{B}_s ^\top  \mathbf{\Sigma}_{s,i}^{out,g} \mathbf{\hat{B}}_\ast) \mathbf{{w}}_{\ast,s,i}\Bigg\|_2 \leq \frac{\beta}{\sqrt{\alpha}} L_{\max}\delta_{out,k}^2 \nonumber \\
\Bigg\|\alpha \frac{2\beta}{nm_{out}} &\sum_{i=1}^n  (\mathbf{B}_s^\top\mathbf{B}_s - \mathbf{B}_s^\top\mathbf{\Sigma}_{s,i}^{out,h}\mathbf{B}_s)\mathbf{B}_s ^\top (\mathbf{X}_{s,i}^{out,g})^\top \mathbf{z}_{s,i}^{out,g}  \Bigg\|_2 \leq \frac{\beta}{\sqrt{\alpha}}\sigma \delta_{out,k}^2
\end{align}
with probability at least $1- $,
where we have used the independence of the samples used for the Hessian estimation, outer loop gradient estimation, and inner loop gradient estimations. Summing these inequalities yields
\begin{align}
    a_{s+1}&\leq a_s + \frac{\beta}{\sqrt{\alpha}}b_s^2 \eta_\ast + \frac{\beta}{\alpha}b_sa_s\frac{\delta_{in}}{\sqrt{n}} +  \frac{\beta}{\sqrt{\alpha}}  b_s L_\ast {\delta_{in}}+ c\frac{\beta}{\alpha} \delta_{out,k}(b_s a_s + c\sqrt{\alpha} L_{\max} + \delta_{in} a_s+\sqrt{\alpha} \sigma \delta_{in})  \nonumber \\
    &\quad + \frac{\beta}{\sqrt{\alpha}}b_s \sigma\delta_{out,k} \nonumber \\
    &= \left(1 + \frac{\beta}{\alpha}(b_s \delta_{out,k} +\delta_{in}\delta_{out,k} + b_s\tfrac{\delta_{in}}{\sqrt{n}}) \right)a_s + \frac{\beta}{\sqrt{\alpha}}\left(L_\ast \delta_{in} + \sigma \delta_{out,k} +b_s \eta_\ast \right)b_s  \nonumber \\
    &\quad + \frac{\beta}{\sqrt{\alpha}}L_{\max}\delta_{out,k} + \frac{\beta}{\sqrt{\alpha}}\sigma \delta_{out,k} \delta_{in}  \nonumber \\
    &= a_s + \frac{\beta}{\sqrt{\alpha}}b_s^2 \eta_{\ast} + \frac{\beta}{\alpha}\nu_s
\end{align}
where $\nu_s \coloneqq (b_s \delta_{out,k} +\delta_{in}\delta_{out,k} + b_s\tfrac{\delta_{in}}{\sqrt{n}})a_s+
\sqrt{\alpha}(L_\ast \delta_{in}b_s+ \sigma \delta_{out,k}b_s + L_{\max}\delta_{out,k} + \sigma \delta_{out,k} \delta_{in} )$. 

We have 
\begin{align}
    b_{t+1} &\leq (1 - \beta E_0 \mu_{\ast}^2 + \beta \sqrt{\alpha}L_{\ast}^2)b_t +\alpha^2 \beta^2 \dist_t^2 L_{\ast}^4 + \alpha \beta  (L_{\max} + \sigma) \left(  L_{\max}\frac{\delta_{out,k}+\delta_{in}}{\sqrt{ n}} +  \left(\frac{a_t}{\sqrt{\alpha}}+\sigma\right)\delta_{in}^2 \right)
\end{align}
Next, let $\gamma \coloneqq 1 - \beta \alpha( E_0 \mu_\ast^2) + c \beta \tau_1\tau_2 + c\beta \sqrt{\alpha\tau_1} L_{\ast} + c \beta^2 \alpha \tau_2 L_\ast^4$ and $\xi \coloneqq \alpha \beta  (L_{\max} + \sigma) \left(  L_{\max}\frac{\delta_{out,k}+\delta_{in}}{\sqrt{ n}} +  \left(\frac{a_t}{\sqrt{\alpha}}+\sigma\right)\delta_{in}^2 \right)$. By $\bigcup_{s=0}^t A_2(s)$, we have
\begin{align}
    \|\mathbf{I}-\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2 &\leq \gamma\|\mathbf{I}-\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2 + 10 \alpha^{2}\beta^2 L_\ast^4 \dist_t^2 + \xi \nonumber \\
    &\leq \gamma^2\|\mathbf{I}-\alpha \mathbf{B}_{t-1}^\top \mathbf{B}_{t-1}\|_2 + \gamma(10\alpha^{2}\beta^2 \dist_{t-1}^2 +\xi) +  10\alpha^{2}\beta^2 \dist_t^2+\xi \nonumber \\
    &\;\;\vdots \nonumber \\
    &\leq  \gamma^{t+1}\|\mathbf{I}-\alpha \mathbf{B}_{0}^\top \mathbf{B}_{0}\|_2 +   \sum_{s=0}^t \gamma^{t-s} (10 \alpha^{2}\beta^2 L_\ast^4\dist_s^2 +\xi) \nonumber \\
    &= \sum_{s=0}^t \gamma^{t-s} ( 10\alpha^{2}\beta^2 L_\ast^4 \dist_s^2 +\xi)
\end{align}
since $\|\mathbf{I}-\alpha \mathbf{B}_{0}^\top \mathbf{B}_{0}\|_2 = 0$ by choice of initialization.
Now, let $\rho\coloneqq 1 - \beta \alpha \mu^2$ and $\xi' \coloneqq L_{\max}(L_{\max}+\sigma) \frac{\delta_{out}}{E_0 \mu_{\ast}^2} $.


We have that $\dist_s \leq \rho^s + \xi' $ for all $s\in \{0,...,t\}$ by $\bigcup_{s=0}^t A_5(s)$. We also have $\gamma \leq \rho$ by choice of $\alpha$.
Thus, for any $s\in \{0,...,t\}$, we have
\begin{align}
    \|\mathbf{I}-\alpha \mathbf{B}_{s+1}^\top \mathbf{B}_{s+1}\|_2 &\leq  \sum_{r=0}^s \gamma^{s-r} ( 10\alpha^{2}\beta^2 L_\ast^4 \dist_r^2 +\xi) \nonumber \\
    &\leq   \sum_{r=0}^s \gamma^{s-r} ( 10\alpha^{2}\beta^2 L_\ast^4 (2\rho^{2r}+ 2 \xi') +\xi) \nonumber \\
    &\leq 20\alpha^{2}\beta^2 L_\ast^4  \sum_{r=0}^s \gamma^{s-r}\rho^{2r}+ 20\alpha^{2}\beta^2 L_\ast^4  \sum_{r=0}^s \gamma^{s-r} \xi' + \sum_{r=0}^s \gamma^{s-r} \xi \nonumber \\
    &\leq \rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1-\rho}  + (20\alpha^{2}\beta^2 L_\ast^4 \xi'+\xi) \frac{1}{1-\gamma}  \nonumber \\
    &=: \zeta_s 
\end{align}
Now, applying \eqref{forall} recursively for $s=t,t-1,\dots,0$ and plugging in the definition of $z_s$ yields
\begin{align}
    a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_t \eta_\ast + \xi'' \nonumber \\
    &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} \zeta_{t-1})(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_{t-1} \eta_\ast(1 + \tfrac{2\beta}{\alpha} \zeta_t)  + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_t L_\ast + \xi''(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \xi'' \nonumber \\
    &\;\; \vdots \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) + \xi'' \sum_{s=1}^t \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) \nonumber \\
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) + \xi'' \sum_{s=1}^t \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) \nonumber \\
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s (1+ \tfrac{1}{t-s-1}\sum_{r=s+1}^t\tfrac{2\beta}{\alpha}\zeta_r)^{t-s-1} + \xi'' \sum_{s=1}^t (1+ \tfrac{1}{t-s-1}\sum_{r=s+1}^t\tfrac{2\beta}{\alpha}\zeta_r)^{t-s-1} \nonumber \\
    &\leq  \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s (1+ \tfrac{1}{t-s-1}\frac{20\beta \rho^{s+1}L_{\ast}^4}{\alpha} + {\beta}^2 L_{\ast}^4 \xi' + \frac{1}{\alpha^2} \xi)^{t-s-1} \nonumber \\
    &\quad + \xi'' \sum_{s=1}^t (1+ \tfrac{1}{t-s-1}\frac{20\beta \rho^{s+1}L_{\ast}^4}{\alpha} + {\beta}^2 L_{\ast}^4 \xi' + \frac{1}{\alpha^2} \xi)^{t-s-1}   \nonumber \\
   &\leq  \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s  \exp\left(\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi'' \sum_{s=1}^t \exp\left(\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)  \nonumber \\ 
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s  \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi'' \sum_{s=1}^t \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)  \nonumber \\ 
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \left( \rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1-\rho}  + (20\alpha^{2}\beta^2 L_\ast^4 \xi'+\xi) \frac{1}{1-\gamma} \right) \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi''  \left(t +\frac{20 L_{\ast}^4}{\alpha^2} +t^2\beta^2 L_\ast^4 \xi' + \tfrac{t^2}{\alpha^2}\xi \right)  \nonumber %\\ 
\end{align}    
to ensure exponent is less than 1 we need:

\end{proof}











% \begin{lemma}[FO-ANIL FS representation concentration I]\label{lem:foanil_rep1}
% Consider any $t \in [T]$. With probability at least $1 - $,
% \begin{align}
%     \|\mathbf{\hat{G}}_{t,\mathbf{B}} - \mathbf{{G}}_{t,\mathbf{B}}\|_2 &\leq 
% \end{align}

% \end{lemma}
% \begin{proof}



% \end{proof}


% \begin{lemma}[FO-ANIL FS representation concentration II]\label{lem:foanil_rep2}
% Consider any $t \in [T]$. With probability at least $1 - $,
% \begin{align}
%     \|\mathbf{B}_t^\top\mathbf{\hat{G}}_{t,\mathbf{B}} - \mathbf{B}_t^\top \mathbf{{G}}_{t,\mathbf{B}}\|_2 &\leq 
% \end{align}

% \end{lemma}
% \begin{proof}


% \begin{align}
    
% \end{align}

% \end{proof}

% \begin{lemma}[FO-ANIL FS head concentration]\label{lem:foanil_rep1}
% Consider any $t \in [T]$. With probability at least $1 - $,
% \begin{align}
%     \|\mathbf{\hat{G}}_{t,\mathbf{w}} -  \mathbf{{G}}_{t,\mathbf{w}}\|_2 &\leq 
% \end{align}
% \end{lemma}
% \begin{proof}


% \begin{align}
    
% \end{align}
% \end{proof}

% \begin{lemma}[FO-ANIL FS $A_1(t+1)$] \label{lem:foanil_fs_a1}
% Suppose ... hold. Then
% \begin{align}
%     \|\mathbf{w}_{t+1}\|_2 &\leq 
% \end{align}
% \end{lemma}
% \begin{proof}


% \begin{align}
    
% \end{align}
% \end{proof}


% \begin{lemma}[FO-ANIL FS $A_2(t+1)$] \label{lem:foanil_fs_a2}
% Suppose ... hold. Then
% \begin{align}
%     \|\del_{t+1}\|_2 &\leq 
% \end{align}
% \end{lemma}
% \begin{proof}


% \begin{align}
    
% \end{align}
% \end{proof}

% \begin{lemma}[FO-ANIL FS $A_3(t+1)$] \label{lem:foanil_fs_a3}
% Suppose ... hold. Then
% \begin{align}
%     \|\del_{t+1}\|_2 &\leq ()\|\del_t\|_2 + \dist_t
% \end{align}
% \end{lemma}
% \begin{proof}


% \begin{align}
    
% \end{align}
% \end{proof}


% \begin{lemma}[FO-ANIL FS $A_4(t+1)$] \label{lem:foanil_fs_a4}
% Suppose ... hold. Then
% \begin{align}
%     \|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t+1}\|_2 &\leq (1 - \beta \alpha )\|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t}\|_2 + 
% \end{align}
% \end{lemma}
% \begin{proof}


% \begin{align}
    
% \end{align}
% \end{proof}





\begin{lemma} \label{lem:concen_exact}
For any $t\in [T]$ and $i\in[n]$, define $\mathbf{q}_{t,i} \coloneqq \mathbf{w}_{t,i} - (\mathbf{I}_k -\alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t -\alpha \mathbf{{B}}_t^\top \mathbf{{B}}_\ast \mathbf{w}_{\ast,t,i}$ for all $i \in [n]$ and $\mathbf{Q}_t \coloneqq \begin{bmatrix}\vdots \\
    \mathbf{q}_{t,i}^\top \\
    \vdots
    \end{bmatrix}$. Assume $\|\mathbf{w}_t\|_2^2 \leq \tau_1$ and $\max_{i\in[n]}\|\mathbf{w}_{\ast,t,i}\|_{2}\leq L_{\max}$ and event $A$ occurs. Assume $m_{in}\geq 2c (k + 10 \log(n))$.  Then
\begin{align}
   \frac{1}{\sqrt{n}} \| \mathbf{Q}_t \|_F \leq \sqrt{\tau_1}{\delta}_{m_{in},k} + \sqrt{\alpha} L_{\max} {\delta}_{m_{in},k}+ \sqrt{\alpha}{\sigma}{\delta}_{m_{in},k}
\end{align}
with probability at least $1 - 6 n^{-99}$.
\end{lemma}
\begin{proof}
Note that the $i$-th row of $\mathbf{Q}_t$ has norm 
\begin{align}
    \|\mathbf{q}_{t,i}\|_2
    &= \| \mathbf{w}_{t,i} - (\mathbf{I}_k -\alpha \mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t - \alpha \mathbf{\hat{B}}_{t}^\top\mathbf{{B}}_\ast{\mathbf{w}_{\ast,t,i}}\|_2 \nonumber \\
    &= \alpha\left\|  (\mathbf{{B}}_t^\top\mathbf{{B}}_t\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_t)\mathbf{{w}}_{t} - (\mathbf{B}_t ^\top \mathbf{{B}}_\ast\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_\ast ) \mathbf{{w}}_{\ast,t,i}\! +\!  \frac{1}{m_{in}} \mathbf{B}_t^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 \nonumber \\
    &\leq \alpha\left\| (\mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t )  \mathbf{{w}}_{t}\right\|_2 + \alpha \left\|(\mathbf{B}_t ^\top \mathbf{{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_\ast) \mathbf{{w}}_{\ast,t,i}\right\|_2\! \nonumber \\
    &\quad \quad +\frac{\alpha}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2 
    \label{twoterms}\\
    &\leq \alpha \sqrt{\tau_1}\left\| \mathbf{{B}}_t^\top\mathbf{{B}}_t\!-\! \mathbf{B}_t ^\top\mathbf{\Sigma}_{t,i}^{in} \mathbf{B}_t  \right\|_2 + \alpha L_{\max} \left\|\mathbf{B}_t ^\top \mathbf{{B}}_\ast\! -\! \mathbf{B}_t ^\top  \mathbf{\Sigma}_{t,i}^{in} \mathbf{{B}}_\ast\right\|_2\! \nonumber \\
    &\quad \quad +\frac{\alpha}{m_{in}}\!\left\|   \mathbf{B}_t ^\top (\mathbf{X}_{t,i}^{in})^\top \mathbf{z}_{t,i}^{in} \right\|_2  \label{cs31}
\end{align}
where \eqref{twoterms} follows from the triangle inequality, \eqref{cs31} follows from the Cauchy-Schwarz inequality and the facts that $\|{\mathbf{w}_{\ast,t,i}}\|_2 \leq L_{\max}$ and $\|{\mathbf{w}_{t}}\|_2 \leq \sqrt{\tau_1}$. 
% (assumed for simplicity, but we can likely show that we can normalize $\mathbf{w}_t$ at the end of each round WLOG). 
Next, using Lemma \ref{lem:basic_concen} along with a union bound over all $i \in [n]$, we have that for all $i \in [n]$,
\begin{align}
    \|\mathbf{q}_{t,i}\|_2 &\leq \sqrt{\tau_1}{\delta}_{m_{in},k} + \sqrt{\alpha} L_{\max} {\delta}_{m_{in},k}+ \sqrt{\alpha}{\sigma}{\delta}_{m_{in},k}
\end{align}
with probability at least $1-6n^{-99}$, which implies that
\begin{align}
    \frac{1}{\sqrt{n}}\|\mathbf{Q}_t\|_F &= \sqrt{\frac{1}{n}\sum_{i=1}^n\| \mathbf{q}_{t,i} \|_2^2} \leq \sqrt{\tau_1}{\delta}_{m_{in},k} + \sqrt{\alpha} L_{\max} {\delta}_{m_{in},k}+ \sqrt{\alpha}{\sigma}{\delta}_{m_{in},k} %=: L_\ast \epsilon
\end{align}
with probability at least $1 - 6n^{-99}$.
\end{proof}




Next, we state some concentration results used throughout the proof.
\begin{lemma}\label{lem:basic_concen}
For any $t,i$, let $\mathbf{X}_{t,i}\in \mathbb{R}^{m \times d}$ be a matrix whose rows are i.i.d. mean zero, $\mathbf{I}_d$-sub-gaussian random vectors. Let $\mathbf{\Sigma}_{t,i} \coloneqq \frac{1}{m} \mathbf{X}_{t,i}^\top \mathbf{X}_{t,i}$. Define $\delta_k\coloneqq \frac{c(\sqrt{k}+\sqrt{\log(n)})}{\sqrt{m}}$ for an absolute constant $c$ and suppose $\sqrt{m} \geq \sqrt{k}+\sqrt{\log(n)}$.
Then each of the following holds:
\begin{enumerate}
    \item $\mathbb{P}( \| \mathbf{{B}}_t^\top\mathbf{{B}}_t- \mathbf{B}_t^\top \mathbf{\Sigma}_{t,i} \mathbf{B}_t \|_2  \leq \|\mathbf{B}_t\|_2^2\delta_k ) \geq 1 - 2n^{-100}$
    % \item $\mathbb{P}( \| \mathbf{{B}}_t^\top\mathbf{{B}}_t- \mathbf{B}_t^\top \mathbf{\Sigma}_{t,i}^{out,h} \mathbf{B}_t \|_2  \leq \tfrac{1}{\alpha}\bar{\delta}_{m_{out},k} ) \geq 1 - 2n^{-100}$
    \item $\mathbb{P}( \| \mathbf{{B}}_t^\top\mathbf{{B}}_\ast- \mathbf{B}_t^\top \mathbf{\Sigma}_{t,i} \mathbf{B}_\ast \|_2  \leq \|\mathbf{B}_t\|_2\delta_k) \geq 1 - 2n^{-100}$
    \item $\mathbb{P}( \tfrac{1}{m}\| \mathbf{{B}}_t^\top  \mathbf{X}_{t,i} \mathbf{z}_{t,i} \|_2  \leq \|\mathbf{B}_t\|_2{\sigma}\delta_k ) \geq 1 - 2n^{-100}$
    % \item $\mathbb{P}( \tfrac{1}{m_{out}}\| \mathbf{{B}}_t^\top  \mathbf{X}_{t,i}^{out,g} \mathbf{z}_{t,i}^{out,g} \|_2  \leq \|\mathbf{B}_t\|_2{\sigma}\bar{\delta}_{m_{out},k} ) \geq 1 - 2n^{-100}$
\end{enumerate}
\end{lemma}

\begin{proof}

%  , e.g. for the third term, the same bound holds with $L_{\max}$ replaced by $\sigma$.
\end{proof}





{\color{red}
% ---

% SUMMARY OF PROOF, FO-ANIL FINITE SAMPLES: 

% We have seen that if the inner-loop adapted heads are diverse, then  the update of the representation subtracts energy from the previous representation and adds energy from the ground-truth representation. 
% Examining this update closer, we see that the only energy in the column space of the new representation that can be orthogonal to the ground-truth subspace is contributed by the previous representation, and the energy in the previous representation is contracting at a rate proportional to  the condition number of the matrix formed by the inner loop-adapted heads. Therefore, the proof is completed by showing two things: (1) this condition number is controlled, i.e. upper bounded by some finite quantity, and (2) the minimum singular value of the representation is staying roughly the same (otherwise, the energy orthogonal to the ground-truth subspace could be decreasing, but the representation could be becoming degenerate, which would mean the distance to the ground-truth subspace is not decreasing). 

% By definition of the inner loop update, if we assume the ground-truth heads are diverse, then the updated heads are diverse as long as $\|\mathbf{w}_t\|_2$ and $\|\del_t\|_2$ are small, where $\del_t := \mathbf{I}- \alpha \b^\top \b$. So, to show (1), we aim to prove that $\|\mathbf{w}_t\|_2$ and $\|\del_t\|_2$ remain small. Conveniently, showing that $\|\del_t\|_2$ remains small also implies (2). Showing these quantities remain small requires an interconnected inductive argument that also accounts for the distance to ground-truth subspace going to zero. In particular, we can show that if the distance is non-increasing and $\|\mathbf{w}_t\|_2$ is small, then $\|\del_{t+1}\|_2$ is the sum of a contraction of $\|\del_{t}\|_2$ plus $\dist_t$, so it is eventually going to zero. Also, $\|\mathbf{w}_{t+1}\|_2$ is the sum of $\|\del_{s}\|_2$ terms for $s=1,\dots,t$, so $\|\mathbf{w}_{t+1}\|_2$ is small because $\|\del_{s}\|_2$ is going to zero.  Lastly, if $\|\w\|_2$ and $\|\del_t\|_2$ are small, then $\dist_{t+1}$ contracts. This completes the proof.


% ---


-----------

OLD:

Now we are ready to formally discuss how we prove our results. We have seen in Section \ref{sec:intuition} suggesting that the key to ANIL and MAML's representation learning ability is the diversity of the $\mathbf{w}_{t,i}$'s. 


In all cases, we execute a multi-way induction that controls four terms:
$\|\w\|$, $\del_t\coloneqq \mathbf{I}_k - \alpha \mathbf{B}_t^\top\b$, $\|\mathbf{B}_{\ast,\perp}^\top\b\|_2$, and $\dist_t$. 

We start by considering FO-ANIL with $m_{in}\!=\!\infty$ and $m_{out}\!=\!\infty$ since this setting best  illuminates the key proof techniques. 
% We discuss how to extend the proof to the other algorithms and the finite-sample case at the end of this section. The result for FO-ANIL in the infinite-sample case is given as follows.
% \begin{thm}[ANIL Infinite Samples]\label{thm:anil_informal_pop}
% % \begin{thm}[ANIL, Infinite Samples]
% Let $m_{in}\!=\!m_{out}\!= \!\infty$. Define 
%  $E_0\!\coloneqq\! 0.9 -\! \dist_0^2$ and assume $\dist_0 \leq \sqrt{0.9}$. 
% %  Suppose Assumption \ref{assump:init} holds. 
% Let $\alpha = O(\tfrac{1}{L_{\ast}})$ and 
%  $\beta = O({\alpha}{\kappa_{\ast}^{-6}})$. Then FO-ANIL satisfies that after $T$ iterations,
% \begin{align}
%     \dist(\mathbf{{B}}_T, \mathbf{{B}}_\ast) \leq \left(1 - 0.5\beta \alpha E_0 \mu_\ast^2   \right)^{T-1}
% \end{align}
% \end{thm}
% For any $T>0$, $\alpha= O(\frac{1}{L_{\ast}})$, $\beta \leq O(\alpha\kappa_\ast^{-6})$, initial representation $\mathbf{B}_0$ satisfying $\dist(\mathbf{B}_0, \mathbf{B}_\ast)\leq c$ for some absolute constant $c$, 
% $m_{in} =\infty$,
% $m_{out} =\infty$,
% and $n \gg k + \log(T)$,
% then FO-MAML achieves the following with high probability:
% \begin{align}
%   \dist(\mathbf{{B}}_{T}, \mathbf{{B}}_\ast ) &\leq \left(1 - \Omega(\beta \alpha \mu_{\ast}^2)\! +\! O(\beta^2 \eta_\ast^2) \right)^{T-1}. 
% \end{align}
% with high probability over the random selection of tasks on each iteration.
% \begin{proof}
We have seen in equation \eqref{intuition} that 

that the outer loop updates are of the form $\b (\mathbf{I} - \beta\mathbf{W}_t^\top \mathbf{W}_t) + \beta \mathbf{B}_\ast\mathbf{W}_{\ast,t}^\top\mathbf{W}_t$, where


The first step in the proof is to notice that the  outer loop updates for the representation can be written as:
\begin{align}
    \mathbf{B}_{t+1}\! &=\! 
    % \mathbf{{B}}_t  - \frac{\beta}{n}\sum_{i=1}^n\nabla_{\mathbf{B}} \mathcal{L}_i(\mathbf{{B}}_t, \mathbf{w}_{t,i}) =  
    \underbrace{\mathbf{{B}}_{t} \Big(  \mathbf{I}_k\! - \!\tfrac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\Big)}_{\text{prior term}}\! +\!  \underbrace{\mathbf{{B}}_\ast\Big(\tfrac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top\Big)}_{\text{signal term}} 
    % - \underbrace{\frac{\beta}{n}\sum_{i=1}^n \nabla_{\mathbf{B}} \mathbf{R}(\mathbf{B}_{t,i})}_{\text{regularization}} \
    % \label{upd_rep_anil_out_pop}
\end{align}
% where $\mathbf{\Lambda}_{t}\!\coloneqq\!\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$
% From \eqref{upd_rep_anil_out_pop}, 
The above shows that if the inner loop updates $\{\mathbf{w}_{t,i}\}_{i=1}^n$ have energy in all directions of $\mathbb{R}^k$, i.e. they are  diverse, then the outer loop update of the representation subtracts energy from $\mathbf{B}_t$ (small prior term) and replaces it with energy from $\mathbf{B}_\ast$ (large signal term).
Formally, we have the following result:
\begin{lemma}
Consider $\mathbf{W}_t=\frac{1}{n}\sum_{i=1}^n(\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top)$. If for
any $t$ we have $\sigma_{\min}\left(\mathbf{W}_t\right)\geq\mu^2$ and $\sigma_{\max}\left(\mathbf{W}_t\right)\leq L^2$, then for any  $\beta \leq \nicefrac{1}{L^2}$ we have
\begin{align}
    \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 \leq (1 - \beta \mu^2)\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}\|_2.
\end{align}
\end{lemma}
The above result shows that $\mathbf{B}_{t+1}$ contains a fraction of energy in $\col(\mathbf{B}_{\ast})^\perp$ that $\mathbf{B}_t$ contains in $\col(\mathbf{B}_{\ast})^\perp$, with the fraction being at most 1 and depending on the diversity of the $\mathbf{w}_{t,i}$'s. In particular, the more diverse the $\mathbf{w}_{t,i}$'s, the less energy that $\mathbf{B}_{t+1}$ contains in $\col(\mathbf{B}_{\ast})^\perp$. If $\mathbf{B}_{t+1}$ is not losing total energy, i.e. $\sigma_{\min}(\mathbf{B}_{t+1}) \approx \sigma_{\min}(\mathbf{B}_t)$, then this implies that $\mathbf{B}_{t+1}$  devotes more of its energy towards the space perpendicular to $\col(\mathbf{B}_\ast)^\perp$. In other words,  $\col(\mathbf{B}_{t+1})$ is approaching $(\col(\mathbf{B}_\ast)^\perp)^\perp = \col(\mathbf{B}_{\ast})$, as desired. Thus, it remains to prove two properties: (I) $\sigma_{\min}(\mathbf{B}_{t+1}) \approx \sigma_{\min}(\mathbf{B}_t)$, and (II) $\{\mathbf{w}_{t,i}\}_{i=1}^n$ is diverse. 

However, proving that these properties hold with high probability is difficult
because the algorithm lacks explicit regularization or a normalization step after each round. 
Empirically, $\sigma_{\min}(\mathbf{B}_t)$ may decrease on any particular round, so it is not clear why $\sigma_{\min}(\mathbf{B}_t)$ does not go to zero.
Moreover, in theory $\mathbf{w}_t$ might blow up, in which case we would have $\mathbf{w}_{t,i}\!\approx\!\mathbf{w}_t$ for all $i\in[n]$, meaning the $\mathbf{w}_{t,i}$'s would not be diverse. To fix these problems, we could add explicit regularization to the loss functions or normalization to the algorithm, but doing so would not be consistent with the ANIL formulation or algorithm (nor with those of MAML).

Instead, it turns out that both (I) and (II) can be shown by controlling the spectral norm of $\del_t\coloneqq \mathbf{I}_k \! - \! \alpha \mathbf{B}_t^\top \mathbf{B}_t$ for all $t$. Clearly, small $\|\del_t\|_2$ and small $\|\del_{t+1}\|_2$ implies (I), but it is not as apparent that small $\|\del_s\|_2$ for all $s\leq t$ implies (II). To see that it indeed holds, first observe that $\mathbf{w}_{t,i}$ can be written as:
\begin{align}
    \mathbf{w}_{t,i}\!=%\!\mathbf{w}_{t}\!-\!\alpha \nabla_{\mathbf{w}}f_{t,i}(\mathbf{B}_{t},\mathbf{w}_{t})\!= 
    \!\underbrace{\del_t\mathbf{w}_t}_{\text{non-diverse}}\!+\alpha \underbrace{\mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}}_{\text{diverse}}, \label{updw}
\end{align}
 Note that $\del_t \mathbf{w}_t$ does not contribute to the diversity of the $\mathbf{w}_{t,i}$'s, so we refer to it as the non-diverse part of $\mathbf{w}_{t,i}$. 
Equation \eqref{updw} shows that if $\del_t \mathbf{w}_t$  is relatively small, then the diverse part of $\mathbf{w}_{t,i}$, namely $\mathbf{B}_{t}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}$, dominates. In this case, 
$\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \!\approx\!\frac{\alpha^2}{n}\sum_{i=1}^n\mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t$, so $\{\mathbf{w}_{t,i}\}_{i=1}^n$ has diversity close to that of the ground-truth heads. We formalize this observation in the following lemma. 
    \begin{lemma} \label{lem:2}
% Let %$\beta \leq 1/L_{\ast}^2$ and
% $\alpha  \leq 1/L_{\max}$.
% Define $\mu^2 \coloneqq \min_{t\in[T], i\in[n]} \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$ and $L^2 \coloneqq \max_{t\in[T], i\in[n]} \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$. 
% Under Assumption \ref{assump:data}, $\max_{i \in [n]} \|\mathbf{w}_{\ast,t,i}\|_2 \leq L_{\max}$, we have 
% The diversity of the inner loop-updated heads is given by
If $\|\mathbf{w}_t\|_2^2 \!\leq \! {\tau_1}$, $\|\del_t\|_2\!\leq\!\tau_2$ and $\dist_0^2\!\leq\!1\!-\!E_0$, then with high probability over the choice of tasks,
 \begin{align}
    \sigma_{\min}\Big(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \Big) &\geq 0.5 \alpha E_0 \mu_\ast^2  - 3 \tau_2 \sqrt{\tau_1 \alpha}L_{\ast} \nonumber  \\
    % \text{ and } 
    \sigma_{\max}\Big(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \Big) &\leq  2 (\sqrt{\alpha} L_\ast + \sqrt{\tau_1}\tau_2 )^2. \nonumber
\end{align}
%  at least $1 - 4 n^{-99} - 2 T^{-99}$ over the choice of tasks and samples per task.
\end{lemma}
In Lemma \ref{lem:2} we have assumed upper bounds on both $\|\del_t\|_2$ {\em and} $\|\mathbf{w}_t\|_2$ in order to characterize the diversity of the $\mathbf{w}_{t,i}$, yet as of now it is not clear how to control $\|\mathbf{w}_t\|_2$. By carefully examining the outer loop update for $\mathbf{w}_{t+1}$, we find that $\|\mathbf{w}_{t+t}\|_2$ is also controlled by $\|\del_t\|_2$. In particular, we have $\|\mathbf{w}_{t+1}-\mathbf{w}_t\|_2\leq O(\|\del_t\|_2)$. Thus, if we can show that $\|\del_t\|_2$ is small, then we will have a bound on $\|\mathbf{w}_t\|_2$ for all $t\leq T$, where $T$ is reasonably large. Even better, we will show that $\|\del_t\|_2$ eventually decreases fast enough such that $\{\|\del_t\|_2\}_t$ is summable, which yields a bound on $\|\mathbf{w}_t\|_2$ for all $t$.

Therefore, the final linchpin in the analysis is to control $\|\del_t\|_2$. Doing so again relies on the diversity of the ground-truth heads, but also on the contraction of $\dist_t$. Specifically, we can show that $\|\del_{t+1}\|_2\leq (1- \Omega(\beta \alpha \mu_\ast^2))\|\del_{t}\|_2+O(\beta^2\alpha^2\dist_t^2)$. This shows that $\|\del_t\|_2$ may initially increase (when $\dist_t \gg 0$), but once $\|\del_t\|_2\gtrsim \dist_t^2$,  $\|\del_t\|_2$ decreases at a linear rate as long as $\dist_t$ is also linearly decreasing. In turn, $\dist_t$ linearly decreases due to the contraction of $\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2$ and the control of $\sigma_{\min}(\mathbf{B}_{t+1})$. 
Since all of the aforementioned bounds are intertwined, we must execute a careful multi-way induction, with inductive hypotheses given as follows.

% Meanwhile, the inner loop updates for the head should satisfy that in some sense, $\mathbf{w}_{t,i}$ moves away from $\mathbf{w}_t$ and towards the ground-truth solution for the $i$-th task on round $t$, $\mathbf{w}_{\ast,t,i}$. So, if the $\mathbf{w}_{\ast,t,i}$'s are spread in all directions, then the $\mathbf{w}_{t,i}$'s should also be spread in all directions -- they should be diverse. 

% We show that this is the case after only one gradient step by writing $\mathbf{w}_{t,i}\!=\!(\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t)\mathbf{w}_t +\alpha \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$, and showing that $\mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t$ and $\mathbf{w}_t$ naturally remain close to zero, without any normalization step or regularization.

% -------


% The proofs of Theorems \ref{thm:anil_informal} and \ref{thm:maml_informal} rely fundamentally on the diversity of the ground-truth heads $\{\mathbf{w}_{\ast,t,i}\}_i$, which we show implies the diversity of the inner-loop updated heads $\{\mathbf{w}_{t,i}\}_i$. Intuitively, the diversity of the $\mathbf{w}_{t,i}$'s means that the outer loop update for $\mathbf{B}_t$ obtains a full `view' of the ground-truth representation.
% % In particular, they cause all 
% We discuss details below, starting with the ANIL population case ($m_{in}=\infty, m_{out}=\infty$). Then we discuss the population case for MAML, and finally discuss how to extend these analyses to achieve the efficient finite-sample results in Theorems \ref{thm:anil_informal} and \ref{thm:maml_informal}. 

%  In particular, the inner loop updates mean that the outer loop update is effectively a gradient descent step with respect to the matrix factorization loss $\|\mathbf{B}_t\mathbf{W}_{t+0.5}^\top - \mathbf{B}_\ast\mathbf{W}_\ast^\top\|_F^2$, where the $i$-th row of $\mathbf{W}_{t+0.5} \in \mathbb{R}^{n\times k}$ is equal to the $i$-th inner loop-updated head $\mathbf{w}_{t,i}^\top$. If $\mathbf{W}_{t+0.5}$ and $\mathbf{W}_\ast$ are rank-$k$, meaning that the inner loop-updated heads and the ground-truth heads are diverse, then $\|\mathbf{B}_t\mathbf{W}_{t+0.5}^\top - \mathbf{B}_\ast\mathbf{W}_\ast^\top\|_F^2$ is a proxy for $\|\mathbf{\hat{B}}_{\ast,\perp}^{\top}\mathbf{B}_t\|_2$. As a result, the outer loop update causes contraction of $\|\mathbf{\hat{B}}_{\ast,\perp}^{\top}\mathbf{B}_t\|_2$.
 
% %  However, this argument does not hold if either $\mathbf{W}_t$ or $\mathbf{W}_\ast$ are not diverse. 

% However, this alone is insufficient to show contraction of $\dist(\mathbf{B}_T, \mathbf{{B}}_\ast)\coloneqq\|\mathbf{\hat{B}}_{\ast,\perp}^{\top}\mathbf{\hat{B}}_T\|_2$, since contraction of $\|\mathbf{\hat{B}}_{\ast,\perp}^{\top}\mathbf{B}_t\|_2$ may be caused by $\mathbf{B}_t\rightarrow \mathbf{0}$, not by $\col({\mathbf{B}_t})\rightarrow \col({\mathbf{B}_\ast})$. To deal with this, we show that 
% % The proofs for both ANIL and MAML fundamentally leverage task diversity 
% % to show contraction of the norm $\|\mathbf{\hat{B}}_{\ast,\perp}^{\top}\mathbf{B}_t\|_2$ on subsequent iterations. 
% task diversity also ensures  that $\tfrac{1}{\sqrt{\alpha}}\mathbf{B}_t$ remains close to orthogonal for all times up to time $T$, i.e $\|\mathbf{I}_k-\alpha \mathbf{B}_t^\top \mathbf{B}_t\|_2^2$ is small for all $t\in[T]$. This ultimately gives us control on $\sigma_{\min}(\mathbf{B}_T)$ and $\sigma_{\max}(\mathbf{B}_T)$, which allows us to turn our bound on $\|\mathbf{\hat{B}}_{\ast,\perp}^{\top}\mathbf{B}_T\|_2$ into a bound on $\dist(\mathbf{B}_T, \mathbf{{B}}_\ast)$. We also need to control $\|\mathbf{w}_t\|_2$ in order to make these conclusions. 
% % These patterns hold for both finite and infinite samples per task, and for both first order and exact versions of the algorithms. 

% \textbf{Population case: ANIL.}
% We state the population case result for ANIL then give the proof sketch. 
% Please see Appendix \ref{app:anil} for the complete proof.

% 1. Ensuring that the learned representation stays well-conditioned, and the head stays close to zero. To show this, we make an inductive argument that accounts for the coupled dynamics of the representation and the head.
% 2. Extending population case to efficient finite-sample analysis.
% We start by showing in this section that the ANIL update procedure specifically harnesses task diversity to learn the ground-truth representation.
% First we need to define some constants. 
% \begin{rem}[Task Diversity] 
% We will show that task diversity enables ANIL and MAML to learn the ground-truth representation.  We measure task diversity by how evenly spread their ground-truth heads are in $\mathbb{R}^k$. In particular, we say that a set of ground-truth heads are $(\mu_\ast, L_\ast)$\textbf{-diverse} if $\mu_\ast^2 \leq \sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right)\leq\sigma_{\max}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \leq L_\ast^2$. The more diverse the tasks are, the smaller that $\nicefrac{L_\ast}{\mu_\ast}$ is. Since the ground-truth heads are i.i.d. from an isotropic sub-Gaussian distribution, standard matrix concentration results  show that there exists some constant $c>0$ such that $n > k$ heads are $\left(1\!-\! \frac{c\sqrt{k}}{\sqrt{n}}, 1\!+\! \frac{c\sqrt{k}}{\sqrt{n}}\right)$-diverse with high probability \citep{vershynin2018high}. % (see Corollary 2.3.5 and Theorem 2.7.5 in tao 2012
% {\em Thus,  the set of tasks sampled on each iteration is very diverse with high probability as long as $n \gg k$.}
% \end{rem}
% The first step is to  establish high-probability bounds on the maximum and minimum singular values of the matrix of ground-truth heads sampled on each iteration. Let
% \begin{lemma} \label{lem:cond}
% Let $\alpha=1$ and $\beta \leq 1/L_{\ast}^2$.
% Define $\mu^2  \coloneqq \min_{t\in [T]} \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$ and $L^2 \coloneqq \max_{t\in[T]}\sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$. 
% Under Assumption \ref{assump:data}, $\|\mathbf{w}_t\|_2 \leq L_{\max}$ and $\max_{i \in [n]} \|\mathbf{w}_{\ast,t,i}\|_2 \leq L_{\max}$, we have 
% \begin{align}
%     L &\leq L_\ast + (2L_{\max}+\sigma)\delta_{in}\\
%     \text{and} \quad \mu &\geq \sqrt{E_0 \mu_\ast^2 - 2 L_\ast (2 L_{\max}+ \sigma)\delta_{in}}
% %\mu_\ast^2 E_0 - 4 L_{\max}^2 (\delta_{in} + \delta_{in}^2) 
%  \end{align}
%  with probability at least $1 - 4 n^{-99} - 2T^{-99}$.
% \end{lemma}
% Next, we show that the parameters remain normalized throughout the execution of the algorithm. Define the event $ $
% \begin{align}
% \delta_{in} &\coloneqq c_{in}\frac{\sqrt{k} + \sqrt{\log(n)}}{\sqrt{m_{in}}}, \quad \delta_{out} \coloneqq c_{out}\frac{\sqrt{d}}{\sqrt{nm_{out}}}, \quad \delta_{out}' \coloneqq c_{out}'\frac{\sqrt{k}}{\sqrt{nm_{out}}}\nonumber \\
% L_\ast &\coloneqq 1 + c_1\frac{\sqrt{k}+\sqrt{\log(T)}}{\sqrt{n}}, \quad \mu_\ast \coloneqq 1 - c_2\frac{\sqrt{k}+\sqrt{\log(T)}}{\sqrt{n}}, \quad L_{\max} \coloneqq c_{\max}\sqrt{k + \sqrt{k\log(nT)}+ \log(nT)} \nonumber \\
% L &\coloneqq L_\ast + (2L_{\max}+\sigma)\delta_{in}, \quad
%  \mu \coloneqq \sqrt{E_0 \mu_\ast^2 - 2 L_\ast (2 L_{\max}+ \sigma)\delta_{in}} \nonumber \\
%     \rho &\coloneqq \beta \mu^2 - \beta L_{\max}^2 \delta_{out}, \quad \varepsilon \coloneqq  {(2 L_{\max}+\sigma)(2+L_{\max}+L_{\max}\delta_{in}+\sigma\delta_{in} )\delta_{in}\delta_{out}}+ {\sigma L_{\max}(1+2\delta_{in}) \delta_{out}} \nonumber \\
%     R &\coloneqq  1 - 2 \beta (L_{\max}+\sigma) L \delta_{in}  - 2\beta(1 - \beta \mu + \beta L_\ast^2 + \beta L_{\ast}(2 L_{\max} + \sigma)\delta_{in})\nonumber\\
%   &\quad \times \left( \left(L_{\max}^2 + (2 L_{\max}+\sigma)(2+L_{\max}+L_{\max}\delta_{in}+\sigma\delta_{in} )\delta_{in}\right) + \sigma L_{\max}  ( 1+2 \delta_{in})  \right)\delta_{out}' \nonumber
% \end{align}
% where $c_{in}, c_{out}, c'_{out}, c_1, c_2, c_{\max}$ are absolute constants.
 %We provide experimental evidence supporting this conjecture in Section \ref{sec:numerics}.
    % discuss log(T) appearance? can be removed by assuming uniform upper bound on norm of w_{\ast,t,i}
% \end{enumerate}
% The  proof of Theorem \ref{thm:anil_formal_main} is given in Appendix \ref{app:anil}. For now, we provide a brief proof sketch.

% \textbf{Proof sketch.}
% \begin{proof}
% First we show diversity of ground truth heads.
% Let $\del_t\coloneqq \mathbf{I}_k\!-\!\alpha\mathbf{B}_t^\top \mathbf{B}_t$.
% The proof makes an inductive argument using the following inductive hypotheses:
% Here we treat $L_\ast, L_{\max}, \mu_\ast$ as constants
% \tau_1 = (\beta \kappa_\ast^4 \eta_\ast/\sqrt{\alpha})^2
\begin{enumerate}
   \item $A_1(t) \coloneqq \big\{\|\del_t\|_2 \leq \big(1\!-\!\Omega(\beta\alpha \mu_{\ast}^2) +O( \beta\tau_1 \tau_2 + %\beta \sqrt{\alpha\tau_1}
 \beta \sqrt{\alpha \tau_1} \eta_\ast)\big)\|\del_{t-1}\|_2
%  \|\mathbf{I}_k-\alpha \mathbf{B}_{t-1}^\top \mathbf{B}_{t-1}\|_2 
 + O(\beta^2\alpha^2\dist^2_{t}L_{\ast}^4)\big\}$, %redefine like A5
       \item $A_2(t) \coloneqq \big\{\|\del_t  \|_2 \leq \tau_2\big\}$, 
       \item $A_3(t) \coloneqq \{\|\mathbf{w}_t\|_2^2 \leq \tau_1\}$,
        \item $A_4(t) \coloneqq \big\{\|\mathbf{{B}}_{\ast,\perp}^\top \mathbf{{B}}_{t} \|_2  \leq (1 - \Omega(\beta \alpha \mu_\ast^2) + O(\beta \sqrt{\alpha\tau_1}\tau_2 \eta_\ast) )) \|\mathbf{{B}}_{\ast,\perp}^\top \mathbf{{B}}_0 \|_2  \big\}$, and 
     \item  $A_5(t)\! \coloneqq\! \{\dist_{t}\! \leq\! (1\! -\! \Omega(\beta \alpha \mu_\ast^2)\! +\! O(\beta \sqrt{\alpha\tau_1}\tau_2 \eta_\ast ))^{t-1} \!\}$,  %$A_3(t) \coloneqq \{\dist(\mathbf{{B}}_t, \mathbf{{B}}_\ast) \leq (1 - \beta E_0 \mu_\ast^2)^{t-1} \dist(\mathbf{{B}}_0, \mathbf{{B}}_\ast)\}$.
\end{enumerate}
where $\tau_1 = O(\frac{\beta^2 \kappa_{\ast}^8 \eta_\ast^2}{\alpha})$ and $\tau_2 = O(\frac{1}{\kappa_\ast^4})$ are parameters used in the analysis only.

% \textbf{Intuition.} As we have seen in \eqref{upd_rep_anil_out_pop}, contraction of $\dist_{t+1}$ relies on the diversity of the inner loop-updated heads. Since $\mathbf{w}_{t,i}\!=\!\del_t\mathbf{w}_t\!+\!\alpha\mathbf{B}_t^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}$, the $\mathbf{w}_{t,i}$'s are diverse only if $\del_t$ and $\mathbf{w}_t$ are small. Inductive hypotheses $A_1(\cdot),A_2(\cdot)$ and $A_3(\cdot)$ show this is indeed the case. 

% In particular, $A_1(\cdot)$ entails that the learned representation remains well-conditioned throughout the execution of the algorithm, i.e. it contains equal energy in all directions of $\col(\mathbf{B}_\ast)$.
% More specifically, $A_1(\cdot)$ and $A_2(\cdot)$ entail that $\tfrac{1}{\sqrt{\alpha}}\mathbf{B}_t$ remains close to an orthonormal matrix for all times $t$. Noting that $\tfrac{1}{\sqrt{\alpha}}\mathbf{B}_0$ is exactly orthonormal, $A_1(\cdot)$ combined with $A_5(\cdot)$ shows that $\|\del_t\|_2$ may initially increase (when $\dist_t \gg 0$), but once $\|\del_t\|_2\gtrsim \dist_t^2$,  $\|\del_t\|_2$ decreases at a linear rate. $A_2(\cdot)$ formalizes that $\|\del_t\|_2$ is always upper bounded and $A_3(\cdot)$ does the same for $\|\mathbf{w}_t\|_2$, while  $A_4(\cdot)$ leverages these bounds to show $\|\mathbf{{B}}_{\ast,\perp}^\top \mathbf{{B}}_{t} \|_2$ is linearly decreasing. Finally, $A_5(t)$ shows this implies that $\dist_t$ linearly converges to zero.
% % by utilizing the near-orthogonality of $\frac{1}{\sqrt{\alpha}}\mathbf{B}_t$.
% Note that $A_4(t)$ alone is insufficient to show this because $\mathbf{B}_t$ is not normalized.

% The arguments to complete each of these inductive hypotheses are given below.

% is a simple consequence of these dynamics, and $A_3(t)$ follows from the fact that $\|\mathbf{I}-\alpha\mathbf{B}_t^\top\mathbf{B}_t\|_2$ eventually decreases linearly. Finally, 



% the representation is well-conditioned throughout the execution of the algorithm. which can be shown with high probability for
% .


% $\tau_2$ can be anything... to get scaling to work, and balance terms, i think we need $\alpha=1/L_\ast^2$ and $\tau_2 = \alpha^2/L_{\ast}^2$ then $\beta$ is $1/(\kappa^6 L_\ast^2)$


% It is easy to see that proving the induction completes the proof due to inductive hypothesis $A_5(t)$. Furthermore,
Clearly each inductive hypothesis holds at time $t\!=\!1$ due to the  initialization.
It remains to show that the inductive hypotheses hold at time $t+1$ if they hold up to time $t$. Note that showing $A_5(t)$ holds for all $t$ implies that $\dist_t$ is linearly converging to zero.

We first give closed-form expressions for the inner and outer loop updates at time $t$:
\begin{align}
\mathbf{w}_{t,i}\!&=\! \mathbf{w}_t - \alpha \mathbf{B}_t^\top(\mathbf{B}_t \mathbf{w}_t\! -\! \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}) \quad \quad \; \text{(Inner head $i$)} \nonumber \\
\mathbf{w}_{t+1}\!&=\! \mathbf{w}_t\! -\! \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_t^\top(\mathbf{B}_t \mathbf{w}_{t,i}\! -\! \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}) \; \; \text{(Outer head)} \nonumber \\
    \mathbf{B}_{t+1}&= \mathbf{B}_t - \beta \mathbf{G}_t \quad \quad \quad \quad \quad \quad \; \; \text{(Outer representation)}\nonumber
\end{align}
where $\mathbf{G}_t = \frac{1}{n}\sum_{i=1}^n( \mathbf{B}_t\mathbf{w}_{t,i} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top.$ 
We also define the following terms for ease of notation:
\begin{align}
    \mathbf{u}_t \coloneqq \mathbf{B}_t^\top \mathbf{B}_t \mathbf{w}_t,\;\; \mathbf{v}_{t,i}\coloneqq \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \; \forall i\in [n]\nonumber
\end{align}
% The inductive hypothesis are
% Note that since $\sigma_{\min}(\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top)\geq \mu_\ast^2$,
% \begin{align}
%     \sigma_{\min}\left( \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \right)&\geq \sigma_{\min}^
% \end{align}
Now we are ready to show the inductive hypotheses. We start by showing contraction of $\dist_{t+1}$ (i.e. $A_4(t+1), A_5(t+1)$) given upper bounds on $\|\del_t\|_2$ and $\|\mathbf{w}_t\|_2$ ($A_2(t),A_3(t)$). Then we show how to control $\|\del_{t+1}\|_2$ and $\|\mathbf{w}_{t+1}\|_2$ ($A_{1}(t+1),A_2(t+1),A_3(t+1)$).
% We do this as follows, using the shorthand $\dist_t\coloneqq \dist(\mathbf{B}_t, \mathbf{B}_\ast)$:
\begin{itemize}[leftmargin=10pt]
    \item $A_1(t), A_3(t) \implies A_4(t+1)$: Before showing contraction of $\dist_{t+1}\coloneqq \|\mathbf{B}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t+1}\|_2$ (where $\mathbf{\hat{B}}_t$ is orthogonalized), it is helpful to show contraction of $\|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t+1}\|_2$, which means that $\mathbf{B_{t+1}}$ contains less energy in $\col(\mathbf{B}_\ast)^{\perp}$ than does $\mathbf{B_{t}}$. The key to this is the diversity of the inner-loop updated heads $\{\mathbf{w}_{t,i}\}_i$. Note
    \begin{align}
        \|\mathbf{B}_{\ast,\perp}^\top\!\mathbf{B}_{t+1}\|_2\! &=\! \Big\|\mathbf{B}_{\ast,\perp}^\top\!\mathbf{B}_{t}\Big(\mathbf{I}_k \!- \!\frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\Big) \Big\|_2 \nonumber \\
        &\leq \|\mathbf{B}_{\ast,\perp}^\top\!\mathbf{B}_{t}\|_2(1\!-\!\sigma_{\min}(\tfrac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top))\nonumber
    \end{align}
    So, a lower bound on $\sigma_{\min}(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top)$ implies contraction of $\|\mathbf{B}_{\ast,\perp}^\top\!\mathbf{B}_{t+1}\|_2$ as long as $\beta \leq \sigma_{\max}(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top)$. Intuitively, if the inner loop-updated heads are diverse, then they reduce the energy in all $k$ directions of $\col(\mathbf{B}_t)$, which are the only directions in $\col(\mathbf{B}_{t+1})$ that may be orthogonal to $\col(\mathbf{B}_\ast)$.
    % other words, control of the diversity of the inner-loop updated heads is sufficient to complete the proof. 
    The following lemma completes the proof by characterizing the diversity of the inner loop-updated heads. 
    \begin{lemma} \label{lem:cond}
% Let %$\beta \leq 1/L_{\ast}^2$ and
% $\alpha  \leq 1/L_{\max}$.
% Define $\mu^2 \coloneqq \min_{t\in[T], i\in[n]} \sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$ and $L^2 \coloneqq \max_{t\in[T], i\in[n]} \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)$. 
% Under Assumption \ref{assump:data}, $\max_{i \in [n]} \|\mathbf{w}_{\ast,t,i}\|_2 \leq L_{\max}$, we have 
% The diversity of the inner loop-updated heads is given by
If $A_2(t),A_3(t),$ and $A_5(t)$ hold and $\dist_0^2\!\leq\!1\!-\!E_0$, then with high probability over the choice of tasks,
 \begin{align}
    \sigma_{\min}\Big(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \Big) &\geq 0.5 \alpha E_0 \mu_\ast^2  - 3 \tau_2 \sqrt{\tau_1 \alpha}L_{\ast} \nonumber  \\
    % \text{ and } 
    \sigma_{\max}\Big(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \Big) &\leq  2 (\sqrt{\alpha} L_\ast + \sqrt{\tau_1}\tau_2 )^2. \nonumber
\end{align}
%  at least $1 - 4 n^{-99} - 2 T^{-99}$ over the choice of tasks and samples per task.
\end{lemma}
    The proof of Lemma \ref{lem:cond} follows by noticing $\mathbf{w}_{t,i}\!=\!\del_t \mathbf{w}_t\!+\!\alpha\mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}$. The second term gives diversity, while the first term is small due to $A_2(t)$ and $A_3(t)$.
    \item $\{\cup_{s=1}^t A_4(s)\}\cup A_2(t+1) \implies A_5(t+1)$: Reducing the energy in $\col(\mathbf{B}_\ast)^{\perp}$ alone is not sufficient for contraction of $\dist_{t+1}$. We must also show that $\mathbf{B}_{t+1}$ gains energy in $\col(\mathbf{B}_\ast)$. Intuitively, this occurs due to the signal term in \eqref{upd_rep_anil_out_pop}. Analytically, we show this by controlling the spectrum of $\mathbf{B}_{t+1}$ via the fact  that $\del_{t+1}$ is small ($A_2(t+1)$). By recursively applying $A_4(\cdot)$, we obtain
    \begin{align}
          \|\mathbf{B}_{\ast,\perp}^\top\!\mathbf{B}_{t+1}\|_2\! &\leq\! \rho^{t}\|\mathbf{B}_{\ast,\perp}^\top\!\mathbf{B}_{0}\|_2 \nonumber \\
          \implies \dist_{t+1}\! &\leq\! \rho^t \dist_0 \frac{\|\mathbf{B}_{0}\|_2}{\sigma_{\min}(\mathbf{B}_{t+1})}\!\stackrel{(a)}{\leq}\!\rho^t \frac{ \dist_0}{1\!-\!\tau_2}\!\stackrel{(b)}{\leq}\!\rho^t \nonumber
    \end{align}
    where $(a)$ follows by $A_2(t\!+\!1)$ and $(b)$ follows for $\dist_0$ smaller than some absolute constant.
    \item $A_1(t), A_3(t), A_5(t) \implies A_1(t+1)$: 
    % First, we write the outer loop update for the representation as $\mathbf{B}_{t+1} = \mathbf{B}_t - \beta \mathbf{G}_t$, where 
    Observe that $\del_{t+1}= \del_{t} + \alpha\beta  (\mathbf{B}_t^\top \mathbf{G}_t + \mathbf{G}_t^\top \mathbf{B}_t) - \alpha\beta^2 \mathbf{G}_t^\top \mathbf{G}_t$. By expanding the  $\mathbf{w}_{t,i}$'s in $\mathbf{G}_t$, we can write $\mathbf{B}_t^\top \mathbf{G}_t$ as:
    \begin{align}
        \mathbf{B}_t^\top \mathbf{G}_t \!= \! \del_t\bigg( \mathbf{A}_t - \frac{\alpha}{n}\sum_{i=1}^n \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \bigg) \label{help1}
    \end{align}
    % where $\mathbf{A}_t = \frac{1}{n}\sum_{i=1}^n \mathbf{B}_t^\top(\mathbf{B}_t \mathbf{w}_t\!-\! \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i}^\top$. Next, by expanding the $\mathbf{w}_{t,i}$ in $\mathbf{A}_t$, we obtain 
    % \begin{align}
    %     \mathbf{A}_t\!=\! \frac{1}{n}\sum_{i=1}^n \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top +\mathbf{A}_t'
    % \end{align}
    where $\mathbf{A}_t\!\coloneqq \!\left(\mathbf{u}_t\! -\! \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{w}_t^\top \del_t %(1-\alpha) \left(\mathbf{u} - \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\right)\mathbf{u}^\top 
    \!+\! \frac{\alpha}{n}\sum_{i=1}^n\mathbf{u}_t\mathbf{v}_{t,i}^\top$. Equation \eqref{help1} shows that $i)$ $\mathbf{B}_t^\top \mathbf{G}_t$ is the product of $\del_t$ and another matrix, and $ii)$ this other matrix is the sum of a term that promotes the contraction of $\|\del_t\|_2$ via task diversity ($-\frac{\alpha}{n}\sum_{i=1}^n \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top$) and a term that inhibits it ($\mathbf{A}_t$). After substituting \eqref{help1} in the definition of $\del_{t+1}$ and using some algebra, we obtain
    \begin{align}
        \|\del_{t+1}\|_2 
        &\leq \bigg\|\mathbf{I}_k - \beta \alpha^2 \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top + \beta \alpha\mathbf{A}_t\bigg\|_2 \|\del_{t}\|_2\nonumber \\
        &\quad +\beta^2 \alpha \|\mathbf{G}_t\|_2^2
    \end{align}
    We now see that $-\beta\alpha^2\frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top$ gives contraction of $\del_t$ since $\|\mathbf{I}_k - \beta \alpha^2 \frac{1}{n}\sum_{i=1}^n\mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top + \beta \alpha\mathbf{A}_t\|_2\leq 1 - \beta \alpha \sigma_{\min}\left( \frac{\alpha}{n}\sum_{i=1}^n \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \right) + \beta \alpha\|\mathbf{A}_t\|_2$ and $\sigma_{\min}\left( \frac{\alpha}{n}\sum_{i=1}^n \mathbf{v}_{t,i}\mathbf{v}_{t,i}^\top \right)&=\Omega(\mu_\ast^2)$ by the diversity of the ground-truth heads. 
    
    

    We upper bound $\|\mathbf{A}_t\|_2$ via straightforward applications of $A_2(t)$, $A_3(t)$ and Assumption \ref{assump:tasks}. To upper bound $\|\mathbf{G}_t\|_2^2$, we write $\mathbf{G}_t = \mathbf{B}_t\del_t \mathbf{w}_t\frac{1}{n}\sum_{i=1}^n\mathbf{w}_{t,i} - (\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top) \mathbf{B}_\ast \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top$.  The first term is easy to deal with because it is a product of $\del_t$, but this is not true for the second term. However, we can use the triangle inequality to write 
    \begin{align}
        \|(\mathbf{I}_d - \alpha\mathbf{B}_t\mathbf{B}_t^\top)\mathbf{B}_\ast\|_2 &\leq \|(\mathbf{I}_d - \mathbf{\hat{B}}_t\mathbf{\hat{B}}_t^\top)\mathbf{B}_\ast\|_2 \nonumber \\
        &\quad +\|(\mathbf{\hat{B}}_t\mathbf{\hat{B}}_t^\top\! -\! \alpha\mathbf{B}_t\mathbf{B}_t^\top)\mathbf{B}_\ast\|_2  \nonumber
    \end{align}
    where $\mathbf{\hat{B}}_t$ is an orthonormalized version of $\mathbf{B}_t$. The norm in the first line (RHS) is exactly $\|\mathbf{\hat{B}}_{t,\perp}^\top \mathbf{B}_\ast\|_2 = \dist_t$, and the norm in the second line is upper bounded by $\|\del_t\|_2$. This confirms that $\|\del_{t+1}\|_2$ is upper bounded by the sum of $\|\del_t\|_2$ terms and a $\dist_t$ term.
    % Please see Lemma \ref{lem:} for the complete proof.
    \item $A_1(t+1) \implies A_2(t+1)$: This implication follows straightforwardly due to our choice of $\beta$.%, please see Lemma \ref{lem:}. 
    \item $A_1(t), A_3(t), A_5(t) \implies A_3(t+1)$: The FO-ANIL dynamics are such that $\|\mathbf{w}_t\|_2$ may increase on every iteration throughout the entire execution of the algorithm. However, we can exploit the fact that the amount that it increases is summable as $t\rightarrow \infty$ due to the linear convergence of $\dist_t$. First, for any $s\in \{0,t\}$, we can recursively apply $A_1(s)$, $A_1(s\!-\!1), ...$ to obtain, 
    \begin{align}
        \|\del_{s}\|_2 &\leq \gamma \|\del_{s-1}\|_2 + c\beta^2 \alpha^2 L_\ast^4 \dist_{s-1}^2 \nonumber \\
        &\leq c\sum_{r=0}^{s-1} \gamma^{s-r}\beta^2 \alpha^2 L_\ast^4 \dist_{r}^2\label{eqn_trot}
    \end{align}
    where we have also used the fact that $\|\del_0\|_2=0$, and $\gamma$ is the contractive factor in $A_1(\cdot)$. Note that we can write $ \gamma\!=\!1\!-\! c_\gamma \beta \alpha\mu_{\ast}^2 $ for some constant $c_\gamma$ and sufficiently small $\beta, \alpha$. From $A_5(r)$, we have $\dist_r \leq \rho^{r-1}$ for $\rho \!=\! 1\!-\!c_\rho \beta\alpha\mu_{\ast}^2$. Let $q\coloneqq \max(\gamma,\rho) $. Equation \eqref{eqn_trot} implies 
    \begin{align}\|\del_{s}\|_2 &\leq c q^{s-1}\sum_{r=0}^{s-1} \beta^2 \alpha^2 L_\ast^4 \min(q^{r-1},1)\nonumber\\
    &\leq c q^{s-1}\frac{\beta^2 \alpha^2 L_\ast^4}{1-q} \leq c' q^{s-1} \beta \alpha \kappa_{\ast}^4 \label{eqneqn}
    \end{align}
    Now we use the equation $\mathbf{w}_{t+1}\! =\! (\mathbf{I}_k\! - \!\beta \mathbf{B}_t^\top \mathbf{B}_t\del_t)\mathbf{w}_t +\frac{\beta}{n}\sum_{i=1}^n \del_t \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$, which implies $\|\mathbf{w}_t\|_2$ increases on each iteration by $O(\frac{\beta}{\sqrt{\alpha}}\|\del_{t}\|_2(\eta_\ast\!+\!\frac{\|\mathbf{w}_t\|_2}{\sqrt{\alpha}}))$, that is:
    \begin{align}
        \|\mathbf{w}_{t+1}\|_2 &\stackrel{(a)}{\leq} (1 +\tfrac{2\beta}{\alpha}\|\del_t\|_2)\|\mathbf{w}_{t}\|_2 + \tfrac{2\beta\eta_\ast}{\sqrt{\alpha}}\|\del_t\|_2 \nonumber \\
        &\stackrel{(b)}{\leq} \sum_{s=0}^{t-1}\tfrac{2\beta\eta_\ast}{\sqrt{\alpha}}\|\del_s\|_2 \prod_{r=s}^{t-1}(1 +\tfrac{2\beta}{\alpha}\|\del_r\|_2)  \nonumber \\
        &\stackrel{(c)}{\leq} \sum_{s=0}^{t-1}\tfrac{2\beta\eta_\ast}{\sqrt{\alpha}}\|\del_s\|_2 \Big(1 +\tfrac{1}{t-s}\sum_{r=s}^{t-1}\tfrac{2\beta}{\alpha}\|\del_r\|_2\Big)^{t-s}  %\label{eqn1} %
        % &\leq  \sum_{s=0}^{t-1}\frac{2\beta\eta_\ast}{\sqrt{\alpha}} z_s \prod_{r=s}^{t-1}(1 +\frac{2\beta}{\alpha}z_r) \nonumber
    \end{align}
    where $(b)$ follows by recursively applying $(a)$ for $t,t\!-\!1,$ etc. and $(c)$ follows by the AM-GM inequality. Plugging \eqref{eqneqn} into $(c)$ shows that \begin{align}
        \|\mathbf{w}_{t+1}\|_2 \leq c\tfrac{\beta}{\sqrt{\alpha}}\kappa_\ast^4\eta_\ast =:\sqrt{\tau_1}
    \end{align}
    % as desired.
\end{itemize}
% The third inductive hypothesis ensures 
% that the term $\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_t\|_2$. 
% The crux of the proof is in leveraging the diversity of the inner-loop updated heads to show that they replace energy from $\mathbf{B}_t$ with energy from $\mathbf{B}_\ast$, as discussed in Section \ref{sec:sot}, so that $\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_t\|_2$ contracts. We formalize this argument below:
% \begin{lemma}[Outer contraction given diverse inner heads] \label{lem:contract}
% Suppose that the inner-loop updated heads are $(\mu,L)$-diverse on round $t$. Then we have 
% \end{lemma}
% \begin{lemma}[Inner task heads are diverse]
% \end{lemma}
% Combining Lemma \ref{lem:contract} with Lemma \ref{lem:cond} completes the proof of inductive hypothesis 2 holding at time $t+1$. This inductive hypothesis can be combined with inductive hypothesis $A_2(t)$ to show linear convergence of the principal angle distance. 
% For now, we provide a  proof outline in the simplified setting in which $m_{in}\!=\!m_{out}\!=\!\infty$.
% Assuming the denominator is $\Omega(1)$ (which it is for $m_{in} \gg k + \log(n)$ and $m_{out} \gg d/n$), the representation converges to a neighborhood of size  $O(\delta_{out}\delta) \equiv O\left(\frac{\sqrt{dk}+\sqrt{d\log(n)}}{\sqrt{nm_{in}m_{out}}}\right)$.
% Again we require $\delta_{in} = \Omega\left(\frac{L_{\max}^4(k + \log(n))}{\mu_\ast^4 E_0^2 }\right) \approx \Omega\left(\frac{k^2(k + \log(n))}{E_0^2}\right)$ and likewise $\delta_{out} = \Omega\left(\frac{L_{\max}^4d}{\mu_\ast^4 E_0^2 }\right) \approx \Omega\left(\frac{k^2 d}{E_0^2}\right)$ for linear convergence to the neighborhood. 
% \begin{rem}[Choice of $\alpha\!=\!1$] With $\alpha \!=\!1$ in the infinite sample case, we solve for the optimal head corresponding to the current representation with only one local update.  However, the above result can be generalized to the case in which $\alpha\!\approx\! 1$ with a smaller contraction factor. The key, at a high level, is that $\alpha$ must be large enough such that the inner-loop heads become sufficiently diverse after only one gradient step.
% \end{rem}
% \subsection{Finite-Sample Case}
% The proof of Theorem \ref{thm:anil_formal_main} follows the same structure as in the infinite sample case with the only difference being that now we have additional finite-sample error terms that we must show converge to zero with a reasonable number of samples. The key is that since the inner loop only requires concentration of a $k\!\times\!k$-dimensional matrix, $m_{in}\!=\!O(k)$ samples are sufficient to learn the representation. This observation helps to explain why ANIL can perform so well in few-shot learning settings in which only a small number of samples are available for the inner loop updates.

%      Please see Appendix \ref{app:anil} for the complete proof.
% \end{proof}
% \end{proof}


The proof for Exact ANIL is identical except that $\mathbf{G}_t$ has an extra $\del_t$ factor, which allows us to show a faster convergence rate. The result and proof for the Exact ANIL population case is in Appendix \ref{app:anil}.


% Note that if we have no inner loop update for the head, i.e. $\mathbf{w}_{t,i} = \mathbf{w}_t$ for all $i,t$, then we do not utilize task diversity in the update of $\mathbf{B}_{t+1}$, and our previous argument implies that we cannot learn $\text{col}(\mathbf{B}_\ast)$ in this case.

\textbf{Population case: MAML.}
% Now we ask whether we can show a similar representation learning result for MAML.
% Again we only consider first-order updates.
% $= (\mathbf{I}_d - \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t)\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast\mathbf{w}_{\ast,i}= (1 - \alpha )\mathbf{w}_t + \alpha \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}$.
% In this case, the outer loop update for the representation can be written as:
% \begin{align}
%     \mathbf{B}_{t+1} &= \mathbf{{B}}_{t} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{B}_{t,i} \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top +   \frac{\beta}{n}\sum_{i=1}^n \mathbf{{B}}_{\ast} \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top - \frac{\beta \lambda}{n}\sum_{i=1}^n \alpha\mathbf{B}_{t,i}(\alpha \mathbf{B}_{t,i}^\top \mathbf{B}_{t,i} - \mathbf{I}_k) \label{upd_rep_MAML}
% \end{align}
% where $\mathbf{B}_{t,i} = \mathbf{B}_t(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top) + \alpha \mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top -\alpha^2\lambda \mathbf{B}_t (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)$ 
% and $\mathbf{w}_{t,i}$ is the same as for ANIL.
The difference between MAML and ANIL is that MAML makes inner loop updates for the representation, while ANIL does not. However, these the inner loop updates for the representation may inhibit representation learning. Observe that the FO-MAML outer loop update for $\mathbf{B}_{t+1}$ is:
\begin{align}
    \mathbf{B}_{t+1} 
   \! &=\! \mathbf{{B}}_{t} \bigg(\mathbf{I}_k- (\mathbf{I}_k\! -\! \alpha \mathbf{w}_t\mathbf{w}_t^\top)  \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top  
    % + \frac{\alpha \beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{t} \mathbf{w}_{t,i}^\top 
    \bigg) \nonumber \\
    &\quad +   \mathbf{{B}}_{\ast}\bigg(\frac{\beta}{n}\sum_{i=1}^n ( 1\!- \!\alpha \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle)  \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top\bigg)  \label{upd_rep_MAML_detailed} 
\end{align}
% where
% $\mathbf{B}_{t,i} = \mathbf{B}_t(\mathbf{I}_k - \alpha \mathbf{w}_t \mathbf{w}_t^\top) + \alpha \mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t}^\top %-\alpha^2\lambda \mathbf{B}_t (\mathbf{B}_t^\top \mathbf{B}_t - \mathbf{I}_k)
% $\mathbf{w}_{t,i}$ is the same as for ANIL.
This is equivalent to the update for ANIL plus two perturbation terms. The first perturbation term, $\alpha \mathbf{w}_{t}\mathbf{w}_{t}^\top\frac{\beta}{n}\sum_{i=1}^n  \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top$ in the coefficient of $\mathbf{{B}}_t$, may increase the energy from $\mathbf{{B}}_t$ in the update. Meanwhile, the second perturbation term, $-\frac{\alpha\beta}{n}\sum_{i=1}^n \langle \mathbf{w}_{t}, \mathbf{w}_{t,i} \rangle \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i}^\top$ in the coefficient of $\mathbf{{B}}_\ast$, may decrease the energy contributed by $\mathbf{B}_\ast$. Thus, to show that MAML learns $\col(\mathbf{B}_\ast)$, we must show that the impact of these perturbation terms is small.
% This suggests that MAML learns the representation slower than ANIL, if it learns it all.

To do this, we notice that the perturbation terms are small when $\|\mathbf{w}_t\|_2$ is small. Thus, small $\|\mathbf{w}_t\|_2$ helps MAML to not only to make the inner-loop updated heads more diverse (as it does for ANIL), but also to limit the effect of the perturbations in the update for $\mathbf{B}_{t+1}$.
% Empirically, we observe that $\|\mathbf{w}_t\|_2$ remains small throughout algorithm execution when MAML learns the representation. If we can show that  $\|\mathbf{w}_t\|_2$ remains small throughout algorithm execution, then  the perturbation terms are dominated and the inner loop-updated heads are diverse, so we can show that MAML indeed learns the representation at a linear rate. 
However, controlling $\|\mathbf{w}_t\|_2$ is not as easy as it is for ANIL, due to perturbations in  $\mathbf{w}_{t+1}$. First, the dynamics of $\mathbf{w}_t$ are fundamentally different for FO-MAML and for Exact MAML. For FO-MAML, the update $\mathbf{w}_{t+1}$ is a contraction of $\mathbf{w}_t$ plus a perturbation term. So, when the contraction is dominant, $\|\mathbf{w}_t\|_2$ is decreasing. Unfortunately, the contraction is dominant only if $\eta_\ast$ is very small, i.e. the empirical mean of the ground-truth heads is very close to zero on every iteration. Otherwise, $\|\mathbf{w}_t\|_2$ may diverge and FO-MAML does not learn the representation.

For Exact MAML, there is no contraction term in $\mathbf{w}_{t+1}$, so we cannot show that $\|\mathbf{w}_t\|_2$ ever decreases. Moreover, the amount that $\|\mathbf{w}_t\|_2$ may increase on each round is not summable like it is for ANIL. Thus, we can only show that  $\|\mathbf{w}_{t}\|_2$ is small for a finite number of rounds. The upshot is that  $\|\mathbf{w}_{t}\|_2$ can increase only by a very small amount on each iteration, so $\|\mathbf{w}_{t}\|_2$ remains small for may rounds.
These observations are formalized below.
% We use this observation to show that MAML indeed learns the representation at a linear rate as long as $\|\mathbf{w}_t\|_2$ is small throughout the entire process. This can be ensured by setting $\mathbf{w}_t = \mathbf{0}_k$ at the start of each iteration. 
% Recent work has shown  that this ``zeroing trick'' indeed empirically improves the performance of MAML \citep{kao2021maml}. The following theorem formalizes this observation. 
% \begin{thm}[MAML Population Case]\label{thm:maml_informal_pop}
% For
% $\dist(\mathbf{B}_0, \mathbf{B}_\ast)\leq c$ for some absolute constant $c$, 
% $m_{in} =\infty$,
% $m_{out} =\infty$, $n \gg k + \log(T)$, $\alpha\leq \frac{1}{L_{\max}}$
% both FO-MAML and Exact MAML achieve linear convergence of the representation at a rate of
% \begin{align}
%   \dist(\mathbf{{B}}_{T}, \mathbf{{B}}_\ast ) &\leq \left(1 - \Omega(\beta \alpha \mu_{\ast}^2)\right)^{T-1} 
% \end{align}
% with high probability over the random selection of tasks on each iteration, under the following additional conditions:
% \begin{itemize}
%     \item FO-MAML: 
%     % \begin{itemize}
%     %     \item 
%         $\eta_\ast \leq c E_0 \frac{\mu_\ast^4}{L_{\max}^3}$, 
%         $\dist_0 \leq c \kappa^{-2}_\ast$ and $\beta \leq \frac{E_0^2  L_{\max}}{\kappa_{\ast}^4}\alpha^2$.
%     % \end{itemize}
%     \item Exact MAML: $\beta \leq \frac{E_0}{\kappa_{\ast,\max}^2}\alpha$, $\dist_0 \leq c \kappa^{-2}_\ast$ and $T\leq \frac{c}{\alpha^{4}( \eta_\ast L_{\max}  + \mu_{\ast}^2 )L_{\max}^2 } $.
% \end{itemize}
% \end{thm}
% \begin{proof}
% \end{proof}
\textit{Proof overview.} The proof follows the same multi-way inductive structure as the proof for ANIL, although it is more challenging because  we must control additional perturbation terms to bound $\|\mathbf{w}_{t+1}\|_2$, $\|\del_{t+1}\|_2$ and $\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|$ due to the inner loop updates of the representation. Importantly, these perturbation terms cause $\mathbf{w}_t$ to behave fundamentally differently for FO-MAML and Exact MAML. For FO-MAML, we show that $\|\mathbf{w}_t\|_2$ contracts under the conditions of $\eta_\ast$ and $\dist_0$, otherwise it may diverge (Fig. \ref{fig:diverge_maml_fo}). 

For Exact MAML, $\|\mathbf{w}_t\|_2$ does not contract. To make matters worse, 
 $\|\del_{t+1}\|_2 = \Theta(\|\del_{t}\|_2 +  \dist_t^2 + \|\mathbf{w}_t\|_2 )$, which compared to ANIL contains an additional $\Theta(\|\mathbf{w}_t\|_2 )$ term that causes $\|\del_{t+1}\|_2$ to not approach zero. As a result, the differences $\{\|\mathbf{w}_{t+1}-\mathbf{w}_t\|_2\}_t$  are not summable, so we can only control $\|\mathbf{w}_t\|_2$ for a finite number of rounds. However, Theorem \ref{thm:maml_informal_pop} shows that this number is quite large, and sufficient to reach advanced numerical precision for reasonable choice of step sizes. Please see Appendix \ref{app:maml} for further discussion.
}





\begin{align}
     \mathbb{P}\left(\|\mathbf{E}_1\|_2\geq  c''(\gamma+ \sqrt{d_1})(\gamma + \sqrt{d_2})c_2 c_3 c_4 \max\left(\tfrac{\sqrt{d+d_2} + \lambda}{\sqrt{n(m-1)}}, \tfrac{d+d_2 + \lambda^2}{n (m-1)}  \right) \right) 
     &\leq 2 e^{-\lambda^2} + 2n e^{-c \gamma^2  }.
\end{align}
Repeating the same argument for all $j\in [m]$ and applying a union bound gives
\begin{align}
    \mathbb{P}&\left(\frac{1}{m}\sum_{j=1}^m\|\mathbf{E}_j\|_2\geq c'' (\gamma+ \sqrt{d_1})(\gamma + \sqrt{d_2}) c_2 c_3 c_4\max\left(\tfrac{\sqrt{d+d_2} + \lambda}{\sqrt{n(m-1)}}, \tfrac{d+d_2 + \lambda^2}{n (m-1)}  \right) \right) \nonumber \\
    &\quad \quad \leq  2me^{-\lambda^2} + 2mn e^{-c \gamma^2}. 
\end{align}
Choose $\lambda = 10 \sqrt{\log(m)}$ and $\gamma= 10 \sqrt{\log(mn)}$, and use $ \sqrt{n(m-1)}\geq \sqrt{d+d_2}+10 \sqrt{\log(m)}$ to obtain 
\begin{align} % + c' c_2c_3c_4\bar{\delta}(m, d_0+d_2)
    \mathbb{P}&\left(\frac{1}{m}\sum_{j=1}^m\|\mathbf{E}_j\|_2\geq c''' c_2c_3c_4(\sqrt{\log(nm)}+ \sqrt{d_1})(\sqrt{\log(nm)} + \sqrt{d_2})\tfrac{\sqrt{d+d_2} + \sqrt{\log(m)}}{\sqrt{nm}}  \right) \nonumber \\
    &\quad \quad \leq  2m^{-99} + 2(mn)^{-99cd_1 } + 2(mn)^{-99 c d_2} \nonumber  \\
    \implies \mathbb{P}&\left(\|\mathbf{E}'\|_2 \geq c'' c_2c_3c_4(\sqrt{\log(nm)}+ \sqrt{d_1})(\sqrt{\log(nm)} + \sqrt{d_2})\tfrac{\sqrt{d+d_2} + \sqrt{\log(m)}}{\sqrt{nm}} + c c_2c_3c_4 \bar{\delta}_{m,\max(d*,d_2)}\right) \nonumber \\
    &\quad \quad \leq  2m^{-99} + 2(mn)^{-99cd_1 } + 2(mn)^{-99 c d_2} + 2e^{-90(d_1+d_2) } \label{hghg} \\
    \implies \mathbb{P}&\left(\|\mathbf{E}'\|_2 \geq c''' c_2c_3c_4(\sqrt{\log(nm)}+ \sqrt{d_1})(\sqrt{\log(nm)} + \sqrt{d_2})\tfrac{\sqrt{d+d_2} + \sqrt{\log(m)}}{\sqrt{nm}}\right) \nonumber \\
    &\quad \quad \leq  2m^{-99} + 2(mn)^{-99cd_1 } + 2(mn)^{-99 c d_2} + 2e^{-90(d_1+d_2) } \label{hghgh}
\end{align}
% using $m>1$ and $\sqrt{nm} > \sqrt{d_1+d_4} + \sqrt{\log(m)}$.
where \eqref{hghg} follows from \eqref{hgh} and \eqref{hghgh} follows by the fact that $\bar{\delta}_{m,\max(d*,d_2)}$ is dominated.
    
    
    \begin{align}
        \left\|\frac{1}{n}\sum_{i=1}^n \mathbf{C}_{1,i}^\top \mathbf{\Sigma}_{1,i} \mathbf{C}_{2,i}\mathbf{C}_{3,i}^\top\mathbf{\Sigma}_{2,i}\mathbf{C}_{4,i} -  \mathbf{C}_{1,i}^\top \mathbf{C}_{2,i}\mathbf{C}_{3,i}^\top \mathbf{C}_{4,i}  \right\|_2
    \end{align}
    

Consider $\mathbf{E}_1$. 








To bound $\|\mathbf{E}_{1,1}\|_2$, note that each $(\mathbf{x}_{t,i,j}^{out})^\top\mathbf{q}_{t,i}\in \mathbb{R}$ is mean-zero sub-gaussian with sub-gaussian norm at most $\max_{i}\|\mathbf{q}_{t,i}\|_2 \leq \|\b\|_2 \|\w\|_2 + L_{\max}$. Also, each $\mathbf{x}_{t,i,j}^{out}\in \mathbb{R}^d$ is mean-zero sub-gaussian with norm at most $c$.  So, using $\Cov(\mathbf{x}_{t,i,j})=\mathbf{I}_d$ and Bernstein's inequality with a covering argument as in Theorem 4.6.1 in \cite{vershynin2018high}, we obtain $\|\tfrac{1}{n}\sum_{i=1}^n \sout \mathbf{q}_{t,i}\| \leq c(\|\b\|_2 \|\w\|_2 + L_{\max})\tfrac{\sqrt{d}+10}{\sqrt{nm_{out}}}$ with probability at least $1 - e^{-100}$, thus $\|\tfrac{1}{n}\sum_{i=1}^n \sout \mathbf{q}_{t,i}\mathbf{w}_t^\top\| \leq c\|\w\|_2(\|\b\|_2 \|\w\|_2 + L_{\max})\tfrac{\sqrt{d}+10}{\sqrt{nm_{out}}}$ with probability at least $1 -e^{-100}$.

To bound $\|\mathbf{E}_{1,2}\|_2$, note that the event 
$\{\|\b^\top \sout\mathbf{q}_{t,i} \|_2 \leq \|\b\|_2(\|\b\|_2 \|\w\|_2 + L_{\max})(1 +\delta_{out,k}) \forall i \in [n]\}$ 
% $\{\|\deldin\|_2 \leq \|\del_t\|_2 + \alpha\|\b\|_2^2\delta_{in,d}, \|\deldin\mathbf{q}_{t,i}\|_2\leq (\|\b\|_2 \|\w\|_2 + L_{\max})( \|\del_t\|_2+ \alpha\|\b\|_2^2\delta_{in,k}) \forall i \in [n]\}$ 
occurs with probability at least $1 - n^{-99}$ by Lemma and a union bound. Conditioning on any fixed $\{\sout\}_{i\in[n]}$ that satisfies this event, we have that each $(\mathbf{x}_{t,i,j}^{in})^\top\b \b^\top\sout\mathbf{q}_{t,i}\in \mathbb{R}$ is (mean-zero) sub-gaussian with norm at most $\|\b\|_2^2(\|\b\|_2 \|\w\|_2 + L_{\max})(1+ \delta_{out,k})\leq 2\|\b\|_2^2(\|\b\|_2 \|\w\|_2 + L_{\max})$ for all $i\in [n],j\in [m_{in}]$. Thus, we have 
\begin{align}
    \mathbb{P}\left( \|\mathbf{E}_{1,2}\|_2 \leq 2\alpha \|\mathbf{w}_t\|_2\|\b\|_2^2(\|\b\|_2 \|\w\|_2 + L_{\max})\tfrac{\sqrt{d}+10}{\sqrt{nm_{in}}}\right) \geq  1 - 2n^{-99} - e^{-100}
\end{align}
An analogous argument shows $\mathbb{P}\left( \|\mathbf{E}_{1,3}\|_2 \leq 2\alpha \|\mathbf{w}_t\|_2\|\b\|_2^2(\|\b\|_2 \|\w\|_2 + L_{\max})\tfrac{10\sqrt{d}}{\sqrt{nm_{out}}}\right) \geq  1 - 2n^{-99} - 2e^{-90d}$.







Next we bound $\|\mathbf{E}_{1,4}\|_2$. This is the most difficult term to bound because it involves fourth-order products in the inner loop samples.
First we use the triangle inequality to write 
\begin{align}
    \|\mathbf{E}_{1,4}\|_2 &\leq \bigg\|\frac{1}{n}\sum_{i=1}^n \alpha^2 \sin\b \b^\top  \sout \b \b^\top \sin \mathbf{q}_{t,i}
    \mathbf{w}_t^\top-  \alpha^2 \b\b^\top\sout \b\b^\top\mathbf{q}_{t,i}\mathbf{w}_t^\top\bigg\|_2 \nonumber \\
    &\quad + \bigg\|\frac{1}{n}\sum_{i=1}^n \alpha^2 \b \b^\top \sout \b \b^\top \mathbf{q}_{t,i}
    \mathbf{w}_t^\top-  \alpha^2 \b\b^\top \b\b^\top\mathbf{q}_{t,i}\mathbf{w}_t^\top\bigg\|_2
\end{align}
Next, we employ Lemma 
% \ref{lem:basic_concen}
and a union bound to obtain that $A \coloneqq\{\|\b^\top \sout \mathbf \b\|_2 \leq \|\b\|_2^2(1+ \delta_{out,k})\leq 2\|\b\|_2^2 \; \forall i \in [n]\}$ occurs with probability at least $1 - n^{-99}$. Now, fix any $\{\sout\}_{i\in[n]}$ that satisfies  $A$.  By Lemma \ref{lem:fourth}, we have
\begin{align}
     &\mathbb{P}\left(\left\|\frac{1}{n}\sum_{i=1}^n  \alpha^2 (\sin\b \b^\top  \sout \b \b^\top \sin \mathbf{q}_{t,i}
    -  \alpha^2 \b\b^\top \sout \b\b^\top\mathbf{q}_{t,i})^\top\right\|_2\leq \epsilon \bigg| \{\sout\}_{i\in[n]}: A\right) \geq 1 -{m_{in}}^{-99} - \tfrac{1}{\poly(nm_{in})}  \nonumber
\end{align}
for 
\begin{align}
    \epsilon &=   c\alpha^2\frac{\log^2(nm_{in})}{\sqrt{nm_{in}}} \left(k\sqrt{d} + (1+C^2)\tfrac{\sqrt{n}}{\sqrt{m_{in}}} \right) \|\b\|_2^4(\|\b\|_2\|\w\|_2 +L_{\max})
\end{align}
This implies that 
\begin{align}
   & \mathbb{P}\left(\left\|\frac{1}{n}\sum_{i=1}^n  \alpha^2 \sin\b \b^\top  \sout \b \b^\top \sin \mathbf{q}_{t,i}
    \mathbf{w}_t^\top-  \alpha^2 \b\b^\top \sout \b\b^\top\mathbf{q}_{t,i}\mathbf{w}_t^\top\right\|_2\leq \|\mathbf{w}_t\|_2\epsilon\right) 
    \nonumber \\
    &\geq 1 -2{m_{in}}^{-99} - \tfrac{1}{\poly(nm_{in})} - \mathbb{P}(A^c) \nonumber \\
    &\geq 1 -2{m_{in}}^{-99} - \tfrac{1}{\poly(nm_{in})} - 2n^{-99}.
\end{align}
Simpler analysis shows that
\begin{align}
   & \mathbb{P}\left(\left\|\frac{1}{n}\sum_{i=1}^n  \alpha^2 \b \b^\top  \sout \b \b^\top  \mathbf{q}_{t,i}
    \mathbf{w}_t^\top-  \alpha^2 \b\b^\top  \b\b^\top\mathbf{q}_{t,i}\mathbf{w}_t^\top\right\|_2\leq c\alpha^2\|\mathbf{w}_t\|_2 \|\b\|_2^4(\|\b\|_2\|\w\|_2+L_{\max})\tfrac{\sqrt{k}}{\sqrt{nm_{out}}} \right) 
    \nonumber \\
    &\geq 1 -2{e}^{-90k} \nonumber \\
\end{align}
which means that 
\begin{align}
   & \mathbb{P}\left(\left\|\mathbf{E}_{1,4}\right\|_2\leq c\alpha^2\|\mathbf{w}_t\|_2 \|\b\|_2^4(\|\b\|_2\|\w\|_2+L_{\max})\left(\frac{k\sqrt{d}\log^2(nm_{in})}{\sqrt{nm_{in}}} + \frac{1+C^2}{m_{in}}+  \frac{\sqrt{k}}{\sqrt{nm_{out}}} \right)\right) 
    \nonumber \\
    &\geq 1 -2{m_{in}}^{-99} - \tfrac{1}{\poly(nm_{in})} - 2n^{-99} -2{e}^{-90k}
\end{align}
Similar analysis shows that 
\begin{align}
   & \mathbb{P}\left(\left\|\mathbf{E}_{1,5}\right\|_2\leq  c\alpha\sigma\|\mathbf{w}_t\|_2 \tfrac{\sqrt{k}}{\sqrt{nm_{in}}}\|\b\|_2^2 (1 + \tfrac{\sqrt{d}+\sqrt{\log(n)}}{\sqrt{m_{out}}}) +c \alpha^2 \sigma\|\mathbf{w}_t\|_2\|\b\|_2^4\sqrt{1 + \delta_{out,k}}(1+\tfrac{\sqrt{d}+\sqrt{\log(n)}}{\sqrt{m_{in}}}) {\tfrac{1}{\sqrt{nm_{in}}}} \right) \nonumber \\
   &\quad \quad  \geq 1 -2{e}^{-100} - 2n^{-99} \nonumber \\
   & \mathbb{P}\left(\left\|\mathbf{E}_{1,6}\right\|_2\leq c\sigma\|\mathbf{w}_t\|_2 \tfrac{\sqrt{d}}{\sqrt{nm_{out}}} +  c\alpha\sigma\|\mathbf{w}_t\|_2 \tfrac{\sqrt{k}}{\sqrt{nm_{out}}}\|\b\|_2^2 (1 + \tfrac{\sqrt{d}+\sqrt{\log(n)}}{\sqrt{m_{in}}})\right)
    \geq 1 -2{e}^{-100} - 2n^{-99}
\end{align}


For e22, note that:
\begin{align}
\alpha\bigg\|{{\frac{1}{n}\sum_{i=1}^n  \sout \b \b^\top \sin \mathbf{q}_{t,i} \mathbf{q}_{t,i}^\top \sin \mathbf{B}_t -  \b \b^\top \mathbf{q}_{t,i}\mathbf{q}_{t,i}^\top \b}}  \bigg\|_2 &\leq \alpha\bigg\|{{\frac{1}{n}\sum_{i=1}^n  \sout \b \b^\top \sin \mathbf{q}_{t,i} \mathbf{q}_{t,i}^\top (\sin - \mathbf{I}_k) \mathbf{B}_t }}  \bigg\|_2  \nonumber \\
&\quad + \alpha\bigg\|\frac{1}{n}\sum_{i=1}^n  \sout \b \b^\top \sin \mathbf{q}_{t,i} \mathbf{q}_{t,i}^\top \mathbf{B}_t - \b \b^\top \mathbf{q}_{t,i}\mathbf{q}_{t,i}^\top \b  \bigg\|_2  \nonumber \\
&\leq \alpha\bigg\|{{\frac{1}{n}\sum_{i=1}^n  \sout \b \b^\top \sin \mathbf{q}_{t,i} \mathbf{q}_{t,i}^\top (\sin - \mathbf{I}_k) \mathbf{B}_t }}  \bigg\|_2  \nonumber \\
&\quad + \alpha\bigg\|\frac{1}{n}\sum_{i=1}^n  (\sout - \mathbf{I}_d) \b \b^\top \sin \mathbf{q}_{t,i} \mathbf{q}_{t,i}^\top \mathbf{B}_t \bigg\|_2  \nonumber \\
&\quad + \alpha\bigg\|\frac{1}{n}\sum_{i=1}^n  \b \b^\top \mathbf{q}_{t,i} \mathbf{q}_{t,i}^\top\sin \mathbf{B}_t - \b \b^\top \mathbf{q}_{t,i}\mathbf{q}_{t,i}^\top \b  \bigg\|_2  \nonumber \\
&\leq q^2/rt(\alpha)(\delta(m_{in}, k) +  \bar{\delta}(m_{out}, d) + \bar{\delta}(m_{in}, k) ) \nonumber \\
&\leq q^2/rt(\alpha)(\delta(m_{in}, k) +  \bar{\delta}(m_{out}, d))
\end{align}
Use that $\|\mathbf{q}_{t,i}^\top (\sin - \mathbf{I}_k) \mathbf{B}_t\|_2 \leq q/rt(\alpha)\delta(m_{in}, k)$ implies $\|\mathbf{q}_{t,i}^\top \sin  \mathbf{B}_t\|_2 \leq q/rt(\alpha)(1+ \delta(m_{in}, k))$




==> old.tex <==
by Weyl's inequality, 
where we have assumed $\sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top \right) = 1$ (really, it should be $\Theta(1)$, but we can deal with this later). Thus we have 
\begin{align}
    \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \|\mathbf{R}^{-1}_{t+1}\|_2 \left( 1 -  \alpha^2\kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\hat{\Sigma}}_i \mathbf{\hat{B}}_{t})
\right) \;    \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
We should be able to control $\kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\hat{\Sigma}} \mathbf{\hat{B}}_{t}))$ with high probability using $O(k)$ samples by standard matrix concentration inequalities.


    % $\tau_2^2 \lambda < L_\ast^2$, and $ \tau_2^2 \lambda \eta_\ast < L_{\max}^3$.
    % Next,
    % \begin{align}
    %     \left\|\alpha \lambda \mathbf{B}_t \frac{1}{n}\sum_{i=1}^n \mathbf{P}_{t,i} \right\|_2 &\leq  \alpha^2 \lambda  \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i} \right\|_2 + \alpha^{7/2} \lambda\left\| \frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i}^\top  \mathbf{G}_{t,i}\right\|_2 \nonumber \\
    %     &\leq c\left( \alpha^2 \lambda  (\tfrac{1}{\sqrt{\alpha}}\tau_1 + \sqrt{\tau_1} \eta_\ast + \sqrt{\alpha} \lambda \tau_2 ) + \alpha^{7/2} \lambda(\tfrac{1}{\alpha}\tau_1^2 +\tau_1 L_\ast^2 + \alpha \lambda^2 \tau_2^2  )\right) \nonumber \\
    %     &\leq c' \alpha^2 \lambda  (\tfrac{1}{\sqrt{\alpha}}\tau_1 + \sqrt{\tau_1} \eta_\ast + \sqrt{\alpha} \lambda \tau_2 )  \nonumber \\
    %     &= c'\left( \alpha^{3/2} \lambda \tau_1 + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast + \alpha^{5/2} \lambda^2 \tau_2\right)
    % \end{align}
    % assuming $\alpha^{1.5}\sqrt{\tau_1}L_\ast^2 \leq \eta_\ast$. Similarly,
    % \begin{align}
    %     \alpha^2\lambda \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i} \mathbf{P}_{t,i} \right\|_2 &\leq c(\alpha^{3/2}\lambda \tau_1 + \alpha^{5/2}\lambda^2 \tau_2 )\left\| \frac{1}{n}\sum_{i=1}^n \mathbf{P}_{t,i} \right\|_2 + \alpha^2\lambda \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{P}_{t,i} \right\|_2 \nonumber \\
    %     %%% &\leq  c'(\alpha^{3/2}\lambda \tau_1 + \alpha^{5/2}\lambda^2 \tau_2 )\alpha^{3/2}( \tfrac{1}{\sqrt{\alpha}}\tau_1 + \sqrt{\tau_1} \eta_\ast + \sqrt{\alpha} \lambda \tau_2  ) + \alpha^2 \lambda \left\| \frac{1}{\sqrt{n}}\mathbf{W}_{\ast,t} \right\|_2 \left\|\frac{1}{\sqrt{n}}[\mathbf{P}_{t,i}^\top\mathbf{w}_t]_{i=1}^n \right\|_2 \nonumber \\
    %     &\leq c'(\alpha^{3/2}\lambda \tau_1 + \alpha^{5/2}\lambda^2 \tau_2 )\alpha^{3/2}( \tfrac{1}{\sqrt{\alpha}}\tau_1 + \sqrt{\tau_1} \eta_\ast + \sqrt{\alpha} \lambda \tau_2  )+\alpha^2\lambda \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{P}_{t,i} \right\|_2 \nonumber \\
    %     % &\quad + c'\alpha^{7/2}\lambda\sqrt{\tau_1}( \tfrac{1}{\sqrt{\alpha}}\tau_1\eta_\ast  + \sqrt{\tau_1} L_\ast^2 + \sqrt{\alpha} \lambda \tau_2 \eta_\ast  ) \nonumber \\
    %     &= c'\Big(\alpha^{5/2} \lambda \tau_1^2 + \alpha^{7/2} \lambda^2 \tau_1 \tau_2 + \alpha^3 \lambda \tau_1^{3/2} \eta_\ast + \alpha^4 \lambda^2 \tau_1^{1/2} \tau_2 \eta_\ast + \alpha^{7/2}\lambda^2 \tau_1 \tau_2 +\alpha^{9/2} \lambda^3 \tau_2^2\Big) \nonumber \\
    %     &\quad +  \alpha^2\lambda \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{P}_{t,i} \right\|_2 \nonumber 
    % % & \alpha^3\lambda\tau_1^{3/2}\eta_\ast  + \alpha^{7/2}\lambda \tau_1^2 L_\ast^2 + \alpha^{4} \lambda^2 \sqrt{\tau_1} \tau_2 \eta_\ast\Big)  
    % \end{align}
    % Now,
    % \begin{align}
    %     \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{P}_{t,i} \right\|_2  &\leq \alpha^2\left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{B}_t^\top \mathbf{G}_{t,i} \right\|_2+\alpha^2\left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{G}_{t,i}^\top \mathbf{B}_t \right\|_2 \nonumber \\
    %     &\quad + \alpha^3\left\| \frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\mathbf{G}_{t,i}^\top \mathbf{G}_{t,i} \right\|_2 \nonumber \\
    %     &\leq c \alpha^2 \left(\tfrac{1}{\alpha}\eta_\ast \tau_1^{3/2} +\tfrac{1}{\sqrt{\alpha}}\tau_1 L_\ast^2 + \lambda \sqrt{\tau_1}\tau_2\eta_\ast\right) + c'\alpha^3\sqrt{\tau_1} \tfrac{\tau_1}{\sqrt{\alpha}}\left(\tfrac{\tau_1}{\alpha}\eta_\ast + \sqrt{\tau_1}L_\ast^2 + \sqrt{\alpha} \lambda \tau_2\eta_\ast  \right)  \nonumber \\
    %     &\quad + c'\alpha^3\sqrt{\alpha\tau_1}\lambda \tau_2 \left(\tfrac{\tau_1}{\alpha}\eta_\ast + \sqrt{\tau_1}L_\ast^2 + \sqrt{\alpha} \lambda \tau_2\eta_\ast  \right) \nonumber \\
    %     &\quad + c'\alpha^3\tau_1  \left(\tfrac{\tau_1}{\alpha} L_\ast^2 + \sqrt{\tau_1}L_{\max}^3 + \sqrt{\alpha} \lambda \tau_1  L_\ast^2 \right) \nonumber \\
    %     &=  c \alpha \eta_\ast \tau_1^{3/2} +c\alpha^{3/2}\tau_1 L_\ast^2 + c\alpha^2 \lambda \sqrt{\tau_1}\tau_2\eta_\ast +  c'\alpha^{3/2} \tau_1^{5/2} \eta_\ast + c'\alpha^{5/2} \tau_1^2 L_\ast^2 + c' \alpha^3 \lambda\tau_1^{3/2} \tau_2\eta_\ast  \nonumber \\
    %     &\quad + c' \alpha^{5/2}\lambda \tau_1^{3/2}\tau_2 \eta_\ast + c' \alpha^{7/2}\lambda \tau_1 
    %     \tau_2 L_\ast^2 + c' \alpha^4 \lambda \sqrt{\tau_1} \tau_2^2 \eta_\ast  \nonumber \\
    %     &\quad + c' \alpha^2 \tau_1^{2} L_\ast^2 + c' \alpha^3 \tau_1^{3/2}L_{\max}^3 + c' \alpha^{7/2} \lambda \tau_1^2 L_\ast^2 \nonumber \\
    %     &\leq c''  \alpha \eta_\ast \tau_1^{3/2}+ c'' \alpha^{3/2}\tau_1 L_\ast^2 + c''\alpha^2 \lambda \sqrt{\tau_1}\tau_2\eta_\ast + c'' \alpha^3 \tau_1^{3/2}L_{\max}^3 + c'' \alpha^{7/2}\lambda \tau_1 (\tau_1+\tau_2) L_\ast^2  \nonumber 
    %     % &\quad + c' \alpha^{7/2}\lambda \tau_1 
    %     % \tau_2 L_\ast^2  + c' \alpha^{7/2} \lambda \tau_1^2 L_\ast^2 
    % \end{align}
%     compared to 
% $\alpha^3\lambda\tau_1^{3/2}\eta_\ast  + \alpha^{7/2}\lambda \tau_1^2 L_\ast^2 + \alpha^{4} \lambda^2 \sqrt{\tau_1} \tau_2 \eta_\ast $ very different... second term must have been mistake, everything else is fine, plus we have two extra terms. check if these are subsumed promptly.
    % {\color{red}need bounds on higher-order moments of $\mathbf{w}_{\ast,t,i}$.} 
%   Hence,
%     \begin{align}
%          \alpha^2\lambda \left\| \frac{1}{n}\sum_{i=1}^n \mathbf{G}_{t,i} \mathbf{P}_{t,i} \right\|_2 &\leq  
%         &\leq 
%     \end{align}
    % We also have
    % \begin{align}
    %   \alpha^2\lambda \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{G}_{t,i}\mathbf{\Delta}_{t}\right\|_2 &\leq c \alpha^2 \tau_2 \lambda (\tfrac{1}{\sqrt{\alpha}}\tau_1 + \sqrt{\tau_1} \eta_\ast + \sqrt{\alpha} \lambda \tau_2 ) \nonumber \\
    %   &= c\alpha^{1.5}\tau_1\tau_2 \lambda + c\alpha^2\sqrt{\tau_1}\tau_2 \eta_\ast \lambda + c\alpha^{5/2} \lambda^2 \tau_2^2 
    % \end{align}
    % Thus
    % \begin{align}
    %     &\alpha \lambda \left(\|\mathbf{B}_t\mathbf{P}_{t,i}\|_2 + \alpha \|\mathbf{G}_{t,i}\mathbf{P}_{t,i}\|_2 +\alpha \|\mathbf{G}_{t,i}\mathbf{\Delta}_{t}\|_2 \right) \nonumber\\
    %     &\leq c\Big(\alpha^{3/2} \lambda \tau_1 + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast + \alpha^{5/2} \lambda^2 \tau_2 \nonumber \\
    %     &\quad +\alpha^{5/2} \lambda \tau_1^2 + \alpha^{7/2} \lambda^2 \tau_1 \tau_2 + \alpha^3 \lambda \tau_1^{3/2} \eta_\ast + \alpha^4 \lambda^2 \tau_1^{1/2} \tau_2 \eta_\ast + \alpha^{7/2}\lambda^2 \tau_1 \tau_2 +\alpha^{9/2} \lambda^3 \tau_2^2 \nonumber \\
    %     &\quad +  \alpha \eta_\ast \tau_1^{3/2}+  \alpha^{3/2}\tau_1 L_\ast^2 + \alpha^2 \lambda \sqrt{\tau_1}\tau_2\eta_\ast +  \alpha^3 \tau_1^{3/2}L_{\max}^3 +  \alpha^{7/2}\lambda \tau_1 (\tau_1+\tau_2) L_\ast^2  \nonumber \\
    %     % &\quad + \alpha^{5/2} \lambda \tau_1^2 + \alpha^{7/2} \lambda^2 \tau_1 \tau_2 + \alpha^3 \lambda \tau_1^{3/2} \eta_\ast + \alpha^4 \lambda^2 \tau_1^{1/2} \tau_2 \eta_\ast + \alpha^{7/2}\lambda^2 \tau_1 \tau_2 +\alpha^{9/2} \lambda^3 \tau_2^2 \nonumber\\
    %     % &\quad + \alpha^{1.5}\tau_1\tau_2 \lambda + \alpha^2\sqrt{\tau_1}\tau_2 \eta_\ast \lambda + \alpha^{5/2} \lambda^2 \tau_2^2  \\
    %     &\quad +  \alpha^3 \lambda\tau_1^{3/2}\eta_\ast  + \alpha^{7/2}\lambda \tau_1^2 L_\ast^2 + \alpha^{4} \lambda^2 \sqrt{\tau_1} \tau_2 \eta_\ast \Big) \nonumber \\
    % %     &\leq c\Big(\alpha^{3/2} \lambda \tau_1 + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast + \alpha^{5/2} \lambda^2 \tau_2 \nonumber \\
    % %     &\quad +\alpha^{9/2} \lambda \tau_2^2  \\
    % %     &\quad +  \alpha \eta_\ast \tau_1^{3/2}+  \alpha^{3/2}\tau_1 L_\ast^2 +   \alpha^3 \tau_1^{3/2}L_{\max}^3 +  \alpha^{7/2}\lambda \tau_1 (\tau_1+\tau_2) L_\ast^2 
    % %     % &\quad + \alpha^{5/2} \lambda \tau_1^2 + \alpha^{7/2} \lambda^2 \tau_1 \tau_2 + \alpha^3 \lambda \tau_1^{3/2} \eta_\ast + \alpha^4 \lambda^2 \tau_1^{1/2} \tau_2 \eta_\ast + \alpha^{7/2}\lambda^2 \tau_1 \tau_2 +\alpha^{9/2} \lambda^3 \tau_2^2 \nonumber\\
    % %     % &\quad + \alpha^{1.5}\tau_1\tau_2 \lambda + \alpha^2\sqrt{\tau_1}\tau_2 \eta_\ast \lambda + \alpha^{5/2} \lambda^2 \tau_2^2  \\
    % %   \Big) \nonumber \\
    %     &\leq c'\left(\alpha \eta_\ast \tau_1^{3/2}+\alpha^{3/2} \tau_1(\lambda +L_\ast^2) + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast + \alpha^{5/2} \lambda^2 \tau_2     + \alpha^{9/2} \lambda^3 \tau_2^2 +\alpha^3 \tau_1^{3/2}L_{\max}^3 \right)
    % \end{align}
    % Thus we have
    % \begin{align}
    %     \mathbf{E}_{t} \coloneqq &\Big\| \frac{1}{n}\sum_{i=1}^n\Big( -\alpha \mathbf{G}_{t,i}\boldsymbol{\Delta}_t \mathbf{w}_t\mathbf{w}_{t,i}^\top - \alpha^2 \mathbf{G}_{t,i} \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i}^\top \nonumber \\
    %      &\quad \quad \quad  \; + \alpha \lambda \mathbf{B}_t \mathbf{P}_{t,i} - \alpha^2 \lambda \mathbf{G}_{t,i} \mathbf{P}_{t,i} - \alpha^2 \lambda \mathbf{G}_{t,i} {\boldsymbol{\Delta}}_t \Big)  \Big\|_2 \nonumber \\
    %      &\leq c\bigg(\sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2} \tau_2 \eta_\ast + \alpha^{3/2}\tau_1 L_*^2  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  +  \alpha^{5/2} \tau_2 L_*^2 \lambda  \nonumber \\
    %      &\quad +\alpha \eta_\ast \tau_1^{3/2}+\alpha^{3/2} \tau_1(\lambda +L_\ast^2) + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast + \alpha^{5/2} \lambda^2 \tau_2     + \alpha^{9/2} \lambda^3 \tau_2^2 +\alpha^3 \tau_1^{3/2}L_{\max}^3  \bigg)\nonumber \\
    %      &\leq c'\bigg(\sqrt{\alpha} \tau_1^{2} \tau_2^2  + \alpha \tau_1^{3/2}  \eta_\ast + \alpha^{3/2}\tau_1 (\lambda +L_*^2)  + \alpha^2 \sqrt{\tau_1} L_{\max}^3  +  \alpha^{5/2} \tau_2 \lambda (\lambda +L_*^2) \nonumber \\
    %      &\quad + \alpha^2 \sqrt{\tau_1}\lambda \eta_\ast  + \alpha^{9/2} \lambda^3 \tau_2^2\bigg)
    %     %  &\leq c_5 L_{\max}^5\sqrt{\alpha}(\tau + \sqrt{\alpha})^2\left(1+ \lambda \tau {\alpha} \right)+ c_6 L_{\max}^2 \lambda \alpha^{1.5} (1 +\lambda \tau \alpha)  \nonumber \\
    %     %  &\leq c_7 L_{\max}^2\sqrt{\alpha}( L_{\max}^3(\tau + \sqrt{\alpha})^2 +  \lambda \alpha) (1 +\lambda \tau \alpha)  \nonumber
    % \end{align}
    % Can we say that $\alpha^2 \delta_2 > RHS$, when $\tau_2 =\alpha^2$? Every term except one has an $\alpha^2$, so maybe. Now, $\delta = \alpha (\lambda + E_0 \mu_\ast^2) - ...$. Yes, we should be able to choose this.

==> old_finite_samples.tex <==

-----


\subsection{Finite samples in inner loop}
We need to show that with finitely-many samples for the inner loop update, the $\mathbf{w}_{t,i}$'s are well-conditioned and satisfy
$\|{\mathbf{w}_{t,i}} - \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast{\mathbf{w}_{\ast,i}}\|_2 \leq \epsilon_i$, such that  $\sqrt{\frac{1}{{n}}\sum_{i=1}^n \epsilon_i^2} < \mu^2/(LL_\ast)$. 

We assume that all samples are i.i.d. sub-Gaussian with identity covariance.

Let there be $m_{in}$ inner loop samples per task.  


Assuming $m_{in}\geq k + 100\log(n)$, we have $\epsilon = c' \frac{\sqrt{k} + 10 \sqrt{\log(n)}}{\sqrt{m_{in}}}$ w.h.p. Since we need $\epsilon \leq \mu^2/(LL_\ast)$, we must set $m_{in} = \Omega (\frac{L^2(k + \log(n))}{\mu^4})$. Of course, we are not done because $L$ and $\mu$ are functions of the $\mathbf{w}_{t,i}$'s. Note that
% \begin{align}
%     \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top &= \frac{1}{n} \sum_{i = 1}^n  (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t \mathbf{{w}}_t^\top (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t) +  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} \mathbf{{w}}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_t \nonumber \\
%     &\quad \quad + (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{{w}}_t  \mathbf{{w}}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\Sigma}_{i,in}\mathbf{\hat{B}}_t +  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast\mathbf{{w}}_{\ast,i} \mathbf{{w}}_t^\top (\mathbf{I}- \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)
% \end{align}
\begin{align}
   \| \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\|_2 &= \| \frac{1}{n}  \mathbf{W}_{t,in}^\top \mathbf{W}_{t,in}\|_2 \nonumber \\
   &= \frac{1}{n}\|\mathbf{W}_{t,in}\|_2^2 \nonumber \\
   &= \frac{1}{n}\|((\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top )^\top\|_2^2 \nonumber \\
   &\leq \frac{2}{n} \|(\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top\|_2^2 +  \frac{2}{n}\|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top \|_2^2 \nonumber \\
   &\leq {2} \|\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\|_2^2 +  \frac{2}{n}\|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top \|_2^2 \nonumber \\
   &\leq c \frac{k+ 100 \log(n)}{m_{in}} + \frac{2}{n}\|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top \|_2^2 \nonumber \\
  &\leq  c \frac{k+ 100 \log(n)}{m_{in}} + {2} L_\ast^2 \|\mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \|_2^2 \nonumber \\
   &\leq 2c \frac{k+ 100 \log(n)}{m_{in}}+ {2} L_\ast^2 \left( 1 +  c\frac{k+ 100 \log(n)}{m_{in}}\right) \nonumber \\
   &\leq {2} L_\ast^2 +  2c(1+ L_\ast^2) \frac{k+ 100 \log(n)}{m_{in}} \\
   &=: L^2 
\end{align}
where $\mathbf{W}_{t,in} \in \mathbb{R}^{n \times k}$ is the matrix whose $i$-th row is equal to $\mathbf{w}_{t,i}^\top$.
Similarly, we can show
\begin{align}
  \sigma_{\min} \left( \frac{1}{n} \sum_{i = 1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) 
   &=\frac{1}{n} \sigma_{\min}^2\left( (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top + \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top  \right) \nonumber \\
   &\geq \frac{1}{n}  \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top  \right) - \frac{2}{n} \sigma_{\max}\left(  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \mathbf{W}_{\ast}^\top \right)  \sigma_{\max}\left( (\mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t)\mathbf{w}_t \mathbf{1}_n^\top\right)   \nonumber \\
   &\geq  \mu_\ast^2 \sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \right) - 2\sigma_{\max}\left(  \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_\ast \right) \sigma_{\max}\left( \mathbf{I}_k - \mathbf{\hat{B}}_t^\top \mathbf{\Sigma}_{i,in} \mathbf{\hat{B}}_t\right)   \nonumber \\
   &\geq \mu_\ast^2 \left(1 - c \frac{k+ 100 \log(n)}{m_{in}}\right) - 2 \sqrt{c/2} \left(1 + \sqrt{c/2} \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \right) \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \nonumber \\
   &= \mu_{\ast}^2 - 2c (1+ \mu_{\ast}^2) \frac{k+ 100 \log(n)}{m_{in}} - 2 \sqrt{c/2}  \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \\
   &=: \mu^2
\end{align}
with high probability. 

Since we need $\epsilon < \mu^2/L$, we require
\begin{align}
     \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}}  < \frac{ \mu_{\ast}^2 - 2c (1+ \mu_{\ast}^2) \frac{k+ 100 \log(n)}{m_{in}} - 2 \sqrt{c/2}  \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} }{\sqrt{{2} L_\ast^2 +  2c(1+ L_\ast^2) \frac{k+ 100 \log(n)}{m_{in}}}}
\end{align}
As long as (i) $2c (1+ \mu_{\ast}^2) \frac{k+ 100 \log(n)}{m_{in}} + 2 \sqrt{c/2}  \frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} \leq \mu^2_\ast/2$ and (ii) $ {2} L_\ast^2 +  2c(1+ L_\ast^2) \frac{k+ 100 \log(n)}{m_{in}} \leq L_\ast^2/2$, we have $\frac{\sqrt{k}+ 10 \sqrt{\log(n)}}{\sqrt{m_{in}}} = O(\mu_\ast^2/L_\ast)$. To satisfy (i) we require $m_{in} = \Omega ( \frac{k + \log(n)}{\mu^4_\ast})$ and to satisfy (ii) we require $m_{in} = \Omega ( {k + \log(n)})$. In total we require
\begin{align}
    m_{in} = \Omega\left(\frac{L_\ast^2(k + \log(n))}{\mu^4_\ast}\right)
\end{align}
for contraction at a constant rate with probability at least $1 - 4n^{-99}$.



\begin{lemma}
Suppose that there are infinite samples for the outer loop update, i.e. $\mathbf{B}_{t+1}= \mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right) + \mathbf{\hat{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right)$. Assume that $\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)\geq \mu^2$,  $\sigma_{\min}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \geq \mu_\ast^2 $, $ \sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)\leq L^2$, and $ \max_{i\in[n]} \|\mathbf{w}_{\ast,i}\|_2  \leq L_\ast$, and $\beta \leq 1/L^2$. Further assume that $\|\mathbf{w}_t\|_2 \leq 1$. Then 
\begin{align}
    \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast)
        &\leq \frac{1 - \mu^2 \beta }{\sqrt{(L^4 + 2 L L_\ast \mu^2 + \mu^2 \mu_\ast^2) \beta^2 - (2L^2 + 2LL_\ast )\beta + 1}}\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
\end{lemma}
\begin{proof}
    Note that 
    \begin{align}
        \mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{B}_{t+1} &= \mathbf{\hat{B}}_{\ast,\perp}^\top\mathbf{\hat{B}}_{t}\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)
    \end{align}
    Let $\mathbf{\hat{B}}_{t+1}\mathbf{R}_{t+1} = \mathbf{B}_{t+1}$ be the QR decomposition of $\mathbf{B}_{t+1}$. Then we have 
    \begin{align}
        \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) \left\|\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2 \nonumber \\
        &\leq \dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) (1 - \beta \mu^2) \|\mathbf{R}_{t+1}^{-1}\|_2 \label{contract1}
    \end{align}
    It remains to upper bound $\|\mathbf{R}_{t+1}^{-1}\|_2$. Note that
    \begin{align}
        \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
        &= \left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)^\top \left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)  \nonumber \\
        &\quad + \left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)^\top \mathbf{\hat{B}}_t^\top\mathbf{\hat{B}}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right) \nonumber \\
        &\quad + \left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right)^\top \mathbf{\hat{B}}_\ast^\top  \mathbf{\hat{B}}_t\left(\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right)  \nonumber \\
        &\quad + \left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right)^\top \left(\frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i} \mathbf{w}_{t,i}^\top \right) \nonumber
    \end{align}
    Therefore
    \begin{align}
        \sigma_{\min}^2(\mathbf{R}_{t+1}) &\geq (1 - \beta L^2)^2 - 2 \beta L L_\ast(1 - \beta \mu^2) + \beta^2 \mu^2 \mu_\ast^2 \nonumber \\
        &= (L^4 + 2 L L_\ast \mu^2 + \mu^2 \mu_\ast^2) \beta^2 - (2L^2 + 2LL_\ast )\beta + 1 =: p(\beta) \label{pbeta}
    \end{align}
    Note that if the ground truth and estimated heads are perfectly conditioned ($L_\ast = L = \mu = \mu_\ast = 1$) and $\beta = 1/L = 1$, then $\sigma_{\min}^2(\mathbf{R}_{t+1}) = 1$. Otherwise, since $p(0) = 1$, we can always choose $\beta$ small enough such that $p(\beta)$ is close to 1. Combining \eqref{contract1} and \eqref{pbeta} yields
     \begin{align}
        \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast)
        &\leq \frac{1 - \mu^2 \beta }{\sqrt{(L^4 + 2 L L_\ast \mu^2 + \mu^2 \mu_\ast^2) \beta^2 - (2L^2 + 2LL_\ast )\beta + 1}}\dist(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast)  \label{contract2}
    \end{align}

%     \begin{align}
%         \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
%         &= \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) \nonumber \\
%         &\quad + \left(\frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top\right) \left(\frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top \right) \nonumber \\
%     &= \mathbf{I}_{k} - \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) \nonumber \\
%     &\quad +\left(\frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top\right) \left(\frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top \right) 
%     \end{align}
% Therefore, using the fact that the $O(\beta^2)$ term is PSD,
% \begin{align}
% \sigma_{\min}^2(\mathbf{R}_{t+1})&\geq 1 - 2 \beta \sigma_{\max}
% \left( \frac{1}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top  \right)\end{align}
% Observe that
% \begin{align}
%     &\sigma_{\max}
% \left( \frac{1}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top  \right) \nonumber \\
% &\leq \sigma_{\max}
% \left( \frac{1}{n} \sum_{i=1}^n  \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right) +\sigma_{\max}\left(\frac{1}{n} \sum_{i=1}^n  \left( \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top\right)  \right) \nonumber \\
% &\leq \frac{1}{8\beta} + \frac{1}{8\beta} = \frac{1}{4\beta}
% \end{align}
% So \begin{align}
% \sigma_{\min}(\mathbf{R}_{t+1})&\geq  \frac{1}{\sqrt{2}}\end{align}
% meaning 
% \begin{align}
%         \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) \left\|\mathbf{I} - \frac{\beta}{n}\sum_{i=1}^n \mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top\right\|_2 \|\mathbf{R}_{t+1}^{-1}\|_2 \nonumber \\
%         &\leq \sqrt{2}(1 - \beta \mu) \dist(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) 
%     \end{align}
\end{proof}

According to Lemma 1, for contraction, we need
\begin{align}
    (  L^4 + 2 L L_\ast \mu^2 + \mu^2 \mu_\ast^2 - \mu^4) \beta &\geq     2L^2 + 2LL_\ast - 2 \mu^2 \\
    %   2  \mu^2 L_\ast/L + \mu^2 \mu_\ast^2/L^2 - \mu^4/L^2 \geq     L^2 + 2LL_\ast - 2 \mu^2 
 \text{and} \quad   \beta &\leq 1/L
\end{align}
These conditions only hold if the heads are extremely well-conditioned (e.g. $\mu^2=\mu_\ast^2 = 0.99$ and $L=L_\ast=1$ works, but $\mu^2=\mu_\ast^2 = 0.9$ and $L^2=L_\ast^2=1.2$ does not).

Alternative approach: Instead of assuming that the locally-updated heads are generally well-conditioned (without using that they may be close to the optimal solutions $\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{i,\ast}$. 




--------------
% we want the wti's to have magnitude close to 1

% {\color{red} 3/12}

Note that as long as $\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top$ and $\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{\ast,i}^\top$ are full rank, all fixed points $\mathbf{B}_t$ of (14) satisfy:
\begin{align}
    \mathbf{B}_t =  \mathbf{B}_\ast  \sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{\ast,i}^\top \left(\sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)^{-1}
\end{align}
so the column space is optimal as desired. But this almost surely never happens, i.e. almost surely $\mathbf{B}_{t+1} \neq \mathbf{B}_{t}$ due to randomness in inner loop. 

Want to show: the column space of $\mathbf{B}_t$ is fixed only if it matches that of $\mathbf{B}_*$.

We can show this as long as the coefficient matrix from the inner loop is full rank.

In particular, if the column space is fixed, i.e. $\mathbf{B}_{t+1} = \mathbf{B}_t \mathbf{R}_t$ for some full rank matrix $\mathbf{R}_t$, then we can show
\begin{align}
    \mathbf{B}_t &= \mathbf{B}_\ast  \sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{\ast,i}^\top \left(\mathbf{R}_t - \mathbf{I}_k + \sum_{i=1}^n\mathbf{w}_{t,i}\mathbf{w}_{t,i}^\top \right)^{-1}
\end{align}

This does not hold for ERM because the coefficient of $\mathbf{B}_*$ is not full rank.

The question is, is the first order ANIL dynamical system such that the column space of $\mathbf{B}_t$ reaches a stable point?
% given a dynamical system, how to show that the fixed points are reachable?
% formulate as a control problem: is wti optimal?

% process is markovian

Even simpler case: $k=1$. The optimal representation $\mathbf{b}_\ast$ is some vector on the unit sphere in $d$ dimensions. Let half of the $w_{i,\ast}$'s be 1 and the other half be $-1$. Note that the optimal initialization is $w=0$.  
% Infinite data for outer loop, finite data for inner loop.
Then:
\begin{align}
    \mathbf{b}_{t+1} &= \left( \mathbf{I}_d - \frac{\beta}{nm}\sum_{i=1}^n \sum_{j=1}^{m_{out}} {w}_{t,i}^2 \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \right)\mathbf{b}_t + \frac{\beta}{nm_{out}}\sum_{i=1}^n\sum_{j=1}^m  {w}_{t,i}{w}_{\ast,i} \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{b}_\ast
\end{align}
where 
\begin{align}
    {w}_{t,i} = {w}_{t} - \frac{\alpha}{m_{in}}\sum_{j=1}^{m_{in}} w_{t} \langle \mathbf{x}_{i,in}^j, \mathbf{b}_t \rangle^2 - w_{\ast,i} \langle \mathbf{x}_{i,in}^j,  \mathbf{b}_t \rangle \langle \mathbf{x}_{i,in}^j,  \mathbf{b}_\ast \rangle
\end{align}
Suppose $w_t$ is optimal, i.e. $w_t=0$. Then
\begin{align}
    {w}_{t,i} &= \frac{\alpha}{m_{in}}\sum_{j=1}^{m_{in}} w_{\ast,i} \langle \mathbf{x}_{i,in}^j,  \mathbf{b}_t \rangle \langle \mathbf{x}_{i,in}^j,  \mathbf{b}_\ast \rangle \nonumber \\
    % &= \alpha  w_{\ast,i} \langle \mathbf{b}_t, \mathbf{b}_\ast \rangle +  {\alpha} w_{\ast,i} \mathbf{b}_t^\top \mathbf{E}_m \mathbf{b}_\ast \nonumber \\
    % &=  w_{\ast,i} \langle \mathbf{b}_t, \mathbf{b}_\ast \rangle + w_{\ast,i} \mathbf{b}_t^\top \mathbf{E}_m \mathbf{b}_\ast \nonumber \\
    &= w_{\ast,i} \langle \mathbf{b}_t,\mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle
\end{align}
where in the last step we have set $\alpha=1$ and let $\mathbf{\bar{\Sigma}}_i = \frac{1}{m_{in}}\sum_{j=1}^{m_{in}} \mathbf{x}_{i,in}^j (\mathbf{x}_{i,in}^j)^\top$.
So 
\begin{align}
{w}_{t,i}^2 &=  \langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle^2
\end{align}
and 
\begin{align}
    \mathbf{b}_{t+1} &= \left( \mathbf{I}_d - \frac{\beta}{nm_{out}}\sum_{i=1}^n \sum_{j=1}^{m_{out}}\langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle^2 \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \right)\mathbf{b}_t + \frac{\beta}{nm_{out}}\sum_{i=1}^n\sum_{j=1}^{m_{out}}  \langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{b}_\ast \nonumber
\end{align}
for infinite outer loop samples, we have
\begin{align}
    \mathbf{b}_{t+1} &= \left( 1 - \frac{\beta}{n}\sum_{i=1}^n \langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle^2 \right)\mathbf{b}_t + \frac{\beta}{n}\sum_{i=1}^n \langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle \mathbf{b}_\ast \nonumber
\end{align}
Now, for unit norm $\mathbf{b}_t$, we need to control $\langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_i \mathbf{b}_\ast \rangle^2$, which we can do with $m_{in} = O(k) = O(1)$ samples, assuming they are sub-Gaussian.

So for $n=1$ and $\beta=1$, we have the system:
\begin{align}
    \mathbf{b}_{t+1} &= (1-z_t^2) \mathbf{b}_{t} + z_t \mathbf{b}_\ast \nonumber \\
    &= \prod_{i=1}^{t} (1-z_i^2)  \mathbf{b}_{1} + \sum_{s=1}^t z_s  \mathbf{b}_\ast \prod_{i=s}^{t-1} (1-z_i^2) \nonumber
\end{align}
where $z_t = \langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_1 \mathbf{b}_\ast \rangle $ is a sub-Gaussian random variable with mean $\langle \mathbf{b}_t, \mathbf{b}_\ast\rangle$. Thus $\mathbf{b}_t$ is always  some linear combination of $\mathbf{b}_1$ and $\mathbf{b}_\ast$. How does this system behave?

We have 
\begin{align}
\|\mathbf{b}_{t+1}\|_2 &= \sqrt{(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} } \nonumber \\
    \frac{(\mathbf{b}_\ast^\top \mathbf{b}_{t+1})^2}{\|\mathbf{b}_{t+1}\|_2^2} > (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2 &\iff (1-(\mathbf{b}_\ast^\top \mathbf{b}_{t})^2)(2 \mathbf{b}_\ast^\top \mathbf{b}_{t} (1- z_t^2) + z_t) > 0 \nonumber \\
    &\iff 2 \mathbf{b}_\ast^\top \mathbf{b}_{t} (1- z_t^2) + z_t > 0 %\nonumber \\
    % &\iff 2 \mathbf{b}_\ast^\top \mathbf{b}_{t} - 2 \mathbf{b}_\ast^\top \mathbf{b}_{t} z_t^2 + z_t > 0
    %\frac{(1-z_t^2) \mathbf{b}_\ast^\top\mathbf{b}_{t} + z_t }{\sqrt{(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} }} > \mathbf{b}_\ast^\top \mathbf{b}_{t} 
\end{align}
%(0.9 - 0.9x^2 + x)/(\sqrt{1-x^2 + x^4 + 2*0.9*x(1-x^2) })
This is a quadratic that is positive on, roughly, $z_t \in [-0.75, 1.25]$, for all $\mathbf{b}_\ast^\top \mathbf{b}_{t} \in (0,1)$. Thus, the sequence $\left\{\frac{(\mathbf{b}_\ast^\top \mathbf{b}_{t})^2}{\|\mathbf{b}_{t}\|_2^2}\right\}_t$ is {\em not non-decreasing}.

% Numerically, we find that $0<z_t < 5/4$ implies the condition on the RHS, as the upper bound on $z_t$ approaches 5/4 from above as $\mathbf{b}_\ast^\top \mathbf{b}_t$ approaches 1.

% Since $z_t$ is sub-exponential with mean $\mathbf{b}_\ast^\top \mathbf{b}_t \in (0,1)$, we have that $\mathbf{b}_\ast^\top \mathbf{b}_t$ increases infinitely often or it reaches and remains at 1. All that is left to show is that the decrease is not too large. Consider 
% \begin{align}
%     \frac{(\mathbf{b}_\ast^\top \mathbf{b}_{t+1})^2}{\|\mathbf{b}_{t+1}\|_2^2} &= \frac{(\mathbf{b}_\ast^\top \mathbf{b}_{t})^2 - 2 (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2 z_t^2 + 2\mathbf{b}_\ast^\top \mathbf{b}_{t} z_t - 2 \mathbf{b}_\ast^\top \mathbf{b}_{t} z_t^3 + (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2z_t^4 + z_t^2 }{(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} } 
%     % &=  \frac{2(\mathbf{b}_\ast^\top \mathbf{b}_{t})^2( 1 - z_t^2) + 2\mathbf{b}_\ast^\top \mathbf{b}_{t}z_t( 1 - z_t^2) + (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2(z_t^4 - 1) + z_t^4
%     % } %correct, just notes
%     % {(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} } \nonumber \\
%     %old below
%     %  &=  \frac{( 1 - z_t^2)( 2\mathbf{b}_\ast^\top \mathbf{b}_{t} z_t + (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2(z_t^2 + 3) ) + z_t^4
%     % }
%     % {(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} } 
% \end{align}

% If $z_t > 5/4$, we have
% \begin{align}
%     \frac{(\mathbf{b}_\ast^\top \mathbf{b}_{t+1})^2}{\|\mathbf{b}_{t+1}\|_2^2} 
%      &=  \frac{( 1 - z_t^2)( 2\mathbf{b}_\ast^\top \mathbf{b}_{t} z_t + (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2(z_t^2 + 3) ) + z_t^4
%     }
%     {(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} }  \nonumber \\ 
%     &\geq \frac{( 1 - z_t^2)( 2\mathbf{b}_\ast^\top \mathbf{b}_{t} z_t + (\mathbf{b}_\ast^\top \mathbf{b}_{t})^2(z_t^2 + 3) ) + 2
%     }
%     {(1-z_t^2)^2 + z_t^2 + 2z_t(1-z_t^2)\mathbf{b}_\ast^\top \mathbf{b}_{t} }  \nonumber \\
% \end{align}

% goal: show that since this thing is lower bounded, it ultimately converges
% do we need to lower bound it? familiarize with other ds

Instead, note that $\mathbf{b}_{t+1} = (1-z_t^2) \mathbf{b}_{t} + z_t \mathbf{b}_\ast$ describes the dynamics of a Markov chain on $\mathbb{R}^d$. For simplicity assume $d=1$, then $|b_\ast|=1$.  WLOG we have $z_t \sim \mathcal{N}( {b}_t {b}_\ast, {b}_t^2\sigma^2 )$. 

An equivalent description of the dynamics is
\begin{align}
    {b}_{t+1} =  {b}_{t} - {b}_{t}^3\epsilon_t^2 + b_t \epsilon_t = b_t(1 + \epsilon_t - {b}_{t}^2\epsilon_t^2)
\end{align}
where $\epsilon_t \sim \mathcal{N}(1, \sigma^2)$. Close to stationary, we have $b_{t+1} \approx  b_t \implies \epsilon_t - b_t^2 \epsilon_t^2 \approx  0 \implies b_t^2 \approx \epsilon_t$ as long as $b_t \neq 0$. If $\epsilon_t$ is well-concentrated about its mean 1, then we have $b_t^2 \approx 1$ as desired. But if $\epsilon_t$ has high variance, then the Markov chain may explode. Empirically, we find a phase transition around $\sigma = 1/4$ when $d=10$. 

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.4\columnwidth]{mamlrep1.png}}
\vspace{-0mm}
\caption{For $d=10$, $\langle \mathbf{b}_t, \mathbf{b}_\ast \rangle^2/\|\mathbf{b}_t\|_2^2$ reaches fixed (and optimal) point for sufficiently small $\sigma$. (In the general $d$ case, we have
$z_t \sim \mathcal{N}( \langle \mathbf{b}_t, \mathbf{b}_\ast\rangle, \langle \mathbf{b}_t, \mathbf{b}_\ast\rangle^2\sigma^2 )$.)}
\label{fig:new_clients22}
\end{center}
\vspace{-0mm}
\end{figure}

For $d=2$ and $n=1$, recall
\begin{align}
    \mathbf{b}_{t+1} = (1 - \beta z_t^2) \mathbf{b}_t + \beta z_t \mathbf{b}_\ast
\end{align}
where $z_t = \langle \mathbf{b}_t, \mathbf{\bar{\Sigma}}_1 \mathbf{b}_\ast \rangle$. We will again achieve convergence in one step if we set $\beta = 1/z_t^2$.

The interesting case is when $k>1$. Set $k=2$ and $d=2$. Then
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{B}_{t} \left(  \mathbf{I}_d -  \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \mathbf{w}_{t,i}^\top\right) +  \mathbf{B}_\ast\left(\frac{\beta}{n} \sum_{i=1}^n   \mathbf{w}_{i,\ast} \mathbf{w}_{t,i}^\top\right) \label{k2}
\end{align}
where $\mathbf{w}_{t,i} =  \alpha\mathbf{B}_t^\top \mathbf{\bar{\Sigma}}\mathbf{B}_\ast\mathbf{w}_{i,\ast}$, assuming again that $\mathbf{w}_t$ is the optimal initialization for the heads, i.e. $\mathbf{w}_t = \mathbf{0}$. So 
\begin{align}
    \mathbf{B}_{t+1} &= \mathbf{B}_{t} \left(  \mathbf{I}_d -  \beta \alpha^2 \mathbf{B}_t^\top \mathbf{\bar{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\bar{\Sigma}} \mathbf{B}_t\right) +  \mathbf{B}_\ast\left(\beta \alpha  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top \mathbf{\bar{\Sigma}} \mathbf{B}_t \right)
\end{align}

We aim to write the update in the same form as the $k=1$ case. Let $\mathbf{B}_{\ast} = [\mathbf{b}_{\ast,1}, \mathbf{b}_{\ast,2}]$ where $\mathbf{b}_{\ast,1}, \mathbf{b}_{\ast,2}\in \mathbb{R}^d$, $\mathbf{B}_{t} = [\mathbf{b}_{t,1}, \mathbf{b}_{t,2}]$ and $\mathbf{B}_{t+1} = [\mathbf{b}_{t+1,1}, \mathbf{b}_{t+1,2}]$. Also let $\mathbf{w}_{\ast,i} = [{w}_{\ast,i,1}; {w}_{\ast,i,2}] \in \mathbb{R}^k$. Then
\begin{align}
       \mathbf{b}_{t+1,1} &= \mathbf{B}_{t} \left(  \begin{bmatrix}1 \\
       0 \\
       \end{bmatrix} -  \beta \alpha^2 \mathbf{B}_t^\top \mathbf{\bar{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\bar{\Sigma}} \mathbf{b}_{t,1}\right) +  \mathbf{B}_\ast\left(\beta \alpha  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top \mathbf{\bar{\Sigma}} \mathbf{b}_{t,1} \right)  \nonumber \\
&=  \left(  \mathbf{I}_d -  \left(\alpha \mathbf{B}_{t}\mathbf{B}_t^\top \mathbf{\bar{\Sigma}} - \mathbf{I}_d \right) \beta \alpha \mathbf{B}_\ast  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top \mathbf{\bar{\Sigma}}  \right)\mathbf{b}_{t,1}  \nonumber  \\
\mathbf{B}_{t+1}&=  \left(  \mathbf{I}_d -  \left(\alpha \mathbf{B}_{t}\mathbf{B}_t^\top \mathbf{\bar{\Sigma}} - \mathbf{I}_d \right) \beta \alpha \mathbf{B}_\ast  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top \mathbf{\bar{\Sigma}}  \right)\mathbf{B}_{t}  \nonumber 
\end{align}
We need to show that the spectral norm of the coefficient of $\mathbf{B}_{t}$ in the RHS is less than 1 whp. Note that we have the same structure as in the previous $k=1$ case, as here showing stationarity comes down to showing $\alpha \mathbf{B}_{t}\mathbf{B}_t^\top \mathbf{\bar{\Sigma}} \approx \mathbf{I}_d $. Exact equality is a measure zero event. What does approximate equality show?

Instead, multiplying both sides of \eqref{k2} by $\mathbf{B}_{\ast,\perp}^\top$ and using Cauchy-Schwarz, and noting $i$ subscript was missing on $\mathbf{\bar{\Sigma}}$ above, we have
\begin{align}
   \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \|\mathbf{R}^{-1}_{t+1}\|_2 \left\| \mathbf{I}_d -  \beta \alpha^2 \frac{1}{n}\sum_{i=1}^n\left( \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast   \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}\right)
\right\|_2 \;    \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
where $\mathbf{\hat{B}}_{t+1}\mathbf{R}_{t+1} = \mathbf{B}_{t+1}$ is the QR decomposition of $\mathbf{B}_{t+1}$.

Set $\beta = 1/\|\frac{1}{n}\sum_{i=1}^n\left( \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast   \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}\right)\|_2 \geq 1/\left(\frac{1}{n}\sum_{i=1}^n \|\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}\|_2^2  \right)$ assuming $\left\|\mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right\|_2 = 1$ for all $i$. 

Further, suppose that $\mathbf{w}_{\ast,i} = \mathbf{e}_{j(i)}$ for all $i \in [n]$, where $j(i)$ is some mapping from $[n]$ to $[k]$. We have 
\begin{align}
    \frac{1}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast  \left( \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}  &= \frac{1}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{{b}}_{\ast,i'}  \mathbf{{b}}_{\ast,i'}^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t} = \mathbf{\hat{B}}_t^\top\left(\frac{1}{n}\sum_{i=1}^n  \mathbf{\bar{\Sigma}}_i  \mathbf{{b}}_{\ast,i'}  \mathbf{{b}}_{\ast,i'}^\top \mathbf{\bar{\Sigma}}_i \right)\mathbf{\hat{B}}_{t} %\frac{1}{n}\sum_{i=1}^n\sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast \right) \sigma_{\min}\left(\mathbf{w}_{\ast,
%i} \mathbf{w}_{\ast,i}^\top \right) = \frac{1}{n}\sum_{i=1}^n\sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast \right)
\end{align}
% \begin{align}
%     \sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast  \left( \mathbf{w}_{\ast,
% i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t} \right) &\geq %\frac{1}{n}\sum_{i=1}^n\sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast \right) \sigma_{\min}\left(\mathbf{w}_{\ast,
% %i} \mathbf{w}_{\ast,i}^\top \right) = \frac{1}{n}\sum_{i=1}^n\sigma_{\min}^2\left( \mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i  \mathbf{\hat{B}}_\ast \right)
% \end{align}
This is the sum of nm2 outer products of two subgaussian random vectors with variance parameter O(k/rt(m)) and two subgaussian random variables with variance parameter O(1/rt(m)). Thus we should be able to use matrix concentration results here.

% {\color{red} left off here}


% by Weyl's inequality, 
% where we have assumed $\sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
% i} \mathbf{w}_{\ast,i}^\top \right) = 1$ (really, it should be $\Theta(1)$, but we can deal with this later). Thus we have 
% \begin{align}
%     \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \|\mathbf{R}^{-1}_{t+1}\|_2 \left( 1 -  \alpha^2\kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t})
% \right) \;    \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
% \end{align}
% We should be able to control $\kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}} \mathbf{\hat{B}}_{t}))$ with high probability using $O(k)$ samples by standard matrix concentration inequalities.

Next, we can show:
\begin{align}
    \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1} &= \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} \nonumber \\
    &= \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_{t} - \frac{\beta}{n} \sum_{i=1}^n \left(\mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_t \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_t - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber \\
    &= \mathbf{I}_{k} - \frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top - \frac{\beta}{n} \sum_{i=1}^n \mathbf{w}_{t,i} \left( \mathbf{w}_{t,i}^\top - \mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \right) + O(\beta^2)  \nonumber
\end{align}
Note that
\begin{align}
    \mathbf{w}_{t,i} = \alpha\mathbf{\hat{B}}_t^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}
\end{align}
so we have 
\begin{align}
    \sigma_{\max}\left(\frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top \right) &=  \frac{\beta}{n}\sigma_{\max}\left( \mathbf{\hat{B}}_t\sum_{i=1}^n \left( \alpha \mathbf{\bar{\Sigma}}_i - \mathbf{I}_d \right)\mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{t,i}^\top \right) \nonumber \\
    &\leq  \frac{ \alpha \beta}{n}\sum_{i=1}^n \sigma_{\max}\left( \mathbf{\hat{B}}_t \left( \alpha \mathbf{\bar{\Sigma}}_i - \mathbf{I}_d \right)\mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}\right) \nonumber \\
    &\leq \frac{ \alpha \beta}{n}\sum_{i=1}^n \sigma_{\max}\left( \mathbf{\hat{B}}_t \left( \alpha \mathbf{\bar{\Sigma}}_i - \mathbf{I}_d \right)\mathbf{\hat{B}}_\ast\right)\sigma_{\max}\left( \mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t}\right)
\end{align}
which we can upper bound close to zero with high probability given O(k) samples, and setting $\alpha=1$.
Say that this bound is $B$, then
% that the cross terms concentrate to zero, i.e.
% \begin{align}
%     \mathbb{E}(\frac{\beta}{n} \sum_{i=1}^n \left( \mathbf{w}_{t,i} - \mathbf{\hat{B}}_{t}^\top \mathbf{\hat{B}}_\ast \mathbf{w}_{\ast,i}\right)\mathbf{w}_{t,i}^\top)  = \mathbf{0}.
% \end{align}
since the $O(\beta^2)$ term is PSD, we have
\begin{align}
    \lambda_{\min}\left( \mathbf{R}_{t+1}^\top \mathbf{R}_{t+1}\right) \geq 1 - 2B \implies \|\mathbf{R}^{-1}_{t+1}\|_2 \leq \frac{1}{\sqrt{1-2B}}
\end{align}
Thus
\begin{align}
    \text{dist}(\mathbf{\hat{B}}_{t+1}, \mathbf{\hat{B}}_\ast) &\leq \frac{ 1 -  \kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t})
}{\sqrt{1-2B}} \;    \text{dist}(\mathbf{\hat{B}}_{t}, \mathbf{\hat{B}}_\ast) 
\end{align}
with high probability.
It remains to compute the high probability bound $B$ and the high probability bound on $\kappa^{-1}(\mathbf{\hat{B}}_\ast^\top \mathbf{\bar{\Sigma}}_i \mathbf{\hat{B}}_{t})$.

==> old_june21_notes.tex <==


\textbf{Two tasks}

% \begin{definition}
% We say that a set of vectors ${\mathbf{w}_{t,i}}_i$ in $\mathbb{R}^k$ is {\em $\mu$-diverse} if $\sum_i \mathbf{w}_{t,i}\mathbf{w}_{t,i}^T$ spans 
% \end{definition}

Here $d=5$, $r=2$. 

There is a ground-truth representation $\mathbf{A}_\ast \in \mathbb{R}^{d \times r}$ and two ground-truth heads $\mathbf{w}_{1,\ast}, \mathbf{w}_{2,\ast} \in \mathbb{R}^r$, such that $(i)$ in the diverse task case: $\mathbf{w}_{1,\ast} = [1,1]/\sqrt{2}$ and $\mathbf{w}_{2,\ast} = [1,-1]/\sqrt{2}$, $(ii)$ in the non-diverse task case: $\mathbf{w}_{1,\ast} = [1,1]/\sqrt{2}$ and $\mathbf{w}_{2,\ast} = [-1,-1]/\sqrt{2}$. 

Meanwhile, we try to learn a representation $\mathbf{A} \in \mathbb{R}^{d \times k}$ and heads $\mathbf{w}_{1,\ast}, \mathbf{w}_{2,\ast} \in \mathbb{R}^k$. In the over-specified case we have $k>r$, otherwise $k=r$.

The loss function for task $i$ is $f_i(\mathbf{A}, \mathbf{w}) = \frac{1}{2m} \|\mathbf{X}_i \mathbf{A}\mathbf{w} - \mathbf{y}_i\|_2^2$. 

ERM: $\min_{\mathbf{A},\mathbf{w}}  \sum_{i} f_i(\mathbf{A}, \mathbf{w})$

ANIL: $\min_{\mathbf{A},\mathbf{w}} \sum_{i} f_i(\mathbf{A}, \mathbf{w}-\alpha \nabla_\mathbf{w} f_i(\mathbf{A}, \mathbf{w}))$

MAML: $\min_{\mathbf{A},\mathbf{w}} \sum_{i} f_i(\mathbf{A}-\alpha \nabla_\mathbf{A} f_i(\mathbf{A}, \mathbf{w}), \mathbf{w}-\alpha \nabla_\mathbf{w} f_i(\mathbf{A}, \mathbf{w}))$

In all cases there was no meaningful difference between ANIL training and MAML training, so in all plots we only plot the results for ANIL. 

In all cases the excess risk is evaluated according to the MAML framework (both $\mathbf{A}$ and $\mathbf{w}$ are updated via one minibatch SGD step for the task before testing).

In the diverse task case the updated heads have rank 2 in expectation, which is smaller than the ambient dimension (5), but matches the dimension of the true representation. In the non-diverse task case they have rank 1 in expectation, which is less than the dimension of the true representation.


\begin{figure}[h]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=\columnwidth]{anil_nos_diverse_04_0.4.pdf}}
\vspace{-0mm}
\caption{Exactly specified ($k=r$), diverse tasks}
\label{fig:11}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[h]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=\columnwidth]{anil_nos_ndiverse_04_0.4.pdf}}
\vspace{-0mm}
\caption{Exactly specified ($k=r$), non-diverse tasks}
\label{fig:11}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[h]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=\columnwidth]{anil_os_diverse__04_0.4.pdf}}
\vspace{-0mm}
\caption{Overspecified ($k=d$), diverse tasks}
\label{fig:11}
\end{center}
\vspace{-0mm}
\end{figure}


\begin{figure}[h]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=\columnwidth]{anil_os_ndiverse_04_0.4.pdf}}
\vspace{-0mm}
\caption{Overspecified ($k=d$), non-diverse tasks}
\label{fig:11}
\end{center}
\vspace{-0mm}
\end{figure}

Takeaway: task diversity is key even in overspecified case.

\newpage

\begin{table}[h]
\caption{Orthogonalizing the heads. $T=100$.}
\vspace{-2mm}
\label{table:data}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ccccc}
\toprule
Dataset & FedRep & FedRep+ortho & ANIL & ANIL+ortho\\
\midrule
% CIFAR10, $S=2, n=100, m=50$  & 74.99  & 74.49  &   & \\
CIFAR10, $S=2, n=100$  & 85.26  & 82.02  &  84.61 &  81.53 \\
CIFAR10, $S=5, n=100$    &  69.91  &  72.03  & 71.86  & 70.84 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


% notes: we may not need to learn the right representation, only the right product BW, if we assume the W
% todo: nuclear norm regularization, evaluate full B on new task. figure out how lee deals with high-dimensional case. analyze only product and make assump on new w? does new jin paper lean true rep? or the product? note new notion of distance of rep in terms of error of classifier
% jin paper: you can always learn the representation by solving fedrep. they consider exactly specified case
% open questions: how fast, how many iterations of SGD, are needed to reach a global min of the proposed objective? since the proposed objective is nonconvex, is it possible to reach a global min? what are the properties of the stationary points? do these results still hold in over-specified case? do sample complexitu benefits still hold even in overspecified case?. try more layers
% lee paper claims that their result extends to overparameterized case easily
% in high-dimensional case there is no benefit of rep learning
% can we show that global min of over specified problem learns rep?
% lee does not assume task diversity in high dim - only that new task is coherent w train
%they only consider property of global min
%proof of thrm 6.1: relies on regularization. can it extend to overspecified? they dont need task diversity. task diversity only needs to match diversity of new task...
% the new insight is that anil optimizes a version of the fedrep loss if we look at BW...
% does our optimization result that MAML learns rep but ERM doesn't contradict the recent Jin result: no because ERM doesn't solve the fedrep objective
% ARGUMENT: MAML learns rep better than ERM because of task diversity.

% interesting cases:
% 1. linear, exactly specified
%.   a. we know task diversity is key. can we show excess risk benefit of MAML over ERM? numerically, yes. with high probability erm does not find ground truth rep and performs worse on new task.
% 2. linear, over specified
%.   a. key is that k < d. otherwise, no difference between erm and anil if we solve least squares for the head because erm learns everything. but this means we use m>=d samples. if we just take one step of gd, then then both erm and anil are pretty bad, for all small sample sizes, anil gets small improvement after many iters
% 3. linear, high-dimensional but intrinsic dim of rep is small
%    a. 

% can subspace task diversity help even in overspecified case? this is the question. this was considered sort of by saunshi. but there was no notion of task diversity, only considered r=1 and exact initialization.
% we need good init in order to find init in over specified case. but we need good init even in exactly specified case too
% would answering this question just be a generalization of saunshi? surely it would be an extension of jin and lee
% jin paper relies on task diversity up to r, the dim of the last layer. can we still learn a high-performing rep even in overspecified case? do they assume that ground truth rep is strictly last layer length r?


% from simulations: why does anil have a bias?
% why is erm performing better on a new task?
% in exactly specified case with d large, there is slight but meaningful advantage for anil
% and in overspecified case there is still advantage as long as k << d
% in overspecified case both maml and erm solve problem exactly if allowed to compute the least squares solution for the head, as long as m >= d = k. if m = k < d, then anil gets slight gain. if m>= d > k, then anil still gets gain over erm. so the key is k < d (even if k > r).
% so what happens in 

% most realistic case: d >> k > r. show that anil picks out the r directions among its k choices, whereas erm does not, as long as tasks have rank r

% or: d = k, test tasks in same direction as train, show anil gain as long as intrinsic dimension >> frob. but i don't think this is realistic.

% problem: lee relu result does not rely on low dimension, only intrinsic dim of Sigma. 
% so we should see 

% lee: thrm 6.1. they assume there exists a teacher network with finitely-many neurons so that when they extend the relu to infinite dimensional problem, they don't have to solve it exactly, they only have to beat the best solution that is d-sparse (the teacher network)
% 6.1 still requires low rank teacher ( << d) for meaningful gain. does thrm 7.1 require the same?
% this matters because we are relying on k << d
% we want the rank of thete* to matter, otherwise erm may also lesrn it. specifically, if the rank of thete* is o(d), then we need k = o(d). we do not expect anil gain over erm in this setting but maybe it can still happen for relu). so if rep learning helps even in this setting, then anil does not achieve the full benefits of rep learning.
% answe: they mysteriously go from R = nuclear norm in thrm 6.1 to R= frob2 in thrm 7.1, which allows them to not have a rank dependence in the LHS... yeah i think it is a bug. the nuclear norm in 6.1 does not only arise because of the regularization
% so - even for high-dim rep and non-linear case, low rank still matters and still implicitly assumed. question remains: what is the difference between assuming low rank and low dim? if it is low-rank but high dim, do tasks need to span the rank or span the dim? answer: they need to be such that B*w*1,...,B*w*n \in R^d spans the r-dim subspace (r = rank(B)). then anil learns B whose span, of dim k, includes this subspace, but erm does not.
% in relu case it is similar? 7.1 tells us that yes the span of B still matters. but need to read Wei paper to see how to optimize it, in particular whether anil may recover the span.

% jin2 paper: we can remove the assumption that the feature map has to be well-conditioned.
% relies on exactly specified last layer (there is a ground truth teacher network that is rank r and has r-diverse tasks. and our model has rank r final layer.

% interesting extension: our model is larger than the rank of the teacher, but it is still << d. show that we still get gain with anil (and fedrep)



% steps:
% show that all global min of 


\section{Two-Layer Linear Network, General Overspecified}
The following holds:
\begin{itemize}
\item Data for the $i$-th task is generated as ${y}_i = \mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top \mathbf{x}_i$ where $\mathbf{x}_i$ is sampled from a sub-gaussian distribution with covariance $\mathbf{I}_d$. 
    \item $\mathbf{w}_{\ast,i} \in \mathbb{R}^r$, $\mathbf{W}_\ast \in \mathbb{R}^{n \times r}$, $\mathbf{B}_\ast \in \mathbb{R}^{d \times r}$, and we let $\mathbf{M}_\ast \coloneqq \mathbf{W}_\ast\mathbf{B}_\ast^\top$.
    \item Given $\mathbf{x}_i$, the $i$-th user predicts ${\hat{y}}_i = \mathbf{w}^\top \mathbf{B}^\top \mathbf{x}_i$, where  $\mathbf{w} \in \mathbb{R}^k$, $\mathbf{B} \in \mathbb{R}^{d \times k}$ for some $r\leq k < \min(d,n)$. We will generally assume $k<< d$ so that we can still obtain sample complexity benefits on a new task.
    \item The population loss function is $f(\mathbf{w}, \mathbf{B}) \coloneqq \frac{1}{2n}  \sum_{i=1}^n f_i(\mathbf{w}, \mathbf{B})$, where $f_i(\mathbf{w}, \mathbf{B})\coloneqq \mathbb{E}_{\mathbf{x}_i ,y_i}[\|\mathbf{w}^\top\mathbf{B}^\top \mathbf{x}_i - y_i\|_2]$ Note that $ f(\mathbf{w}, \mathbf{B})= \|\mathbf{1}\mathbf{w}^\top \mathbf{B}^\top - \mathbf{M}_\ast \|_F^2$. 
    \item We consider the ANIL framework: we are allowed to take one gradient step w.r.t. the head for each task before evaluation. Then the ANIL loss is $f_{ANIL}(\mathbf{w}, \mathbf{B})\coloneqq \frac{1}{2n}  \sum_{i=1}^n f_i(\mathbf{w} - \alpha \nabla_{\mathbf{w}} f_i(\mathbf{w}, \mathbf{B}), \mathbf{B}) $.
    \item We let $\mathbf{M}_\ast = \mathbf{U}_1 \mathbf{\Sigma} \mathbf{V}_1^\top$ be an SVD of $\mathbf{M}_\ast$. Note that $\mathbf{U}_1 \in \mathbb{R}^{n\times r}$, $\mathbf{\Sigma} \in \mathbb{R}^{r \times r}$ and $\mathbf{V}_1 \in \mathbb{R}^{d \times r}$. Let $\mathbf{U}_2 \in \mathbb{R}^{n\times(n- r)}$ and $\mathbf{V}_2 \in \mathbb{R}^{d \times (d-r)}$ such that $[\mathbf{U}_1, \mathbf{U}_2]$ is an orthonormal basis of $\mathbb{R}^n$ and $[\mathbf{V}_1, \mathbf{V}_2]$ is an orthonormal basis of $\mathbb{R}^d$.
    \item For any matrices $\mathbf{W} \in \mathbb{R}^{n\times k}$ and $\mathbf{B} \in \mathbb{R}^{d\times k}$, we can write $\mathbf{W} = \mathbf{U}_1 \mathbf{W}_1 + \mathbf{U}_2 \mathbf{W}_2$ and $\mathbf{B} = \mathbf{V}_1 \mathbf{B}_1 + \mathbf{V}_2 \mathbf{B}_2$.
\end{itemize}

\subsection{Population Case}

We consider the population loss: $ f(\mathbf{W}, \mathbf{B})= \| \mathbf{W} \mathbf{B}^\top - \mathbf{M}_\ast \|_F^2 $. 

For general $\mathbf{W}$, we have
$\mathbf{G}_{\mathbf{W}}(\mathbf{W},\mathbf{B}) \coloneqq \nabla_{\mathbf{W}} f(\mathbf{W}, \mathbf{B}) = \mathbf{U}_1(\mathbf{W}_1 \mathbf{B}_1^\top - \mathbf{D}) \mathbf{B}_1 + \mathbf{U}_2 \mathbf{W}_2 \mathbf{B}_1^\top \mathbf{B}_1 + \mathbf{W} \mathbf{B}_2^\top \mathbf{B}_2$ thus \begin{align}
    \mathbf{W}_+ \coloneqq \mathbf{W} - \alpha\mathbf{G}_{\mathbf{W}}(\mathbf{W},\mathbf{B}) &= \mathbf{U}_1(\mathbf{W}_1(\mathbf{I} - \alpha \mathbf{B}_2^\top \mathbf{B}_2 ) ) -\alpha (\mathbf{W}_1 \mathbf{B}_1^\top - \mathbf{D}) \mathbf{B}_1) \nonumber \\
    &\quad + \mathbf{U}_2( \mathbf{W}_2 (\mathbf{I} - \alpha \mathbf{B}_1^\top \mathbf{B}_1 - \alpha \mathbf{B}_2^\top \mathbf{B}_2))
\end{align}

Now, for ANIL, we start each iteration with $\mathbf{W} = \mathbf{1} \mathbf{w}^\top$.
Note that in this case, $\mathbf{W}_+ = \mathbf{W} - \alpha \mathbf{G}_{\mathbf{W}}(\mathbf{W},\mathbf{B}) $ is the matrix whose $i$-th row is $\mathbf{w} - \alpha \nabla_{\mathbf{w}}f_i(\mathbf{w}, \mathbf{B})$, which corresponds to the matrix of locally-updated heads.

We will repeatedly use the notation: $\mathbf{W} = \mathbf{U}_1 \mathbf{W}_1 + \mathbf{U}_2 \mathbf{W}_2$ and $\mathbf{W}_+ = \mathbf{U}_1 \mathbf{W}_{+,1} + \mathbf{U}_2 \mathbf{W}_{+,2}$.

There are two cases:

\textbf{Case 1:} $\mathbf{1} \in col(\mathbf{U}_1)$.

In this case, $\mathbf{W} = \mathbf{U}_1 \mathbf{s} \mathbf{w}^\top$ for some $\mathbf{s} \in \mathbb{R}^r$, so $\mathbf{W}_1 = \mathbf{s} \mathbf{w}^\top$ and $\mathbf{W}_2 = \mathbf{0}$. Thus
\begin{align}
    \mathbf{W}_+  &= \mathbf{U}_1(\mathbf{s} \mathbf{w}^\top(\mathbf{I} - \alpha \mathbf{B}_2^\top \mathbf{B}_2 ) ) -\alpha (\mathbf{s} \mathbf{w}^\top  \mathbf{B}_1^\top - \mathbf{D}) \mathbf{B}_1)  \\
     \mathbf{W}_{+,1}  &=\mathbf{s} \mathbf{w}^\top(\mathbf{I} - \alpha \mathbf{B}_1^\top \mathbf{B}_1  - \alpha \mathbf{B}_2^\top \mathbf{B}_2 ) ) +\alpha  \mathbf{D} \mathbf{B}_1 \\
     \mathbf{W}_{+,2}  &=\mathbf{0}
\end{align}
Then, the update for $\mathbf{B}$ is:
\begin{align}
    \mathbf{B} - \eta \mathbf{G}_{B}(\mathbf{W}_+, \mathbf{B}) &= \mathbf{V}_1 \left(\mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} - \eta \mathbf{W}_{+,2}\mathbf{W}_{+,2}^\top) +  \eta \mathbf{D}\mathbf{W}_{+,1} \right)  \nonumber \\
    &\quad + \mathbf{V}_2 \left(\mathbf{B}_2 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} - \eta \mathbf{W}_{+,2}\mathbf{W}_{+,2}^\top) \right)    \\
    &= \mathbf{V}_1 \left(\mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} ) +  \eta \mathbf{D}\mathbf{W}_{+,1} \right)  \nonumber \\
    &\quad + \mathbf{V}_2 \left(\mathbf{B}_2 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} ) \right) 
\end{align}
In order to gain in the signal direction and contract in the noise direction, we would like $\eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} \approx \mathbf{I}_k$. 
 We can see that if this holds exactly then we exactly recover the column space of $\mathbf{V}_1$, as desired.
However, $\mathbf{W}_{+,1}^\top\mathbf{W}_{+,1}$ is not full rank ($k$), which will slow down convergence.

% how does jiacheng avoid this? something unique to symmetric case?
% to do: 1. simulate 2. real exp new tasks 3. come back

Let $\mathbf{\Gamma} = \mathbf{I} - \alpha \mathbf{B}_1^\top \mathbf{B}_1  - \alpha \mathbf{B}_2^\top \mathbf{B}_2$.
Note that
\begin{align}
    \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} = \mathbf{\Gamma}^\top\mathbf{w} \mathbf{s}^\top \mathbf{s} \mathbf{w}^\top\mathbf{\Gamma} +\alpha^2  \mathbf{B}_1^\top \mathbf{D}^2 \mathbf{B}_1 +\alpha \mathbf{B}_1^\top \mathbf{D} \mathbf{s} \mathbf{w}^\top\mathbf{\Gamma}  + \alpha \mathbf{w} \mathbf{s}^\top \mathbf{D} \mathbf{B}_1 
\end{align}
We should be able to say that the rank-1 terms are small.

We may need a new notion of distance. Define $d_1 = \|\mathbf{B}_1\mathbf{B}_1^\top - \mathbf{D}^2\|_2$ and $d_2 = \|\mathbf{B}_2\mathbf{B}_2^\top\|_2$. If $d_1 = d_2 = 0$ then $\mathbf{B} = \mathbf{V}_1 \mathbf{R}$ for some rank-$r$ matrix $\mathbf{R}$, as desired. Note
\begin{align}
    \mathbf{B}_{+,1} &= \mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} ) +  \eta \mathbf{D}\mathbf{W}_{+,1} \nonumber \\
    \mathbf{B}_{+,2} &= \mathbf{B}_2 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})
\end{align}
Thus,
\begin{align}
    d_{1,+} &= \|\mathbf{B}_{+,1}\mathbf{B}_{+,1}^\top - \mathbf{D}^2\|_2  \nonumber \\
    &= \|\mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} )(\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} )\mathbf{B}_1^\top + \eta \mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})\mathbf{W}_{+,1}^\top \mathbf{D}\nonumber \\
    &\quad \quad  + \eta\mathbf{D}\mathbf{W}_{+,1}(\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})\mathbf{B}_1^\top + \eta^2 \mathbf{D}\mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top \mathbf{D}  - \mathbf{D}^2\|_2^2 \nonumber \\
    &= \|\mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} )(\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} )\mathbf{B}_1^\top + \eta \mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})\mathbf{W}_{+,1}^\top \mathbf{D}\nonumber \\
    &\quad \quad  + \eta\mathbf{D}\mathbf{W}_{+,1}(\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})\mathbf{B}_1^\top +  \mathbf{D}( \eta^2\mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top   - \mathbf{I}_r)\mathbf{D}\|_2 \nonumber \\
    % &= \|\mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} )(\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1} )\mathbf{B}_1^\top + \eta \mathbf{B}_1 (\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})\mathbf{W}_{+,1}^\top \mathbf{D}\nonumber \\
    % &\quad \quad  + \eta\mathbf{D}\mathbf{W}_{+,1}(\mathbf{I} - \eta \mathbf{W}_{+,1}^\top\mathbf{W}_{+,1})\mathbf{B}_1^\top +  \mathbf{D}( \eta^2\mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top   - \mathbf{I}_r)\mathbf{D}\|_2 \nonumber
\end{align}
Note that
\begin{align}
    \mathbf{B}_{+,1}\mathbf{B}_{+,1}^\top - \mathbf{D}^2 &= (\mathbf{B}_{1}\mathbf{B}_{1}^\top - \mathbf{D}^2) - \eta \mathbf{B}_{1} \mathbf{W}_{+,1}^\top (\mathbf{I} - \eta \mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top)\mathbf{W}_{+,1} \mathbf{B}_{1}^\top \nonumber \\
    &\quad + \eta \left(\mathbf{B}_{1} \mathbf{W}_{+,1}^\top (\mathbf{I} - \eta \mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top )\mathbf{W}_{+,1} \mathbf{B}_{1}^\top \right)^\top \nonumber \\
    &\quad + \eta \mathbf{B}_{1} \mathbf{W}_{+,1}^\top
    ( \mathbf{I} -\eta \mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top) \mathbf{D} +[\eta^2 \mathbf{D} \mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top \mathbf{D} - \eta \mathbf{B}_{1} \mathbf{W}_{+,1}^\top \mathbf{W}_{+,1} \mathbf{B}_{1}^\top] 
    %I + II \nonumber \\
    %\text{where } I &= 
\end{align}

The $(\mathbf{I}_k -\eta \mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top )$ terms should give us contraction (because $\mathbf{W}_{+,1}$ is rank-$k$) 
%, but the $[\eta^2 \mathbf{D} \mathbf{W}_{+,1}\mathbf{W}_{+,1}^\top \mathbf{D} - \eta \mathbf{B}_{+,1} \mathbf{W}_{+,1}^\top \mathbf{W}_{+,1} \mathbf{B}_{+,1}^\top] $ term will not (i think), so we will not have linear convergence.
% $(\mathbf{B}_{1}\mathbf{B}_{1}^\top - \mathbf{D}^2)$ and

% note for relu, need to show that we recover the nodes exactly up to scaling and permutation. PA dist doesn't matter.



\textbf{Case 2:} $\mathbf{1} \in col(\mathbf{U}_2)$. The conclusion is the same as Case 1, we omit the calculations for now.


\subsection{ReLU Activation}

\subsubsection{Population Case}

The update in $\mathbf{B}$ for ERM is:
\begin{align}
    \mathbf{B}_+ &= \mathbf{B} - \frac{\eta}{n} \sum_{i=1}^n \sum_{j=1}^m \left(
    \left(\mathbf{x}_j^\top \mathbf{B}\right)_+ \mathbf{w} - \mathbf{y}_{i,o}\right)\mathbf{x}_j \mathbf{1}_{\mathbf{x}_j \mathbf{B}> 0}(\mathbf{w}^\top)
\end{align}
The key difference for ANIL is that the heads are updated before the representation. Thus
\begin{align}
    \mathbf{B}_+ &= \mathbf{B} - \frac{\eta}{n} \sum_{i=1}^n \sum_{j=1}^m \left(
    \left(\mathbf{x}_j^\top \mathbf{B}\right)_+ \mathbf{w}_i - \mathbf{y}_{i,o}\right)\mathbf{x}_j \mathbf{1}_{\mathbf{x}_j \mathbf{B}> 0}(\mathbf{w}_i^\top)
\end{align}

Goal: Show that $\mathbf{B}_+$ for ANIL is closer to the true representation in some sense than for ERM.

Because the last layer is linear, can we say that a few steps of SGD solves the inner minimization almost exactly? Still, this doesn't prove that the algorithm reaches a global optima of FedRep objective.

Problem is that for ReLU, recovering the subspace spanned by the first layer is not sufficient to achieve the global minimum. Since $\mathbf{B} = \mathbf{B}_\ast \mathbf{R}$ may select a distinct set of data from $\mathbf{B} = \mathbf{B}_\ast$. We need to recover the columns (neurons) of $\mathbf{B}_\ast$ exactly up to permutation of the columns (but not rotation).

Results are still coming out now that show that GD or SGD recovers the neurons in single-task setting with overparameterization... our goal is to show that ANIL and FedRep do it in multitask setting, maybe without overparameterization
% but does this contradict experiments? no because there is not result showing that gd recovers rep in multitask setting


% Jin proof: cluster the neurons, then say average in each cluster is close to a teacher neuron



% \subsubsection{Population case}

% \subsection{Quadratic Activations}

Challenges: Unlike in the linear case, the sample complexity for single relu task is not well understood. Recent work requires $O(r^7 d^2)$ samples to learn all of the neurons in the hidden layer.

In the multitask setting, we can either show exact learning of the neurons, or that the loss goes to zero.



% We would like to show that there can be a 1/n factor in the error. 

Consider the simplest possible case. There are only two tasks, $k=r=1$, and we have access to the population loss. Then the question is, can Fedrep recover $\mathbf{b}_\ast$ by solving 
\begin{align}
    &\min_{\mathbf{b} \in \mathbb{R}^d, {w}_{1},w_2 \in \mathbb{R}} \mathbb{E}_{\mathbf{x}}[ (w_1(\mathbf{b}\mathbf{x})_+ - w_{1,\ast}(\mathbf{b}_\ast\mathbf{x})_+ )^2 + (w_2(\mathbf{b}\mathbf{x})_+ - w_{2,\ast}(\mathbf{b}_\ast\mathbf{x})_+ )^2 ] \\
    &\equiv \min_{\mathbf{b} \in \mathbb{R}^d} w_{1,\ast}\mathbb{E}_{\mathbf{x}}[ (a_1(\mathbf{b}\mathbf{x})_+ - (\mathbf{b}_\ast\mathbf{x})_+ )^2] + w_{2,\ast} \mathbb{E}_{\mathbf{x}}[ (a_2(\mathbf{b}\mathbf{x})_+ - (\mathbf{b}_\ast\mathbf{x})_+ )^2 ]
\end{align}
Note that $a_1, a_2$ are functions of $\mathbf{b}$. We care about maximizing $\langle\mathbf{b}, \mathbf{b}_\ast\rangle/\|\mathbf{b}\|_2$.

We need to show that learning the representation with two heads is somehow better than doing it with one.

% write gradient after update. how does <b,b*> change?


\textbf{Hermite basis approach}

Let's return to the basic FedRep setting. 

The ground-truth representation $\mathbf{B}_\ast \in \mathbb{R}^{d \times k}$ has $k$ neurons. We consider exact specification, and aim to learn $\mathbf{B} \in \mathbb{R}^{d \times k}$ close to the ground truth. We have heads in $\mathbf{W}, \mathbf{W}_\ast \in \mathbb{R}^{n \times k}$ as usual.
 
Consider the FedRep population loss function for two-layer ReLU with $\ell_2$ loss:
\begin{align}
    F(\mathbf{W}, \mathbf{B}) &= \frac{1}{2n}\sum_{i=1}^n \mathbb{E}_{\mathbf{x}_i} [(\mathbf{w}_i^\top (\mathbf{B}^\top \mathbf{x}_i)_+ - \mathbf{w}_{i,\ast}^\top (\mathbf{B}_{\ast}^\top \mathbf{x}_i)_+)^2] \nonumber 
\end{align}
By simple extension of Theorem 2.1 in GLM17 \url{https://arxiv.org/pdf/1711.00501.pdf}, this function is equal to the following infinite sum.
\begin{align}
    F(\mathbf{W}, \mathbf{B}) &= \frac{1}{2n} \sum_{s \in \mathbb{N}} \hat{\sigma}_s^2 \;\sum_{i=1}^n \left\| \sum_{l=1}^k w_{i,l} \mathbf{b}_{l}^{\otimes s} -  \sum_{l=1}^k w_{\ast,i,l} \mathbf{b}_{\ast,l}^{\otimes s} \right\|_F^2 %\\
    % &= \frac{1}{2n}\sum_{s \in \mathbb{N}} \hat{\sigma}_s^2 \left\|  \mathbf{W} \begin{bmatrix}\mathbf{b}_{1}^{\otimes s}\end{bmatrix} -   \mathbf{W}_{\ast} \mathbf{b}_{\ast,l}^{\otimes s} \right\|_F^2 \\
\end{align}
where $\hat{\sigma}_s^2$ is the $s$-th Hermite coefficient of the ReLU function. First note that this can be viewed as a sum of tensor decomposition problems. Also, note that the single-task version of this loss is:
\begin{align}
    F^1(\mathbf{W}, \mathbf{B}) &= \frac{1}{2} \sum_{s \in \mathbb{N}} \hat{\sigma}_s^2 \; \left\| \sum_{l=1}^k w_{l} \mathbf{b}_{l}^{\otimes s} -  \sum_{l=1}^k w_{\ast,l} \mathbf{b}_{\ast,l}^{\otimes s} \right\|_F^2 %\\
    % &= \frac{1}{2n}\sum_{s \in \mathbb{N}} \hat{\sigma}_s^2 \left\|  \mathbf{W} \begin{bmatrix}\mathbf{b}_{1}^{\otimes s}\end{bmatrix} -   \mathbf{W}_{\ast} \mathbf{b}_{\ast,l}^{\otimes s} \right\|_F^2 \\
\end{align} 
Numerous works have empirically observed that SGD on the finite-sample approximation of the single-task objective gets stuck in bad local minima (GLM17, GHJY17) hence the need for overparameterization (LMZ20) or using a complicated surrogate loss function (GLM17) in the single-task setting.

However, perhaps optimizing the FedRep objective in the multi-task setting with sufficient task diversity is another way to learn the representation. Suppose in the multitask setting, $n=k$ (this is for simplicity - $n>k$ is fine, we just need the heads to span $\mathbb{R}^k$) and each $\mathbf{w}_{\ast,i} = \mathbf{e}_i$ is a standard basis vector. Suppose also that we know the optimal heads. Then the multitask problem reduces to 
\begin{align}
    F(\mathbf{W}, \mathbf{B}) &= \frac{1}{2n} \sum_{s \in \mathbb{N}} \hat{\sigma}_s^2 \;\sum_{i=1}^k \left\|  \mathbf{b}_{i}^{\otimes s} -   \mathbf{T}_i^s \right\|_F^2 \nonumber \\
    &= a_1 \|\mathbf{B} - \mathbf{B}^\ast\|_F^2 + a_4\sum_{i=1}^k\|\mathbf{b}_i^{\otimes 4}- \mathbf{b}_{\ast,i}^{\otimes 4}\|_F^2 + a_6\sum_{i=1}^k\|\mathbf{b}_i^{\otimes 6}- \mathbf{b}_{\ast,i}^{\otimes 6}\|_F^2 + ... %\\
    % &= \frac{1}{2n}\sum_{s \in \mathbb{N}} \hat{\sigma}_s^2 \left\|  \mathbf{W} \begin{bmatrix}\mathbf{b}_{1}^{\otimes s}\end{bmatrix} -   \mathbf{W}_{\ast} \mathbf{b}_{\ast,l}^{\otimes s} \right\|_F^2 \\
\end{align}
which is the sum of {\em rank-1} tensor decomposition problems, where $\mathbf{T}_i^s \coloneqq \mathbf{b}_{\ast,i}^{\otimes s}$. It is well known that rank-one tensor decomposition has a well-behaved optimization landscape (GHJY17,FJK96). Here there is coupling across the rank-1 decomposition problems, which complicates things. 
% In particular, the gradient $\nabla_{\mathbf{B}} F(\mathbf{W}_\ast, \mathbf{B})$ in this case is 
% \begin{align}
%     \nabla_{\mathbf{B}} F(\mathbf{W}_\ast, \mathbf{B}) &= c_1 (\mathbf{B} - \mathbf{B}^\ast) + %c_4\sum_{i=1}^k\|\mathbf{b}_i^{\otimes 4}- \mathbf{b}_{\ast,i}^{\otimes 4}\|_F^2 + c_6\sum_{i=1}^k\|\mathbf{b}_i^{\otimes 6}- \mathbf{b}_{\ast,i}^{\otimes 6}\|_F^2 + ...
% \end{align}

Another complication is that we do not exactly have  $\mathbf{w}_{\ast,i} = \mathbf{e}_i$, instead we view the sum of tensors in a non-standard basis. But we still have views that span $\mathbb{R}^{k}$, so the conclusion should be the same. 

On the other hand, note that we cannot reduce the single task problem to the sum of rank-1 tensor decompositions (the tensor decompositions are of the form $ \left\| \sum_{l=1}^k w_{l} \mathbf{b}_{l}^{\otimes s} -  \mathbf{T}^{s'} \right\|_F^2$ instead of $\sum_{i=1}^n \left\| \sum_{l=1}^k w_{i,l} \mathbf{b}_{l}^{\otimes s} -  w_{\ast,i,l}\mathbf{T}_i^{s'} \right\|_F^2$). And for rank-2 or greater tensor decomposition problems, it is not known whether the objective satisfies the strict saddle property, and GD empirically does not converge to the ground truth (GHJY17).

% Simulations verify that GD reaches a local min in the single task case, and linearly converges to the ground truth in the multi-task case.

We know that the problem $\min_{\mathbf{b}_1,...,\mathbf{b}_k \in \mathbb{R}^d}\|\sum_{l =1}^k \mathbf{b}_l^{\otimes s} - \mathbf{T}\|_2^F$, where $\mathbf{T} = \sum_{l =1}^k \mathbf{b}_{\ast,l}^{\otimes s}$ is hard for any $s \geq 3$ and $k \gg d$ [Mondelli, Montanari 2019] It is solvable for the ground-truth having linearly independent components (thus $k\ll d^{3/2}$) [Ma et al. 2016], but as far as I know, we do not know whether GD can solve it.

Path for analysis:
\begin{enumerate}
    \item Assume that we know the optimal heads and they are standard basis vectors. Show that gradient descent wrt $\mathbf{B}$ on the population loss recovers $\mathbf{B}_\ast$.
    \item Assume that we know the optimal heads and they are  arbitrary basis vectors of $\mathbb{R}^k$. Show that gradient descent wrt $\mathbf{B}$ on the population loss recovers $\mathbf{B}_\ast$ up to permutation of the columns.
    \item Now we do not know the optimal heads. Show that solving least squares minimization problem recovers the true heads up to the current error in $\mathbf{B}$. Show that this is good enough for convergence in $\mathbf{B}$.
    \begin{itemize}
        \item Hard because we have an infinite sum. When solving the least squares problem, we will have to take the inverse of an infinite sum of matrices. I think we need to show that some terms are dominant.
    \end{itemize}
    \item Show that FedRep recovers the ground-truth neurons $\mathbf{b}_{\ast,i}$ (i.e. for every $\mathbf{b}_{\ast,i}$, there is at least one $\mathbf{b}_{i'}$ s.t. $\|\mathbf{b}_{\ast,i} - \mathbf{b}_{i'}\|_2 \leq \epsilon$.
\end{enumerate}
% Again recall the three questions we are trying to answer:

% (1) Can AltMinGD/AltGDGD solve the FedRep objective for nonlinear neural nets? (2) How close is ANIL to AltMinGD/AltGDGD? (3) Which of these methods is the best?

More general approach: extend single-neuron gd analysis to k larger than 1.

Key to single neuron analysis [Yehudai and Shamir 2020]: showing that population gradient is always correlated with the direction from the ground truth to the current iterate.
Thus GD always moves towards the ground truth. In particular, they show that in the single neuron, single task, one-layer case (i.e. ${w} = {w}_\ast = 1$), the population gradient $\nabla F(\mathbf{b})$ satisfies
\begin{align}
    \left\langle \nabla F(\mathbf{b}), \mathbf{b}- \mathbf{b}_\ast \right\rangle = \mathbb{E}_{\mathbf{x}}[ (\sigma(\mathbf{b}^\top \mathbf{x}) - \sigma(\mathbf{b}_\ast^\top \mathbf{x}) )\sigma'(\mathbf{b}_\ast^\top \mathbf{x}) (\mathbf{b}^\top\mathbf{x} - \mathbf{b}_\ast^\top\mathbf{x})] \geq c > 0
\end{align}
for any monotonically non-decreasing activation function $\sigma$ (including ReLU) and some number $c > 0$. Note that the monotonic non-decreasing property of $\sigma$ means that the random variable inside the expectation is almost surely non-negative, which is key to the proof.

This argument breaks down in the two-neuron case because the gradient $\nabla_{\mathbf{b}_1} F(\mathbf{B})$ includes terms with $\mathbf{b}_2$, thus we can no longer use the monotonically non-decreasing property to say $\left\langle  \nabla_{\mathbf{b}_1} \hat{F}(\mathbf{B}; \mathbf{x}), \mathbf{b}_1 - \mathbf{b}_{1,\ast}\right\rangle \geq 0 $ for all $\mathbf{x}$. However, if we have multiple tasks with different heads (assume for now that we know the optimal heads) this gives us two different ``views'' of the first-layer neurons. Can we therefore reduce the two-task, two-neuron, two-layer case to the single-task, single-neuron, single-layer case?



\subsection{Goal theorems}

\begin{assumption}
The tasks are rank-$r$ diverse.
\end{assumption}

\begin{theorem}
In the exactly-specified linear and ReLU cases, ANIL exactly recovers the column space of the true representation in terms of principal angle distance for sufficient initialization, samples/task, and iterations. 
\end{theorem}


\begin{theorem}
In the over-specified linear case, ANIL recovers the column space of the true representation in terms of some reasonable notion of distance between subspaces of different dimensions (e.g. the subspace learned by ANIL contains the true, lower-dimensional subspace) up to error depending on the $r$, $k$, $d$, $\kappa$, the initialization, the number of tasks, samples/task, and iterations. 
\end{theorem}

Then, we can adapt the result from Du et al. 2020 Section 6 to say something like
\begin{theorem}
Recovering this subspace reduces the sample complexity for a new task by a factor of $\Omega(k/d)$ compared to learning the network using only the samples from the new task.
\end{theorem}

ReLU case: learning the subspace does not necessarily help (easy counterexamples). We need to recover the directions of the neurons themselves. Or, we stay at a higher level and only care about reducing the excess risk. We ultimately need to show that GD for ERM objective has large error on new task, whereas ANIL does not.
% make sure sims are working
% 


Finally,
\begin{theorem}
Lower bound on representation learning error without rank-$r$ task diversity.
\end{theorem}

\begin{theorem}
Lower bound on representation learning error for ERM in exactly specified case.
\end{theorem}

\subsection{Simulations}

2 orthogonal training tasks, models evaluated using ANIL procedure on new tasks from the same subspace, given 20 samples to fine-tune the head before excess risk is calculated.

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{lin_exactd10.pdf}}
\vspace{-0mm}
\caption{Linear exactly specified, d = 10, k = r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{lin_exactd20.pdf}}
\vspace{-0mm}
\caption{Linear exactly specified, d = 20, k = r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{lin_overd10.pdf}}
\vspace{-0mm}
\caption{Linear over specified, d = 10, k = 5, r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{lin_overd20.pdf}}
\vspace{-0mm}
\caption{Linear over specified, d = 20, k = 5, r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}


\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{relu_exactd10.pdf}}
\vspace{-0mm}
\caption{ReLU exactly specified, d = 10, k = r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{relu_exactd20.pdf}}
\vspace{-0mm}
\caption{ReLU exactly specified, d = 20, k = r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{relu_overd10.pdf}}
\vspace{-0mm}
\caption{ReLU over specified, d = 10, k = 5, r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}

\begin{figure}[H]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.58\columnwidth]{relu_overd20.pdf}}
\vspace{-0mm}
\caption{ReLU over specified, d = 20, k = 5, r = 2}
\label{fig:relu1}
\end{center}
\vspace{-0mm}
\end{figure}





\newpage

\section{Big Picture Thoughts}
Observation: recent work has shown that solving 
\begin{align}
    F_{FedRep}^\ast \coloneqq \min_{\mathbf{g} \in \mathcal{G}} F_{FedRep}(\mathbf{g}) \coloneqq \sum_{i =1}^n   f_i (\mathbf{h}_i \circ \mathbf{g}) \quad \text{ where } \quad \mathbf{h}_i \in \arg \min_{\mathbf{h}_i \in \mathcal{H}} f_i (\mathbf{h}_i \circ \mathbf{g}) \label{fedrep_obj1}
\end{align}
learns a representation $\mathbf{g}_{FedRep}$ that transfers well to new tasks (TJJ2020, TJJ2020, Du et al 2020, but besides our FedRep paper, there have not been results on how to solve this). Instead, ANIL solves:
\begin{align}
    F_{ANIL}^\ast \coloneqq \min_{\mathbf{g} \in \mathcal{G}}F_{ANIL}(\mathbf{g}) \coloneqq \min_{\mathbf{h} \in \mathcal{H}} \sum_{i =1}^n   f_i (\mathbf{\hat{h}}_i \circ \mathbf{g}) \quad \text{ where } \quad \mathbf{\hat{h}}_i \in \arg \min_{\mathbf{h}_i \in \mathcal{N}(\mathbf{h})} f_i (\mathbf{h} \circ \mathbf{g}) + (\mathbf{h}_i - \mathbf{h})^\top \nabla_{\mathbf{h}} f_i(\mathbf{h} \circ \mathbf{g}) 
\end{align}
Let $\mathbf{g}_{ANIL}$ denote a global minimizer.
Let $\hat{f}_i(\mathbf{h}_i, \mathbf{h} \circ \mathbf{g})\coloneqq f_i (\mathbf{h} \circ \mathbf{g}) + (\mathbf{h}_i - \mathbf{h})^\top \nabla_{\mathbf{h}} f_i(\mathbf{h} \circ \mathbf{g})$.

Two questions:
\begin{enumerate}
    \item Are the global optima of these objectives close?
    \begin{enumerate} \item Clearly, $F_{FedRep} \leq F_{ANIL}$, and further $F_{FedRep}(\mathbf{g}) \leq F_{ANIL}(\mathbf{g})$ for all $\mathbf{g}$.
        \item We can use the safe assumptions that each $f_i(\cdot, \mathbf{g})$ is convex, $M$-Lipschitz and  $L$-smooth, and we can further assume $\mu$-strongly convex by adding weight decay. So we can closely control the distance $\mathbf{\hat{h}}_i - \mathbf{h}_i$ and the corresponding function values.
        \item Still, the optimal solutions for $\mathbf{g}$ may be very different in general. Example: consider two representations $\mathbf{g}_1$,  $\mathbf{g}_2$. For fixed $\mathbf{g}_1$, the loss landscape over $\mathcal{H}$ is well behaved, i.e. all the corresponding optimal $\mathbf{h}_i$ are close to each other, so taking one step GD for the heads is roughly equivalent to minimization. Meanwhile, for fixed $\mathbf{g}_2$, the optimal heads are far apart (cannot be reached with one step of GD), yet their corresponding function values are smaller than in the first case. So FedRep chooses $\mathbf{g}_2$ while ANIL chooses  $\mathbf{g}_1$, which may be very different representations.
        \item In order to make a general argument, can we make an assumption that implies this never happens, and show that this assumption holds for many realistic settings? In particular, can we show that under mild assumptions, \textit{all optimal representations in \eqref{fedrep_obj1} are such that the corresponding optimal heads can be reached \textbf{in a small number} of steps of SGD?}
        \item This implies that all global optima of FedRep are global optima of ANIL. By (a), this implies that the global optima of FedRep and ANIL are equivalent. (because we already have $F_{FedRep}^\ast \approx F_{ANIL}^\ast$, so if ANIL had a global optimum $\mathbf{g}^\ast$ that was not also a global optimum for FedRep,  we would have $F_{FedRep}(\mathbf{g}^\ast) > F_{ANIL}(\mathbf{g}^\ast) $, a contradiction).  
        So if we can show (c), then all we need to show is that ANIL reaches a global optimum.
        \item This seems to contradict our need for diverse tasks. However, we need diverse tasks within some {\em low dimensional space}... so the point is that the optimal $\mathbf{g}$'s should be (effectively) low-dimensional...
        \item Of course, the task solutions existing in a low-dimensional space also makes them close in the sense that only a small number of samples are needed to find them.
        \item Note that for fixed number of samples, larger dimension increases the variance of the stochastic gradient, and thereby makes SGD slower.
        \item Summary: if optimal representation for FedRep is such that the corresponding optimal heads can be reached in a few steps of SGD (e.g. if the optimal representation is low-dimensional), then the optimal representations for FedRep and ANIL agree.
        \item It remains to show that ANIL reaches a global optimum for certain settings.
        %(reaching a global min of ANIL means it has learned the FedRep optimal representation, which recent works have shown reduces sample complexity for a new task, which again (circular) implies that these reps are optimal for ANIL).
        % implies that all global optima of fedrep are global optima of anil
        % Assume $f_i(\cdot, \mathbf{g})$ is $L$-smooth, then \begin{align}f_i (\mathbf{\hat{h}}_i \circ \mathbf{g}) &\leq  f_i (\mathbf{h} \circ \mathbf{g}) + (\mathbf{\hat{h}}_i - \mathbf{h})^\top \nabla_{\mathbf{h}} f_i(\mathbf{h} \circ \mathbf{g}) + \frac{L}{2}\|\mathbf{\hat{h}}_i - \mathbf{h}\|_2^2 \\
        % &= \end{align} for any $\mathbf{\hat{h}}_i$. 
    \end{enumerate}
    \item Which objective is easier to optimize?
    \begin{enumerate}
        \item In the two-layer linear case with exact specification, we roughly know that GD on both objectives converges linearly with optimal sample complexity (up to log factors) (we haven't worked out all of the details for ANIL, but we see that this will be the case).
        \item Over-specified linear case?
        \item Non-linear cases?
    \end{enumerate}
\end{enumerate}
% can it be possible to have a much different rep that performs worse on F1 but better on F2



\newpage




\newpage

--------

\newpage


Choose 
$$ \beta = \lambda_{\max} \left(\alpha\left(\alpha \mathbf{B}_{t}\mathbf{B}_t^\top \mathbf{\hat{\Sigma}} - \mathbf{I}_d \right)   \mathbf{B}_\ast  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top \mathbf{\hat{\Sigma}} \right)$$. 
We have
\begin{align}
   \left\|  \mathbf{I}_d -  \left(\alpha \mathbf{B}_{t}\mathbf{B}_t^\top \mathbf{\hat{\Sigma}} - \mathbf{I}_d \right) \beta \alpha \mathbf{B}_\ast  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top \mathbf{\hat{\Sigma}}  \right\|_2 &\leq  1- 
\end{align}
we cannot use the Weyl inequality because non-symmetric

% now compute distance? need other func. need dependence on beta. relate to simpler case

Then
\begin{align}
    \|\mathbf{B}_{t+1}\|_2 &\leq  \|\mathbf{B}_t\|_2\left\|  \mathbf{I}_d -  \beta \alpha^2 \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\right\| +  \beta \alpha\left\| \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\right\|_2 \nonumber \\
&\leq 1 -\frac{1}{\kappa\left( \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t \right)} + \frac{\left\| \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\right\|_2}{\alpha\| \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\|_2} \nonumber \\
% &= 1 -\frac{1}{\kappa\left( \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
% i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t \right)} + \frac{\left\| \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \right\|_2}{\alpha\| \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
% i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\|_2} \nonumber \\
\end{align}
Note that
\begin{align}
    \left\| \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\right\|_2 &= \left\|  \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top\right)^{1/2}\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\right\|_2^2 \nonumber \\
&\geq \sigma_{\min} \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top \right)\left\|  \mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\right\|_2^2 
\end{align}
Thus, assuming $\kappa\left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
i} \mathbf{w}_{\ast,i}^\top \right) = 1$, we have
\begin{align}
    \|\mathbf{B}_{t+1}\|_2 &\leq 1 -\frac{1}{\kappa\left( \mathbf{B}_t^\top \mathbf{\hat{\Sigma}}\mathbf{B}_\ast \left(\frac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,
 i} \mathbf{w}_{\ast,i}^\top\right)\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t \right)} + \frac{1}{\alpha\|\mathbf{B}_\ast^\top\mathbf{\hat{\Sigma}} \mathbf{B}_t\|_2}
\end{align}

Two-layer linear, over-specified:

We first start with the population case. 


==> w_bounds.tex <==







Let $a_s \coloneqq \|\mathbf{w}_s\|_2$ for all $s\in\{0,\dots,t\!+\!1\}$. Note that $\bigcup_{s=0}^t A_3(s)$ implies $\sigma_{\max}(\mathbf{B}_s^\top \mathbf{B}_s) \leq \frac{1+\tau_2}{\alpha}< \frac{2}{\alpha}$ for all $s\in\{0,\dots,t\!+\!1\}$. Using this fact with \eqref{uuu}, we obtain
\begin{align}
    a_{s+1} &\leq (1 + \tfrac{2\beta}{\alpha} \|\mathbf{I}_k - \alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2 )a_s + \tfrac{2\beta}{\sqrt{\alpha}} \|\mathbf{I}_k - \alpha \mathbf{B}_s^\top \mathbf{B}_s\|_2 L_\ast \
    \label{forall}
\end{align}  
for all $s\in\{0,\dots,t\}$.
Next, let $\gamma \coloneqq 
   1 - \beta \alpha E_0 \mu_\ast^2 + c \tfrac{\beta^3}{\alpha}\kappa_\ast^8 \eta_{\ast}^2\tau_2 + c\beta^2 \kappa_\ast^4 \eta_{\ast}^2 + c \beta^2 \alpha^2 \tau_2 L_\ast^4$. By $\bigcup_{s=0}^t A_2(s)$, we have
\begin{align}
    \|\mathbf{I}-\alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1}\|_2 &\leq \gamma\|\mathbf{I}-\alpha \mathbf{B}_{t}^\top \mathbf{B}_{t}\|_2 + 10 \alpha^{2}\beta^2 L_\ast^4 \dist_t^2 \nonumber \\
    &\leq \gamma^2\|\mathbf{I}-\alpha \mathbf{B}_{t-1}^\top \mathbf{B}_{t-1}\|_2 + 10\alpha^{2}\beta^2\gamma \dist_{t-1}^2 +  10\alpha^{2}\beta^2 \dist_t^2 \nonumber \\
    &\;\;\vdots \nonumber \\
    &\leq  \gamma^{t+1}\|\mathbf{I}-\alpha \mathbf{B}_{0}^\top \mathbf{B}_{0}\|_2 + 10 \alpha^{2}\beta^2 L_\ast^4  \sum_{s=0}^t \gamma^{t-s} \dist_s^2  \nonumber \\
    &= 10\alpha^{2}\beta^2 L_\ast^4  \sum_{s=0}^t \gamma^{t-s} \dist_s^2
    % \nonumber \\
    % &\leq \sum_{s=1}^t \gamma^{t-s} \rho^s \nonumber \\
    % &= \gamma^t \sum_{s=1}^t \left(\frac{\rho}{\gamma}\right)^s \nonumber \\
    % &=: z_t
\end{align}
since $\|\mathbf{I}-\alpha \mathbf{B}_{0}^\top \mathbf{B}_{0}\|_2 = 0$ by choice of initialization.
Now, let $\rho\coloneqq 1  - \beta \left(0.5 \alpha E_0 \mu_\ast^2 - 3  \tau_2 \sqrt{\tau_1 \alpha} \eta_\ast  \right) $. We have that $\dist_s \leq \rho^s$ for all $s\in \{0,...,t\}$ by $\bigcup_{s=0}^t A_5(s)$. 
% We also have $\gamma \leq \rho$ by choice of $\alpha,\lambda$.
Let $q\coloneqq \max(\gamma, \rho)$.
% {\color{red} deal with min gamma rho}
Thus, for any $s\in \{0,...,t\}$, we have
\begin{align}
    \|\mathbf{I}-\alpha \mathbf{B}_{s+1}^\top \mathbf{B}_{s+1}\|_2 &\leq 10 \alpha^{2}\beta^2 L_\ast^4 \sum_{r=0}^s \gamma^{s-r} \rho^{2r} \nonumber \\
    &\leq 10 \alpha^{2}\beta^2L_\ast^4  \sum_{r=0}^s q^{s-r} q^{2r} \nonumber \\
    &= 10 \alpha^{2}\beta^2 L_\ast^4  q^s \sum_{r=0}^s q^r \nonumber \\
    &\leq  q^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1-q} \nonumber \\
    &=: {z}_s
\end{align}
% Now, suppose that $\|\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\|_2 \leq L_\ast$ for all $t$ with high probability. Let $a_t \coloneqq \|\mathbf{w}_t\|_2$ for all $t$.
Now, applying \eqref{forall} recursively for $s=t,t-1,\dots,0$ and plugging in the definition of $z_s$ yields
\begin{align}
    a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
    &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} {z}_{t-1})(1 + \tfrac{2\beta}{\alpha} {z}_t) + \tfrac{2\beta}{\sqrt{\alpha}} {z}_{t-1} L_\ast(1 + \tfrac{2\beta}{\alpha} {z}_t)  + \tfrac{2\beta}{\sqrt{\alpha}} {z}_t L_\ast \nonumber \\
    &\;\; \vdots \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t {z}_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
    &=  \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t z_s\prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}z_r) \nonumber \\
    &= \tfrac{2\beta}{\sqrt{\alpha}} L_\ast \sum_{s=1}^t q^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1- q}\prod_{r=s+1}^t(1+ q^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1- q}) \nonumber \\
    &= \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast \sum_{s=0}^t q^{s} \prod_{r=s+1}^t\left(1+ q^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - q}\right) \nonumber
\end{align}    
where the first equality follows under the assumption that $a_0 = 0$. By the AM-GM inequality and sum of geometric series, we have, for $s\leq t-1$,
\begin{align}
    \prod_{r=s+1}^t\left(1+ q^{r} \tfrac{{20\alpha}\beta^3 L_\ast^4 }{1 - q}\right) &\leq \left(1 + \tfrac{1}{t-s} \sum_{r=s+1}^t q^{r} \tfrac{{20\alpha}\beta^3L_\ast^4 }{1 - q}\right)^{t-s} \nonumber \\
    &\leq \left(1 + \tfrac{20}{t-s} \tfrac{{\alpha}\beta^3q^{s+1}L_\ast^4 }{(1- q)^2} \right)^{t-s} 
\end{align}
The RHS is monotonically increasing in $t$ (since each additional $t$ means multiplication by a number greater than 1) so we can upper bound it by its limit as $t \rightarrow \infty$. This limit is
$\exp\left( {20} \tfrac{{\alpha}\beta^3q^{s+1}}{(1- q)^2} \right)$ (note that it is of the form $\lim_{x \rightarrow \infty} (1+\tfrac{a}{x})^x = a$). Note that $q = 1 - \Omega(\beta \alpha \mu_{\ast}^2)$ for sufficiently small $\beta,\alpha$, 
% {\color{red} (since $\tau_2 = $}), 
thus $1-q \leq c\beta \alpha \mu_{\ast}^2$.
As a result, to ensure $\exp\left( {20} \tfrac{{\alpha}\beta^3q^{s+1}}{(1- q)^2} \right)\leq 1$, we can choose
\begin{align}
  {20\alpha}\beta^3 L_\ast^4  &\leq   (1- q)^2 \nonumber \\
  \iff {20\alpha}\beta^3 L_\ast^4 &\leq  c \alpha^2 \beta^2\mu_{\ast}^4 \nonumber \\
  \iff \beta &\leq c' \frac{\alpha \mu_{\ast}^4}{L_\ast^4}. \label{betac1}
\end{align}
Under this condition on $\beta$, we have
\begin{align}
    a_{t+1} &\leq \tfrac{20 \alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast\sum_{s=1}^{t-1} q^{s} \exp\left( {20} \tfrac{{\alpha}\beta^3q^{s+1}L_\ast^4 }{(1- q)^2} \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast q^{t} \nonumber \\
    &\leq \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast\sum_{s=1}^{t-1} q^{s}\left( 1+ {40} \tfrac{{\alpha}\beta^3q^{s+1}L_\ast^4 }{(1- q)^2}  \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast q^{t} \label{usenum}\\
    &\leq \tfrac{20\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast \sum_{s=1}^{t-1} q^{s}\left( 1+ 2q^{s+1}  \right) + \tfrac{20\alpha^{1.5}\beta^3L_\ast^4 }{1 - q} L_\ast q^{t} \label{usebeta}\\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{1 - q} L_\ast\sum_{s=1}^{t} q^{s} \nonumber \\
    &\leq \tfrac{60\alpha^{1.5}\beta^3 L_\ast^4 }{(1 - q)^2} L_\ast \nonumber \\
    &\leq c \frac{\beta}{\sqrt{\alpha}}\kappa_\ast^4 \eta_\ast \nonumber
    % &\leq \sqrt{\alpha}
    % &\leq \tfrac{\alpha\beta^3}{\gamma - q^2} c \exp\left( \tfrac{1}{t-s} \tfrac{\sqrt{\alpha}\beta^3}{(1- q)^2} \right)\sum_{s=1}^t \gamma^{s+1}  \nonumber \\
    % &\leq \tfrac{\alpha\beta^3}{\gamma - q^2} c \exp\left( \tfrac{\alpha\beta^3}{\gamma - q^2}\tfrac{\gamma^{2}}{1- \gamma}\right)\tfrac{\gamma^2}{1-\gamma} 
\end{align} 
where \eqref{usenum} follows from the numerical inequality $e^x \leq 1+2x$ for $x\in [0,1]$ and \eqref{usebeta} follows from the condition on $\beta$ in \eqref{betac1}.






\begin{align}
    a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_t \eta_\ast + \xi'' \nonumber \\
    &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} \zeta_{t-1})(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_{t-1} \eta_\ast(1 + \tfrac{2\beta}{\alpha} \zeta_t)  + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_t L_\ast + \xi''(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \xi'' \nonumber \\
    &\;\; \vdots \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) + \xi'' \sum_{s=1}^t \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) \nonumber \\
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) + \xi'' \sum_{s=1}^t \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) \nonumber \\
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s (1+ \tfrac{1}{t-s-1}\sum_{r=s+1}^t\tfrac{2\beta}{\alpha}\zeta_r)^{t-s-1} + \xi'' \sum_{s=1}^t (1+ \tfrac{1}{t-s-1}\sum_{r=s+1}^t\tfrac{2\beta}{\alpha}\zeta_r)^{t-s-1} \nonumber \\
    &\leq  \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s (1+ \tfrac{1}{t-s-1}\frac{20\beta \rho^{s+1}L_{\ast}^4}{\alpha} + {\beta}^2 L_{\ast}^4 \xi' + \frac{1}{\alpha^2} \xi)^{t-s-1} \nonumber \\
    &\quad + \xi'' \sum_{s=1}^t (1+ \tfrac{1}{t-s-1}\frac{20\beta \rho^{s+1}L_{\ast}^4}{\alpha} + {\beta}^2 L_{\ast}^4 \xi' + \frac{1}{\alpha^2} \xi)^{t-s-1}   \nonumber \\
   &\leq  \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s  \exp\left(\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi'' \sum_{s=1}^t \exp\left(\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)  \nonumber \\ 
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s  \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi'' \sum_{s=1}^t \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)  \nonumber \\ 
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \left( \rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1-\rho}  + (20\alpha^{2}\beta^2 L_\ast^4 \xi'+\xi) \frac{1}{1-\gamma} \right) \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi''  \left(t +\frac{20 L_{\ast}^4}{\alpha^2} +t^2\beta^2 L_\ast^4 \xi' + \tfrac{t^2}{\alpha^2}\xi \right)  \nonumber
\end{align}   


\begin{align}
    a_{t+1} &\leq a_t(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_t \eta_\ast + \xi'' \nonumber \\
    &\leq a_{t-1}(1 + \tfrac{2\beta}{\alpha} \zeta_{t-1})(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_{t-1} \eta_\ast(1 + \tfrac{2\beta}{\alpha} \zeta_t)  + \tfrac{2\beta}{\sqrt{\alpha}} \zeta_t L_\ast + \xi''(1 + \tfrac{2\beta}{\alpha} \zeta_t) + \xi'' \nonumber \\
    &\;\; \vdots \nonumber \\
    &\leq a_0\prod_{s=1}^t(1+\tfrac{2\beta}{\alpha}{z}_s) +\tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) + \xi'' \sum_{s=1}^t \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) \nonumber \\
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) + \xi'' \sum_{s=1}^t \prod_{r=s+1}^t(1+ \tfrac{2\beta}{\alpha}\zeta_r) \nonumber \\
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s (1+ \tfrac{1}{t-s-1}\sum_{r=s+1}^t\tfrac{2\beta}{\alpha}\zeta_r)^{t-s-1} + \xi'' \sum_{s=1}^t (1+ \tfrac{1}{t-s-1}\sum_{r=s+1}^t\tfrac{2\beta}{\alpha}\zeta_r)^{t-s-1} \nonumber \\
    &\leq  \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s (1+ \tfrac{1}{t-s-1}\frac{20\beta \rho^{s+1}L_{\ast}^4}{\alpha} + {\beta}^2 L_{\ast}^4 \xi' + \frac{1}{\alpha^2} \xi)^{t-s-1} \nonumber \\
    &\quad + \xi'' \sum_{s=1}^t (1+ \tfrac{1}{t-s-1}\frac{20\beta \rho^{s+1}L_{\ast}^4}{\alpha} + {\beta}^2 L_{\ast}^4 \xi' + \frac{1}{\alpha^2} \xi)^{t-s-1}   \nonumber \\
   &\leq  \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s  \exp\left(\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi'' \sum_{s=1}^t \exp\left(\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)  \nonumber \\ 
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \zeta_s  \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi'' \sum_{s=1}^t \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)  \nonumber \\ 
    &\leq \tfrac{2\beta}{\sqrt{\alpha}} \eta_\ast \sum_{s=1}^t \left( \rho^{s} \tfrac{10\alpha^{2}\beta^2 L_\ast^4 }{1-\rho}  + (20\alpha^{2}\beta^2 L_\ast^4 \xi'+\xi) \frac{1}{1-\gamma} \right) \left(1+\frac{20\beta \rho^{s+1} L_{\ast}^4}{\alpha} +t\beta^2 L_\ast^4 \xi' + \tfrac{t}{\alpha^2}\xi \right)\nonumber \\
    &\quad + \xi''  \left(t +\frac{20 L_{\ast}^4}{\alpha^2} +t^2\beta^2 L_\ast^4 \xi' + \tfrac{t^2}{\alpha^2}\xi \right)  \nonumber %\\ 
\end{align}   









-------------

Old exact maml:



----

From this, we can say that:
\begin{align}
    \|\mathbf{w}_{t+1}\|_2 &\leq \|\mathbf{w}_t\|_2 + \beta \alpha^{3.5} L^{5} + \beta \alpha^{5.5} L^{7} + \beta \alpha^{3.5} L^5 + \beta \alpha^{1.5} L^3 \dist_t^2  + \beta \alpha^{3.5} L^5 \dist_t^2 +\beta \alpha^{5.5}L^7 + \beta \alpha^{3.5}L^5 
\end{align}
There is one term that ruins it: the $\alpha^{1.5}$ term, namely:
\begin{align}
    \alpha^2 \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \deld_t \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}
\end{align}
Need to assume: $\dist_0^2 \leq \frac{\mu_\ast^3}{L_\ast^3}$




By applying the chain rule, we find that the the gradients of $F_{t,i}(\mathbf{B}_{t}, \mathbf{w}_{t})$ with respect to $\mathbf{w}$ and $\mathbf{B}$ are given as follows:
\begin{align}
    \nabla_\mathbf{w}F_{t,i}(\mathbf{B}_{t}, \mathbf{w}_{t}) &= \del_t \lam_t \mathbf{B}_t^\top \mathbf{v}_{t,i} - \alpha (\mathbf{B}_t^\top \mathbf{v}_{t,i}\mathbf{w}_t^\top\del_t + \del_t\mathbf{w}_t \mathbf{v}_{t,i}^\top \mathbf{B}_t) \mathbf{w}_t \nonumber \\
    &\quad + 2\alpha (\mathbf{w}_{\ast,i}^\top \mathbf{B}_{\ast}^\top \mathbf{v}_{t,i})\del_t \mathbf{w}_{t} -\alpha^2 \mathbf{B}_t^\top( \mathbf{v}_{t,i} \mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top  +  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{v}_{t,i}^\top)\mathbf{B}_t\mathbf{w}_t  + \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{v}_{t,i}^\top  \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \nonumber \\
    &= \del_t  \mathbf{B}_t^\top \mathbf{v}_{t,i} - \alpha \del_t \mathbf{w}_t\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{v}_{t,i} - \alpha (\mathbf{B}_t^\top \mathbf{v}_{t,i}\mathbf{w}_t^\top\del_t + \del_t\mathbf{w}_t \mathbf{v}_{t,i}^\top \mathbf{B}_t) \mathbf{w}_t \nonumber \\
    &\quad + 2\alpha (\mathbf{w}_{\ast,i}^\top \mathbf{B}_{\ast}^\top \mathbf{v}_{t,i})\del_t \mathbf{w}_{t} -\alpha^2 \mathbf{B}_t^\top( \mathbf{v}_{t,i} \mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top  +  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{v}_{t,i}^\top)\mathbf{B}_t\mathbf{w}_t  + \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i}  \nonumber  \\
    &= \del_t  \mathbf{B}_t^\top \mathbf{v}_{t,i} - \mathbf{e}_{1,t,i} - \mathbf{e}_{2,t,i}  + \mathbf{e}_{3,t,i} -\mathbf{e}_{4,t,i}+ \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i}  
    \end{align}
    where $\mathbf{e}_{1,t,i}\coloneqq \alpha \del_t \mathbf{w}_t\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{v}_{t,i}$, $\mathbf{e}_{2,t,i}\coloneqq \alpha (\mathbf{B}_t^\top \mathbf{v}_{t,i}\mathbf{w}_t^\top\del_t + \del_t\mathbf{w}_t \mathbf{v}_{t,i}^\top \mathbf{B}_t) \mathbf{w}_t$, $\mathbf{e}_{3,t,i}\coloneqq 2\alpha (\mathbf{w}_{\ast,i}^\top \mathbf{B}_{\ast}^\top \mathbf{v}_{t,i})\del_t \mathbf{w}_{t}$, $\mathbf{e}_{4,t,i}\coloneqq \alpha^2 \mathbf{B}_t^\top( \mathbf{v}_{t,i} \mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top  +  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{v}_{t,i}^\top)\mathbf{B}_t\mathbf{w}_t  $ for all $t,i$. These terms are not helpful for bounding $\|\mathbf{w}_{t+1}\|_2$ so we treat them as error terms. 
    % $\|\del_{t+1}\|_2$ and $\dist_{t+1}$, as we will see shortly.
    
% { if we make $\alpha$ small enough, the dominant terms in $\mathbf{v}_{t,i}$ become $\deld_t \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$ and the dominant terms in the gradient become:
% \begin{align}
%   & \del_t \mathbf{B}_t^\top \mathbf{v}_{t,i} - \alpha^2 \mathbf{B}_t^\top (\mathbf{v}_{t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top + \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{v}_{t,i}^\top )\mathbf{B}_t \mathbf{w}_t + \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i} \nonumber \\
%     &\approx \del_t \mathbf{B}_t^\top \mathbf{v}_{t,i}  + \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i} \nonumber \\
%     &\approx \del_t^2 \mathbf{B}_t^\top\mathbf{B}_t\mathbf{w}_t - \del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i} - \alpha^2  \del_t \mathbf{B}_t^\top \mathbf{B}_t\mathbf{w}_t\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} + \alpha^2  \del_t \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t\mathbf{w}_t \nonumber \\
%     &\quad + \alpha^2 \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t \del_t \mathbf{w}_t - \alpha^2  \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \deld_t \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \nonumber \\
%     &\quad -  \alpha^4 \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{w}_t\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} + \alpha^4 \mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t\mathbf{w}_t 
% \end{align}}
%     (empirically, middle term is not necessary either)
    
    



The helpful terms in $ \nabla_\mathbf{w}F_{t,i}(\mathbf{B}_{t}, \mathbf{w}_{t})$ are those composed of $\mathbf{w}_t$ multiplied on the left by a positive (semi-)definite matrix. Let the sum of these terms, averaged over all $i$, be written as $\mathbf{H}\mathbf{w}_t$ for $\mathbf{H}\succeq\mathbf{0}$, and let $\mathbf{n}= \frac{1}{n}\sum_{i=1}^n\nabla_\mathbf{w}F_{t,i}(\mathbf{B}_{t}, \mathbf{w}_{t})-\mathbf{H}\mathbf{w}_t$. Then, we can see that since
 $\mathbf{w}_{t+1}= \mathbf{w}_t -  \frac{\beta}{n}\sum_{i=1}^n\nabla_\mathbf{w}F_{t,i}(\mathbf{B}_{t}, \mathbf{w}_{t}) = (\mathbf{I} - \beta \mathbf{H})\mathbf{w}_{t} + \beta \mathbf{n}$, and $\|\mathbf{I}_k - \beta \mathbf{H}\|_2 \leq 1$ for small enough $\beta$, the helpful terms do not expand the energy of $\mathbf{w}_t$, and may contract it if they are positive definite. 
 
 The helpful terms can be extracted from $\del_t  \mathbf{B}_t^\top \mathbf{v}_{t,i}$ and $  \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i} $ by expanding $\mathbf{v}_{t,i}$.
 In particular, we can write
 \begin{align}
     \del_t  \mathbf{B}_t^\top \mathbf{v}_{t,i} &= \del_t  \mathbf{B}_t^\top  \deld_t\mathbf{B}_t \mathbf{w}_t + 
    \del_t  \mathbf{B}_t^\top  \left( \mathbf{v}_{t,i} - \deld_t \mathbf{B}_t \mathbf{w}_t  \right) \nonumber \\
    &= \underbrace{\del_t  \mathbf{B}_t^\top  \mathbf{B}_t \del_t \mathbf{w}_t}_{\text{helpful}} + 
    \underbrace{\del_t  \mathbf{B}_t^\top  \left( \mathbf{v}_{t,i} - \deld_t \mathbf{B}_t \mathbf{w}_t  \right)}_{\text{not helpful}} \label{helpful1} \\
     \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i}  &=   \alpha^4 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{w}_t  \nonumber \\
     &\quad +   \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top(\mathbf{v}_{t,i} - \alpha^2 \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{w}_t) \nonumber\\
     &=  \underbrace{ \alpha^4\|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}   \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{w}_t}_{\text{helpful}}  \nonumber \\
     &\quad + \underbrace{  \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top(\mathbf{v}_{t,i} - \alpha^2 \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{w}_t)}_{\text{not helpful}} \label{helpful2}
 \end{align}
Note that the coefficient matrix of $\mathbf{w}_t$ in the helpful term in \eqref{helpful1} is only positive semi-definite, not positive definite, even after averaging over $i$, because $\del_t$ may be rank deficient.
 However, we can lower bound the minimum singular value of the coefficient matrix of $\mathbf{w}_t$ in the helpful term in \eqref{helpful2} after averaging over all $i\in[n]$:
 \begin{align}
     \sigma_{\min}\left(\frac{\alpha^4}{n}\sum_{i=1}^n\|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}   \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \right) &\geq \alpha^4 \sigma_{\min}^2(\mathbf{B}_\ast^\top \mathbf{B}_t) \sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n\|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{\ast,t,i}   \mathbf{w}_{\ast,t,i}^\top \right)\nonumber \\
     &\geq \alpha^4 \frac{E_0(1-\tau_2)}{\alpha}\tilde{\mu}_{\ast}^2 \nonumber \\
     &\geq c \alpha^3 E_0 \tilde{\mu}_\ast^2
 \end{align}
 where $\tilde{\mu}_\ast^2 \coloneqq \sigma_{\min}\left(\frac{1}{n}\sum_{i=1}^n\|\mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{\ast,t,i}   \mathbf{w}_{\ast,t,i}^\top \right)$.
 Next we upper bound the norms of the non-helpful terms :
\begin{align}
    \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{1,t,i}\right\|_2 \leq c\sqrt{\alpha} \tau_2 \tau_1 v_a, \quad 
    \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{2,t,i}\right\|_2 &\leq c\sqrt{\alpha} \tau_1 \tau_2 v_a ,\nonumber \\ 
    \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{3,t,i}\right\|_2 \leq   \alpha \tau_2\sqrt{\tau_1} \tilde{v}_a,\quad
    % (\eta_\ast \tau_2 \sqrt{\tau_1}\tfrac{1}{\sqrt{\alpha}} + (\tau_2 + \dist_t)L_{\max}^2 +\sqrt{\alpha} \tau_{1}^{3/2}\tau_2 + L_{\max}^2 \tau_1 \tau_2 +\alpha \tau_1 L_{\ast}^2 + \alpha^{3/2} \sqrt{\tau_1}L_{\max}^3)  
    \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{4,t,i}\right\|_2 &\leq \alpha \sqrt{\tau_1}\tilde{v}_a \nonumber \\
    \left\|\frac{1}{n}\sum_{i=1}^n\del_t  \mathbf{B}_t^\top  \left( \mathbf{v}_{t,i} - \deld_t \mathbf{B}_t \mathbf{w}_t  \right) \right\|_2 &\leq  { \tau_2\frac{1}{\sqrt{\alpha}}\left( \tau_2\eta_\ast+\alpha \tau_1\eta_\ast + \alpha^{3/2}\sqrt{\tau_1}L_\ast^2\right)} \nonumber \\
     \left\|\frac{1}{n}\sum_{i=1}^n\alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top(\mathbf{v}_{t,i} - \alpha^2 \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t\mathbf{w}_t)\right\|_2 &\leq  \alpha^{3/2}\big( \tau_2 \sqrt{\tau_1}\frac{1}{\sqrt{\alpha}}L_\ast^2 +
     (\tau_2+\dist_t)L_{\max}^3\nonumber \\
     &\quad \quad\quad \quad +\alpha \tau_1 L_{\max}^3 + \alpha^{3/2}\sqrt{\tau_1}\tilde{L}_\ast^2\big)  \nonumber 
\end{align}
where $\tilde{v}_a = (\eta_\ast \tau_2 \sqrt{\tau_1}\tfrac{1}{\sqrt{\alpha}} + (\tau_2+{\color{red}\dist_t})L_{\max}^2 +\sqrt{\alpha} \tau_{1}^{3/2}\tau_2 + L_{\max}^2 \tau_1 \tau_2 +\alpha \tau_1 L_{\ast}^2 + \alpha^{3/2}
\sqrt{\tau_1}L_{\max}^3)$. Note that
$\dist_t$ is present for $\mathbf{e}_3$ but not $\mathbf{e}_4$.
This allows us to write
% \begin{align}
%     \del_t  \mathbf{B}_t^\top \mathbf{v}_{t,i} &\rightarrow \mathbf{B}_t^\top \del_t^2 \mathbf{B}_t \mathbf{w}_t \nonumber \\
%     \alpha \del_t \mathbf{w}_t\mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{v}_{t,i} &\rightarrow\text{none}\nonumber \\
%     \alpha (\mathbf{B}_t^\top \mathbf{v}_{t,i}\mathbf{w}_t^\top\del_t + \del_t\mathbf{w}_t \mathbf{v}_{t,i}^\top \mathbf{B}_t) \mathbf{w}_t&\rightarrow \text{none}\nonumber \\
%     2\alpha (\mathbf{w}_{\ast,i}^\top \mathbf{B}_{\ast}^\top \mathbf{v}_{t,i})\del_t \mathbf{w}_{t}&\rightarrow \text{none} \nonumber \\
%     \alpha^2 \mathbf{B}_t^\top( \mathbf{v}_{t,i} \mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top  +  \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} \mathbf{v}_{t,i}^\top)\mathbf{B}_t\mathbf{w}_t &\rightarrow \text{none} \nonumber \\
%   \alpha^2 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top\mathbf{v}_{t,i}  &\rightarrow  \alpha^4 \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t\mathbf{w}_t
% \end{align}
% Expanding the $\lam_t$'s, we get 
\begin{align}
    \|\mathbf{w}_{t+1}\|_2&= \left\|\mathbf{w}_t - \frac{\beta}{n}\sum_{i=1}^n\nabla_\mathbf{w}F_{t,i}(\mathbf{B}_{t}, \mathbf{w}_{t})\right\|_2 \nonumber \\
    &\leq \left\|\left(\mathbf{I}_k -  \beta \mathbf{B}_t^\top \del_t^2 \mathbf{B}_t - \beta\alpha^4\frac{1}{n}\sum_{i=1}^n \mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t \right)\mathbf{w}_t \right\|_2 \nonumber \\
    &\quad + \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{1,t,i}\right\|_2  + \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{2,t,i}\right\|_2 + \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{3,t,i}\right\|_2 +\left\|\frac{1}{n}\sum_{i=1}^n\mathbf{e}_{4,t,i}\right\|_2  \nonumber \\
    &\quad + \left\|\frac{1}{n}\sum_{i=1}^n \del_t\mathbf{B}_t^\top (\mathbf{v}_{t,i} - \deld_t\mathbf{B}_t \mathbf{w}_t) \right\|_2 + \alpha^4 \left\|\frac{1}{n}\sum_{i=1}^n\mathbf{B}_t^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top (\mathbf{v}_{t,i} - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t\mathbf{w}_t) \right\|_2 \nonumber \\
    &\leq (1 - \beta \alpha^3 E_0 \tilde{\mu}_{\ast}^2)\sqrt{\tau_1} + \sqrt{\alpha} \tau_2 \tau_1 v_a + 2\sqrt{\alpha} \tau_1 \tau_2 v_a \nonumber \\
    &\quad + (2\alpha \tau_2\sqrt{\tau_1}+2 \alpha \sqrt{\tau_1})(\eta_\ast \tau_2 \sqrt{\tau_1}\tfrac{1}{\sqrt{\alpha}} + (\tau_2 + \dist_t)L_{\max}^2 +\sqrt{\alpha} \tau_{1}^{3/2}\tau_2 + L_{\max}^2 \tau_1 \tau_2 +\alpha \tau_1 L_{\ast}^2 + \alpha^{3/2} \sqrt{\tau_1}L_{\max}^3) \nonumber\\
    &\quad + \tau_2\frac{1}{\sqrt{\alpha}}\left( (\tau_2+\dist_t)\eta_\ast+\alpha \tau_1\eta_\ast + \alpha^{3/2}\sqrt{\tau_1}L_\ast^2\right) \nonumber \\
    &\quad + \alpha^{7/2}( \tau_2 \sqrt{\tau_1}\frac{1}{\sqrt{\alpha}}L_\ast^2 + (\tau_2+\dist_t)L_{\max}^3 +\alpha \tau_1 L_{\max}^3 + \alpha^{3/2}\sqrt{\tau_1}\tilde{L}_\ast^2)  \nonumber \\
    % &\leq  (1 - \beta \alpha^3 E_0 \tilde{\mu}_{\ast}^2)\sqrt{\tau_1} + \tau_2^2 \tau_1^{3/2}\nonumber \\
    % &\quad + 2 \alpha \sqrt{\tau_1}((\tau_2 + \dist_t)L_{\max}^2 +\sqrt{\alpha} \tau_{1}^{3/2}\tau_2 + \alpha \tau_1 L_{\ast}^2 + \alpha^{3/2} \sqrt{\tau_1}L_{\max}^3) \nonumber\\
    % &\quad + \tau_2\frac{1}{\sqrt{\alpha}}\left( (\tau_2+\dist_t)\eta_\ast+ \alpha^{3/2}\sqrt{\tau_1}L_\ast^2\right) \nonumber \\
    % &\quad + \alpha^{7/2}( (\tau_2+\dist_t)L_{\max}^3 + \alpha^{3/2}\sqrt{\tau_1}\tilde{L}_\ast^2)  \nonumber \\
%     &=  (1 - \beta \alpha^3 E_0 \tilde{\mu}_{\ast}^2)\sqrt{\tau_1} + \tau_2^2 \tau_1^{3/2} + \alpha \sqrt{\tau_1}\tau_2 L_{\max}^2 + \alpha^{3/2}\tau_1^2 \tau_2 + \alpha^2 \tau_1^{3/2}L_\ast^2 +\alpha^{5/2}\tau_1 L_{\max}^3\nonumber \\
%     % &\quad + 2 \alpha \sqrt{\tau_1}((\tau_2 + \dist_t)L_{\max}^2 +\sqrt{\alpha} \tau_{1}^{3/2}\tau_2 + \alpha \tau_1 L_{\ast}^2 + \alpha^{3/2} \sqrt{\tau_1}L_{\max}^3) \nonumber\\
%     &\quad +\tau_2^2 \frac{1}{\sqrt{\alpha}}\eta_\ast  + \alpha \tau_2 \sqrt{\tau_1}L_\ast^2 + \alpha^{7/2}\tau_2 L_{\max}^3 + \alpha^5\sqrt{\tau_1}\tilde{L}_\ast^2 \nonumber \\
%     % &\quad + \tau_2\frac{1}{\sqrt{\alpha}}\left( (\tau_2+\dist_t)\eta_\ast+ \alpha^{3/2}\sqrt{\tau_1}L_\ast^2\right) \nonumber \\
%     % &\quad + \alpha^{7/2}( (\tau_2+\dist_t)L_{\max}^3 + \alpha^{3/2}\sqrt{\tau_1}\tilde{L}_\ast^2) ...
%   &\quad + \tau_2 \frac{1}{\sqrt{\alpha}} \dist_t \eta_\ast +  \alpha^{7/2}\dist_t L_{\max}^3  + \alpha\sqrt{\tau_1}\dist_t L_{\max}^2 \nonumber\\
   &\leq \left(1 - \beta \alpha^3 E_0 \tilde{\mu}_{\ast}^2 + \tau_2^2 \tau_1 + \alpha \tau_2 L_{\max}^2 + \alpha^{3/2}\tau_1^{3/2}\tau_2 + \alpha^2 \tau_1 L_\ast^2+\alpha^{5/2}\sqrt{\tau_1} L_{\max}^3  +  \alpha^5\tilde{L}_\ast^2 +  +\alpha L_{\max}^2 \dist_t \right)\sqrt{\tau_1}   \nonumber \\
    &\quad +\tau_2^2 \frac{1}{\sqrt{\alpha}}\eta_\ast  + \alpha^{7/2}\tau_2 L_{\max}^3 + \left(\tau_2 \frac{1}{\sqrt{\alpha}}\eta_\ast +   \alpha^{7/2}L_{\max}^3 \right)\dist_t \nonumber \\
    &\leq 
\end{align}
where we have subsumed dominated terms. Now, we can execute a similar proof as for FO-ANIL. Note that 
$\tau_{2,r}\leq $




% from experiments: sqrt(tau1) - 3; 4, 6

% when alpha is smaller,

% empirically: 

% does eta matter? smaller eta helps convergence rate but large eta still converges.
% what happens when alpha is really small.

% convergence rate is highly dependent on alpha.

% left off: w might be scaling with rt(alpha). Not clear from experiments, even when heads are standard basis vectors. if it's scaling with rt(alpha), we need to figure out why its working



% The dominant terms are:
% \begin{align}
    
% \end{align}


\begin{lemma}
New bound on $\|\mathbf{w}_{t+1}\|$
\end{lemma}
\begin{proof}



\begin{align}
    \nabla_{\mathbf{w}} F_{i}(\mathbf{B}_t,\mathbf{w}_t)&= \tilde{\nabla}_{\mathbf{w}}F_{i}(\mathbf{B}_t,\mathbf{w}_t) + \alpha \del_t \mathbf{w}_t\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{v}_{t,i} + \alpha \del_t \mathbf{w}_t \mathbf{v}_{t,i}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} + \alpha\mathbf{B}_t^\top \deld_t \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top \del_t \mathbf{w}_t \nonumber \\
    &\quad + \alpha^3 \mathbf{B}_t^\top \mathbf{A}_i \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_t^\top\del_t\mathbf{w}_t - \alpha^2 \mathbf{B}_t^\top \mathbf{v}_{t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \mathbf{w}_t - \alpha^2 \mathbf{B}_t^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i} \mathbf{v}_{t,i}^\top \mathbf{B}_t \mathbf{w}_t \nonumber \\
    &\quad - \alpha^2\mathbf{B}_t^\top \deld_t \mathbf{B}_t\mathbf{w}_t \mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i} - \alpha^4 \mathbf{B}_t^\top \mathbf{A}_i \mathbf{B}_t\mathbf{w}_t \mathbf{w}_t^\top \mathbf{B}_t^\top \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}
\end{align}
Problem: all other terms are $O(\alpha^{3.5})$, besides  the two terms with $\mathbf{w}_t^\top\del_t \mathbf{w}_t$ which are $O(\alpha^{5.5})$. So we must deal with the rest of the terms.
\end{proof}







notes -- i think these were for exact maml


\begin{align}
    \|\mathbf{w}_{t+1}\|_2 &\leq \|\mathbf{w}_{t}\|_2 + \frac{\beta}{\sqrt{\alpha}} \tau_{t,2}^2  \eta_{\ast} \nonumber \\
    &\leq \frac{\beta}{\sqrt{\alpha}}  \sum_{s=1}^t  \tau_{s,2}^2 \nonumber \\
    &\leq \frac{\beta}{\sqrt{\alpha}}  \sum_{s=1}^t \left( \rho^2 \tau_{s-1,2}^2 + \beta^4 \alpha^4 \dist_{s-1}^4 + \beta^2 \alpha^{5}\|\mathbf{w}_{s-1}\|_2 \right) \nonumber \\
    &\leq \frac{\beta}{\sqrt{\alpha}}  \sum_{s=1}^t \left( \rho^2 \tau_{s-1,2}^2 + \beta^4 \alpha^4 \dist_{s-1}^4 + \beta^3 \alpha^{9/2}\sum_{r=1}^{s-1} \tau_{r,2}^2 \right) \nonumber \\
    &\leq \frac{\beta}{\sqrt{\alpha}}  \sum_{s=1}^t \left( (\rho^2 + (t-s)\beta^3 \alpha^{9/2}) \tau_{s-1,2}^2 + \beta^4 \alpha^4 \dist_{s-1}^4 \right) \nonumber \\
    &\leq \frac{\beta}{\sqrt{\alpha}}  \sum_{s=1}^t \Big( (\rho^2 + (t-s)\beta^3 \alpha^{9/2})((\rho^2 + (\rho^2 + (t-s)\beta^3 \alpha^{9/2})(t-s-1)\beta^3 \alpha^{9/2})) \tau_{s-2,2}^2 \nonumber \\
    &\quad + (\rho^2 + (t-s)\beta^3 \alpha^{9/2}) \tau_{s-1,2}^2\beta^4 \alpha^4 \dist_{s-2}^4  + \beta^4 \alpha^4 \dist_{s-1}^4 \Big) \nonumber \\
    &\leq \sum_{s=1}^t \sum_{r=1}^s \left(\prod_{j=s-r}^s(\rho^2 + ) \right) \dist_r^4
\end{align}

$a_t \leq \frac{\beta}{\sqrt{\alpha}}\sum_{s=1}^{t-1} \tau_s^2$

$\tau_s \leq \rho \tau_{s-1} + {\beta^2}{\alpha^2}\dist_{s-1}^2 +\beta \alpha^{5/2}a_{s-1}$

to show $\tau_s$ is decreasing until $a_s$:use $a_s \leq \tau_s$

but once we have this, how does it help? if we know $\tau_s \leq a_s$, then we have $a_{s+1}\leq a_s+\beta/\sqrt{\alpha} a_s^2$, which doesn't help.

$\tau_s \leq \sum_{r=1}^{s-1} \rho^{s-1-r}({\beta^2}{\alpha^2}\gamma^{2r} +\beta \alpha^{5/2}a_{r})$ 

$\tau_s^2 \leq 3\rho^2 \tau_{s-1}^2 + 3{\beta^4}{\alpha^4}\dist_{s-1}^4 +3\beta^2 \alpha^{5}a_{s-1}^2$

$--> $ from experiments, the direction  doesn't matter... 

Assume that $\|\mathbf{w}_s\|_2 \leq \alpha^{3/2}$ for all $s \leq t$ (loose bound). Then we have
\begin{align}
    \|\mathbf{w}_{t+1}\|_2 &\leq  \frac{\beta}{\sqrt{\alpha}}\sum_{s=1}^t \rho^2 \tau_{s-1,2}^2 +\beta^4\alpha^4\dist_{s-1}^4 + \beta^2 \alpha^{6.5} \nonumber \\
    &\leq t \beta^3 \alpha^6 + c_1 \beta^5 \alpha^{3.5} + 
\end{align}
or just
\begin{align}
    a_{t+1}\leq \alpha +\epsilon (t-1) + c\frac{\beta}{\sqrt{\alpha}}\tau_{2}^2
\end{align}
but this might be too loose because we have uniform tau bound. can we show tau is decreasing?
\begin{align}
    a_{t+1}\leq \alpha^{1.5} + c {\beta}\alpha^{3.5}t
\end{align}
need $c {\beta}\alpha^{3.5}t \leq \alpha^{1.5} \iff t \leq c'/(\beta \alpha^{2}) $

% need to use the above arithmetic argument, but somehow use that 
% $(1 - \beta \alpha)^{1/(\beta\alpha^2)}$
